Fast Rates for Noisy Interpolation Require Rethinking the Effects of Inductive Bias

Good generalization performance on high-dimensional data crucially hinges on a simple structure of the ground truth and a corresponding strong inductive bias of the estimator. Even though this intuition is valid for regularized models, in this paper we caution against a strong inductive bias for interpolation in the presence of noise: While a stronger inductive bias encourages a simpler structure that is more aligned with the ground truth, it also increases the detrimental effect of noise. Specifically, for both linear regression and classification with a sparse ground truth, we prove that minimum $\ell_p$-norm and maximum $\ell_p$-margin interpolators achieve fast polynomial rates close to order $1/n$ for $p > 1$ compared to a logarithmic rate for $p = 1$. Finally, we provide preliminary experimental evidence that this trade-off may also play a crucial role in understanding non-linear interpolating models used in practice.

==> ICML 22-3/sections/discussion.tex <==



 \begin{figure*}
    \centering
\begin{subfigure}[b]{0.32\linewidth}
         \centering
         \includegraphics[width=\textwidth]{figures/synthetic_regression_bias_variance.pdf}
         \caption{ New bias-variance trade-off}
         \label{fig:synthetic_regression_bias_variance}
     \end{subfigure}
     \begin{subfigure}[b]{0.32\linewidth}
         \centering
   \includegraphics[width=\textwidth]{figures/synthetic_lp_svm_p_vs_risk_multiple_lines.pdf}
         \caption{Simulations Classification}
         \label{fig:synthetic classification subplot}
     \end{subfigure}
\begin{subfigure}[b]{0.32\linewidth}
         \centering
         \includegraphics[width=\textwidth]{figures/leukemia_lp_svm_p_vs_risk.pdf}
         \caption{Leukemia classification dataset}
         \label{fig:leukemia classification subplot}
     \end{subfigure} 
         \caption{
         \textbf{(a)} The averaged estimation error (risk) as well as the estimated bias and variance of the min-$\ell_p$-norm interpolator \eqref{eq:minlpnomrinterpol} as a function of $p$. We run 50 independent simulations with data drawn from the distribution in Section~\ref{subsec:regsetting} and choose $n= 100,d=5000$, $\sigma =1$ (noisy) and $\sigma = 0$ (noiseless).
         %The bias and variance are estimated from 50 simulation rounds.
         \textbf{(b)} Average and individual classification error for the max-$\ell_p$-margin interpolator \eqref{eq:svm problem} with $n=100$, $d=5000$ over 50 independent runs. 
         %data generated with a 1-sparse ground truth $w^{\star}$ and $y=\sign(\langle x, w^{\star}\rangle) \xi$ and fixed fraction $\sigma\%$ of label noise. %\fy{i feel like need to at least briefly mention in text what that has to do with our noise model for precision}
         %, with $\mathbb{P}(\xi=-1)=\sigma, \mathbb{P}(\xi=+1)=1-\sigma$. 
         \textbf{(c)}
         Mean and variance of the classification error for the max-$\ell_p$-margin interpolator \eqref{eq:svm problem}
          on the Leukemia data set with $d=7070$ and $72$ data points in total. See Section~\ref{sec:discussion} for further details.}
    \label{fig:classification svm}
\end{figure*}


\section{Numerical Simulations and Interpretation of the Results}
\label{sec:discussion}

%We recall that $p$ stands for the strength of the inductive bias towards sparse solutions, which increases for $p\to 1$. 
%In this section, we provide experiments that show the superiority of interpolators with moderate inductive bias, i.e., $p \in (1,2)$, compared to strong ($p=1$) and no inductive bias ($p=2$). While this is predicted by Theorem~\ref{thm:regressionlpmain} for large $d,n$, we present empirical evidence that the phenomenon holds for finite (and moderate) $d,n$ as well.
We now present empirical evidence for our theory\footnote{We release the code for the replication of the experiments at \url{https://github.com/nickruggeri/fast-rates-for-noisy-interpolation}}, 
which predicts the superiority of min-$\ell_p$-norm/max-$\ell_p$-margin interpolators with moderate inductive bias $p\in(1,2)$ compared to $p=1,2$.
Further, we discuss how varying the strength of the inductive bias induces a trade-off between 
structural simplicity aligning with the ground truth and noise resilience in high dimensions.
%that arises in the upper bounds in Theorems~\ref{thm:regressionlpmain} and \ref{thm:classificationlp}. \fy{somehow sounds fishy to talk about upper bounds and tradeoff}
%\emph{the structural alignment with ground truth} and the \emph{regularizing effect due to high-dimensionality} that arises in the upper bounds in Theorems~\ref{thm:regressionlpmain} and \ref{thm:classificationlp}. 
Finally, we show experimentally that this trade-off can also be intuitively  understood as a "new" bias-variance trade-off induced by varying the inductive bias.


\vspace{-1mm}
\paragraph{Simulations for regression and classification}
While Theorems~\ref{thm:regressionlpmain} and \ref{thm:classificationlp} hold for "large enough" $d, n$, we now illustrate experimentally in Figure~\ref{fig:synthetic_regression_bias_variance} and \ref{fig:synthetic classification subplot} that the superiority of the choice $p\in(1,2)$ over $p=1$ and $p=2$ also holds for finite $d,n$ of practically relevant orders:
For $d=5000,n=100$, the min-$\ell_p$-norm/max-$\ell_p$-margin interpolators with $p\in(1,2)$ achieve lowest (directional) estimation error in the noisy case ($\sigma >0$), while $p=1$ is optimal in the noiseless case ($\sigma = 0$).
Both experiments are run on a synthetic dataset with a 1-sparse ground truth $\wstar$, as described in Section~\ref{subsec:regsetting} (regression) and Section~\ref{subsec:clasetting} (classification). For the regression experiment, we plot the average risks over 50 runs for $\sigma =1$ (noisy) and $\sigma = 0$ (noiseless) and the bias and variance in the noisy case. 
For the classification experiment, we randomly flip a fixed amount of $\sigma\%$ of the labels.
 We plot the error of individual random draws and their mean over 50 independent runs.

Furthermore, we examine the performance of the max-$\ell_p$-margin classifier on the Leukemia classification dataset \cite{leukemiapaper} with $d=7070$.
In line with our theory, Figure~\ref{fig:classification svm} shows
that the value of $p$ which minimizes the (directional) estimation error shifts from $p=1$, in the noiseless case,  to $p\in(1,2)$ in the presence random label flips in the data. Noiseless, i.e. $\sigma=0$, here means that we are not adding artificial label noise.   We plot the  averaged error and its variance over $100$ random train-test splits with training set size $n=65$. 
Finally, note that in practical applications with noisy data, we do not advocate  the use of interpolators but recommend using regularized estimators instead. 

\vspace{-1mm}
\paragraph{The strength of the inductive bias induces a new bias-variance trade-off.}
Why the optimal choice of $p$ does not  correspond to the strongest inductive bias ($p=1)$  can be explained by a
trade-off between two competing factors:
the regularizing effect of high-dimensionality and the effective sparsity of the solutions, matching the simple structure of the ground truth. In particular, with increasing inductive bias (decreasing $p\to 1$), noise resilience due to high dimensions decreases while the interpolator becomes effectively sparser and hence achieves better performance on noiseless data. This trade-off is also reflected  in Theorems~\ref{thm:regressionlpmain} and \ref{thm:classificationlp}: The terms of order $\frac{\sigma^2 n  \exp(\kappa_4 q)}{qd}$ 
capture the noise resilience due to high-dimensionality, or rather vulnerability, and monotonically decrease with $d$ but increase as $p\to 1$.
On the other hand, the terms of order $\frac{ q^p\sigma^{4-2p}d^{2p-2}}{n^p}$ and $\frac{q^{\frac{3}{2}p}d^{3p-3} \log^{3/2}d }{n^{\frac{3}{2}p}}$
capture the benefits of
the structural alignment with the sparse ground truth as they decrease with $p\to1$. 


We now give a more intuitive reasoning for this trade-off,  which may also translate to more general models. Clearly, to recover noiseless signals in high dimensions, the space of possible solutions must be restricted by using an inductive
bias that encourages the structure of the interpolator to match that of the ground truth.
For instance, the solution of the min-$\ell_1$-norm interpolator is always $n$-sparse despite having $d$ parameters. 
However, exactly  this restriction  towards a certain structure (such as sparsity)  becomes harmful
when fitting noisy labels: Instead of low $\ell_2$-norm 
solutions that can distribute noise across all dimensions, 
the interpolator is forced to find $n$-sparse 
solutions with a higher $\ell_2$-norm.






%\fy{maybe related work if at all}
%Finally, we would like to note that this intuition also allows the two-stage interpolator  \cite{muthukumar_2020} (not a min-norm interpolator) to achieve minimax optimal risk. It essentially profits from the best of both worlds by having both a strong inductive bias towards sparse solutions in the first stage  and benefit significantly from a strong regularizing effect due to high-dimensionality when fitting the residual in the second step. 

% In fact, this term follows the same trend as reguarlized e when changing $d$ and $p$ for fixed $n$ it
% As also discussed below Theorem~\ref{thm:regressionlpmain}, we motivate future work to investigate whether $\ell_p$-regularized estimators/classifiers attain the same rate as this term, which would give interesting insights on when regularization can be avoided and when it is necessary to achieve optimal performance for $\ell_p$-norm structured models. 
% term of order   does not explicitly depend on the noise $\sigma$. Unlike the first term, this term decreases when $p \to 1$ and increases with $d$ and therefore follows exactly the same trend as the noiseless risk in Proposition~\ref{prop:noiseless}. Therefore, we argue that this term can be understood as the \emph{penalty due to an insufficient of structural bias} towards sparse solutions.
%\red{for this i would like to see an experiment} Importantly, and differently form regularized models, the optimum is therefore attained when the structural bias is balanced to compensate the effects of noise. \\
%\kd{rewrite:}
% In addition to the risk, Figure~\ref{fig:synthetic regression} shows the estimated bias and variance terms. We can clearly see that the optimal $p$ can also be explained as a trade-off of these two terms.  We further discuss this relation in Section~\ref{sec:trade-off}.
% illustrate the risk for both classification and regression a a synthetic data set. As expected, we can see that both times  the optimal $p\in(1,2)$. \kd{describe synthetic setting briefely here}. 

In Figure~\ref{fig:synthetic_regression_bias_variance}, we demonstrate how
the trade-off 
can also be viewed as a novel kind of bias-variance trade-off for interpolating models. 
In the classical bias-variance trade-off, increasing  model complexity (e.g., by decreasing the regularization penalty) leads to larger variance but smaller (statistical) bias. For interpolating models, we observe a similar trade-off when varying the strength of the inductive.  Figure~\ref{fig:synthetic_regression_bias_variance} depicts this trade-off and shows that the optimal (directional) estimation error is attained at the $p$ where both terms are approximately the same. 





% the complexity of the model does not change. Yet, we still see in Figure~\ref{fig:synthetic_regression_bias_variance} that the bias decreases with $p\to1$ and the variance increases. 




% are always capable of interpolating any $n$-points when $d>n$. 


% are al does not reduce the capacity of the min-$\ell_p$-norm interpolators are always 


% While for regularized models, the BV tradeoff arises 
% by varying model complexity via the penalty $\lambda$ that trades off smaller approximation error with a higher ability to fit noise, in interpolation there is no model complexity knob $\lambda$ - instead we may look at BV as the strenghts of inductive bias varies, that is biases towards structures of varying simplicity.  In our experiment with linear models, again as $p \to 1$, the strength of the indudctive bias increases.


%induced by varying the strength of inductive bias (as opposed to model complexity for regularized models).
%As suggested by our simulation in Figure~\ref{fig:synthetic regression}, illustrating the estimated bias and variance of the interpolator, this is indeed the case. Clearly, the bias term monotonically decreases with the strength of the inductive bias and the variance increases. In particular, we see that the optimal risk is attained where both terms are approximately the same. We leave a formalization of this observation as future work.



%theoretical work on how the bias-variance captures this phenomenon and appears in the upper bound in Theorem~\ref{thm:regressionlpmain} as a future work.

% We now wonder how the trade-off between 
% As suggested by our simulation in Figure~\ref{fig:synthetic regression}, the trade-off can also be understood as some sort of bias /variance trade-off for interpolating models. However, we are not aware of any approximation for the bias and variance terms when $p \neq 2$ and leave a theoretical investigation on how the expressions relate to the terms appearing in the upper bound in Theorem~\ref{thm:regressionlp} as a future work. More generally, we motivate future work to explore formal definitions for terms capturing the structural bias and terms capturing the regularizing effect of overparametrization and to show how they appear in the non-asymptotic bounds in Theorem~\ref{thm:regressionlp},\ref{thm:classificationlp}. 







% In fact, as can be seen from the analysis in \cite{wang2021tight} and the proof of Theorem~\ref{thm:regressionlpmain}, for $p=1 $ this term corresponds to the term $\frac{\sigma^2}{\log(d/n)}$ and therefore is responsible for the rate of the min-$\ell_1$-norm interpolator compared to its regularized variant the LASSO. 




% On the other had, the first term is of order $\frac{\sigma^{4-2p} d^{2p-2}}{n^p}$ and follows exactly the expected trend for regularized estimators; the term monotonically increases with $d$ for fixed $n$ and monotonically decreases  with  $p\to 1$ (neglecting the term $\sigma^{4-2p}$) (increasing $\alpha$ with $\beta$ in Figure~\ref{fig:rates_reg}).   We therefore argue that this risk reflects the \emph{strength of the structural bias of the estimator} towards sparse solutions.








% I suggest the following structure here: Scope ( at most 3/4 of a page!)
% \begin{itemize}
%     \item Regression lp - Indeed, we can see that the optimal p is in (1,2). We wonder whether this trade-off is also captured by the bias and variance terms =... . Indeed, as we can see, one term goes down and one goes up. We discuss the relation between the bias variance trade-off and Thm 1 in the future work section (because currently it is not well understood). 
%     \item We also observe this trade-off for classification with lp-svm on synthetic data. 
%     \item While real world regression data sets are usually inherently noisy and thus regularized estimators are a nat ural choice, classification data sets used in real world examples can sometimes also be considered as noiselss (when being labeled by some human representing the  ground truth). Thus, the use of hard margin support vector machine relevant in practice ( cite here). Figure bla the performance with respect to $p$. We observe that in the noiseless case $p=1$ performs indeed the best. However, in the presence of random label flips, we observe that the expected trade-off occurs. \red{i feel like this real world motivation is quite weak...}
% \end{itemize}




% We saw from the results in the previous two sections that $p\in(1,2)$ achieves faster rates compared to $p=1,2$. In this section we present numerical simulations addressing the following two question: is the optimal $p$ also attained in $(1,2)$ for finite $n,d$ of practically relevant order? Furthermore, can this phenomenon be related to a bias-variance trade-off in regression?


% Yet, it is unclear whether a trade-off between $p=1$ and $2$ also occurs for finite $n,d$ of practically relevant orders. In this Section, we study the performance of interpolating for different values of $p$ in practical scenarios and observe a correspondence with the trend predicted by the theoretical results.
% \kd{in practical scenarios but not on real world data? rephrase}


% % one might wonder whether the optimal $p$ is also attained in $(1,2)$ for real world data set. This is indeed the case as we can see in Figure~\ref{fig:classification svm} which illustrates the performance of the max-$\ell_p$-margin interpolator, or also called \emph{hard-margin $\ell_p$-support vector machine}, on the Leukemia data set \cite{leukemiapaper}. 







% % \kd{WIP}
% % Real world regression tasks are in general considered to be noisy, thus in such scenarios regularized estimators are a natural choice. Oppositely, classification data sets can sometimes be considered noiseless. In such cases, classification with hard-margin support vector machines is a practically relevant case \cite{noble2004support, brown1999support, guyon2002gene, furey2000support, cervantes2020comprehensive} \red{check if these are enough, the last is a survey and we can find many more there}. Figure~\ref{fig:classification svm} shows the performance of the max-$\ell_p$-margin interpolator, or also called \emph{hard-margin $\ell_p$-support vector machine}, on the Leukemia data set \cite{leukemiapaper}, and a synthetic data set with 1-sparse ground truth $w^{\star}$ as in Section~\ref{subsec:clasetting} with random label flips given by $\mathbb{P}(\xi=-1)=\sigma, \mathbb{P}(\xi=+1)=1-\sigma$. Again, in the noiseless case the optimal choice of $p=1$ yields the best risk. However, and as expected from the Theorems~\ref{thm:mainl1} and \ref{thm:classificationlp}, for higher levels of noise higher values of $p$ yield the optimal estimator.

% \begin{figure}[t]
%     \centering
%     \hspace{-0.6cm}
%     \includegraphics[width=0.5\textwidth]{figures/leukemia_lp_svm_p_vs_risk.pdf}
%     \caption{Leukemia: \kd{change} Risk and bias-variance trade-off of the minimum $\ell_p$ norm interpolator as a function of $p$ on a synthetic data set generated as described in Section~\ref{subsec:regsetting}, with $n=100, d=5000$. The risk is plotted for a noiseless training data set as well as for noise $\sigma=2$. The bias and variance terms are computed on the noisy data set. All results are averaged over 50 simulations.}
%     \label{fig:synthetic regression}
% \end{figure}



% %While our theorems do not present an explicit connection with the classical notions of bias and variance for the mean squared error, we observe the presence of the noise $\sigma$ in the $\frac{\sigma^{4-2p} d^{2p-2}}{n^p} $ term from bound \eqref{eq:thmregboundhighnoiseupper}. We wonder whether this can be understood as some sort of variance of the final estimator, and leave the study of this connection for future work.



% Figure a shows the risk for lp svm.. \red{describe the setting}

% Figure bla shows the risk for regression \red{also say here what the setting is}



==> ICML 22-3/sections/experiments.tex <==




% \section{Empirical results}
% % I suggest the following structure here: Scope ( at most 3/4 of a page!)
% % \begin{itemize}
% %     \item Regression lp - Indeed, we can see that the optimal p is in (1,2). We wonder whether this trade-off is also captured by the bias and variance terms =... . Indeed, as we can see, one term goes down and one goes up. We discuss the relation between the bias variance trade-off and Thm 1 in the future work section (because currently it is not well understood). 
% %     \item We also observe this trade-off for classification with lp-svm on synthetic data. 
% %     \item While real world regression data sets are usually inherently noisy and thus regularized estimators are a nat ural choice, classification datasets used in real world examples can sometimes also be considered as noiselss (when being labeled by some human representing the  ground truth). Thus, the use of hard margin support vector machine relevant in practice ( cite here). Figure bla the performance with respect to $p$. We observe that in the noiseless case $p=1$ performs indeed the best. However, in the presence of random label flips, we observe that the expected trade-off occurs. \red{i feel like this real world motivation is quite weak...}
% % \end{itemize}


% We saw from the results in the previous two sections that $p\in(1,2)$ achieves faster rates compared to $p=1,2$. In this section we present numerical simulations addressing the following two question: is the optimal $p$ also attained in $(1,2)$ for finite $n,d$ of practically relevant order? Furthermore, can this phenomenon be related to a bias-variance trade-off in regression?


% % Yet, it is unclear whether a trade-off between $p=1$ and $2$ also occurs for finite $n,d$ of practically relevant orders. In this Section, we study the performance of interpolating for different values of $p$ in practical scenarios and observe a correspondence with the trend predicted by the theoretical results.
% % \kd{in practical scenarios but not on real world data? rephrase}


% \paragraph{Regression and the bias-variance trade-off}
% \begin{figure}
%     \centering
%     \includegraphics[width=0.5\textwidth]{figures/synthetic_regression_bias_variance.pdf}
%     \caption{Risk and bias-variance trade-off of the minimum $\ell_p$ norm interpolator as a function of $p$ on a synthetic dataset generated as described in Section~\ref{subsec:regsetting}, with $n=100, d=5000$. The risk is plotted for a noiseless training dataset as well as for noise $\sigma=2$. The bias and variance terms are computed on the noisy dataset. All results are averaged over 50 simulations.}
%     \label{fig:synthetic regression}
% \end{figure}
% Figure~\ref{fig:synthetic regression} shows the performance of the min-$\ell_p$ norm interpolator $\what$ from Equation~\eqref{eq:minlpnomrinterpol} on a synthetic dataset with 1-sparse ground truth, as described in Section~\ref{subsec:regsetting}.
% The optimal risk on noiseless data is achieved for the strongest structural bias $p=1$, while $p=2$ yields constant risk. However, in agreement with the theoretical observations from Theorem~\kd{thm:regressionlp}, noise causes a shift in the optimal $p$ which lies inside $(0, 1)$.
% %\red{for this i would like to see an experiment} Importantly, and differently form regularized models, the optimum is therefore attained when the structural bias is balanced to compensate the effects of noise. \\
% %\kd{rewrite:}
% In addition to the risk, Figure~\ref{fig:synthetic regression} shows the estimated bias and variance terms. We can clearly see that the optimal $p$ can also be explained as a trade-off of these two terms.  We further discuss this relation in Section~\ref{sec:trade-off}.

% %While our theorems do not present an explicit connection with the classical notions of bias and variance for the mean squared error, we observe the presence of the noise $\sigma$ in the $\frac{\sigma^{4-2p} d^{2p-2}}{n^p} $ term from bound \eqref{eq:thmregboundhighnoiseupper}. We wonder whether this can be understood as some sort of variance of the final estimator, and leave the study of this connection for future work.

% \paragraph{Classification with $\ell_p$ support vector machines.} 


% % \begin{figure*}[t!]
% %     \centering
% %     \begin{subfigure}[t][width=0.4\textwidth]
% %          \centering
% %          \includegraphics[width=\textwidth]{figures/synthetic_lp_svm_p_vs_risk.pdf}
% %          \caption{Synthetic data. The data are generated with a 1-sparse ground truth $w^{\star}$ and $y=\sign(<x, w^{\star}>)$. Here $n=100$, $d=5000$.}
% %          \label{fig:synthetic classification subplot}
% %      \end{subfigure}
% %      \hfill
% %      \begin{subfigure}[t][width=0.4\textwidth]
% %          \centering
% %          \includegraphics[width=\textwidth]{figures/leukemia_lp_svm_p_vs_risk.pdf}
% %          \caption{Leukemia dataset. The results are averaged over 100 random train-validation splits of the dataset, resulting in $n=65$. The data dimension is $d=7070$.}
% %          \label{fig:leukemia classification subplot}
% %      \end{subfigure}
% %     \caption{Risk for $\ell_p$ support vector machine \eqref{eq:svm prob} on synthetic (a) and real (b) data.}
% %     \label{fig:classification svm}
% % \end{figure*}


% Real world regression tasks are in general considered to be noisy, thus in such scenarios regularized estimators are a natural choice. Oppositely, classification datasets can sometimes be considered noiseless. In such cases, classification with hard-margin support vector machines is a practically relevant case \cite{noble2004support, brown1999support, guyon2002gene, furey2000support, cervantes2020comprehensive} \red{check if these are enough, the last is a survey and we can find many more there}. Figure~\ref{fig:classification svm} shows the performance of the max-$\ell_p$-margin interpolator, or also called \emph{hard-margin $\ell_p$-support vector machine}, on the Leukemia dataset \cite{leukemiapaper}, and a synthetic dataset with 1-sparse ground truth $w^{\star}$ as in Section~\ref{subsec:clasetting} with random label flips given by $\mathbb{P}(\xi=-1)=\sigma, \mathbb{P}(\xi=+1)=1-\sigma$. Again, in the noiseless case the optimal choice of $p=1$ yields the best risk. However, and as expected from the Theorems~\ref{thm:mainl1} and \ref{thm:classificationlp}, for higher levels of noise higher values of $p$ yield the optimal estimator.
% \begin{figure*}[t]
%     \centering
%      \begin{subfigure}[b]{0.45\linewidth}
%          \centering
%   \includegraphics[width=\textwidth]{figures/synthetic_lp_svm_p_vs_risk.pdf}
%          \caption{Synthetic data.}
%          \label{fig:synthetic classification subplot}
%      \end{subfigure}
%           \begin{subfigure}[b]{0.45\linewidth}
%          \centering
%          \includegraphics[width=\textwidth]{figures/leukemia_lp_svm_p_vs_risk.pdf}
%          \caption{Leukemia dataset.}
%          \label{fig:leukemia classification subplot}
%      \end{subfigure}
%          \caption{\red{update this caption when we have confidence intervals for regression as well} Risk for the $\ell_p$ support vector machine \eqref{eq:svm problem} on synthetic (a) and real (b) data. (a) the data is generated with a 1-sparse ground truth $w^{\star}$ and $y=\sign(<x, w^{\star}>) \xi$, with $\mathbb{P}(\xi=-1)=\sigma, \mathbb{P}(\xi=+1)=1-\sigma$. Here $n=100$, $d=5000$. (b)  The results are averaged over 100 random train-test splits of the dataset, resulting in $n=65$. The data dimension is $d=7070$.}
%     \label{fig:classification svm}
% \end{figure*}




% % Figure a shows the risk for lp svm.. \red{describe the setting}

% % Figure bla shows the risk for regression \red{also say here what the setting is}



==> ICML 22-3/sections/introduction.tex <==


\begin{abstract}
Good generalization performance on high-dimensional data crucially hinges on a simple structure of the ground truth and a corresponding strong inductive bias of the estimator. Even though this intuition is valid for regularized models, in this paper we caution against a strong inductive bias for interpolation in the presence of noise: While a stronger inductive bias encourages a simpler structure that is more aligned  with the ground truth, it also increases the detrimental effect of noise. Specifically, for both linear regression and classification with a sparse ground truth, we prove that minimum $\ell_p$-norm and maximum $\ell_p$-margin interpolators achieve fast polynomial rates close to order $1/n$ for $p > 1$ compared to a logarithmic rate for $p = 1$. Finally, we provide preliminary experimental evidence that this trade-off may also play a crucial role in understanding non-linear interpolating models used in practice. 
\end{abstract}

\section{Introduction}
Despite being extremely overparameterized, large complex models such as deep convolutional neural networks generalize surprisingly well, even when interpolating noisy training data. 
If the noise in the training data is low,  a natural explanation could be that these models are biased towards having a certain structural simplicity. %assumptions on 
%or this observation is that these models have a strong \emph{inductive bias} towards an inherently ``simple'' structure that matches the ground truth.
% Mathematically speaking, structural simplicity is often captured by a small norm. 
%Such structure a machine learning model 
%is often characterized by a norm.
%which captures the underlying structure of the model. 
%For example, for regularized empirical risk minimizers, this is simply the norm of the corresponding regularization penalty. 
% Moreover, 
%norms characterize the implicit bias of optimization algorithms on neural network architectures, 
For example, in deep learning theory, a long line of work studies the \emph{implicit bias} of standard optimization algorithms towards solutions with a small structured norm, 
see e.g. \cite{telgarski_gradient_descent, Lyu2020Gradient, soudry18, chizat2020implicit,arora2019exact,jacot2018neural}.
If the optimal prediction model also has a small corresponding norm, then, intuitively, the implicit bias effectively reduces the search space
to a "good" subset that includes a good model.

Even though this intuition is valid in the low-noise regime, it is unclear why the generalization error might stay low when the (structured) models are forced to interpolate non-negligible noise in the data.
Further, it is hard to mathematically characterize structural simplicity for complex prediction models, and theoretical analysis is difficult.
%Even though this intuition is valid in the low-noise regime, it is  unclear why the generalization error might stay low when the (structured) models are forced to interpolate noise in the data.
%these models generalize well even when forced to interpolate a considerable amount of noise in the data.


Interestingly, some of the fundamental phenomena revolving around the generalization behavior of interpolating complex overparameterized models even occur for high-dimensional linear models (see e.g., \cite{hastie2019surprises,muthukumar_2020,bartlett_2020,deng21}  and references therein). Although the latter are significantly simpler to analyze, 
the literature has yet to %paint a complete picture 
provide a comprehensive theoretical understanding for interpolating models as it exists for example for regularized estimators. This paper aims to take an important step in that direction.
%existing theoretical explanations  \fy{paint an incomplete picture} despite recent advancement. 
%With this paper, we aim to enhance our intuitive understanding for interpolating models in the hope that the intuition can aid the complex overparameterized models. 
%this line of research in the hope to develop new intuition for interpolating linear models that may also transfer to 
%gain intuition for linear models  also transfers to 
%complex overparameterized models. 

As mentioned above, high-dimensional parametric models with structural simplicity may correspond to parameter vectors with a small particular norm.
%be modeled by a norm that captures a certain structure.
For linear models, the common structural simplicity assumption is sparsity, induced by the $\ell_0$/$\ell_1$-norms -- the concrete example we focus on in this paper.
%we focus on sparse linear regression as a concrete example.
%sparsity inducing $\ell_0$/$\ell_1$ norms
%or an RKHS norm for structured kernels such as convolutional/pooled kernels \cite{arora2019exact}.
We say that estimators with small $\ell_0$/$\ell_1$-norm 
%the corresponding model 
have a \emph{strong inductive bias} towards ``simple'', in this case sparse, solutions. 
%We contrast such \emph{structured} norms \fy{hae, what does structured norm mean? do we actually use this term?}
In contrast, the more frequently studied rotationally invariant $\ell_2$-norm
%or RKHS norm of rotationally invariant kernels. 
%These rotationally invariant norms 
uniformly shrinks the estimator in all directions, thereby inducing only weak to no inductive bias towards sparse solutions.


% Although estimators with a strong inductive bias can yield fast minimax optimal rates when the dimension $d$ 
% grows with the sample size $n$,
% their good performance crucially relies on sacrificing data fit via regularization  (see e.g. $\ell_1$-norm regularized estimators for regression \cite{tibshirani_1996,vandegeer_2008} and classification \cite{Zhang2014EfficientAF}.
%kernel ridge regression \cite{misiakiewicz2021learning} and convex neural networks \cite{bach2017breaking}).
%Instead, state-of-the-art overparameterized models are often structured interpolators and generalize well even though trained to perfectly fit noisy data. 
%Aiming to gain a better intuition on this phenomenon, in this paper we discuss how the inductive bias affects the generalization 
%capabilities of interpolating models % performance
%in the presence of noise.

For noiseless interpolation, it is well-known that the min-$\ell_1$-norm interpolator (aka basis pursuit) yields exact recovery for sparse ground truths \cite{chen_1998}. Moreover, when the measurements are noisy,
its regularized variant, the LASSO \cite{tibshirani_1996}, achieves minimax optimal rates of order $\frac{s\log(d)}{n}$
\cite{vandegeer_2008} (where $s$ is the $\ell_0$-norm of the ground truth).
However, when forcing structured models to interpolate the noisy samples, it is unclear why the generalization error might stay low. In fact, the min-$\ell_1$-norm interpolator achieves rates of order $\frac{1}{\log(d/n)}$ \cite{wang2021tight,muthukumar_2020}, suggesting that models with strong inductive biases suffer heavily from noise.

% It is  unclear why the generalization error might stay low when the (structured) models are forced to interpolate noise in the data.However, when forcing the model to  interpolate the noisy samples, the min-$\ell_1$-norm interpolator achieves rates of order $\frac{1}{\log(d/n)}$ \cite{wang2021tight,muthukumar_2020}. This reasons that models with strong inductive biases suffer heavily from noise.

On the other hand, a long line of work establishes how 
min-$\ell_2$-norm interpolators with a weak inductive bias  benefit from noise resilience in high dimensions
(see e.g., \cite{hastie2019surprises,bartlett_2020,muthukumar_2020,muthukumar2021classification} and references therein). 
However, these uniform shrinkage estimators do not encode structural assumptions on the ground truth --- thus
fail to learn the signal  for
inherently high-dimensional covariates such as isotropic Gaussians (see e.g., \cite{muthukumar_2020}). 

The apparent trade-off between structural simplicity and noise resilience in high dimensions raises a natural question:
\begin{center}
\emph{Can min-norm interpolators in noisy high dimensional settings achieve fast or even close to minimax optimal rates using a moderate inductive bias?}
\end{center}


To the best of our knowledge, in this paper, we first provide a positive answer for sparse linear models. Specifically, we bound the (directional) estimation error of min-$\ell_p$-norm interpolators (for regression) and max-$\ell_p$-margin interpolators (for classification).
For isotropic Gaussian features with dimension $d \asymp n^\beta$ for $\beta>1$ and in the presence of observation noise in the data, 
\begin{itemize}
    \item we provide upper and lower bounds  for
    min-$\ell_p$-norm interpolators with ${p\in(1,2)}$. For large enough $d,n$, the estimation error decays at polynomial rates close to order $1/n$ compared to logarithmic or constant rates for $p=1$ or $2$ (Section \ref{sec:reg}). \vspace{-0.05in}
    \item we further provide upper bounds for the %risk%\footnotemark[1] 
     max-$\ell_p$-margin interpolators (or equivalently, hard $\ell_p$-margin SVM) with ${p\in(1,2)}$. Surprisingly, for large enough $d,n$, they even match minimax optimal rates  of order $1/n$ up to logarithmic factors in the regime $\beta \geq 2$  (Section~\ref{sec:cla}). 
\end{itemize}

We confirm the better generalization properties for the choice $p\in (1,2)$ compared to $p=1$ and $p=2$ on synthetic and real-world data in Section~\ref{sec:discussion}.
Our results on linear models suggest that when interpolating noisy data, a moderate inductive bias yields the optimal performance. Additional experiments with convolutional neural tangent kernels in Section~\ref{sec:trade-off} provide  preliminary evidence that this intuition may also extend to non-linear models, prompting an exciting line of future work. In particular, we hypothesize that this trade-off between
structural simplicity and noise resilience may be an important ingredient for understanding the good generalization capabilities of overparameterized interpolating models used in practice.



==> ICML 22-3/sections/main_classification.tex <==



\section{Maximum-margin Interpolators for Classification}
\label{sec:cla}
We now establish upper bounds for max-$\ell_p$-margin interpolators, also called hard-margin $\ell_p$-SVMs or sparse-SVMs \cite{blanco2020lp,bennett2000duality}.
We show that these interpolators achieve fast rates for $p\in(1,2)$ and even match minimax optimal rates up to logarithmic factors. 



\subsection{Setting}
\label{subsec:clasetting}
% \fy{this is not standard! or rather its unclear what that is!}
We study a discriminative linear classification setting with $n$ pairs of random input features $x_i \overset{\iid}{\sim} \NNN(0,I_d)$ and associated labels 
$y_i =\sgn(\langle \xui, \wgt \rangle)\xi_i$
where the label noise 
$\xi_i \in \{+1, -1\}$ follows the conditional distribution 
\begin{equation}
    \xi_i | x_i \sim \probsigma( \cdot; \langle x_i, \wgt \rangle)
\end{equation}
for some parameter~$\sigma$.
We again choose $\wgt = (1,0,\cdots,0)$ for the same reason as in Section~\ref{subsec:regsetting}.
Notice that the noise only depends on the input features in the direction of the ground truth.
More specifically,  we make the 
following assumption on the noise distribution~$\probsigma$:
\begin{itemize}
  \item[]
    The function ${z \to \probsigma(\xi=1; z)}$ is a piece-wise continuous function such that the minimum ${\nubar := \underset{\nu}{\arg\min}~ \EE_{Z \sim \NNN(0,1)} \EE_{\xi \sim \probsigma(\cdot; Z)} \left( 1- \xi \nu \vert Z \vert\right)_+^2 }$ exists and is positive $\nubar>0$.  
 \end{itemize}



Assumption A is rather weak and satisfied by most noise models in the literature,  such as
\begin{itemize}
    \item\textit{Logistic regression} with  $\probsigma(\xi_i=1; z) = h(z \sigma)$ and $h(z) = \frac{e^{\vert z\vert}}{1+e^{\vert z\vert}}$ and $\sigma >0$. 
    \item \textit{Random label flips} with  $\probsigma(\xi=1; \langle \xui, \wstar \rangle) = 1-\sigma$ and  $\sigma \in (0,\frac{1}{2})$. 
    \item \textit{Random noise before quantization} where $\yui = \sgn(\langle \wgt, \xui \rangle + \tilde{\xi}_i)$ with $\tilde{\xi}_i\vert x_i \sim \NNN(0, \sigma^2)$ and  $\sigma^2>0$.
\end{itemize}

Given the data set $\{\left(\xui, \yui\right)\}_{i=1}^n$, the goal is to obtain an estimate $\what$ that
%points in a similar direction as \fy{sounds like a kid}
directionally aligns with the  normalized ground truth $\wgt$ and thus has a small directional estimation error
\begin{align}
\label{eq:prediction_error_cla}
    \RiskC(\what) := \norm{\frac{\what}{\norm{\what}_2} - \wgt}_2^2.
\end{align}
This  classification error is also studied for example in the 1-bit compressed sensing literature (see e.g., \cite{Boufounos2008,plan2012robust} and references therein). 
Note that a small value $\RiskC(\what)$ corresponds to a small expected (noiseless)  0-1 error via the relation
\ifarxiv
\begin{align}
  &\EE_{x\sim \NNN(0,I_d)} \idvec[\sgn(\langle x, \what\rangle) \neq \sgn(\langle x,\wgt \rangle)] \nonumber = \frac{1}{\pi} \arccos\left(1- \frac{\RiskC(\what)}{2}  \right) \approx \frac{1}{\pi} \sqrt{\frac{\RiskC(\what)}{2}} \, .
\end{align}
\else
\begin{align}
  &\EE_{x\sim \NNN(0,I_d)} \idvec[\sgn(\langle x, \what\rangle) \neq \sgn(\langle x,\wgt \rangle)] \nonumber\\
    &= \frac{1}{\pi} \arccos\left(1- \frac{\RiskC(\what)}{2}  \right) \approx \frac{1}{\pi} \sqrt{\RiskC(\what)} \, .
\end{align}

\fi

Throughout this section, we study the \emph{max-$\ell_p$-margin interpolators}, or equivalently, the hard-margin $\ell_p$-SVM solutions  for $p\in [1,2]$ defined by 
      \begin{equation}\label{eq:svm problem}
    \what = \argmin_{w} \norm{w}_p \subjto \forall i:~ \yui \langle \xui, w \rangle \geq 1.
\end{equation}




\subsection{Maximum-\texorpdfstring{$\ell_p$}{lp}-margin Interpolation} 
\label{subsec:clalp}
% \kd{first time mentioning minimax lower bounds should be discussed}
We are the first to present non-asymptotic upper bounds for the directional estimation error of max-$\ell_p$-margin interpolators.

\begin{theorem}
\label{thm:classificationlp}
    Let the data distribution be as described in Section~\ref{subsec:clasetting} and assume that the noise model $\probsigma$ is independent of $n,d$ and $p$.
Let $q$ be such that $\frac{1}{p} + \frac{1}{q} =1$. 
There exist universal constants 
%$\kappa_1,\kappa_2,\kappa_3,\kappa_4,\kappa_5,\kappa_6,\kappa_7>0$
$\kappa_1,\cdots,\kappa_7>0$
such that for any $n\geq \kappa_1$, any $p \in\left(1+\frac{\kappa_2}{\log\log d},2\right)$ and any
$ n \log^{\kappa_3}n \lesssim d \lesssim \frac{n^{q/2}}{\log^{\kappa_4 q}n}$, the directional estimation error of the max-$\ell_p$-norm interpolator~\eqref{eq:svm problem} satisfies
% There exist universal constants $\cn,\cl,\cd,\cp,\cone, \ctwo>0$ such that for any $q \lesssim \log\log(d)$ and any
% $ n \log(n)^2 \lesssim d \lesssim \frac{n^{q/2}}{\log(n)^{c q}}$ and
%     $n \gtrsim 1$, the prediction error is upper- and lower-bounded 
% There exist universal constants $ c, c_n, c_l, c_u > 0 $ such that, if $ n\geq c_n $ and $ c_l n \leq d \leq \exp \left( c_u n^{1/5} \right) $, then
\begin{equation}
\label{eq:classificationlp}
\RiskC(\what) \lesssim  \frac{ q^{\frac{3}{2}p}d^{3p-3} \log^{3/2}d}{n^{\frac{3}{2}p} } \lor \frac{n  \exp(\kappa_4q)}{qd} \lor  \frac{\log^{\kappa_5} d}{n} \, ,
\end{equation}
with probability at least $ 1 - \kappa_6 d^{-\kappa_7}$ over the draws of the data set. 
\end{theorem}
% The dependency on the noise is captured by constants only depending on $\probsigma$  hidden in  the universal constants.
The proof of the result is presented in Appendix~\ref{apx:claslpproof}.
The dependence on the noise  $\probsigma$ is hidden in  the universal constants but can be made explicit when carefully following the steps in the proof.   We refer to Section~\ref{rm:p} for a discussion on the assumptions in the theorem. Throughout the discussion we consider the regime $d \asymp n^{\beta}$ with $\beta>1$. 




\begin{figure}[t!]
    \centering
    \ifarxiv
    \includegraphics[width=0.4\linewidth]{figures/classification_rates.pdf}
    \else 
        \includegraphics[width=\linewidth]{figures/classification_rates.pdf}
    \fi
         \caption{Depiction of Theorem~\ref{thm:classificationlp} for classification  when $d\asymp n^{\beta}$. We plot the exponent $\alpha$ of the resulting  upper bound of the (directional) estimation error rate 
        $\tilde{O}(n^{\alpha})$  for different strengths of inductive bias $p$ and different high-dimensional regimes $\beta$.}
    \label{fig:ratescla}
   % \vspace{-0.2in}
\end{figure}





\paragraph{Close to  minimax optimal rates}
As for regression, Theorem~\ref{thm:classificationlp} 
implies that 
 the estimation error $\Risk(\what) = \tilde{O}(\alpha)$ of the max-$\ell_p$-margin interpolator with ${p \in \left(1 + \frac{\kappa_2}{\log\log d}, \frac{3 \beta}{3 \beta - 1.5}\right)}$ vanishes at a polynomial rate ($\alpha<0$).  We again illustrate the rates in Figure~\ref{fig:ratescla} where we plot the exponent of the rate $\alpha$ as a function of $\beta$ for different values of $p$, assuming that $d,n$ is sufficiently large. Furthermore, we plot the minimax optimal lower bounds  (dotted line at $\alpha=-1$) for the directional estimation error $\RiskC$, which are known to be of order $\frac{\log d}{n}$  \cite{Wainwright2009InformationTheoreticLO,abramovich2018high}. 
When $\beta>2$ and $p$ is small, the rates of the max-$\ell_p$-norm interpolator
are of order $\tilde{O}(\frac{1}{n})$ and hence minimax optimal up to logarithmic factors. 
More specifically, for any  $\beta>2$ and $p\in \left( 1 + \frac{\kappa_2}{\log\log d}, \frac{6\beta-2}{6\beta - 3} \right)$, the term $ \frac{\log^{\kappa_5}d}{n}$ dominates the RHS in Equation~\eqref{eq:classificationlp} and we obtain a minimax optimal rate up to logarithmic factors. 

 

 
%  We compare the rates against the minimax optimal rate for sparse regression  of order $\frac{\sigma^2 \log d}{n}$ (dotted horizontal line at $\alpha = -1$) \cite{Raskutti2011MinimaxRO}.
% We can clearly see in Figure~\ref{fig:rates_reg} that for $\beta>2$ and small values of $p$, the rates of the error are close to the minimax optimal rate. In fact, when choosing $\beta =2$ and $p = 1 + \kappa_4/\log\log d$, Theorem~\ref{thm:regressionlpmain} shows that, for $n,d$ sufficiently large, the rate of the error is close to the minimax optimal rate up to logarithmic factors. 





% in Figure~\ref{fig:ratescla} we illustrate the rates of the upper bound \eqref{eq:classificationlp}. We again plot the decay rate $\alpha$ 
% for the directional estimation error $\RiskC(\what) = \tilde{O}(n^{\alpha})$ as a function of $\beta>1$ with $d \asymp  n^{\beta}$ for different values of $p$, assuming $d,n$ is sufficiently large. 
% Minimax lower bounds (dotted line at $\alpha=-1$) for the directional estimation error $\RiskC$ are known to be of order $\frac{\log d}{n}$  \cite{Wainwright2009InformationTheoreticLO,abramovich2018high}. 

\vspace{-1mm}
\paragraph{Faster rates than $p=1$}
So far, previous non-asymptotic upper bounds for the error of the max-$\ell_1$-margin interpolator  \cite{chinot2021adaboost}  are non-vanishing, while to the best of our knowledge we are not aware of any lower bounds. However, using the same tools as used for bounding the error of the min-$\ell_1$-norm interpolator in \cite{wang2021tight} and the tools introduced in the proof of Theorem~\ref{thm:classificationlp}, we can upper and lower bound\footnote{The explicit theorem statement is moved from the camera ready version of this paper as a response to the reviewers concerns on the length of the paper. The statement will instead appear in a followup work of \cite{wang2021tight}.} the directional estimation error \eqref{eq:prediction_error_cla} by  $\RiskC(\what) \asymp \frac{1}{\log(d/n)}$.


Analogous to regression, Figure~\ref{fig:ratescla}  shows how the max-$\ell_p$-margin interpolators with $p>1$ achieve faster rates compared to $p =1$ and $2$ (dashed line at $\alpha=0$ in Figure~\ref{fig:ratescla}).
More specifically, for any fixed $\beta>1$, we obtain  faster rates  with any $p \in \left(1 + \frac{\kappa_2}{\log\log d}, \frac{3 \beta}{3 \beta - 1.5}\right)$ than with $p=1$ and $2$.


\paragraph{Lower bounds} Unlike Theorem~\ref{thm:regressionlpmain}, Theorem~\ref{thm:classificationlp} does not provide matching lower bounds.
However, when $\beta \geq 2$ and $p$ is small, the rates in Theorem~\ref{thm:classificationlp} are close to minimax lower bounds and therefore cannot be improved. Furthermore, 
similar to regression, in Proposition~\ref{prop:uniformlowerbound} we provide  a uniform lower bound of order $\frac{n}{d}$ for all interpolating classifiers that matches the upper bound  in Theorem~\ref{thm:classificationlp}  for the regime $\beta\leq 2$ and when $p$ is small.  
% For $\beta>2$ in turn, we obtain minimax optimal rates. 
%both together illustrates how "tight" these bounds are.} 
 The proof can be found in Appendix~\ref{apx:uniformlowerbound}. 
\begin{proposition}[Universal lower bound for all interpolating classifiers]
\label{prop:uniformlowerbound}
  Let the data distribution be as described in Section~\ref{subsec:clasetting} and assume that the noise model $\probsigma$ is independent of $n,d$ and $p$.
  There exist universal constants $\kappa_1,\kappa_2>0$ such that 
for all non-zero ground truths $\wgt\in\mathbb{R}^d$, with probability $\geq 1-\exp(-\kappa_1 n) -\exp(-\kappa_2 d)$ for some $\kappa>0$,
the directional estimation error of any interpolator $\what$ satisfying $\forall i: \yui \langle \xui, \what \rangle \geq 0$ satisfies
\begin{equation}
    \RiskC(\what) \geq \frac{c n}{d}. 
\end{equation}
\end{proposition}
% As we can see, this lower bound is again of the same order as the term $\frac{n  \exp(\kappa_5q)}{qd}$ appearing in the upper bound in Theorem~\ref{thm:classificationlp}, assuming that $p$ (and thus $q$) is constant. 
% Finally, we note that a similar uniform lower bound has been established for linear regression
% \cite{muthukumar_2020,zhou20} using a very different proof technique. 

\paragraph{Comparison with regression.}
Comparing the rates in Figures~\ref{fig:rates_reg} and \ref{fig:ratescla}, we can see that the max-$\ell_p$-margin interpolators in classification achieve faster rates than the corresponding min-$\ell_p$-norm interpolators in regression, in the sense that they are of order of minimax lower bounds for a wider range of $\beta$ and $p\in(1,2)$. 
% Indeed, the max-$\ell_p$-margin interpolators achieve minimax optimal rates for $\beta \in [2,\frac{\frac{3}{2} p-1}{3p-3}]$ compared to $\beta =2$  for min-$\ell_p$-norm interpolators in regression.
We remark that the proofs of Theorems~\ref{thm:regressionlpmain} and \ref{thm:classificationlp} follow a similar scheme (see
detailed discussion in Section~\ref{sec:proofidea}).
Intuitively,
the difference in performance mostly originates from the fact that the  directional estimation error $\RiskC$ merely depends on the direction of the interpolator $\what$ and not its magnitude,
as it is the case for the estimation error $\RiskR$ in regression. We note that the authors in \cite{muthukumar2021classification} observe a similar difference in performance between max-margin and min-norm interpolators for $p=2$
and Gaussians features with spiked covariance matrices. 










%%%%%%%%%%%%%%%%%%%%%%%
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%  \subsection{Maximum-\texorpdfstring{$\ell_1$}{l1}-margin interpolation} 
%  \label{subsec:clal1}
% Existing upper bounds for max-$\ell_1$-margin interpolation on data sets with a constant fraction of mislabeled training points are non-vanishing for $d\gg n$ \cite{chinot2021adaboost}.
% In contrast, under Assumption (A) on the label noise, we prove tight non-asymptotic bounds that imply
% consistency for $d\propto n^\beta$ with $\beta>1$.

  
% \begin{theorem} \label{thm:mainl1}
%     % where
%     % $O(\cdot)$ hides constants independent of $d,n$ and~$\sigma$. 
%     Let the data distribution be as described in Section~\ref{subsec:clasetting} and assume that the noise model $\probsigma$ is independent of $n,d$ and $p$.
%     Then there exist universal constants $\kappa_1,\kappa_2,\kappa_3,\kappa_4>0$ such that,
%     for any $n\geq \kappa_1$ and
%     % $d \leq \exp(c_d n)$ and $\log(d/n) \geq c_l$,
%     $\kappa_2 n \leq d \leq \exp(\kappa_3 n^{1/5})$, the directional estimation error of the max-$\ell_1$-margin interpolator~\ref{eq:svm problem} is upper- and lower-bounded as
%     \begin{equation}
%     \label{eq:mainboundl1}
%          \left\vert \RiskC(\what)  - \frac{\kappanoise}
%           {\log(d/n)} \right\vert \lesssim \frac{ 1}{\log^{5/4}(d/n)} \, ,
%     \end{equation}
%     with probability at least 
%     ${1- \kappa_4\exp\left(-\frac{n}{\log^6(d/n)}\right)}$ over the draws of the data set and with $\kappanoise$  a constant only depending on $\probsigma$ (see Equation~\eqref{eq:kappanoise} in Appendix~\ref{apx:proofl1} for the definition). 
% \end{theorem}
% The exact expression for $\kappanoise$ and the proof of the result can be found in Appendix~\ref{apx:proofl1}. We refer to Appendix~\ref{rm:p}  for a discussion on how the assumptions in the theorem can be generalized. 

% Even though our non-asymptotic bound shows consistency
% for high-dimensional data when $d\gg n$, %While being consistent when $d\gg n$, we  see that, as for min-$\ell_1$-norm regression, 
% our lower bounds show that the max-$\ell_1$-margin interpolator converges very slowly. In comparison, the  $\ell_1$-regularized classifier  achieves rates  of order $\frac{\log^{\kappa}(d)}{n}$ with $\kappa \geq1$ \cite{Zhang2014EfficientAF}.
% Analogous to regression \cite{wang2021tight}, the max-$\ell_1$-margin interpolator achieves fast rates in the noiseless case \cite{chinot2021adaboost}, but is highly sensitive to noise in the training data. 



==> ICML 22-3/sections/main_regression.tex <==






\section{Minimum-norm Interpolators for Regression}
\label{sec:reg}
In this section we derive non-asymptotic bounds for sparse linear regression for the estimation error of min-$\ell_p$-norm interpolators with $p\in(1,2)$. We describe the setting in Section~\ref{subsec:regsetting} and present the main theorem followed by a discussion in Section~\ref{subsec:regmain}. 


% Introduction: we study sparse linear regression. for sparse lin reg regularized /noiseless clearly l1 is minimax optimal, l2 has no chance even in noiseless case. however recent work shows a slow rate (lower bound). In this section we show we can do significantly better than l1 in Theorem bla. In fact, we give tight bounds for lp interpolation (in some regimes). Can even achieve minimax optimal rate  The section is structured as follows:
% Introduce Setting, present main theorem and discuss. 





\subsection{Setting}
\label{subsec:regsetting}
We study a standard linear regression model where we observe $n$ pairs of standard normal distributed features $x_i \overset{\iid}{\sim} \NNN(0,I_d)$ and observations $y_i = \langle \xui, \wstar \rangle + \xi_i$ with Gaussian noise $\xi_i \overset{\iid}{\sim} \NNN(0,\sigma^2)$.  For simplicity,  
we consider the 1-sparse ground truth $\wgt = (1,0,\cdots,0)$ and discuss in Section~\ref{rm:p} how to generalize this assumption. 
Given the data set $\{\left(\xui, \yui\right)\}_{i=1}^n$, the goal is to find an estimator $\what$ that has small estimation error
\begin{equation}
    \label{eq:prediction_error_reg}
 \RiskR(\what) := \norm{\what -\wgt}_2^2 = \EE_{x\sim \NNN(0,I_d)} \langle x, \what - \wgt \rangle^2    \, ,
\end{equation}
which also corresponds to the irreducible prediction error. We specifically study \emph{min-$\ell_p$-norm interpolators} with $p\in (1,2)$, given by
      \begin{equation}\label{eq:minlpnomrinterpol}
    \what = \argmin_{w} \norm{w}_p \subjto \forall i:~\langle \xui, w \rangle = y_i, 
\end{equation}
where $\|w\|_p := \left(\sum_i w_i^p\right)^{1/p}$. 
%For any $p \geq 1$, Equation~\eqref{eq:minlpnomrinterpol} is a strictly convex optimization problem and thus has a unique solution. 


\subsection{Main Result}
\label{subsec:regmain}
We now state our main result for regression that provides a  non-asymptotic upper bound for the estimation error of min-$\ell_p$-norm interpolators.\footnote{
We use $\lesssim,\gtrsim$ and $\asymp$ to hide universal constants, without any hidden dependence on $d$, $n$ or $p$. Further, $\tilde{O}(\cdot),\tilde{\Theta}(.)$ hide logarithmic factors in $d,n$ or $p$ and $a \lor b = \max(a,b)$.
}
\begin{theorem}
\label{thm:regressionlpmain}
Let the data distribution be as described in Section~\ref{subsec:regsetting} and assume that $\sigma \asymp  1 $. Further, let $q$ be such that $\frac{1}{p} + \frac{1}{q} =1$.  Then there exist universal constants $\kappa_1,\cdots,\kappa_7>0$ such that for any $n\geq \kappa_1$ and any ${p \in\left(1+\frac{\kappa_2}{\log\log d},2\right)}$ and ${n \log^{\kappa_3} n \lesssim d \lesssim n^{q/2}\log^{-\kappa_4 q}n}$, the estimation error of the min-$\ell_p$-norm interpolator~\eqref{eq:minlpnomrinterpol} satisfies
% There exist universal constants $ c, c_n, c_l, c_u > 0 $ such that, if $ n\geq c_n $ and $ c_l n \leq d \leq \exp \left( c_u n^{1/5} \right) $, then
\ifarxiv
\begin{align}
\label{eq:thmregboundhighnoiseuppermain}
      &\frac{\sigma^{4-2p}q^pd^{2p-2}}{ n^p} 
    \lor \frac{\sigma^2n}{d} \lesssim
    \RiskR\left( \what \right) \lesssim  \frac{\sigma^{4-2p}q^p d^{2p-2}}{n^p} 
    \lor \frac{\sigma^2n  \exp(\kappa_5 q)}{q d} \, ,
\end{align}
\else
\begin{align}
\label{eq:thmregboundhighnoiseuppermain}
      &\RiskR\left( \what \right) \gtrsim \frac{\sigma^{4-2p}q^pd^{2p-2}}{ n^p} 
    \lor \frac{\sigma^2n}{d} ~~\mathrm{and}\\
    &\RiskR\left( \what \right) \lesssim  \frac{\sigma^{4-2p}q^p d^{2p-2}}{n^p} 
    \lor \frac{\sigma^2n  \exp(\kappa_5 q)}{q d} \, , \nonumber
\end{align}
\fi
with probability at least $ 1 - \kappa_6 d^{-\kappa_7}$ over the draws of the data set. 
\end{theorem}
% \fy{so then if we never use $O$ anymore, we can indeed use $O$ to hide log factors? throughout (and ditch $\tilde{O})$? - I see in classification theres an $O$ left, but then we can just write a constant?}
% t\fy{also wonder if we should do: Note that these results require $d$ suff. large, not just the relation between $d,n$ maybe also thing about noise = 0}
The proof of the theorem can be found in Appendix~\ref{apx:regproof}.  We now discuss the implications of the theorem and  refer to Section~\ref{rm:p} for a discussion on the assumptions in the theorem. Throughout the discussion we consider the regime $d \asymp n^{\beta}$ with $\beta>1$. 


\paragraph{Close to  minimax optimal rates.}
Theorem~\ref{thm:regressionlpmain} implies that for any fixed $\beta>1$, the estimation error $\Risk(\what) = \tilde{O}(\alpha)$ of the min-$\ell_p$-norm interpolator with ${p \in \left(1 + \frac{\kappa_2}{\log\log d}, \frac{ 2\beta}{2 \beta - 1}\right)}$ vanishes at a polynomial rate ($\alpha<0$). To illustrate these rates, Figure~\ref{fig:rates_reg} plots the exponent of the rate $\alpha$ as a function of $\beta$ for different values of $p$, assuming that $d,n$ are sufficiently large. We compare the rates against the minimax optimal rate for sparse regression  of order $\frac{\sigma^2 \log d}{n}$ (dotted horizontal line at $\alpha = -1$) \cite{Raskutti2011MinimaxRO}.
We can clearly see in Figure~\ref{fig:rates_reg} that for $\beta>2$ and small values of $p$, the rates of the error are close to the minimax optimal rate. In fact, when choosing $\beta =2$ and $p = 1 + \frac{ \kappa_4}{\log\log d}$, Theorem~\ref{thm:regressionlpmain} shows that, for $n,d$ sufficiently large, the rate of the error equals the minimax optimal rate up to logarithmic factors. 



\paragraph{Faster rates than for $p=1$}
For comparison, we also indicate the rates of the min-$\ell_2$- and min-$\ell_1$-norm interpolators by the dashed horizontal line at $\alpha=0$, which are of constant and  $\frac{\sigma^2}{(\beta-1) \log n}$ order, respectively, \cite{wang2021tight,muthukumar_2020}. Clearly, we can see that the minimum-$\ell_p$-norm interpolator with $p\in(1,2)$ achieves faster rates than with $p=1$ and $2$. 
We emphasize that Figure~\ref{fig:rates_reg} depicts the exponent of the rate at which the error vanishes up to logarithmic factors for fixed values of $p$ as $d,n \to \infty$. For fixed $n,d$, our non-asymptotic bounds only hold for $p \in (1+\frac{\kappa}{\log\log d}, 2)$. We refer to Section~\ref{rm:p} for a discussion of this limitation and motivate future work on tight bounds for the full interval $p\in[1,2]$  in Section~\ref{subsec:optimalp}.



\begin{figure}[t!]
    \centering
        %   \begin{subfigure}[b]{0.45\linewidth}
         \centering
         \ifarxiv
    \includegraphics[width=0.4\linewidth]{figures/regression_rates.pdf}
    \else 
        \includegraphics[width=\linewidth]{figures/regression_rates.pdf}
\fi
        % \caption{Comparison with rates in Theorem~\ref{cr:koehler}}
        \caption{Depiction of Theorem~\ref{thm:regressionlpmain} for regression
        when $d\asymp n^{\beta}$. We plot the exponent $\alpha$ of the resulting estimation error rate 
        $\tilde{O}(n^{\alpha})$ for different strengths of inductive bias $p$ at different high-dimensional regimes $\beta$.}
    \label{fig:rates_reg}
   % \vspace{-0.2in}
\end{figure}

\paragraph{Tightness of the upper and lower bounds in Theorem~\ref{thm:regressionlpmain} } 
We note that for any fixed $p$ and $n,d$ sufficiently large, the upper and lower bounds in Theorem~\ref{thm:regressionlpmain} are of the same order. In fact, 
the second term in the lower bound of order $\frac{n}{d}$ is a universal lower bound for all interpolators  \cite{muthukumar_2020}. This bound is tight when the term $\frac{\sigma^2n  \exp(\kappa_5 q)}{q d} $  dominates the upper bound in Theorem~\ref{thm:regressionlpmain}, which is the case when  $\beta\leq 2$ and $p$ is small constant. 














% small, and thus the termdominates the upper bound. 

% For large enough $n,d$ the upper bounds in Theorem~\ref{thm:regressionlpmain}  match universal lower bound $n/d$ fo and even $1/n$ for $\beta=2$. For $\beta>2$ the first term blabla dominates in the lower and upper bounds which then match.

% As we can see from Equation~\eqref{eq:thmregboundhighnoiseuppermain}, for any constant $p$, the upper and lower bounds are of the same order. When $\beta<2$ the terms of order $\sigma^2 n/d$ dominate for $p\leq 2\beta / (2\beta -1)$, whereas when $\beta>2$

% Further, we remark that the term $\frac{\sigma^2 n}{d}$ in the lower bound is exactly of the same order as uniform lower bounds for \emph{all} interpolating models  (see \cite{zhou20,muthukumar_2020}) --- which hold even under full knowledge of the ground truth \fy{don't understand}. As a consequence, we can see that for constant $p$, if the term $\frac{\sigma^2n  \exp(\kappa_5 q)}{q d}$ dominates the upper bound in Equation~\eqref{eq:thmregboundhighnoiseuppermain}, the min-$\ell_p$-norm interpolator yields the optimal rate for all interpolating models. 




\paragraph{Comparison with existing bounds for min-$\ell_p$-norm interpolators.}
We now discuss existing results for min-$\ell_p$-norm interpolators from the literature. %and refer to 
To the best of our knowledge,  previous works do not  study the rates of the  min-$\ell_p$-norm interpolator. However, we may obtain an upper bound
%in Corollary~\ref{cr:koehler} 
as a consequence of Theorem~4 in \cite{koehler2021uniform} which follows straightforwardly from applying Lemma~\ref{cor:hqbound2} in Appendix~\ref{apx:subsec:localisationproofreg}
  and Lemma~\ref{cor:hqbound1} in Appendix~\ref{apx:proofdualnormconc}.

\begin{theorem}[Corollary of Theorem~4 from
\cite{koehler2021uniform} (informal)]
\label{cr:koehler}
Let the data distribution be as described in Section~\ref{subsec:regsetting} with general ground truth $\wgt\in\RR^d$. Under the same conditions on $d,n$ as in Theorem~\ref{thm:regressionlpmain}, there exist universal constants $\kappa_1,\kappa_2,\kappa_3>0$ such that for any $p\in (1,2]$ and $q$ such that $ \frac{1}{p} + \frac{1}{q} =1 $, we have that 
\ifarxiv
\begin{align}
    \RiskR(\what) &\lesssim \sigma^2 \left( \sqrt{\frac{\log d}{q}} \frac{1}{ d^{1/q}} + \sqrt{\frac{\log d}{n}}
    + \frac{n\exp(\kappa_1 q)}{qd} \right) + \sigma \norm{\wgt}_p d^{1/q} \sqrt{\frac{q}{n}} + \norm{\wgt}_p^2 \frac{ q d^{2/q}}{n} \nonumber
\end{align}
\else 
\begin{align}
    \RiskR(\what) &\lesssim \sigma^2 \left( \frac{\sqrt{\log d}}{\sqrt{q} d^{1/q}} + \sqrt{\frac{\log d}{n}}
    + \frac{n\exp(\kappa_1 q)}{qd} \right) \\
    &~~~~~+ \sigma \norm{\wgt}_p d^{1/q} \sqrt{\frac{q}{n}} + \norm{\wgt}_p^2 \frac{ q d^{2/q}}{n} \nonumber
\end{align}
\fi
with probability at least $1- \kappa_2 d^{-\kappa_3}$ over the draws of the data set.
\end{theorem}

We remark that it already follows from Theorem~\ref{cr:koehler}, in combination with the results in \cite{wang2021tight},  that $p>1$ achieves faster rates compared to $p=1$. However, for any $p$ and $\beta>1$ with $d=n^{\beta}$ the rates in the upper bound in Theorem~\ref{cr:koehler} are at most of order $n^{-1/4}$, and thus much slower than the rates in Theorem~\ref{thm:regressionlpmain} that can reach orders even close to $n^{-1}$.  
For a better comparison, we illustrate both the rates in Theorem~\ref{thm:regressionlpmain} and Theorem~\ref{cr:koehler} in Figure~\ref{fig:ratesk} in Appendix~\ref{rm:koehler}, which also provides a detailed comparison of the proof techniques used to derive Theorems~\ref{thm:regressionlpmain} and~\ref{cr:koehler}. 



\paragraph{Comparison with $\ell_p$-norm regularized estimators}
We are only aware of existing bounds in the literature for $\ell_p$-norm regularized estimators that characterize the ground truth by the  $\ell_p$-norm (e.g. see \cite{lecue17}). These bounds are at least of order $\|\wgt\|_p \frac{d^{2 - 2/p}}{n}$ (see Theorem 5.4 in  \cite{lecue17}), and thus slower than the bounds for the corresponding interpolating estimator in Theorem~\ref{thm:regressionlpmain}, for some choices of $\beta$.
Furthermore, we hypothesize when the term  $\frac{\sigma^{4-2p}q^p d^{2p-2}}{n^p}$ on the RHS in Equation~\eqref{eq:thmregboundhighnoiseuppermain} dominates, the optimally $\ell_p$-norm regularized estimator achieves the same rates as the corresponding interpolator. As can be seen in the proof of Theorem~\ref{thm:regressionlpmain} in Appendix~\ref{apx:regproof}, this term captures the error that arises from the orthogonal projection of $\what$ onto the direction of the signal $\wstar$. This error is expected to increase when adding explicitly regularization, and thus shrinking the estimator. 








==> ICML 22-3/sections/notation.tex <==


% %%%%%%%%%%%%%%%%%%%%



% \section{Notation} \label{sec:notation}
% \red{some of the notation will be moved to the appendix}

% We begin by introducing the notation used throughout the proof. 
% On the finite-dimensional space $\RR^d$, we write $\norm{\cdot}_2$ for the Euclidean norm and $\innerprod{\cdot}{\cdot}$ for the inner product.
% The $\ell_1$ and $\ell_{\infty}$-norms are denoted by $\norm{\cdot}_1$ and $\norm{\cdot}_\infty$, respectively. We denote by $\loneball{\lonebound}$ $l_1$-ball with radius $\lonebound$. $\onevec \in \RR^d$ is the vector with all components equal to $1$.
% $\NNN(\mu, \Sigma)$ is the normal distribution with mean $\mu$ and covariance $\Sigma$, $\Phi(x)$ is
% the cumulative distribution function of the scalar standard normal distribution, $\Phic(x) = 1-\Phi(x)$,
% and $\log$ denotes the natural logarithm. An arbitrary vector $v$ with all nonnegative entries we denote by $v\geq 0$. If $v$ is a vector, then we denote by $v_i$ its $i$-th component.

% The $n$ samples $x_i \in \RR^d$
% form the rows of the data matrix \mbox{$\matX = \left[ x_1 ~...~ x_n
%     \right]^\top$}, with $\matX_{ij} \sim \NNN(0,1)$ for each $i,j$.  The
% measurements $y_i \in \{\pm 1\}$ for $i=1,\dots,n$ are given by $y_i = \sign(\innerprod{x_i}{\wgt})\xi_i$ where $\wgt \in \RR^d$ is the ground truth signal and $\xi_i\in\{\pm 1\}$ is the noise distributed according to $\prob_{\xi}$. We define a diagonal matrix $\matDy \in \RR^{n\times n}$ with $(\matDy)_{i,i} = y_i$. 

% Projection operators to the space spanned by $\wgt$ and orthogonal complement are denoted by $\projpar$ and $\projperp$, respectively. For vector $w\in \RR^d$ we use notation $w=(\wone,\wtwo)$ to denote that $w$ is split into components such that $\wone = \projpar{w}$ and $\wtwo = \projperp{w}$. For the time being we assume that $\wgt$ is 1-sparse vector and without loss of generality assume that $\wgt = \left[ 1\ 0 ~...~ 0\right]^\top$. Furthermore we define $\nu = \norm{\wone}_1$ and $\eta = \norm{\wtwo}_2$.

% For vector $z=(\gausswone ,\gausswtwo)$ we define $z_{(1)} = \max_{i=1,\dots,n} \{ \abs{\gausswone_i}, \abs{\gausswtwo_i} \}$. 

% To easily keep track of the dependency on dimension and
% sample size,
% we reserve the $O(\cdot)$ notation to contain only universal constants, without any hidden dependency
% on $d$, $n$ or $\sigma^2$.





==> ICML 22-3/sections/proofidea.tex <==
\vspace{2mm}
\section{Proof Idea and Discussion of the Assumptions}
\label{sec:proofidea}
We now provide the proof sketch followed by a discussion of the assumptions in Theorem~\ref{thm:regressionlpmain} and \ref{thm:classificationlp}. 
\subsection{Proof idea}
\label{subsec:proofintuition}


The proofs of Theorem~\ref{thm:regressionlpmain} and \ref{thm:classificationlp} follow a localized uniform convergence argument which is standard in the literature on empirical risk minimization. More specifically, we first upper bound the $\ell_p$-norm of the interpolators by 
%\vspace{-0.1in}
\begin{equation}
     \min_{ \forall i:\:\langle \xui , w\rangle =y_i } \norm{w}_p^p  \leq \loneboundreg~~\mathrm{and}  \min_{\forall i:\:\yui \langle x, w \rangle \geq 1} \norm{w}_p^p   \leq \loneboundclas.
\end{equation}
%\vspace{-0.1in}
In a second step, we uniformly bound the risk over all interpolating models with $\loneboundreg$/$\loneboundclas$-bounded $\ell_p$-norm
\ifarxiv
\begin{align}
    \RiskR(\what) &\leq  \max_{\substack{\norm{w}_p^p \leq \loneboundreg \\ \forall i:\:\langle \xui , w\rangle =\yui}} \norm{w - \wgt}_2^2 =: \Phi_{\mathcal{R}} %\label{eq:proofideareg} 
    ~~\mathrm{and}~~
    \RiskC(\what)\leq 2 - 2 \underbrace{\left[
    %\frac{1}{2} - \frac{1}{2} \Risk(\what) &\geq  
    \min_{\substack{\norm{w}_p^p \leq \loneboundclas\\ 
    \forall i:\:\yui \langle x_i, w \rangle \geq 1}}
    \frac{\langle w, \wgt\rangle}{\norm{w}_2} \right]}_{=: \Phi_{\mathcal{C}}}. %\label{eq:proofideaclas}
\end{align}
\else
\begin{align}
    \RiskR(\what) &\leq  \max_{\substack{\norm{w}_p^p \leq \loneboundreg \\ \forall i:~\langle \xui , w\rangle =\yui}} \norm{w - \wgt}_2^2 =: \Phi_{\mathcal{R}} \label{eq:proofideareg} 
        \\
    \RiskC(\what) &\leq 2 - 2 \underbrace{\left[
    %\frac{1}{2} - \frac{1}{2} \Risk(\what) &\geq  
    \min_{\substack{\norm{w}_p^p \leq \loneboundclas~~\mathrm{and} \\ 
    \forall i:~ \yui \langle x_i, w \rangle \geq 1}}
    \frac{\langle w, \wgt\rangle}{\norm{w}_2} \right]}_{=: \Phi_{\mathcal{C}}}. \label{eq:proofideaclas}
\end{align}
\fi
We now only discuss the uniform convergence argument as the localization step to upper bound $\loneboundreg$ and $\loneboundclas$ follows from a similar argument. 

The proof exploits the assumption that the ground truth is $1$-sparse (the extension to $s$-sparse ground truths is discussed in Appendix~\ref{rm:p}).  We decompose $w = (\wone, \wtwo)$, with $\wone$ the first entry of $w$ (since $\wgt = (1,0,\cdots,0)$), and abbreviate $\eta = \norm{\wtwo}_2$. Furthermore,  we define $\nu = (w -\wgt)_{[1]} = \wone -1$  for regression and $\nu = \wone$  for classification. Define \vspace{-5mm}

\ifarxiv
\begin{align}
         &\phi_{\mathcal{R}} := \max_{(\nu,\eta) \in \Omegareg} \nu^2 +\eta^2
         \leq \max_{\nu \in \Omegareg}~\nu^2 + \max_{\eta \in \Omegareg}~\eta^2  \\\nonumber 
         \mathrm{and}~~
 &\phi_{\mathcal{C}} :=\min_{ (\nu,\eta) \in \Omegaclas} \frac{\nu }{\sqrt{\nu^2+\eta^2}} \geq \left(1 + \frac{\max_{\eta \in \Omegaclas} ~\eta^2}{\min_{\nu \in \Omegaclas}~ \nu^2}  \right)^{-1/2} \label{eq:phimlpv1main} \, ,
    \end{align}
    \else
\begin{align}
         &\phi_{\mathcal{R}} := \max_{(\nu,\eta) \in \Omegareg} \nu^2 +\eta^2
         \leq \max_{\nu \in \Omegareg}~\nu^2 + \max_{\eta \in \Omegareg}~\eta^2  \nonumber \\
 &\phi_{\mathcal{C}} :=\min_{ (\nu,\eta) \in \Omegaclas} \frac{\nu }{\sqrt{\nu^2+\eta^2}} \geq \left(1 + \frac{\max_{\eta \in \Omegaclas} ~\eta^2}{\min_{\nu \in \Omegaclas}~ \nu^2}  \right)^{-1/2} \label{eq:phimlpv1main} \, ,
    \end{align}
\fi
with constraint sets 
\ifarxiv
\begin{multline}%\label{eq:omegareg}
    \Omegareg = 
    \bigg\{(\nu, \eta) \:\vert \:\exists b>0 \subjto (1+\nu)^p + b^p \leq \loneboundreg \text{ and}~
    \frac{1}{n}\norm{H}_q^2 b^2  \geq \frac{1}{n}\sumin \left( \xi_i - Z_i \nu  - \tilde{Z}_i \eta\right)^2 \bigg\} \, ,
\end{multline}
\else
\begin{multline}%\label{eq:omegareg}
    \Omegareg = 
    \bigg\{(\nu, \eta) \:\vert \:\exists b>0 \subjto (1+\nu)^p + b^p \leq \loneboundreg \text{ and} \\
    \frac{1}{n}\norm{H}_q^2 b^2  \geq \frac{1}{n}\sumin \left( \xi_i - Z_i \nu  - \tilde{Z}_i \eta\right)^2 \bigg\} \, ,
\end{multline}
\fi
and
\ifarxiv
\begin{multline}\label{eq:omegaclas}
    \Omegaclas = 
    \bigg\{(\nu, \eta) \:\vert\: \exists b>0 \subjto \nu^p + b^p \leq \loneboundclas \text{ and }
      \frac{1}{n}\norm{H}_q^2 b^2  \geq    \frac{1}{n}\sumin \possq{1-\xi_i \vert Z_i\vert \nu  + \tilde{Z}_i \eta} \bigg\} \, ,
\end{multline}
\else 
\begin{multline}\label{eq:omegaclas}
    \Omegaclas = 
    \bigg\{(\nu, \eta) \:\vert\: \exists b>0 \subjto \nu^p + b^p \leq \loneboundclas \text{ and } \\
      \frac{1}{n}\norm{H}_q^2 b^2  \geq    \frac{1}{n}\sumin \possq{1-\xi_i \vert Z_i\vert \nu  + \tilde{Z}_i \eta} \bigg\} \, ,
\end{multline}
\fi
where ${(\cdot)_+ = \max(0,\cdot)}$ and  $H,Z, \tilde{Z}$ are \iid~ Gaussian random vectors.

The key ingredient for the proofs is now that via the (Convex) Gaussian Minimax Theorem (C)GMT \cite{thrampoulidis2015regularized,gordon1988milman},
we can show that $\prob(\Phi_{\mathcal{R}} > t \vert \xi, X') \leq 2 \prob(\phi_{\mathcal{R}}\geq t \vert \xi, X' )$ and $\prob(\Phi_{\mathcal{C}} < t \vert \xi, X') \leq 2 \prob(\phi_{\mathcal{C}} \leq t\vert \xi, X')$ with $X'$ being the subset of features $X$ in the direction of the ground truth. In short, high probability upper and lower bounds for $\phi_{\mathcal{R}}$ and $\phi_{\mathcal{C}}$, yield corresponding high probability bounds for $\Phi_{\mathcal{R}} $ and $\Phi_{\mathcal{C}}$. The (C)GMT has been used previously to obtain similar bounds for regression in \cite{koehler2021uniform,wang2021tight}.

The result can then be obtained by 
carefully bounding the constraint sets $\Omegaclas$ and $\Omegareg$ 
using tight concentration inequalities for the $\ell_q$-norm of \iid~Gaussian random vectors in \cite{paouris_2017}. 


\vspace{4mm}
\subsection{Limitations and discussion of the assumptions}
\label{rm:p}
In the following subsections, we  now discuss the assumptions of our main results and how they can be generalized. 

\label{apx:remarks}
\paragraph{Assumption on  $p~ \&~ d$}
While for very large $d$, Theorems~\ref{thm:regressionlpmain} and \ref{thm:classificationlp} hold for most $p\in(1,2)$, even close to $1$, for fixed $n,d$ our theorems apply to the range $p\in \left(1+\frac{\kappa_2}{\log\log d},2\right)$.
This assumption is used to obtain a high probability concentration of the dual norm $\norm{H}_q$ in Lemma~\ref{lm:dualnormconc}.
It is possible and straightforward to relax the assumption on $p$ to allow for smaller $p$, such as  $p \in (1+\frac{\kappa \log \log d}{\log d},2)$, by choosing $\epsilon(n,d)$ in Lemma~\ref{lm:dualnormconc} larger. However, this choice comes at the price of non-matching upper and lower bounds. In fact, when choosing $p =  1 + \frac{\kappa}{\log d}$, the $\ell_q$-norm $\norm{H}_q$ behaves similarly as the $\ell_{\infty}$-norm $\norm{H}_\infty$ (see \cite{paouris_2017}).






\paragraph{Assumption on the sparsity of $\wgt$}
In this paper we study the special case where the ground truth is  $1$-sparse and thus aligns "maximally" with the sparse inductive bias of the $\ell_1$-norm. 
Precisely, choosing a $1$-sparse ground truth significantly simplifies the analysis 
(see Section~\ref{sec:proofidea}) and the  presentation of the bounds in Theorem~\ref{thm:regressionlpmain} and \ref{thm:classificationlp}. However, the application of the (C)GMT in Propositions~\ref{prop:CGMT_applicationreg} and \ref{prop:CGMT_application_classification} holds more generally for $s$-sparse ground truths and even non-sparse ground truths as exploited in \cite{koehler2021uniform}. 
Therefore, the proof methodology presented in this paper can 
also be employed to bound the risk of general $s$-sparse ground truths. However, this would come at the cost of more involved theorems statements, and non-tight upper and lower bounds in $s$. 


\paragraph{Assumption on the noise}
Theorems~\ref{thm:regressionlpmain} and \ref{thm:classificationlp} assume that the amount of noise $\sigma$ is fixed and non-vanishing as $n\to\infty$.
This setting is of particular interest as the ground truth is still consistently learnable (unlike in settings where the noise dominates), while the noise prevents  the min-$\ell_1$-norm/max-$\ell_1$-margin interpolators from generalizing well.  In fact, we are the first to prove, for a constant noise setting, that we can consistently learn with min-norm/max-margin interpolators at fast rates.

On the other hand, several works including \cite{chinot_2021,chinot2021adaboost,wojtaszczyk_2010} have also studied the low noise regime where $\sigma\to 0$  as $n,d$ tend to infinity. We remark that  our proof of Theorem~\ref{thm:regressionlpmain} can be directly extended to cover vanishing noise for regression.  On the other hand, the methodology used for the classification results, i.e. Theorem~\ref{thm:classificationlp}, strongly relies on the noise model and we leave the extension of our results to low noise settings (i.e. vanishing fraction of flipped labels)  as an interesting future work. 


\paragraph{Assumption on the distribution of the features}
Our proofs strongly rely on the (C)GMT (Propositions~\ref{prop:CGMT_applicationreg} and \ref{prop:CGMT_application_classification}), which crucially hinges on the assumption that the input features are Gaussian. We believe that generalizing the input distribution $\prob_X$ requires the development of novel tools -- an important task for future work. 
For instance, the small-ball method that is known to yield tight bounds for general input distributions for many estimators  \cite{mendelson_2014, koltchinskii_2015} results in loose bounds when applied directly (\cite{chinot_2021}, see also the discussion on this topic in \cite{wang2021tight}). It remains to be seen whether a modified technique based on the small-ball method can be  powerful enough to yield tight bounds for min-norm/max-margin interpolators studied in this paper.





 %which boils down to bounding the constraint sets $\Omegaclas$ and $\Omegareg$. 
%This \fy{constitutes} the bulk of the proof and essentially relies on a carful analysis using tight concentration inequalities for the $\ell_p$-norm of \iid~Gaussian random vectors in \cite{paouris_2017}. 

%  the problem to the one of bounding the set $\Omega$. Combining the two inequalities in the constraint set $\Omega$, we obtain the following inequality which allows us to bound $\nu,\eta$,


% Finally we want to note that simply bounding the risk of the max-$\ell_1$-margin interpolator in Theorem~\ref{thm:mainl1} based on Equation~\eqref{eq:omegaclas} leads to loose bounds. Instead, the proof technique, inspired by \cite{wang2021tight}, is more involved and specifically tailored to the $\ell_1$-norm.
%and is , where the authors derive bounds for risk of the related minimum-$\ell_1$-norm interpolator for regression.








%  Inspired by \cite{koehler2021uniform}, an elementary ingredient for the proof is the application of the (Convex) Gaussian Minimax Theorem due to \cite{thrampoulidis2015regularized,gordon1988milman}. We refer to Appendix~\ref{apx:subsec:gmtreg} for a detailed description of the application of the (C)GMT and refer to Remark~\ref{rm:koehler} in Appendix~\ref{apx:regproof} for a comparison with the proofs in \cite{koehler2021uniform}. 
% % However, in order to obtain tight bounds a more refined analysis is required than the one presented by \cite{koehler2021uniform}, relying on specific concentration inequalities for the $\ell_p$-norm of Gaussian random vectors \red{cite}. Furthermore, the analysis used to prove Theorem~4~\cite{koehler2021uniform} uses the concentration of $\frac{1}{n} \norm{\xi}_2^2$ around $\sigma^2$, which explains the dependency on the term $\frac{1}{\sqrt{n}}$ in the upper bounds. Instead, to avoid this term, our upper bound for the $\ell_p$-norm $\norm{\what}_p^p \leq B$ explicitly depends on  $\xi$.
% % Similar to \red{Thrompolidis}, we make use of the CGMT, and using the fact that the ground truth is

% We only discuss the uniform convergence upper bound as the lower bound and the upper bound for the norm $\norm{\what}_p^p$ follow from the same idea. 
% As an implication of the (C)GMT we first show that  we can instead bound the expression
% % \begin{align}
% %     \tag{$A_+$} \label{eq:phip}
% %         \phidp \leq  \max_{\eta\geq 0 ,b\geq 0, \nu} \frac{\nu }{\sqrt{\nu^2+\eta^2}} 
% %         \subjto \begin{cases}
% %             \frac{1}{n} \norm{H}_q^2 b^2 \geq  \fn(\nu,\eta)\\
% %           \vert \nu \vert^p+b^p \leq M
% %         \end{cases}\\
% %     \tag{$A_-$} \label{eq:phim}
% %         \phidm \geq \min_{\eta\geq 0 ,b\geq 0, \nu} \frac{\nu }{\sqrt{\nu^2+\eta^2}} 
% %         \subjto \begin{cases}
% %     \frac{1}{n} \norm{H}_q^2 b^2 \geq  \fn(\nu,\eta)\\                     \vert \nu \vert+b^p \leq M
% %         \end{cases}
% %     \end{align}


%  %Similarly, we can also obtain a lower bound for the risk when bounding $ \min_{\eta\geq 0 ,b\geq 0, \nu} \nu^2 +\eta^2
%  %       \subjto (\nu,\eta) \in \Omega \geq \min_{\nu \in \Omega}~\nu^2$.
%  As a consequence, we reduced the problem to the one of bounding the set $\Omega$. Combining the two inequalities in the constraint set $\Omega$, we obtain the following inequality which allows us to bound $\nu,\eta$,
%   \begin{align}
%           &\frac{1}{n} b^2 \norm{H}_q^2  
%           =  \frac{1}{n} \norm{H}_q^2 \left(\lonebound - (\nu+\nugt)^p \right)^{2/p} \nonumber \\
%           &~~\approx \frac{1}{n}  \norm{H}_q^2 \lonebound^{2/p}\left(1 -\frac{2}{\lonebound} \left(\frac{1}{p} + \nu\right) \right)   \geq f_n(\nu, \eta).
%           \label{eq:proofideareg2}
% \end{align}
% In order to obtain bounds for $\nu,\eta$, we use an approximation for $\fn$ of the form $ \fn(\nu, \eta) \approx \sigmaxi^2 + \nu^2 +\eta^2$ with $\sigmaxi^2 = \frac{1}{n} \|\xi\|_2^2$ and use concentration inequalities for $\|H\|_q$ from \cite{paouris2017random}. 
% Finally, denote with $O_c = O(t_2^2 + t_1 t_2 + t_1^2\frac{1}{\log(d)})$ with $t_1,t_2$ form Theorem~\ref{thm:regressionlpmain}. In summary, we show the following bounds for $\nu,\eta$ which result in the desired bound in Equation~\eqref{eq:thmregboundhighnoiseuppermain}: $\label{eq:proofintuition1}
%     \vert \nu - t_1\vert^2 = O_c$ and $\eta^2 = O_c.$



% \label{subsec:claproof}
% The proofs for Theorem~\ref{thm:mainl1} and Theorem~\ref{thm:classificationlp} are again based on a localization-uniform convergence argument, where we first upper bound 
% $ \min_w \norm{w}_p^p \subjto \min_i \yui \langle x, w \rangle \geq 1 =: \Phi_N\leq B$. In a second step, we then upper/lower bound the term $\frac{\langle \wgt, w \rangle}{\|w\|_2}$  uniformly over all vectors $w$ with ${\min_i \yui \langle x_i, w\rangle \geq 1}$ and $\norm{w}_p^p$, which then gives us bounds for the risk when using that $\norm{\frac{w}{\norm{w}_2} - \wgt}_2^2 = 2 - 2\frac{\langle \wgt, w \rangle}{\|w\|_2}$.
% Following a similar idea as in \cite{deng21}, we can also apply (C)GMT in the classification setting. In fact, we can again show that we obtain valid bounds for the risk when bounding
% \begin{align}
%         &\min_{\eta\geq 0 ,b\geq 0, \nu} \frac{\nu }{\sqrt{\nu^2+\eta^2}} 
%                 \subjto (\nu,\eta) \in \Omega 
%                 \\&\geq \left(1 + \frac{\max_{\eta \in \Omega} ~\eta^2}{\min_{\nu \in \Omega}~ \nu^2}  \right)^{-1/2} \label{eq:phimlpv1main}
% \end{align}
%  with $\Omega = \{ (\nu, \eta)\vert  \frac{1}{n} \norm{H}_q^2 b^2  \geq  f_n(\nu, \eta) ~~\mathrm{and}~~ \nu^p + b^p \leq M \}$. 
%  Here, $\fn(x,y)= $ and $H,Z, \tilde{Z}$ are again \iid~ Gaussian random vectors.   A similar result also applies for the  the upper bounds on $B$ and $\frac{\langle \wgt, w \rangle}{\|w\|_2}$. 

% As a consequence, we see that there is a strong analogy between classification and regression. In order to apply the same analysis as used for the proof of Theorem~\ref{thm:regressionlpmain}, the key challenge here is to control the function $\fn(x,y)$. For the moment, assume that $\fn(x,y) \approx \EE \fn(x,y) = f(x,y)$ with $f$ from Section~\ref{subsec:clasetting}. By the Taylor series approximation,  we have $\fn(x,y) \approx \fnstar + \fnnstar \eta^2 + \fetaeta \deltanu^2$ with $\nubar = \nu - \nubar$ and $\nubar$ form Assumption A1.  Yet, the resulting bound would involve a term depending on $\frac{1}{n^{1/4}}$ and thus prevent rates close to the minmax optimal risk. Instead, in order to obtain the tighter bounds in Theorem~\ref{thm:classificationlp}, more refined bounds for $\fn$ are needed  which do not rely on the concentration of $\fn$ around $f$ (see Appendix~\ref{apx:subsec:prooffnlp}). 
 
   

 

==> ICML 22-3/sections/relatedwork.tex <==

% \section{Related work} 
% %We now summarize the related work.
% \paragraph{Max-margin/min-norm interpolation}
% % So far, the majority of papers focus on models which are invariant under rotations of the input features, including linear and logistic regression \cite{muthukumar_2020,muthukumar2021classification,hastie2019surprises,bartlett_2020,tsigler_2020,Dobriban15}, random feature models \cite{mei_2019} and rotational kernel methods \cite{ghorbani_2021}. 
% % As shown in the literature, these models benefit from a regularizing effect due to overparameterization (i.e., $d\gg n$ for linear models), which allows them to achieve consistency assuming that the data has some underlying spiked covariance matrix structure. However, such models do not incorporate any structural assumptions of the ground truth and therefore suffer from a bias issue when the features are inherently high dimensional \cite{ghorbani_2021,donhauser21}.

% %  On the other hand, the theoretical understanding of interpolating models with structural biases is much less developed. Notably, recent work shows that the min-$\ell_1$-norm interpolator (basis pursuit) \cite{wang2021tight} achieves consistency on isotropic (and thus inherently high-dimensional) input features when $d \gg n$. However, the estimator is highly sensitive to noise in the training data (see also \cite{muthukumar_2020}) and therefore the risk vanishes at very slow rates compared to its regularized variant LASSO \cite{tibshirani_1996}. \red{say more here}
 
 
 
 
 
%  The majority of papers that attempt to rigorously understand minimum-norm interpolation from a non-asymptotic viewpoint have so far
% %"positive" results for min-norm interpolation so far 
% centered around norms that are rotationally invariant, such as $\ell_2$ (e.g., \cite{bartlett_2020,muthukumar_2020,muthukumar2021classification,Dobriban15} and references therein). In particular, this line of work has formalized the intuition that for such norms high dimensionality, i.e. the regime where $d \gg n$, has a \emph{regularizing} effect on the variance of the interpolator. At the same time however, rotationally invariant norms do not encourage low-dimensional structure but uniform shrinkage - this leads to problems for the model's bias\footnote{to be distinguished from the inductive bias} in exactly these relevant high-dimensional regimes, even when the ground truth itself is structured. 
% %Either you learn nothing (polynomial or zero function), or 
% As an instance, for min-$\ell_2$-norm interpolation to be asymptotically consistent as $d,n\to\infty$, the covariates need to be effectively low-dimensional and aligned with the direction of the ground truth (via a spiked covariance structure, e.g., see \cite{bartlett_2020,muthukumar_2020,muthukumar2021classification} and references therein). 
% Albeit realistic in settings where prior knowledge allows for feature selection, this assumption is not apt to model scientific applications, such as genetics, where inherently high-dimensional measurements naturally arise.
% For high-dimensional isotropic Gaussians for example, minimum RKHS or $\ell_2$ norm interpolators are \emph{inconsistent} 
% %unless the ground truth is the zero function or low-degree polynomials 
% \cite{tsigler_2020,muthukumar_2020}. As this inconsistency 
% %persists in 
% carries over to the noiseless case, we refer to it as a "bias issue". 

% On the other hand, the existing literature on structured interpolators is much more limited. So far, the majority of non-asymptotic results are for the min-$\ell_1$-norm interpolation \cite{wang2021tight,muthukumar_2020,chinot_2021,wojtaszczyk_2010,chatterji_2021}. In particular, in \cite{wang2021tight} the authors recently proved the exact rate of order  $\frac{\sigma^2}{\log(d/n)}$ for the interpolator assuming \iid~Gaussian features. 
% Note that this rate  is very slow -- $1/\log(d/n)$ compared to regularized estimators $\log(d)/n$.
% Further, recent work \cite{chinot2021adaboost} also derives non-asymptotic bounds for the max-$\ell_1$-margin, although for the more general case where the noise is also allowed to be adversarial. Finally, the papers \cite{chinot_2021,koehler2021uniform} present frameworks to obtain non-asymptotic bounds for general min-norm interpolators. 

% Finally, there is also a substantial line of research which studies interpolating models form an asymptotic view point. The majority of in this field papers study regimes where the risk does not vanish as $d,n \to \infty$ and give precise characterisations of the asymptotic risk (e.g., see \cite{hastie2019surprises, dobriban_2018,deng21} and references therein; see also \cite{mei_2019} for non-linear examples). Furthermore, several papers also show asymptotic consistency of kernel methods when $d,n \to \infty$ in a fixed regime where $d \asymp n$ \cite{Ghorbani2020b, ghorbani_2021,misiakiewicz2021learning,donhauser21}. While this type of research gives important insights on what sorts of functions can be learned consistently, the literature does not provide the rate (note that \cite{misiakiewicz2021learning} only gives rates for the regularized case). 




% % As a solution, one might think that a strong inductive bias such as the one of minimum $\ell_1$-norm interpolators could
% % resolve inconsistency for sparse ground truths, as it yields minimax optimal rates in regularized regression (e.g., studied in \cite{wang2021tight,chinot_2021,koehler2021uniform,muthukumar_2020,chinot2021adaboost}). 
% % %A natural alternative instead is to study \fy{rather, use} interpolators with strong inductive bias such as the min-$\ell_1$-interpolator -- with $\ell_1$ being an inductive bias that achieves minimax optimal rates in regularized regression. 
% % Indeed, recent work has  proven consistency for isotropic Gaussians and sparse ground truth \cite{wang2021tight},
% % %and hence improves upon min-$\ell_2$-norm interpolation, 
% % but the rates are still very slow -- $1/\log(n)$ compared to regularized estimators $1/n$.
% % %\fy{sentence too long, but along those lines} The reason why this strong inductive leads to poor performance for interpolation, 
% % Despite being optimal for regularization, a major caveat of this strong inductive bias is the higher sensitivity to perfect noise-fitting.
% % %has a major caveat when forced to fit noise seems to be that enforcing the fitting of noise is much more detrimental for estimators with strong inductive bias towards low-dim structure rather than uniform shrinkage. 
% % In summary, the strength of the inductive bias seems to induce a trade-off between the effect of noise in the training data and the ability to recover noiseless signal.
% % %Intuitively hence, uniform shrinkage \fy{i wouldn't say this has no structure, cause what would you translate that to for general overparam models?}
 
 
 


% \paragraph{Implicit bias of gradient descent}
% Recent literature studies the norm and margin properties of models trained with gradient descent. Specifically, several papers show that gradient descent methods converge to solutions with various minimum norm and maximum margin properties \cite{chizat2020implicit,telgarsky_13,soudry18, Lyu2020Gradient, stochastimirrordescent21, oymak2019overparameterized, montanari2019generalization}. 
% This phenomenon, named \emph{implicit bias of gradient descent}, displays the importance of optimization in determining the structural bias of various parametric models. The connection between the weight space and function space of such models is still unclear \cite{parhi2021kinds}, and it is in fact debated whether neural networks' generalization properties can be explained via norm arguments \cite{neyshaburexploring, jiang2019fantastic}.
% % The literature is yet inconclusive on the interplay between optimization, input data, and structural properties of neural networks, such as depth, width, batch normalization, and skip connections, to name a few. 
% % Moreover, there are no formal definitions of structural bias for neural networks. We believe this is an open and interesting avenue for future research.





==> ICML 22-3/sections/tradeoff_future_work.tex <==



% \kd{this section is entirely garbage so far, needs to be done!}

% \begin{itemize}
%     \item So what do we want to discuss here?
%     \item Future work on Lp - here we can have several things; generalize assumptions, talk about the small ball property for the features; talk about the tradeoff, i.e. regularized version; what is the optimal p ?
%     \item Rethinking inductive bias  - this is the general perspective on it; experimentall and theoretically
% \end{itemize}

% In this section, we give an intuitive explanation for why the optimal performance is achieved for $p\in(1,2)$. Furthermore, we discuss the implications of our results in a broader scope and motivate future work.

% Yet, in order to better understand this trade-off, we motivate future work on  linear min-norm/max-margin interpolators to explore formal definitions for the inductive bias (similarly to concept of the bias of an estimator) and the sensitivity to noise (similarly to concept of the variance of an estimator) and show how  they appear in the non-asymptotic bounds. 
% fomrlaize
% Yet, a solid theoretical understanding for this trade-off is left as an avenue for future work. 
% In particular, we motivate future work on to extend the scope of our results and to establish a matching upper and lower bounds capturing the optimal inductive bias depending on the noise of the training data. Furthermore, we motivate future theoretical work  to give evidence for the existence of the trade-off beyond linear models. 
% not developed. Wand motivated as a future work. In particular, 
% understood and we motivate future work to 
% Lay ground for a solid theoretical foundataion for minimum-norm interpolators
% Explore its generality and beyond linear models and give theoretical evidence for its existence for non-linear models
% L1 and L2 perform bad but due to different reasons. -l1 noise, l2 bias (holds both for classification and regression).
% In particular, we observed that for p in (1,2) we achieve faster rates, which suggests a trade-off: 
% When increasing the strength of the inductive bias the estimator can better recover noiseless signals but becomes more sensitive to noise in the training data. The optimal performance for the noisy setting is obtained when both terms trade-off and thus for a moderate strenght of the inductive bias. 
% This is also suggested by our Theorem as discussed in the theory section (see the paragraph interpretation of the terms). 


% This conclusion is also suggested by empirical observations where increasing the depth of the network (which can be vaguely understood as a measure for the inductive bias, e.g., see \cite{gunasekar2018implicit, parhi2021kinds, ergen2021revealing, Tibshirani2021EquivalencesBS} \red{are these ok?}) leads to an increase in the variance. \kd{replace by nicolos experiment if we get anything} However the scope of these experiments is rather limited as for instance the hyperparameters remain unchanged for all depths.
% We believe that a crucial ingredient why certain generalize well albeit interpolating noisy data is because when training until convergence, their implicit bias tradesoff inductive bias matching the structure of the  ground truth with the regularizing effect of overparametrization.
% In particular, we conjecture that also for neural networks and other complex non-linear interpolators, in the presence of noise, less inductive bias can lead to better performance. 
% This conclusion is also suggested by empirical observations where increasing the depth of the network (which can be vaguely understood as a measure for the inductive bias, e.g., see \red{would cite some papers here}) leads to an increase in the variance. \red{replace by nicolos experiment if we get anything} However the scope of these experiments is rather limited as for instance the hyperparameters remain unchanged for all depths. We leave more conclusive empirical and theoretical work on this for important future work. 

\vspace{1.5mm}
\section{Related Work}
The majority of works that attempt to rigorously understand minimum-norm/max-margin interpolation from a non-asymptotic viewpoint have so far
focused on $\ell_2$-norm interpolators, \cite{bartlett_2020,tsigler_2020,muthukumar_2020}.
However, to be asymptotically consistent as $d,n\to\infty$,  the covariates need to be effectively low-dimensional and aligned with the direction of the ground truth, e.g.~via a spiked covariance structure. 

On the other hand, the existing literature on structured interpolators primarily focuses on the min-$\ell_1$-norm interpolator \cite{wang2021tight,muthukumar_2020,chinot_2021,wojtaszczyk_2010,chatterji_2021}, showing exact rates of order $\frac{1}{\log(d/n)}$. Even though  \cite{koehler2021uniform,zhou2021optimistic,chinot_2021} present frameworks to obtain non-asymptotic bounds for general min-norm interpolators, the discussion of the implications of their results center around the  
$\ell_1$/$\ell_2$-norms.
For classification, so far the only known non-asymptotic upper bound holds for the max-$\ell_1$-margin interpolator --- however, assuming that a constant fraction of data points are mislabeled, the upper bound diverges with growing sample size  \cite{chinot2021adaboost}. %\nr{Unclear here. Do you mean that DESPITE assuming constant noise they hvae diverging bounds?}

Beyond the mentioned non-asymptotic results, many more papers study linear regression and classification in the limit as $d,n \to \infty$ \cite{muthukumar2021classification, hastie2019surprises, dobriban_2018,deng21,li2021minimum}.
In contrast to this paper, these works study the linear regime where ${d/n \to \gamma>0}$ and thus where the errors of interpolators do not vanish. 



%Further, many papers study the asymptotic setting where $d,n \to \infty$ and characterize the regimes where the risk asymptotically vanishes \cite{muthukumar2021classification} or give precise characterisations of the asymptotic risk in various regimes where the risk does not vanish (e.g., see \cite{hastie2019surprises, dobriban_2018,deng21}). \fy{yuting?} 
%  These   results can only distinguish between asymptotic consistency and inconsistency but  do not capture the rates at which the (directional) estimation error vanishes - which is needed to study the superiority of the interpolator with $p\in(1,2)$ compared to $p=1$. 
 
 
 
\vspace{1.5mm}
\section{Generality and Future Work}
\label{sec:trade-off}
Our results naturally suggests a variety of impactful follow-up work that may advance the understanding of the effect of inductive bias and interpolation both from a theoretical and empirical perspective. 


\subsection{Future  Work on Theory for Linear Interpolators}
%\texorpdfstring{$\ell_p$}{lp}-norm interpolators}
\label{subsec:optimalp}
As a specific question for future work, a natural quantity of interest would be the optimal choice  among all $p \in (1,2)$ as a function of  $n,d$. 
Unfortunately, our presented bounds are not sufficient to provide an explicit answer.
Note that for $\beta <2$ and $p = 1 +\frac{\kappa_2}{ \log \log d}$, our rates match the uniform lower bounds for all interpolators when $n,d$ are sufficiently large. 
On the other hand, for larger $\beta$, the optimum of the upper bound is achieved at $p< 1 + \frac{\kappa_2}{\log \log d}$
which is beyond the range of our analysis. We refer to Section~\ref{rm:p} for a discussion on smaller choices of $p$. 
Giving a precise expression and tight lower bounds supporting the choice remains a challenging task. 




% As a specific research question for future work,  min-$\ell_p$-norm  and max-$\ell_p$-margin, anatural quantity of interest would be the optimal choice  among all $p \in (1,2)$ as a function of  $n,d$.
% Unfortunately, our bounds are not sufficient to provide an explicit answer.
% Note that for $\beta <2$ and $p = 1 +\frac{\kappa_2}{ \log \log d}$, our rates match the uniform lower bounds for all interpolators. 
% On the other hand, for larger $\beta$, the optimum of the upper bound is achieved at $p< 1 + \frac{1}{\log \log d}$
% which is beyond the range of our analysis. We refer to Section~\ref{rm:p} for a discussion on potential extensions of our results to smaller choices of $p$. 
% Giving a precise expression and tight lower bounds supporting the choice remains a challenging task for future work. 
% We believe that addressing this question is important
% to gain deeper understanding of the trade-off 
% and crucial to generalize our findings beyond linear models. 


%\vspace{-0.1in}
% \paragraph{Explicit expressions for the trade-off}
% Aiming to gain a better understanding of the trade-off, also beyond min-$\ell_p$-norm and max-$\ell_p$-margin interpolators, we motivate future work to formalize the trade-off induced by the inductive bias. 
% Importantly, it is unclear how the bias and variance terms relate to the terms appearing in the upper bounds in Theorems~\ref{thm:regressionlpmain} and \ref{thm:classificationlp}. Contributions in this direction may also lay the foundations for novel experimental settings which allow better understanding of the effect of inductive biases in interpolating models used in practice.





% We motivate future work to formalize the trade-off induced by the inductive bias. Importantly, it is unclear how the bias and variance terms relate to the terms appearing in the upper bounds in Theorems~\ref{thm:regressionlpmain} and \ref{thm:classificationlp}. Contributions in this direction may also lay the foundations for novel experimental settings which allow better understanding of the effect of inductive biases in interpolating models used in practice.


\begin{figure}[!t]
    \centering
    \ifarxiv
    \includegraphics[width=.5\linewidth]{figures/cntk_depth_vs_risk.pdf}
    \else
    \includegraphics[width=\linewidth]{figures/cntk_depth_vs_risk.pdf}
    \fi
    \caption{Classification with convolutional neural tangent kernels on binarized MNIST. We plot the $0-1$~classification error on the test set as a function of the depth of the model, i.e. the number of stacked convolutional layers with ReLU activation. Means and confidence bands are computed across 50 independent draws of the training set with $n =500$. \vspace{-4mm}}
    \label{fig:cntk}
\end{figure}

\subsection{Non-linear Overparameterized Interpolators}
%{Rethinking the role of inductive bias in interpolation for non-linear models (NN)}

The discussion in Section~\ref{sec:discussion} suggests that
good generalization of interpolating models in the noisy case hinges on a careful choice of the inductive bias and that stronger is not automatically better, as is  perhaps widely assumed.
This stands in contrast to regularized models and noiseless interpolation, where  the best performance is usually attained at the strongest inductive bias with the right amount of regularization. 
One analogous conclusion is that the optimal inductive bias for \emph{noiseless} interpolation may not be optimal for \emph{noisy} interpolation, in particular for small sample sizes. % regime.
 
As a step towards more complex non-linear models, we provide experimental evidence to support our claim on convolutional neural tangent kernels \cite{cntk}. Kernel regression with kernels with convolutional filter structure has shown good performance on real world image datasets  \cite{lee2020} and is thus a good candidate to move towards state-of-the-art models. 
In Figure~\ref{fig:cntk}, we plot the test error as a function of the depth in a binary classification task on the MNIST data for a  small sample size regime (see Appendix~\ref{appendixsec:cntk} for the experimental details).  
When we do not add artificial label noise in the training data, we observe how increasing the depth leads to a monotonic increase in error, suggesting that the inductive bias decreases with depth. However, when adding label noise, the optimal performance is attained at a medium depth and hence a moderate  inductive bias.
These findings suggest a promising avenue for empirical and theoretical investigations evolving around the new bias variance trade-off. 


% \subsection{Future work on \texorpdfstring{$\ell_p$}{lp}-norm regularized estimators}
% Finally, it would be interesting to study how the rates in Theorem~\ref{thm:regressionlpmain} compare to the rates of optimally $\ell_p$-norm regularized estimators. 
% We are only aware of existing bounds in the literature for general non-sparse ground truths (e.g. see \cite{lecue17}). 
% As a consequence, these bounds are at least of order $\|\wgt\|_p \frac{d^{2 - 2/p}}{n}$ (see Theorem 5.4 in  \cite{lecue17}), and thus, for some choices of $\beta$, slower than the bounds for the corresponding interpolating estimator in Theorem~\ref{thm:regressionlpmain}, assuming that the ground truth is sparse. 




% Existing bounds for general non-sparse ground truths are at least of order $\|\wgt\|_p \frac{d^{2 - 2/p}}{n}$ (see Theorem 5.4 in  \cite{lecue17}), and thus, for some choices of $\beta$, slower than the bounds for the corresponding interpolating estimator in Theorem~\ref{thm:regressionlpmain} assuming that the ground truth is sparse!
%This strongly suggests that one can tighten the upper bounds of regularized $\ell_p$ norm estimators. 
% One direct avenue of future work is hence
% to investigate whether our in our theoretical results  can be generalized (see Remark~\ref{rm:sparsity}-\ref{rm:gaussian} in Appendix~\ref{apx:remarks} for a detailed discussion) to show faster rates compared to the corresponding interpolators. 
% %We hypothesize that the rate $\frac{\sigma^{4-2p}d^{2p-2}}{n}$ in the upper bound in Equation~\eqref{eq:thmregboundhighnoiseuppermain} is also optimal for $\ell_p$-regularized estimators when $\wgt $ is sparse and motivate future work on this. 
% In particular, we hypothesize that the order terms $\frac{q^{p}d^{2p-2}}{n^{p} }$ and  $\frac{\log^{\kappa_5}(d)}{n}\lor\frac{q^{\frac{3}{2}p}d^{3p-3}}{n^{\frac{3}{2}p} }$ appearing in the bounds in Theorems~\ref{thm:regressionlpmain} and \ref{thm:classificationlp} are also optimal for $\ell_p$-norm regularized estimators. Matching lower bounds for regularized estimators would lead to novel insights on when regularization can be avoided in high-dimensional settings, in the sense that we cannot improve the rates of the corresponding interpolator. (see also \cite{zhou2021optimistic} for related work). 

%We motivate future work to better understand $\ell_p$-norm penalized linear models. Maybe surprisingly, our rates in Theorem~\ref{thm:regressionlpmain} and \ref{thm:classificationlp} for \emph{noisy} settings are faster in some regimes \fy{ranges of $\beta$?} compared to existing rates for the corresponding regularized estimators (see \cite{lecue17}) and the \emph{noiseless} max-$\ell_1$-margin interpolator.
%One relevant direction for future work is to generalize the assumptions in our theoretical results (see Remark~\ref{rm:sparsity}-\ref{rm:gaussian} in Appendix~\ref{apx:remarks} for a detailed discussion) and  investigate when regularized estimators/classifiers can achieve faster rates compared to the corresponding interpolators. In fact, we wonder whether the terms of order $\frac{q^{p}d^{2p-2}}{n^{p} }$ and  $\frac{\log(d)^\kappa_3}{n}\lor\frac{q^{\frac{3}{2}p}d^{3p-3}}{n^{\frac{3}{2}p} }$ appearing in the bounds in Theorems~\ref{thm:regressionlpmain} and \ref{thm:classificationlp} are also optimal for $\ell_p$-norm regularized estimators. 





%  only suggest a partial answer to the this question. When $p \to 1$, we can 
% see that the first term on the RHS in Equation~\eqref{eq:thmregboundhighnoiseuppermain} increases and the second term decreases. 
% Thus, when $\beta<2$, we expect that the optimal $p$ is attained when both terms are roughly equal. This is the case for large $d,n$ when both terms are of the same order and thus $p = \frac{\beta+1}{2\beta -1}$
%  On the other hand, when $\beta>2$ the first term always dominates and hence our result only suggest that the optimal $p$ is attained at  $p \in (1, 1 + \frac{c}{\log\log(d)})$, however, while still clearly $p\neq 1$. 

 
% \red {a whole lot of bla..}
% While Theorem~\ref{thm:regressionlp} and~\ref{thm:classificationlp} derive rates for $\ell_p$-norm interpolators when $d,n$ is very large, our results provide only limited insights for $n,d$ of the size of practically relevant orders because of the  assumption that $p \geq 1 + \frac{c}{\log \log(d)}$. We believe that our proof methodology can also be used to obtain bounds for smaller values of $p$ and motivate this as a future work. Furthermore, albeit our statements only hold in the high-noise regime with 1-sparse ground truth, the results can be extended to more general settings using the same methodology. %(see also Appendix~\ref{apx:lownoise}). 
% the focus of this paper lies on high noise regimes where the ground truth matches the he inductive bias of the $\ell_1$-norm, 
% focus on the high-noise settings and a 1-sparse ground truth, as this is the case where the inductive bias of the $\ell_1$-norm matches the ground truth.   the inductive bias. 
% and leave the generalization of these assumptions as a future work.

% the assumptions on hte ground truth and the noise in Theorem~\ref{thm:regressionlp},\ref{thm:classificationlp},\ref{thm:mainl1} 

% Furthermore, several papers study when interpolators can achieve asymptotic consistency in high dimensional regimes without providing explicit rates (e.g., see \cite{muthukumar2021classification} for linear and also  \cite{Ghorbani2020b, ghorbani_2021,misiakiewicz2021learning,donhauser21} for non-linear models). 



\section{Conclusion}
\label{sec:conc}
In this paper, we showed that min-$\ell_p$-norm/ max-$\ell_p$-margin interpolators can achieve much faster rates with a moderate inductive bias, i.e.,  $p\in(1,2)$,  compared to a strong inductive bias, i.e., $p=1$. 
This arises from a novel bias-variance type trade-off induced by the inductive bias of the interpolating model, balancing the regularizing effect of high-dimensionality and the structural alignment with the ground truth. Based on preliminary experiments on image data with the CNTK in Figure~\ref{fig:cntk}, we further hypothesize that this trade-off carries over to more complex interpolating models and datasets used in practice and leave a thorough investigation as future work. 

\section*{Acknowledgements}
K.D.~is supported by the ETH AI Center and the ETH Foundations of Data Science. N.R.~is supported by the Max Planck ETH Center for Learning Systems.
We would like to thank Nikita Zhivotovskiy for helpful discussions and Kai Lion for his preliminary experiments. Finally we would like to thank the anonymous reviewers for their feedback.

% We presented the first non-asymptotic bounds for the risk of min-$\ell_p$-norm regression and max-$\ell_p$-margin classification in high dimensions. While the results themselves are novel, the faster (and sometimes minimax optimal) convergence rates attained by $p$ values inside $(1, 2)$ reveal an inherently different behaviour of interpolating models




% We presented the first non-asymptotic bounds for the risk of min-$\ell_p$-norm regression and max-$\ell_p$-margin classification in high dimensions. While the results themselves are novel, the faster (and sometimes minimax optimal) convergence rates attained by $p$ values inside $(1, 2)$ reveal an inherently different behaviour of interpolating models with respect to regularized ones: in the presence of noise, the optimum inductive bias is not the strongest, but rather the one that balances the \emph{regularizing effect of high-dimensionality} and the emph{structural alignment with the ground truth}. We conjecture that this inductive bias argument carries over to more complex interpolating models used in practice, and leave such connection as important future work.





%is a strong limitation for the applicability which we motivate future work to improve is the fact that 

==> ICML 22-3/sections_proof/0_main_proof.tex <==



\section{Experimental details for the convolutional NTK}
\label{appendixsec:cntk}
We include here details on the experiments with the convolutional neural tangent kernel (CNTK) presented in Section~\ref{sec:trade-off}. 

\paragraph{Binarized MNIST} We perform a binary classification task on a reduced version of the MNIST data set \cite{deng2012mnist}. In particular, we only utilize the digits from 0 to 5 (included), and define the binary labels as $y=-1$ if the digit is even, $y=+1$ if it is odd. To stay closer to the high dimensional regime, we randomly subsample only $n=500$ data points for training, the remaining ones are used for testing. The label noise is added by randomly flipping exactly $\sigma \%$ of the labels only on the training set.

\paragraph{The CNTK} The CNTK is a kernel method based on the analytical solutions of infinite width neural networks trained via gradient flow. In particular, a convolutional neural network with a given architecture has a corresponding CNTK, defined as its limit for an infinite number of channels and trained to convergence via MSE loss. We include here a short description of the model. For additional details we refer to \cite{cntk, neuraltangents2020} and references therein. \\
Consider a given neural network architecture $f_\theta$, parameterized by $\theta$. \cite{jacot2018neural, cntk} showed that, under initialization and optimization conditions, the CNTK can be formalized as a kernel method with
\begin{equation}
    k(x, x') = \mathbb{E}_\theta \left< 
        \frac{\partial f_\theta(x)}{\partial \theta} ,
        \frac{\partial f_\theta(x')}{\partial \theta}
    \right> \, .
\end{equation}
For Gaussian weights, the expected value above can be computed in closed form via recursion through the layers, which allows this model to be used in practice and without sampling.

\paragraph{Architecture} All the implementations of the CNTK are done via the Neural Tangents Python library \cite{neuraltangents2020}. In our experiments, we utilize CNTK architectures with the following structure: 
\begin{itemize}
    \item we stack convolutional layers followed by a ReLU activation $l$ times, where $l$ is what we call the depth of the architecture.
    We utilize a kernel size 3, stride 1 and padding at every layer. 
    \item a final flatten layer followed by a linear layer with one output neuron, containing the logit of the classification probability.
\end{itemize}

The results for this experiment are presented in Figure~\ref{fig:cntk}.


































% \section{Additional remarks and notation}
% We now summarize the notation and discuss  additional remarks on our theoretical analysis.

% \paragraph{Notation used in the Appendix.} We use $\kappa_1,\kappa_2,...$ and $c_1,c_2,...$ for generic universal positive constants independent of $d$, $n$ or $p$. The value $c_1,c_2,...$ may change from display to display throughout the derivations. The standard notations $O(\cdot),\Omega(\cdot)$ and $\Theta(\cdot)$, as well as $\lesssim,\gtrsim$ and $\asymp$, are utilized to hide universal constants, without any hidden dependence on $d$, $n$ or $p$.  Further we use $\tilde{O}(\cdot)$ to also hide the dependency on logarithmic factors in $d,n$ or $p$. 


% \subsection{Discussion of the assumptions}
% \label{rm:p}

% We now discuss the assumptions of our main results in the following subsections. 


% \label{apx:remarks}
% \paragraph{Assumption on  $p$}
% %\fy{i would say this more high level "for concentration" (instead of $\epsilon$) and could move to proof idea perhaps - or partially merge with the "optimal $p$" discussion in limitations} 
%  While for very large $d$, Theorems~\ref{thm:regressionlpmain} and \ref{thm:classificationlp} hold for most $p$, even close to $1$, for fixed $n,d$ our theorems apply to only a small range of $p\in(1,2)$, that is, more specifically for $p\in \left(1+\frac{\kappa_2}{\log\log(d)},2\right)$. This assumption is used to obtain a high probability concentration of the dual norm $\norm{H}_q$ in Lemma~\ref{lm:dualnormconc}.
% It is possible and straightforward to relax the assumption on $p$ to allow for smaller $p$, such as  $p \in (1+\frac{\kappa \log \log(d)}{\log(d)},2)$, by choosing $\epsilon(n,d)$ in Lemma~\ref{lm:dualnormconc} larger. However, this choice comes at the price of non-matching upper and lower bounds. In fact, when choosing $p =  1 + \frac{\kappa}{\log(d)}$, the $\ell_q$-norm $\norm{H}_q$ behaves similarly as the $\ell_{\infty}$-norm $\norm{H}_\infty$ (see \cite{paouris_2017}). Hence,  expect already a similar risk as when choosing $p = 1$. 






% \paragraph{Assumption on the sparsity of $\wgt$}
% We now discuss how the assumption of a $1$-sparse ground truth
% can be relaxed to $s$-sparse ground truths, i.e., $\norm{\wgt}_0 =s$. 
%  We only discuss the classification case, as regression follows exactly from the same argument. In fact, note that both Propositions~\ref{prop:CGMT_applicationreg} and \ref{prop:CGMT_application_classification} hold for general degrees of sparsity. In the general $s$-sparse case, we have $\wone \in \RR^{s}$ and $\wtwo \in \RR^{d-s}$. We write   $\wgtp$ as the subvector containing the support of $\wgt$ and decompose $\wone$ into the two orthogonal components $\wonepar \parallel \wgtp$ and $\woneper \perp \wgtp$. Similarly, decompose $\xs$ into $\xsparpi$ and $\xsperpi$ and note that these two vectors are independent.
%  We can then write $ \fnclas$ from Proposition~\ref{prop:CGMT_application_classification} as
% \begin{align}
%   \fnclas(\wone,\norm{\wtwo}_2) &= \frac{1}{n} \sumin \possq{1-\xi_i\sgn(\langle  \xsui,\wgt \rangle) \langle \xsui, \wone\rangle -\Ggaussian_i \norm{\wtwo}_2}   \\
%   &\sim \frac{1}{n} \sumin \possq{1-\xi_i\sgn(\langle  \xsparpi,\wgt \rangle) \langle \xsparpi, \wonepar\rangle -\langle \xsperpi,\woneper\rangle  -\Ggaussian_i  \norm{\wtwo}_2}, 
% \end{align}
% where $\sim$ denotes that both terms have the same distribution. Thus, we can straightforwardly extend all the lemmas presented in Appendix~\ref{apx:technicallemmas} to also control $ \fnclas(\wone,\norm{\wtwo}_2) $ in the $s$-sparse case.
% We can then follow the same line of reasoning used in the proofs of Theorems~\ref{thm:regressionlpmain} and \ref{thm:classificationlp}, and  relax/tighten the assumption 
% $\norm{\wone}_p^p + \norm{\wtwo}_p^p \leq \lonebound$ 
% by 
% $\vert \norm{\wonepar}_p^p - \norm{\woneper}_p^p\vert \leq \norm{\wone}_p^p \leq \norm{\wonepar}_p^p + \norm{\woneper}_p^p$. However, we remark that such a procedure might lead to loose bounds as a function of $s$ but still tight in all other parameters.





% \paragraph{Assumption on the noise}
% Theorems~\ref{thm:regressionlpmain} and \ref{thm:classificationlp} assume that the signal to noise ratio is fixed, respectively, that there is a non vanishing proportion of flipped labels. This setting is of particular interest for this paper as the ground truth is still consistently learnable (unlike settings where the noise dominates), while the effect of the noise makes it challenging to achieve fast rates, as it is for instance the case for the min-$\ell_1$-norm interpolator \cite{wang2021tight}. In fact, we are  the first to prove for a constant noise setting that we can consistently learn using interpolation and even at a fast rate. 

% Besides, several works including \cite{chinot_2021,chinot2021adaboost,wojtaszczyk_2010} have also studied the low noise regime where the proportion of flipped label goes to zero or  the strength $\sigma$ of the additive noise, respectively, as $n,d$ tend to infinity. We remark that  our proof of Theorem~\ref{thm:regressionlpmain} can be directly extended to cover vanishing noise for regression.  On the other hand, the methodology used for the classification results, i.e. Theorem~\ref{thm:classificationlp}, strongly relies on the noise model and we leave the extension of our results to low noise settings (i.e. vanishing fraction of flipped labels)  as an interesting future work. 

\section{Comparison of Theorem~\ref{thm:regressionlpmain} and \ref{cr:koehler}}
\label{rm:koehler}
We now discuss how our proof of Theorem~\ref{thm:regressionlpmain} differs from the proof of Theorem~\ref{cr:koehler} (i.e., Theorem~4 \cite{koehler2021uniform}). Theorem 4 in \cite{koehler2021uniform} (summarized in  Theorem~\ref{cr:koehler}) also applies to non-sparse ground truths $\wgt$ and is therefore expected to be less tight. Nevertheless, we  discuss the major differences with respect to their proof, which allow us to obtain tighter bounds and illustrate the different rates in Figure~\ref{fig:ratesk}.
Balancing the terms $\sqrt{\frac{d^{2/q}}{n}} $ and $\frac{1}{d^{1/q}}$, we obtain an optimal rate of order~$n^{-1/4}$ in Theorem~\ref{cr:koehler}. We now discuss how each of these terms can be further tightened in the bounds in Theorem~\ref{thm:regressionlpmain}. 


\paragraph{Use of triangular inequality in $\PhiNR,\PhipR$ and $\PhimR$.} The definitions of the terms  $\PhiNR,\PhipR$ and $\PhimR$  in the proof of Theorem~\ref{thm:regressionlpmain} in Appendix~\ref{apx:regproof} differ from the ones used in \cite{koehler2021uniform} for the localization and uniform convergence steps. In \cite{koehler2021uniform}  the authors rely on  the triangular inequality in the localization and  uniform convergence steps by bounding 
\begin{align}
   &\PhiNR := \norm{\what}_p^p = \min_{X w = \xi}  \norm{w+\wgt}_p^p
        \leq \|\wgt\|_p +  \min_{X w = \xi}  \norm{w}_p \leq \widetilde{\lonebound} \, ~~~\mathrm{and}\\
    & \PhipR :=
\max_{\substack{
      \norm{w+\wgt}_p \leq  \widetilde{\lonebound} \\ 
            Xw=\xi
        }}  \norm{w}_2^2 \leq \max_{\substack{
            \norm{w}_p \leq  \widetilde{\lonebound} + \norm{\wgt}_p \\ 
            Xw=\xi
        }}  \norm{w}_2^2.
\end{align}
While such a procedure also covers non-sparse ground truth, the resulting bounds are not tight when $\wgt$ is sparse.
Instead, we directly bound the terms $\PhiNR$, $\PhipR$(for which we make use of the sparsity of $\wgt$), which effectively allows us to  improve the terms of order $\sqrt{\frac{  d^{2/q}}{n}}$ in Theorem~\ref{cr:koehler} to the term of order $\frac{\sigma^{4-2p}q^pd^{2p-2}}{ n^p}$ in Theorem~\ref{thm:regressionlpmain}. 





\paragraph{Bounds for $\fnreg$.} Another important improvement is in the bounds used for $\fnreg$. While the proofs in \cite{koehler2021uniform} rely on a bound of the form of Equation~\eqref{eq:lpreghighnoisestep1}, in order to obtain faster rates, our analysis requires on the tighter bound in Equation~\eqref{eq:regressionfn1}. 
More specifically, in Theorem~\ref{thm:regressionlpmain} this allows us to avoid the term  $\sqrt{\frac{\log d}{n}}$.

\paragraph{Concentration inequalities for $\norm{H}_q$.}
The concentration inequalities for the dual norm $\norm{H}_q$ are a crucial ingredient for the proof of the theorem. The ones used in the proofs in \cite{koehler2021uniform} rely on the concentration of Lipschitz continuous functions (see, \cite{Ledoux1992AHS}) and also apply to more general norms. However, for the specific case of $\ell_p$-norms we can make use of much tighter concentration inequalities from \cite{paouris_2017} (see Appendix~\ref{apx:proofdualnormconc}) to avoid the terms involving $\sqrt{\frac{\log(d)}{q}} \frac{1}{ d^{1/q}}$  in the bound in Theorem~\ref{cr:koehler}.




\begin{figure}[t]
    \centering
    \includegraphics[width=0.5\linewidth]{figures/ratesreg.pdf}
         \caption{Depiction of the rates in  Theorem~\ref{thm:regressionlpmain} (solid line) and Theorem~\ref{cr:koehler} (dashed lines): classification. Order of the theoretical rates $\tilde{O}(n^{\alpha})$ for different strengths of inductive bias $p$ at different asymptotic regimes. On the x-axis we represent the value $\beta$ defining the regime $d=n^{\beta}$, on the y-axis the risk decay $\alpha$.}
         \vspace{-0.1in}
    \label{fig:ratesk}
\end{figure}











==> ICML 22-3/sections_proof/1_regression.tex <==




\section{Proof of Theorem~\ref{thm:regressionlpmain}}
\label{apx:regproof}
Throughout the remainder of the appendix we use $\kappa_1,\kappa_2,...$ and $c_1,c_2,...$ for generic universal positive constants independent of $d$, $n$ or $p$. The value $c_1,c_2,...$ may change from display to display throughout the derivations. The standard notations $O(\cdot), o(\cdot), \Omega(\cdot), w(\cdot)$ and $\Theta(\cdot)$, as well as $\lesssim,\gtrsim$ and $\asymp$, are utilized to hide universal constants, without any hidden dependence on $d$, $n$ or $p$.   
Throughout the proof, whenever we say with high-probability, we mean with probability $\geq 1 - c_1 d^{-c_2}$ with universal constants $c_1,c_2 >0$. 


The lower bound $\RiskR(\what) \gtrsim \frac{n}{d}$ follows  simply from the uniform lower bound for all interpolators in Theorem~1 and Corollary~1 in \cite{muthukumar_2020}. 

For the rest of the proof of the statement, 
we use a  localization/maximization approach,
similar to the papers \cite{chinot_2021,koehler2021uniform,ju_2020,muthukumar_2020,wang2021tight}, and common in the literature. More specifically, the proof consists of two major parts:
\begin{enumerate}
    \item \emph{Localization.}
    We derive a  high-probability upper bound $\loneboundreg$ in Proposition~\ref{prop:phidnhighreg} that only depends on the noise $\xi$ but not on the draws of the features $X$. 
    More specifically, for the norm of the min-$\ell_p$-norm interpolator $\what$
    \begin{align} \label{eq:Phi_Nreg} 
         \PhiNR := \norm{\what}_p^p =  \min_{ X(w-\wgt) = \xi} & \norm{w}_p^p
        = \min_{X w = \xi}  \norm{w+\wgt}_p^p
        \leq \loneboundreg
    \end{align}
    and consequently
    \mbox{$\norm{\what}_p^p \leq \loneboundreg$},
    with high probability.
    
    \item \emph{Uniform convergence.}
     Conditioning on the  draw of the noise $\xi$, we derive high-probability uniform upper and lower bounds (Proposition~\ref{prop:highnoiselpreg}) on the prediction error for all interpolators $w$ with  $\|w\|_p^p \leq \loneboundreg $, 
    \begin{align} \label{eq:Phi_+reg}
        \PhipR := \max_{\substack{
            % \norm{w}_p^p \leq \loneboundreg \\ % CONVENTION 1
            \norm{w}_p^p \leq \loneboundreg \\ % CONVENTION 2
             X(w-\wgt)=\xi
        }} & \norm{w-\wgt}_2^2 
        = \max_{\substack{
            % \norm{w}_p^p \leq \loneboundreg+\norm{\wgt}_p^p \\ % CONVENTION 1
            \norm{w+\wgt}_p^p \leq \loneboundreg \\ % CONVENTION 2
            Xw=\xi
        }}  \norm{w}_2^2
        ~~~\mathrm{and}\\
     \label{eq:Phi_-reg} 
            \PhimR := \min_{\substack{
            % \norm{w}_p^p \leq \loneboundreg \\ % CONVENTION 1
            \norm{w}_p^p \leq \loneboundreg \\ % CONVENTION 2
             X(w-\wgt)=\xi
        }} & \norm{w-\wgt}_2^2 
        = \min_{\substack{
            % \norm{w}_p^p \leq \loneboundreg+\norm{\wgt}_p^p \\ % CONVENTION 1
            \norm{w+\wgt}_p^p \leq \loneboundreg \\ % CONVENTION 2
            Xw=\xi
        }}  \norm{w}_2^2.
    \end{align}

\end{enumerate}
% Note that unlike \cite{wang2021tight,koehler2021uniform}, we do not further simplify the problems via the triangular inequality for $\|\wgt + w\|_p^p \leq\|\wgt\|_p^p + \|w\|_p^p  $. Furthermore, by the definition of $\loneboundreg$ in the Equation~\eqref{eq:Phi_Nreg},  the min-$\ell_p$-norm interpolator $\what$ belongs with high probability to the set of feasible solutions in  Equation~\eqref{eq:Phi_+reg} and \eqref{eq:Phi_-reg}. Therefore, the uniform convergence step yields high-probability upper and lower bounds for the prediction error. 



%  The proof of the Theorem is divided into three steps: 
% \begin{enumerate}
%     \item \emph{Application of the (Convex) Gaussian Minimax Theorem:} In a first step, we show that we can study the auxiliary optimization problems $\phiRdn,\phiRdm$ and $\phiRdm$ instead of
%     the primary optimization problems $\PhiNR, \PhipR$ and $\PhimR$ via an application of the (Convex) Gaussian Minimax Theorem. 
%     % \item \emph{Concentration inequalities:} Before starting with the actual proof, in a next step, we summarize concentration inequalities used throughout the rest of the proof.
%     \item \emph{Localization:} We derive an upper bound on $\phiRdn \leq \loneboundreg$.
%     \item \emph{Uniform convergence:}
%     % We relax the auxiliary optimization problems defining $\phiRdn,\phiRdm$ by upper bounding $\langle w, H\rangle \leq \|H\|_q \|w\|_p$.  
%     We derive upper and lower bounds for  $\phiRdm,\phiRdm$ by bounding the constraint sets in the optimization problems in Equations~\eqref{eq:phipreg}, \eqref{eq:phimreg}.
% \end{enumerate}



% As a result, the proof then follows straight forwardly form Proposition~\ref{prop:CGMT_applicationreg}. 



% and therefore $H \in \RR^{d-1}$ from  Proposition~\ref{prop:CGMT_applicationreg}. 




% \paragraph{A simplifying modification of the proof.}
% The proof heavily relies the  separation of the vector $w = (\wone,\wtwo)$ where $\wone$ contains the support of $\wgt$ and $\wtwo$ the remaining entries as in Proposition~\ref{prop:CGMT_applicationreg}. 
% Since by assumption $\wgt$ is $1$-sparse, $\wtwo \in \RR^{d-1}$. However, it is more convenient to prove Theorem~\ref{thm:regressionlpmain} assuming that $\wgt, x_i \in \RR^{d+1}$, which implies that  $\wtwo \in \RR^{d}$. In fact, this modification does not affect the expression for the bounds in Equation~\eqref{eq:thmregboundhighnoiseupper} in Theorem~\ref{thm:regressionlpmain}. 






\subsection{Application of the (C)GMT}
\label{apx:subsec:gmtreg}
Similar to \cite{koehler2021uniform}, we now discuss how the (Convex) Guassian Minimax Theorem ((C)GMT) \cite{gordon1988milman,thrampoulidis2015regularized} can be used to simplify the study of the primal optimization problems defining $\PhiNR,\PhipR$ and
$\PhimR$ via the introduction of auxiliary optimization problems $\phiRdn,\phiRdp$ and $\phiRdm$ defined below. This approach also applies to general sparse ground truths with $\norm{\wgt}_0 =s$. 
% \paragraph{Application of the (Convex) Gaussian Minimax Theorem.} 



We begin with the introduction of some additional notation. Assume that $\wgt$ is $s$-sparse which motivates us to separate $w$ into the vector $\wone \in \RR^s$ consisting of the $s$-sparse entries containing the support of $\wgt$ and $\wtwo \in \RR^{d-s}$ consisting of the remaining entries. Similarly, decompose $\wgt$ into $\wgtp$ and $\wgtp'=0$. 
Using this notation, we can express $\yui \langle \xui, w \rangle = \yui \left(\langle \xsui, \wone \rangle + \langle \xscui, \wtwo \rangle\right)$ with $\xsui$ and $\xscui$ the corresponding subvectors of $\xui$.  
We denote by $\Xs = ( x'_1,\cdots,x'_n )$ and $X'' = (  x''_1,\cdots,x''_n )$ the sub-matrices  of $X=(x_1,\cdots,x_n )$.



 We now make use of the fact that $\xscui$ is independent of $\yui$ and $\xsui$ and define $\fnreg : \RR^{s}\times\RR \to \RR_+$ with 
    \begin{equation}
        \fnreg(\wone,\|\wtwo\|_2 ) = \frac{1}{n}\| \xi - \Xs \wone - \Ggaussian \|\wtwo\|_2 \|_2^2.
    \end{equation}
  with $\Ggaussian \sim \NNN(0,I_n)$, 
 By reformulating the optimization problems via  Lagrange multipliers, we can then apply the CGMT to  $\PhiNR$ and the GMT to  $\PhipR,\PhimR$. As a result, we obtain the following result: 
% can use a standard arguemnt as presented in (cite some works) to apply the (C)GMT, resulting in Proposition~\ref{prop:CGMT_application}. Details for the proof are given in Appendix.... 


\begin{proposition}
% \begin{proposition} 
\label{prop:CGMT_applicationreg}
    % Denote $\loneboundregp = \loneboundreg + \norm{\wgt}_p^p$. % CONVENTION 1
    %Denote $\loneboundregp =  \loneboundreg + 2\norm{\wgt}_p^p$. % CONVENTION 2
      Let $p \geq 1$ be some constant and assume that $\wgt$ is $s$-sparse. 
  For $\Hgaussian \sim \NNN(0,I_{d-s})$ define the stochastic auxiliary optimization problems:\footnote{We define $\PhiNR,\PhimR,\phiRdn,\phiRdm = \infty$ and $\PhipR,\phiRdm = -\infty$ if the corresponding optimization problems have no feasible solution.}
        \begin{align}
        \label{eq:phin}
            \phiRdn &= \min_{(\wone,\wtwo)} \norm{\wone + \wgtp}_p^p+\norm{\wtwo}_p^p
            \subjto \frac{1}{n} \innerprod{\wtwo}{\Hgaussian}^2 \geq  \fnreg(\wone,\|\wtwo\|_2) \\
       \label{eq:phip}
            \phiRdp &= \max_{(\wone,\wtwo)} \norm{\wone}_2^2+\norm{\wtwo}_2^2
            \subjto \begin{cases}
                \frac{1}{n} \innerprod{\wtwo}{\Hgaussian}^2 \geq  \fnreg(\wone,\|\wtwo\|_2)\\
              \norm{\wone+\wgtp}_p^p+\norm{\wtwo}_p^p \leq \loneboundreg
            \end{cases}\\
        \label{eq:phim}
            \phiRdm &= \min_{(\wone,\wtwo)} \norm{\wone}_2^2+\norm{\wtwo}_2^2
            \subjto \begin{cases}
               \frac{1}{n} \innerprod{\wtwo}{\Hgaussian}^2 \geq  \fnreg(\wone,\|\wtwo\|_2) \\
               \norm{\wone + \wgtp}_p^p+\norm{\wtwo}_p^p  \leq \loneboundreg
            \end{cases}
        \end{align}
where $\loneboundreg>0$ is a constant possibly depending on $\xi$ and $\Xs$.  Then for any $t \in \RR$, we have:
        \begin{align}
            \PP( \PhiNR > t \vert \xi, \Xs) &\leq 2\PP( \phiRdn \geq t \vert \xi, \Xs)
            \\
            \PP( \PhipR > t \vert \xi, \Xs) &\leq 2\PP( \phiRdp \geq t \vert \xi, \Xs) 
            \\
            \PP( \PhimR < t \vert \xi, \Xs) &\leq 2\PP( \phiRdm \leq t \vert \xi, \Xs) 
           ,
        \end{align}
        where the probabilities on the LHS and RHS are over the draws of $X''$ and of $\Ggaussian,\Hgaussian$, respectively. 
\end{proposition}   
The proof is analogous to Lemma 4 and Lemma 7 in \cite{koehler2021uniform}. Proposition~\ref{prop:CGMT_applicationreg} allows us to reduce the optimization problems depending on the random matrix $\datamat\in \mathbb{R}^{n \times d}$ to optimization problems depending on the much smaller random matrix $\Xs \in \mathbb{R}^{n \times s} $ and two additional random vectors $\Hgaussian,\Ggaussian$. 







% \begin{remark}[Proof idea]
% The proof of the theorem is then essentially based on the following idea. Using the fact that $\wgtp$ is 1-sparse, the constraints in the auxiliary optimization problems in Equation~\eqref{eq:phinreg},\eqref{eq:phipreg} and \eqref{eq:phimreg} rewrite to:
% \begin{align}
%       \frac{1}{n} \langle \wtwo, H\rangle^2 \geq  f_n(\wone, \norm{\wtwo}_2) ~~\mathrm{and}~~ (\wone+\nugt)^p + \|\wtwo\|_p^p \leq \loneboundreg.
% \end{align}
% Furthermore, we can use H\"olders inequality to bound the term $\langle \wtwo, H \rangle \leq \norm{H}_q \norm{\wtwo}_p$. Denote with $b = \norm{w}_p$, we can relax the constraints to:
% \begin{align}
%           \frac{1}{n} b^2 \norm{H}_q^2  =  \frac{1}{n} \norm{H}_q^2 \left(\loneboundreg - (\wone+\nugt)^p \right)^{2/p} \approx \frac{1}{n}  \norm{H}_q^2 \loneboundreg^{2/p}\left(1 -\frac{2}{\loneboundreg} \left(\frac{1}{p} + \wone\right) \right)   \geq f_n(\wone, \norm{w}_2). 
% \end{align}
% Finally, to obtain bounds for $\nu,\eta$, we can then use the fact that w.h.p.~$ f_n(\nu, \eta) \approx \sigmaxi^2 + \nu^2 +\eta^2$ with $\sigmaxi^2 = \frac{1}{n} \|\xi\|_2^2$.
% % onditioned on the  where $q$ is the dual norm of $p$. Thus, assuming $\|w\|_p^p \leq b$ we can relax the constraint set in $\phiRdm,\phiRdn$ to:
% % $$  \loneboundreg^{2/p} \|H\|_{q}^2 \geq \fnreg(\nu, \eta)$$
% % where we use again the notation $\nu = \wone \in \RR$ (since the ground truth is 1-sparse by assumption) and $\eta = \|\wtwo \|_2$. Following this approach, we already obtain a non-trivial bound - however, in order to obtain tight upper bounds for $\phiRdm$ and $\phiRdm$ a more refined analysis is need as described below.
% \end{remark}




% \subsection{Preliminaries: Concentration inequalities}
% \label{apx:subsec:concentineqreg}
% Before bounding the quantities $\phiRdn,\phiRdm$ and $\phiRdm$, we first summarize the concentration inequalities which we condition on thought the reminder of the proof. 

% \paragraph{Concentration of $\|H\|_q$.}

% When bounding the quantities $\phiRdn,\phiRdm$ and $\phiRdm$ we make heavily use of the sub gradient $\wgrad = \partial \norm{H}_p$, i.e., the vector which satisfies $\langle \wgrad, H \rangle = \norm{H}_q$ and $\norm{\wgrad}_p =1$. In particular, we will make use of the following lemma.  Denote with $\dmoment{q} = \EE \|H\|_{q}$, the expected $\ell_q$-norm of $H$ and define  $\mutild := \frac{\dmoment{2q/p}^{2q/p}}{\dmoment{q}^{2q/p}}$


% \begin{lemma}
% \label{lm:dualnormconc}
% there exist a universal constant $c_1,c_2,c_3>0$ such that for $\epsilon(d,n) = \max\left(\frac{1}{\logjone{d}}\frac{n}{d}, \frac{\logjone{d}^c_1}{n}\right)$
% and for any $q \leq \log\logjone{d}$, with probability $\geq 1-c_2 d^{-c_3}$,
% \begin{align}
% \langle \wgrad, H\rangle &= \norm{H}_q = \dmoment{q}\left(1+O\left(\epsilon(d,n) \right)\right)   = \Theta(d^{1/q +\frac{q}{\log(q)}}) \label{eq:dualnormconc1}\\
% \norm{\wgrad}_2^2 &= \frac{\norm{H}_{2q/p}^{2q/p}}{\norm{H}_q^{2q/p}} = \mutild
% \left( 1 + O\left(\epsilon(d,n) p \right)\right) = \Theta\left(d^{1/q-1/p + \frac{q}{\logjone{d}}}\right)\label{eq:dualnormconc2}
% \end{align}
% \end{lemma}
% For the reminder of the proof,  define
%  \begin{equation}
%  \label{eq:rho}
%      \rho = \frac{\logjone{d}^c}{\sqrt{n}}
%  \end{equation}
% with $c>1$ some universal constant chosen sufficiently large such that Equation~\eqref{eq:dualnormconc1},\eqref{eq:dualnormconc2} hold. 
% The proof of Lemma~\ref{lm:dualnormconc} can be found in Appendix~\ref{apx:proofdualnormconc}. In particular, the lemma is essentially a consequence of the following two corollaries:
% % These tools allow us to study the concentration of the sub gradient $\wgrad = \partial \norm{H}_p$, i.e. the vector which satisifes $\langle \wgrad, H \rangle = \norm{H}_q$ and $\norm{\wgrad}_p =1$ with $q$ the dual number of $p$. In particular, we show that:
%  \begin{corollary}[Theorem 1 \cite{paouris_2017}]
%  \label{cor:hqbound1}
% For all sufficiently large $d$ and any $2<q <c_0\logjone{d}$, one has: 
% \begin{equation}
%     \Prob(| \|H\|_q - \dmoment{p} | \geq \epsilon \EE \|H\|_q ) \leq c_1 \exp(-c_2 \min(q^2 2^{-q} \epsilon^2 d, (\epsilon d )^{2/q}))
% \end{equation}
% where $c_0,c_1,c_2>0$ are universal constants.
% \end{corollary}
% \label{cor:hqbound2}
% \begin{corollary}[Proposition 2.4 \cite{paouris_2017}, \cite{schechtman_89}]
% \label{eq:hqbound2}
% For all $q \leq \logjone{d}$,
% \begin{equation}
%     \dmoment{q} \asymp \sqrt{q} d^{1/q}
% \end{equation}
% \end{corollary}



% % These tools allow us to study the concentration of the sub gradient $\wgrad = \partial \norm{H}_p$, i.e. the vector which satisifes $\langle \wgrad, H \rangle = \norm{H}_q$ and $\norm{\wgrad}_p =1$ with $q$ the dual number of $p$. In particular, we show that:
% % \stefan{it wasn't clear to me why we want to study sub gradient at first, maybe adding explanation if not part of the general knowledge would help}
% % Recall that by definition, 
% % \begin{equation}
% %     f_n = \frac{1}{n} \sum_{i=1}^n \left( 1- \xi \nu \|X_i\| - \eta Y_i\right)_+^2 
% % \end{equation}
% % The goal is now to upper and lower bound $f_n$ as done in the previous section for regression. However, this is much more involved. 





% \paragraph{Concentration of $\fnreg$.} We make use of the following two bounds on $\fnreg$. Define $\sigmaxi^2 = \frac{1}{n}\|\xi\|_2^2$, we have
% \begin{lemma}
% \label{lm:regressionfn}
% With probability at least $1-c_1d^{-c_2}$ over the draws of $\Ggaussian$ and $\Xs$, we have that uniformly for all $ \eta\geq0, \nu$,
% \begin{align}
%     \label{eq:regressionfn2}
%   \vert \fnreg(\nu, \eta) - \sigma^2 -\nu^2 -\eta^2\vert &\lesssim \rho (\sigma^2+\nu^2 +\eta^2) \\
% \label{eq:regressionfn1}
%   \mathrm{and}~~  \vert \fnreg(\nu, \eta) - \sigmaxi^2 -\nu^2 -\eta^2\vert &\lesssim \rho \sigmaxi  \eta + \rho \sigmaxi \vert \nu \vert + \rho (\nu^2 +\eta^2)
% \end{align}
% \end{lemma}

% Both Equations in Lemma~\ref{lm:regressionfn} follow straight forwardly form standard concentration arguments as for instance presented here: 
% \cite{koehler2021uniform,wang2021tight}.

% \paragraph{Further inequalities.} 
% We condition on the event where
% $\vert \sigmaxi^2 - \sigma^2 \vert \lesssim \rho$, which holds with probability $\geq 1-c_1 d^{-c_2}$.
% Furthermore, we repetitively make use of the following inequalities which are needed to control the error terms:
% \begin{lemma}
% \label{lm:quantconcentration}
% We can choose $\kappa_2$ to be a universal constant such that for all $n,d$ as in Theorem~\ref{thm:regressionlpmain}, we have
% \begin{align}
%   \rho \left(\frac{\dmoment{q}^{p}}{n^{p/2}}+\frac{\mutild^{1/2} n^{1/2}}{\dmoment{q}}\right)^{-1} = O\left(\frac{1}{\logjone{d}}\right) 
%   ~~\mathrm{and}~~\OOOc = O\left(\frac{1}{\logjone{d}}\right)~~\mathrm{and}~~ \frac{\dmoment{q}^2} {n}= O\left(\frac{1}{\logjone{d}}\right).
%   \label{eq:facteq2}
% \end{align}
% \end{lemma}
% The proof of Lemma~\ref{lm:quantconcentration} is straight forwardly obtained from Corollary~\ref{cor:hqbound2} and the assumptions on $d,n$ and $p$. 








% \label{apx:subsec:highnoise}
% We now bound $\phiRdn$ and $\phiRdm,\phiRdn$ form Proposition~\ref{prop:CGMT_applicationreg}. 
% For brevity of notation define $\nu := \wone$, $\eta := \norm{\wtwo}_2$. Further, throughout this section define $\nu_0 = \frac{-\sigmaxi^{2p}}{\left(\frac{n \sigmaxi^2}{\dmoment{q}^2}\right)^{p/2}} = \frac{\dmoment{q}^{2p}}{n^p}$. 
\subsection{Localization step - bounding \texorpdfstring{$\phiRdn$}{phiN}}
\label{apx:subsec:localisationproofreg}

The goal of this first step is to give a high probability upper bound on $\phiRdn$ from Proposition~\ref{prop:CGMT_applicationreg}. We now return to the $1$-sparse ground truth $\wgt=(1,0,\cdots,0)$ assumed in the theorem statement, which allows us to write $\phiRdn$ as
\begin{equation}
\label{eq:lpregphidnproof}
    \phiRdn = \min_{(\wone,\wtwo)} \vert \wone + 1\vert^p+\norm{\wtwo}_p^p
            \subjto \frac{1}{n} \innerprod{\wtwo}{\Hgaussian}^2 \geq  \fnreg(\wone,\|\wtwo\|_2)
\end{equation}




\begin{remark}[A simplifying modification for the proof.]
\label{rm:simplicification}
By definition,  $\Hgaussian \in \RR^{d-1}$. Instead, for the ease of presentation, we  prove the result assuming that $\wgt, x_i \in \RR^{d+1}$ and hence $\Hgaussian \in \RR^d$, which does not affect the expression for the bounds in Equation~\eqref{eq:thmregboundhighnoiseuppermain} in Theorem~\ref{thm:regressionlpmain}. 
\end{remark}

We now  derive  a bound for $\phiRdn$ that holds with high probability over the draws of $H,G,X',\xi$ and define $\dmoment{q} = \EE \|H\|_{q}$ and  $\sigmaxi^2 = \frac{1}{n} \|\xi\|_2^2$ with $H \sim N(0,I_d)$ and $\mutild := \frac{\dmoment{2q/p}^{2q/p}}{\dmoment{q}^{2q/p}}$. 

% \end{proposition}
\begin{proposition}
\label{prop:phidnhighreg}
Let the data distribution be as described in Section~\ref{subsec:regsetting} and assume that $\sigma = \Theta(1)$. 
Under the same conditions as in Theorem~\ref{thm:regressionlpmain} for $n,d,p$, there exist universal constants $c_1,c_2,\cdots,c_8>0$ such that with  probability at least $ 1- c_1 d^{-c_2}$ over the draws of $\Ggaussian,\Hgaussian,\Xs,\xi$, it holds that
\begin{align}
\phiRdn  \leq \left(\frac{n \sigmaxi^2}{\dmoment{q}^2}\right)^{p/2}\left(1+ \frac{p}{2} \frac{\nu_0^2}{\sigmaxi^2}  \left(1+ c_6 \rho \right) + \OOOc + c_7 \left( \rho^2 + \frac{\rho \vert \nu_0 \vert}{\sigmaxi}\right) \right)
+ \nugt + p\nu_0\left(1+ c_8 \nu_0 \right) =: \loneboundreg,
\label{eq:lpphinbound}
\end{align}
with $\OOOc = c_5 \frac{ n \exp(c_3q)}{d q }$,  $\rho = \frac{\log^{c_4}d}{\sqrt{n}}$ and $\nunull =  -\sigmaxi^{2} \left(\frac{\dmoment{q}^2}{n \sigmaxi^2}\right)^{p/2} =  \Theta \left( \frac{q^p d^{2p-2}}{n^p} \right)^{1/2}$.
\end{proposition}
Note that $\loneboundreg$ only depends on $\xi$  but not on $\Hgaussian$ and $\Ggaussian$, and thus, $\loneboundreg$ is a valid choice for the upper bound of the $\ell_p$-norm of $w$ in the constraints of $\PhipR,\PhimR$ and  Proposition~\ref{prop:CGMT_applicationreg}.  Furthermore, we note that the bound in the proposition holds with high-probability over the draws of $\xi$ despite explicitly depending on $\sigmaxi$.  However, replacing $\sigmaxi$ with $\sigma$ in the Equation~\eqref{eq:lpphinbound} by applying the high-probability bound $\vert \sigmaxi^2 -\sigma^2\vert \lesssim \sqrt{\frac{\logjone{d}}{n}}$ \fy{fix this} would lead to a loose bound in the subsequent uniform convergence step (Section~\ref{apx:subsec:unfiformconvreg}).
\begin{proof}






%  Furthermore, we recall that $\wone$ is just a one dimensional scalar. We abbreviate $\wone= \nu$ and $\norm{\wtwo}_2 = \eta$. Further, we denote with $\nugt = \wgt_1 \in \RR^d$ to be the only non-zero entry. 
%\fy{say somewhere that on a high level here we wanna get bound for $b^2$ first and then use simple Taylor to get the $b^p$ (and vice versa in the other auxiliary thing}
We condition on the high probability event $\vert \sigmaxi - \sigma\vert \lesssim \sqrt{\frac{\log d }{n}}$ and $\sigma \asymp 1$ by assumption, which we will use in multiple occasions implicitly throughout the reminder of the proof. 
By definition, any feasible $w=(w',w'')$ in Equation~\eqref{eq:lpregphidnproof} must satisfy $\frac{1}{n} 
\innerprod{\wtwo}{\Hgaussian}^2  \geq \fnreg(\wone,\|\wtwo\|_2 ) $.
Since the goal is to upper bound the solution of the minimization problem in Equation~\eqref{eq:lpregphidnproof}, it suffices to find one feasible point. 
In a first step, 
%we make use of high-probability upper bounds for $\fnreg$. In particular, 
following standard concentration arguments (as used for instance in the  proof of Lemma 5 in \cite{koehler2021uniform}), we can show that with probability at least $ 1-c_1 d^{-c_2}$ the following equation holds uniformly over all $w',w''$ 
\begin{align}
    \label{eq:regressionfn1}
 \vert \fnreg(\wone, \norm{\wtwo}_2) - \sigmaxi^2 -(\wone)^2 -\norm{\wtwo}_2^2\vert &\lesssim \tilde{\rho}\left[\sigmaxi  (\norm{\wtwo}_2 + \vert \wone \vert) + (\wone)^2 +\norm{\wtwo}_2^2\right]
\end{align}
with $\tilde{\rho} = \sqrt{\frac{\logjone{d}}{n}} $. 
We now show that we can choose $\wone = \nu_0$  and   $\wtwo$ to be a rescaled version of the subgradient of $H$, i.e. $\wtwo = b \wgrad = b \partial \|H\|_q$ with some $b \in \RR_+$. We have $\langle \wtwo, H \rangle = \|w\|_p \norm{H}_q =  b \norm{\wgrad}_p \norm{H}_q  = b \norm{H}_q$ and  thus suffices to show that
\begin{align}
\frac{b^2 \norm{H}_q^2}{n} &\geq  \sigmaxi^2+  (\nunull^2+b^2 \|\wgrad\|_2^2)(1+ c_1 \tilde{\rho} ) + c_2 \tilde{\rho} \sigmaxi (\vert \nunull\vert+b\|\wgrad\|_2) \\ 
\impliedby
b^2 &\geq \frac{ \sigmaxi^2 +  \nunull^2(1+ c_1 \tilde{\rho} ) + c_2 \tilde{\rho} \sigmaxi (\vert \nunull\vert+b\|\wgrad\|_2) }{\frac{\norm{H}_q^2}{n} - \norm{\wgrad}_2^2 (1+ c_1 \tilde{\rho} ) }. \label{eq:lpboundphinb} 
\end{align}
% \begin{align}\frac{1}{n} \innerprod{\wtwo}{\Ggaussian}^2 \geq \fnreg(\|\wone\|_2,\|\wtwo\|_2) \\ \impliedby
% b^2 \norm{H}_q^2/n \geq  \sigmaxi^4 + \tilde{\rho} \sigmaxi^2 \vert b \norm{\wgrad}_2 \vert +\rho b \norm{\wgrad}_2 \vert \nunull\vert + \rho \sigmaxi^2 \vert \nunull \vert + (1+\rho) (\nunull^2 + b^2 \norm{\wgrad}_2^2) \\
% \impliedby
% b^2 \geq \frac{1}{\norm{H}_q^2/n - (1+\rho)\norm{\wgrad}_2^2 } \left(  \sigmaxi^4 + \rho \sigmaxi^2 \vert b \norm{\wgrad}_2 \vert + \rho \sigmaxi^2 \vert \nunull \vert +  (1+\rho) \nunull^2  \right)\\
% \end{align}

\paragraph{Finding feasible $b$} We begin by studying the denominator, for which we can use concentration results for the $\ell_q$-norm of Gaussian random vectors in \cite{paouris_2017}, summarized in the following lemma
%Appendix~\ref{apx:concentrationdual}. 
\begin{lemma}
\label{lm:dualnormconc}
There exist universal constants $c_1,c_2,\cdots,c_6>0$ such that for any $n \geq c_1$, $n \lesssim d \lesssim \exp(n^{c_2})$, $q \lesssim \log\logjone{d}$ 
and for $\epsilon = \max\left(\frac{n}{d}, \frac{\log^{c_3}(d)}{n}\right)$ 
%\red{fix macro, also seems unclear regarding log notation, also after moving the $\epsilon$ notation should be adjusted to this section}
 with probability at least $ 1-c_4 d^{-c_5}$, 
\begin{align}
\langle \wgrad, H\rangle & = \dmoment{q}\left(1+O\left(\epsilon \right)\right)   %= \Theta(d^{\frac{1}{q} +\frac{\log(q)}{2\logjone{d}}})
~~\mathrm{and} \label{eq:dualnormconc1}
\\
\norm{\wgrad}_2^2 &= %\frac{\norm{H}_{2q/p}^{2q/p}}{\norm{H}_q^{2q/p}} =
\mutild
\left( 1 + O\left(\epsilon q \right)\right)  \label{eq:dualnormconc2}%= O\left(d^{\frac{1}{q}-\frac{1}{p} + \frac{c_6 q}{\logjone{d}}}\right) \lor \Omega\left(d^{\frac{1}{q}-\frac{1}{p} - \frac{c_6 q}{\logjone{d}}}\right)\label{eq:dualnormconc2},
\end{align}
where $p$ is such that $\frac{1}{p} + \frac{1}{q} = 1$. %\red{make fractions consistent}
Further it holds that
\begin{equation}
    \dmoment{q} = \Theta(d^{\frac{1}{q} + \frac{\log q}{2 \log d}}) \:\: \text{and} \:\: \mutild = O\left(d^{\frac{1}{q}-\frac{1}{p} + \frac{c_6 q}{\logjone{d}}}\right) \lor \Omega\left(d^{\frac{1}{q}-\frac{1}{p} - \frac{c_6 q}{\logjone{d}}}\right). 
\end{equation}
\end{lemma}

In particular, as a consequence of Lemma~\ref{lm:dualnormconc} and Proposition~\ref{cor:hqbound2}, we have with high probability that



\begin{align}
    \frac{\norm{H}_q^2}{n} - \norm{\wgrad}_2^2(1+ c_1 \tilde{\rho}) &= \frac{\dmoment{q}^2}{n}(1+O(\epsilon)) - \mutild (1+O(q\epsilon))(1+ c_1 \tilde{\rho} ) \\
    &=\frac{\dmoment{q}^2}{n} \left(1 + O(\epsilon) - \frac{\mutild n}{ \dmoment{q}^2} (1+O(q \epsilon +
        \tilde{\rho}))\right),
    \label{eq:regapplyconc}
\end{align}
with $\epsilon =  \max\left(\frac{n}{d}, \frac{\log^{2 c}d}{n}\right) = O(\frac{ n \exp(c_3q)}{d q } +\rho^2)$ and 
$  \rho = \frac{\log^{c} d}{\sqrt{n}} \geq \tilde{\rho}$ with universal constant $c>1$. Note that this step requires the assumption that $q \lesssim \log\log d$ or equivalently $p \geq 1 + \frac{\kappa_2}{\log\log d}$ when choosing $\epsilon$. 
In fact, the small choice of $\epsilon$ is necessary such that the error term $1 + O(\epsilon)$ arising from the concentration in  Equation~\eqref{eq:regapplyconc} does not affect the final error bound in Theorem~\ref{thm:regressionlpmain}.
 
Next, it is straight forward to check that both terms $\nunull, \frac{\mutild n}{ \dmoment{q}^2} \to0$ using Proposition~\ref{cor:hqbound2} and the assumptions in the theorem statement on $n,d$ and $p$. More precisely, we choose $\kappa_1,\cdots, \kappa_4>0$ in the theorem statement such that 
\begin{align}
 &\frac{\mutild  n}{\dmoment{q}^2} = O\left(\frac{ n \exp(c_3q)}{d q }\right)  = O\left(\frac{1}{\log d}\right)
 %=  O \left( \frac{ n \exp(c_5 q)}{d q } \right)=  ~\mathrm{and}~
 %\frac{\mutild  n}{\dmoment{q}^2} =  \Omega \left( \frac{ n \exp(-c_5 q)}{d q } \right) ~
\end{align}
% \begin{lemma}
% \label{lm:lpreg}
% %\label{lm:quantconcentration}
% We can choose universal $c_1,c_2,c_3,c_4,c_5>0$  such that for
% any ${n \log^{c_1}(n) \lesssim d \lesssim n^{q/2}\log^{-c_2 q}(n)}$, and any $p \in\left(1+\frac{c_3}{\log\logjone{d}},2\right)$ ( and hence $q \lesssim \log\logjone{d}$) and $n\geq c_4$, we have
% \begin{align}
%  &\frac{\mutild  n}{\dmoment{q}^2} = O(\frac{ n \exp(c_3q)}{d q }) = \OOOc = o(1)
%  %=  O \left( \frac{ n \exp(c_5 q)}{d q } \right)=  ~\mathrm{and}~
%  %\frac{\mutild  n}{\dmoment{q}^2} =  \Omega \left( \frac{ n \exp(-c_5 q)}{d q } \right) ~
%  ~\mathrm{and}~
%  \frac{\dmoment{q}^{2p} \sigmaxi^{4-2p}} {n^p}= \nu_0^2 = \Theta \left( \frac{q^p d^{2p-2}}{n^p} \right) = o(1). \label{eq:facteq2}
% \end{align}
% \end{lemma}
As a result, Equation~\eqref{eq:regapplyconc} becomes
\begin{align}
         %\frac{\dmoment{q}^2}{n} \left(1 + O(\epsilon) - \frac{\mutild n}{ \dmoment{q}^2} (1+O(q \epsilon +
        %\tilde{\rho}))\right) = 
        \frac{\norm{H}_q^2}{n} - \norm{\wgrad}_2^2(1+c_1\tilde{\rho}) =
        \frac{ \dmoment{q}^2}{n }\left(1 +  O\left(\frac{ n \exp(c_3q)}{d q } + \rho^2 \right) \right),
        %\OOOc + O(\rho^2\right)), 
\end{align}
where we further used that $O(q\epsilon) = O\left(\frac{\log\log d }{\log d}\right)$. 



We now study the the nominator.
Recall that we conditioned on the event where $\sigmaxi$ is lower bounded by a constant. 
We again use Lemma~\ref{lm:dualnormconc}  for the concentration of $\|\wgrad\|_2$ around $\sqrt{\mutild}$ and $\sqrt{\mutild} = 
\frac{\OOOc^{1/2} \dmoment{q}}{n^{1/2}}$, with  $\OOOc = c_5 \frac{ n \exp(c_3q)}{d q }$,  which yields 
that it suffices to satisfy
\begin{align}
b^2 &\geq \frac{ \sigmaxi^2 \left( 1 +  \frac{\nunull^2}{\sigmaxi^2}(1+c_1 \rho) + c_2\frac{\rho}{\sigmaxi}\left(\vert \nunull\vert+b \frac{\OOOc^{1/2} \dmoment{q}}{n^{1/2}}\right)\right)}{        \frac{ \dmoment{q}^2}{n }\left(1 +c_4\left(\frac{ n \exp(c_3q)}{d q } + \rho^2 \right) \right)}.
%\\ \impliedby b^2 &\geq 
\end{align}

We can now combine our bounds on the denominator and nominator using Equation~\eqref{eq:lpboundphinb}. First recall that $\tilde{\rho} \leq \rho$.
We can now take the Taylor series approximation of $\frac{1}{1+x} = 1 - x + O(x^2)$ to further tighten the inequality in  Equation~\eqref{eq:lpboundphinb}
so that it suffices to find $b$ satisfying
\begin{align}
\label{eq:regloctemp1}
%    b^2 &\geq \frac{n \sigmaxi^2}{\dmoment{q}^2} \left( 1 +  \frac{\nunull^2}{\sigmaxi^2}(1+O( \rho)) + O\left(\frac{\rho}{\sigmaxi}\right)(\vert \nunull\vert+b\sqrt{\mutild (1+O(\epsilon q +\rho))})\right)\left( 1 +O(\rho^2) + \OOOc \right) \\
    b^2 &\geq \frac{n \sigmaxi^2}{\dmoment{q}^2} \left( 1 +  \frac{\nunull^2}{\sigmaxi^2}(1+ c_1 \rho) + c_2 \frac{\rho}{\sigmaxi} \left(\vert \nunull\vert+b \frac{\OOOc^{1/2} \dmoment{q}}{n^{1/2}}\right) \right)(1
    +c_3 \rho^2 + \OOOc ),\\
    \impliedby b^2 &\geq  \frac{n \sigmaxi^2}{\dmoment{q}^2} \left( 1 +  \frac{\nunull^2}{\sigmaxi^2}(1+ c_1\rho ) + c_2 \frac{\rho |\nu_0|}{\sigmaxi}
    +c_3\rho^2 + \OOOc \right)+ \frac{ c_4b n^{1/2}\rho \OOOc^{1/2} }{\dmoment{q}}.
\label{eq:tempeqlp}
\end{align}
%using that $ \left(\frac{n \sigmaxi^2}{\dmoment{q}^2} \right)^{1/2}  \frac{\OOOc^{1/2} \dmoment{q}}{n^{1/2}} = \OOOc^{1/2} \sigmaxi$. % this is pure algebra
Furthermore, we choose $\kappa_1,\cdots, \kappa_4>0$ in the theorem statement such that 
$\nu_0^2 = \frac{\dmoment{q}^{2p} \sigmaxi^{4-2p}} {n^p} = \Theta \left( \frac{q^p d^{2p-2}}{n^p} \right) = O\left(\frac{1}{\log d}\right)$ and therefore, we can  choose $b$ satisfying
\begin{equation}
\label{eq:bsatisfies}
b^2 = \frac{n \sigmaxi^2}{\dmoment{q}^2} \left(1+\frac{ \nu_0^2}{\sigmaxi^2}\left(1+ c_1\rho \right) + c_2(\frac{\rho |\nu_0| }{\sigmaxi} + \rho^2) + \OOOc \right). 
\end{equation}
to satisfy Equation~\eqref{eq:lpboundphinb} and hence the feasibility constraint for \texorpdfstring{$\phiRdn$}{phiN}.

We can now obtain the upper bound in Proposition~\ref{prop:phidnhighreg} noting that $\phiRdn \leq b^p + (\nugt + \nu_0)^p $ and 
taking the Taylor series expansion $(1+x)^p \approx 1 + px + O(x^2)$, using that $\nu_0^2 = O\left(\frac{1}{\log d}\right)$ 
\end{proof}



\subsection{Uniform convergence step}
\label{apx:subsec:unfiformconvreg}
We use the same notation as in Appendix~\ref{apx:subsec:localisationproofreg}. We now prove upper and lower bounds for $\phiRdp,\phiRdm$, respectively, for the choice $\loneboundreg$ from Proposition~\ref{prop:phidnhighreg}.Note that both problems only depend on $\wtwo$ via $\norm{\wtwo}_2$ and $\norm{\wtwo}_p$. 
We are now going to decouple these two quantities.  Define 
\begin{equation}
    \Gamma = \{ (\nu, \eta) \in \mathbb{R} \times \mathbb{R}_+\vert \exists b>0 \subjto \frac{1}{n} \norm{H}_q^2 b^2  \geq  \fnreg(\nu, \eta) ~~\mathrm{and}~~ (\nu+\nugt)^p + b^p \leq \loneboundreg \}
\end{equation} 
Using H\"older's inequality (i.e., $\langle w, \Hgaussian \rangle \leq \|\Hgaussian\|_q \|w\|_p$)  to relax the optimization problems defining  $\phiRdp,\phiRdm$ in Proposition~\ref{prop:CGMT_applicationreg}, we can show that
\begin{align}
        \phiRdp &\leq \left[ \max_{(\nu,\eta) \in \Gamma} \nu^2 +\eta^2
        \right]
   ~~ \mathrm{and}~~
        \phiRdm \geq \left[\min_{(\nu,\eta) \in \Gamma} \nu^2 +\eta^2
                  \right].
    \end{align}
Hence,  Equation~\eqref{eq:thmregboundhighnoiseuppermain} in Theorem~\ref{thm:regressionlpmain} follows directly from the following proposition. 
\begin{proposition}
\label{prop:highnoiselpreg}
Let the data distribution be as described in Section~\ref{subsec:regsetting} and assume that $\sigma = \Theta(1)$. 
Under the same conditions as in Theorem~\ref{thm:regressionlpmain} for $n,d,p$  and for the choice $\loneboundreg$ in Proposition~\ref{prop:phidnhighreg}, there exist universal constants $c_1,c_2,\cdots,c_5>0$ such that with probability at least $ 1- c_1 d^{-c_2}$ over the draws of $\Ggaussian,\Hgaussian,\Xs,\xi$, it holds that
\begin{align}
  \Gamma \subseteq \left\{(\nu,\eta) \vert   ( \nu - \nu_0)^2 \lor \eta^2 \lesssim  \nu_0^{3/2} + \nunull^2 \rho^{1/2}  +  \sigma^2 (\OOOc + c_4 \rho^2 ) +  \sigma\rho \nu_0
\right\},
\end{align}
with $\OOOc = c_5 \frac{ n \exp(c_3 q)}{d q } $,   $\rho = \frac{\log^{c_4}d}{\sqrt{n}}$ and $\nunull =  -\sigmaxi^{2} \left(\frac{\dmoment{q}^2}{n \sigmaxi^2}\right)^{p/2} =  \Theta \left( \frac{q^p d^{2p-2}}{n^p} \right)^{1/2}$.
%\stefan{should you keep $\OOO(1/\log d)$ terms (i.e. $\nu-\nu_0 -\OOO$ and $\eta -\OOO$)? i think you use this form in equation (3) (statement of theorem 1)?}
\end{proposition}







\begin{proof}
First we show that any $\nu,\eta \in \Gamma$ vanishes, i.e. $\nu,\eta \to 0$ as $d,n \to \infty$, which we then use for the second step where we derive a tight bound. %We can then obtain the 
We condition on the high probability event $\vert \sigmaxi - \sigma\vert \lesssim \sqrt{\frac{\log d }{n}}$ and $\sigma \asymp 1$ by assumption, which we will use in multiple occasions implicitly throughout the reminder of the proof. 
 

\paragraph{Step 1: $ \Gamma \subset \left\{(\nu,\eta) \vert \nu^2 + \eta^2 = O\left( \left(\frac{\dmoment{q}^2}{n \sigmaxi^2}\right)^{p/2} + 
  \rho \right)+\OOOc \right\}$}
First note that we can relax the constraints in $\Gamma$ to $\frac{1}{n} \norm{H}_q^2 \loneboundreg^{2/p}  \geq  \fnreg(\nu, \eta) $. Conditioning on Equation~\eqref{eq:regressionfn1} to control $\fnreg$ we then obtain
\begin{equation}
\label{eq:lpreghighnoisestep1}
    \frac{\loneboundreg^{2/p}\|\Hgaussian\|_q^2}{n} \geq  \fnreg(\nu,\eta) \geq \left(\sigma^2 +   \nu^2 +  \eta^2\right)(1+ c_3 \rho),
\end{equation}
which holds with probability
at least $ 1- c_1 d^{-c_2}$, where we again choose $\rho = \frac{\log^{c_4}d}{\sqrt{n}}$ with universal constant $c_4>1$.

Recalling the definition of $\loneboundreg$ from Proposition~\ref{prop:phidnhighreg}, and using the Taylor series approximation $\frac{1}{1+x} = 1 -x + O(x^2)$, it holds that
\begin{align}
\label{eq:lpMunif}
       \loneboundreg^{2/p} \leq \frac{n \sigmaxi^2}{\dmoment{q}^2}\left(1+ \frac{\nu_0^2}{\sigmaxi^2}  \left(1+ c_6 \rho \right) + \OOOc+ c_7 (\rho^2 + \rho \nu_0) + \frac{2 + 2p \nu_0 + c_8 \nu_0^2 }{p \left(\frac{n \sigmaxi^2}{\dmoment{q}^2}\right)^{p/2}} \right),
\end{align}
and hence by Lemma~\ref{lm:dualnormconc} we have 
\begin{equation}
 \frac{\loneboundreg^{2/p}\|\Hgaussian\|_q^2}{n} \leq \sigmaxi^2 \left(1 + c_3 \left(\frac{\dmoment{q}^2}{n \sigmaxi^2}\right)^{p/2}  +\OOOc\right),
 \end{equation}
  where we only keep track of the dominating terms. In particular,  the following upper bound holds from Equation~\eqref{eq:lpreghighnoisestep1},
 
\begin{equation}
\label{eq:bound2lpeq}
   \nu^2 + \eta^2 =O\left( \left(\frac{\dmoment{q}^2}{n \sigmaxi^2}\right)^{p/2} + 
  \rho \right)+\OOOc = O(\nunull + \rho) + \OOOc =:  \OOO_b= O(\frac{1}{\log d}).
\end{equation}






\paragraph{Step 2: Bound in Proposition~\ref{prop:highnoiselpreg}}
% Conditioning on the event where Equation~\eqref{eq:bound2lpeq} holds and thus $\Omega \subset \{(\nu,\eta) \vert \vert \nu - \nugt\vert \leq O\left(\frac{1}{\logjone{d}}\right)  ~~\mathrm{and}~~ \eta \leq O\left(\frac{1}{\logjone{d}}\right)\}$, we can 
%The analysis in the previous step was not tight. 
%\fy{instead of bla, we now use $\sigmaxi$ ...} 
Conditioning on  the event where Equation~\eqref{eq:bound2lpeq} holds, we  now show how we can obtain a tighter bound on $\nu^2$ and $\eta^2$ using a more refined analysis.
As  in the proof of Proposition~\ref{prop:phidnhighreg}, we condition on the event where Equation~\eqref{eq:regressionfn1} holds, which allows us to relax the first constraint in  $\Gamma$ to 
%\fy{tilde rho below? - i mean sure doesn't make a difference but then why do you even have two different $\rho$?}
\begin{align}
\label{eq:lptightcond1reg}
     \frac{1}{n} \norm{H}_q^2 b^2 \geq   \fnreg(\nu,\eta) &\geq  \sigmaxi^2 + (\nu^2  + \eta^2)(1+ c_1 \rho ) +  c_2 \sigmaxi \rho(\nu + \eta). 
     \end{align}
     
% \stefan{better to use the same form as previously (lemma 3) and the proof, i.e. with: $\geq  \sigmaxi^2 + \nu^2  + \eta^2  +(\nu^2 + \eta^2) O\left(\rho\right) +  O( \sigmaxi\rho(\nu + \eta)) $ ?}

% Using the fact that with high probability $\eta^2 + \nu^2 \leq c \sigmax^2$, we can lower bound (using $\delta = c\sqrt{\frac
% {\logjone{d}}{n}}$):
% \begin{equation}
%     \frac{1}{n} \fnreg \geq \sigmaxi^4 + ( v - \sigmaxi^2 \delta)^2 + (\nu - \sigmaxi^2 \delta)^2 - 2 \sigmaxi^4 \delta^2 
% \end{equation}
% Thus, we obtain the conditions:
% \begin{align}
% \frac{1}{n} \innerprod{\wtwo}{\Ggaussian}^2 \geq  \sigmaxi^4 + ( v - \sigmaxi^2 \delta)^2 + (\nu - \sigmaxi^2 \delta)^2 - 2 \sigmaxi^4 \delta^2 \\
% (\nu+\nugt)^p + \norm{\wtwo}_p^p \leq \loneboundreg
% \end{align}
Unlike the previous step, we do not further simplify the second constraint in $\Gamma$ but instead use that $\nu^2 = \OOO_b \to 0$ which allows us to take the Taylor series $(1+\nu)^p \approx 1 + p \nu + O(\nu^2) = 1 + p \nu (1 + \OOO_b^{1/2})$, and hence
\begin{align}
    b^p &\leq \loneboundreg - (\nu+\nugt)^p \leq \loneboundreg - 1 - p \nu (1 + \OOO_b^{1/2})
    \\ &=\left(\frac{n \sigmaxi^2}{\dmoment{q}^2}\right)^{p/2}\left(1+ \frac{p}{2} \frac{\nu_0^2}{\sigmaxi^2}  \left(1+ c_6 \rho \right) + \OOOc + c_7 (\rho^2 + \frac{\rho \nu_0}{\sigmaxi}) \right) 
 + p(\nu_0 - \nu) \left(1+ \OOO_b^{1/2}\right).
\end{align}

% Thus, by definition we have:
% \begin{align}
% \label{eq:lptightcond2}
%     b^p \leq \loneboundreg - (\nu+\nugt)^p &= \left(\frac{n \sigmaxi^2}{\dmoment{q}^2}\right)^{p/2}\left(1+ \frac{p}{2} \right(\frac{\nu_0^2}{\sigmaxi^2} + 
% \OOOc\left)\left(1+O\left(\frac{1}{\logjone{d}}\right)\right)\right) + p\left(\nu_0-\nu\right)(1+ O\left(\frac{1}{\logjone{d}}\right) ),
% \end{align}
% where we have used that $\nu = O\left(\frac{1}{\logjone{d}}\right)$ conditioned on the event where Equation~\eqref{eq:bound2lpeq} holds. 
Further, using the Taylor series approximation $(1+x)^{2/p} = 1 + \frac{2}{p} x + O(x^2)$ and following the same reasoning as for Equation~\eqref{eq:lpMunif} (by applying Lemma~\ref{lm:dualnormconc}), we get
\begin{align}
    \frac{1}{n} \norm{H}_q^2 b^2 &\leq  
  \sigmaxi^2
    \left(1+  \frac{\nu_0^2}{\sigmaxi^2}  \left(1+ c_6 \rho \right) + \OOOc + c_7 (\rho^2 + \frac{\rho \nu_0}{\sigmaxi})
 + \frac{2(\nu_0 - \nu)}{\left(\frac{n \sigmaxi^2}{\dmoment{q}^2}\right)^{p/2}} \left(1+ \OOO_b^{1/2} )\right) \right).
%     \frac{1}{n} \norm{H}_q^2 \frac{n \sigmaxi^2}{\dmoment{q}^2}\left(1+ \left(\frac{\nu_0^2}{\sigmaxi^2} + 
% \OOOc \right)\left(1+O\left(\frac{1}{\logjone{d}}\right)\right)  + \frac{2}{\left(\frac{n \sigmaxi^2}{\dmoment{q}^2}\right)^{p/2}}\left(\nu_0-\nu\right)\left(1+ O\left(\frac{1}{\logjone{d}}\right)\right)\right) \\
% &=
% \sigmaxi^2 \left(1+ \left(\frac{\nu_0^2}{\sigmaxi^2} + 
% \OOOc\right)\left((1+O\left(\frac{1}{\logjone{d}}\right)\right)  - \frac{2\nu_0 \left(\nu_0-\nu\right)}{\sigmaxi^2}\left(1+ O\left(\frac{1}{\logjone{d}})\right)\right) \right) \\
% &=\sigmaxi^2 + \left(\nu_0^2+
% \OOOc \sigmaxi^2 - 2\nu_0 \left(\nu_0-\nu\right) \right)\left(1+O\left(\frac{1}{\logjone{d}}\right)\right) 
\label{eq:lpboundonbreg}
\end{align}
Plugging the inequality from Equation~\eqref{eq:lpboundonbreg}  into Equation~\eqref{eq:lptightcond1reg} and using that by definition $\nu_0 = -\frac{\sigmaxi^2 \dmoment{q}^p}{n^{p/2} \sigmaxi^p}$,  we obtain from completing the square:
\begin{align}
\label{eq:lptightcond2reg}
    &\sigmaxi^2
    \left(1+  \frac{\nu_0^2}{\sigmaxi^2}  \left(1+ c_6 \rho \right) + \OOOc + c_7 (\rho^2 +  \frac{\rho \nu_0}{\sigmaxi})
 + \frac{2(\nu_0- \nu)}{\left(\frac{n \sigmaxi^2}{\dmoment{q}^2}\right)^{p/2}} \left(1+ \OOO_b^{1/2}\right) \right)\\
\geq~~&\sigmaxi^2 + (\nu^2 + \eta^2)(1+ c_1 \rho) +  c_2 \sigmaxi\rho(\nu + \eta) \\
\implies 
& c_1 \nu_0^2 (\rho^{1/2} + |\nunull|^{1/2}) +  \sigmaxi^2\OOOc + c_7(\sigmaxi^2\rho^2 + \sigmaxi\rho \nu_0) 
 \geq  (\nu-\nu_0(1+ \OOO_b^{1/2}) +c_2\sigmaxi \rho)^2  + (\eta + c_3\sigmaxi \rho)^2,
\end{align}
which implies 
\begin{equation}
    c_1 \rho^2 + \OOO_c + \nu_0^2
 \gtrsim  \nu^2  + \eta^2 ~~~\mathrm{and}~~~ \nu^2 \gtrsim \nu_0^2 +   c_2 \rho^2 + \OOO_c
\end{equation}
Hence, we can conclude the proof when plugging in the definition of $\nu_0$ and using that   $\vert \sigma^2-\sigmaxi^2\vert \lesssim \rho$, and additionally note that we can choose $\kappa_2$ in Theorem~\ref{thm:regressionlpmain} such that for any $p \in\left(1+\frac{\kappa_2}{\log\logjone{d}},2\right)$ and any $d \geq n$, $\frac{\log^{\kappa_8}d}{n} = O(\nunull^2)$. 





%have we used Lemma~\ref{lm:lpreg},\ref{lm:lpreg2} to hide the terms depending on $\rho$ in the term $O\left(\frac{1}{\logjone{d}}\right)$.
\end{proof}

==> ICML 22-3/sections_proof/2_thm1.tex <==















\section{Proof of Theorem \ref{thm:mainl1}}
\label{apx:proofl1}
Recall the definition of  $f(\nu,\eta) = \EE_{Z_1,Z_2 \sim \NNN(0,1)} \EE_{\xi \sim \prob(\cdot\vert Z_1)} \left( 1- \xi \nu \vert Z_1 \vert - \eta Z_2\right)_+^2 $ and $\nubar := \arg\min f(\nu, 0)$ in Section~\ref{subsec:clasetting}. Further, as in the proof of Theorem~\ref{thm:classificationlp} in Appendix~\ref{apx:claslpproof}, define the quantities ${\fstar = f(\nubar, 0)}$, ${\feestar = \frac{d^2}{d^2 \eta}\vert_{(\nu, \eta) = (\nubar, 0)} f(\nu,\eta)}$ and ${\fnnstar = \frac{d^2}{d^2 \nu}\vert_{(\nu, \eta) = (\nubar, 0)} f(\nu,\eta)}$ which are all non-zero positive constants.  We now show the proof of Theorem~\ref{thm:mainl1} with  
% \kd{stefan, we need ot check this once more}
\begin{equation}
\label{eq:kappanoise}
  \kappanoise = \frac{ 2 \fstar }{\feestar \nubar^2}.
\end{equation}

The proof follows a similar structure as the proof of Theorem~\ref{thm:regressionlpmain},\ref{thm:classificationlp} in Appendix~\ref{apx:regproof},\ref{apx:claslpproof}. In particular, we first apply the CGMT in Proposition~\ref{prop:CGMT_application_classification} (which also holds for $p=1$) and then separately bound $\phidn$ in the localization step  and $\phidp,\phidm$ in the uniform convergence step. 
However, as also noted in \cite{wang2021tight} for the related min $\ell_1$-norm interpolator (basis pursuit), the relaxation $\|H\|_{\infty} \|w\|_1 \geq \langle w, H\rangle$ in the constraint sets defining $\phidn,\phidp$ and $\phidm$ in Proposition ~\ref{prop:CGMT_application_classification} leads to non-tight bounds. Instead, as described in Appendix~\ref{apx:subsec:l1path}, we use a path approach as described in \cite{wang2021tight} to show that $\phidn,\phidp$ and $\phidm$ are also the solution of a simpler $3$-dimensional optimization problem. This allows us to then obtain tight bounds for $\phidn$ in Appendix~\ref{apx:subsec:l1localization} and $\phidp,\phidm$ in Appendix~\ref{apx:subsec:l1uniform}. The proof then follows straight forwardly from Proposition~\ref{prop:CGMT_application_classification} and the fact that $\RiskC(\what) =\norm{\frac{w}{\norm{w}_2} - \wgt}_2^2 = 2 - 2\frac{\langle w, \wgt\rangle}{\norm{w}_2}$.






% By definition of $\gennormbound$ is an upper bound for \eqref{eq:Phi_N}, with high probability the min-$\ell_1$-norm interpolator $\what$ belongs to the set of feasible solutions in \eqref{eq:Phi_+} and \eqref{eq:Phi_-},
% and hence the second step yields high-probability upper and lower bounds on $\frac{\langle \what, \wgtbar\rangle}{\norm{\what}_2} $ and thus also on the prediction error. 
% % = \Risk(\what)$. %, proving Theorem~\ref{thm:main}.






% Essentially, both the proof of Theorem~\ref{thm:mainl1} and \ref{thm:mainlp} rely on an application of the (Convex) Guassian Minimax Theorem \cite{gordon1988milman,thrampoulidis2015regularized}, which allows us to equivalently study optimization problems involving random vectors $H \in \RR^d, G\in \RR^n$ instead of the random matrix $X\in \RR^{d \timex n}$. For this, note that by assumption, $\wgt$ is $s$-sparse. We therefore separate $w$ into two vectors $\wone \in \RR^s$ and $\wtwo \in \RR^{d-s}$ with the first one on containing the support $\wgt$. In particular, we have $\yui \langle \xui, w \rangle = \yui \left(\langle \xsui, \wone \rangle + \langle \xscui, \wtwo \rangle\right)$ with $\xsui$ and $\xscui$ the corresponding subvectors of $\xui$. We write and $\Xs = \{ \xsui \}_{i=1}^n$.
% Because $\xscui$ is independent on $\yui$ and $\xsui$, we can use a standard arguemnt as presented in (cite some works) to apply the (C)GMT, resulting in Proposition~\ref{prop:CGMT_application}. Details for the proof are given in Appendix.... 






% Following the work in \cite{konst} we can recast \eqref{eq:phin}, \eqref{eq:phip}, \eqref{eq:phim} as optimization problems in three scalar variables. Let $b,\alpha$ be scalar variables with $b\geq 0$, $\alpha\in[1,\alpham]$ with $\alpham = d\frac{\norm{\Hgaussian}_{\infty}}{\norm{\Hgaussian}_p^p}$. Then we define parametric path $b\gamma(\alpha)$ with $\RR^d$-valued function $\gamma$ given by:
% \begin{equation}
%     \gamma(\alpha) = \argmin_{\wtwo} \norm{\wtwo}_2^2
%     \subjto \begin{cases}
%                 \innerprod{\wtwo}{\Hgaussian} \geq \norm{\Hgaussian}_{\infty}\\
%                 \wtwo\geq 0\\
%                 \transp{\onevec} \wtwo = \norm{\wtwo}_p^p = \alpha
%             \end{cases}
% \end{equation}
% \begin{restatable}{proposition}{propparam}
% % \begin{proposition} 
% \label{prop:parametrization}
% Optimization problems \eqref{eq:phin}, \eqref{eq:phip}, \eqref{eq:phim} are equivalently given by:
%         \begin{align}
%         \tag{$A_N$}\label{eq:phin}
%             \phidn &= \min_{\nu,b,\alpha} \nu + \alpha b
%             \subjto \frac{1}{n}  b^2\norm{\Hgaussian}_{\infty}^2  \geq  \fnclas(\|\wone\|_2,b\|\gamma(\alpha)\|_2). \\
%         \tag{$A_+$} \label{eq:phip}
%             \phidp &= \max_{\nu,b,\alpha}  \frac{\nu}{\sqrt{\nu^2+b^2\norm{\gamma(\alpha)}_2^2}}
%             \subjto \begin{cases}
%               \frac{1}{n}  b^2\norm{\Hgaussian}_{\infty}^2  \geq  \fnclas(\|\wone\|_2,b\|\gamma(\alpha)\|_2)\\
%                 \nu+b  \leq \loneboundclas
%             \end{cases}\\
%         \tag{$A_-$} \label{eq:phim}
%             \phidm &= \min_{\nu,b,\alpha}  \frac{\nu}{\sqrt{\nu^2+b^2\norm{\gamma(\alpha)}_2^2}}
%             \subjto \begin{cases}
%               \frac{1}{n}  b^2\norm{\Hgaussian}_{\infty}^2  \geq  \fnclas(\|\wone\|_2,b\|\gamma(\alpha)\|_2)\\
%                 \nu+b \leq \loneboundclas
%             \end{cases}
%         \end{align}
% for some scalars $\nu,b>0$ and $\alpha\in[1,\alpham]$.

% \end{restatable}   






































\paragraph{A simplifying modification of the proof.}
Following the same reasoning as in the prove of Theorem~\ref{thm:regressionlp} in Appendix~\ref{apx:regproof}, we instead proof the result
assuming that $\wgt, x_i \in \RR^{d+1}$, which implies that  $H \in \RR^{d}$. This modification does not affect the expression for the bounds in Equation~\eqref{eq:mainboundl1} in Theorem~\ref{thm:mainl1}. 


















































\subsection{Step 1: Reduce the optimization problem via a path approach.}
\label{apx:subsec:l1path}
\label{step_1_thm3_proof}

Following the work in \cite{wang2021tight} we can recast the optimization problems defining $\phidn,\phidp$ and $\phidm$ in Proposition~\ref{prop:CGMT_application_classification} as optimization problems in three scalar variables. Let $b,\alpha$ be scalar variables with $b\geq 0$, $\alpha\in[1,\alpham]$ and $\alpham = d\frac{\norm{\Hgaussian}_{\infty}}{\norm{\Hgaussian}_1}$.  We define the parametric path $\alpha  \mapsto \gamma(\alpha) \in \RR^{d}$ given by:
\begin{equation}
\label{eq:def_gamma_alpha}
    \gamma(\alpha) = \argmin_{\wtwo} \norm{\wtwo}_2^2
    \subjto \begin{cases}
                \innerprod{\wtwo}{\Hgaussian} \geq \norm{\Hgaussian}_{\infty}\\
                \wtwo\geq 0\\
                \transp{\onevec} \wtwo = \norm{\wtwo}_1 = \alpha
            \end{cases}
\end{equation}

Following exactly the same arguments as in Lemma 1 in \cite{wang2021tight} we obtain: 
\begin{proposition}
% \begin{proposition} 
\label{prop:parametrization}
The optimization defining $\phidn,\phidp$ and $\phidm$ in
Proposition~\ref{prop:CGMT_application_classification} are equivalently given by optimization problems \eqref{eq:phin_par}, \eqref{eq:phip_par}, \eqref{eq:phim_par} respectively, defined by:
    \begin{align}
        \tag{$A_N'$}\label{eq:phin_par}
            \phidn &= \min_{\nu,b,\alpha} \vert \nu \vert  + b \alpha
            \subjto \frac{1}{n}  b^2\norm{\Hgaussian}_{\infty}^2  \geq  \fnclas(\nu,b\|\gamma(\alpha)\|_2).
            \\
        \tag{$A_+'$} \label{eq:phip_par}
            \phidp &= \max_{\nu,b,\alpha}  \frac{\nu}{\sqrt{\nu^2+b^2\norm{\gamma(\alpha)}_2^2}}
            \subjto 
            (\nu, b, \alpha) \in \Gamma_0
            \\
        \tag{$A_-'$} \label{eq:phim_par}
            % \phidm &= \min_{\nu,b,\alpha}  \frac{\nu}{\sqrt{\nu^2+b^2\norm{\gamma(\alpha)}_2^2}}
            % \subjto \begin{cases}
            %   \frac{1}{n}  b^2\norm{\Hgaussian}_{\infty}^2  \geq  \fnclas(\wone,b\|\gamma(\alpha)\|_2)\\
            %     \nu+b \leq \loneboundclas
            % \end{cases}
            \phidm &= \min_{\nu,b,\alpha}  \frac{\nu}{\sqrt{\nu^2+b^2\norm{\gamma(\alpha)}_2^2}}
            \subjto
            (\nu, b, \alpha) \in \Gamma_0
    \end{align}
for some scalars $\nu, b>0, \alpha\in[1,\alpham]$ and set $\Gamma_0$ given by:
\begin{align}
    \Gamma_0 = \left\{ (\nu, b, \alpha) \subjto\frac{1}{n}  b^2\norm{\Hgaussian}_{\infty}^2  \geq  \fnclas(\nu,b\|\gamma(\alpha)\|_2) ~~\andtxt~~  \nu + b\alpha \leq \loneboundclas \right\}.
    \label{eq:Omega_0_def}
\end{align}
% \begin{align}
%     \Gamma_0 = \left\{ (\nu,\eta) \subjto\frac{1}{n}  b^2\norm{\Hgaussian}_{\infty}^2  \geq  \fnclas(\nu,b\|\gamma(\alpha)\|_2) ~~\andtxt~~  \nu+b \leq \loneboundclas \right\}.
% \end{align}
% \begin{align}
%     \Gamma_0 = \left\{ (\wone,\wtwo) \subjto \frac{\innerprod{\wtwo}{H}}{n}^2  \geq  \fnclas( \wone, \wtwo ) ~~\andtxt~~  \norm{\wone}_1 + \norm{\wtwo}_1 \leq \loneboundclas \right\}.
% \end{align}
\end{proposition}  
For the reminder of the proof, we can assume without loss of generality that $H_i >0$ and that $H_i > H_j$ for all $i>j$ (see also \cite{wang2021tight}). 
In order to study this reformulated optimization problem, we make use of the following three properties of the path $\gamma(\alpha)$:


\paragraph{Concentration of $\norm{\gamma(\alpha)}_1$ and $\norm{\gamma(\alpha)}_2$.} 
As proven in Section 3.4 in \cite{wang2021tight} the path $ \gamma ( \alpha ) $ is a piecewise linear with breakpoints at $ \alpha_s $ for integers $ s = 2, \dots, d$, with
\begin{equation}
    \alpha_s = \frac{ \left( \norm{\Hvecs}_1-s H_s \right) \norm{H}_{\infty} } {\norm{\Hvecs}_2^2 - \norm{\Hvecs}_1 H_s }
\end{equation}
where $\Hvecs \in \RR^{d}$ denotes vector which is equal to $H \in \RR^{d}$ on first $s$ components and zero elsewhere. Moreover, the following concentration result holds as shown in Proposition 4 in \cite{wang2021tight}.

\begin{proposition}
\label{prop:concentrationl1}
Let $\ts$ be given by $2\Phic(\ts) = s/d$. There exists universal positive constants $c_1,c_2,c_3,c_4>0$ such that for any $s,d$ with $s\geq c_1$ and $c_2 s\leq d\leq \exp(c_3 s^{1/5})$ we have that:
    \begin{align}
        \abs{
            \frac{\norm{\gamma(\alphathr{s})}_1}{\norm{\Hgaussian}_\infty} - \left(\frac{1}{\ts} - \frac{2}{\ts^3}\right)
        }
        &\leq \frac{c_4}{\ts^5}
        \qquad \andtxt \qquad
        \abs{
            \frac{\norm{\gamma(\alphathr{s})}_2^2}{\norm{\Hgaussian}_\infty^2} - \frac{2}{s \ts^2}
        }
        \leq \frac{c_4}{s \ts^4}, \label{eq:concentration}
    \end{align}
with probability at least $1-6\exp\left(-\frac{2s}{\log^5(d/s)}\right)$ over the draws of $H$.
\label{lemma_gamma_conc}
\end{proposition}

\paragraph{Convexity and monotonicity of  $\gamma(\alpha)$. }
According to Lemma 4 in \cite{wang2021tight} the mapping $ \alpha \mapsto \norm{ \gamma(\alpha) }_2^2 $ is convex over $ [ 1, \alpham ]$ and the map $ \alpha \mapsto \frac{ \norm{\gamma(\alpha)}_2^2} {\norm{\gamma(\alpha)}_1^2 }  =\frac{ \norm{\gamma(\alpha)}_2^2} {\alpha^2 }$ is monotonically decreasing.

\paragraph{Inequality constraint at optimal point.} According to Claim 3 in \cite{wang2021tight} the first inequality constraints the definition of $\gamma(\alpha)$ in Equation~\eqref{eq:def_gamma_alpha} is tight for the optimal solution, i.e.,  $\innerprod{\gamma(\alpha)}{H} = \norm{H}_{\infty}$. 


Furthermore we will use the following two characterizations of $t_s$:
\paragraph{Approximation of $t_s$.}
From Remark 2 in \cite{wang2021tight} there exists universal constant $\kappa$ such that, for all $s \leq d/\kappa$ holds that 
\begin{equation}
   t_s^2 = 2 \log(d/s) - \log \log (d/s) -\log(\pi) +\frac{\log\log(d/s)}{2\log(d/s)} + O\left(\frac{1}{\log(d/s)}\right).
\end{equation}

\paragraph{Upper and lower bounds of $\tnstar$.}
Define $\nopt = n\feestar/2$. Following the same argument as in Claim 7 and Claim 9 in \cite{wang2021tight}, we can prove the following lemma:
\begin{lemma}
\label{lemma_uls_ols_exp}
    Let any fixed constant $ 0 < \lambda \leq  \log^{1/4} (c_2) $ where by assumption $d\geq n c_2$ and let $\uls$ be the largest integer such that $\tuls^2 \geq \tnstar^2 + \frac{\lambda}{\sqrt{\tnstar}}$. Then
    \begin{align}
        \uls = \nstar \exp \left( -\frac{ \lambda }{ 2 \sqrt{\tnstar} } \right) \left( 1 + O \left( \frac{1}{\tnstar^2} \right) \right)
        \andtxts
        \left| \tuls^2 - \left( \tnstar^2 + \frac{\lambda}{\sqrt{\tnstar}} \right) \right| \leq O \left( \frac{1}{n} \right)
    \end{align}
    Moreover, let $\ols$ be the smallest integer such that $\tols^2 \leq \tnstar^2 - \frac{\lambda}{\sqrt{\tnstar}}$. Then
    \begin{align}
        \ols = \nstar \exp \left( \frac{ \lambda }{ 2 \sqrt{\tnstar} } \right) \left( 1 + O \left( \frac{1}{\tnstar^2} \right) \right)
        \andtxts
        \left| \tols^2 - \left( \tnstar^2 - \frac{\lambda}{\sqrt{\tnstar}} \right) \right| \leq O \left( \frac{1}{n} \right)
    \end{align}
\end{lemma}
 Furthermore, analogously as in proof of Claim 8 in \cite{wang2021tight} we get:
\begin{align}
    \frac{\tnstar^2}{\tuls^2} 
    =
    \frac{1}{1 + \frac{\lambda}{\tnstar^2\sqrt{\tnstar}} + O \left( \frac{1}{\tnstar^2 \nstar} \right)}
    =
    1 - \frac{\lambda}{\tnstar^2\sqrt{\tnstar}} + O \left( \frac{1}{\tnstar^2 \nstar} \right) + O \left( \frac{\lambda^2}{\tnstar^5} \right)
\end{align}
Similar result holds for $\tols$.



\subsection{Step 2: Localization step - bounding \texorpdfstring{$\phidn$}{phiN}.}
\label{apx:subsec:l1localization}

As in the proof of Theorem~\ref{thm:regressionlpmain},\ref{thm:classificationlp} in Appendix~\ref{apx:regproof},\ref{apx:claslpproof}, we defined $\eta = \norm{\wtwo}_2$ and by using parametric path approach we have that $\eta = b\norm{\gamma(\alpha)}_2$. Hence for the ease of notation we will sometimes only write  $\eta$ with dependence on $b$ and $\alpha$ implicitly assumed. 

We now derive an upper bound on $\phidn$. For this, it is sufficient to find a feasible point satisfying the constraint in the optimisation problem defining $\phidn$. Using the concentration of Lipschitz continuous function (see e.g., \cite{Ledoux1992AHS}), it is straight forward to show that:
\begin{lemma}
\label{lemma_point_conv}
For any $\nu,\eta>0$ holds that:
    \begin{align}
        \prob \left( \abs{ \fnclas \left( \nu, \eta \right) - \EE \left[ \fnclas \left( \nu, \eta \right) \right] }  \geq \epsilon \right) \leq 2 \exp \left( - c \frac{ n \epsilon^2 }{ \nu^2 + \eta^2 } \right)
    \end{align}
where $c>0$ is a positive universal constant. 
\end{lemma} 
To goal is now to use Lemma~\ref{lemma_point_conv} to relax the constraints in the optimization problem defining $\phidn$ to show the following result.

% The goal is now to show that we can find a feasible point $(\nubar, \eta)$ with $\nubar = \argmin f(\nu, 0)$ and $\eta = O \left( \frac{1}{\log(d/n)} \right)$. For this, we can take the Taylor series approximation of $f$ around $(\nuopt,0)$,   $f(\nubar, \eta) \approx \fstar + \frac{\feestar}{2} \eta^2$, which allows us to rewrite the constraint in $\phidn$ to 
% \begin{equation}
%     \frac{1}{n}  b^2\norm{\Hgaussian}_{\infty}^2  \geq  \fstar + \frac{\feestar}{2} \eta^2 + O \left( \frac{1}{\log (d/n)^{3/2}} \right).
% \end{equation}



% Further, following a similar approach as in Proposition~2 in \cite{wang2021tight} by applying the concentration results in Proposition~\ref{prop:concentrationl1}, we can show the following Proposition~\ref{prop:Rbound} which gives an upper bound on $\phidn$.

% a similar approach in the proof of Proposition~2 in \cite{wang2021tight}, where tight bounds for $\phidn$ for min-l1-norm interpolation are derived, we can show the following bound on $\phidn$ given in  Proposition \ref{prop:Rbound}. The proof may be found in Appendix~... 
\begin{proposition}
\label{prop:Rbound}
     Let the data distribution be as described in Section~\ref{subsec:clasetting} and assume that the noise model $\probsigma$ is independent of $n,d$ and $p$.
Let $t_{\nopt}$ be given by $2\Phic(t_{\nopt}) = \nopt/d$ with $\nopt = n\feestar/2$. There exist universal positive constants $c_1,c_2,c_3,c_4,c_5>0$ such that, if $n\geq c_1$ and $c_2 n\leq d\leq \exp(c_3 n^{1/5})$ then
    \begin{align} \label{phidn_bound}
        (\phidn)^2 
        \leq
        \frac{ n \fstar }{ \tnstar^2 } \left( 1 - \frac{ 2 }{ \tnstar^2 } + \frac{c_5}{ \tnstar^3 } \right) =:\loneboundclas^2
    \end{align}
with probability at least $ 1 - 2 \exp \left( -\frac{ c_4 n }{ \tnstar^6 } \right) - 6 \exp \left( -\frac{\nstar}{\log^5(d/\nstar)} \right) $ over the draws of $\Hgaussian$, $\Ggaussian$, $\Xs$ and $\xi$.
\end{proposition}  


\begin{proof}[Proof of Proposition~\ref{prop:Rbound}]

Recall that $\phidn$ is given by:
\begin{align}
    \phidn &= \min_{\nu,b,\alpha} \vert \nu \vert  + b \norm{ \gamma \left( \alpha \right) }_1 
    \subjto \frac{ b^2\norm{\Hgaussian}_{\infty}^2 }{n} \geq \fnclas \left( \nu, b \norm{ \gamma \left( \alpha \right) }_2 \right)
\end{align}

Given that $(\tnu,\tb,\talpha)$ is a feasible point of for the optimization problem defining $\phidn$ in Equation~\eqref{eq:phin_par}, we have that $\phidn \leq  \vert \tnu \vert + \tb \norm{ \gamma( \talpha) }_1$, which gives us an upper bound on $\phidn$. In the following discussion our goal is to find a single feasible point of the constraint set of $\phidn$.

From definition of $\gamma ( \alpha )$ we know that $ \norm{ \gamma ( \alpha ) }_1 = \alpha$ and hence we can equivalently formulate $\phidn$ as an optimization over $\nu$ and $ b_{\alpha} := b \alpha $
\begin{align}
    \phidn &= \min_{ \nu, b_{\alpha} } \nu + b_{\alpha}
    \subjto \frac{ b_{\alpha}^2 \norm{\Hgaussian}_{\infty}^2 }{n \alpha^2} \geq \fnclas \left( \nu, b_{\alpha} \frac{ \norm{ \gamma \left( \alpha \right) }_2}{ \alpha } \right)
\end{align}

 Using Lemma \ref{lemma_point_conv} with $ \epsilon = \fstar \tnstar^{-3} $ and for a feasible point $( \nu, b_{\alpha} \frac{ \norm{ \gamma \left( \alpha \right) }_2}{ \alpha } )$ we have that:
\begin{align} \label{eq:constraint_f_conc}
    \frac{ b_{\alpha}^2 \norm{\Hgaussian}_{\infty}^2 }{n \alpha^2} 
    \geq
    f \left( \nu, b_{\alpha} \frac{ \norm{ \gamma \left( \alpha \right) }_2}{ \alpha } \right) + \frac{\fstar}{\tnstar^{3}}
\end{align}
with probability at least $ 1 - 2 \exp \left( -c \frac{ n }{ \tnstar^6 \left( \nu^2 + b_{\alpha}^2  \norm{ \gamma \left( \alpha \right) }_2^2 / \alpha^2 \right) } \right) $.
% > 1 - 2 \exp \left( - \tc \frac{ n }{ \log^3 \left( \frac{d}{n} \right)  } \right) $.

Let's now choose $ \nu = \nubar $ and show that there exists a pair $ ( b, \alpha )$  such that $ ( \nubar, b, \alpha) $ is feasible for constraint \eqref{eq:constraint_f_conc}. Furthermore, we propose to search for a point with parameter $ ( b, \alpha ) $ such that $ b \norm{ \gamma ( \alpha )}_2 = b_{\alpha} \frac{ \norm{ \gamma \left( \alpha \right) }_2}{ \alpha } $ is near zero. Hence, using Taylor series approximation of the function $ f ( \nubar, \cdot ) : \eta \mapsto f (\nubar, \eta) $ around  the point $(\nuopt,0)$ we can rewrite the constraint \eqref{eq:constraint_f_conc} as:
\begin{align}
     \frac{ b_{\alpha}^2 \norm{\Hgaussian}_{\infty}^2 }{n \alpha^2}   
     \geq
      \fstar + \frac{1}{2}\feestar b_{\alpha}^2 \frac{ \norm{ \gamma \left( \alpha \right) }_2^2}{ \alpha^2 } + O \left( b_{\alpha}^3 \frac{ \norm{ \gamma \left( \alpha \right) }_2^3}{ \alpha^3 } \right) + \frac{\fstar}{\tnstar^{3}}
\end{align}
since $\zeta_{\eta} := \frac{\partial f(\nuopt,\eta)}{\partial \eta}\Big|_{\eta=0} = 0$ and where we recall that by definition $\fstar = f \left( \nubar, 0 \right)$, $\feestar = \frac{\partial^2 f(\nuopt,\eta)}{\partial \eta^2}\Big|_{\eta=0}$ and $\nstar = \frac{1}{2}\feestar n$.

As we mentioned in section \ref{step_1_thm3_proof}, $ \gamma ( \alpha ) $ is a piecewise linear function with breakpoints at $ \alpha_s $ for $ s = 2, \dots, d $. Hence instead of optimizing over $\alpha$ we optimize over $s$. Note that we have only one constraint but two free variables $ ( b, \alpha ) $ and so we can set $ \alpha = \alpha_{\nstar} $ with $ \nstar = \frac{1}{2}\feestar n $. To gain an intuition for why this choice is approximately optimal, one can follow a similar argument as in Remark 1 in \cite{wang2021tight}.  Combining all the previous results we get the constraint:
\begin{align} \label{eq:B_ineq}
     \frac{ b_{\alpha_{\nstar}}^2 \norm{\Hgaussian}_{\infty}^2 }{n \alpha_{\nstar}^2}   
     \geq
      \fstar + \frac{1}{2}\feestar b_{\alpha_{\nstar}}^2 \frac{ \norm{ \gamma \left( \alpha_{\nstar} \right) }_2^2}{ \alpha_{\nstar}^2 } + O \left( b_{\alpha_{\nstar}}^3 \frac{ \norm{ \gamma \left( \alpha_{\nstar} \right) }_2^3}{ \alpha_{\nstar}^3 } \right) + \frac{\fstar}{\tnstar^{3}}
\end{align}

We now claim that
\begin{equation}
    b_{\alpha_{\nstar}}^2 = \frac{ n \alpha_{\nstar}^2 }{ \norm{\Hgaussian}_2^2 } \frac{ \fstar \left( 1 + \frac{1}{\tnstar^{3}} \right) }{ 1 - \frac{1}{2} n \feestar \frac{ \norm{ \gamma \left( \alpha_{\nstar} \right) }_2^2 }{ \norm{H}_{\infty}^2 } - O \left( \frac{1}{\tnstar^3} \right) }
\end{equation}
satisfies inequality \eqref{eq:B_ineq} with probability at least $ 1 - 6 \exp \left( -\frac{2\nstar}{\log^5(d/\nstar)} \right)$. Using Proposition \ref{lemma_gamma_conc} we have that:
\begin{equation}
    1 - \frac{1}{2} n \feestar \frac{ \norm{ \gamma \left( \alpha_{\nstar} \right) }_2^2 }{ \norm{H}_{\infty}^2 } - O \left( \frac{1}{\tnstar^3} \right) > 1 - \frac{1}{2} n \feestar  \frac{2}{\nstar \tnstar^2} - O \left( \frac{1}{\tnstar^3} \right) = 1 - \frac{2}{\tnstar^2} - O \left( \frac{1}{\tnstar^3} \right)  > 0
\end{equation}
holding for $d,n$ sufficiently large. Applying Lemma \ref{lemma_gamma_conc} once again we get:
\begin{equation}
    b_{\alpha_{\nstar}}^2 
    \leq
    \frac{ n \fstar }{ \tnstar^2 } \left( 1 + \frac{1}{\tnstar^3} \right) \left( 1 - \frac{4}{\tnstar^2} + \frac{c}{\tnstar^4} \right) \frac{1}{ 1 - \frac{2}{\tnstar^2} - O \left( \frac{1}{\tnstar^3} \right)}
    \leq
    \frac{ n \fstar }{ \tnstar^2 } \left( 1 - \frac{2}{\tnstar^2} + \frac{c}{\tnstar^3} \right)
\end{equation}

Hence we have that $ O \left( b_{\alpha_{\nstar}}^3 \frac{ \norm{ \gamma \left( \alpha_{\nstar} \right) }_2^3}{ \alpha_{\nstar}^3 } \right) = O \left( \frac{1}{\tnstar^3} \right)$ and this $b_{\alpha_{\nstar}}^2$ indeed satisfies equation \eqref{eq:B_ineq}. Now we define the upper bound on $\phidn$ as:
\begin{align}
\label{eq:lonebound_def}
    \loneboundclas := \sqrt{ \frac{ n \fstar }{ \tnstar^2 } \left( 1 - \frac{2}{\tnstar^2} + \frac{c}{\tnstar^3} \right) }
\end{align}
which holds with probability at least $ 1 - 2 \exp \left( -c \frac{ n }{ \tnstar^6 \left( \nubar^2 + b_{\alpha_{\nstar}}^2  \norm{ \gamma \left( \alpha_{\nstar} \right) }_2^2 / \alpha_{\nstar}^2 \right) } \right) - 6 \exp \left( -\frac{2\nstar}{\log^5(d/\nstar)} \right) $. The proposition is proved after noting that $ \nubar^2 + b_{\alpha_{\nstar}}^2  \norm{ \gamma \left( \alpha_{\nstar} \right) }_2^2 / \alpha_{\nstar}^2 = O(1)$.

\end{proof}

































\subsection{Step 3: Uniform convergence.}
\label{apx:subsec:l1uniform}
The goal of this step is to study the constraint set $\Gamma_0$ from Proposition~\ref{prop:parametrization} with $\loneboundclas \geq \phidn$ from the previous step. In particular, we show the following Proposition ~\ref{prop:BoundOmegal1}. The bounds on $\phidp$ and $\phidm$ then follow straightforwardly as proven after the proposition statement. 

\begin{proposition}
\label{prop:BoundOmegal1}
    Let the data distribution be as described in Section~\ref{subsec:clasetting} and assume that the noise model $\probsigma$ is independent of $n,d$ and $p$.
Under the same conditions on $n,d$ as in Theorem~\ref{thm:mainl1},
there exist universal constants $ c_1, c_2, c_3, c_4 > 0 $ such that, if $ n\geq c_1 $ and $ c_2 n \leq d \leq \exp \left( c_3 n^{1/5} \right) $, then
\begin{align}
    \Gamma_0 
    \subset
    \left\{ (\nu, b, \alpha) \subjto  
    \abs{ \eta^2 - \frac{2\fstar}{\feestar \log(d/\nstar) } } =   O \left( \frac{1}{\log^{5/4}(d/\nstar)} \right) ~~\andtxt~~ 
    \deltanu^2 = \abs{ \nu-\nubar }^2 = O \left( \frac{1}{ \log(d/\nstar)} \right) \right\} =: \tilde{\Gamma}
    % \frac{2 \fstar \lambda}{\fnstar}\frac{1}{\log(d/n)^{5/4}} \left( 1 + O \left( \frac{1}{\log(d/n)^{1/4}} \right) \right) \} %
\end{align}
with probability at least $ 1 - c_4 \exp\left(-\frac{n}{\log^6(d/n)}\right) $ over the draws of $\Hgaussian$, $\Ggaussian$, $\Xs$ and $\xi$ and with $\nstar = n \feestar/2$.
\end{proposition}  
%\subsection{Summary. }
From the Propositions \ref{prop:CGMT_application_classification} and \ref{prop:BoundOmegal1} we get the following bounds on $\phidp$ and $\phidm$:
\begin{align}
    %\max_{\nu,\eta} \frac{ \nu }{ \sqrt{ \nu^2 + \eta^2 } } 
    \phidp
    & \leq \left(1 + \frac{\min_{\eta \in \tilde{\Gamma}} ~\eta^2}{\max_{\nu \in \tilde{\Gamma}}~ \nu^2}  \right)^{-1/2}
    % \frac{1}{ \sqrt{ (1 + \frac{\eta^2 }{ (\nubar + \deltanu)^2}} }
    % \\
    % & = 
    % \left( 1 + \frac {\deltanu}{\nubar} \right) \left( 1 - \frac{1}{2} \left( \frac{2\deltanu}{\nubar} + \frac{\deltanu^2 + \eta^2}{(\nubar)^2} \right) + \frac{3}{8} \left( \frac{2\deltanu}{\nubar}\right)^2 + O \left( \deltanu^3, \deltanu \eta^2, \eta^4 \right) \right)
    % \\
    % & = 1 - \frac{\eta^2}{2(\nubar)^2} + O \left( \frac{1}{ \tnstar^{13/4}} \right) 
    % \leq 
    % %1 - W \left( \frac{1}{\log (d/n) } \right)
    % 1 - \frac{ 2 \fstar }{ \feestar (\nubar)^2 } \frac{1}{\tnstar^2} + \frac{\lambda}{\tnstar^{5/2}} +O \left( \frac{1}{ \tnstar^{13/4}} \right) 
    % \\
    % & = 1 - \frac{ \fstar }{ \feestar (\nubar)^2 } \frac{1}{ \log(d/ \nstar)} + \frac{\lambda}{2\log(d/\nstar)^{5/4}} + O \left( \frac{1}{ \log (d/n)^{13/8}} \right)
    % \\
     \leq 1 - \frac{ \fstar }{ \feestar \nubar^2 } \frac{1}{ \log(d/ \nstar)} \left( 1 -O\left( \frac{1}{\log(d/\nstar)^{1/4}} \right)\right) \\
    & \leq 1 -  \frac{\kappanoise}{2 \log(d/ \nstar)} \left( 1 - O\left(\frac{1}{\log(d/\nstar)^{1/4}}\right) \right) \\
\end{align}
and
\begin{align}
    %\min_{\nu,\eta} \frac{ \nu }{ \sqrt{ \nu^2 + \eta^2 } } 
    \phidm &\geq \left(1 + \frac{\max_{\eta \in \tilde{\Gamma}} ~\eta^2}{\min_{\nu \in \tilde{\Gamma}}~ \nu^2}  \right)^{-1/2}
    % & \geq
    % \frac{ \nubar - \deltanu }{ \sqrt{ ( \nubar - \deltanu )^2 + \eta^2 } }
    % \\
    % & = 
    % \left( 1 - \frac {\deltanu}{\nubar} \right) \left( 1 - \frac{1}{2} \left( -\frac{2\deltanu}{\nubar} + \frac{\deltanu^2 + \eta^2}{(\nubar)^2} \right) + \frac{3}{8} \left( \frac{2\deltanu}{\nubar}\right)^2 + O \left( \deltanu^3, \deltanu \eta^2, \eta^4 \right) \right)
    % \\
    % & = 1 - \frac{\eta^2}{2(\nubar)^2} + O \left( \frac{1}{ \tnstar^{13/4}} \right) 
    % \geq 
    % %1 - W \left( \frac{1}{\log (d/n) } \right)
    % 1 - \frac{ 2 \fstar }{ \feestar (\nubar)^2 } \frac{1}{\tnstar^2} - \frac{ \lambda }{\tnstar^{5/2}} +O \left( \frac{1}{ \tnstar^{13/4}} \right) 
    % \\
    % & = 1 - \frac{ \fstar }{ \feestar (\nubar)^2 } \frac{1}{ \log(d/ \nstar)} - \frac{\lambda}{2\log(d/\nstar)^{5/4}} + O \left( \frac{1}{ \log (d/n)^{13/8}} \right)
    % \\
     \geq 1 - \frac{ \fstar }{ \feestar (\nubar)^2 } \frac{1}{ \log(d/ \nstar)} \left( 1 +O\left( \frac{1}{\log(d/\nstar)^{1/4}}\right) \right)\\
    & \geq 1 -  \frac{ \kappanoise}{2 \log(d/ \nstar)} \left( 1 + O\left(\frac{1}{\log(d/\nstar)^{1/4}}\right) \right)
\end{align}

% \red{edit to match new risk} Using approximation $ \arccos(1-x) \approx \sqrt{2x} + O (x\sqrt{x}) $ we can bound $R(\what)$ as follows:
% \begin{align}
%     %W \left( \frac{1}{\log (d/n)^{1/2} }  \right) 
%     \sqrt{\frac{ 2 \fstar }{ \fnstar (\nubar)^2 }} \frac{1}{\sqrt{\log (d/ \nstar)}} \left( 1 - \frac{\lambda'}{\log(d/\nstar)^{1/4}} \right)
%     \leq
%     R(w) = \frac{1}{\pi} \arccos \left( \frac{\innerprod{w}{\wgt}}{\norm{w}_2} \right) 
%     \leq 
%     \sqrt{\frac{ 2 \fstar }{ \fnstar (\nubar)^2 }} \frac{1}{\sqrt{\log (d/ \nstar)}} \left( 1 + \frac{\lambda'}{\log(d/\nstar)^{1/4}} \right)
% \end{align}
% \begin{align}
%     %\frac{1}{\pi} \arccos \left( \frac{\innerprod{ \what }{ \wgt }}{ \norm{\what}_2 } \right)
%     \abs{ R(\what) - \frac{ \sqrt{2 \fstar} }{ \nubar \pi \sqrt{\feestar} } \frac{1}{\sqrt{\log (d/ \nstar)}} }
%     \leq 
%     \frac{\lambda'}{\log(d/n)^{5/4}}
% \end{align}
% Thus, we can bound the risk $\Risk(\what)$ as
% \begin{align}
%     \abs{ \Risk(\what) - \frac{ 2 \fbar }{ \nubar^2 \feebar } \frac{1}{\log (d/ n)} }
%     \leq 
%     \frac{\lambda'}{\log(d/n)^{5/4}}
% \end{align}
% with probability at least $ 1 - $ over the draws of the data set.




\subsection{Proof of Proposition~\ref{prop:BoundOmegal1}}
The proof of the proposition follows from several steps where in each step we approximate $\fnclas$ using the bounds on $(\nu, \eta)$ from the previous steps to obtain a tighter bound on $(\nu, \eta)$ using the tools developed in \cite{wang2021tight}.  
The probability statement in Proposition~\ref{prop:BoundOmegal1} follows when taking the union bound over all equations which we condition on throughout the proof. 
Furthermore, we note that $\Gamma_0$ is not empty as it clearly the choice $\alpha=\alpha_n$ leads with high probability to a feasible point due to the choice of $M$ in Proposition~\ref{prop:Rbound}. 




\subsubsection{Bound 1: \texorpdfstring{$\nu^2,\eta^2 = O(1)$}{}} \label{sec:l1class_nueta_const_bound}
In order to apply Lemma~\ref{lemma_quadratic_plus_fstar_bound} in the next step,  which gives tight bounds for $\fnclas$, we first need to show that with high probability, $\nu^2,\eta^2 = O(1)$. This is the goal of this first step. More specifically, 
the goal of this first step is to show that there exist universal constants $B_{\nu,1}, B_{\eta,1} > 0$ such that for any element $(\nu, b, \alpha)$ of $\Gamma_0$ we have that $ \nu \leq B_{\nu,1} $ and $ \eta = b \norm{ \gamma(\alpha)}_2 \leq B_{\eta,1}$ with probability high probability over the draws of $\Hgaussian,\Ggaussian$ and $\Xs, \xi$. 

For this first step, we use the fact that in the presence of label noise, $\fnclas$ is lower bounded by a quadratic function as stated in Lemma ~\ref{quadratic_bound_fn}. 
As a result, we can relax the first constraint in Definition \eqref{eq:Omega_0_def} of $\Gamma_0$ to 
\begin{equation}
    \frac{1}{n} b^2\norm{\Hgaussian}_{\infty}^2  \geq  \constnu \nu^2  + \consteta  b^2 \norm{\gamma(\alpha)}_2^2 .
\end{equation} 
 
% \red{say more about the intuition, then we can show:}
This approximation leads to an optimization problem similar to the ones discussed in Lemma 1 in \cite{wang2021tight}. After further relaxations we obtain exactly the same form of the inequality, and hence we can use the arguments from \cite{wang2021tight}. 

% \begin{lemma} \label{lemma_first_reduction}
%     There exist universal constants $B_{\nu,1}, B_{\eta,1} > 0$ such that for any element $(\nu, b, \alpha)$ of $\Gamma_0$ we have that $ \nu \leq B_{\nu,1} $ and $ \eta = b \norm{ \gamma(\alpha)}_2 \leq B_{\eta,1}$ with probability at least $ 1 - $ over the draws of $H$ and the data set.
% \end{lemma}


% According to Lemma \ref{quadratic_bound_fn} we have that for any pair $ ( \nu, \eta ) $ with probability at least $ 1 - \exp \left( - n \kldiv{\frac{\sigma}{2}}{\frac{\sigma}{4}} \right) - \exp \left( -\frac{ n\sigma }{ 128 } \right) $ that $ \fnclas ( \nu, \eta) \geq \constnu \nu^2 + \consteta \eta^2 $ for some positive constants $\constnu$ and $\consteta $. Hence with high probability we can relax first constraint defining $\Gamma_0$ to
% % \begin{align}
% %     \frac{ \innerprod{\wtwo}{H}^2 }{ n } \geq \constnu \nu^2 + \consteta  \eta^2
% % \end{align}
% \begin{align}
%     \frac{1}{n} b^2 \norm{H}_{\infty}^2 \geq \constnu \nu^2 + \consteta b^2 \norm{\gamma(\alpha)}_2^2    
% \end{align}

Let's first consider bounding of $\eta$ and then we use the obtained result to bound $\nu$.
\paragraph{Upper bound on $\eta$.}
For this part of the proof we further relax both constraints from Definition \eqref{eq:Omega_0_def} of $\Gamma_0$ and define the following set:
\begin{align}
    \Gamma_1^{\eta} &= \left\{ (\nu, b, \alpha) \subjto \frac{1}{n} b^2 \norm{H}_{\infty}^2 \geq \consteta  b^2 \norm{\gamma(\alpha)}_2^2 \andtxts b \alpha \leq \loneboundclas  \right\} \\
    &= \left\{ (\nu, b, \alpha) \subjto \frac{1}{n} \norm{H}_{\infty}^2 \geq \consteta  \norm{\gamma(\alpha)}_2^2 \andtxts b \alpha \leq \loneboundclas  \right\} \label{eq:lpstep1set}
\end{align}
% \begin{align}
%     \Gamma_1^{\eta} = \left\{ (\wone,\wtwo) \subjto \frac{ \innerprod{\wtwo}{H}^2 }{ n } \geq \consteta  \eta^2 \andtxts \norm{ \wtwo }_1 \leq \loneboundclas  \right\}
% \end{align}
It is evident from definition that $ \Gamma_0 \subset \Gamma_1^{\eta}$ with high probability. Also note that constraints in the set $\Gamma_1^{\eta}$ do not depend on $\nu$ and hence we will now consider only variables $b$ and $\alpha$ and bound $ \eta $ as:
\begin{align}
    &\eta^2 \leq \left[\max_{b,\alpha} b^2 \norm{\gamma(\alpha)}_2^2 \subjto (b,\alpha) \in \Gamma_1^{\eta} \right]
    =  \left[
    \max_{1\leq \alpha \leq \alpham} \loneboundclas^2 \frac{ \norm { \gamma ( \alpha ) }_2^2 }{ \alpha^2 } 
    \subjto
    %B\gamma \left( \alpha \right) \in \Gamma_1^{\eta}
    \left( \frac{\loneboundclas}{\alpha}, \alpha \right) \in \Gamma_1^{\eta} \right]
    \label{eq:l1proofstep1bound}
\end{align}

Now note that as discussed in Appendix~\ref{apx:subsec:l1path} $\norm{\gamma(\alpha)}_2^2$ is convex. Therefore, the set of feasible $\alpha$ in the Set $\Gamma_1^{\eta}$ is an non-empty interval. Indeed, to see that the interval is non empty, recall that we defined $ \loneboundclas $ in such way that $ (b,\alpha_{\nstar}) \in \Gamma_0 $ with high probability for $b \alpha_{\nstar}\leq \loneboundclas$. As $ \Gamma_0 \subset \Gamma_1^{\eta}$, with high probability there exists some $ b > 0 $ such that $ (b, \alpha_{\nstar} ) \in \Gamma_1^{\eta} $ proving that $\Gamma_1^{\eta} \neq \emptyset$. Furthermore,  since $\frac{ \norm { \gamma ( \alpha ) }_2^2 }{ \alpha^2 }$ is monotonically decreasing, to upper bound Equation~\eqref{eq:l1proofstep1bound} it is sufficient to find $\ulalpha < \alpha_{\nstar}$ such that
\begin{align}
\label{eq:s_condition_one}
    \norm{\gamma(\ulalpha)}_2^2 > \frac{1}{\consteta n} \norm{H}_{\infty}^2. 
\end{align}

It is sufficient to only consider the discretized version of $\alpha$, i.e., $\alpha_s$, for which we have access to tight concentration inequalities from Proposition~\ref{prop:concentrationl1}. We now  claim that $\alpha_{\uls}$ with $\uls =\lambda_{\uls} \frac{ n }{ \log (d/n) }$ satisfies the inequality Equation~\eqref{eq:s_condition_one} for some positive universal constant $ \lambda_{\uls} >0  $. Using the characterization $t_s^2 = 2\log (d/s) + O (\log \log (d/s) ) $ from section \ref{step_1_thm3_proof} we get:
\begin{align}
    \frac{ 2 }{ \uls \tuls^2 } \left( 1 - O \left( \frac{ 1 }{ \tuls^2 } \right) \right)
    & >
    \frac{ 1 }{ n \lambda_{\uls} } \left( 1 - O \left( \frac{\log\log (d/n) }{\log (d/n) } \right) \right) > \frac{1}{\consteta n}
\end{align}
where last inequality holds for $d/n$ sufficiently large and $\lambda_{\uls}$ small enough.

Therefore, from Equation~\eqref{eq:l1proofstep1bound} and the concentration inequality from Proposition \ref{lemma_gamma_conc}, we get:
\begin{align}
    \eta^2 \leq \frac{ n \fstar }{ \tnstar^2 } \frac{2}{\uls}\left( 1 + O \left( \frac{1}{\tuls^2} \right) \right) %\leq \boundeta' \left( 1 + O \left( \frac{1}{ \log (d/n) } \right) \right) 
    =: B_{\eta,1}^2,
\end{align}
with $B_{\eta,1}= \Theta (1)$, as desired. 

\paragraph{Upper bound on $\nu$.} Now we derive an upper bound for $\nu$. Using the result from the previous sub-step, we consider the following set:
\begin{align}
    \Gamma_1^{\nu} = \left\{ (\nu, b, \alpha) 
    \subjto
    \frac{1}{n} b^2 \norm{H}_{\infty}^2 \geq \constnu \nu^2 \andtxts b\alpha \leq \loneboundclas \andtxts b\norm{\gamma(\alpha)}_2 \leq B_{\eta,1} \right\}
    %\frac{ \innerprod{\wtwo}{H}^2 }{ n } \geq \constnu \norm{\wone}_2^2 \andtxts \norm{ \wtwo }_1 \leq \loneboundclas \andtxts \norm{ \wtwo }_2 \leq \boundeta  \right\}
\end{align}
% \begin{align}
%     \Gamma_1^{\nu} = \left\{ (\wone,\wtwo) 
%     \subjto
%     \frac{ \innerprod{\wtwo}{H}^2 }{ n } \geq \constnu \nu^2 \andtxts \norm{ \wtwo }_1 \leq \loneboundclas \andtxts \norm{ \wtwo }_2 \leq \boundeta  \right\}
% \end{align}
Clearly, we have again  $\Gamma_0 \subset \Gamma_1^{\nu}$ with high probability. Hence we can upper bound $\nu$ as follows:
\begin{align} \label{eq:nu_opt_first_reduction}
    \nu^2 &\leq \frac{ 1 }{ n \constnu } \left[\max_{b,\alpha} b^2 \norm{H}_{\infty}^2
    \subjto 
    b^2 \leq \frac{\loneboundclas^2}{\alpha^2}
    \andtxts 
    b^2 \leq \frac{B_{\eta,1}^2}{\norm{ \gamma(\alpha)  }_2^2}\right]
    \\
    &= \frac{ 1 }{ n \constnu }  \norm{H}_{\infty}^2 ~\max_{\alpha}\min\left(\frac{\loneboundclas^2}{\alpha^2}, \frac{B_{\eta,1}^2}{\norm{\gamma(\alpha)}_2^2}\right)
\end{align}
Now recall that $\norm{\gamma(\alpha)}_2$ is convex with global minimum at $\alpha_{d+1/2} = \frac{\norm{H}_1 \norm{H}_{\infty}}{\norm{H}_2^2}$ (see Lemma 4 in \cite{wang2021tight}). Thus, the optimal $\alphaopt$ is obtained for $\alphaopt < \alpha_{d+1/2}$ with 
\begin{equation}
    \frac{\loneboundclas^2}{\alphaopt^2} =  \frac{B_{\eta,1}^2 }{\norm{\gamma(\alphaopt)}_2^2}.
\end{equation}
We now show that we can upper and lower bound by $\alpha_{\uls} <\alphaopt < \alpha_{\ols}$ with high probability with $\uls =  \lambda_{\uls} \frac{ \nstar}{ \log (d/\nstar)} $ and $\ols =  \lambda_{\ols} \frac{ \nstar }{ \log (d/\nstar) }$ and $0<\lambda_{\uls}<1< \lambda_{\ols}$ universal constants. For this, we need to show that with high probability, 
\begin{align}
        \frac{\norm{\gamma(\alphaols)}_2^2}{\alphaols^2} <  \frac{B_{\eta,1}^2 }{\loneboundclas^2} < \frac{\norm{\gamma(\alphauls)}_2^2}{\alphauls^2}.
\end{align}
However,  similarly to bounding $\eta$ in the previous sub-step, we can straight forwardly verify that this statement holds with high probability when using Proposition~\ref{prop:concentrationl1} and the characterization $t_s = 2\log (d/s) + O (\log \log (d/s) ) $ from section \ref{step_1_thm3_proof}. 
Therefore, as a result, we obtain the desired upper bound
\begin{align}%\label{eq:nu_opt_first_reduction}
    \nu^2 &\leq  \frac{ 1 }{ n \constnu }  \norm{H}_{\infty}^2 ~\min\left(\frac{\loneboundclas^2}{\alphauls^2}, \frac{B_{\eta,1}^2}{\norm{\gamma(\alphaols)}_2^2}\right) \leq \frac{ 1 }{ n \constnu }  \norm{H}_{\infty}^2 ~\frac{\loneboundclas^2}{\alphauls^2}
    =: B_{\nu,1},
\end{align}
and in particular, we have again that $B_{\nu,1} = \Theta(1)$, which completes the first step of the proof. 














% \subsubsection{Bound 1: $\nu^2,\eta^2 = O(1)$} \label{sec:l1class_nueta_const_bound}
% The goal of this first step is to show that there exist universal constants $B_{\nu,1}, B_{\eta,1} > 0$ such that for any element $(\nu, b, \alpha)$ of $\Gamma_0$ we have that $ \nu \leq B_{\nu,1} $ and $ \eta = b \norm{ \gamma(\alpha)}_2 \leq B_{\eta,1}$ with probability high probability over the draws of $\Hgaussian,\Ggaussian$ and $\Xs, \xi$. 

% For this first step, we use the fact that in the presence of label noise, $\fnclas$ is lower bounded by a quadratic function as stated in Lemma ~\ref{quadratic_bound_fn}. 
% As a result, we can relax the first constraint in definition \eqref{eq:Omega_0_def} of $\Gamma_0$ to 
% \begin{equation}
%     \frac{1}{n} b^2\norm{\Hgaussian}_{\infty}^2  \geq  \constnu \nu^2  + \consteta  b^2 \norm{\gamma(\alpha)}_2^2 .
% \end{equation} 
 
% % \red{say more about the intuition, then we can show:}
% This approximation leads to an optimization problem similar to the ones discussed in Lemma 1 in \cite{wang2021tight}. After further relaxation we obtain exactly the same form of the inequality, and hence we can use arguments from \cite{wang2021tight}. 

% % \begin{lemma} \label{lemma_first_reduction}
% %     There exist universal constants $B_{\nu,1}, B_{\eta,1} > 0$ such that for any element $(\nu, b, \alpha)$ of $\Gamma_0$ we have that $ \nu \leq B_{\nu,1} $ and $ \eta = b \norm{ \gamma(\alpha)}_2 \leq B_{\eta,1}$ with probability at least $ 1 - $ over the draws of $H$ and the data set.
% % \end{lemma}


% % According to Lemma \ref{quadratic_bound_fn} we have that for any pair $ ( \nu, \eta ) $ with probability at least $ 1 - \exp \left( - n \kldiv{\frac{\sigma}{2}}{\frac{\sigma}{4}} \right) - \exp \left( -\frac{ n\sigma }{ 128 } \right) $ that $ \fnclas ( \nu, \eta) \geq \constnu \nu^2 + \consteta \eta^2 $ for some positive constants $\constnu$ and $\consteta $. Hence with high probability we can relax first constraint defining $\Gamma_0$ to
% % % \begin{align}
% % %     \frac{ \innerprod{\wtwo}{H}^2 }{ n } \geq \constnu \nu^2 + \consteta  \eta^2
% % % \end{align}
% % \begin{align}
% %     \frac{1}{n} b^2 \norm{H}_{\infty}^2 \geq \constnu \nu^2 + \consteta b^2 \norm{\gamma(\alpha)}_2^2    
% % \end{align}

% Let's first consider bounding of $\eta$ and then we use obtained result to bound $\nu$.
% \paragraph{Upper bound on $\eta$.}
% For this part of the proof we further relax both constraints from definition \eqref{eq:Omega_0_def} of $\Gamma_0$ and define the following set:
% \begin{align}
%     \Gamma_1^{\eta} = \left\{ (\nu, b, \alpha) \subjto \frac{1}{n} b^2 \norm{H}_{\infty}^2 \geq \consteta  b^2 \norm{\gamma(\alpha)}_2^2 \andtxts b \alpha \leq \loneboundclas  \right\}
% \end{align}
% % \begin{align}
% %     \Gamma_1^{\eta} = \left\{ (\wone,\wtwo) \subjto \frac{ \innerprod{\wtwo}{H}^2 }{ n } \geq \consteta  \eta^2 \andtxts \norm{ \wtwo }_1 \leq \loneboundclas  \right\}
% % \end{align}


% It is evident from definition that $ \Gamma_0 \subset \Gamma_1^{\eta}$ with high probability. Also note that constraints in the set $\Gamma_1^{\eta}$ do not depend on $\nu$ and hence we will now consider only variables $b$ and $\alpha$. Now we bound $ \eta $ as:
% \begin{align}
%     \eta^2 \leq \max_{b,\alpha} b^2 \norm{\gamma(\alpha)}_2^2 \subjto (b,\alpha) \in \Gamma_1^{\eta}
% \end{align}

% We proceed following the path arguments established in \cite{wang2021tight}. First we show that set $\Gamma_1^{\eta}$ is not empty. Let's choose $ \alpha = \alpha_{\nstar}$ with $\nstar = n\feestar/2$. Recall that we defined $ \loneboundclas $ in such way that $ (b,\alpha_{\nstar}) \in \Gamma_0 $ with high probability for $b \alpha_{\nstar}\leq \loneboundclas$. As $ \Gamma_0 \subset \Gamma_1^{\eta}$, with high probability there exists some $ b > 0 $ such that $ (b, \alpha_{\nstar} ) \in \Gamma_1^{\eta} $ proving that $\Gamma_1^{\eta} \neq \emptyset$.

% Recall from definition \eqref{eq:def_gamma_alpha} that $\norm{\gamma(\alpha)}_1 = \alpha$. Then using the same arguments as in Lemma 1 in \cite{wang2021tight}, we set $ b = \frac{\loneboundclas}{\alpha} $ and obtain:
% \begin{align}
% \label{eq:step_one_eta_bound_alpha}
%     \eta^2 
%     \leq
%     \max_{1\leq \alpha \leq \alpham} \loneboundclas^2 \frac{ \norm { \gamma ( \alpha ) }_2^2 }{ \norm { \gamma ( \alpha ) }_1^2 } 
%     \subjto
%     %B\gamma \left( \alpha \right) \in \Gamma_1^{\eta}
%     \left( \frac{\loneboundclas}{\alpha}, \alpha \right) \in \Gamma_1^{\eta}
% \end{align}

% As mentioned in section \ref{step_1_thm3_proof} the map $ \alpha \mapsto \frac{ \norm{ \gamma ( \alpha ) }_2^2 }{ \norm{ \gamma ( \alpha ) }_1^2 } $ is monotonically decreasing and the mapping $ \alpha \mapsto \consteta b^2 \norm{\gamma(\alpha)}_2^2 $ is convex. The interval of $\alpha \in [1,\alpham]$ for which constraint in equation \eqref{eq:step_one_eta_bound_alpha} holds is an interval since it is as a sublevel set of a convex function. Therefore if we find value of $\alpha_{\uls}$ such that $\alphauls \leq \alpha_{\nstar}$ and $ ( \frac{M}{\alphauls}, \alphauls ) \not \in \Gamma_1^{\eta}$, then we have:
% \begin{align} \label{eq:eta_bound_first_reduction}
%     \eta^2 \leq  \loneboundclas^2 \frac{ \norm { \gamma ( \alphauls ) }_2^2 }{ \norm { \gamma ( \alphauls ) }_1^2 }
% \end{align}

% % In order to saturate constraint $ \norm{ \wtwo }_1 \leq \loneboundclas $ let $ b = \frac{\loneboundclas}{\alphauls}$. 
% In order to have $ ( \frac{M}{\alphauls}, \alphauls ) \not \in \Gamma_1^{\eta}$ we will chose $\uls$ as the smallest integer for which first constraint in definition of $\Gamma_1^{\eta}$ is not satisfied, i.e. choose  $\uls$ satisfying
% % \begin{align}
% %     \loneboundclas^2 \frac{ \innerprod{ \gamma ( \alphauls )}{H}^2 }{ n \alphauls^2 } < \consteta \loneboundclas^2 \frac{ \norm{ \gamma ( \alphauls ) }_2^2 }{ \alphauls^2 }
% % \end{align}
% \begin{align}
% \label{eq:s_condition_one}
%     \frac{1}{n} \frac{\loneboundclas^2}{\alphauls^2} \norm{H}_{\infty}^2 
%     <
%     \consteta \frac{\loneboundclas^2}{\alphauls^2} \norm{ \gamma ( \alphauls ) }_2^2 
% \end{align}
% % Rewriting this inequality gives:
% % \begin{align} \label{eq:s_condition_one}
% %   \frac{ \norm{ \gamma ( \alphauls ) }_2^2 }{ \norm{H}_{\infty}^2 } > \frac{ 1 }{ \consteta n } 
% % \end{align}
% After rewriting and using concentration result from Proposition \ref{lemma_gamma_conc} we obtain the following condition on $\uls$:
% \begin{align}
%     \frac{ 2 }{ \uls \tuls^2 } \left( 1 - O \left( \frac{ 1 }{ \tuls^2 } \right) \right) > \frac{ 1 }{ \consteta n }
% \end{align}

%  We claim that $\uls =\lambda_{\uls} \frac{ n }{ \log (d/n) }$ satisfies this inequality for some positive universal constant $ \lambda_{\uls} >0  $. Using characterization $t_s = 2\log (d/s) + O (\log \log (d/s) ) $ from section \ref{step_1_thm3_proof} we get:
% \begin{align}
%     \frac{ 2 }{ \uls \tuls^2 } \left( 1 - O \left( \frac{ 1 }{ \tuls^2 } \right) \right) 
%     & >
%     % \frac{ 2\log (d/n)  }{ n \lambda_{\uls} } \frac{ 1 }{ 2\log (d/\uls) + O \left(\log \log (d/\uls) \right) } \left( 1 - O \left( \frac{1}{\log (d/n)} \right) \right)
%     % \\
%     % & = 
%     \frac{ 1 }{ n \lambda_{\uls} } \left( 1 - O \left( \frac{\log\log (d/n) }{\log (d/n) } \right) \right) > \frac{1}{\consteta n}
% \end{align}
% where last inequality holds for $d/n$ sufficiently large and $\lambda_{\uls}$ small enough.

% Now from equation \eqref{eq:eta_bound_first_reduction} and concentration Proposition \ref{lemma_gamma_conc}, for some positive constant $B_{\eta,1}$ we get:
% \begin{align}
%     \eta^2 \leq \frac{ n \fstar }{ \tnstar^2 } \frac{2}{\uls}\left( 1 + O \left( \frac{1}{\tuls^2} \right) \right) %\leq \boundeta' \left( 1 + O \left( \frac{1}{ \log (d/n) } \right) \right) 
%     =: B_{\eta,1}^2
% \end{align}
% since for the chosen $\uls$ the term on the right hand side of inequality is of the order $O (1)$.


% \paragraph{Upper bound on $\nu$.} Now we derive an upper bound for $\nu$. We consider the following set:
% \begin{align}
%     \Gamma_1^{\nu} = \left\{ (\nu, b, \alpha) 
%     \subjto
%     \frac{1}{n} \innerprod{b\gamma(\alpha)}{H}^2 \geq \constnu \nu^2 \andtxts b\alpha \leq \loneboundclas \andtxts b\norm{\gamma(\alpha)}_2 \leq B_{\eta,1} \right\}
%     %\frac{ \innerprod{\wtwo}{H}^2 }{ n } \geq \constnu \norm{\wone}_2^2 \andtxts \norm{ \wtwo }_1 \leq \loneboundclas \andtxts \norm{ \wtwo }_2 \leq \boundeta  \right\}
% \end{align}
% % \begin{align}
% %     \Gamma_1^{\nu} = \left\{ (\wone,\wtwo) 
% %     \subjto
% %     \frac{ \innerprod{\wtwo}{H}^2 }{ n } \geq \constnu \nu^2 \andtxts \norm{ \wtwo }_1 \leq \loneboundclas \andtxts \norm{ \wtwo }_2 \leq \boundeta  \right\}
% % \end{align}
% and note that we have again with high probability that $\Gamma_0 \subset \Gamma_1^{\nu}$. 

% As we noted in Section \ref{step_1_thm3_proof}, from Claim 3 in \cite{wang2021tight} follows that $\innerprod{\gamma(\alpha)}{H} = \norm{H}_{\infty}$ and we obtain that $\Gamma_0 \subset \Gamma_1^{\nu}$ with high probability. Hence we can upper bound $\nu$ as follows:
% \begin{align} \label{eq:nu_opt_first_reduction}
%     \nu^2 \leq \frac{ 1 }{ n \constnu } \max_{b,\alpha} b^2 \innerprod{\frac{\gamma(\alpha)}{\alpha}}{H}^2
%     \subjto 
%     b \leq \loneboundclas 
%     \andtxts 
%     b\norm{ \frac{\gamma(\alpha) }{\alpha} }_2 \leq B_{\eta,1}
% \end{align}

% First note that choosing $b=M$ maximizes the objective if the second constraint is satisfied as well. Now we show how this optimization problem can be rewritten in a more suitable form for solving via parametrized path approach. Similarly as in \cite{wang2021tight} we define function $\olw : \left[ \frac{1}{d}, 1 \right] \to \RR^{d-1}$ as
% \begin{align}
%     \olw(\beta) = \argmax_{\wtwo} \innerprod{\wtwo}{\Hgaussian}
%     \subjto \begin{cases}
%                 \norm{\wtwo}_2^2 \leq \beta \\
%                 \wtwo\geq 0\\
%                 \norm{\wtwo}_1 = 1
%             \end{cases}
% \end{align}
% From Claim 2 in \cite{wang2021tight} we know that for any $\beta \in \left[ \frac{1}{d}, 1 \right] $ there exists $ \alpha \in \left[ 1, \alpham \right] $ such that $ \olw (\beta) = \frac{ \gamma(\alpha) }{ \alpha }$. Following similar argument as in Lemma 4 in \cite{wang2021tight} we have that $ \olw (\beta) $ is monotonically increasing function in $\beta$. Hence we can rewrite \eqref{eq:nu_opt_first_reduction} as:
% \begin{align} 
% \label{eq:first_iteration_nu_gamma_beta}
%     \nu^2 \leq \frac{ \loneboundclas^2 }{ n \constnu } \max_{\beta} \innerprod{ \olw(\beta) }{ H }^2
%     \subjto 
%     \norm{ \olw(\beta) }_2 \leq \frac{ B_{\eta,1} }{ \loneboundclas }
% \end{align}

% Similarly as in the first part of this proof, we first show that there exists $\beta_{\nstar}$ which satisfies constraints, and then find smallest $\beta_{\ols}$ which does not satisfy constraints in \eqref{eq:first_iteration_nu_gamma_beta} and such that $ \beta_{\ols} \geq \beta_{\nstar}$. From monotonicity of $ \olw (\beta)$ follows that $ \olw (\beta_{\ols}) \geq \olw (\beta_{\nstar})$. Since the constraints in \eqref{eq:first_iteration_nu_gamma_beta} are convex in $\olw(\beta)$, the expression is maximized for $\beta = \beta_{\ols}$.

% Since $\alpha = \alpha_{\nstar}$ satisfies constraints in \eqref{eq:nu_opt_first_reduction} by definition of $M$, we define $\beta_{\nstar}$ such that $\gamma(\beta_{\nstar}) = \frac{\gamma(\alpha_{\nstar})}{\alpha_{\nstar}}$ and hence $\beta_{\nstar}$ satisfies constraints in \eqref{eq:first_iteration_nu_gamma_beta}. Furthermore, if we find $\alpha_{\uls}$ such that $\alpha_{\uls} \leq \alpha_{\nstar}$ and
% \begin{align}\label{s_condition_nu_first_reduction}
%     \frac{ \norm{ \gamma ( \alphauls ) }_2 }{ \alphauls } 
%     >
%     \frac{ B_{\eta,1} }{ \loneboundclas }
% \end{align}
% we automatically obtain $\beta_{\uls}$ such that $\gamma(\beta_{\uls}) = \frac{\gamma(\alpha_{\uls})}{\alpha_{\uls}}$ which does not satisfy constraint in \eqref{eq:first_iteration_nu_gamma_beta}. 
% Now from \eqref{s_condition_nu_first_reduction} and using concentration result from Proposition \ref{lemma_gamma_conc} and expression \eqref{phidn_bound} we obtain condition:
% \begin{align}
%     \frac{2}{\uls} \left( 1 - O \left( \frac{1}{\tuls^2} \right) \right)
%     >
%     \frac{B_{\eta,1}^2 \tnstar^2}{ n \fstar } \left( 1 + O \left( \frac{1}{\tnstar^2} \right) \right)
% \end{align}
% Once again we claim that this equality is satisfied for $ \uls = \lambda_{\uls} \frac{ n }{ \log (d/n) } $ for some positive constant $\lambda_{\uls}$. The proof follows use the same reasoning as in the previous part of the proof.

% Hence we can bound $\nu$ from expression \eqref{eq:nu_opt_first_reduction} as follows:
% \begin{align}\label{nu_bound_first_reduction}
%     \nu^2 
%     \leq
%     \frac{ \loneboundclas^2 }{ n \constnu } \frac{ \innerprod{ \gamma (\alphauls) }{ H }^2 }{ \alphauls^2 }
%     =
%     \frac{ \loneboundclas^2 }{ n \constnu } \frac{ \norm{H}_{\infty}^2 }{ \alphauls^2 }
% \end{align}
% with the equality holding for $\gamma(\alpha)$ as discussed in Section \ref{step_1_thm3_proof}. Using concentration results from Proposition \ref{lemma_gamma_conc} we conclude that there exists a positive constant $B_{\nu,1}$ such that:
% \begin{align}
%     \nu^2 \leq \frac{ \fstar \tuls^2 }{ \constnu \tnstar^2 } \left( 1 + O \left( \frac{1}{\tuls^2} \right) \right)
%     % \leq c'_{\nu} \left( 1 + O \left( \frac{ \log \log (d/n) }{\log (d/n) } \right) \right) \leq
%     =: B_{\nu,1}^2
% \end{align}
% since the term on the right hand side is of the order $O(1)$ for chosen $\uls$. This concludes the proof of the lemma.













































\subsubsection{Bound 2: \texorpdfstring{$\nu^2,\eta^2 = O\left(\frac{1}{\log(d/n)}\right)$}{} =}

Conditioning on the event where the bounds form the first step hold for $\nu,\eta$, the goal of this second step is to show that for any element $(\nu, b, \alpha)$ of $\Gamma_0$ we have that $\deltanu^2 = O \left( \frac{1}{ \log \left( d/n \right) }  \right) $ and $ \eta^2 = b^2 \norm{\gamma(\alpha)}_2^2 = O \left( \frac{1}{ \log \left( d/n \right) } \right)$ with high probability over the draws of $\Hgaussian, \Ggaussian, \Xs$ and $\xi$. 

% Define $\deltanu = \nu - \nubar$. Using the fact from the previous section that $\nu \leq B_{\nu,1}, \eta \leq B_{\eta,1}$, we obtain a tighter uniform lower bound for $\fnclas$ from Lemma~\ref{lemma_quadratic_4lus_fstar_bound}. 

% Plugging in this expression, we can again show:
% \begin{lemma} \label{lemma_second_reduction}
%     For any element $(\nu, b, \alpha)$ of $\Gamma_0$ we have that $\deltanu^2 = O \left( \frac{1}{ \log \left( d/n \right) }  \right) $ and $ \eta^2 = b^2 \norm{\gamma(\alpha)}_2^2 = O \left( \frac{1}{ \log \left( d/n \right) } \right)$ with probability at least $ 1 - $ over the draws of $H$ and the data set.
% \end{lemma}

Define $\deltanu = \nu - \nubar$. 
From the previous step, we know that with high probability, $ \nu \leq B_{\nu,1} $ and $ \eta \leq B_{\eta,1} $. Hence we can use Lemma~\ref{lemma_quadratic_plus_fstar_bound} to obtain a tight lower bound for $\fnclas$, which is based on uniform convergence of $\fnclas$ to its expectation in Proposition \ref{prop:unifConv}, and relax the constraint from definition of the set $\Gamma_0$ as follows:
\begin{align}
\label{eq:second_iteration_relaxed_constraint_f}
    \frac{1}{n} b^2 \norm{H}_{\infty}^2 \geq \fnclas (\nu, b\norm{\gamma(\alpha)}_2) \geq f ( \nu, b\norm{\gamma(\alpha)}_2 ) - \constconc \geq  \fstar  + \tconstnu \deltanu^2 + \tconsteta b^2\norm{\gamma(\alpha)}_2^2 - \constconc, 
\end{align}
where we choose $\constconc =  O \left( \frac{1}{\tnstar^3} \right)$. 
Again we first consider the bounding of $\eta$ and then use the obtained result to bound $\deltanu = \nu -\nubar$.

\paragraph{Upper bound on $\eta$.} 
We similarily to the previous step, we consider the set:
\begin{align}
    \Gamma_2^{\eta} = \left\{ (\nu, b, \alpha) 
    \subjto 
    \frac{ 1 }{ n } b^2 \norm{H}_{\infty}^2 \geq \fstar +  \tconsteta b^2 \norm{\gamma(\alpha)}_2^2 - \constconc
    \andtxts
    b\alpha \leq \loneboundclas
    \right\} 
\end{align}
% \begin{align}
%     \Gamma_2^{\eta} = \left\{ (\wone,\wtwo) \subjto \frac{ \innerprod{\wtwo}{H}^2 }{ n } \geq \fstar - \constconc +  \tconsteta \norm{\wtwo}_2^2  \andtxts \norm{ \wtwo }_1 \leq \loneboundclas  \right\}
% \end{align}
% \begin{align}
%     \Gamma_2^{\eta} = \left\{ (\wone,\wtwo) \subjto \frac{ \innerprod{\wtwo}{H}^2 }{ n } \geq \fstar - \constconc +  \tconsteta \eta^2  \andtxts \norm{ \wtwo }_1 \leq \loneboundclas  \right\}
% \end{align}
Again, we have that with high probability $\Gamma_0 \subset \Gamma_2^{\eta} $.
Clearly, to upper bound $\eta = b \norm{\gamma(\alpha)}_2$, we can again set $ b = \frac{\loneboundclas}{\alpha} $ and thus obtain:
\begin{align}
    \eta^2 &\leq \max_{b,\alpha} b^2 \norm{\gamma(\alpha)}_2^2 \subjto \left(\frac{M}{\alpha},\alpha \right) \in \Gamma_2^{\eta}  \\
    &= \max_{\alpha} \frac{M^2}{\alpha^2} \norm{\gamma(\alpha)}_2^2 \subjto \frac{ 1 }{ n } \frac{M^2}{\alpha^2} \norm{H}_{\infty}^2 \geq \fstar +  \tconsteta \frac{M^2}{\alpha^2} \norm{\gamma(\alpha)}_2^2 - \constconc.
    \label{eq:l1proofstep2eta}
\end{align}
Multiplying the constraint on both sides with $\alpha^2$ and using the fact that $\norm{\gamma(\alpha)}_2^2$ is convex shows that the set of feasible $\alpha$ is again a (non-empty) interval. 
Thus, by the monotonicity of $ \frac{\norm{\gamma(\alpha)}_2^2}{\alpha^2} $ the problem reduces again to finding $\alphauls < \alpha_{\nstar}$ (where we use again that $\alpha_{\nstar}$ satisfies the constraints with high probability) such that $\alphauls$ violates the constraint in Equation~\eqref{eq:l1proofstep2eta}, i.e., 
\begin{align}
\label{eq:l1proofstep2eta2}
    \left( \fstar - \constconc \right) \frac{ n \alphauls^2 }{  \loneboundclas^2 \norm{H}_{\infty}^2 } + \tconsteta n \frac{ \norm{ \gamma(\alphauls) }_2^2 }{ \norm{H}_{\infty}^2 } > 1
\end{align}
% In order for inequality above to be satisfied we need:
% \begin{align}
%     \left( 1 - \frac{ \constconc }{ \fstar } \right) 
%     \frac{\tnstar^2}{t_s^2}
%     \left( 1 - \frac{4}{t_s^2} + O \left( \frac{1}{\tnstar^3} \right) \right) 
%     \left( 1 + \frac{2}{\tnstar^2} + O \left( \frac{1}{\tnstar^3} \right) \right) 
%     + \frac{2 n \tconsteta}{s t_s^2} \left( 1 + O \left( \frac{1}{t_s^2} \right) \right) 
%     > 1
% \end{align}
We now show that we can choose $ \uls = \lambda_{\uls} \nstar$ with universal constant $\lambda_{\uls} \in (0,1)$. Indeed, applying  Propositions \ref{prop:concentrationl1} and using the characterization $t_s =   2 \log(d/s) - \log \log (d/s) -\log(\pi) +\frac{\log\log(d/s)}{2\log(d/s)} + O\left(\frac{1}{\log(d/s)}\right)$ from section \ref{step_1_thm3_proof} we get:
\begin{align}
 \left( \fstar - \constconc \right) \frac{ n \alphauls^2 }{  \loneboundclas^2 \norm{H}_{\infty}^2} &= 1 + \frac{\log(\lambda_{\uls})-2}{\tnstar^2} + O\left(\frac{1}{\tnstar^3}\right) \\
 \mathrm{and}~~\tconsteta n \frac{ \norm{ \gamma(\alphauls) }_2^2 }{ \norm{H}_{\infty}^2 } &= 
\frac{1}{\tnstar^2}\frac{4\tconsteta}{\lambda_{\uls}}  +  O \left( \frac{1}{ \tnstar^3} \right)
\end{align}
where $O(.)$ has hidden dependencies on $\lambda_{\uls}$. Hence, it is straight forward to see that for any $d \geq c n$ with universal constant $c>0$ (and thus $\tnstar$ lower bounded), we can find a universal constant $\lambda_{\uls}$ such that Equation~\eqref{eq:l1proofstep2eta2} holds. 


% \begin{align}
%     \frac{\tnstar^2}{t_s^2}
%     \left( 1 + \frac{ \frac{4\tconsteta}{\lambda\feestar}  - 4}{t_s^2} + \frac{2}{\tnstar^2} + O \left( \frac{1}{\tnstar^3}, \frac{1}{t_s^3} \right) \right)
%     > 1
% \end{align}
% Fix $\ulambda > 0$. Choose $\uls = \lambda_{\uls} \nstar$ such that $\uls < n$ is the largest integer for which $ \tuls^2 \geq \tnstar^2 + \ulambda $. Then we have condition:
% \begin{align}
%     \left( 1 - \frac{\ulambda}{\tuls^2} \right) \left( 1 + \frac{ \frac{4\tconsteta}{\lambda_{\uls}\feestar}  - 4}{\tuls^2} + \frac{2}{\tnstar^2} + O \left( \frac{1}{t_n^3} \right) \right)
%     > 1
% \end{align}
% For $\ulambda$ large enough inequality holds (Note: second brackets grow as $\lambda_{\uls}^{-1}$ and the first decays like $\log ( \lambda_{\uls} )$ - TO CHECK).


% \red{okay I messed this up - sorry. Can you make the following section a bit clearer? In particular, the connection to tn and s is not clear, cite the result form our paper. . So here we need to say that essentially we obtain the same problem as studied in my paper.}

% Fix $\olambda > 0$. Now we choose $\ols = c_{\ols} \nstar$ such that $ \ols > n $ is the smallest integer for which $ t_{\ols}^2 \leq \tnstar^2 - \olambda $. Then we have:
% \begin{align}
%     \left( 1 + \frac{\olambda}{\tols^2} \right) \left( 1 + \frac{ \frac{4\tconsteta}{c_{\ols}\feestar}  - 4}{\tols^2} + \frac{2}{\tnstar^2} + O \left( \frac{1}{t_n^3} \right) \right)
%     > 1
% \end{align}
% We claim that there exists $\olambda$ large enough such that this inequality holds (e.g. $\ulambda > 4$).

Hence, we can upper bound $\eta^2$ in Equation \eqref{eq:l1proofstep2eta} as follows:
\begin{align} \label{eq:eta_bound_second_reduction}
    \eta^2 
    \leq
    \loneboundclas^2 \frac{ \norm { \gamma ( \alphauls ) }_2^2 }{ \alpha_{\uls}^2 } 
    \leq
    \frac{ n \fstar }{ \tnstar^2 } \frac{2}{\uls}\left( 1 + O \left( \frac{1}{\tuls^2} \right) \right) 
    \leq
    % \frac{c_{\eta,2}}{\log (d/n) } \left( 1 + O \left( \frac{1}{ \log (d/n) } \right) \right) 
    \frac{2\fstar}{\feestar \lambda_{\uls} \log (d/n) } \left( 1 + O \left( \frac{1}{ \log (d/n) } \right) \right) 
    =:
    \frac{B_{\eta,2}^2}{\tnstar^2}
\end{align}
with $B_{\eta,2}^2 = \Theta(1)$.
% and similarly we get:
% \begin{align}
%     \eta^2 
%     \geq
%     B^2 \frac{ \norm { \gamma ( \alphaols ) }_2^2 }{ \norm { \gamma ( \alphaols ) }_1^2 } 
%     \geq
%     \left( \frac{ \overline{B}_{\eta,2} }{ \sqrt{\log (d/n)} } \right)^2
% \end{align}

















\paragraph{Upper bound on $\deltanu$.}
We now again bound $\nu$ using the previous upper bound on $\eta^2 = O(\log^{-1}(d/n))$. More specifically, we bound $\deltanu$ with $\nu = \nubar +\deltanu$ and thus obtain both an upper and lower bound for $\nu$. 
 First, we again define
\begin{align}
    \Gamma_2^{\nu} = \left\{ (\nu, b, \alpha) 
    \subjto
    \frac{1}{n}b^2\norm{H}_{\infty}^2 \geq \fstar - \constconc + \tconstnu \deltanu^2
    \andtxts
    b\alpha \leq \loneboundclas 
    \andtxts
    b\norm{ \gamma(\alpha) }_2 \leq \frac{B_{\eta,2}}{\tnstar}  \right\}
\end{align}
as in the previous step. 

Clearly, we have again  $\Gamma_0 \subset \Gamma_2^{\nu}$ with high probability. Hence we can upper bound $\deltanu$ by:
\begin{align} %\label{eq:nu_opt_first_reduction}
    \nu^2 &\leq \frac{1}{\tconstnu}\left(\frac{ 1 }{ n } \norm{H}_{\infty}^2 \max_{\alpha}\min\left(\frac{\loneboundclas^2}{\alpha^2}, \frac{B_{\eta,2}^2}{\tnstar^2 \norm{\gamma(\alpha)}_2^2}\right) - \fstar + \constconc \right)
\end{align}
In particular, we obtain again an upper bound for $\deltanu$ (as for $\nu$ in the previous step) when bounding finding $\alpha_{\uls} < \alphaopt < \alpha_{\ols}$ where $\alphaopt \leq \alpha_{d+1/2}$ is the $\alpha$ such that the two terms in the $\min$ match. However, we can verify from a similar argument as for the upper bound for $\eta^2$ in the previous sub-step that we can choose $ \uls = \lambda_{\uls} \nstar$ with universal constant $\lambda_{\uls} \in (0,1)$ and $\ols =\lambda_{\ols} \nstar$ with universal constant $\lambda_{\ols} >1$. Hence, we obtain the upper bound

\begin{align}
    \deltanu^2 
    &\leq
    \frac{\norm{H}_{\infty}^2}{ n \tconstnu }  \frac{ \loneboundclas^2}{\alphauls^2}
    \leq 
    \frac{ \fstar t_{\uls}^2}{\tnstar^2 \tconstnu } \left( 1 + \frac{2}{\tnstar^2}  \right)
    - \frac{\fstar}{\tconstnu} + O \left( \frac{1}{\tnstar^3} \right)\\
    & = \frac{\fstar(2 -2\log(\lambda_{\uls})) }{\tconstnu 2\log(d/n)}\left( 1 + O \left( \frac{1}{\sqrt{\log(d/n)}} \right) \right)
    =: 
    \frac{B_{\deltanu,2}^2}{\tnstar^2} 
\end{align}
which concludes the proof.








\subsubsection{Bound 3: Proof of the proposition. }
We already know that $\nu$ concentrates around $\nubar$. However, in order to get a tight expression for the risk and also a valid lower bound, we need to get tighter bounds for $\eta^2$ conditioning on the bounds on $\eta^2,\deltanu^2$ from the previous step,  leading to Proposition~\ref{prop:BoundOmegal1}.


% In this part of the proof we use Taylor series approximation of function $f$ up to quadratic terms as shown in equation \eqref{eq:f_taylor_approx}. Using similar arguments as in previous two bounding steps, we obtain Proposition \ref{prop:BoundOmegal1}.
% \begin{lemma}
%     There exist universal constant $B_{\nu,3} > 0, B_{\eta,3} > 0$ such that for any element $(\wone,\wtwo)$ of $\Gamma_0$ we have that $\deltanu^2 \leq \frac{B_{\nu,3}^2}{ \left( \log \left( d/n \right) \right)^{3/2} }$ and $ \eta^2 \leq \frac{B_{\eta,3}^2}{ \log \left( d/n \right) }$ with probability at least $ 1 - $ over the draws of $..$.
% \end{lemma}
% \begin{proof}
% Conditioning on the event where the bounds for $\nu,\eta$ from the previous second step hold, we now derive the tight bounds
In this part of the proof we use Taylor series approximation of the function $f$ where we use the result form the last step to bound the  higher order terms involving $\eta$. Similarly as in equation \eqref{eq:second_iteration_relaxed_constraint_f}, we obtain form Proposition~\ref{prop:unifConv} and the second order Taylor series approximation of $f$ around the point $(\nubar, 0)$ that with high probability,
\begin{align}
    \label{eq:f_taylor_approx}
    \frac{1}{n} b^2 \norm{H}_{\infty}^2 
    \geq 
    % f ( \nu, \eta ) =
    \fstar + \frac{1}{2}\feestar b^2 \norm{\gamma(\alpha)}_2^2 + \frac{1}{2}\fnnstar \deltanu^2 - \constconc - \OOOc
    % \underbrace{O \left( \frac{1}{ \log (d/n)^{3/2} } \right)}_{\OOOc}
\end{align}
with $\OOO_f = O(\deltanu^3 + \eta^3) =  O \left( \frac{1}{\tnstar^3} \right)$ and $\OOOc = O \left( \frac{1}{\tnstar^3} \right)$. 
% \end{proof}

\paragraph{Upper and lower bound on $\eta$.}
We proceed in the same manner as in the previous two steps. We relax the constraint in definition of $\Gamma_0$ and define the following set:
\begin{align}
    \Gamma_3^{\eta} = \left\{ (\nu, b, \alpha) 
    \subjto 
    \frac{ 1 }{ n } b^2 \norm{H}_{\infty}^2 \geq \fstar +  \frac{1}{2}\feestar  b^2 \norm{\gamma(\alpha)}_2^2  -\constconc - \OOOc
    \andtxts
    b\alpha \leq \loneboundclas
    \right\}
\end{align}
Clearly, we have again with high probability that $\Gamma_0 \subset \Gamma_3^{\eta}$. The only difference between $\Gamma_3^{\eta}$ and $\Gamma_2^{\eta}$ lies in the constant $\tconsteta$ which is replaced by the tighter constant $\feestar/2$. However, this makes a big difference, as this allows us to choose $\uls < \nstar <\ols$ much tighter. Similar to Equation~\eqref{eq:l1proofstep2eta2} we again require that $s=\uls,\ols$ satisfies
\begin{align}
\label{eq:l1thirdeta}
    \left( \fstar - \constconc - \OOOc \right) \frac{ \alpha_s^2 }{ \norm{H}_{\infty}^2 } \frac{ n }{ \loneboundclas^2 } 
    +
    \frac{1}{2} \feestar n \frac{ \norm{ \gamma (\alpha_s) }_2^2 }{ \norm{H}_{\infty}^2 } 
    > 1.
\end{align}
However, this expression allows us to choose $\uls$ and $\ols$ as in Lemma~\ref{lemma_uls_ols_exp}. We only show it for $\uls$ as the same argument holds for $\ols$. Applying Proposition~\ref{prop:concentrationl1}, the LHS from Equation~\eqref{eq:l1thirdeta} can be bounded by

% \begin{align} (this is the last version of this equation)
%     \left( \fstar -\constconc - \OOOc \right) \frac{ \alphauls^2 }{ \norm{H}_{\infty}^2 } \frac{ n }{ \loneboundclas^2 } 
%     \geq 
%     1 - \frac{2}{\tnstar^2} - \frac{\lambda}{\tnstar^{5/2}} + O \left( \frac{1}{\tnstar^3} \right) + O \left( \frac{1}{\tnstar^5} \right) + O \left( \frac{1}{\tnstar^2 \nstar} \right)
% \end{align}
% 
% \begin{align}
%     \left( \fstar -\constconc - \OOOc \right) \frac{ \alphauls^2 }{ \norm{H}_{\infty}^2 } \frac{ n }{ \loneboundclas^2 } \geq &
%     \fstar \left( 1 + O \left( \frac{1}{\tnstar^3} \right) \right) \frac{1}{\tuls^2}\left( 1 - \frac{4}{\tuls^2} + O \left( \frac{1}{\tuls^4} \right) \right)\frac{n \tnstar^2}{n\fstar} \left( 1 + \frac{2}{\tnstar^2} + O \left( \frac{1}{\tnstar^3} \right) \right)
%     \\
%     \geq &
%     \left( 1 - \frac{\lambda}{\tnstar^2\sqrt{\tnstar}} + O \left( \frac{1}{\tnstar^2 \nstar} \right) + O \left( \frac{\lambda^2}{\tnstar^5} \right) \right) \left( 1 - \frac{2}{\tnstar^2} + O \left( \frac{1}{\tnstar^3} \right) \right)
% \end{align}
% 
% \begin{align} (this is the last version of this equation)
%     \frac{1}{2} \feestar n \frac{ \norm{ \gamma (\alphauls) }_2^2 }{ \norm{H}_{\infty}^2 } 
%     \geq 
%     \frac{2}{\tnstar^2} + \frac{\lambda}{(\tnstar)^{5/2}} + \frac{\lambda^2}{2\tnstar^3} + O \left( \frac{1}{\tnstar^{7/2}} \right) 
% \end{align}
% 
% \begin{align}
%     \frac{1}{2} \feestar n \frac{ \norm{ \gamma (\alphauls) }_2^2 }{ \norm{H}_{\infty}^2 } 
%     \geq &
%     \nstar \frac{2}{\uls \tuls^2} \left( 1 + O \left( \frac{1}{\tuls^2} \right) \right)\\
%     \geq &
%     \frac{2}{\tnstar^2} \exp \left( \frac{\lambda}{2\sqrt{\tnstar}} \right)  \left( 1 + O \left( \frac{1}{\tnstar^2} \right) \right) \\
%     \geq &
%     \frac{2}{\tnstar^2} \left( 1 + \frac{\lambda}{2\sqrt{\tnstar}} + \frac{\lambda^2}{4\tnstar} + O \left( \frac{\lambda^3}{\tnstar\sqrt{\tnstar}} \right) \right) \left( 1 + O \left( \frac{1}{\tnstar^2} \right) \right) 
% \end{align}
% 
% Hence we have:
\begin{align}
    \left( \fstar - \constconc - \OOOc \right) \frac{ \alphauls^2 }{ \norm{H}_{\infty}^2 } \frac{ n }{ \loneboundclas^2 } 
    &= \frac{\tnstar^2}{t_{\uls}^2}\left(1 -\frac{4}{t_{\uls}^2}+\frac{2}{\tnstar^2} + O\left(\frac{1}{\tnstar^3}\right)\right)  = 1- \frac{\lambda}{\tnstar^{5/2}} -\frac{2}{\tnstar^2} + O\left(\frac{1}{\tnstar^3}\right) + O\left(\frac{1}{\tnstar^2 \nstar}\right)
    \\
    ~~\mathrm{and}\:\: \frac{1}{2} \feestar n \frac{ \norm{ \gamma (\alphauls) }_2^2 }{ \norm{H}_{\infty}^2 } &= 
    \frac{2}{\tnstar^2} + \frac{\lambda}{\tnstar^{5/2}} + \frac{\lambda^2}{2\tnstar^3} + O \left( \frac{1}{\tnstar^3} \right) + O \left( \frac{1}{\tnstar^2 \nstar} \right)
\end{align}
with $O(.)$ having hidden dependencies on $\lambda$. In particular, as a result, we see that we can choose $\lambda$ such that Equation~\eqref{eq:l1thirdeta} hold for any $d >c n$ with universal constant $c>0$. 
Hence we can bound $\eta^2$ as follows:
\begin{align} \label{eq:eta_bound_third_reduction}
    \eta^2 
    \leq
    \loneboundclas^2 \frac{ \norm { \gamma ( \alphauls ) }_2^2 }{ \norm { \gamma ( \alphauls ) }_1^2 } 
    & \leq
    \frac{ n \fstar }{ \tnstar^2 } \frac{2}{\uls}\left( 1 + O\left( \frac{1}{\tnstar^2} \right) \right)
    \leq
    % \frac{4\fstar}{\feestar} \frac{1}{\tnstar^2}  \exp \left( \frac{\lambda}{2\sqrt{\tnstar}} \right) \left( 1 + O\left( \frac{1}{\tnstar^2} \right) \right) \\
    % & \leq
    \frac{4\fstar}{\feestar} \frac{1}{\tnstar^2} \left( 1 + \frac{\lambda}{2\sqrt{\tnstar}} + O \left( \frac{1}{\tnstar} \right) \right) =: B_{\eta,3}^2
\end{align}
Furthermore, we also obtain a lower bound for $\eta^2$. Similar as in Lemma~5/6 \cite{wang2021tight}, we can lower bound (using again the monotonicity of $\frac{\norm{\gamma(\alpha)}_2}{\alpha}$ and the fact that any feasible $\alpha \leq \alphaols$)
\begin{align}
    \eta^2 &\geq \left[\min_b b^2 \norm{\gamma(\alpha_{\ols})}_2^2 \subjto b^2   
    \geq \frac{\fstar   -\constconc - \OOOc}{\frac{  \norm{H}_{\infty}^2}{ n } -\frac{1}{2}\feestar  \norm{\gamma(\alpha_{\ols})}_2^2} \right] =\frac{\fstar  -\constconc - \OOOc}{\frac{  \norm{H}_{\infty}^2}{ n } -\frac{1}{2}\feestar  \norm{\gamma(\alpha_{\ols})}_2^2} \norm{\gamma(\alpha_{\ols})}_2^2 \\
    &\geq  \frac{4\fstar}{\feestar} \frac{1}{\tnstar^2} \left( 1 - \frac{\lambda}{2\sqrt{\tnstar}} + O \left( \frac{1}{\tnstar} \right) \right) 
\end{align}
Hence we can conclude the proof. 



% \paragraph{Upper bound on $\deltanu$.}
% Now let
% % \begin{align}
% %     \Gamma_3^{\nu} = \left\{ (\nu, b, \alpha) 
% %     \subjto
% %     \frac{1}{n}\innerprod{b\gamma(\alpha)}{H}^2 \geq \fstar + \frac{1}{2}\feestar \eta^2 + \frac{1}{2}\fnstar \deltanu^2 - O \left( \frac{1}{\tnstar^3} \right)
% %     \andtxts 
% %     b\alpha \leq \loneboundclas 
% %     \andtxts
% %     b\norm{ \gamma(\alpha) }_2 \leq \frac{B_{\eta,3}}{\log (d/n) }  \right\}
% % \end{align}
% \begin{equation}
%     \Gamma_3^{\nu} = \Bigg\{ (\nu, b, \alpha) 
%     \subjto \begin{cases}
%                 \frac{1}{n}\innerprod{b\gamma(\alpha)}{H}^2 \geq \fstar - \constconc - \OOOc + \frac{1}{2}\feestar b\norm{\gamma(\alpha)}_2^2 + \frac{1}{2}\fnstar \deltanu^2
%                 \\
%                 b\alpha \leq \loneboundclas
%                 \\
%                 b\norm{ \gamma(\alpha) }_2 \leq B_{\eta,3}
%             \end{cases}
%              \Bigg\}
% \end{equation}
% % \begin{align}
% %     \Gamma_3^{\nu} = \left\{ (\wone,\wtwo) 
% %     \subjto
% %     \frac{ \innerprod{\wtwo}{H}^2 }{ n } \geq \fstar - \constconc - \OOOc + \frac{1}{2}\feestar \eta^2 + \frac{1}{2}\fnstar \deltanu^2
% %     \andtxts 
% %     \norm{ \wtwo }_1 \leq \loneboundclas 
% %     \andtxts
% %     \norm{ \wtwo }_2 \leq B_{\eta,3}  \right\}
% % \end{align}

% % \begin{align}
% % \label{s_condition_nu_third_reduction}
% %     \frac{ \norm{ \gamma ( \alphauls ) }_2 }{ \alphauls } > \frac{B_{\eta,3}}{\loneboundclas}
% % \end{align}
% Analogously to equation \eqref{s_condition_nu_first_reduction} we derive new condition for $\uls$ with new bound $B_{\eta,3}$. Using concentration result from Proposition \ref{lemma_gamma_conc} and expression \eqref{phidn_bound} we get the condition:
% % \begin{align}
% %     \frac{2}{\uls} \left( 1 + O\left( \frac{1}{\tuls^2} \right) \right) 
% %     >
% %     \frac{4\fstar}{\feestar} \frac{1}{\tnstar^2} \left( 1 + \frac{\lambda}{2\sqrt{\tnstar}} + O \left( \frac{1}{\tnstar} \right) \right) \frac{\tnstar^2}{ n \fstar } \left( 1 + \frac{2}{\tnstar^2} + O \left( \frac{1}{\tnstar^3} \right) \right)
% % \end{align}
% % then
% \begin{align}
%     \frac{2}{\uls} \left( 1 + O \left( \frac{1}{\tuls^2} \right) \right) > \frac{4}{\feestar} \frac{1}{n} \left( 1 + \frac{\lambda}{2\sqrt{\tnstar}} + O \left( \frac{1}{\tnstar} \right) \right)
% \end{align}
% Hence let $\uls = \nstar \exp \left( -\frac{\lambda}{2\sqrt{\tnstar}} \right)$. %\frac{n\feestar}{2} \left( 1 - \frac{\lambda}{\sqrt{\tnstar}} + O \left( \frac{1}{\tnstar} \right) \right)$.  
% \begin{align}
%     \deltanu^2 
%     \leq
%     \frac{ 2\loneboundclas^2 }{ n \fnstar } \frac{ \norm{H}_{\infty}^2 }{ \alphauls^2 } - \frac{2}{\fnstar} \left( \fstar - \constconc - \OOOc \right) - \frac{\feestar}{\fnstar} \frac{ \norm{ \gamma(\alphaols) }_2^2 }{ \alphaols^2 } \loneboundclas^2
%     \leq
%     \frac{4 \fstar \lambda}{\fnstar \tnstar^{5/2}} \left( 1 + O \left( \frac{1}{\sqrt{\tnstar}} \right) \right) =: B_{\deltanu,3}^2
% \end{align}
% \begin{align}
%     \deltanu^2 
%     &\leq
%     \frac{ 2\loneboundclas^2 }{ n \fnstar } \frac{ \norm{H}_{\infty}^2 }{ \alphauls^2 } - \frac{2\fstar}{\fnstar} \left( 1 - \constconc - \OOOc \right) - \frac{\feestar}{\fnstar} \frac{ \norm{ \gamma(\alphaols) }_2^2 }{ \alphaols^2 } \loneboundclas^2\\
%     &\leq 
%     \frac{2}{n\fnstar} \frac{n\fstar}{\tnstar^2} \left(1-\frac{2}{\tnstar^2}+O \left( \frac{1}{\tnstar^3} \right) \right) \tuls^2 \left( 1 + \frac{4}{\tuls^2} + O \left( \frac{1}{\tuls^4} \right) \right)
%     - \frac{2\fstar}{\fnstar} \left( 1 + O \left( \frac{1}{\tnstar^3} \right) \right)
%     \\
%      & - \frac{\feestar}{\fnstar} \frac{2}{\nstar} \exp \left( -\frac{\lambda}{2\sqrt{\tnstar}} \right) \left( 1 + O \left( \frac{1}{\tnstar^2} \right) \right) \frac{n\fstar}{\tnstar^2}  \left( 1 - \frac{2}{\tnstar^2} + O \left( \frac{1}{\tnstar^3} \right) \right)
%      \\
%      &\leq \frac{2\fstar}{\fnstar} \left( 1 + \frac{2}{\tnstar^2} + \frac{\lambda}{\tnstar^{5/2}} + O \left( \frac{1}{\tnstar^3} \right) \right) 
%      - \frac{2\fstar}{\fnstar} \left( 1 + O \left( \frac{1}{\tnstar^3} \right) \right)
%      -\frac{2\fstar}{\fnstar}\left( \frac{2}{\tnstar^2} - \frac{\lambda}{\tnstar^{5/2}} + O \left( \frac{1}{\tnstar^3} \right) \right)
%      \\
%      & \leq \frac{4 \fstar \lambda}{\fnstar}\frac{1}{\tnstar^{5/2}} \left( 1 + O \left( \frac{1}{\sqrt{\tnstar}} \right) \right) =: B_{\deltanu,3}^2
% \end{align}





% \begin{align}
%     f ( \nu, \eta ) = \fstar + \frac{1}{2}\feestar \eta^2 + \frac{1}{2}\fnstar \deltanu^2 + O \left( \frac{1}{ \log (d/n)^{3/2} } \right)
% \end{align}


% \begin{lemma}
%     There exist universal constant $B_{\nu,3} > 0, B_{\eta,3} > 0$ such that for any element $(\wone,\wtwo)$ of $\Gamma_0$ we have that $\deltanu^2 \leq \frac{B_{\nu,3}^2}{ \left( \log \left( d/n \right) \right)^{3/2} }$ and $ \eta^2 \leq \frac{B_{\eta,3}^2}{ \log \left( d/n \right) }$ with probability at least $ 1 - $ over the draws of $..$.
% \end{lemma}







% \subsection{Proof of Proposition~\ref{prop:Rbound}}


% Recall that $\phidn$ is given by:
% \begin{align}
%     \phidn &= \min_{\nu,b,\alpha} \nu + b \norm{ \gamma \left( \alpha \right) }_1 
%     \subjto \frac{ b^2\norm{\Hgaussian}_{\infty}^2 }{n} \geq \fnclas \left( \nu, b \norm{ \gamma \left( \alpha \right) }_2 \right)
% \end{align}

% Given that $(\tnu,\tb,\talpha)$ is a feasible point of $\phidn$ we have that $\phidn \leq  \tnu + \tb \norm{ \gamma( \talpha) }_1$, which gives us an upper bound on $\phidn$. In the following discussion our goal is to find a single feasible point of the constraint set of $\phidn$.

% From definition of $\gamma ( \alpha )$ we know that $ \norm{ \gamma ( \alpha ) }_1 = \alpha$ and hence we can equivalently formulate $\phidn$ as an optimization over $\nu$ and $ b_{\alpha} := b \alpha $
% \begin{align}
%     \phidn &= \min_{ \nu, b_{\alpha} } \nu + b_{\alpha}
%     \subjto \frac{ b_{\alpha}^2 \norm{\Hgaussian}_{\infty}^2 }{n \alpha^2} \geq \fnclas \left( \nu, b_{\alpha} \frac{ \norm{ \gamma \left( \alpha \right) }_2}{ \alpha } \right)
% \end{align}

% Define $\fstar = f \left( \nubar, 0 \right)$, $\feestar = \frac{\partial^2 f(\nuopt,\eta)}{\partial \eta^2}\Big|_{\eta=0}$ and $\nstar = \frac{1}{2}\feestar n$. Now using lemma \ref{lemma_point_conv} with $ t = \fstar \tnstar^{-3} $ and for a feasible point $( \nu, b_{\alpha} \frac{ \norm{ \gamma \left( \alpha \right) }_2}{ \alpha } )$ we have that:
% \begin{align} \label{eq:constraint_f_conc}
%     \frac{ b_{\alpha}^2 \norm{\Hgaussian}_{\infty}^2 }{n \alpha^2} 
%     \geq
%     f \left( \nu, b_{\alpha} \frac{ \norm{ \gamma \left( \alpha \right) }_2}{ \alpha } \right) + \frac{\fstar}{\tnstar^{3}}
% \end{align}
% with probability at least $ 1 - 2 \exp \left( -c \frac{ n }{ \tnstar^6 \left( \nu^2 + b_{\alpha}^2  \norm{ \gamma \left( \alpha \right) }_2^2 / \alpha^2 \right) } \right) $.
% % > 1 - 2 \exp \left( - \tc \frac{ n }{ \log^3 \left( \frac{d}{n} \right)  } \right) $.

% Let's now choose $ \nu = \nubar $ and show that there exists a pair $ ( b, \alpha )$  such that $ ( \nubar, b, \alpha) $ is feasible for constraint \eqref{eq:constraint_f_conc}. Furthermore, we propose to search for a point with parameter $ ( b, \alpha ) $ such that $ b \norm{ \gamma ( \alpha )}_2 = b_{\alpha} \frac{ \norm{ \gamma \left( \alpha \right) }_2}{ \alpha } $ is near zero. Hence, using Taylor series approximation of function $ f ( \nubar, \cdot ) : \eta \mapsto f (\nubar, \eta) $ around point $(\nuopt,0)$ we can rewrite constraint \eqref{eq:constraint_f_conc} as:
% \begin{align}
%      \frac{ b_{\alpha}^2 \norm{\Hgaussian}_{\infty}^2 }{n \alpha^2}   
%      \geq
%       \fstar + \frac{1}{2}\feestar b_{\alpha}^2 \frac{ \norm{ \gamma \left( \alpha \right) }_2^2}{ \alpha^2 } + O \left( b_{\alpha}^3 \frac{ \norm{ \gamma \left( \alpha \right) }_2^3}{ \alpha^3 } \right) + \frac{\fstar}{\tnstar^{3}}
% \end{align}
% since $\feta = \frac{\partial f(\nuopt,\eta)}{\partial \eta}\Big|_{\eta=0} = 0$.

% Now from \cite{wang2021tight} we know that $ \gamma ( \alpha ) $ is a piecewise linear function with breakpoints at $ \alpha_s $ for $ s = 2, \dots, d $. Hence instead of optimizing over $\alpha$ we optimize over $s$. Note that we have only one constraint but two free variables $ ( b, \alpha ) $ and so we can set $ \alpha = \alpha_{\nstar} $ with $ \nstar = \frac{1}{2}\feestar n $. We explain this choice of $s$ in the remark after the proof. Combining all these results we get constraint:
% \begin{align} \label{eq:B_ineq}
%      \frac{ b_{\alpha_{\nstar}}^2 \norm{\Hgaussian}_{\infty}^2 }{n \alpha_{\nstar}^2}   
%      \geq
%       \fstar + \frac{1}{2}\feestar b_{\alpha_{\nstar}}^2 \frac{ \norm{ \gamma \left( \alpha_{\nstar} \right) }_2^2}{ \alpha_{\nstar}^2 } + O \left( b_{\alpha_{\nstar}}^3 \frac{ \norm{ \gamma \left( \alpha_{\nstar} \right) }_2^3}{ \alpha_{\nstar}^3 } \right) + \frac{\fstar}{\tnstar^{3}}
% \end{align}

% Now we claim that
% \begin{equation}
%     b_{\alpha_{\nstar}}^2 = \frac{ n \alpha_{\nstar}^2 }{ \norm{\Hgaussian}_2^2 } \frac{ \fstar \left( 1 + \frac{1}{\tnstar^{3}} \right) }{ 1 - \frac{1}{2} n \feestar \frac{ \norm{ \gamma \left( \alpha_{\nstar} \right) }_2^2 }{ \norm{H}_{\infty}^2 } - O \left( \frac{1}{\tnstar^3} \right) }
% \end{equation}
% satisfies inequality \eqref{eq:B_ineq} with probability at least $ 1 - 6 \exp \left( -\frac{\nstar}{\log^5(d/\nstar)} \right)$. Using lemma \ref{lemma_gamma_conc} we have that:
% \begin{equation}
%     1 - \frac{1}{2} n \feestar \frac{ \norm{ \gamma \left( \alpha_{\nstar} \right) }_2^2 }{ \norm{H}_{\infty}^2 } - O \left( \frac{1}{\tnstar^3} \right) > 1 - \frac{1}{2} n \feestar  \frac{2}{\nstar \tnstar^2} - O \left( \frac{1}{\tnstar^3} \right) = 1 - \frac{2}{\tnstar^2} - O \left( \frac{1}{\tnstar^3} \right)  > 0
% \end{equation}
% holding for $d,n$ sufficiently large. Applying lemma \ref{lemma_gamma_conc} once again we get:
% \begin{equation}
%     b_{\alpha_{\nstar}}^2 
%     \leq
%     \frac{ n \fstar }{ \tnstar^2 } \left( 1 + \frac{1}{\tnstar^3} \right) \left( 1 - \frac{4}{\tnstar^2} + \frac{c}{\tnstar^4} \right) \frac{1}{ 1 - \frac{2}{\tnstar^2} - O \left( \frac{1}{\tnstar^3} \right)}
%     \leq
%     \frac{ n \fstar }{ \tnstar^2 } \left( 1 - \frac{2}{\tnstar^2} + \frac{c}{\tnstar^3} \right)
% \end{equation}

% Hence we have that $ O \left( b_{\alpha_{\nstar}}^3 \frac{ \norm{ \gamma \left( \alpha_{\nstar} \right) }_2^3}{ \alpha_{\nstar}^3 } \right) = O \left( \frac{1}{\tnstar^3} \right)$ and this $b_{\alpha_{\nstar}}^2$ indeed satisfies equation \ref{eq:B_ineq}. Now we define the upper bound on $\phidn$ as:
% \begin{align}
%     \loneboundclas := \sqrt{ \frac{ n \fstar }{ \tnstar^2 } \left( 1 - \frac{2}{\tnstar^2} + \frac{c}{\tnstar^3} \right) }
% \end{align}
% which holds with probability at least $ 1 - 2 \exp \left( -c \frac{ n }{ \tnstar^6 \left( (\nubar)^2 + b_{\alpha_{\nstar}}^2  \norm{ \gamma \left( \alpha_{\nstar} \right) }_2^2 / \alpha_{\nstar}^2 \right) } \right) - 6 \exp \left( -\frac{\nstar}{\log^5(d/\nstar)} \right) $. The proposition is proved after noting that $ (\nubar)^2 + b_{\alpha_{\nstar}}^2  \norm{ \gamma \left( \alpha_{\nstar} \right) }_2^2 / \alpha_{\nstar}^2 = O(1)$.

% \subsection{Proof of Lemma~\ref{lemma_first_reduction}}
% According to lemma \ref{quadratic_bound_fn} we have that for any pair $ ( \nu, \eta ) $ with probability at least $ 1 - \exp \left( - n \kldiv{\frac{\sigma}{2}}{\frac{\sigma}{4}} \right) - \exp \left( -\frac{ n\sigma }{ 128 } \right) $ that $ \fnclas ( \nu, \eta) \geq \constnu \nu^2 + \consteta \eta^2 $ for some positive constants $\constnu$ and $\consteta $. Hence with high probability we can relax first constraint defining $\Gamma_0$ to
% \begin{align}
%     \frac{ \innerprod{\wtwo}{H}^2 }{ n } \geq \constnu \nu^2 + \consteta  \eta^2
% \end{align}

% \paragraph{Bounding $\eta$.}
% We can furthermore relax both constraints to define the following set:
% \begin{align}
%     \Gamma_1^{\eta} = \left\{ (\wone,\wtwo) \subjto \frac{ \innerprod{\wtwo}{H}^2 }{ n } \geq \consteta  \eta^2 \andtxts \norm{ \wtwo }_1 \leq \loneboundclas  \right\}
% \end{align}
% It is evident from definition that $ \Gamma_0 \subset \Gamma_1^{\eta}$ with high probability. Also note that constraints in the set $\Gamma_1^{\eta}$ depend only on $\wtwo$ and hence we will now consider only this variable. Now we bound $ \eta = \norm{ \wtwo }_2 $ as:
% \begin{align}
%     \eta^2 \leq \max_{\wtwo} \norm { \wtwo }_2 \subjto \wtwo \in \Gamma_1^{\eta}
% \end{align}

% We proceed following the path arguments established in \cite{wang2021tight}. We parametrize variable $\wtwo$ as $ \wtwo = b \norm { \gamma ( \alpha ) } $. 

% First we show that set $\Gamma_1^{\eta}$ is not empty. Let's choose $ \alpha = \alpha_{\nstar}$ with $\nstar = n\feestar/2$. Since we defined $ \loneboundclas $ in such way that $ \alpha_{\nstar} \in \Gamma_0 $ with high probability and we have $ \Gamma_0 \subset \Gamma_1^{\eta}$, this implies that with high probability there exists some $ b > 0 $ such that $ b \gamma ( \alpha ) \in \Gamma_1^{\eta} $.

% Using the same argument as in lemma 1 in \cite{wang2021tight} for $\phidp$ we can write:
% \begin{align}
%     \eta^2 \leq \max_{1\leq \alpha \leq \alpham} B^2 \frac{ \norm { \gamma ( \alpha ) }_2^2 }{ \norm { \gamma ( \alpha ) }_1^2 } \subjto B\gamma \left( \alpha \right) \in \Gamma_1^{\eta}
% \end{align}

% Now from lemma 4 in \cite{wang2021tight} we have that map $ \alpha \mapsto \frac{ \norm{ \gamma ( \alpha ) }_2^2 }{ \norm{ \gamma ( \alpha ) }_1^2 } $ is monotonically decreasing. 
% \red{Say that it is a interval - this follows from the convexity.}



% Hence if we find value of $\alpha_{\uls}$ such that $\alpha_{\uls} \leq \alpha_{\nstar}$ and $ b \gamma ( \alpha_{\uls} ) \not \in \Gamma_1^{\eta}$ for any $ b > 0 $ then we have:
% \begin{align} \label{eq:eta_bound_first_reduction}
%     \eta^2 \leq  B^2 \frac{ \norm { \gamma ( \alphauls ) }_2^2 }{ \norm { \gamma ( \alphauls ) }_1^2 }
% \end{align}

% In order to saturate constraint $ \norm{ \wtwo }_1 \leq B $ let $ b = \frac{B}{\alphauls}$. Since we want that $  b \gamma ( \alpha_{\uls} ) \not \in \Gamma_1^{\eta} $ we will chose $s$ such that:
% \begin{align}
%     B^2 \frac{ \innerprod{ \gamma ( \alphauls )}{H}^2 }{ n \alphauls^2 } < \consteta B^2 \frac{ \norm{ \gamma ( \alphauls ) }_2^2 }{ \alphauls^2 }
% \end{align}
% Rewriting this inequality gives:
% \begin{align} \label{eq:s_condition_one}
%   \frac{ \norm{ \gamma ( \alphauls ) }_2^2 }{ \norm{H}_{\infty}^2 } > \frac{ 1 }{ \consteta n } 
% \end{align}
% Now we use concentration result from lemma \ref{lemma_gamma_conc} to get the following condition on $s$:
% \begin{align}
%     \frac{ 2 }{ \uls t_s^2 } \left( 1 - \frac{ c }{ \tuls^2 } \right) > \frac{ 1 }{ \consteta n }
% \end{align}

%  We claim that $\uls =\lambda_{\uls} \frac{ n }{ \log (d/n) }$ satisfies this inequality for some positive universal constant $ \lambda_{\uls} >0  $. From lemma 3 in \cite{wang2021tight} we know that if $ d/\uls \geq 11 $ we have that $ \log (d/\uls) \leq \tuls^2 \leq 2 \log (d/\uls) $. Using both of these bounds into expression \eqref{eq:s_condition_one} gives that:
% \begin{align}
%     \frac{ 2 }{ \uls \tuls^2 } \left( 1 - \frac{ c }{ \tuls^2 } \right) &> \frac{ 1 }{ 2 n \lambda_{\uls} } \frac{ \log (d/n) }{ \log (d/n) + \log \log (d/n) - \log \lambda_{\uls} } \left( 1 - \frac{c}{ \log (d/n) + \log \log (d/n) - \log \lambda_{\uls} } \right)
%     \\
%     & = \frac{ 1 }{ 2 n \lambda_{\uls} } \left( 1 - O \left( \frac{\log (d/n) }{\log \log (d/n) } \right) \right) > \frac{1}{\consteta n}
% \end{align}
% where last inequality holds for $d/n$ sufficiently large.

% Now from equation \eqref{eq:eta_bound_first_reduction} and concentration lemma \ref{lemma_gamma_conc} we have:
% \begin{align}
%     \eta^2 \leq \frac{ n \fstar }{ \tnstar^2 } \frac{2}{\uls}\left( 1 + \frac{c}{\tuls^2} \right) \leq \boundeta' \left( 1 + O \left( \frac{1}{ \log (d/n) } \right) \right) \leq \boundeta^2
% \end{align}

% \paragraph{Upper bound on $\nu$.} Now we derive an upper bound for $\nu$. We consider the following set:
% \begin{align}
%     \Gamma_1^{\nu} = \left\{ (\wone,\wtwo) 
%     \subjto
%     \frac{ \innerprod{\wtwo}{H}^2 }{ n } \geq \constnu \nu^2 \andtxts \norm{ \wtwo }_1 \leq \loneboundclas \andtxts \norm{ \wtwo }_2 \leq \boundeta  \right\}
% \end{align}
% Once again it follows that $\Gamma_0 \subset \Gamma_1^{\nu}$. Hence we can upper bound $\nu$ as follows:
% \begin{align} \label{eq:nu_opt_first_reduction}
%     \nu^2 \leq \frac{ 1 }{ n \constnu } \max_{\wtwo} \innerprod{\wtwo}{H}^2
%     \subjto 
%     \norm{ \wtwo }_1 \leq \loneboundclas 
%     \andtxts 
%     \norm{ \wtwo }_2 \leq \boundeta
% \end{align}

% Now we show can this optimization problem can be rewritten in a form suitable for using parametrized path approach. Similarly as in \cite{wang2021tight} we define function $\olw : \left[ \frac{1}{d}, 1 \right] \to \RR^{d-1}$ as
% \begin{align}
%     \olw(\beta) = \argmax_{\wtwo} \innerprod{\wtwo}{\Hgaussian}
%     \subjto \begin{cases}
%                 \norm{\wtwo}_2^2 \leq \beta \\
%                 \wtwo\geq 0\\
%                 \norm{\wtwo}_1 = 1
%             \end{cases}
% \end{align}
% From claim 2 in \cite{wang2021tight} we know that for any $\beta \in \left[ \frac{1}{d}, 1 \right] $ there exists $ \alpha \in \left[ 1, \alpham \right] $ such that $ \olw (\beta) = \frac{ \gamma(\alpha) }{ \alpha }$. Following similar argument as in fourth statement of lemma 4 in \cite{wang2021tight} we have that $ \olw (\beta) $ is monotonically increasing function in $\beta$. 

% Setting $ \tildewtwo = \frac{ \wtwo }{ B }$ we can rewrite \eqref{eq:nu_opt_first_reduction} as:
% \begin{align} 
%     \nu^2 \leq \frac{ B^2 }{ n \constnu } \max_{\tildewtwo} \innerprod{ \tildewtwo }{ H }^2
%     \subjto 
%     \norm{ \tildewtwo }_1 \leq 1 
%     \andtxts 
%     \norm{ \tildewtwo }_2 \leq \frac{ \boundeta }{ B }
% \end{align}
% Hence solution of this problem must be of the form $ \tildewtwo = \olw (\beta) $ for some $\beta$. 
% Similarly as in the first part of this proof, we first show that there exists $\beta_{\nstar}$ which satisfies constraints, and then find $\beta_{\ols}$ such that $ \beta_{\ols} \geq \beta_{\nstar}$. From monotonicity of $ \olw (\beta)$ follows that $ \olw (\beta_{\ols}) \geq \olw (\beta_{\nstar})$. \red{so this is unclear: explain why equivalentely.} Equivalently, we can find $\alpha_{\uls}$ such that $\alpha_{\uls} \leq \alpha_{\nstar}$.

% \begin{align}\label{nu_bound_first_reduction}
%     \nu^2 
%     \leq
%     \frac{ B^2 }{ n \constnu } \frac{ \innerprod{ \gamma (\alphauls) }{ H }^2 }{ \alphauls^2 } 
%     \leq 
%     \frac{ B^2 }{ n \constnu } \frac{ \norm{H}_{\infty}^2 }{ \alphauls^2 }
% \end{align}

% Let $\tildewtwo = \frac{ \gamma (\alpha) }{ \alpha }$. The claim that $\alpha_{\nstar}$ satisfies constraints is once again straightforward from our definition of $B$. Now we want to find $\alphauls$ such that:
% \begin{align}\label{s_condition_nu_first_reduction}
%     \norm{ \tildewtwo }_2^2 = \frac{ \norm{ \gamma ( \alphauls ) }_2^2 }{ \alphauls^2 } > \frac{ \boundeta^2 }{ B^2 }
% \end{align}
% Using concentration result from lemma \ref{lemma_gamma_conc} and expression \eqref{phidn_bound} we get the condition:
% \begin{align}
%     \frac{2}{\uls} \left( 1 - \frac{c}{\tuls^2} \right) > \frac{\boundeta^2 \tnstar^2}{ n \fstar }
% \end{align}
% Once again we claim that this equality is satisfied for $ \uls = \frac{ c n }{ \log (d/n) } $ for some positive constant $c$. It is easy to see that this is the same condition as in the previous part of the proof up to the constants and hence we can use the same proof here.

% From \eqref{nu_bound_first_reduction} we now have:
% \begin{align}
%     \nu^2 \leq \frac{ \fstar \tuls^2 }{ \constnu \tnstar^2 } \left( 1 - \frac{4}{\tuls^2} \right)^{-1} 
%     \leq c'_{\nu} \left( 1 + O \left( \frac{ \log \log (d/n) }{\log (d/n) } \right) \right) \leq \boundnu^2
% \end{align}
% concluding the proof.



% \subsection{Proof of Lemma~\ref{lemma_second_reduction}}


% From lemma \ref{lemma_first_reduction} we know that with high probability $ \nu \leq c_{\nu} $ and $ \eta \leq c_{\eta} $. Hence we can use uniform convergence of $\fnclas$ to its expectation (proposition \ref{prop:unifConv}). Hence we can relax constraints from definition of set $\Gamma_0$ as follows:
% \begin{align}
%     \frac{ \innerprod{\wtwo}{H}^2 }{ n } \geq f ( \nu, \eta ) - \constconc \geq  \fstar  + \tconstnu \deltanu^2 + \tconsteta \eta^2 - \constconc
% \end{align}
% where the second inequality follows from lemma \ref{lemma_quadratic_4lus_fstar_bound}. Hence we consider set:
% \begin{align}
%     \Gamma_2^{\eta} = \left\{ (\wone,\wtwo) \subjto \frac{ \innerprod{\wtwo}{H}^2 }{ n } \geq \fstar - \constconc +  \tconsteta \eta^2  \andtxts \norm{ \wtwo }_1 \leq \loneboundclas  \right\}
% \end{align}

% \paragraph{Bounding $\eta$} 
% Following the same argument as in proof of lemma \ref{lemma_first_reduction} instead of inequality \eqref{eq:s_condition_one} we get:
% \begin{align}
%     \frac{ \left( \fstar - \constconc \right) \alpha_s^2 }{ B^2 \norm{H}_{\infty}^2 } + \tconsteta \frac{ \norm{ \gamma(\alpha_s) }_2^2 }{ \norm{H}_{\infty}^2 } > \frac{1}{n}
% \end{align}
% In order for inequality above to be satisfied we need:
% \begin{align}
%     \left( 1 - \frac{ \constconc }{ \fstar } \right) 
%     \frac{\tnstar^2}{t_s^2}
%     \left( 1 - \frac{4}{t_s^2} + O \left( \frac{1}{t_s^4} \right) \right) 
%     \left( 1 + \frac{2}{\tnstar^2} + O \left( \frac{1}{\tnstar^3} \right) \right) 
%     + \frac{2 n \tconsteta}{s t_s^2} \left( 1 + O \left( \frac{1}{t_s^2} \right) \right) 
%     > 1
% \end{align}
% Assuming that $ s = \lambda \nstar$ and $ \constconc = O \left( \frac{1}{\tnstar^3} \right) $ we have:
% \begin{align}
%     \frac{\tnstar^2}{t_s^2}
%     \left( 1 + \frac{ \frac{4\tconsteta}{\lambda\feestar}  - 4}{t_s^2} + \frac{2}{\tnstar^2} + O \left( \frac{1}{\tnstar^3}, \frac{1}{t_s^3} \right) \right)
%     > 1
% \end{align}
% Fix $\ulambda > 0$. Choose $\uls = \lambda_{\uls} \nstar$ such that $\uls < n$ is the largest integer for which $ \tuls^2 \geq \tnstar^2 + \ulambda $. Then we have condition:
% \begin{align}
%     \left( 1 - \frac{\ulambda}{\tuls^2} \right) \left( 1 + \frac{ \frac{4\tconsteta}{\lambda_{\uls}\feestar}  - 4}{\tuls^2} + \frac{2}{\tnstar^2} + O \left( \frac{1}{t_n^3} \right) \right)
%     > 1
% \end{align}
% For $\ulambda$ large enough inequality holds (Note: second brackets grow as $\lambda_{\uls}^{-1}$ and the first decays like $\log ( \lambda_{\uls} )$ - TO CHECK).


% \red{okay I messed this up - sorry. Can you make the following section a bit clearer? In particular, the connection to tn and s is not clear, cite the result form our paper. . So here we need to say that essentially we obtain the same problem as studied in my paper.}
% Fix $\olambda > 0$. Now we choose $\ols = c_{\ols} \nstar$ such that $ \ols > n $ is the smallest integer for which $ t_{\ols}^2 \leq \tnstar^2 - \olambda $. Then we have:
% \begin{align}
%     \left( 1 + \frac{\olambda}{\tols^2} \right) \left( 1 + \frac{ \frac{4\tconsteta}{c_{\ols}\feestar}  - 4}{\tols^2} + \frac{2}{\tnstar^2} + O \left( \frac{1}{t_n^3} \right) \right)
%     > 1
% \end{align}
% We claim that there exists $\olambda$ large enough such that this inequality holds (e.g. $\ulambda > 4$).

% Hence we can bound $\eta^2$ as follows:
% \begin{align} \label{eq:eta_bound_first_reduction}
%     \eta^2 
%     \leq
%     B^2 \frac{ \norm { \gamma ( \alphauls ) }_2^2 }{ \norm { \gamma ( \alphauls ) }_1^2 } 
%     \leq
%     \frac{ n \left( \fstar - \constconc \right) }{ \tnstar^2 } \frac{2}{\uls}\left( 1 + \frac{c}{\tuls^2} \right) 
%     \leq
%     \frac{c_{\eta}'}{\log (d/n) } \left( 1 + O \left( \frac{1}{ \log (d/n) } \right) \right) 
%     \leq
%     \left( \frac{ B_{\eta,2} }{ \sqrt{\log (d/n)} } \right)^2
% \end{align}
% and similarly we get:
% \begin{align}
%     \eta^2 
%     \geq
%     B^2 \frac{ \norm { \gamma ( \alphaols ) }_2^2 }{ \norm { \gamma ( \alphaols ) }_1^2 } 
%     \geq
%     \left( \frac{ \overline{B}_{\eta,2} }{ \sqrt{\log (d/n)} } \right)^2
% \end{align}

% \paragraph{Bounding $\nu$.}
% Following the proof of lemma \ref{lemma_first_reduction} we determine tighter upper bound for $\nu^2$.
% \begin{align}
%     \Gamma_2^{\nu} = \left\{ (\wone,\wtwo) 
%     \subjto
%     \frac{ \innerprod{\wtwo}{H}^2 }{ n } \geq \fstar - \constconc + \tconstnu \nu^2 \andtxts \norm{ \wtwo }_1 \leq \loneboundclas \andtxts \norm{ \wtwo }_2 \leq \frac{B_{\eta,2}}{\sqrt{ \log (d/n) }}  \right\}
% \end{align}

% Analogously to equation \eqref{s_condition_nu_first_reduction} we derive new condition for $\uls$ as:
% \begin{align}
%     \norm{ \tildewtwo }_2^2 = \frac{ \norm{ \gamma ( \alphauls ) }_2^2 }{ \alphauls^2 } > \frac{ B_{\eta,2}^2 }{ B^2 \log (d/n) }
% \end{align}
% which is again satisfied for some $\uls = \lambda_{\uls} n$ with $ \lambda_{\uls} > 0 $. Hence from \eqref{nu_bound_first_reduction} we obtain bound:
% \begin{align}
%     \deltanu^2 
%     \leq
%     \frac{ B^2 }{ n \tconstnu } \frac{ \norm{H}_{\infty}^2 }{ \alphauls^2 } - \frac{\fstar - \constconc }{\tconstnu}
%     \leq 
%     \frac{ \fstar }{ \tconstnu \tnstar^2 } \left( 1 + \frac{4}{\tuls^2} \right) - \frac{\fstar - \constconc }{\tconstnu}
%     \leq 
%     \left( \frac{ B_{\nu,2} }{ \sqrt{\log (d/n)} } \right)^2
% \end{align}
% which concludes the proof.











































% \section{Proof of Theorem \ref{thm:mainl1}}

% \red{Improve this, here we need to have the proof for L1}.

% \end{document}




















































% \subsection{Step 1: Reduce optimization problem via a path approach.}
% Following the work in \cite{wang2021tight} we can recast \eqref{eq:phin}, \eqref{eq:phip}, \eqref{eq:phim} as optimization problems in three scalar variables. Let $b,\alpha$ be scalar variables with $b\geq 0$, $\alpha\in[1,\alpham]$ with $\alpham = d\frac{\norm{\Hgaussian}_{\infty}}{\norm{\Hgaussian}_1}$. Then we define parametric path $b\gamma(\alpha)$ with $\RR^d$-valued function $\gamma$ given by:
% \begin{equation}
%     \gamma(\alpha) = \argmin_{\wtwo} \norm{\wtwo}_2^2
%     \subjto \begin{cases}
%                 \innerprod{\wtwo}{\Hgaussian} \geq \norm{\Hgaussian}_{\infty}\\
%                 \wtwo\geq 0\\
%                 \transp{\onevec} \wtwo = \norm{\wtwo}_1 = \alpha
%             \end{cases}
% \end{equation}

% We then obtain the following result. 
% \begin{restatable}{proposition}{propparam}
% % \begin{proposition} 
% \label{prop:parametrization}
% Optimization problems \eqref{eq:phin}, \eqref{eq:phip}, \eqref{eq:phim} are equivalently given by:
%         \begin{align}
%         \tag{$A_N$}\label{eq:phin}
%             \phidn &= \min_{\nu,b,\alpha} \nu + \alpha b
%             \subjto \frac{1}{n}  b^2\norm{\Hgaussian}_{\infty}^2  \geq  \fnclas(\nu,b\|\gamma(\alpha)\|_2). \\
%         \tag{$A_+$} \label{eq:phip}
%             \phidp &= \max_{\nu,b,\alpha}  \frac{\nu}{\sqrt{\nu^2+b^2\norm{\gamma(\alpha)}_2^2}}
%             \subjto 
%                   (\nu, b\norm{ \gamma(\alpha) }_2) \in \Gamma_0 \\
%         \tag{$A_-$} \label{eq:phim}
%             % \phidm &= \min_{\nu,b,\alpha}  \frac{\nu}{\sqrt{\nu^2+b^2\norm{\gamma(\alpha)}_2^2}}
%             % \subjto \begin{cases}
%             %   \frac{1}{n}  b^2\norm{\Hgaussian}_{\infty}^2  \geq  \fnclas(\wone,b\|\gamma(\alpha)\|_2)\\
%             %     \nu+b \leq \loneboundclas
%             % \end{cases}
%     \phidm &= \min_{\nu,b,\alpha}  \frac{\nu}{\sqrt{\nu^2+b^2\norm{\gamma(\alpha)}_2^2}}
%             \subjto
%               (\nu, b\norm{ \gamma(\alpha) }_2) \in \Gamma_0
%         \end{align}
% for some scalars $\nu,b>0$ and $\alpha\in[1,\alpham]$,
%  with
% $ \eta = b\norm{ \gamma(\alpha) }_2 $ and
% \begin{align}
%     \Gamma_0 = \left\{ (\nu,\eta) \subjto\frac{1}{n}  b^2\norm{\Hgaussian}_{\infty}^2  \geq  \fnclas(\nu,b\|\gamma(\alpha)\|_2) ~~\andtxt~~  \nu+b \leq \loneboundclas \right\}.
% \end{align}

% \end{restatable}  
% In order to study this reformulated optimization problem, we make use of the following two properties of $\gamma(\alpha)$ from \cite{wang2021tight}:

% \paragraph{Concentration of  $\norm{\gamma(\alpha)}_2$.} 
% From \cite{wang2021tight} we know that $ \gamma ( \alpha ) $ is a piecewise linear function with breakpoints at $ \alpha_s $ for $ s = 2, \dots, d$, with
% \begin{equation}
%     \alpha_s =....
% \end{equation}


% \begin{proposition}[Proposition 4 form \cite{wang2021tight}]
% \label{prop:concentrationl1}
% (Concentration of norms of $\gamma(\alpha_s)$, proposition 4 in \cite{konst}) Let $\ts$ be given by $2\Phic(\ts) = s/d$. There exists universal positive constants $c,c_s,c_2,c_3>0$ such that for any $s,d$ with $s\geq c_s$ and $c_2s\leq d\leq \exp(c_3 s^{1/5})$ we have that:
%     \begin{align}
%         \abs{
%             \frac{\norm{\gamma(\alphathr{s})}_1}{\norm{\Hgaussian}_\infty} - \left(\frac{1}{\ts} - \frac{2}{\ts^3}\right)
%         }
%         &\leq \frac{c}{\ts^5}
%         \qquad \andtxt \qquad
%         \abs{
%             \frac{\norm{\gamma(\alphathr{s})}_2^2}{\norm{\Hgaussian}_\infty^2} - \frac{2}{s \ts^2}
%         }
%         \leq \frac{c}{s \ts^4}, \label{eq:concentration}
%     \end{align}
% with probability at least $1-6\exp\left(-\frac{s}{\log(d/s)^5}\right)$ over the draws of $h$.
% \label{lemma_gamma_conc}
% \end{proposition}

% \paragraph{Convexity and monotonicity of  $\gamma(\alpha)$. }


% \red{State monotinicity result here.}


% \subsection{Step 2: Localisation step - bounding $\phidn$}
% In a first step, we derive an upper bound on $\phidn$. For this, it is sufficient to find a feasible point. Let $f(\nu,\eta) = \EE \left[ \possq{1-\xi\abs{\gausswone}\nu-\gausswtwo \eta} \right] $ be the expectation of $\fnclas$ over $\xsui$, $\Ggaussian$ and $\xi$. Using the concentration of Lipschitz continuous function, we can show that:
% \begin{lemma}
% \label{lemma_point_conv}
% For any $\nu,\eta>0$ holds that:
%     \begin{align}
%         \prob \left( \abs{ \fnclas \left( \nu, \eta \right) - \EE \left[ \fnclas \left( \nu, \eta \right) \right] }  \geq t \right) \leq 2 \exp \left( - c \frac{ n t^2 }{ \nu^2 + \eta^2 } \right)
%     \end{align}
% where $c$ is a positive universal constant. 
% \end{lemma} 

% The goal is now to show that we can find a feasible point $(\nubar, \eta)$ with $\nubar = \argmin f(\nu, 0)$ and $\eta = O(\frac{1}{\log(d/n)}$. For this, we can take the Taylor series approximation of $f$ around$(\nuopt,0)$,   $f(\nu, \vstar) \approx \fstar + \fnclasunu \nu^2$, which allows us to rewrite the constraint in $\phidn$ to 
% \begin{equation}
%     \frac{1}{n}  b^2\norm{\Hgaussian}_{\infty}^2  \geq  \fstar + \fnclasunu \nu^2 + O(...).
% \end{equation}

% Further, following a similar approach as in Proposition~2 in \cite{wang2021tight} by applying the concentration results in Proposition~\ref{prop:concentrationl1}, we can show the following Proposition~\ref{prop:Rbound} which gives an upper bound on $\phdn$. The proof is devoted to Appendix ...

% % a similar approach in the proof of Proposition~2 in \cite{wang2021tight}, where tight bounds for $\phidn$ for min-l1-norm interpolation are derived, we can show the following bound on $\phidn$ given in  Proposition \ref{prop:Rbound}. The proof may be found in Appendix~... 
% \begin{restatable}{proposition}{propRbound}
% \label{prop:Rbound}
% Let $t_{\nopt}$ be given by $2\Phic(t_{\nopt}) = \nopt/d$ with $\nopt = n\feestar/2$. There exist universal positive constants $c,c_1,c_2,c_3,c_4$ such that, if $n\geq c_1$ and $c_2 n\leq d\leq \exp(c_3 n^{1/5})$ then
%     \begin{align} \label{phidn_bound}
%         (\phidn)^2 
%         \leq
%         \frac{ n f (\nuopt, 0) }{ \tnstar^2 } \left( 1 - \frac{ 2 }{ \tnstar^2 } + \frac{c}{ \tnstar^3 } \right) =:\loneboundclas^2
%     \end{align}
% with probability at least $ 1 - 2 \exp \left( -\frac{ c_4 n }{ \tnstar^6 } \right) - 6 \exp \left( -\frac{\nstar}{\log^5(d/\nstar)} \right) $ over the draws of $\Hgaussian$, $\gausswone$ and $\gausswtwo$.
% \end{restatable}  





% \subsection{Step 3: Uniform convergence.}
% The goal of this is to study the constraint set $\Gamma_0$ given the bound $M \geq \phidn$ from the previous step. In particular, we show the following Proposition ~\ref{prop:BoundOmegal1}. The bounds on $\phidn$ and $\phidp$ then follow straightforwardly in the next section. 

% \begin{restatable}{proposition}{BoundOmegal1}
% \label{prop:BoundOmegal1}
% There exist universal constants $ c_1, c_2, c_1, c_2, c_3 > 0 $ such that, if $ n\geq c_1 $ and $ c_2 n \leq d \leq \exp \left( c_3 n^{1/5} \right) $, then
% \red{Stefan, need to make this tighter!}
% \begin{align}
% \Gamma_0 \subset \{(\nu, \eta) \subjto  \vert \eta^2 \vert = \Gamma(1/\log(d/n))~~\andtxt~~ \vert \nu-\nubar\vert = O(1/\log(d/n))\}
% \end{align}
% with probability at least $ 1 - $.
% \end{restatable}  
% \begin{proof}
% The proof of the proposition follows from several steps where in each step we approximate $\fnclas$ using the the bounds on $(\nu, \eta)$ from the previous steps to obtain a tighter bound on $(\nu, \eta)$ using the tools developed in \cite{wang2021tight}.  



% \paragraph{Bound 1:}
% In a first step, we use the fact that in the presence of label noise, $\fnclas$ is lower bounded by a quadratic function:
% \begin{lemma} \label{quadratic_bound_fn}
%     There exist positive constants $\constnu$ and $\consteta$ such that for any $\nu,\eta$ we have that: 
%         \begin{align}
%             \fnclas(\nu,\eta) \geq \constnu \nu^2  + \consteta \eta^2
%         \end{align}
%     with probability at least $1 - \exp \left( - n \kldiv{\frac{\sigma}{2}}{\frac{\sigma}{4}} \right) - \exp \left( -\frac{ n\sigma }{ 128 } \right)$ over the draws of $\gausswone,\gausswtwo,\xi$.
% \end{lemma}
% As a result, we can approximate relax the first constraint in $\Gamma_0$ to 
% \begin{equation}
%     b^2\norm{\Hgaussian}_{\infty}^2  \geq  \constnu \nu^2  + \consteta \eta^2.
% \end{equation} 

% \red{say more about the intuition, then we can show:}

% \begin{lemma} \label{lemma_first_reduction}
%     There exist universal constant $c > 0$ such that for any element $(\wone,\wtwo)$ of $\Gamma_0$ we have that $\norm{ \wone }_2 = \nu \leq \boundnu $ and $\norm{ \wtwo }_2 = \eta \leq \boundeta$ with probability at least $ 1 - $ over the draws of $..$.
% \end{lemma}


% \paragraph{Bound 2:}
% Define $\deltanu= \nu - \nubar$. Using the fact from the previous section that $\nu \leq \constnu, \eta \leq \consteta$, we obtain a tigher lower bound for $\fnclas$ form the following lemma. 

% \begin{lemma} \label{lemma_quadratic_4lus_fstar_bound}
%     There exist positive constants $\tconstnu$ and $\tconsteta$ such that for any $\nu \leq \constnu, \eta \leq \consteta$ we have that: 
%         \begin{align}
%             f(\nu,\eta) \geq \fstar + \tconstnu \left( \deltanu \right)^2  + \tconsteta \eta^2+ \OOOc
%         \end{align}
%     with probability at least $1 - \exp \left( - n \kldiv{\frac{\sigma}{2}}{\frac{\sigma}{4}} \right) - \exp \left( -\frac{ n\sigma }{ 128 } \right)$ over the draws of $\gausswone,\gausswtwo,\xi$.
% \end{lemma}

% Plugging in this expression, we can again show:
% \begin{lemma} \label{lemma_second_reduction}
%     There exist universal constants $B_{\nu,2} > 0, B_{\eta,2} > 0$ such that for any element $(\wone,\wtwo)$ of $\Gamma_0$ we have that $\deltanu^2 \leq \frac{B_{\nu,2}^2}{ \log \left( d/n \right) }$ and $ \eta^2 \leq \frac{B_{\eta,2}^2}{ \log \left( d/n \right) }$ with probability at least $ 1 - $ over the draws of $..$.
% \end{lemma}


% \paragraph{Bound 3:}
% This is still under work...
% \begin{lemma}
%     There exist universal constant $B_{\nu,3} > 0, B_{\eta,3} > 0$ such that for any element $(\wone,\wtwo)$ of $\Gamma_0$ we have that $\deltanu^2 \leq \frac{B_{\nu,3}^2}{ \left( \log \left( d/n \right) \right)^{3/2} }$ and $ \eta^2 \leq \frac{B_{\eta,3}^2}{ \log \left( d/n \right) }$ with probability at least $ 1 - $ over the draws of $..$.
% \end{lemma}






% \end{proof}



% \subsection{Summary. }
% We have:
% \begin{align}
%     \max \frac{ \nu }{ \sqrt{ \nu^2 + \eta^2 } } 
%     & \leq
%     \frac{ \nubar + \deltanu }{ \sqrt{ ( \nubar + \deltanu )^2 + \eta^2 } }
%     \\
%     & = 
%     \left( 1 + \frac {\deltanu}{\nubar} \right) \left( 1 - \frac{1}{2} \left( \frac{2\deltanu}{\nubar} + \frac{\deltanu^2 + \eta^2}{(\nubar)^2} \right) + \frac{3}{8} \left( \frac{2\deltanu}{\nubar}\right)^2 + O \left( \frac{1}{ \log (d/n)^{3/2}} \right) \right)
%     \\
%     & = 1 - \frac{\eta^2}{2(\nubar)^2} + O \left( \frac{1}{ \log (d/n)^{3/2}} \right) 
%     \leq 
%     1 - W \left( \frac{1}{\log (d/n) } \right)
% \end{align}
% and
% \begin{align}
%     \min \frac{ \nu }{ \sqrt{ \nu^2 + \eta^2 } } 
%     & \geq
%     \frac{ \nubar - \deltanu }{ \sqrt{ ( \nubar - \deltanu )^2 + \eta^2 } }
%     \\
%     & = 
%     \left( 1 - \frac {\deltanu}{\nubar} \right) \left( 1 - \frac{1}{2} \left( -\frac{2\deltanu}{\nubar} + \frac{\deltanu^2 + \eta^2}{(\nubar)^2} \right) + \frac{3}{8} \left( \frac{2\deltanu}{\nubar}\right)^2 + O \left( \frac{1}{ \log (d/n)^{3/2}} \right) \right)
%     \\
%     & = 1 - \frac{\eta^2}{2(\nubar)^2} + O \left( \frac{1}{ \log (d/n)^{3/2}} \right) 
%     \geq 
%     1 - O \left( \frac{1}{\log (d/n) } \right)
% \end{align}

% Using approximation $ \arccos(1-x) \approx \sqrt{2x} + O (x\sqrt{x}) $ we have
% \begin{align}
%     W \left( \frac{1}{\log (d/n)^{1/2} }  \right) 
%     \leq
%     R(w) = \frac{1}{\pi} \arccos \left( \frac{\innerprod{w}{\wgt}}{\norm{w}_2} \right) 
%     \leq 
%     O \left( \frac{1}{\log (d/n)^{1/2} } \right)
% \end{align}
% with high probability $ 1 - $.





% \subsection{Proof of Proposition~\ref{prop:Rbound}}


% Recall that $\phidn$ is given by:
% \begin{align}
%     \phidn &= \min_{\nu,b,\alpha} \nu + b \norm{ \gamma \left( \alpha \right) }_1 
%     \subjto \frac{ b^2\norm{\Hgaussian}_{\infty}^2 }{n} \geq \fnclas \left( \nu, b \norm{ \gamma \left( \alpha \right) }_2 \right)
% \end{align}

% Given that $(\tnu,\tb,\talpha)$ is a feasible point of $\phidn$ we have that $\phidn \leq  \tnu + \tb \norm{ \gamma( \talpha) }_1$, which gives us an upper bound on $\phidn$. In the following discussion our goal is to find a single feasible point of the constraint set of $\phidn$.

% From definition of $\gamma ( \alpha )$ we know that $ \norm{ \gamma ( \alpha ) }_1 = \alpha$ and hence we can equivalently formulate $\phidn$ as an optimization over $\nu$ and $ b_{\alpha} := b \alpha $
% \begin{align}
%     \phidn &= \min_{ \nu, b_{\alpha} } \nu + b_{\alpha}
%     \subjto \frac{ b_{\alpha}^2 \norm{\Hgaussian}_{\infty}^2 }{n \alpha^2} \geq \fnclas \left( \nu, b_{\alpha} \frac{ \norm{ \gamma \left( \alpha \right) }_2}{ \alpha } \right)
% \end{align}

% Define $\fstar = f \left( \nubar, 0 \right)$, $\feestar = \frac{\partial^2 f(\nuopt,\eta)}{\partial \eta^2}\Big|_{\eta=0}$ and $\nstar = \frac{1}{2}\feestar n$. Now using lemma \ref{lemma_point_conv} with $ t = \fstar \tnstar^{-3} $ and for a feasible point $( \nu, b_{\alpha} \frac{ \norm{ \gamma \left( \alpha \right) }_2}{ \alpha } )$ we have that:
% \begin{align} \label{eq:constraint_f_conc}
%     \frac{ b_{\alpha}^2 \norm{\Hgaussian}_{\infty}^2 }{n \alpha^2} 
%     \geq
%     f \left( \nu, b_{\alpha} \frac{ \norm{ \gamma \left( \alpha \right) }_2}{ \alpha } \right) + \frac{\fstar}{\tnstar^{3}}
% \end{align}
% with probability at least $ 1 - 2 \exp \left( -c \frac{ n }{ \tnstar^6 \left( \nu^2 + b_{\alpha}^2  \norm{ \gamma \left( \alpha \right) }_2^2 / \alpha^2 \right) } \right) $.
% % > 1 - 2 \exp \left( - \tc \frac{ n }{ \log^3 \left( \frac{d}{n} \right)  } \right) $.

% Let's now choose $ \nu = \nubar $ and show that there exists a pair $ ( b, \alpha )$  such that $ ( \nubar, b, \alpha) $ is feasible for constraint \eqref{eq:constraint_f_conc}. Furthermore, we propose to search for a point with parameter $ ( b, \alpha ) $ such that $ b \norm{ \gamma ( \alpha )}_2 = b_{\alpha} \frac{ \norm{ \gamma \left( \alpha \right) }_2}{ \alpha } $ is near zero. Hence, using Taylor series approximation of function $ f ( \nubar, \cdot ) : \eta \mapsto f (\nubar, \eta) $ around point $(\nuopt,0)$ we can rewrite constraint \eqref{eq:constraint_f_conc} as:
% \begin{align}
%      \frac{ b_{\alpha}^2 \norm{\Hgaussian}_{\infty}^2 }{n \alpha^2}   
%      \geq
%       \fstar + \frac{1}{2}\feestar b_{\alpha}^2 \frac{ \norm{ \gamma \left( \alpha \right) }_2^2}{ \alpha^2 } + O \left( b_{\alpha}^3 \frac{ \norm{ \gamma \left( \alpha \right) }_2^3}{ \alpha^3 } \right) + \frac{\fstar}{\tnstar^{3}}
% \end{align}
% since $\feta = \frac{\partial f(\nuopt,\eta)}{\partial \eta}\Big|_{\eta=0} = 0$.

% Now from \cite{wang2021tight} we know that $ \gamma ( \alpha ) $ is a piecewise linear function with breakpoints at $ \alpha_s $ for $ s = 2, \dots, d $. Hence instead of optimizing over $\alpha$ we optimize over $s$. Note that we have only one constraint but two free variables $ ( b, \alpha ) $ and so we can set $ \alpha = \alpha_{\nstar} $ with $ \nstar = \frac{1}{2}\feestar n $. We explain this choice of $s$ in the remark after the proof. Combining all these results we get constraint:
% \begin{align} \label{eq:B_ineq}
%      \frac{ b_{\alpha_{\nstar}}^2 \norm{\Hgaussian}_{\infty}^2 }{n \alpha_{\nstar}^2}   
%      \geq
%       \fstar + \frac{1}{2}\feestar b_{\alpha_{\nstar}}^2 \frac{ \norm{ \gamma \left( \alpha_{\nstar} \right) }_2^2}{ \alpha_{\nstar}^2 } + O \left( b_{\alpha_{\nstar}}^3 \frac{ \norm{ \gamma \left( \alpha_{\nstar} \right) }_2^3}{ \alpha_{\nstar}^3 } \right) + \frac{\fstar}{\tnstar^{3}}
% \end{align}

% Now we claim that
% \begin{equation}
%     b_{\alpha_{\nstar}}^2 = \frac{ n \alpha_{\nstar}^2 }{ \norm{\Hgaussian}_2^2 } \frac{ \fstar \left( 1 + \frac{1}{\tnstar^{3}} \right) }{ 1 - \frac{1}{2} n \feestar \frac{ \norm{ \gamma \left( \alpha_{\nstar} \right) }_2^2 }{ \norm{H}_{\infty}^2 } - O \left( \frac{1}{\tnstar^3} \right) }
% \end{equation}
% satisfies inequality \eqref{eq:B_ineq} with probability at least $ 1 - 6 \exp \left( -\frac{\nstar}{\log^5(d/\nstar)} \right)$. Using lemma \ref{lemma_gamma_conc} we have that:
% \begin{equation}
%     1 - \frac{1}{2} n \feestar \frac{ \norm{ \gamma \left( \alpha_{\nstar} \right) }_2^2 }{ \norm{H}_{\infty}^2 } - O \left( \frac{1}{\tnstar^3} \right) > 1 - \frac{1}{2} n \feestar  \frac{2}{\nstar \tnstar^2} - O \left( \frac{1}{\tnstar^3} \right) = 1 - \frac{2}{\tnstar^2} - O \left( \frac{1}{\tnstar^3} \right)  > 0
% \end{equation}
% holding for $d,n$ sufficiently large. Applying lemma \ref{lemma_gamma_conc} once again we get:
% \begin{equation}
%     b_{\alpha_{\nstar}}^2 
%     \leq
%     \frac{ n \fstar }{ \tnstar^2 } \left( 1 + \frac{1}{\tnstar^3} \right) \left( 1 - \frac{4}{\tnstar^2} + \frac{c}{\tnstar^4} \right) \frac{1}{ 1 - \frac{2}{\tnstar^2} - O \left( \frac{1}{\tnstar^3} \right)}
%     \leq
%     \frac{ n \fstar }{ \tnstar^2 } \left( 1 - \frac{2}{\tnstar^2} + \frac{c}{\tnstar^3} \right)
% \end{equation}

% Hence we have that $ O \left( b_{\alpha_{\nstar}}^3 \frac{ \norm{ \gamma \left( \alpha_{\nstar} \right) }_2^3}{ \alpha_{\nstar}^3 } \right) = O \left( \frac{1}{\tnstar^3} \right)$ and this $b_{\alpha_{\nstar}}^2$ indeed satisfies equation \ref{eq:B_ineq}. Now we define the upper bound on $\phidn$ as:
% \begin{align}
%     \loneboundclas := \sqrt{ \frac{ n \fstar }{ \tnstar^2 } \left( 1 - \frac{2}{\tnstar^2} + \frac{c}{\tnstar^3} \right) }
% \end{align}
% which holds with probability at least $ 1 - 2 \exp \left( -c \frac{ n }{ \tnstar^6 \left( (\nubar)^2 + b_{\alpha_{\nstar}}^2  \norm{ \gamma \left( \alpha_{\nstar} \right) }_2^2 / \alpha_{\nstar}^2 \right) } \right) - 6 \exp \left( -\frac{\nstar}{\log^5(d/\nstar)} \right) $. The proposition is proved after noting that $ (\nubar)^2 + b_{\alpha_{\nstar}}^2  \norm{ \gamma \left( \alpha_{\nstar} \right) }_2^2 / \alpha_{\nstar}^2 = O(1)$.

% \subsection{Proof of Lemma~\ref{lemma_first_reduction}}
% According to lemma \ref{quadratic_bound_fn} we have that for any pair $ ( \nu, \eta ) $ with probability at least $ 1 - \exp \left( - n \kldiv{\frac{\sigma}{2}}{\frac{\sigma}{4}} \right) - \exp \left( -\frac{ n\sigma }{ 128 } \right) $ that $ \fnclas ( \nu, \eta) \geq \constnu \nu^2 + \consteta \eta^2 $ for some positive constants $\constnu$ and $\consteta $. Hence with high probability we can relax first constraint defining $\Gamma_0$ to
% \begin{align}
%     \frac{ \innerprod{\wtwo}{H}^2 }{ n } \geq \constnu \nu^2 + \consteta  \eta^2
% \end{align}
% Furthermore we can relax both constraints to define the following set:
% \begin{align}
%     \Gamma_1^{\eta} = \left\{ (\wone,\wtwo) \subjto \frac{ \innerprod{\wtwo}{H}^2 }{ n } \geq \consteta  \eta^2 \andtxts \norm{ \wtwo }_1 \leq \loneboundclas  \right\}
% \end{align}
% It is evident from definition that $ \Gamma_0 \subset \Gamma_1^{\eta}$ with high probability. Also note that constraints in the set $\Gamma_1^{\eta}$ depend only on $\wtwo$ and hence we will now consider only this variable. Now we bound $ \eta = \norm{ \wtwo }_2 $ as:
% \begin{align}
%     \eta^2 \leq \max_{\wtwo} \norm { \wtwo }_2 \subjto \wtwo \in \Gamma_1^{\eta}
% \end{align}

% We proceed following the path arguments established in \cite{wang2021tight}. We parametrize variable $\wtwo$ as $ \wtwo = b \norm { \gamma ( \alpha ) } $. 

% First we show that set $\Gamma_1^{\eta}$ is not empty. Let's choose $ \alpha = \alpha_{\nstar}$ with $\nstar = n\feestar/2$. Since we defined $ \loneboundclas $ in such way that $ \alpha_{\nstar} \in \Gamma_0 $ with high probability and we have $ \Gamma_0 \subset \Gamma_1^{\eta}$, this implies that with high probability there exists some $ b > 0 $ such that $ b \gamma ( \alpha ) \in \Gamma_1^{\eta} $.

% Using the same argument as in lemma 1 in \cite{wang2021tight} for $\phidp$ we can write:
% \begin{align}
%     \eta^2 \leq \max_{1\leq \alpha \leq \alpham} B^2 \frac{ \norm { \gamma ( \alpha ) }_2^2 }{ \norm { \gamma ( \alpha ) }_1^2 } \subjto B\gamma \left( \alpha \right) \in \Gamma_1^{\eta}
% \end{align}

% Now from lemma 4 in \cite{wang2021tight} we have that map $ \alpha \mapsto \frac{ \norm{ \gamma ( \alpha ) }_2^2 }{ \norm{ \gamma ( \alpha ) }_1^2 } $ is monotonically decreasing. Hence if we find value of $\alpha_{\uls}$ such that $\alpha_{\uls} \leq \alpha_{\nstar}$ and $ b \gamma ( \alpha_{\uls} ) \not \in \Gamma_1^{\eta}$ for any $ b > 0 $ then we have:
% \begin{align} \label{eq:eta_bound_first_reduction}
%     \eta^2 \leq  B^2 \frac{ \norm { \gamma ( \alphauls ) }_2^2 }{ \norm { \gamma ( \alphauls ) }_1^2 }
% \end{align}

% In order to saturate constraint $ \norm{ \wtwo }_1 \leq B $ let $ b = \frac{B}{\alphauls}$. Since we want that $  b \gamma ( \alpha_{\uls} ) \not \in \Gamma_1^{\eta} $ we will chose $s$ such that:
% \begin{align}
%     B^2 \frac{ \innerprod{ \gamma ( \alphauls )}{H}^2 }{ n \alphauls^2 } < \consteta B^2 \frac{ \norm{ \gamma ( \alphauls ) }_2^2 }{ \alphauls^2 }
% \end{align}
% Rewriting this inequality gives:
% \begin{align} \label{eq:s_condition_one}
%   \frac{ \norm{ \gamma ( \alphauls ) }_2^2 }{ \norm{H}_{\infty}^2 } > \frac{ 1 }{ \consteta n } 
% \end{align}
% Now we use concentration result from lemma \ref{lemma_gamma_conc} to get the following condition on $s$:
% \begin{align}
%     \frac{ 2 }{ \uls t_s^2 } \left( 1 - \frac{ c }{ \tuls^2 } \right) > \frac{ 1 }{ \consteta n }
% \end{align}

% We claim that $\uls = \lambda_{\uls} \frac{ n }{ \log (d/n) }$ satisfies this inequality for some positive constant $ \lambda_{\uls} $. From lemma 3 in \cite{wang2021tight} we know that if $ d/\uls \geq 11 $ we have that $ \log (d/\uls) \leq \tuls^2 \leq 2 \log (d/\uls) $. Using both of these bounds into expression \eqref{eq:s_condition_one} gives that:
% \begin{align}
%     \frac{ 2 }{ \uls \tuls^2 } \left( 1 - \frac{ c }{ \tuls^2 } \right) &> \frac{ 1 }{ 2 n \lambda_{\uls} } \frac{ \log (d/n) }{ \log (d/n) + \log \log (d/n) - \log \lambda_{\uls} } \left( 1 - \frac{c}{ \log (d/n) + \log \log (d/n) - \log \lambda_{\uls} } \right)
%     \\
%     & = \frac{ 1 }{ 2 n \lambda_{\uls} } \left( 1 - O \left( \frac{\log (d/n) }{\log \log (d/n) } \right) \right) > \frac{1}{\consteta n}
% \end{align}
% where last inequality holds for $d/n$ sufficiently large.

% Now from equation \eqref{eq:eta_bound_first_reduction} and concentration lemma \ref{lemma_gamma_conc} we have:
% \begin{align}
%     \eta^2 \leq \frac{ n \fstar }{ \tnstar^2 } \frac{2}{\uls}\left( 1 + \frac{c}{\tuls^2} \right) \leq \boundeta' \left( 1 + O \left( \frac{1}{ \log (d/n) } \right) \right) \leq \boundeta^2
% \end{align}

% Now we derive an upper bound for $\nu$. We consider the following set:
% \begin{align}
%     \Gamma_1^{\nu} = \left\{ (\wone,\wtwo) 
%     \subjto
%     \frac{ \innerprod{\wtwo}{H}^2 }{ n } \geq \constnu \nu^2 \andtxts \norm{ \wtwo }_1 \leq \loneboundclas \andtxts \norm{ \wtwo }_2 \leq \boundeta  \right\}
% \end{align}
% Once again it follows that $\Gamma_0 \subset \Gamma_1^{\nu}$. Hence we can upper bound $\nu$ as follows:
% \begin{align} \label{eq:nu_opt_first_reduction}
%     \nu^2 \leq \frac{ 1 }{ n \constnu } \max_{\wtwo} \innerprod{\wtwo}{H}^2
%     \subjto 
%     \norm{ \wtwo }_1 \leq \loneboundclas 
%     \andtxts 
%     \norm{ \wtwo }_2 \leq \boundeta
% \end{align}

% Now we show can this optimization problem can be rewritten in a form suitable for using parametrized path approach. Similarly as in \cite{wang2021tight} we define function $\olw : \left[ \frac{1}{d}, 1 \right] \to \RR^{d-1}$ as
% \begin{align}
%     \olw(\beta) = \argmax_{\wtwo} \innerprod{\wtwo}{\Hgaussian}
%     \subjto \begin{cases}
%                 \norm{\wtwo}_2^2 \leq \beta \\
%                 \wtwo\geq 0\\
%                 \norm{\wtwo}_1 = 1
%             \end{cases}
% \end{align}
% From claim 2 in \cite{wang2021tight} we know that for any $\beta \in \left[ \frac{1}{d}, 1 \right] $ there exists $ \alpha \in \left[ 1, \alpham \right] $ such that $ \olw (\beta) = \frac{ \gamma(\alpha) }{ \alpha }$. Following similar argument as in fourth statement of lemma 4 in \cite{wang2021tight} we have that $ \olw (\beta) $ is monotonically increasing function in $\beta$. 

% Setting $ \tildewtwo = \frac{ \wtwo }{ B }$ we can rewrite \eqref{eq:nu_opt_first_reduction} as:
% \begin{align} 
%     \nu^2 \leq \frac{ B^2 }{ n \constnu } \max_{\tildewtwo} \innerprod{ \tildewtwo }{ H }^2
%     \subjto 
%     \norm{ \tildewtwo }_1 \leq 1 
%     \andtxts 
%     \norm{ \tildewtwo }_2 \leq \frac{ \boundeta }{ B }
% \end{align}
% Hence solution of this problem must be of the form $ \tildewtwo = \olw (\beta) $ for some $\beta$. Similarly as in the first part of this proof, we first show that there exists $\beta_{\nstar}$ which satisfies constraints, and then find $\beta_{\ols}$ such that $ \beta_{\ols} \geq \beta_{\nstar}$. From monotonicity of $ \olw (\beta)$ follows that $ \olw (\beta_{\ols}) \geq \olw (\beta_{\nstar})$. Equivalently, we can find $\alpha_{\uls}$ such that $\alpha_{\uls} \leq \alpha_{\nstar}$.

% \begin{align}\label{nu_bound_first_reduction}
%     \nu^2 
%     \leq
%     \frac{ B^2 }{ n \constnu } \frac{ \innerprod{ \gamma (\alphauls) }{ H }^2 }{ \alphauls^2 } 
%     \leq 
%     \frac{ B^2 }{ n \constnu } \frac{ \norm{H}_{\infty}^2 }{ \alphauls^2 }
% \end{align}

% Let $\tildewtwo = \frac{ \gamma (\alpha) }{ \alpha }$. The claim that $\alpha_{\nstar}$ satisfies constraints is once again straightforward from our definition of $B$. Now we want to find $\alphauls$ such that:
% \begin{align}\label{s_condition_nu_first_reduction}
%     \norm{ \tildewtwo }_2^2 = \frac{ \norm{ \gamma ( \alphauls ) }_2^2 }{ \alphauls^2 } > \frac{ \boundeta^2 }{ B^2 }
% \end{align}
% Using concentration result from lemma \ref{lemma_gamma_conc} and expression \eqref{phidn_bound} we get the condition:
% \begin{align}
%     \frac{2}{\uls} \left( 1 - \frac{c}{\tuls^2} \right) > \frac{\boundeta^2 \tnstar^2}{ n \fstar }
% \end{align}
% Once again we claim that this equality is satisfied for $ \uls = \frac{ c n }{ \log (d/n) } $ for some positive constant $c$. It is easy to see that this is the same condition as in the previous part of the proof up to the constants and hence we can use the same proof here.

% From \eqref{nu_bound_first_reduction} we now have:
% \begin{align}
%     \nu^2 \leq \frac{ \fstar \tuls^2 }{ \constnu \tnstar^2 } \left( 1 - \frac{4}{\tuls^2} \right)^{-1} 
%     \leq c'_{\nu} \left( 1 + O \left( \frac{ \log \log (d/n) }{\log (d/n) } \right) \right) \leq \boundnu^2
% \end{align}
% concluding the proof.



% \subsection{Proof of Lemma~\ref{lemma_second_reduction}}


% From lemma \ref{lemma_first_reduction} we know that with high probability $ \nu \leq c_{\nu} $ and $ \eta \leq c_{\eta} $. Hence we can use uniform convergence of $\fnclas$ to its expectation (proposition \ref{prop:unifConv}). Hence we can relax constraints from definition of set $\Gamma_0$ as follows:
% \begin{align}
%     \frac{ \innerprod{\wtwo}{H}^2 }{ n } \geq f ( \nu, \eta ) - \constconc \geq  \fstar  + \tconstnu \deltanu^2 + \tconsteta \eta^2 - \constconc
% \end{align}
% where the second inequality follows from lemma \ref{lemma_quadratic_4lus_fstar_bound}. Hence we consider set:
% \begin{align}
%     \Gamma_2^{\eta} = \left\{ (\wone,\wtwo) \subjto \frac{ \innerprod{\wtwo}{H}^2 }{ n } \geq \fstar - \constconc +  \tconsteta \eta^2  \andtxts \norm{ \wtwo }_1 \leq \loneboundclas  \right\}
% \end{align}

% Following the same argument as in proof of lemma \ref{lemma_first_reduction} instead of inequality \eqref{eq:s_condition_one} we get:
% \begin{align}
%     \frac{ \left( \fstar - \constconc \right) \alpha_s^2 }{ B^2 \norm{H}_{\infty}^2 } + \tconsteta \frac{ \norm{ \gamma(\alpha_s) }_2^2 }{ \norm{H}_{\infty}^2 } > \frac{1}{n}
% \end{align}
% In order for inequality above to be satisfied we need:
% \begin{align}
%     \left( 1 - \frac{ \constconc }{ \fstar } \right) 
%     \frac{\tnstar^2}{t_s^2}
%     \left( 1 - \frac{4}{t_s^2} + O \left( \frac{1}{t_s^4} \right) \right) 
%     \left( 1 + \frac{2}{\tnstar^2} + O \left( \frac{1}{\tnstar^3} \right) \right) 
%     + \frac{2 n \tconsteta}{s t_s^2} \left( 1 + O \left( \frac{1}{t_s^2} \right) \right) 
%     > 1
% \end{align}
% Assuming that $ s = c \nstar$ and $ \constconc = O \left( \frac{1}{\tnstar^3} \right) $ we have:
% \begin{align}
%     \frac{\tnstar^2}{t_s^2}
%     \left( 1 + \frac{ \frac{4\tconsteta}{c\feestar}  - 4}{t_s^2} + \frac{2}{\tnstar^2} + O \left( \frac{1}{\tnstar^3}, \frac{1}{t_s^3} \right) \right)
%     > 1
% \end{align}
% Fix $\ulambda > 0$. Choose $\uls = \lambda_{\uls} \nstar$ such that $\uls < n$ is the largest integer for which $ \tuls^2 \geq \tnstar^2 + \ulambda $. Then we have condition:
% \begin{align}
%     \left( 1 - \frac{\ulambda}{\tuls^2} \right) \left( 1 + \frac{ \frac{4\tconsteta}{\lambda_{\uls}\feestar}  - 4}{\tuls^2} + \frac{2}{\tnstar^2} + O \left( \frac{1}{t_n^3} \right) \right)
%     > 1
% \end{align}
% For $\ulambda$ large enough inequality holds (Note: second brackets grow as $\lambda_{\uls}^{-1}$ and the first decays like $\log ( \lambda_{\uls} )$ - TO CHECK).

% Fix $\olambda > 0$. Now we choose $\ols = c_{\ols} \nstar$ such that $ \ols > n $ is the smallest integer for which $ t_{\ols}^2 \leq \tnstar^2 - \olambda $. Then we have:
% \begin{align}
%     \left( 1 + \frac{\olambda}{\tols^2} \right) \left( 1 + \frac{ \frac{4\tconsteta}{c_{\ols}\feestar}  - 4}{\tols^2} + \frac{2}{\tnstar^2} + O \left( \frac{1}{t_n^3} \right) \right)
%     > 1
% \end{align}
% We claim that there exists $\olambda$ large enough such that this inequality holds (e.g. $\ulambda > 4$).

% Hence we can bound $\eta^2$ as follows:
% \begin{align} \label{eq:eta_bound_first_reduction}
%     \eta^2 
%     \leq
%     B^2 \frac{ \norm { \gamma ( \alphauls ) }_2^2 }{ \norm { \gamma ( \alphauls ) }_1^2 } 
%     \leq
%     \frac{ n \left( \fstar - \constconc \right) }{ \tnstar^2 } \frac{2}{\uls}\left( 1 + \frac{c}{\tuls^2} \right) 
%     \leq
%     \frac{c_{\eta}'}{\log (d/n) } \left( 1 + O \left( \frac{1}{ \log (d/n) } \right) \right) 
%     \leq
%     \left( \frac{ B_{\eta,2} }{ \sqrt{\log (d/n)} } \right)^2
% \end{align}
% and similarly we get:
% \begin{align}
%     \eta^2 
%     \geq
%     B^2 \frac{ \norm { \gamma ( \alphaols ) }_2^2 }{ \norm { \gamma ( \alphaols ) }_1^2 } 
%     \geq
%     \left( \frac{ \overline{B}_{\eta,2} }{ \sqrt{\log (d/n)} } \right)^2
% \end{align}

% Following the proof of lemma \ref{lemma_first_reduction} we determine tighter upper bound for $\nu^2$.
% \begin{align}
%     \Gamma_2^{\nu} = \left\{ (\wone,\wtwo) 
%     \subjto
%     \frac{ \innerprod{\wtwo}{H}^2 }{ n } \geq \fstar - \constconc + \tconstnu \nu^2 \andtxts \norm{ \wtwo }_1 \leq \loneboundclas \andtxts \norm{ \wtwo }_2 \leq \frac{B_{\eta,2}}{\sqrt{ \log (d/n) }}  \right\}
% \end{align}

% Analogously to equation \eqref{s_condition_nu_first_reduction} we derive new condition for $\uls$ as:
% \begin{align}
%     \norm{ \tildewtwo }_2^2 = \frac{ \norm{ \gamma ( \alphauls ) }_2^2 }{ \alphauls^2 } > \frac{ B_{\eta,2}^2 }{ B^2 \log (d/n) }
% \end{align}
% which is again satisfied for some $\uls = \lambda_{\uls} n$ with $ \lambda_{\uls} > 0 $. Hence from \eqref{nu_bound_first_reduction} we obtain bound:
% \begin{align}
%     \deltanu^2 
%     \leq
%     \frac{ B^2 }{ n \tconstnu } \frac{ \norm{H}_{\infty}^2 }{ \alphauls^2 } - \frac{\fstar - \constconc }{\tconstnu}
%     \leq 
%     \frac{ \fstar }{ \tconstnu \tnstar^2 } \left( 1 + \frac{4}{\tuls^2} \right) - \frac{\fstar - \constconc }{\tconstnu}
%     \leq 
%     \left( \frac{ B_{\nu,2} }{ \sqrt{\log (d/n)} } \right)^2
% \end{align}
% which concludes the proof.















% \subsection{Proof of Lemma~}


% \begin{lemma}
%     There exist universal constant $B_{\nu,3} > 0, B_{\eta,3} > 0$ such that for any element $(\wone,\wtwo)$ of $\Gamma_0$ we have that $\deltanu^2 \leq \frac{B_{\nu,3}^2}{ \left( \log \left( d/n \right) \right)^{3/2} }$ and $ \eta^2 \leq \frac{B_{\eta,3}^2}{ \log \left( d/n \right) }$ with probability at least $ 1 - $ over the draws of $..$.
% \end{lemma}

% \begin{proof}
% In this part of the proof we use Taylor series approximation of function $f$:
% \begin{align}
%     f ( \nu, \eta ) = \fstar + \frac{1}{2}\feestar \eta^2 + \frac{1}{2}\fnstar \deltanu^2 + \underbrace{O \left( \frac{1}{ \log (d/n)^{3/2} } \right)}_{\OOOc}
% \end{align}
% where we bound higher terms by results from lemma \ref{lemma_second_reduction}.
% \end{proof}
% Now we proceed in the same manner as in the previous two steps. We relax constraint from definition of $\Gamma_0$ and define the following set:
% \begin{align}
%     \Gamma_3^{\eta} = \left\{ (\wone,\wtwo) \subjto \frac{ \innerprod{\wtwo}{H}^2 }{ n } \geq \fstar - \constconc - \OOOc + \frac{1}{2}\feestar \eta^2  \andtxts \norm{ \wtwo }_1 \leq \loneboundclas  \right\}
% \end{align}
% \begin{align}
%     \left( \fstar - \constconc - \OOOc \right) \frac{ \alpha_s^2 }{ \norm{H}_{\infty}^2 } \frac{ n }{ B^2 } + \frac{1}{2} \feestar n \frac{ \norm{ \gamma (\alpha_s) }_2^2 }{ \norm{H}_{\infty}^2 } > 1
% \end{align}
% \begin{lemma}
%     Let any fixed constant $ 0 < \lambda \leq ( \log (c_2) )^{1/4} $ where by assumption $d\geq n c_2$ and let $\uls$ be the largest integer $s$ such that $t_s^2 \geq \tnstar^2 + \frac{\lambda}{\sqrt{\tnstar}}$. Then
%     \begin{align}
%         \uls = \nstar \exp \left( -\frac{ \lambda }{ 2 \sqrt{\tnstar} } \right) \left( 1 + O \left( \frac{1}{\tnstar^2} \right) \right)
%         \andtxts
%         \left| \tuls^2 - \left( \tnstar^2 + \frac{\lambda}{\sqrt{\tnstar}} \right) \right| \leq O \left( \frac{1}{n} \right)
%     \end{align}
%     Moreover, let $\ols$ be the smallest integer $s$ such that $t_s^2 \leq \tnstar^2 - \frac{\lambda}{\sqrt{\tnstar}}$. Then
%     \begin{align}
%         \ols = \nstar \exp \left( \frac{ \lambda }{ 2 \sqrt{\tnstar} } \right) \left( 1 + O \left( \frac{1}{\tnstar^2} \right) \right)
%         \andtxts
%         \left| \tols^2 - \left( \tnstar^2 - \frac{\lambda}{\sqrt{\tnstar}} \right) \right| \leq O \left( \frac{1}{n} \right)
%     \end{align}
% \end{lemma}
% Proof follows the same steps as in Claim 7 in \cite{wang2021tight}. From these results follows:
% \begin{align}
%     \frac{\tnstar^2}{\tuls^2} 
%     =
%     \frac{1}{1 + \frac{\lambda}{\tnstar^2\sqrt{\tnstar}} + O \left( \frac{1}{\tnstar^2 \nstar} \right)}
%     =
%     1 - \frac{\lambda}{\tnstar^2\sqrt{\tnstar}} + O \left( \frac{1}{\tnstar^2 \nstar} \right) + O \left( \frac{\lambda^2}{\tnstar^5} \right)
% \end{align}
% Then for $ \constconc + \OOOc = O \left( \frac{1}{\tnstar^3} \right)$ we have
% \begin{align}
%     \left( \fstar -\constconc - \OOOc \right) \frac{ \alphauls^2 }{ \norm{H}_{\infty}^2 } \frac{ n }{ B^2 } \geq &
%     \fstar \left( 1 + O \left( \frac{1}{\tnstar^3} \right) \right) \frac{1}{\tuls^2}\left( 1 - \frac{4}{\tuls^2} + O \left( \frac{1}{\tuls^4} \right) \right)\frac{n \tnstar^2}{n\fstar} \left( 1 + \frac{2}{\tnstar^2} + O \left( \frac{1}{\tnstar^3} \right) \right)\\
%     \geq &
%     \left( 1 + O \left( \frac{1}{\tnstar^3} \right) \right) \left( 1 - \frac{\lambda}{\tnstar^2\sqrt{\tnstar}} + O \left( \frac{1}{\tnstar^2 \nstar} \right) + O \left( \frac{\lambda^2}{\tnstar^5} \right) \right) \left( 1 - \frac{2}{\tnstar^2} + O \left( \frac{1}{\tnstar^3} \right) \right)
% \end{align}
% \begin{align}
%     \frac{1}{2} \feestar n \frac{ \norm{ \gamma (\alphauls) }_2^2 }{ \norm{H}_{\infty}^2 } 
%     \geq &
%     \nstar \frac{2}{\uls \tuls^2} \left( 1 + O \left( \frac{1}{\tuls^2} \right) \right)\\
%     \geq &
%     \frac{2}{\tnstar^2} \exp \left( \frac{\lambda}{2\sqrt{\tnstar}} \right)  \left( 1 + O \left( \frac{1}{\tnstar^2} \right) \right) \\
%     \geq &
%     \frac{2}{\tnstar^2} \left( 1 + \frac{\lambda}{2\sqrt{\tnstar}} + \frac{\lambda^2}{4\tnstar} + O \left( \frac{\lambda^3}{\tnstar\sqrt{\tnstar}} \right) \right) \left( 1 + O \left( \frac{1}{\tnstar^2} \right) \right) 
% \end{align}
% Hence we have:
% \begin{align}
%     \left( \fstar - \constconc - \OOOc \right) \frac{ \alphauls^2 }{ \norm{H}_{\infty}^2 } \frac{ n }{ B^2 } + \frac{1}{2} \feestar n \frac{ \norm{ \gamma (\alphauls) }_2^2 }{ \norm{H}_{\infty}^2 } 
%     >
%     1 + \frac{\lambda^2}{2\tnstar^3} + O \left( \frac{1}{\tnstar^3} \right) + O (...)
% \end{align}

% Hence we can bound $\eta^2$ as follows:
% \begin{align} \label{eq:eta_bound_third_reduction}
%     \eta^2 
%     \leq
%     B^2 \frac{ \norm { \gamma ( \alphauls ) }_2^2 }{ \norm { \gamma ( \alphauls ) }_1^2 } 
%     & \leq
%     \frac{ n \fstar }{ \tnstar^2 } \frac{2}{\uls}\left( 1 + O\left( \frac{1}{\tnstar^2} \right) \right)
%     \leq
%     \frac{4\fstar}{\feestar} \frac{1}{\tnstar^2}  \exp \left( \frac{\lambda}{2\sqrt{\tnstar}} \right) \left( 1 + O\left( \frac{1}{\tnstar^2} \right) \right) \\
%     & \leq
%     \frac{4\fstar}{\feestar} \frac{1}{\tnstar^2} \left( 1 + \frac{\lambda}{2\sqrt{\tnstar}} + O \left( \frac{1}{\tnstar} \right) \right) =: B_{\eta,3}^2
% \end{align}
% and similarly we get:
% \begin{align}
%     \eta^2 
%     \geq
%     B^2 \frac{ \norm { \gamma ( \alphaols ) }_2^2 }{ \norm { \gamma ( \alphaols ) }_1^2 } 
%     \geq
%     \frac{4\fstar}{\feestar} \frac{1}{\tnstar^2} \left( 1 - \frac{\lambda}{2\sqrt{\tnstar}} + O \left( \frac{1}{\tnstar} \right) \right) 
% \end{align}
% Now let
% \begin{align}
%     \Gamma_3^{\nu} = \left\{ (\wone,\wtwo) 
%     \subjto
%     \frac{ \innerprod{\wtwo}{H}^2 }{ n } \geq \fstar - \constconc - \OOOc + \frac{1}{2}\feestar \eta^2 + \frac{1}{2}\fnstar \deltanu^2
%     \andtxts 
%     \norm{ \wtwo }_1 \leq \loneboundclas 
%     \andtxts
%     \norm{ \wtwo }_2 \leq B_{\eta,3}  \right\}
% \end{align}
% \begin{align}\label{s_condition_nu_third_reduction}
%     \norm{ \tildewtwo }_2^2 = B^2 \frac{ \norm{ \gamma ( \alphauls ) }_2^2 }{ \alphauls^2 } > B_{\eta,3}^2 
% \end{align}
% Using concentration result from lemma \ref{lemma_gamma_conc} and expression \eqref{phidn_bound} we get the condition:
% \begin{align}
%     \frac{2}{\uls} \left( 1 + O\left( \frac{1}{\tuls^2} \right) \right) 
%     >
%     \frac{4\fstar}{\feestar} \frac{1}{\tnstar^2} \left( 1 + \frac{\lambda}{2\sqrt{\tnstar}} + O \left( \frac{1}{\tnstar} \right) \right) \frac{\tnstar^2}{ n \fstar } \left( 1 + \frac{2}{\tnstar^2} + O \left( \frac{1}{\tnstar^3} \right) \right)
% \end{align}
% then
% \begin{align}
%     \frac{2}{\uls} \left( 1 + O \left( \frac{1}{\tuls^2} \right) \right) > \frac{4}{\feestar} \frac{1}{n} \left( 1 + \frac{\lambda}{2\sqrt{\tnstar}} + O \left( \frac{1}{\tnstar} \right) \right)
% \end{align}
% Hence let $\uls = \nstar \exp \left( -\frac{\lambda}{2\sqrt{\tnstar}} \right)$. %\frac{n\feestar}{2} \left( 1 - \frac{\lambda}{\sqrt{\tnstar}} + O \left( \frac{1}{\tnstar} \right) \right)$.  
% \begin{align}
%     \deltanu^2 
%     &\leq
%     \frac{ 2B^2 }{ n \fnstar } \frac{ \norm{H}_{\infty}^2 }{ \alphauls^2 } - \frac{2\fstar}{\fnstar} \left( 1 - \constconc - \OOOc \right) - \frac{\feestar}{\fnstar} \frac{ \norm{ \gamma(\alphaols) }_2^2 }{ \alphaols^2 }B^2\\
%     &\leq 
%     \frac{2}{n\fnstar} \frac{n\fstar}{\tnstar^2} \left(1-\frac{2}{\tnstar^2}+O \left( \frac{1}{\tnstar^3} \right) \right) \tuls^2 \left( 1 + \frac{4}{\tuls^2} + O \left( \frac{1}{\tuls^4} \right) \right)
%     - \frac{2\fstar}{\fnstar} \left( 1 + O \left( \frac{1}{\tnstar^3} \right) \right)
%     \\
%      & - \frac{\feestar}{\fnstar} \frac{2}{\nstar} \exp \left( -\frac{\lambda}{2\sqrt{\tnstar}} \right) \left( 1 + O \left( \frac{1}{\tnstar^2} \right) \right) \frac{n\fstar}{\tnstar^2}  \left( 1 - \frac{2}{\tnstar^2} + O \left( \frac{1}{\tnstar^3} \right) \right)
%      \\
%      &\leq \frac{2\fstar}{\fnstar} \left( 1 + \frac{2}{\tnstar^2} + \frac{\lambda}{\tnstar^{5/2}} + O \left( \frac{1}{\tnstar^3} \right) \right) 
%      - \frac{2\fstar}{\fnstar} \left( 1 + O \left( \frac{1}{\tnstar^3} \right) \right)
%      -\frac{2\fstar}{\fnstar}\left( \frac{2}{\tnstar^2} - \frac{\lambda}{\tnstar^{5/2}} + O \left( \frac{1}{\tnstar^3} \right) \right)
%      \\
%      & \leq \frac{4 \fstar \lambda}{\fnstar}\frac{1}{\tnstar^{5/2}} \left( 1 + O \left( \frac{1}{\sqrt{\tnstar}} \right) \right)
% \end{align}







==> ICML 22-3/sections_proof/3_bound_phiN.tex <==

% \subsection{Proof of Proposition~\ref{prop:Rbound}: $l_1$ bound}
% \label{apx:subsec:probRbound}





% Recall that $\phidn$ is given by:
% \begin{align}
%     \phidn &= \min_{\nu,b,\alpha} \nu + b \norm{ \gamma \left( \alpha \right) }_1 
%     \subjto \frac{ b^2\norm{\Hgaussian}_{\infty}^2 }{n} \geq \fn \left( \nu, b \norm{ \gamma \left( \alpha \right) }_2 \right)
% \end{align}

% Given that $(\tnu,\tb,\talpha)$ is a feasible point of $\phidn$ we have that $\phidn \leq  \tnu + \tb \norm{ \gamma( \talpha) }_1$, which gives us an upper bound on $\phidn$. In the following discussion our goal is to find a single feasible point of the constraint set of $\phidn$.

% From definition of $\gamma ( \alpha )$ we know that $ \norm{ \gamma ( \alpha ) }_1 = \alpha$ and hence we can equivalently formulate $\phidn$ as an optimization over $\nu$ and $ b_{\alpha} := b \alpha $
% \begin{align}
%     \phidn &= \min_{ \nu, b_{\alpha} } \nu + b_{\alpha}
%     \subjto \frac{ b_{\alpha}^2 \norm{\Hgaussian}_{\infty}^2 }{n \alpha^2} \geq \fn \left( \nu, b_{\alpha} \frac{ \norm{ \gamma \left( \alpha \right) }_2}{ \alpha } \right)
% \end{align}

% Define $\fstar = f \left( \nustar, 0 \right)$, $\feestar = \frac{\partial^2 f(\nuopt,\eta)}{\partial \eta^2}\Big|_{\eta=0}$ and $\nstar = \frac{1}{2}\feestar n$. Now using lemma \ref{lemma_point_conv} with $ t = \fstar \tnstar^{-3} $ and for a feasible point $( \nu, b_{\alpha} \frac{ \norm{ \gamma \left( \alpha \right) }_2}{ \alpha } )$ we have that:
% \begin{align} \label{eq:constraint_f_conc}
%     \frac{ b_{\alpha}^2 \norm{\Hgaussian}_{\infty}^2 }{n \alpha^2} 
%     \geq
%     f \left( \nu, b_{\alpha} \frac{ \norm{ \gamma \left( \alpha \right) }_2}{ \alpha } \right) + \frac{\fstar}{\tnstar^{3}}
% \end{align}
% with probability at least $ 1 - 2 \exp \left( -c \frac{ n }{ \tnstar^6 \left( \nu^2 + b_{\alpha}^2  \norm{ \gamma \left( \alpha \right) }_2^2 / \alpha^2 \right) } \right) $.
% % > 1 - 2 \exp \left( - \tc \frac{ n }{ \log^3 \left( \frac{d}{n} \right)  } \right) $.

% Let's now choose $ \nu = \nustar $ and show that there exist a pair $ ( b, \alpha )$  such that $ ( \nustar, b, \alpha) $ is feasible for constraint \eqref{eq:constraint_f_conc}. Furthermore, we propose to search for a point with parameter $ ( b, \alpha ) $ such that $ b \norm{ \gamma ( \alpha )}_2 = b_{\alpha} \frac{ \norm{ \gamma \left( \alpha \right) }_2}{ \alpha } $ is near zero. Hence, using Taylor series approximation of function $ f ( \nustar, \cdot ) : \eta \mapsto f (\nustar, \eta) $ around point $(\nuopt,0)$ we can rewrite constraint \eqref{eq:constraint_f_conc} as:
% \begin{align}
%      \frac{ b_{\alpha}^2 \norm{\Hgaussian}_{\infty}^2 }{n \alpha^2}   
%      \geq
%       \fstar + \frac{1}{2}\feestar b_{\alpha}^2 \frac{ \norm{ \gamma \left( \alpha \right) }_2^2}{ \alpha^2 } + \OOO \left( b_{\alpha}^3 \frac{ \norm{ \gamma \left( \alpha \right) }_2^3}{ \alpha^3 } \right) + \frac{\fstar}{\tnstar^{3}}
% \end{align}
% since $\feta = \frac{\partial f(\nuopt,\eta)}{\partial \eta}\Big|_{\eta=0} = 0$.

% Now from \cite{wang2021tight} we know that $ \gamma ( \alpha ) $ is a piecewise linear function with breakpoints at $ \alpha_s $ for $ s = 2, \dots, d $. Hence instead of optimizing over $\alpha$ we optimize over $s$. Note that we have only one constraint but two free variables $ ( b, \alpha ) $ and so we can set $ \alpha = \alpha_{\nstar} $ with $ \nstar = \frac{1}{2}\feestar n $. We explain this choice of $s$ in the remark after the proof. Combining all these results we get constraint:
% \begin{align} \label{eq:B_ineq}
%      \frac{ b_{\alpha_{\nstar}}^2 \norm{\Hgaussian}_{\infty}^2 }{n \alpha_{\nstar}^2}   
%      \geq
%       \fstar + \frac{1}{2}\feestar b_{\alpha_{\nstar}}^2 \frac{ \norm{ \gamma \left( \alpha_{\nstar} \right) }_2^2}{ \alpha_{\nstar}^2 } + \OOO \left( b_{\alpha_{\nstar}}^3 \frac{ \norm{ \gamma \left( \alpha_{\nstar} \right) }_2^3}{ \alpha_{\nstar}^3 } \right) + \frac{\fstar}{\tnstar^{3}}
% \end{align}

% Now we claim that
% \begin{equation}
%     b_{\alpha_{\nstar}}^2 = \frac{ n \alpha_{\nstar}^2 }{ \norm{\Hgaussian}_2^2 } \frac{ \fstar \left( 1 + \frac{1}{\tnstar^{3}} \right) }{ 1 - \frac{1}{2} n \feestar \frac{ \norm{ \gamma \left( \alpha_{\nstar} \right) }_2^2 }{ \norm{H}_{\infty}^2 } - \OOO \left( \frac{1}{\tnstar^3} \right) }
% \end{equation}
% satisfies inequality \eqref{eq:B_ineq} with probability at least $ 1 - 6 \exp \left( -\frac{\nstar}{\log(d/\nstar)^5} \right)$. Using lemma \ref{lemma_gamma_conc} we have that:
% \begin{equation}
%     1 - \frac{1}{2} n \feestar \frac{ \norm{ \gamma \left( \alpha_{\nstar} \right) }_2^2 }{ \norm{H}_{\infty}^2 } - \OOO \left( \frac{1}{\tnstar^3} \right) > 1 - \frac{1}{2} n \feestar  \frac{2}{\nstar \tnstar^2} - \OOO \left( \frac{1}{\tnstar^3} \right) = 1 - \frac{2}{\tnstar^2} - \OOO \left( \frac{1}{\tnstar^3} \right)  > 0
% \end{equation}
% holding for $d,n$ sufficiently large. Applying lemma \ref{lemma_gamma_conc} once again we get:
% \begin{equation}
%     b_{\alpha_{\nstar}}^2 
%     \leq
%     \frac{ n \fstar }{ \tnstar^2 } \left( 1 + \frac{1}{\tnstar^3} \right) \left( 1 - \frac{4}{\tnstar^2} + \frac{c}{\tnstar^4} \right) \frac{1}{ 1 - \frac{2}{\tnstar^2} - \OOO \left( \frac{1}{\tnstar^3} \right)}
%     \leq
%     \frac{ n \fstar }{ \tnstar^2 } \left( 1 - \frac{2}{\tnstar^2} + \frac{c}{\tnstar^3} \right)
% \end{equation}

% Hence we have that $ \OOO \left( b_{\alpha_{\nstar}}^3 \frac{ \norm{ \gamma \left( \alpha_{\nstar} \right) }_2^3}{ \alpha_{\nstar}^3 } \right) = \OOO \left( \frac{1}{\tnstar^3} \right)$ and this $b_{\alpha_{\nstar}}^2$ indeed satisfies equation \ref{eq:B_ineq}. Now we define the upper bound on $\phidn$ as:
% \begin{align}
%     \lonebound := \sqrt{ \frac{ n \fstar }{ \tnstar^2 } \left( 1 - \frac{2}{\tnstar^2} + \frac{c}{\tnstar^3} \right) }
% \end{align}
% which holds with probability at least $ 1 - 2 \exp \left( -c \frac{ n }{ \tnstar^6 \left( \nustar^2 + b_{\alpha_{\nstar}}^2  \norm{ \gamma \left( \alpha_{\nstar} \right) }_2^2 / \alpha_{\nstar}^2 \right) } \right) - 6 \exp \left( -\frac{\nstar}{\log(d/\nstar)^5} \right) $. The proposition is proved after noting that $ \nustar^2 + b_{\alpha_{\nstar}}^2  \norm{ \gamma \left( \alpha_{\nstar} \right) }_2^2 / \alpha_{\nstar}^2 = \OOO(1)$.


==> ICML 22-3/sections_proof/3_thm2.tex <==






\section{Proof of Theorem~\ref{thm:classificationlp}}
\label{apx:claslpproof}


Since $\RiskC(\what) = 2 -2\frac{\langle \what, \wgt \rangle}{\norm{\what}_2}$, in order to obtain a valid upper bound for $\RiskC(\what)$, it is sufficient to lower bound $\frac{\langle \what, \wgt \rangle}{\norm{\what}_2}$.
The proof of the theorem is again divided into several steps and has essentially the same structure as the proof of Theorem~\ref{thm:regressionlpmain}.
Let again $\Xs = \{\xsui\}_{i=1}^n$ be the features containing the support of $\wgt$ (i.e., the first entries of $\xui$).

Define the set $\setSdelta:= \{ (\wone,\wtwo) : \abs{\innerprod{\wone}{\wgtp}} \geq \delta \}$ with small $\delta>0$. 
The proof consists of two major parts: 


\begin{enumerate}
    \item \emph{Localization.}
    We derive a  high-probability upper bound $\loneboundclas$ (Proposition~\ref{prop:phiuppercla}), which only depends on $\xi$ and $\Xs$, on the norm of the max-$\ell_p$-margin interpolator $\what$ ,
    by finding $\loneboundclas>0$ such that
    \begin{align} \label{eq:Phi_N} 
       \PhiCN :=  \|\hat{w}\|_p^p = \min_{\substack{ \forall i:\:y_i \langle \xui, w \rangle \geq 1 \\
             w \in \setSdelta} } & \norm{w}_p^p
        ~
        \leq \loneboundclas.
\end{align}

    
    \item \emph{Uniform convergence.}
    Conditioning on $\xi$ and $\Xs$, 
    we derive high-probability uniform upper bound  on the classification error for all interpolators $w$ with  $\norm{w}_p^p \leq \loneboundclas$.
    More precisely, we find a high-probability lower bound (Proposition~\ref{prop:unifconvcla}) for
    \begin{align} %\label{eq:Phi_+} 
      \label{eq:Phi_-} 
       \PhiCm := \min_{\substack{
            % \norm{w}_p^p \leq \loneboundclas \\ % CONVENTION 1
            \norm{w}_p^p \leq \loneboundclas \\ % CONVENTION 2
             \forall i:\:y_i \langle \xui, w \rangle \geq 1\\
             w \in \setSdelta}
        } & \frac{\langle w, \wgt\rangle}{\norm{w}_2}
        ,
    \end{align}
    which in turn then gives us a high probability upper bound for the classification error using that $\RiskC(\what) = 2 -2\frac{\langle \what, \wgt \rangle}{\norm{\what}_2}$. 
\end{enumerate}


\begin{remark}
The constraint $(\wone,\wtwo)\in \setSdelta$ in the definitions of $\PhiCN, \PhiCm$ is needed to ensure that the optimization objective $\frac{\langle \wone, \wgtp \rangle }{\sqrt{\norm{\wone}_2^2+\norm{\wtwo}_2^2}} $ is continuous. Since we can choose $\delta$ arbitrarily small, we can neglect the constraint $w \in \setSdelta$ as long as, with high probability, the set of feasible points satisfying the other constraints in $\PhiCN, \PhiCm$ does not contain an open ball around $(0,0)$. 
\end{remark}





\subsection{Application of the (C)GMT}
\label{apx:subsec:gmtclas}

% While Theorem~\ref{thm:classificationlp} only gives an upper bound for the classification error, and thus lower bounding $\PhiCm$ is sufficient, we rem
While we only need bounds for $\PhiCN$ and $\PhiCm$ for the proof of Theorem~\ref{thm:classificationlp}, for completeness of the following Proposition~\ref{prop:CGMT_application_classification}, we also define
\begin{align}
       \max_{\substack{
            % \norm{w}_p^p \leq \loneboundclas \\ % CONVENTION 1
            \norm{w}_p^p \leq \loneboundclas \\ % CONVENTION 2
             \forall i:\:y_i \langle \xui, w \rangle \geq 1\\
             w \in \setSdelta}
        } & \frac{\langle w, \wgt \rangle}{\norm{w}_2} 
        =: \PhiCp 
\end{align}
and the function $\fnclas : \RR^{s}\times\RR_+ \to \RR_+$, 
    \begin{align}\label{eq:fnclas_def}
    \fnclas(\wone,\norm{\wtwo}_2) = \frac{1}{n} \sumin \possq{1-\xi_i\sgn(\langle  \xsui,\wgtp \rangle) \langle \xsui, \wone\rangle -\Ggaussian_i \norm{\wtwo}_2}, 
    \end{align}
     with  $\Ggaussian \sim \NNN(0,I_n)$. 
Using the same notation as for the regression setting (Proposition~\ref{prop:CGMT_applicationreg}), and by following a standard argument relying on the Lagrange multiplier, we can bring $\PhiCN,\PhiCp$ and $\PhiCm$ in a suitable form to apply the (C)GMT (see e.g. \cite{deng21} for a similar application), we have
\begin{proposition}
% \begin{proposition} 
\label{prop:CGMT_application_classification}
    % Denote $\loneboundclasp = \loneboundclas + \norm{w^*}_p^p$. % CONVENTION 1
    %Denote $\loneboundclasp =  \loneboundclas + 2\norm{w^*}_p^p$. % CONVENTION 2
    Let $p \geq 1$ be some constant and assume that $\wgt$ is s-sparse. 
   Further, let $\Hgaussian \sim \NNN(0,I_{d-s})$ and let $\delta>0$ be an arbitrary constant. Define the stochastic auxiliary optimization problems:\footnote{We define $\PhiCN,\PhiCm,\PhiCdn,\PhiCdm = \infty$ and $\PhiCp,\PhiCdp = -\infty$ if the corresponding optimization problems have no feasible solution.}
        \begin{align}
         \label{eq:phinreg}
            \PhiCdn &= \min_{(\wone,\wtwo)} \norm{\wone}_p^p+\norm{\wtwo}_p^p
            \subjto \frac{1}{n} \innerprod{\wtwo}{\Hgaussian}^2 \geq  \fnclas(\wone,\|\wtwo\|_2) \\
         \label{eq:phipreg}
            \PhiCdp &= \max_{(\wone,\wtwo)\in \setSdelta} \frac{\langle \wone, \wgtp \rangle }{\sqrt{\norm{\wone}_2^2+\norm{\wtwo}_2^2}} 
            \subjto \begin{cases}
                \frac{1}{n} \innerprod{\wtwo}{\Hgaussian}^2 \geq  \fnclas(\wone,\|\wtwo\|_2)\\
              \norm{\wone}_p^p+\norm{\wtwo}_p^p \leq \loneboundclas
            \end{cases}\\
        \label{eq:phimreg}
            \PhiCdm &= \min_{(\wone,\wtwo)\in \setSdelta} \frac{\langle \wone, \wgtp \rangle }{\sqrt{\norm{\wone}_2^2+\norm{\wtwo}_2^2}}  
            \subjto \begin{cases}
               \frac{1}{n} \innerprod{\wtwo}{\Hgaussian}^2 \geq  \fnclas(\wone,\|\wtwo\|_2) \\
               \norm{\wone}_p^p+\norm{\wtwo}_p^p  \leq \loneboundclas
            \end{cases}
        \end{align}
    where $\loneboundclas>0$ is a constant possibly depending on $\xi$ and $\Xs$. Then for any $t \in \RR$,  we have:
        \begin{align}
            \PP( \PhiCN > t \vert \xi, \Xs) &\leq 2\PP( \PhiCdn \geq t \vert \xi, \Xs)
             \\
            \PP( \PhiCp > t \vert \xi, \Xs) &\leq 2\PP( \PhiCdp \geq t \vert \xi, \Xs) 
             \\
            \PP( \PhiCm < t \vert \xi, \Xs) &\leq 2\PP( \PhiCdm \leq t \vert \xi, \Xs) ,
        \end{align}
        where the probabilities on the LHS and RHS are over the draws of $X''$ and of $\Ggaussian,\Hgaussian$, respectively.
\end{proposition}   

The proof of the proposition is presented in Appendix \ref{apx:subsec:cgmtproof}. \\







% \begin{proof}
% % \subsection{Proof of Proposition~\ref{prop:CGMT_application_classification}: CGMT}
% % \label{apx:subsec:cgmtproof}
% % \red{Stefan, can you take care of this one? not yet worked on this}
% % Proof of this proposition is based on (Convex) Gaussian Minimax Theorem \cite{gordon1988milman,thrampoulidis2015regularized} which relates auxiliary optimization $\PhiCdn$, $\PhiCdp$ and $\PhiCdm$ with vector random variables with $\PhiCN$, $\PhiCp$ and $\PhiCm$ depending on random matrix $\matX$. 
% We follow similar proof strategy as in \cite{koehler2021uniform} with a few modifications which we describe next. First we introduce a result from the literature

% \begin{lemma}[Theorem 9 in \cite{koehler2021uniform}]
% \label{lemma:CGMT_variant}
% Let $\matX'' \in \RR^{n\times {d-s}}$ be a matrix with i.i.d. $\NNN(0,1)$ entries and let $\Ggaussian \sim \NNN(0,I_n)$ and $\Hgaussian \sim \NNN(0,I_{d-s})$ independent of $\matX$ and each other. Let $\compactw \subset \RR^{s}\times \RR^{d-s}$ and $\compactv \subset \RR^{n}$ be compact and convex sets, and let $\psi: \compactw \times \compactv \to \RR$ be continuous convex-concave function. Then for the following two optimization problems:
%     \begin{equation}
%         \Phi = \min_{(\wone,\wtwo)\in \compactw}\max_{v\in \compactv} \innerprod{v}{\matX'' \wtwo} + \psifcn((\wone,\wtwo),v)
%     \end{equation}
%     \begin{equation}
%         \phi = \min_{(\wone,\wtwo)\in \compactw}\max_{v \in \compactv} \norm{\wtwo}_2\innerprod{G}{v} + \norm{v}_2\innerprod{H}{\wtwo}+\psifcn((\wone,\wtwo),v)
%     \end{equation}
%     and any $t\in\RR$ holds that:
%     \begin{equation}
%         \prob(\Phi>t)\leq 2\prob(\phi\geq t) 
%     \end{equation}
%     where the probabilities on the LHS and RHS are over the draws of $\matX''$, and of $G$, $H$, respectively
% \end{lemma}
% % The proof of this theorem follows from Theorem 10 in \cite{koehler2021uniform} and proof of CGMT as discussed in Theorem 3 in \cite{thrampoulidis2015regularized}.

% Let's start by rewriting $\PhiCN$ using the Lagrange multipliers $\lmult_i$ to obtain:
% \begin{align}
%     \PhiCN 
%     % = \min_{w} \max_{\lmult\geq 0} \norm{w}_p^p + \sumin \lmult_i                 (1-y_i\innerprod{x_i}{w})
%       &= \min_{w} \max_{\lmult\geq 0} \norm{w}_p^p + \transp{\lmult}\onevec - \transp{\lmult}\matDy\matX w\\
% % \end{align}
% % Rewriting this optimization problem in terms of $\wone$ and $\wtwo$ we get:
% % \begin{align}
% %     \PhiCN = \min_{(\wone,\wtwo)} \max_{\lmult\geq 0} \norm{\wone}_p^p + \norm{\wtwo}_p^p + \transp{\lmult}\onevec - \transp{\lmult}\matDy\matX'' \wone- \transp{\lmult}\matDy\matX'' \wtwo
% % \end{align}
% % \begin{align}
%     &= \min_{(\wone,\wtwo)} \max_{\lmult\geq 0} \norm{\wone}_p^p + \norm{\wtwo}_p^p + \transp{\lmult}\onevec - \transp{\lmult}\matDy\matXs \wone- \transp{\lmult}\matDy\matXsc \wtwo
% \end{align}
% where $\matXsc$ is the sub-matrix of the last $d-s$ columns of $X$.
% Now note that $\matDy\matX \in \RR^{n\times d}$ has i.i.d. entries distributed according to standard normal distribution. Also, the function $\psi((\wone,\wtwo),\lmult) = \norm{\wone}_p^p - \transp{\lmult}(\matDy \matXs \wone - \onevec)$ is a convex-concave function on the whole domain. For now let's not worry about compactness of the sets over which we optimize and use Lemma \ref{lemma:CGMT_variant} on $\PhiCN$ to get:
% \begin{align}
%     \PhiCdn &= \min_{(\wone,\wtwo)} \max_{\lmult\geq 0} \norm{\wone}_p^p + \norm{\wtwo}_p^p + \transp{\lmult}\onevec - \transp{\lmult}\matDy\matXs \wone- \transp{\lmult} \matDy \Ggaussian\norm{\wtwo}_2 - \norm{\transp{\lmult}\matDy}_2\transp{\Hgaussian}\wtwo\\
%     % &= \min_{(\wone,\wtwo)} \max_{\lmult\geq 0} \norm{\wone}_p^p + \norm{\wtwo}_p^p + \transp{\lmult}(\onevec - \matDy\matXs \wone- \matDy \Ggaussian\norm{\wtwo}_2) - \norm{\lmult}_2\transp{\Hgaussian}\wtwo\\
%     &= \min_{(\wone,\wtwo)} \max_{\lmult\geq 0} \norm{\wone}_p^p + \norm{\wtwo}_p^p - \norm{\lmult}_2\left(\innerprod{\wtwo}{\Hgaussian}-\norm{\pos{\onevec - \matDy\matXs \wone- \matDy \Ggaussian\norm{\wtwo}_2}}_2 \right) \\
%     % & = \min_{(\wone,\wtwo)} \max_{\lambda\geq 0} \norm{\wone}_p^p + \norm{\wtwo}_p^p - \lambda(\innerprod{\wtwo}{\Hgaussian}-\norm{\pos{\onevec - \matDy\matXs \wone- \matDy \Ggaussian\norm{\wtwo}_2}}_2\\
%     & = \min_{(\wone,\wtwo)} \norm{\wone}_p^p + \norm{\wtwo}_p^p
%     \subjto \innerprod{\wtwo}{\Hgaussian}\geq \norm{\pos{\onevec - \matDy\matXs \wone- \matDy \Ggaussian\norm{\wtwo}_2}}_2
% \end{align}
% Now note that the RHS of the last inequality is given by:
%     \begin{align}
%     \frac{1}{n}\norm{\pos{\onevec - \matDy\matXs \wone- \matDy \Ggaussian\norm{\wtwo}_2}}_2^2 = \frac{1}{n} \sumin \possq{1-\xi_i\sgn(\langle \wgt, \xsui \rangle) \langle \xsui, \wone \rangle -\Ggaussian_i \norm{\wtwo}_2}, 
%     \end{align}
% which is exactly function $\fnclas(\wone, \norm{\wtwo}_2^2)$ as defined in equation \eqref{eq:fnclas_def}. 

% % Let's now define truncated optimization problem:
% % \begin{align}
% %         \PhiCN^r(t) = \min_{\norm{\wone}+\norm{\wtwo}\leq t} \max_{\lmult\geq 0,\norm{\lmult}\leq r} \norm{\wone}_p^p + \norm{\wtwo}_p^p + \transp{\lmult}\onevec - \transp{\lmult}\matDy\matXs \wone- \transp{\lmult}\matDy \matXsc \wtwo
% % \end{align}
% Now we discuss the problem of the compactness of the underlying optimization sets. Following similar argument as in proof of Lemma 7 in \cite{koehler2021uniform} we can define truncated optimization problems $\PhiCN^r$ and $\PhiCdn^r$ for which we can apply Lemma~\ref{lemma:CGMT_variant} and thus it holds that $\prob(\PhiCN^r>t|\xi,\Xs) \leq 2\prob(\PhiCdn^r\geq t|\xi,\Xs)$. Furthermore, following the same  limit argument as in the proof of Lemma 7 in \cite{koehler2021uniform}, we can show that for large $r$, $\prob(\PhiCN>t|\xi,\Xs) \leq \prob(\PhiCN^r>t|\xi,\Xs)$ and $\prob(\PhiCdn^r>t|\xi,\Xs)\leq \prob(\PhiCdn>t|\xi,\Xs)$. Hence, the proof for $\PhiCN$ is complete.

% % \begin{align}
% %     \PhiCdn^r(t) &= \min_{\norm{\wone}+\norm{\wtwo}\leq t} \max_{\lmult\geq 0,\norm{\lmult}\leq r} \norm{\wone}_p^p + \norm{\wtwo}_p^p + \transp{\lmult}\onevec - \transp{\lmult}\matDy\matXs \wone- \transp{\lmult} \matDy \Ggaussian\norm{\wtwo}_2 - \norm{\transp{\lmult}\matDy}_2\transp{\Hgaussian}\wtwo
% % \end{align}

% % Combining previous results we have that:
% % \begin{align}
% %     \prob(\PhiCN^r(t)>t)\leq 2\prob(\PhiCdn^r(t)\geq t) .....\lim_{r\to\infty}\prob(\PhiCdn^r(t)\geq t)\leq \prob(\PhiCdn\geq t)
% % \end{align}


% Finally, we note that the proof for $\PhiCp$ and $\PhiCm$ follows similar steps as discussed above. The result is essentially a consequence of the GMT (Theorem 10 in \cite{koehler2021uniform}) when noting that we optimize over $(\wone,\wtwo)\in \compactw$ where $\compactw$ is an $l_p$-ball of radius $M$ and hence a compact set, and by defining function $\psi$ as $\psi((\wone,\wtwo),v) = \frac{\innerprod{\wone}{\wgtp}}{\sqrt{\norm{\wone}_2^2+\norm{\wtwo}_2^2}} - \transp{v}(\matDy \matXs \wone - \onevec)$ which is clearly a continuous function. In order to have compact set $\compactv$ for optimization over $\lmult$ we can use the same truncation argument as proposed in Lemma 4 in \cite{koehler2021uniform}.
% \end{proof}
















\subsection{Localization step - bounding \texorpdfstring{$\PhiCdn$}{phiN}}

\label{apx:subsec:localisationproofcla}
Similar to proof of Theorem~\ref{thm:regressionlpmain} in Appendix~\ref{apx:subsec:localisationproofreg}, we first derive an upper bound for $\PhiCdn$, where we again assume for simplicity that $\wgt, x_i \in \RR^{d+1}$ and thus $H \in \RR^d$ (see Remark \ref{rm:simplicification}). In particular, using that $\wgt = (1,0,\cdots,0)$ we can rewrite the optimization problem defining $\PhiCdn$ in Proposition~\ref{prop:CGMT_application_classification} as:
\begin{equation}
  \PhiCdn = \min_{(\wone,\wtwo)} \vert \wone\vert^p+\norm{\wtwo}_p^p
            \subjto \frac{1}{n} \innerprod{\wtwo}{\Hgaussian}^2 \geq  \fnclas(\wone,\|\wtwo\|_2),
    \end{equation}
with  $\fnclas(\wone,\norm{\wtwo}_2) = \frac{1}{n} \sumin \possq{1-\wone \xi_i \vert \xsui\vert  -\norm{\wtwo}_2 \Ggaussian_i }$. 

Before stating the proof, we first introduce some additional notation. We define $\nu := w'$ and $\eta = \norm{\wtwo}_2$, and define
\begin{align}
\label{eq:defineg1}
    \fnstar &:= \min_{\nu} \fnclas(\nu,0) ~~\mathrm{and}~~ \nubarn := \argmin_{\nu} \fnclas(\nu,0)~~\mathrm{and}\\
     \cfnone &:= \frac{\partial^2}{\partial\nu^2}\fnclas(\nubarn,0) = \frac{2}{n}\sum_{i=1}^n \idvec[ 1- \xi_i\nubarn \abs{\gausswone_i}] (\gausswone_i)^2 ~~\mathrm{and}~~ \cfntwo := \frac{2}{n}\sum_{i=1}^n \idvec[ 1- \xi_i\nubarn \abs{\gausswone_i}].
     \label{eq:defineg2}
\end{align}
Furthermore, we define $\fclas (\nu,\eta) := \EE_{Z_1,Z_2 \sim \NNN(0,1)} \EE_{\xi \sim \prob(\cdot\vert Z_1)} \left( 1- \xi \nu \vert Z_1 \vert - \eta Z_2\right)_+^2 $ and $\nubar := \arg\min \fclas(\nu, 0)$ and define the quantities ${\fstar := \fclas(\nubar, 0)}$, $\feestar := \frac{d^2}{d^2 \eta}\vert_{(\nu, \eta) = (\nubar, 0)} \fclas(\nu,\eta)$ and $\fnnstar := \frac{d^2}{d^2 \nu}\vert_{(\nu, \eta) = (\nubar, 0)} \fclas(\nu,\eta)$, which are all non-zero positive constants independent of $n,d$ and $p$ as they only depend on $\probsigma$. Throughout the proof, we implicitly make use of the fact that, with high probability over the draws of $X'$ and $\xi$, the following lemma holds.


\begin{lemma}
\label{lm:quantconcentration}
There exists universal constants $c_1,c_2>0$ such that with probability  $\geq 1-c_1 d^{-c_2}$ over the draws of $\gausswone$ and $\xi$, we have that
\begin{align}
    \max\left(\vert \nubar - \nubarn \vert, \vert \fstar - \fnstar\vert, \vert \cfnone - \fnnstar \vert, \vert \cfntwo -\feestar \vert \right) \lesssim \left(\frac{\log d}{n}\right)^{1/4}
\end{align}
\end{lemma}

\begin{proof}
Both $\fnclas$ and $\fclas$ are convex functions with unique global minima with high probability. In particular, because of Lemma~\ref{quadratic_bound_fn} we know that $\nubarn$ is attained in a bounded domain around zero with probability $\geq 1-c_1 d^{-c_2}$. Further, by Lemma~\ref{lemma_quadratic_plus_fstar_bound} we see that, with high probability, $\vert \fnstar - \fstar \vert \lesssim \frac{\log d}{\sqrt{n}}$ and $\vert \nubar - \nubarn \vert \lesssim \frac{\log^{1/2} d}{n^{1/4}}$. 

To control the quantities $\cfnone,\cfntwo$,
note that we can use exactly the same uniform convergence argument as for Proposition~\ref{prop:unifConv} to show that the functions $\nu \mapsto  \frac{2}{n}\sum_{i=1}^n \idvec[ 1- \xi_i\nu \abs{\gausswone_i}] (\gausswone_i)^2$ and  $\nu \mapsto  \frac{2}{n}\sum_{i=1}^n \idvec[ 1- \xi_i\nu \abs{\gausswone_i}]$ also converge uniformly for any bounded domain $\nu \in [\nubar - \delta, \nubar + \delta]$ with $\delta >0$. Thus, the proof then follows from  $\nubarn \to \nubar$  and the fact that 
$h_1(\nu) = \EE_{\gausswone,\xi} 
2\idvec[ 1- \xi \nu \abs{\gausswone}] (\gausswone)^2$ and $h_2(\nu) = \EE_{\gausswone,\xi} 
2\idvec[ 1- \xi\nu \abs{\gausswone}]$ are both Lipschitz continuous functions
in the domain $[\nubar - \delta, \nubar + \delta]$ with $h_1(\nubar) = \fnnstar$, $h_2(\nubar) = \feestar$.
\end{proof}


 

The goal of this section is to show the following upper bound on $\PhiCdn$:
% \begin{proposition}
% \label{prop:phiuppercla}
%     Let the data distribution be as described in Section~\ref{subsec:clasetting} and assume that the noise model $\probsigma$ is independent of $n,d$ and $p$.
% Under the same assumptions as in Theorem~\ref{thm:classificationlp} for $n,d,p$, there exists universal constants $c_1,c_2,c_3,c_4>0$ such that with probability at least $ 1- c_1 d^{-c_2}$ over the draws of $\Ggaussian,\Hgaussian,\Xs,\xi$, it holds that
% \begin{align}
% \label{eq:upperboundlpcla}
% \PhiCdn \leq&  \left(\frac{n \fnstar}{\dmoment{q}^2}\right)^{p/2}\left(1+ \frac{p}{2} \frac{\cfnone \deltanu_0^2}{2\fnstar}\left(1 + \OOOc^{1/2} \log^{3/2} d  + O\left(
% \abs{\deltanu_0} \log^{3/2} d +  \log d \rho\right)\right) + \OOOc +O\left(  \rho^2\right) \right)\\
% &+ \nubarn^{p} + p\nubarn^{p-1}\deltanu_0(1+ O(\deltanu_0)) =: \loneboundclas,
% \end{align}
% with $\OOOc = O( \frac{ n \exp(c_3 q)}{d q } )$,  $\rho = \frac{\log^{c_4} d}{\sqrt{n}}$ and $\deltanu_0 := -\frac{ 2\nubarn^{p-1} \fnstar \dmoment{q}^p}{\cfnone \left(n \fnstar\right)^{p/2}}$.
% \end{proposition}
\begin{proposition}
\label{prop:phiuppercla}
    Let the data distribution be as described in Section~\ref{subsec:clasetting} and assume that the noise model $\probsigma$ is independent of $n,d$ and $p$.
Under the same assumptions as in Theorem~\ref{thm:classificationlp} for $n,d,p$, there exists universal constants $c_1,c_2,\cdots,c_8>0$ such that with probability at least $ 1- c_1 d^{-c_2}$ over the draws of $\Ggaussian,\Hgaussian,\Xs,\xi$, it holds that
\begin{align}
\label{eq:upperboundlpcla}
\PhiCdn \leq&  \left(\frac{n \fnstar}{\dmoment{q}^2}\right)^{p/2}\left(1+ \frac{p}{2} \frac{\cfnone \deltanu_0^2}{2\fnstar}\left(1 + \OOOc^{1/2} \log^{3/2} d  + c_6 \left(
\abs{\deltanu_0} \log^{3/2} d +  \log d \rho\right)\right) + \OOOc +c_7   \rho^2 \right)\\
&+ \nubarn^{p} + p\nubarn^{p-1}\deltanu_0(1+ c_8\deltanu_0) =: \loneboundclas,
\end{align}
with $\OOOc = c_5 \frac{ n \exp(c_3 q)}{d q } $,  $\rho = \frac{\log^{c_4} d}{\sqrt{n}}$ and $\deltanu_0 := -\frac{ 2\nubarn^{p-1} \fnstar \dmoment{q}^p}{\cfnone \left(n \fnstar\right)^{p/2}}$.
\end{proposition}
\begin{proof}
The proof essentially follows again from exactly the same argument as used in the proof of Proposition~\ref{prop:phidnhighreg}, where the goal is again to find one feasible point. We choose $\wtwo = b \wgrad = b \partial \|H\|_q$ and $\wone = \nubarn + \deltanu_0$. 
Conditioning on the event where the lower bound for $\fnclas$ in Equation~\eqref{eq:lpfn} from Lemma~\ref{lm:lpfn} holds, we obtain the following lower bound on $b$ (we choose again  $\wtwo = b \wgrad = b \partial \|H\|_q$):

\begin{align}
&\frac{1}{n} 
\innerprod{\wtwo}{\Hgaussian}^2 \geq \fnclas(\wone,\|\wtwo\|_2 ) = \fnclas(\nubarn + \deltanu_0,\|\wtwo\|_2 ) \\
\impliedby
&b^2 \frac{\norm{H}_q^2}{n} \geq  \fnstar+ ( \frac{\cfnone}{2} \deltanu_0^2+b^2 \frac{\cfntwo}{2} \|\wgrad\|_2^2)(1+c_1\rho) + c_2\rho b\|\wgrad\|_2 \\ &~~~~~+c_3(\rho + \sqrt{\log d}(\vert \deltanu_0 \vert + b\|\wgrad\|_2))^3
\\ 
\impliedby
&b^2 \geq \frac{ \fnstar + \frac{\cfnone}{2} \deltanu_0^2(1+c_1\rho) +  c_2\rho b\|\wgrad\|_2  + c_3(\rho + \sqrt{\log d}(\vert \deltanu_0\vert + b\|\wgrad\|_2))^3 }{\frac{\norm{H}_q^2}{n} - \frac{\cfntwo}{2} (1 + c_1 \rho ) \norm{\wgrad}_2^2 },\\ \label{eq:lpboundphinbclas} 
\end{align}

where we can again choose $\rho = \frac{\log^{c} d}{\sqrt{n}}$ with $c>1$ some universal constant. We can now apply the concentration inequalities for $\|H\|_q$ and $\norm{\wgrad}_2^2$ from Lemma~\ref{lm:dualnormconc} to show that 

\begin{align}
b^2 =  \frac{n \fnstar}{\dmoment{q}^2} \left(1+\frac{\cfnone \deltanu_0^2}{2\fnstar}\left(1 + \OOOc^{1/2} \log^{3/2} d + c_6\left(
\vert \deltanu_0\vert \log^{3/2} d + \log d \rho \right)  \right)  + \OOOc + c_7  \rho^2 \right)
%  + O\left(\rho^2 + \rho \sqrt{\frac{ \nu_0^2}{\sigmaxi^2} + 
% \OOOc}\right)
% \right)
\end{align}
satisfies Equation~\eqref{eq:lpboundphinbclas}. Unlike in the proof of Proposition~\ref{prop:phidnhighreg}, we used that 
\begin{align} \OOOc = O(\log^{-5} d)
 %=  O \left( \frac{ n \exp(c_5 q)}{d q } \right)=  ~\mathrm{and}~
 %\frac{\mutild  n}{\dmoment{q}^2} =  \Omega \left( \frac{ n \exp(-c_5 q)}{d q } \right) ~
 ~\mathrm{and}~
 \deltanu_0^2 = \Theta \left( \frac{q^p d^{2p-2}}{n^p} \right) = O(\log^{-5}d), \label{eq:facteq2clas}
\end{align}
which is again satisfied when applying Proposition~\ref{cor:hqbound2} and choosing  $\kappa_1,\cdots, \kappa_4 >0$ characterizing $n,d$ and $p$ in Theorem~\ref{thm:classificationlp} appropriately. Hence, we can conclude the proof.


\end{proof}



\subsection{Uniform convergence step}
\label{apx:subsec:clauniformproof}

We use the same notation as in Appendix~\ref{apx:subsec:localisationproofcla} and Appendix~\ref{apx:subsec:localisationproofreg}. 
Similarly to Appendix~\ref{apx:subsec:unfiformconvreg}, we can again relax the constraints in the optimization problem defining $\PhiCdm$ in Proposition~\ref{prop:CGMT_application_classification} by using H\"olders inequality $\langle w, \Hgaussian \rangle \leq \|w\|_p \|\Hgaussian\|_q $. Note that both problems again only depend on $\wtwo$ via $\norm{\wtwo}_2$ and $\norm{\wtwo}_p$. 
Define 
\begin{equation}
    \Gamma = \{ (\nu, \eta)\vert \exists b>0 \subjto \frac{1}{n} \norm{H}_q^2 b^2  \geq  \fnclas(\nu, \eta) ~~\mathrm{and}~~ \nu^p + b^p \leq M \}
\end{equation}. It is again straight forward to verify that 
\begin{align}
        \PhiCdm \geq \left[\min_{(\nu,\eta) \in \Gamma } \frac{\nu }{\sqrt{\nu^2+\eta^2}} 
                \right]\geq \left( 1 + \frac{\max_{(\nu,\eta) \in \Gamma}\eta^2}{\min_{(\nu,\eta) \in \Gamma}\nu^2}\right)^{-1/2},
    \end{align}
where the last inequality holds when  $\min_{\nu \in \Gamma}\nu >0$. 
The goal of this section is to prove the following proposition, from which the theorem then straightforwardly follows. 
\begin{proposition}
\label{prop:unifconvcla}
    Let the data distribution be as described in Section~\ref{subsec:clasetting} and assume that the noise model $\probsigma$ is independent of $n,d$ and $p$.
Under the same conditions as in Theorem~\ref{thm:classificationlp} for $n,d$ and $p$ and for the choice of $\loneboundclas$ as in Proposition~\ref{prop:phiuppercla},  there exists universal constants $c_1,c_2,c_3,c_4,c_5>0$ such that with probability at least $ 1- c_1 d^{-c_2}$ over the draws of $\Ggaussian,\Hgaussian,\Xs,\xi$, it holds that
\begin{align}
        \Gamma \subseteq \left\{ (\nu,\eta) \in \mathbb{R}\times \mathbb{R}_+\vert (\nu - \nubarn)^2 \lesssim  \OOOc +\deltanu_0^2 +  \rho^2  ~~\mathrm{and}   ~~
   \eta^2 \lesssim \OOOc + \deltanu_0^3 \log^{3/2} d  +\rho^2 \right\}
\end{align}
with $\OOOc = c_5 \frac{ n \exp(c_3 q)}{d q } $,  $\rho = \frac{\log^{c_4} d}{\sqrt{n}}$ and $\deltanu_0 := -\frac{ 2\nubarn^{p-1} \fnstar \dmoment{q}^p}{\cfnone \left(n \fnstar\right)^{p/2}}$.
\end{proposition}

 





\begin{proof}
The proof is very similar to the proof of the uniform convergence bound in Appendix~\ref{apx:subsec:unfiformconvreg}, and consists of iteratively bounding $\eta+ \nu$. The primary difference lies in the control of $\fnclas$, which requires more care. 


\paragraph{Step 1: $\Gamma \subset \{ (\nu,\eta)\vert \nu^2+ \eta^2 = O(1) \}$} 
A first  bound is obtained from the relaxation $b^p \leq \loneboundclas$, which implies that ${\frac{1}{n} \norm{H}_q^2 \loneboundclas^{2/p}  \geq  \fnclas(\nu, \eta)}$.

Conditioning on the event where Equation~\eqref{eq:quadratic_bound_fn} in Lemma \ref{quadratic_bound_fn} holds, we have that $\fnclas(\nu, \eta) \geq c_1 \nu^2 + c_2 \eta^2$, and thus we can relax
\begin{equation}
    \frac{\loneboundclas^{2/p}\|\Hgaussian\|_q^2}{n} \geq  c_1 \nu^2 + c_2 \eta^2
\end{equation}
We obtain the desired upper bound from the concentration of $\|\Hgaussian\|_q^2$ from Lemma~\ref{lm:dualnormconc}  and when noting that  the dominating term in $\loneboundclas$ is $ \left(\frac{n \fnstar}{\dmoment{q}^2}\right)^{p/2}$:
\begin{align}
\label{eq:bound1lpeq}
        \nu^2 + \eta^2 = O(\fnstar) = O(1). 
\end{align}


\paragraph{Step 2:  $\Gamma \subset \{ (\nu,\eta) \vert (\nu - \nubarn)^2+ \eta^2 = O(\log^{-5}d) \}$ }
Define $\deltanu := \nu -  \nubarn$.
Conditioning on Equation~\eqref{eq:bound1lpeq}, we can now repeat the same argument but using the tighter lower bound for $\fnclas$ from Equation~\eqref{eq:quadratic_plus_fstar_bound} in Lemma~\ref{lemma_quadratic_plus_fstar_bound}, where we let $\epsilon$ in Lemma~\ref{lemma_quadratic_plus_fstar_bound} be $ \frac{\log^{c} d}{\sqrt{n}} =: \rho$ with universal constant $c>1$. Thus, we obtain the high probability upper bound:
\begin{align}
    \frac{\loneboundclas^{2/p}\|\Hgaussian\|_q^2}{n} \geq \fnclas(\nu,\eta) &\geq  \fstar + \tconstnu  (\nu - \nubar)^2+ \tconsteta \eta^2 + c_1\rho 
    \\ &=  \fstar + \tconstnu  (\deltanu^2 + 2 \deltanu(\nubarn - \nubar) +  (\nubarn - \nubar)^2) + \tconsteta \eta^2 + c_1\rho,\\
    &\geq \fnstar + \tconstnu  \deltanu^2 +  \tconsteta \eta^2 + c_2 (\rho^{1/2} + \deltanu \rho^{1/2}).
    \label{eq:lpclastep2}
\end{align}
In particular, we can take the Taylor series approximation of $\loneboundclas^{2/p}$ which gives us
\begin{align}
    \loneboundclas^{2/p} =  \frac{n \fnstar}{\dmoment{q}^2} \left(1 +\OOOc + O\left(\frac{\cfnone \deltanu_0^2}{2\fnstar} +  \rho^2 + \frac{\nubarn^{p}}{ \left(\frac{n \fnstar}{\dmoment{q}^2}\right)^{p/2}} \right)\right).
\end{align}
And hence, applying again  Lemma~\ref{lm:dualnormconc} to control $\norm{H}_q^2$ as in Appendix~\ref{apx:subsec:localisationproofreg}, the bound in Equation~\eqref{eq:lpclastep2} implies 
\begin{equation}
\label{eq:bound2lpeqclas}
  \tconstnu \deltanu^2 + \tconsteta \eta^2 = \OOOc + O \left(\left(\frac{\dmoment{q}^2}{n \fnstar}\right)^{p/2} + \rho^{1/2} \right) = O\left(\log^{-5}d\right),
\end{equation}
where in the last line we used Equation~\eqref{eq:facteq2clas}. 


\paragraph{Step 3: $\Gamma \subset \{ (\nu,\eta) \vert (\nu - \nubarn)^2 \lor \eta^2 = \OOOc +O(\deltanu_0^2 +  \rho^2)$}
We are now able to derive a tighter bound 
conditioning on the event where Equation~\eqref{eq:bound2lpeqclas} holds and thus $\Gamma \in \{(\nu,\eta) \vert\ \vert \nu - \nubarn\vert^2 \lesssim \log^{-5}d  ~~\mathrm{and}~~ \eta^2 \lesssim \log^{-5}d\}$.  We can apply  Lemma~\ref{lm:lpfn}, which allows us, with high probability, to uniformly bound
\begin{equation}
   \left| \fnclas(\nu, \eta)  -  \fnstar -\deltanu^2 \frac{\cfnone}{2} - \eta^2 \frac{\cfntwo}{2} \right| \lesssim (\deltanu^2 + \eta^2) \log^{-1}d + \eta \rho + \rho^3
\end{equation}
where we choose again $\rho = \frac{\log^{c}d}{\sqrt{n}}$. 
Furthermore, we can relax the  second constraint in $\Gamma$ to
\begin{align}
    b^p &\leq \loneboundclas - (\deltanu+\nubarn)^p =  \left(\frac{n \fnstar}{\dmoment{q}^2}\right)^{p/2}\left(1+ \OOOc +c_1(\deltanu_0^2 +  \rho^2) + \frac{p\nubarn^{p-1}}{ \left(\frac{n \fnstar}{\dmoment{q}^2}\right)^{p/2}} c_2\left(\deltanu_0-\deltanu\right)\right)
    \\
    &=  \left(\frac{n \fnstar}{\dmoment{q}^2}\right)^{p/2}\left( 1+ \OOOc +c_1(\deltanu_0^2 +  \rho^2) +  c_3\left(\deltanu_0^2-\deltanu_0\deltanu\right)\right
    )\\
    &=  \left(\frac{n \fnstar}{\dmoment{q}^2}\right)^{p/2}\left(1+  \OOOc +c_4(\deltanu_0^2 +  \rho^2  + \deltanu_0\deltanu)\right)\label{eq:lpregtighter}
\end{align}
 with $\loneboundclas$ from Proposition~\ref{prop:phiuppercla} and where we used that by definition $\deltanu_0 = -\frac{ 2\nubarn^{p-1} \fnstar}{\cfnone \left(\frac{n \fnstar}{\dmoment{q}^2}\right)^{p/2}}$. 
In summary, we can again obtain an upper bound for $\eta^2$ and $\deltanu^2$ from $  \frac{1}{n} \norm{H}_q^2 b^2 \geq \fnclas(\nu,\eta)$ and when following the same argument as in Appendix~\ref{apx:subsec:localisationproofreg}. We have  
\begin{align}
     &\frac{1}{n} \norm{H}_q^2 b^2 \geq \fnclas(\nu,\eta)\\
     \implies ~~&\frac{\fnstar}{ \frac{n \fnstar}{\dmoment{q}^2}}(1+\epsilon)  \frac{n \fnstar}{\dmoment{q}^2}\left(1+  \OOOc + c_4(\deltanu_0^2 +  \rho^2  + \deltanu_0\deltanu)\right) \\
     &\geq   \fnstar + \deltanu^2 \frac{\cfnone}{2} + \eta^2 \frac{\cfntwo}{2}
     +c_5((\deltanu^2 + \eta^2) \log^{-1}d + \rho\eta + \rho^3)\\
     \implies~~&\OOOc + c_4(\deltanu_0^2 + \rho^2  + \deltanu_0\deltanu) \geq 
      \deltanu^2 \frac{\cfnone}{2} + \eta^2 \frac{\cfntwo}{2}
     +c_5((\deltanu^2 + \eta^2) \log^{-1}d + \rho\eta + \rho^3)\\
     \implies   ~~&\deltanu^2 \lor \eta^2 = \OOOc +O(\deltanu_0^2 +  \rho^2 ),
     \label{eq:lpclassstep3}
\end{align}
where we used in the second line that, with high probability, by Lemma~\ref{lm:dualnormconc}, $\frac{\norm{H}_q}{n} \leq \frac{\fnstar}{ \frac{n \fnstar}{\dmoment{q}^2}}(1 + \epsilon)$ with $\epsilon \lesssim \OOOc + \rho^2$.

% where we further implicitly used Lemma~\ref{lm:quantconcentration}. 

\paragraph{Step 4: Bound in Proposition~\ref{prop:unifconvcla}} We are now ready to prove the bounds in Proposition~\ref{prop:unifconvcla}.
We already know from the previous steps that $\deltanu \to 0$ and hence $\nu$ concentrates around $\nubarn$, which itself concentrates around $\nubar$ by Lemma~\ref{lm:quantconcentration}. However, the classification error in Theorem~\ref{thm:classificationlp} depends on the term $\frac{\eta^2}{\nu^2}$, which allows us to obtain a tighter bound when further bounding $\eta^2$. 

 Lemma~\ref{lm:lpfn} together with the previous bound on $\eta^2$ and $\deltanu^2$ implies that uniformly over all $\deltanu^2 \lor \eta^2 = \OOOc + O(\deltanu_0^2 +  \rho^2 )$, we have:
\begin{align}
    \left| \fnclas(\nu, \eta) -  \fnstar - \deltanu^2 \frac{\cfnone}{2} - \eta^2 \frac{\cfntwo}{2} \right| &\lesssim (\deltanu^2+\eta^2) \OOO_b + \rho^2  + \rho \eta,
\end{align}
where we define $\OOO_b =  c_1 \log^{3/2}d~(\sqrt{ \OOOc} +  O\left( \rho + \deltanu_0  \right))$. 

Instead of Equation~\eqref{eq:lpregtighter}, we can analogously obtain the tighter expression (using that $\deltanu = \OOO_b$)
\begin{align}
\label{eq:lptightcond2clas}
    b^p &\leq \loneboundclas - (\deltanu+\nubarn)^p \\&\leq  \left(\frac{n \fnstar}{\dmoment{q}^2}\right)^{p/2}\left(1+ \frac{p}{2} \frac{\cfnone\deltanu_0^2}{2\fnstar}(1+ \OOO_b)
    +\OOOc+ c_1 \rho^2 + \frac{p\nubarn^{p-1}}{ \left(\frac{n \fnstar}{\dmoment{q}^2}\right)^{p/2}}\left(\deltanu_0-\deltanu\right)(1+ \OOO_b)\right).
\end{align}

Therefore, applying the Taylor series approximation and Lemma~\ref{lm:dualnormconc} as in Appendix~\ref{apx:subsec:localisationproofreg}, we can upper bound 

















\begin{align}
\label{eq:lptightcond2clas2}
    \frac{1}{n} \norm{H}_q^2 b^2 &\leq   \frac{1}{n} \norm{H}_q^2  \frac{n \fnstar}{\dmoment{q}^2}\left(1+ \frac{\cfnone\deltanu_0^2}{2\fnstar} (1+\OOO_b) +
  \OOOc +   c_1 \rho^2 + 
    \frac{2\nubarn^{p-1}}{ \left(\frac{n \fnstar}{\dmoment{q}^2}\right)^{p/2}}\left(\deltanu_0-\deltanu\right)(1+ \OOO_b)\right) \\
&=
(1 + \epsilon) \fnstar\left(1+ \frac{\cfnone\deltanu_0^2}{2\fnstar} (1+\OOO_b) +
  \OOOc + c_1 \rho^2 + 
    \frac{2\nubarn^{p-1}}{ \left(\frac{n \fnstar}{\dmoment{q}^2}\right)^{p/2}}\left(\deltanu_0-\deltanu\right)(1+ \OOO_b)\right) \\
%&= \fnstar +  \frac{\cfnone\deltanu_0^2}{2} (1+\OOO_b) +
%  \OOOc + c_1\rho^2 + 
%    \cfnone(-\deltanu_0^2+\deltanu_0 \deltanu)(1+ \OOO_b) \\
&= \fnstar + \frac{\cfnone}{2} (2 \deltanu_0 \deltanu -\deltanu_0^2) (1+\OOO_b) +
   \OOOc + c_1 \rho^2 ,
   \label{eq:lpboundonb}
\end{align}
where we used the same argument as in the previous step.
As a result, we obtain the upper bound 
\begin{align}
%\label{eq:lptightcond1}
\label{eq:lptightcond2clas3}
&\frac{1}{n}b^2\norm{H}_q^2 \geq \fnclas(\nu,\eta) \\
\implies~~&
\fnstar + \frac{\cfnone}{2} (2 \deltanu_0 \deltanu -\deltanu_0^2) (1+\OOO_b) +
   \OOOc + c_1\rho^2
   \\&\geq   \fnstar + \deltanu^2 \frac{\cfnone}{2} + \eta^2 \frac{\cfntwo}{2}  + (\deltanu^2+\eta^2)  \OOO_b  +c_2\rho^2 + c_3\rho \eta\\
%   \implies ~~& 
%   \OOOc +  c_1\rho^2 \geq (\deltanu^2 + \deltanu_0^2 - 2\deltanu \deltanu_0) \frac{\cfnone}{2} (1+\OOO_b) +  \eta^2 \frac{\cfntwo}{2}  + (\deltanu^2+\eta^2)  \OOO_b  +c_2\rho^2 + c_3\rho \eta \\
%   \implies ~~& \deltanu_0^2\OOO_b +  \OOOc + c_1\rho^2 \geq 
%   \left[\frac{\cfntwo}{2}(\eta - c_2\rho))^2 +\frac{\cfnone}{2}(\deltanu - \deltanu_0)^2\right](1+  \OOO_b)\\
  \implies ~~& \deltanu_0^2\OOO_b + \OOOc + c_1\rho^2 \geq 
   \frac{\cfntwo}{2}(\eta - c_2\rho)^2 +\frac{\cfnone}{2}(\deltanu - \deltanu_0)^2.
  \end{align}

  Finally, we get the desired result from the fact that $\cfnone$ and $\cfntwo$ concentrate around $\fnnstar$ and $\feestar$ by Lemma~\ref{lm:quantconcentration}.  Hence we can conclude the proof.



\end{proof}












==> ICML 22-3/sections_proof/4_1st_reduction.tex <==
% \documentclass[appendix.tex]{subfiles}
% \begin{document}


% Recall that we defined $ \nu = \wone $ and $ \eta = \norm{ \wtwo }_1 $. Define the following set:
% \begin{align}
%     \Omega_0 = \left\{ (\wone,\wtwo) \subjto \frac{ \innerprod{\wtwo}{H}^2 }{ n } \geq \fn \left( \nu, \eta \right) \andtxts \abs{ \nu } + \norm{ \wtwo }_1 \leq \lonebound \right\}
% \end{align}

% \subsubsection{Step 1: Bounding $\nu,\eta$ by universal constants}
% \label{apx:subsec:firstReduction}

% \begin{lemma} \label{lemma_first_reduction}
%     There exist universal constant $c > 0$ such that for any element $(\wone,\wtwo)$ of $\Omega_0$ we have that $\norm{ \wone }_2 = \nu \leq \boundnu $ and $\norm{ \wtwo }_2 = \eta \leq \boundeta$ with probability at least $ 1 - $ over the draws of $..$.
% \end{lemma}

% \begin{proof}
% According to lemma \ref{quadratic_bound_fn} we have that for any pair $ ( \nu, \eta ) $ with probability at least $ 1 - \exp \left( - n \kldiv{\frac{\sigma}{2}}{\frac{\sigma}{4}} \right) - \exp \left( -\frac{ n\sigma }{ 128 } \right) $ that $ \fn ( \nu, \eta) \geq \constnu \nu^2 + \consteta \eta^2 $ for some positive constants $\constnu$ and $\consteta $. Hence with high probability we can relax first constraint defining $\Omega_0$ to
% \begin{align}
%     \frac{ \innerprod{\wtwo}{H}^2 }{ n } \geq \constnu \nu^2 + \consteta  \eta^2
% \end{align}
% Furthermore we can relax both constraints to define the following set:
% \begin{align}
%     \Omega_1^{\eta} = \left\{ (\wone,\wtwo) \subjto \frac{ \innerprod{\wtwo}{H}^2 }{ n } \geq \consteta  \eta^2 \andtxts \norm{ \wtwo }_1 \leq \lonebound  \right\}
% \end{align}
% It is evident from definition that $ \Omega_0 \subset \Omega_1^{\eta}$ with high probability. Also note that constraints in the set $\Omega_1^{\eta}$ depend only on $\wtwo$ and hence we will now consider only this variable. Now we bound $ \eta = \norm{ \wtwo }_2 $ as:
% \begin{align}
%     \eta^2 \leq \max_{\wtwo} \norm { \wtwo }_2 \subjto \wtwo \in \Omega_1^{\eta}
% \end{align}

% We proceed following the path arguments established in \cite{wang2021tight}. We parametrize variable $\wtwo$ as $ \wtwo = b \norm { \gamma ( \alpha ) } $. 

% First we show that set $\Omega_1^{\eta}$ is not empty. Let's choose $ \alpha = \alpha_{\nstar}$ with $\nstar = n\fetaeta/2$. Since we defined $ \lonebound $ in such way that $ \alpha_{\nstar} \in \Omega_0 $ with high probability and we have $ \Omega_0 \subset \Omega_1^{\eta}$, this implies that with high probability there exists some $ b > 0 $ such that $ b \gamma ( \alpha ) \in \Omega_1^{\eta} $.

% Using the same argument as in lemma 1 in \cite{wang2021tight} for $\phidp$ we can write:
% \begin{align}
%     \eta^2 \leq \max_{1\leq \alpha \leq \alpham} B^2 \frac{ \norm { \gamma ( \alpha ) }_2^2 }{ \norm { \gamma ( \alpha ) }_1^2 } \subjto B\gamma \left( \alpha \right) \in \Omega_1^{\eta}
% \end{align}

% Now from lemma 4 in \cite{wang2021tight} we have that map $ \alpha \mapsto \frac{ \norm{ \gamma ( \alpha ) }_2^2 }{ \norm{ \gamma ( \alpha ) }_1^2 } $ is monotonically decreasing. Hence if we find value of $\alpha_{\uls}$ such that $\alpha_{\uls} \leq \alpha_{\nstar}$ and $ b \gamma ( \alpha_{\uls} ) \not \in \Omega_1^{\eta}$ for any $ b > 0 $ then we have:
% \begin{align} \label{eq:eta_bound_first_reduction}
%     \eta^2 \leq  B^2 \frac{ \norm { \gamma ( \alphauls ) }_2^2 }{ \norm { \gamma ( \alphauls ) }_1^2 }
% \end{align}

% In order to saturate constraint $ \norm{ \wtwo }_1 \leq B $ let $ b = \frac{B}{\alphauls}$. Since we want that $  b \gamma ( \alpha_{\uls} ) \not \in \Omega_1^{\eta} $ we will chose $s$ such that:
% \begin{align}
%     B^2 \frac{ \innerprod{ \gamma ( \alphauls )}{H}^2 }{ n \alphauls^2 } < \consteta B^2 \frac{ \norm{ \gamma ( \alphauls ) }_2^2 }{ \alphauls^2 }
% \end{align}
% Rewriting this inequality gives:
% \begin{align} \label{eq:s_condition_one}
%   \frac{ \norm{ \gamma ( \alphauls ) }_2^2 }{ \norm{H}_{\infty}^2 } > \frac{ 1 }{ \consteta n } 
% \end{align}
% Now we use concentration result from lemma \ref{lemma_gamma_conc} to get the following condition on $s$:
% \begin{align}
%     \frac{ 2 }{ \uls t_s^2 } \left( 1 - \frac{ c }{ \tuls^2 } \right) > \frac{ 1 }{ \consteta n }
% \end{align}

% We claim that $\uls = c_{\uls} \frac{ n }{ \log (d/n) }$ satisfies this inequality for some positive constant $ c_{\uls} $. From lemma 3 in \cite{wang2021tight} we know that if $ d/\uls \geq 11 $ we have that $ \log (d/\uls) \leq \tuls^2 \leq 2 \log (d/\uls) $. Using both of these bounds into expression \eqref{eq:s_condition_one} gives that:
% \begin{align}
%     \frac{ 2 }{ \uls \tuls^2 } \left( 1 - \frac{ c }{ \tuls^2 } \right) &> \frac{ 1 }{ 2 n c_{\uls} } \frac{ \log (d/n) }{ \log (d/n) + \log \log (d/n) - \log c_{\uls} } \left( 1 - \frac{c}{ \log (d/n) + \log \log (d/n) - \log c_{\uls} } \right)
%     \\
%     & = \frac{ 1 }{ 2 n c_{\uls} } \left( 1 - \OOO \left( \frac{\log (d/n) }{\log \log (d/n) } \right) \right) > \frac{1}{\consteta n}
% \end{align}
% where last inequality holds for $d/n$ sufficiently large.

% Now from equation \eqref{eq:eta_bound_first_reduction} and concentration lemma \ref{lemma_gamma_conc} we have:
% \begin{align}
%     \eta^2 \leq \frac{ n \fstar }{ \tnstar^2 } \frac{2}{\uls}\left( 1 + \frac{c}{\tuls^2} \right) \leq \boundeta' \left( 1 + \OOO \left( \frac{1}{ \log (d/n) } \right) \right) \leq \boundeta^2
% \end{align}

% Now we derive an upper bound for $\nu$. We consider the following set:
% \begin{align}
%     \Omega_1^{\nu} = \left\{ (\wone,\wtwo) 
%     \subjto
%     \frac{ \innerprod{\wtwo}{H}^2 }{ n } \geq \constnu \nu^2 \andtxts \norm{ \wtwo }_1 \leq \lonebound \andtxts \norm{ \wtwo }_2 \leq \boundeta  \right\}
% \end{align}
% Once again it follows that $\Omega_0 \subset \Omega_1^{\nu}$. Hence we can upper bound $\nu$ as follows:
% \begin{align} \label{eq:nu_opt_first_reduction}
%     \nu^2 \leq \frac{ 1 }{ n \constnu } \max_{\wtwo} \innerprod{\wtwo}{H}^2
%     \subjto 
%     \norm{ \wtwo }_1 \leq \lonebound 
%     \andtxts 
%     \norm{ \wtwo }_2 \leq \boundeta
% \end{align}

% Now we show can this optimization problem can be rewritten in a form suitable for using parametrized path approach. Similarly as in \cite{wang2021tight} we define function $\olw : \left[ \frac{1}{d}, 1 \right] \to \RR^{d-1}$ as
% \begin{align}
%     \olw(\beta) = \argmax_{\wtwo} \innerprod{\wtwo}{\Hgaussian}
%     \subjto \begin{cases}
%                 \norm{\wtwo}_2^2 \leq \beta \\
%                 \wtwo\geq 0\\
%                 \norm{\wtwo}_1 = 1
%             \end{cases}
% \end{align}
% From claim 2 in \cite{wang2021tight} we know that for any $\beta \in \left[ \frac{1}{d}, 1 \right] $ there exists $ \alpha \in \left[ 1, \alpham \right] $ such that $ \olw (\beta) = \frac{ \gamma(\alpha) }{ \alpha }$. Following similar argument as in fourth statement of lemma 4 in \cite{wang2021tight} we have that $ \olw (\beta) $ is monotonically increasing function in $\beta$. 

% Setting $ \tildewtwo = \frac{ \wtwo }{ B }$ we can rewrite \eqref{eq:nu_opt_first_reduction} as:
% \begin{align} 
%     \nu^2 \leq \frac{ B^2 }{ n \constnu } \max_{\tildewtwo} \innerprod{ \tildewtwo }{ H }^2
%     \subjto 
%     \norm{ \tildewtwo }_1 \leq 1 
%     \andtxts 
%     \norm{ \tildewtwo }_2 \leq \frac{ \boundeta }{ B }
% \end{align}
% Hence solution of this problem must be of the form $ \tildewtwo = \olw (\beta) $ for some $\beta$. Similarly as in the first part of this proof, we first show that there exists $\beta_{\nstar}$ which satisfies constraints, and then find $\beta_{\ols}$ such that $ \beta_{\ols} \geq \beta_{\nstar}$. From monotonicity of $ \olw (\beta)$ follows that $ \olw (\beta_{\ols}) \geq \olw (\beta_{\nstar})$. Equivalently, we can find $\alpha_{\uls}$ such that $\alpha_{\uls} \leq \alpha_{\nstar}$.

% \begin{align}\label{nu_bound_first_reduction}
%     \nu^2 
%     \leq
%     \frac{ B^2 }{ n \constnu } \frac{ \innerprod{ \gamma (\alphauls) }{ H }^2 }{ \alphauls^2 } 
%     \leq 
%     \frac{ B^2 }{ n \constnu } \frac{ \norm{H}_{\infty}^2 }{ \alphauls^2 }
% \end{align}

% Let $\tildewtwo = \frac{ \gamma (\alpha) }{ \alpha }$. The claim that $\alpha_{\nstar}$ satisfies constraints is once again straightforward from our definition of $B$. Now we want to find $\alphauls$ such that:
% \begin{align}\label{s_condition_nu_first_reduction}
%     \norm{ \tildewtwo }_2^2 = \frac{ \norm{ \gamma ( \alphauls ) }_2^2 }{ \alphauls^2 } > \frac{ \boundeta^2 }{ B^2 }
% \end{align}
% Using concentration result from lemma \ref{lemma_gamma_conc} and expression \eqref{phidn_bound} we get condition:
% \begin{align}
%     \frac{2}{\uls} \left( 1 - \frac{c}{\tuls^2} \right) > \frac{\boundeta^2 \tnstar^2}{ n \fstar }
% \end{align}
% Once again we claim that this equality is satisfied for $ \uls = \frac{ c n }{ \log (d/n) } $ for some positive constant $c$. It is easy to see that this is the same condition as in the previous part of the proof up to the constants and hence we can use the same proof here.

% From \eqref{nu_bound_first_reduction} we now have:
% \begin{align}
%     \nu^2 \leq \frac{ \fstar \tuls^2 }{ \constnu \tnstar^2 } \left( 1 - \frac{4}{\tuls^2} \right)^{-1} 
%     \leq c'_{\nu} \left( 1 + \OOO \left( \frac{ \log \log (d/n) }{\log (d/n) } \right) \right) \leq \boundnu^2
% \end{align}
% concluding the proof.
% \end{proof}

% \end{document}

==> ICML 22-3/sections_proof/5_2nd_reduction.tex <==
% \documentclass[appendix.tex]{subfiles}
% \begin{document}

% \subsubsection{Step 2: Bounding $\deltanu,\eta$ by terms of the order $\frac{1}{\sqrt{\log (d/n)}}$}
% \label{apx:subsec:secondReduction}

% \begin{lemma} \label{lemma_second_reduction}
%     There exist universal constants $B_{\nu,2} > 0, B_{\eta,2} > 0$ such that for any element $(\wone,\wtwo)$ of $\Omega_0$ we have that $\deltanu^2 \leq \frac{B_{\nu,2}^2}{ \log \left( d/n \right) }$ and $ \eta^2 \leq \frac{B_{\eta,2}^2}{ \log \left( d/n \right) }$ with probability at least $ 1 - $ over the draws of $..$.
% \end{lemma}

% \begin{proof}



% From lemma \ref{lemma_first_reduction} we know that with high probability $ \nu \leq c_{\nu} $ and $ \eta \leq c_{\eta} $. Hence we can use uniform convergence of $f_n$ to its expectation (proposition \ref{prop:unifConv}). Hence we can relax constraints from definition of set $\Omega_0$ as follows:
% \begin{align}
%     \frac{ \innerprod{\wtwo}{H}^2 }{ n } \geq f ( \nu, \eta ) - \constconc \geq  \fstar  + \tconstnu \deltanu^2 + \tconsteta \eta^2 - \constconc
% \end{align}
% where the second inequality follows from lemma \ref{lemma_quadratic_plus_fstar_bound}. Hence we consider set:
% \begin{align}
%     \Omega_2^{\eta} = \left\{ (\wone,\wtwo) \subjto \frac{ \innerprod{\wtwo}{H}^2 }{ n } \geq \fstar - \constconc +  \tconsteta \eta^2  \andtxts \norm{ \wtwo }_1 \leq \lonebound  \right\}
% \end{align}

% Following the same argument as in proof of lemma \ref{lemma_first_reduction} instead of inequality \eqref{eq:s_condition_one} we get:
% \begin{align}
%     \frac{ \left( \fstar - \constconc \right) \alpha_s^2 }{ B^2 \norm{H}_{\infty}^2 } + \tconsteta \frac{ \norm{ \gamma(\alpha_s) }_2^2 }{ \norm{H}_{\infty}^2 } > \frac{1}{n}
% \end{align}
% In order for inequality above to be satisfied we need:
% \begin{align}
%     \left( 1 - \frac{ \constconc }{ \fstar } \right) 
%     \frac{\tnstar^2}{t_s^2}
%     \left( 1 - \frac{4}{t_s^2} + \OOO \left( \frac{1}{t_s^4} \right) \right) 
%     \left( 1 + \frac{2}{\tnstar^2} + \OOO \left( \frac{1}{\tnstar^3} \right) \right) 
%     + \frac{2 n \tconsteta}{s t_s^2} \left( 1 + \OOO \left( \frac{1}{t_s^2} \right) \right) 
%     > 1
% \end{align}
% Assuming that $ s = c \nstar$ and $ \constconc = \OOO \left( \frac{1}{\tnstar^3} \right) $ we have:
% \begin{align}
%     \frac{\tnstar^2}{t_s^2}
%     \left( 1 + \frac{ \frac{4\tconsteta}{c\feestar}  - 4}{t_s^2} + \frac{2}{\tnstar^2} + \OOO \left( \frac{1}{\tnstar^3}, \frac{1}{t_s^3} \right) \right)
%     > 1
% \end{align}
% Fix $\ulambda > 0$. Choose $\uls = c_{\uls} \nstar$ such that $\uls < n$ is the largest integer for which $ \tuls^2 \geq \tnstar^2 + \ulambda $. Then we have condition:
% \begin{align}
%     \left( 1 - \frac{\ulambda}{\tuls^2} \right) \left( 1 + \frac{ \frac{4\tconsteta}{c_{\uls}\feestar}  - 4}{\tuls^2} + \frac{2}{\tnstar^2} + \OOO \left( \frac{1}{t_n^3} \right) \right)
%     > 1
% \end{align}
% For $\ulambda$ large enough inequality holds (Note: second brackets grow as $c_{\uls}^{-1}$ and the first decays like $\log ( c_{\uls} )$ - TO CHECK).

% Fix $\olambda > 0$. Now we choose $\ols = c_{\ols} \nstar$ such that $ \ols > n $ is the smallest integer for which $ t_{\ols}^2 \leq \tnstar^2 - \olambda $. Then we have:
% \begin{align}
%     \left( 1 + \frac{\olambda}{\tols^2} \right) \left( 1 + \frac{ \frac{4\tconsteta}{c_{\ols}\feestar}  - 4}{\tols^2} + \frac{2}{\tnstar^2} + \OOO \left( \frac{1}{t_n^3} \right) \right)
%     > 1
% \end{align}
% We claim that there exists $\olambda$ large enough such that this inequality holds (e.g. $\ulambda > 4$).

% Hence we can bound $\eta^2$ as follows:
% \begin{align} \label{eq:eta_bound_first_reduction}
%     \eta^2 
%     \leq
%     B^2 \frac{ \norm { \gamma ( \alphauls ) }_2^2 }{ \norm { \gamma ( \alphauls ) }_1^2 } 
%     \leq
%     \frac{ n \left( \fstar - \constconc \right) }{ \tnstar^2 } \frac{2}{\uls}\left( 1 + \frac{c}{\tuls^2} \right) 
%     \leq
%     \frac{c_{\eta}'}{\log (d/n) } \left( 1 + \OOO \left( \frac{1}{ \log (d/n) } \right) \right) 
%     \leq
%     \left( \frac{ B_{\eta,2} }{ \sqrt{\log (d/n)} } \right)^2
% \end{align}
% and similarly we get:
% \begin{align}
%     \eta^2 
%     \geq
%     B^2 \frac{ \norm { \gamma ( \alphaols ) }_2^2 }{ \norm { \gamma ( \alphaols ) }_1^2 } 
%     \geq
%     \left( \frac{ \overline{B}_{\eta,2} }{ \sqrt{\log (d/n)} } \right)^2
% \end{align}

% Following the proof of lemma \ref{lemma_first_reduction} we determine tighter upper bound for $\nu^2$.
% \begin{align}
%     \Omega_2^{\nu} = \left\{ (\wone,\wtwo) 
%     \subjto
%     \frac{ \innerprod{\wtwo}{H}^2 }{ n } \geq \fstar - \constconc + \tconstnu \nu^2 \andtxts \norm{ \wtwo }_1 \leq \lonebound \andtxts \norm{ \wtwo }_2 \leq \frac{B_{\eta,2}}{\sqrt{ \log (d/n) }}  \right\}
% \end{align}

% Analogously to equation \eqref{s_condition_nu_first_reduction} we derive new condition for $\uls$ as:
% \begin{align}
%     \norm{ \tildewtwo }_2^2 = \frac{ \norm{ \gamma ( \alphauls ) }_2^2 }{ \alphauls^2 } > \frac{ B_{\eta,2}^2 }{ B^2 \log (d/n) }
% \end{align}
% which is again satisfied for some $\uls = c_{\uls} n$ with $ c_{\uls} > 0 $. Hence from \eqref{nu_bound_first_reduction} we obtain bound:
% \begin{align}
%     \deltanu^2 
%     \leq
%     \frac{ B^2 }{ n \tconstnu } \frac{ \norm{H}_{\infty}^2 }{ \alphauls^2 } - \frac{\fstar - \constconc }{\tconstnu}
%     \leq 
%     \frac{ \fstar }{ \tconstnu \tnstar^2 } \left( 1 + \frac{4}{\tuls^2} \right) - \frac{\fstar - \constconc }{\tconstnu}
%     \leq 
%     \left( \frac{ B_{\nu,2} }{ \sqrt{\log (d/n)} } \right)^2
% \end{align}
% which concludes the proof.
% \end{proof}

% \end{document}

==> ICML 22-3/sections_proof/8_Regression.tex <==





\red{this is for regressino, just adavpt}


We have $f_n(\nu,\eta) = \|\xi - Z\eta - G\nu\|_2^2 $. We use the following approximations for $f_n$:
\begin{itemize}
    \item $\frac{1}{n} f_n \geq \sigmaxi^2 - \rho \sigmaxi \vert \eta\vert - \rho \sigmaxi \vert \nu \vert + (1-\rho) (\nu^2 + \eta^2)$
        \item $\frac{1}{n} f_n \leq \sigmaxi^2 + \rho \sigmaxi \vert \eta\vert + \rho \sigmaxi \vert \nu \vert + (1+\rho) (\nu^2 + \eta^2)$
\end{itemize}
where $\rho = \frac{\log(2/\delta}{\sqrt{n}}$. We use these approximations throughout the proof. 
We begin with the bound for $\phidn$.


==> ICML 22-3/sections_proof/9_Technical_proofs_thm1.tex <==
\section{Auxiliary proofs for Theorem 1}

\subsection{Proof of Proposition~\ref{prop:Rbound}}
\label{sec:appendix_proof_bound_phidn}

Recall that $\phidn$ is given by:
\begin{align}
    \phidn &= \min_{\nu,b,\alpha} \nu + b \norm{ \gamma \left( \alpha \right) }_1 
    \subjto \frac{ b^2\norm{\Hgaussian}_{\infty}^2 }{n} \geq \fn \left( \nu, b \norm{ \gamma \left( \alpha \right) }_2 \right)
\end{align}

Given that $(\tnu,\tb,\talpha)$ is a feasible point of $\phidn$ we have that $\phidn \leq  \tnu + \tb \norm{ \gamma( \talpha) }_1$, which gives us an upper bound on $\phidn$. In the following discussion our goal is to find a single feasible point of the constraint set of $\phidn$.

From definition of $\gamma ( \alpha )$ we know that $ \norm{ \gamma ( \alpha ) }_1 = \alpha$ and hence we can equivalently formulate $\phidn$ as an optimization over $\nu$ and $ b_{\alpha} := b \alpha $
\begin{align}
    \phidn &= \min_{ \nu, b_{\alpha} } \nu + b_{\alpha}
    \subjto \frac{ b_{\alpha}^2 \norm{\Hgaussian}_{\infty}^2 }{n \alpha^2} \geq \fn \left( \nu, b_{\alpha} \frac{ \norm{ \gamma \left( \alpha \right) }_2}{ \alpha } \right)
\end{align}

Define $\fstar = f \left( \nustar, 0 \right)$, $\feestar = \frac{\partial^2 f(\nuopt,\eta)}{\partial \eta^2}\Big|_{\eta=0}$ and $\nstar = \frac{1}{2}\feestar n$. Now using lemma \ref{lemma_point_conv} with $ t = \fstar \tnstar^{-3} $ and for a feasible point $( \nu, b_{\alpha} \frac{ \norm{ \gamma \left( \alpha \right) }_2}{ \alpha } )$ we have that:
\begin{align} \label{eq:constraint_f_conc}
    \frac{ b_{\alpha}^2 \norm{\Hgaussian}_{\infty}^2 }{n \alpha^2} 
    \geq
    f \left( \nu, b_{\alpha} \frac{ \norm{ \gamma \left( \alpha \right) }_2}{ \alpha } \right) + \frac{\fstar}{\tnstar^{3}}
\end{align}
with probability at least $ 1 - 2 \exp \left( -c \frac{ n }{ \tnstar^6 \left( \nu^2 + b_{\alpha}^2  \norm{ \gamma \left( \alpha \right) }_2^2 / \alpha^2 \right) } \right) $.
% > 1 - 2 \exp \left( - \tc \frac{ n }{ \log^3 \left( \frac{d}{n} \right)  } \right) $.

Let's now choose $ \nu = \nustar $ and show that there exists a pair $ ( b, \alpha )$  such that $ ( \nustar, b, \alpha) $ is feasible for constraint \eqref{eq:constraint_f_conc}. Furthermore, we propose to search for a point with parameter $ ( b, \alpha ) $ such that $ b \norm{ \gamma ( \alpha )}_2 = b_{\alpha} \frac{ \norm{ \gamma \left( \alpha \right) }_2}{ \alpha } $ is near zero. Hence, using Taylor series approximation of function $ f ( \nustar, \cdot ) : \eta \mapsto f (\nustar, \eta) $ around point $(\nuopt,0)$ we can rewrite constraint \eqref{eq:constraint_f_conc} as:
\begin{align}
     \frac{ b_{\alpha}^2 \norm{\Hgaussian}_{\infty}^2 }{n \alpha^2}   
     \geq
      \fstar + \frac{1}{2}\feestar b_{\alpha}^2 \frac{ \norm{ \gamma \left( \alpha \right) }_2^2}{ \alpha^2 } + \OOO \left( b_{\alpha}^3 \frac{ \norm{ \gamma \left( \alpha \right) }_2^3}{ \alpha^3 } \right) + \frac{\fstar}{\tnstar^{3}}
\end{align}
since $\feta = \frac{\partial f(\nuopt,\eta)}{\partial \eta}\Big|_{\eta=0} = 0$.

As we mentioned in section \ref{step_1_thm3_proof}, $ \gamma ( \alpha ) $ is a piecewise linear function with breakpoints at $ \alpha_s $ for $ s = 2, \dots, d-1 $. Hence instead of optimizing over $\alpha$ we optimize over $s$. Note that we have only one constraint but two free variables $ ( b, \alpha ) $ and so we can set $ \alpha = \alpha_{\nstar} $ with $ \nstar = \frac{1}{2}\feestar n $. We explain this choice of $s$ in the remark after the proof. Combining all these results we get constraint:
\begin{align} \label{eq:B_ineq}
     \frac{ b_{\alpha_{\nstar}}^2 \norm{\Hgaussian}_{\infty}^2 }{n \alpha_{\nstar}^2}   
     \geq
      \fstar + \frac{1}{2}\feestar b_{\alpha_{\nstar}}^2 \frac{ \norm{ \gamma \left( \alpha_{\nstar} \right) }_2^2}{ \alpha_{\nstar}^2 } + \OOO \left( b_{\alpha_{\nstar}}^3 \frac{ \norm{ \gamma \left( \alpha_{\nstar} \right) }_2^3}{ \alpha_{\nstar}^3 } \right) + \frac{\fstar}{\tnstar^{3}}
\end{align}

Now we claim that
\begin{equation}
    b_{\alpha_{\nstar}}^2 = \frac{ n \alpha_{\nstar}^2 }{ \norm{\Hgaussian}_2^2 } \frac{ \fstar \left( 1 + \frac{1}{\tnstar^{3}} \right) }{ 1 - \frac{1}{2} n \feestar \frac{ \norm{ \gamma \left( \alpha_{\nstar} \right) }_2^2 }{ \norm{H}_{\infty}^2 } - \OOO \left( \frac{1}{\tnstar^3} \right) }
\end{equation}
satisfies inequality \eqref{eq:B_ineq} with probability at least $ 1 - 6 \exp \left( -\frac{\nstar}{\log(d/\nstar)^5} \right)$. Using lemma \ref{lemma_gamma_conc} we have that:
\begin{equation}
    1 - \frac{1}{2} n \feestar \frac{ \norm{ \gamma \left( \alpha_{\nstar} \right) }_2^2 }{ \norm{H}_{\infty}^2 } - \OOO \left( \frac{1}{\tnstar^3} \right) > 1 - \frac{1}{2} n \feestar  \frac{2}{\nstar \tnstar^2} - \OOO \left( \frac{1}{\tnstar^3} \right) = 1 - \frac{2}{\tnstar^2} - \OOO \left( \frac{1}{\tnstar^3} \right)  > 0
\end{equation}
holding for $d,n$ sufficiently large. Applying Lemma \ref{lemma_gamma_conc} once again we get:
\begin{equation}
    b_{\alpha_{\nstar}}^2 
    \leq
    \frac{ n \fstar }{ \tnstar^2 } \left( 1 + \frac{1}{\tnstar^3} \right) \left( 1 - \frac{4}{\tnstar^2} + \frac{c}{\tnstar^4} \right) \frac{1}{ 1 - \frac{2}{\tnstar^2} - \OOO \left( \frac{1}{\tnstar^3} \right)}
    \leq
    \frac{ n \fstar }{ \tnstar^2 } \left( 1 - \frac{2}{\tnstar^2} + \frac{c}{\tnstar^3} \right)
\end{equation}

Hence we have that $ \OOO \left( b_{\alpha_{\nstar}}^3 \frac{ \norm{ \gamma \left( \alpha_{\nstar} \right) }_2^3}{ \alpha_{\nstar}^3 } \right) = \OOO \left( \frac{1}{\tnstar^3} \right)$ and this $b_{\alpha_{\nstar}}^2$ indeed satisfies equation \eqref{eq:B_ineq}. Now we define the upper bound on $\phidn$ as:
\begin{align}
\label{eq:lonebound_def}
    \lonebound := \sqrt{ \frac{ n \fstar }{ \tnstar^2 } \left( 1 - \frac{2}{\tnstar^2} + \frac{c}{\tnstar^3} \right) }
\end{align}
which holds with probability at least $ 1 - 2 \exp \left( -c \frac{ n }{ \tnstar^6 \left( \nustar^2 + b_{\alpha_{\nstar}}^2  \norm{ \gamma \left( \alpha_{\nstar} \right) }_2^2 / \alpha_{\nstar}^2 \right) } \right) - 6 \exp \left( -\frac{\nstar}{\log(d/\nstar)^5} \right) $. The proposition is proved after noting that $ \nustar^2 + b_{\alpha_{\nstar}}^2  \norm{ \gamma \left( \alpha_{\nstar} \right) }_2^2 / \alpha_{\nstar}^2 = \OOO(1)$.









\subsection{Proof of Lemma~\ref{lemma_first_reduction}}
According to Lemma \ref{quadratic_bound_fn} we have that for any pair $ ( \nu, \eta ) $ with probability at least $ 1 - \exp \left( - n \kldiv{\frac{\sigma}{2}}{\frac{\sigma}{4}} \right) - \exp \left( -\frac{ n\sigma }{ 128 } \right) $ that $ \fn ( \nu, \eta) \geq \constnu \nu^2 + \consteta \eta^2 $ for some positive constants $\constnu$ and $\consteta $. Hence with high probability we can relax first constraint defining $\Gamma_0$ to
% \begin{align}
%     \frac{ \innerprod{\wtwo}{H}^2 }{ n } \geq \constnu \nu^2 + \consteta  \eta^2
% \end{align}
\begin{align}
    \frac{1}{n} b^2 \norm{H}_{\infty}^2 \geq \constnu \nu^2 + \consteta b^2 \norm{\gamma(\alpha)}_2^2    
\end{align}

Let's first consider bounding of $\eta$ and then we use obtained result to bound $\nu$.
\paragraph{Upper bound on $\eta$.}
For this part of the proof we further relax both constraints from definition \eqref{eq:Omega_0_def} of $\Gamma_0$ and define the following set:
\begin{align}
    \Gamma_1^{\eta} = \left\{ (\nu, b, \alpha) \subjto \frac{1}{n} b^2 \norm{H}_{\infty}^2 \geq \consteta  b^2 \norm{\gamma(\alpha)}_2^2 \andtxts b \alpha \leq \lonebound  \right\}
\end{align}
% \begin{align}
%     \Gamma_1^{\eta} = \left\{ (\wone,\wtwo) \subjto \frac{ \innerprod{\wtwo}{H}^2 }{ n } \geq \consteta  \eta^2 \andtxts \norm{ \wtwo }_1 \leq \lonebound  \right\}
% \end{align}
It is evident from definition that $ \Gamma_0 \subset \Gamma_1^{\eta}$ with high probability. Also note that constraints in the set $\Gamma_1^{\eta}$ do not depend on $\nu$ and hence we will now consider only variables $b$ and $\alpha$. Now we bound $ \eta $ as:
\begin{align}
    \eta^2 \leq \max_{b,\alpha} b^2 \norm{\gamma(\alpha)}_2^2 \subjto (b,\alpha) \in \Gamma_1^{\eta}
\end{align}

We proceed following the path arguments established in \cite{wang2021tight}. First we show that set $\Gamma_1^{\eta}$ is not empty. Let's choose $ \alpha = \alpha_{\nstar}$ with $\nstar = n\fetaeta/2$. Recall that we defined $ \lonebound $ in such way that $ (b,\alpha_{\nstar}) \in \Gamma_0 $ with high probability for $b \alpha_{\nstar}\leq \lonebound$. As $ \Gamma_0 \subset \Gamma_1^{\eta}$, with high probability there exists some $ b > 0 $ such that $ (b, \alpha_{\nstar} ) \in \Gamma_1^{\eta} $ proving that $\Gamma_1^{\eta} \neq \emptyset$.

Recall from definition \eqref{eq:def_gamma_alpha} that $\norm{\gamma(\alpha)}_1 = \alpha$. Then using the same arguments as in Lemma 1 in \cite{wang2021tight}, we set $ b = \frac{\lonebound}{\alpha} $ and obtain:
\begin{align}
\label{eq:step_one_eta_bound_alpha}
    \eta^2 
    \leq
    \max_{1\leq \alpha \leq \alpham} \lonebound^2 \frac{ \norm { \gamma ( \alpha ) }_2^2 }{ \norm { \gamma ( \alpha ) }_1^2 } 
    \subjto
    %B\gamma \left( \alpha \right) \in \Gamma_1^{\eta}
    \left( \frac{\lonebound}{\alpha}, \alpha \right) \in \Gamma_1^{\eta}
\end{align}

As mentioned in section \ref{step_1_thm3_proof} the map $ \alpha \mapsto \frac{ \norm{ \gamma ( \alpha ) }_2^2 }{ \norm{ \gamma ( \alpha ) }_1^2 } $ is monotonically decreasing and the mapping $ \alpha \mapsto \consteta b^2 \norm{\gamma(\alpha)}_2^2 $ is convex. The interval of $\alpha \in [1,\alpham]$ for which constraint in equation \eqref{eq:step_one_eta_bound_alpha} holds is an interval since it is as a sublevel set of a convex function. Therefore if we find value of $\alpha_{\uls}$ such that $\alphauls \leq \alpha_{\nstar}$ and $ ( \frac{M}{\alphauls}, \alphauls ) \not \in \Gamma_1^{\eta}$, then we have:
\begin{align} \label{eq:eta_bound_first_reduction}
    \eta^2 \leq  \lonebound^2 \frac{ \norm { \gamma ( \alphauls ) }_2^2 }{ \norm { \gamma ( \alphauls ) }_1^2 }
\end{align}

% In order to saturate constraint $ \norm{ \wtwo }_1 \leq \lonebound $ let $ b = \frac{\lonebound}{\alphauls}$. 
In order to have $ ( \frac{M}{\alphauls}, \alphauls ) \not \in \Gamma_1^{\eta}$ we will chose $\uls$ as the smallest integer for which first constraint in definition of $\Gamma_1^{\eta}$ is not satisfied, i.e. choose  $\uls$ satisfying
% \begin{align}
%     \lonebound^2 \frac{ \innerprod{ \gamma ( \alphauls )}{H}^2 }{ n \alphauls^2 } < \consteta \lonebound^2 \frac{ \norm{ \gamma ( \alphauls ) }_2^2 }{ \alphauls^2 }
% \end{align}
\begin{align}
\label{eq:s_condition_one}
    \frac{1}{n} \frac{\lonebound^2}{\alphauls^2} \norm{H}_{\infty}^2 
    <
    \consteta \frac{\lonebound^2}{\alphauls^2} \norm{ \gamma ( \alphauls ) }_2^2 
\end{align}
% Rewriting this inequality gives:
% \begin{align} \label{eq:s_condition_one}
%   \frac{ \norm{ \gamma ( \alphauls ) }_2^2 }{ \norm{H}_{\infty}^2 } > \frac{ 1 }{ \consteta n } 
% \end{align}
After rewriting and using concentration result from Proposition \ref{lemma_gamma_conc} we obtain the following condition on $\uls$:
\begin{align}
    \frac{ 2 }{ \uls \tuls^2 } \left( 1 - \OOO \left( \frac{ 1 }{ \tuls^2 } \right) \right) > \frac{ 1 }{ \consteta n }
\end{align}

 We claim that $\uls =\lambda_{\uls} \frac{ n }{ \log (d/n) }$ satisfies this inequality for some positive universal constant $ \lambda_{\uls} >0  $. Using characterization $t_s = 2\log (d/s) + \OOO (\log \log (d\s) ) $ from section \ref{step_1_thm3_proof} we get:
\begin{align}
    \frac{ 2 }{ \uls \tuls^2 } \left( 1 - \OOO \left( \frac{ 1 }{ \tuls^2 } \right) \right) 
    & >
    % \frac{ 2\log (d/n)  }{ n \lambda_{\uls} } \frac{ 1 }{ 2\log (d/\uls) + \OOO \left(\log \log (d/\uls) \right) } \left( 1 - \OOO \left( \frac{1}{\log (d/n)} \right) \right)
    % \\
    % & = 
    \frac{ 1 }{ n \lambda_{\uls} } \left( 1 - \OOO \left( \frac{\log\log (d/n) }{\log (d/n) } \right) \right) > \frac{1}{\consteta n}
\end{align}
where last inequality holds for $d/n$ sufficiently large and $\lambda_{\uls}$ small enough.

Now from equation \eqref{eq:eta_bound_first_reduction} and concentration Proposition \ref{lemma_gamma_conc}, for some positive constant $B_{\eta,1}$ we get:
\begin{align}
    \eta^2 \leq \frac{ n \fstar }{ \tnstar^2 } \frac{2}{\uls}\left( 1 + \OOO \left( \frac{1}{\tuls^2} \right) \right) %\leq \boundeta' \left( 1 + \OOO \left( \frac{1}{ \log (d/n) } \right) \right) 
    =: B_{\eta,1}^2
\end{align}
since for the chosen $\uls$ the term on the right hand side of inequality is of the order $\OOO (1)$.


\paragraph{Upper bound on $\nu$.} Now we derive an upper bound for $\nu$. We consider the following set:
\begin{align}
    \Gamma_1^{\nu} = \left\{ (\nu, b, \alpha) 
    \subjto
    \frac{1}{n} \innerprod{b\gamma(\alpha)}{H}^2 \geq \constnu \nu^2 \andtxts b\alpha \leq \lonebound \andtxts b\norm{\gamma(\alpha)}_2 \leq B_{\eta,1} \right\}
    %\frac{ \innerprod{\wtwo}{H}^2 }{ n } \geq \constnu \norm{\wone}_2^2 \andtxts \norm{ \wtwo }_1 \leq \lonebound \andtxts \norm{ \wtwo }_2 \leq \boundeta  \right\}
\end{align}
% \begin{align}
%     \Gamma_1^{\nu} = \left\{ (\wone,\wtwo) 
%     \subjto
%     \frac{ \innerprod{\wtwo}{H}^2 }{ n } \geq \constnu \nu^2 \andtxts \norm{ \wtwo }_1 \leq \lonebound \andtxts \norm{ \wtwo }_2 \leq \boundeta  \right\}
% \end{align}
As we noted in Section \ref{step_1_thm3_proof}, from Claim 3 in \cite{wang2021tight} follows that $\innerprod{\gamma(\alpha)}{H} = \norm{H}_{\infty}$ and we obtain that $\Gamma_0 \subset \Gamma_1^{\nu}$ with high probability. Hence we can upper bound $\nu$ as follows:
\begin{align} \label{eq:nu_opt_first_reduction}
    \nu^2 \leq \frac{ 1 }{ n \constnu } \max_{b,\alpha} b^2 \innerprod{\frac{\gamma(\alpha)}{\alpha}}{H}^2
    \subjto 
    b \leq \lonebound 
    \andtxts 
    b\norm{ \frac{\gamma(\alpha) }{\alpha} }_2 \leq B_{\eta,1}
\end{align}

First note that choosing $b=M$ maximizes the objective if the second constraint is satisfied as well. Now we show how this optimization problem can be rewritten in a more suitable form for solving via parametrized path approach. Similarly as in \cite{wang2021tight} we define function $\olw : \left[ \frac{1}{d}, 1 \right] \to \RR^{d-1}$ as
\begin{align}
    \olw(\beta) = \argmax_{\wtwo} \innerprod{\wtwo}{\Hgaussian}
    \subjto \begin{cases}
                \norm{\wtwo}_2^2 \leq \beta \\
                \wtwo\geq 0\\
                \norm{\wtwo}_1 = 1
            \end{cases}
\end{align}
From Claim 2 in \cite{wang2021tight} we know that for any $\beta \in \left[ \frac{1}{d}, 1 \right] $ there exists $ \alpha \in \left[ 1, \alpham \right] $ such that $ \olw (\beta) = \frac{ \gamma(\alpha) }{ \alpha }$. Following similar argument as in Lemma 4 in \cite{wang2021tight} we have that $ \olw (\beta) $ is monotonically increasing function in $\beta$. Hence we can rewrite \eqref{eq:nu_opt_first_reduction} as:
\begin{align} 
\label{eq:first_iteration_nu_gamma_beta}
    \nu^2 \leq \frac{ \lonebound^2 }{ n \constnu } \max_{\beta} \innerprod{ \olw(\beta) }{ H }^2
    \subjto 
    \norm{ \olw(\beta) }_2 \leq \frac{ B_{\eta,1} }{ \lonebound }
\end{align}

Similarly as in the first part of this proof, we first show that there exists $\beta_{\nstar}$ which satisfies constraints, and then find smallest $\beta_{\ols}$ which does not satisfy constraints in \eqref{eq:first_iteration_nu_gamma_beta} and such that $ \beta_{\ols} \geq \beta_{\nstar}$. From monotonicity of $ \olw (\beta)$ follows that $ \olw (\beta_{\ols}) \geq \olw (\beta_{\nstar})$. Since the constraints in \eqref{eq:first_iteration_nu_gamma_beta} are convex in $\olw(\beta)$, the expression is maximized for $\beta = \beta_{\ols}$.

Since $\alpha = \alpha_{\nstar}$ satisfies constraints in \eqref{eq:nu_opt_first_reduction} by definition of $M$, we define $\beta_{\nstar}$ such that $\gamma(\beta_{\nstar}) = \frac{\gamma(\alpha_{\nstar})}{\alpha_{\nstar}}$ and hence $\beta_{\nstar}$ satisfies constraints in \eqref{eq:first_iteration_nu_gamma_beta}. Furthermore, if we find $\alpha_{\uls}$ such that $\alpha_{\uls} \leq \alpha_{\nstar}$ and
\begin{align}\label{s_condition_nu_first_reduction}
    \frac{ \norm{ \gamma ( \alphauls ) }_2 }{ \alphauls } 
    >
    \frac{ B_{\eta,1} }{ \lonebound }
\end{align}
we automatically obtain $\beta_{\uls}$ such that $\gamma(\beta_{\uls}) = \frac{\gamma(\alpha_{\uls})}{\alpha_{\uls}}$ which does not satisfy constraint in \eqref{eq:first_iteration_nu_gamma_beta}. 
Now from \eqref{s_condition_nu_first_reduction} and using concentration result from Proposition \ref{lemma_gamma_conc} and expression \eqref{phidn_bound} we obtain condition:
\begin{align}
    \frac{2}{\uls} \left( 1 - \OOO \left( \frac{1}{\tuls^2} \right) \right)
    >
    \frac{B_{\eta,1}^2 \tnstar^2}{ n \fstar } \left( 1 + \OOO \left( \frac{1}{\tnstar^2} \right) \right)
\end{align}
Once again we claim that this equality is satisfied for $ \uls = \lambda_{\uls} \frac{ n }{ \log (d/n) } $ for some positive constant $\lambda_{\uls}$. The proof follows use the same reasoning as in the previous part of the proof.

Hence we can bound $\nu$ from expression \eqref{eq:nu_opt_first_reduction} as follows:
\begin{align}\label{nu_bound_first_reduction}
    \nu^2 
    \leq
    \frac{ \lonebound^2 }{ n \constnu } \frac{ \innerprod{ \gamma (\alphauls) }{ H }^2 }{ \alphauls^2 }
    =
    \frac{ \lonebound^2 }{ n \constnu } \frac{ \norm{H}_{\infty}^2 }{ \alphauls^2 }
\end{align}
with the equality holding for $\gamma(\alpha)$ as discussed in Section \ref{step_1_thm3_proof}. Using concentration results from Proposition \ref{lemma_gamma_conc} we conclude that there exists a positive constant $B_{\nu,1}$ such that:
\begin{align}
    \nu^2 \leq \frac{ \fstar \tuls^2 }{ \constnu \tnstar^2 } \left( 1 + \OOO \left( \frac{1}{\tuls^2} \right) \right)
    % \leq c'_{\nu} \left( 1 + \OOO \left( \frac{ \log \log (d/n) }{\log (d/n) } \right) \right) \leq
    =: B_{\nu,1}^2
\end{align}
since the term on the right hand side is of the order $\OOO(1)$ for chosen $\uls$. This concludes the proof of the lemma.











\subsection{Proof of Lemma~\ref{lemma_second_reduction}}

From Lemma \ref{lemma_first_reduction} we know that with high probability $ \nu \leq B_{\nu,1} $ and $ \eta \leq B_{\eta,1} $. Hence we can use uniform convergence of $f_n$ to its expectation (Proposition \ref{prop:unifConv}) and relax constraint from definition of set $\Gamma_0$ as follows:
\begin{align}
\label{eq:second_iteration_relaxed_constraint_f}
    \frac{1}{n} b^2 \norm{H}_{\infty}^2 \geq f_n (\nu, b\norm{\gamma(\alpha)}_2) \geq f ( \nu, b\norm{\gamma(\alpha)}_2 ) - \constconc \geq  \fstar  + \tconstnu \deltanu^2 + \tconsteta b^2\norm{\gamma(\alpha)}_2^2 - \constconc
\end{align}
Again we first consider bounding of $\eta$ and then use obtained result for bounding of $\deltanu = \nu -\nustar$.

\paragraph{Upper bound on $\eta$.} 
We consider the set:
\begin{align}
    \Gamma_2^{\eta} = \left\{ (\nu, b, \alpha) 
    \subjto 
    \frac{ 1 }{ n } b^2 \norm{H}_{\infty}^2 \geq \fstar +  \tconsteta b^2 \norm{\gamma(\alpha)}_2^2 - \constconc
    \andtxts
    b\alpha \leq \lonebound
    \right\}
\end{align}
% \begin{align}
%     \Gamma_2^{\eta} = \left\{ (\wone,\wtwo) \subjto \frac{ \innerprod{\wtwo}{H}^2 }{ n } \geq \fstar - \constconc +  \tconsteta \norm{\wtwo}_2^2  \andtxts \norm{ \wtwo }_1 \leq \lonebound  \right\}
% \end{align}
% \begin{align}
%     \Gamma_2^{\eta} = \left\{ (\wone,\wtwo) \subjto \frac{ \innerprod{\wtwo}{H}^2 }{ n } \geq \fstar - \constconc +  \tconsteta \eta^2  \andtxts \norm{ \wtwo }_1 \leq \lonebound  \right\}
% \end{align}
Now we can use the same arguments as in proof of Lemma \ref{lemma_first_reduction} since adding a constant term to the constraint essentially does not change the problem. Instead of inequality \eqref{eq:s_condition_one} we get condition:
\begin{align}
    \left( \fstar - \constconc \right) \frac{ n \alphauls^2 }{  \lonebound^2 \norm{H}_{\infty}^2 } + \tconsteta n \frac{ \norm{ \gamma(\alphauls) }_2^2 }{ \norm{H}_{\infty}^2 } > 1
\end{align}
% In order for inequality above to be satisfied we need:
% \begin{align}
%     \left( 1 - \frac{ \constconc }{ \fstar } \right) 
%     \frac{\tnstar^2}{t_s^2}
%     \left( 1 - \frac{4}{t_s^2} + \OOO \left( \frac{1}{\tnstar^3} \right) \right) 
%     \left( 1 + \frac{2}{\tnstar^2} + \OOO \left( \frac{1}{\tnstar^3} \right) \right) 
%     + \frac{2 n \tconsteta}{s t_s^2} \left( 1 + \OOO \left( \frac{1}{t_s^2} \right) \right) 
%     > 1
% \end{align}
Assuming that $ \uls = \lambda_{\uls} \nstar$ and $ \constconc = \OOO \left( \frac{1}{\tnstar^3} \right) $ and using Propositions \ref{prop:concentrationl1} and \ref{prop:Rbound} we get condition:
\begin{align}
    1 + \frac{1}{\tnstar^2} \left( \frac{2\tconsteta}{\lambda} - 2 \right) + \OOO \left( \frac{1}{\tnstar^3} \right) > 1
\end{align}
which holds for $\lambda_{\uls}$ sufficiently small.

% \begin{align}
%     \frac{\tnstar^2}{t_s^2}
%     \left( 1 + \frac{ \frac{4\tconsteta}{\lambda\feestar}  - 4}{t_s^2} + \frac{2}{\tnstar^2} + \OOO \left( \frac{1}{\tnstar^3}, \frac{1}{t_s^3} \right) \right)
%     > 1
% \end{align}
% Fix $\ulambda > 0$. Choose $\uls = \lambda_{\uls} \nstar$ such that $\uls < n$ is the largest integer for which $ \tuls^2 \geq \tnstar^2 + \ulambda $. Then we have condition:
% \begin{align}
%     \left( 1 - \frac{\ulambda}{\tuls^2} \right) \left( 1 + \frac{ \frac{4\tconsteta}{\lambda_{\uls}\feestar}  - 4}{\tuls^2} + \frac{2}{\tnstar^2} + \OOO \left( \frac{1}{t_n^3} \right) \right)
%     > 1
% \end{align}
% For $\ulambda$ large enough inequality holds (Note: second brackets grow as $\lambda_{\uls}^{-1}$ and the first decays like $\log ( \lambda_{\uls} )$ - TO CHECK).


% \red{okay I messed this up - sorry. Can you make the following section a bit clearer? In particular, the connection to tn and s is not clear, cite the result form our paper. . So here we need to say that essentially we obtain the same problem as studied in my paper.}

% Fix $\olambda > 0$. Now we choose $\ols = c_{\ols} \nstar$ such that $ \ols > n $ is the smallest integer for which $ t_{\ols}^2 \leq \tnstar^2 - \olambda $. Then we have:
% \begin{align}
%     \left( 1 + \frac{\olambda}{\tols^2} \right) \left( 1 + \frac{ \frac{4\tconsteta}{c_{\ols}\feestar}  - 4}{\tols^2} + \frac{2}{\tnstar^2} + \OOO \left( \frac{1}{t_n^3} \right) \right)
%     > 1
% \end{align}
% We claim that there exists $\olambda$ large enough such that this inequality holds (e.g. $\ulambda > 4$).

Hence, as in \eqref{eq:eta_bound_first_reduction}, we can bound $\eta^2$ as follows:
\begin{align} \label{eq:eta_bound_second_reduction}
    \eta^2 
    \leq
    \lonebound^2 \frac{ \norm { \gamma ( \alphauls ) }_2^2 }{ \norm { \gamma ( \alphauls ) }_1^2 } 
    \leq
    \frac{ n \fstar }{ \tnstar^2 } \frac{2}{\uls}\left( 1 + \OOO \left( \frac{1}{\tuls^2} \right) \right) 
    \leq
    % \frac{c_{\eta,2}}{\log (d/n) } \left( 1 + \OOO \left( \frac{1}{ \log (d/n) } \right) \right) 
    \frac{2\fstar}{\feestar \lambda_{\uls} \log (d/n) } \left( 1 + \OOO \left( \frac{1}{ \log (d/n) } \right) \right) 
    =:
    B_{\eta,2}^2
\end{align}
% and similarly we get:
% \begin{align}
%     \eta^2 
%     \geq
%     B^2 \frac{ \norm { \gamma ( \alphaols ) }_2^2 }{ \norm { \gamma ( \alphaols ) }_1^2 } 
%     \geq
%     \left( \frac{ \overline{B}_{\eta,2} }{ \sqrt{\log (d/n)} } \right)^2
% \end{align}

\paragraph{Upper bound on $\deltanu$.}
Following the proof of Lemma \ref{lemma_first_reduction} we determine tighter upper bound for $\nu^2$. First we define
\begin{align}
    \Gamma_2^{\nu} = \left\{ (\nu, b, \alpha) 
    \subjto
    \frac{1}{n}\innerprod{b\gamma(\alpha)}{H}^2 \geq \fstar - \constconc + \tconstnu \deltanu^2 
    \andtxts
    b\alpha \leq \lonebound 
    \andtxts
    b\norm{ \gamma(\alpha) }_2 \leq B_{\eta,2}  \right\}
\end{align}

% \begin{align}
%     \Gamma_2^{\nu} = \left\{ (\wone,\wtwo) 
%     \subjto
%     \frac{ \innerprod{\wtwo}{H}^2 }{ n } \geq \fstar - \constconc + \tconstnu \norm{\wone}_2^2 \andtxts \norm{ \wtwo }_1 \leq \lonebound \andtxts \norm{ \wtwo }_2 \leq \frac{B_{\eta,2}}{\sqrt{ \log (d/n) }}  \right\}
% \end{align}
% \begin{align}
%     \Gamma_2^{\nu} = \left\{ (\wone,\wtwo) 
%     \subjto
%     \frac{ \innerprod{\wtwo}{H}^2 }{ n } \geq \fstar - \constconc + \tconstnu \nu^2 \andtxts \norm{ \wtwo }_1 \leq \lonebound \andtxts \norm{ \wtwo }_2 \leq \frac{B_{\eta,2}}{\sqrt{ \log (d/n) }}  \right\}
% \end{align}

Analogously to equation \eqref{s_condition_nu_first_reduction} we derive new condition for $\uls$ with new bound $B_{\eta,2}$ 
% \begin{align}
%     \frac{ \norm{ \gamma ( \alphauls ) }_2 }{ \alphauls } > \frac{ B_{\eta,2} }{ \lonebound }
% \end{align}
which is again satisfied for some $\uls = \lambda_{\uls} n$ with $ \lambda_{\uls} > 0 $. Hence from \eqref{nu_bound_first_reduction} we obtain bound:
\begin{align}
    \deltanu^2 
    &\leq
    \frac{ \lonebound^2 }{ n \tconstnu } \frac{ \norm{H}_{\infty}^2 }{ \alphauls^2 } - \frac{\fstar - \constconc }{\tconstnu}
    \leq 
    \frac{ \fstar }{ \tconstnu } \left( 1 + \frac{2}{\tnstar^2}  \right) - \frac{\fstar}{\tconstnu} + \OOO \left( \frac{1}{\tnstar^3} \right)\\
    & = \frac{\fstar}{\tconstnu \log(d/n)}\left( 1 + \OOO \left( \frac{1}{\sqrt{\log(d/n)}} \right) \right)
    =: 
    B_{\deltanu,2}^2 
\end{align}
which concludes the proof.
































\subsection{Proof of Proposition \ref{prop:BoundOmegal1}}


% \begin{lemma}
%     There exist universal constant $B_{\nu,3} > 0, B_{\eta,3} > 0$ such that for any element $(\wone,\wtwo)$ of $\Gamma_0$ we have that $\deltanu^2 \leq \frac{B_{\nu,3}^2}{ \left( \log \left( d/n \right) \right)^{3/2} }$ and $ \eta^2 \leq \frac{B_{\eta,3}^2}{ \log \left( d/n \right) }$ with probability at least $ 1 - $ over the draws of $..$.
% \end{lemma}

% \begin{proof}
In this part of the proof we use Taylor series approximation of function $f$ with higher order terms bounded by results from Lemma \ref{lemma_second_reduction}. Similarly as in equation \eqref{eq:second_iteration_relaxed_constraint_f} we obtain the following relaxation of constraint defining $\Gamma_0$:
\begin{align}
    \label{eq:f_taylor_approx}
    \frac{1}{n} b^2 \norm{H}_{\infty}^2 
    \geq 
    % f ( \nu, \eta ) =
    \fstar + \frac{1}{2}\feestar b^2 \norm{\gamma(\alpha)}_2^2 + \frac{1}{2}\fnnstar \deltanu^2 - \constconc - \OOOc
    % \underbrace{\OOO \left( \frac{1}{ \log (d/n)^{3/2} } \right)}_{\OOOc}
\end{align}
% \end{proof}

\paragraph{Upper and lower bound on $\eta$.}
Now we proceed in the same manner as in the previous two steps. We further relax constraint from definition of $\Gamma_0$ and define the following set:
\begin{align}
    \Gamma_3^{\eta} = \left\{ (\nu, b, \alpha) 
    \subjto 
    \frac{ 1 }{ n } b^2 \norm{H}_{\infty}^2 \geq \fstar +  \frac{1}{2}\feestar  b^2 \norm{\gamma(\alpha)}_2^2  -\constconc - \OOOc
    \andtxts
    b\alpha \leq \lonebound
    \right\}
\end{align}

% \begin{align}
%     \Gamma_3^{\eta} = \left\{ (\wone,\wtwo) \subjto \frac{ \innerprod{\wtwo}{H}^2 }{ n } \geq \fstar - \constconc - \OOOc + \frac{1}{2}\feestar \eta^2  \andtxts \norm{ \wtwo }_1 \leq \lonebound  \right\}
% \end{align}
Let $\uls$ and $\ols$ be given as in Lemma \ref{lemma_uls_ols_exp}.
\begin{align}
\label{eq:third_iteration_eta_condition}
    \left( \fstar - \constconc - \OOOc \right) \frac{ \alpha_s^2 }{ \norm{H}_{\infty}^2 } \frac{ n }{ \lonebound^2 } 
    +
    \frac{1}{2} \feestar n \frac{ \norm{ \gamma (\alpha_s) }_2^2 }{ \norm{H}_{\infty}^2 } 
    > 1
\end{align}
for $s = \uls \leq \nstar $ and $ s = \ols \geq \nstar $.

Let $ \constconc + \OOOc = \OOO \left( \frac{1}{\tnstar^3} \right)$. Then following similar arguments as in proof of Claim 7 in \cite{wang2021tight} we obtain:
% \begin{align} (this is the last version of this equation)
%     \left( \fstar -\constconc - \OOOc \right) \frac{ \alphauls^2 }{ \norm{H}_{\infty}^2 } \frac{ n }{ \lonebound^2 } 
%     \geq 
%     1 - \frac{2}{\tnstar^2} - \frac{\lambda}{\tnstar^{5/2}} + \OOO \left( \frac{1}{\tnstar^3} \right) + \OOO \left( \frac{1}{\tnstar^5} \right) + \OOO \left( \frac{1}{\tnstar^2 \nstar} \right)
% \end{align}
% 
% \begin{align}
%     \left( \fstar -\constconc - \OOOc \right) \frac{ \alphauls^2 }{ \norm{H}_{\infty}^2 } \frac{ n }{ \lonebound^2 } \geq &
%     \fstar \left( 1 + \OOO \left( \frac{1}{\tnstar^3} \right) \right) \frac{1}{\tuls^2}\left( 1 - \frac{4}{\tuls^2} + \OOO \left( \frac{1}{\tuls^4} \right) \right)\frac{n \tnstar^2}{n\fstar} \left( 1 + \frac{2}{\tnstar^2} + \OOO \left( \frac{1}{\tnstar^3} \right) \right)
%     \\
%     \geq &
%     \left( 1 - \frac{\lambda}{\tnstar^2\sqrt{\tnstar}} + \OOO \left( \frac{1}{\tnstar^2 \nstar} \right) + \OOO \left( \frac{\lambda^2}{\tnstar^5} \right) \right) \left( 1 - \frac{2}{\tnstar^2} + \OOO \left( \frac{1}{\tnstar^3} \right) \right)
% \end{align}
% 
% \begin{align} (this is the last version of this equation)
%     \frac{1}{2} \feestar n \frac{ \norm{ \gamma (\alphauls) }_2^2 }{ \norm{H}_{\infty}^2 } 
%     \geq 
%     \frac{2}{\tnstar^2} + \frac{\lambda}{(\tnstar)^{5/2}} + \frac{\lambda^2}{2\tnstar^3} + \OOO \left( \frac{1}{\tnstar^{7/2}} \right) 
% \end{align}
% 
% \begin{align}
%     \frac{1}{2} \feestar n \frac{ \norm{ \gamma (\alphauls) }_2^2 }{ \norm{H}_{\infty}^2 } 
%     \geq &
%     \nstar \frac{2}{\uls \tuls^2} \left( 1 + \OOO \left( \frac{1}{\tuls^2} \right) \right)\\
%     \geq &
%     \frac{2}{\tnstar^2} \exp \left( \frac{\lambda}{2\sqrt{\tnstar}} \right)  \left( 1 + \OOO \left( \frac{1}{\tnstar^2} \right) \right) \\
%     \geq &
%     \frac{2}{\tnstar^2} \left( 1 + \frac{\lambda}{2\sqrt{\tnstar}} + \frac{\lambda^2}{4\tnstar} + \OOO \left( \frac{\lambda^3}{\tnstar\sqrt{\tnstar}} \right) \right) \left( 1 + \OOO \left( \frac{1}{\tnstar^2} \right) \right) 
% \end{align}
% 
% Hence we have:
\begin{align}
    \left( \fstar - \constconc - \OOOc \right) \frac{ \alphauls^2 }{ \norm{H}_{\infty}^2 } \frac{ n }{ \lonebound^2 } + \frac{1}{2} \feestar n \frac{ \norm{ \gamma (\alphauls) }_2^2 }{ \norm{H}_{\infty}^2 } 
    >
    1 + \frac{\lambda^2}{2\tnstar^3} + \OOO \left( \frac{1}{\tnstar^3} \right) + \OOO \left( \frac{1}{\tnstar^{7/2}} \right) + \OOO \left( \frac{1}{\tnstar^2 \nstar} \right)
\end{align}
By choosing $\lambda$ sufficiently large the inequality \eqref{eq:third_iteration_eta_condition} is satisfied. Hence we can bound $\eta^2$ as follows:
\begin{align} \label{eq:eta_bound_third_reduction}
    \eta^2 
    \leq
    \lonebound^2 \frac{ \norm { \gamma ( \alphauls ) }_2^2 }{ \norm { \gamma ( \alphauls ) }_1^2 } 
    & \leq
    \frac{ n \fstar }{ \tnstar^2 } \frac{2}{\uls}\left( 1 + \OOO\left( \frac{1}{\tnstar^2} \right) \right)
    \leq
    % \frac{4\fstar}{\feestar} \frac{1}{\tnstar^2}  \exp \left( \frac{\lambda}{2\sqrt{\tnstar}} \right) \left( 1 + \OOO\left( \frac{1}{\tnstar^2} \right) \right) \\
    % & \leq
    \frac{4\fstar}{\feestar} \frac{1}{\tnstar^2} \left( 1 + \frac{\lambda}{2\sqrt{\tnstar}} + \OOO \left( \frac{1}{\tnstar} \right) \right) =: B_{\eta,3}^2
\end{align}
and similarly we get:
\begin{align}
    \eta^2 
    \geq
    \lonebound^2 \frac{ \norm { \gamma ( \alphaols ) }_2^2 }{ \norm { \gamma ( \alphaols ) }_1^2 } 
    \geq
    \frac{4\fstar}{\feestar} \frac{1}{\tnstar^2} \left( 1 - \frac{\lambda}{2\sqrt{\tnstar}} + \OOO \left( \frac{1}{\tnstar} \right) \right) 
\end{align}



\paragraph{Upper bound on $\deltanu$.}
Now let
% \begin{align}
%     \Gamma_3^{\nu} = \left\{ (\nu, b, \alpha) 
%     \subjto
%     \frac{1}{n}\innerprod{b\gamma(\alpha)}{H}^2 \geq \fstar + \frac{1}{2}\feestar \eta^2 + \frac{1}{2}\fnnstar \deltanu^2 - \OOO \left( \frac{1}{\tnstar^3} \right)
%     \andtxts 
%     b\alpha \leq \lonebound 
%     \andtxts
%     b\norm{ \gamma(\alpha) }_2 \leq \frac{B_{\eta,3}}{\log (d/n) }  \right\}
% \end{align}
\begin{equation}
    \Gamma_3^{\nu} = \Bigg\{ (\nu, b, \alpha) 
    \subjto \begin{cases}
                \frac{1}{n}\innerprod{b\gamma(\alpha)}{H}^2 \geq \fstar - \constconc - \OOOc + \frac{1}{2}\feestar b\norm{\gamma(\alpha)}_2^2 + \frac{1}{2}\fnnstar \deltanu^2
                \\
                b\alpha \leq \lonebound
                \\
                b\norm{ \gamma(\alpha) }_2 \leq B_{\eta,3}
            \end{cases}
             \Bigg\}
\end{equation}
% \begin{align}
%     \Gamma_3^{\nu} = \left\{ (\wone,\wtwo) 
%     \subjto
%     \frac{ \innerprod{\wtwo}{H}^2 }{ n } \geq \fstar - \constconc - \OOOc + \frac{1}{2}\feestar \eta^2 + \frac{1}{2}\fnnstar \deltanu^2
%     \andtxts 
%     \norm{ \wtwo }_1 \leq \lonebound 
%     \andtxts
%     \norm{ \wtwo }_2 \leq B_{\eta,3}  \right\}
% \end{align}

% \begin{align}
% \label{s_condition_nu_third_reduction}
%     \frac{ \norm{ \gamma ( \alphauls ) }_2 }{ \alphauls } > \frac{B_{\eta,3}}{\lonebound}
% \end{align}
Analogously to equation \eqref{s_condition_nu_first_reduction} we derive new condition for $\uls$ with new bound $B_{\eta,3}$. Using concentration result from Proposition \ref{lemma_gamma_conc} and expression \eqref{phidn_bound} we get condition:
% \begin{align}
%     \frac{2}{\uls} \left( 1 + \OOO\left( \frac{1}{\tuls^2} \right) \right) 
%     >
%     \frac{4\fstar}{\feestar} \frac{1}{\tnstar^2} \left( 1 + \frac{\lambda}{2\sqrt{\tnstar}} + \OOO \left( \frac{1}{\tnstar} \right) \right) \frac{\tnstar^2}{ n \fstar } \left( 1 + \frac{2}{\tnstar^2} + \OOO \left( \frac{1}{\tnstar^3} \right) \right)
% \end{align}
% then
\begin{align}
    \frac{2}{\uls} \left( 1 + \OOO \left( \frac{1}{\tuls^2} \right) \right) > \frac{4}{\feestar} \frac{1}{n} \left( 1 + \frac{\lambda}{2\sqrt{\tnstar}} + \OOO \left( \frac{1}{\tnstar} \right) \right)
\end{align}
Hence let $\uls = \nstar \exp \left( -\frac{\lambda}{2\sqrt{\tnstar}} \right)$. %\frac{n\feestar}{2} \left( 1 - \frac{\lambda}{\sqrt{\tnstar}} + \OOO \left( \frac{1}{\tnstar} \right) \right)$.  
\begin{align}
    \deltanu^2 
    \leq
    \frac{ 2\lonebound^2 }{ n \fnnstar } \frac{ \norm{H}_{\infty}^2 }{ \alphauls^2 } - \frac{2}{\fnnstar} \left( \fstar - \constconc - \OOOc \right) - \frac{\feestar}{\fnnstar} \frac{ \norm{ \gamma(\alphaols) }_2^2 }{ \alphaols^2 } \lonebound^2
    \leq
    \frac{4 \fstar \lambda}{\fnnstar \tnstar^{5/2}} \left( 1 + \OOO \left( \frac{1}{\sqrt{\tnstar}} \right) \right) =: B_{\deltanu,3}^2
\end{align}
% \begin{align}
%     \deltanu^2 
%     &\leq
%     \frac{ 2\lonebound^2 }{ n \fnnstar } \frac{ \norm{H}_{\infty}^2 }{ \alphauls^2 } - \frac{2\fstar}{\fnnstar} \left( 1 - \constconc - \OOOc \right) - \frac{\feestar}{\fnnstar} \frac{ \norm{ \gamma(\alphaols) }_2^2 }{ \alphaols^2 } \lonebound^2\\
%     &\leq 
%     \frac{2}{n\fnnstar} \frac{n\fstar}{\tnstar^2} \left(1-\frac{2}{\tnstar^2}+\OOO \left( \frac{1}{\tnstar^3} \right) \right) \tuls^2 \left( 1 + \frac{4}{\tuls^2} + \OOO \left( \frac{1}{\tuls^4} \right) \right)
%     - \frac{2\fstar}{\fnnstar} \left( 1 + \OOO \left( \frac{1}{\tnstar^3} \right) \right)
%     \\
%      & - \frac{\feestar}{\fnnstar} \frac{2}{\nstar} \exp \left( -\frac{\lambda}{2\sqrt{\tnstar}} \right) \left( 1 + \OOO \left( \frac{1}{\tnstar^2} \right) \right) \frac{n\fstar}{\tnstar^2}  \left( 1 - \frac{2}{\tnstar^2} + \OOO \left( \frac{1}{\tnstar^3} \right) \right)
%      \\
%      &\leq \frac{2\fstar}{\fnnstar} \left( 1 + \frac{2}{\tnstar^2} + \frac{\lambda}{\tnstar^{5/2}} + \OOO \left( \frac{1}{\tnstar^3} \right) \right) 
%      - \frac{2\fstar}{\fnnstar} \left( 1 + \OOO \left( \frac{1}{\tnstar^3} \right) \right)
%      -\frac{2\fstar}{\fnnstar}\left( \frac{2}{\tnstar^2} - \frac{\lambda}{\tnstar^{5/2}} + \OOO \left( \frac{1}{\tnstar^3} \right) \right)
%      \\
%      & \leq \frac{4 \fstar \lambda}{\fnnstar}\frac{1}{\tnstar^{5/2}} \left( 1 + \OOO \left( \frac{1}{\sqrt{\tnstar}} \right) \right) =: B_{\deltanu,3}^2
% \end{align}








==> ICML 22-3/sections_proof/LP-proof_classification.tex <==
%\documentclass[../main.tex]{subfiles}
%\begin{document}





\section{Proof of Proposition~\ref{prop:uniformlowerbound}: Uniform lower bound for interpolating classifiers }
\label{apx:uniformlowerbound}

% We now derive a uniform lower bound for sparse interpolating classifiers with non zero margin, which following a similar strategy as the proof for the uniform lower bound for interpolating estimators in the regression setting of order $\Omega(\frac{n}{d})$ presented in \cite{wang2021tight} (and also earlier presented using a different proof technique in \cite{muthukumar_2020}). More detailed, we show
% \begin{proposition}
% \label{prop:uniformlowerbound}
% Assume that the observation noise satisfies assumption (A1) independent of $d,n$.  Then, for any non-zero ground truth $\wgt$ (not necessarily sparse) the risk of any interpolator $\what$ satisfying $\forall i: \yui \langle \xui, \what \rangle \geq 0$ is lower bounded by
% \begin{equation}
%     \Risk(\what) = \Theta\left(\sqrt{\frac{n}{d}}\right)
% \end{equation}
% with probability $\geq 1-\exp(-c n)$ with universal constant $c>0$; some positive universal constants independent of $d,n$ and $\what$.
% \end{proposition}
% \begin{proof}



% \begin{proposition}
% \label{prop:uniformlowerbound}
% Assume that the observation noise satisfies assumption (A1) independent of $d,n$.  Then, for any non-zero ground truth $\wgt$ (not necessarily sparse) the risk of any interpolator $\what$ satisfying $\forall i: \langle \yui \xui, \what \rangle \geq 0$ is lower bounded by
% \begin{equation}
%     \Risk(\what) = \Theta\left(\sqrt{\frac{n}{d}}\right)
% \end{equation}
% with probability $\geq 1-\exp(-c n)$ for some positive universal constants independent of $d,n$ and $\what$.
% \end{proposition}


First, note that we can assume without loss of generality that $\wgt$ is normalized, i.e. $\norm{\wgt}_2^2 = 1$. Furthermore, because the classification error is invariant under rotations of the input features, we can assume without loss of generality that $\wgt = (1,0,\cdots,0)$. This trick only works for rotational invariant distributions, including the Gaussian distribution,  where the marginal distribution for every sample rotated by a orthogonal matrix is again i.i.d.\ Gaussian. More precisely, let $\tilde{X} = OX$ with $O$ an orthogonal matrix and $X \sim \NNN(0,I_d)$, then $\tilde{X} \sim \NNN(0,I_d)$ as well. 

We now distinguish between the two cases where $\langle \hat{w}, \wgt \rangle \leq 0$ and $\langle \hat{w}, \wgt \rangle > 0$. Clearly, in the first case we have that $\RiskC(\what) \geq 2$, and hence, we only need to bound the second case. Furthermore, because the risk is invariant under rescalings of the vector $\what$, we can assume without loss of generality that $\langle \what, \wgt \rangle = 1$. 



For any $B >0$ define
\begin{align} 
    \Phip^{(B)} &= \max_w \frac{\innerprod{w}{\wgt}}{\norm{w}_2}
    \subjto \begin{cases}
        \min_i y_i\innerprod{x_i}{w}\geq 0\\
        \langle \wgt, w \rangle = 1 \\
        \norm{w}_2^2 \leq B,
    \end{cases}
\end{align}
where we remark that we could also choose for this proof any other norm or compact set to bound $w$ instead of the $\ell_2$-norm. 

We can now apply again the GMT (with slight trivial modifications) from Proposition~\ref{prop:CGMT_application_classification} to show that for any $t\in \mathbb{R}$, we have
\begin{equation}
                \PP( \Phip^{(B)} >t ) \leq 2\PP( \phidp^{(B)} \geq t ) 
            \label{eq:probeq3} ,
\end{equation}
with 
\begin{equation}
              \phidp^{(B)} = \max_{(\nu,\wtwo)} \frac{\nu}{\sqrt{\nu^2 +\norm{\wtwo}_2^2}}  
            \subjto \begin{cases}
               \frac{1}{n} \innerprod{\wtwo}{\Ggaussian}^2 \geq  \tilde{\fn}(\nu,\|\wtwo\|_2) \\
                 \nu^2  +\norm{\wtwo}_2^2  \leq B\\
                        \nu = 1 
            \end{cases}
\end{equation}
and $\tilde{\fn}(\nu,\eta) = \frac{1}{n} \sumin \possq{-\xi_i\sgn(\langle \wgt, \xsui \rangle) \langle \xsui, \nu\rangle -\Ggaussian_i y}$. 
Note that since we only assume that $\min_i \yui \langle \xui, \what\rangle \geq 0$ and not $\geq 1$, the constant $1$ factor in $\fnclas$ from Proposition~\ref{prop:CGMT_application_classification} in the term $(.)_+$ disappears in in $\tilde{\fn}$ . 

We can now again lower bound $\tilde{\fn}$, where we a straight forward modification of Lemma~\ref{quadratic_bound_fn} shows that, with probability at least $1-\exp(-cn)$, uniformly for all $\nu,\eta$,  we have
\begin{equation}
    \tilde{\fn}(\nu,\eta) \geq \constnu \nu^2  + \consteta \eta^2,
\end{equation} 
with $\constnu,\consteta>0$ some universal constants. Further, using Cauchy-Schwarz, we can upper bound 
$\frac{1}{n}\langle \wtwo, \Hgaussian\rangle^2 \leq \frac{1}{n}\|\Hgaussian\|_2^2 \|\wtwo\|_2^2 \leq \frac{2d \|\wtwo\|_2^2}{n}  $
 where the last inequality holds with probability at least $1- \exp(-c d)$ using standard concentration arguments. Hence, in summary we have the upper bound
 \begin{equation}
     \frac{2d \|\wtwo\|_2^2}{n} \geq \constnu \nu^2 \implies \frac{\|\wtwo\|_2^2}{\nu^2} \geq \Omega\left(\frac{n}{d}\right)
 \end{equation}
 
 Therefore, we have that for all $B>0$, $\phidp^{(B)} \leq 1 - \Omega\left(\frac{n}{d}\right)$ with universal constants independent of $B$ and thus the proof is complete.
 
 
 
%  Furthermore, by definition of $\Phip^{(B)}$, 
%  we have that for any $B_1 >B_2$ and any $t>0$ that $\prob(\Phip^{(B_2)} > t)  \leq \prob(\Phip^{(B_1)} >t )$. 
%  Since none of the constants $\constnu, \consteta$ and $c$ do not depend on $B$, we also have that $\lim_{B\to \infty} \prob(\Phip^{(B)} > 1- \Omega(\frac{n}{d})) \lesssim \exp(-cn)$. Finally, we conclude the proof from  $\RiskC(\what) \geq 2- 2 \Phip^{(\norm{\what}_1)}\geq 2 - 2\lim_{B\to\infty} \Phip^{(B)}\gtrsim \Omega(\frac{n}{d})$ with high probability.
% %  \end{proof}

 
 
% $\fn \geq \max(\min(f^* + c_1 \deltanu^2 + c_2 \eta^2, f^* + c_1 \B_{\nu}^2 + c_2 B_{\eta}^2)- \rho,  c_1 \deltanu^2 + c_2 \eta^)\gtrsim f^* + c_1 \deltanu^2 + c_2 \eta^2$. 
% Therefore, we immediately obtain the lower bound
% \begin{equation}
%     \eta^2 \gtrsim \frac{n}{d}\max( f^* +c_1 \deltanu^2)
% \end{equation}
%  Finally, since by $v^*$ is some constant, we obtain, 
 
% \begin{equation}
%      1-\arccos(\frac{\nu}{\sqrt{\nu + \eta}})\geq \Omega(\frac{n f^*}{d})
% \end{equation}
 
 
























% \begin{restatable}{proposition}{propRbound}
% \label{prop:Rbound}
% Let $t_{\nopt}$ be given by $2\Phic(t_{\nopt}) = \nopt/\tilded$ with $\nopt = n\fetaeta/2$. There exist universal constants $c,c_n,c_l,c_u,c_p$ such that, if $n\geq c_n$ and $c_l n\leq \tilded\leq \exp(c_u n^{1/5})$ then
%     \begin{align}
%         (\phidn)^2 \leq \frac{nf(\nuopt,0)}{t_{\nopt}^2}\left(1-\frac{2}{t_{\nopt}^2}+\frac{c}{t_{\nopt}^3} \right) =:\lonebound^2(n,\tilded)
%     \end{align}
% with probability at least $1-c_p\exp \left(-\frac{\nopt}{{\log(\tilded/\nopt)}^5}\right)-\OOO_c(!)$ over the draws of $\Hgaussian$, $\gausswone$ and $\gausswtwo$.

% \end{restatable}  
























%\end{document}



% Furthermore, we also study the case where $q$ is even of order $\log(d)$. In this case, we have the following Lemma:

% \begin{lemma}
% For any $c_1 \frac{\log(d)}{\log\log(d)} \leq q \leq c_0\log(d)$, we have with probability $\geq 1-c_1 d^{-c_2}$. 
% \begin{align}
% \langle \wgrad, H\rangle &= \norm{H}_q = \dmoment{q}\left(1+O\left(\frac{\log(d)}{q d^{2/q}} \right)\right) \\
% \norm{\wgrad}_2^2 &= \frac{\norm{H}_{2q/p}^{2q/p}}{\norm{H}_q^{2q/p}} = \frac{\dmoment{2q/p}^{2q/p}}{\dmoment{q}^{2q/p}}
% \left( 1 + O\left(\frac{\log(d)}{d^{2/q}\dmoment{q}} \right)\right) \leq  \Omega\left(d^{1/q-1/p + \frac{q}{\log(d)}}\right)
% \end{align}
% \end{lemma}




% We have
% \begin{itemize}
%     \item 
%     \item $\langle \wgrad, H\rangle = \norm{H}_q = \tilded^{1/q}(1+ O(\frac{log(2/\delta)}{\tilded^{1/q}}))$
%     \item  $\norm{\wgrad}_2^2 = \frac{\norm{H}_{2q/p}^{2q/p}}{\norm{H}_q^{2q/p}} = \mutild \tilded^{1-2/p} \left(1+O(\log(2/\delta) \tilded^{-p/(2q)}\right). $  \red{check correct big O term, though not super important at the moment. } 
% \end{itemize}










% All we use is this Equation:
% $$| \|X\|_p - \tilded^{1/p}\moment{p}^{1/p}  | \leq \sqrt{2\log(2/\delta)} L + c' \tilded^{1/p-1} = O(\log(2/\delta)$$









% \red{From here this needs to be rewritten...}



% Before starting with the bounding of $\phi_N''$ and $\phi_+'', \phi_-''$ we would have to study the concentration of norms of $\gamma(1)$ and $\gamma(\olalpha)$.

% We make use of the following lemma:
% \begin{lemma}
% Let $p >1$ and let $X \in \RR^\tilded$ be a random vector with standard normal i.i.\tilded. entries. For every $p \leq 2$ there exists a uniform constant $c > 0$ such that with probability $\geq 1-\delta$ 
% $$ |\frac{\EE \|X\|_p^p}{\tilded} -  \moment{p} | \leq c (\sqrt{2\log(2/\delta)}^p \tilded^{-p/2} + (\sqrt{2\log(2/\delta)}+1) \tilded^{-1/2})$$
% and for $p>2$
% $$ |\frac{\EE \|X\|_p^p}{\tilded} -  \moment{p} | \leq c( \sqrt{2\log(2/\delta)}^p \tilded^{-1}+ (\sqrt{2\log(2/\delta)}+1) \tilded^{-1/p})$$
% \end{lemma}
% \begin{proof}
% First, note that $\|.\|_p$ is a L-Lipschitz continous function with respect to the $L_2$-norm with $\begin{cases} L = \tilded^{1/p - 1/2} ~~~ p <2 \\
%     L = 1 
% \end{cases}$. 

% Therefore, we can use concentration of Measure to show that 
% $$ P(| \|X\|_p - \EE \|X\|_p | \geq t) \leq 2 \exp(-t^2/(2L^2)). $$
% In particular, this implies that for every $\delta \in ( 0,1)$ with probability $\geq 1-\delta$ we have that
% $$| \|X\|_p - \EE \|X\|_p | \leq \sqrt{2\log(2/\delta)} L.$$
% To proceed the proof, we would like to approximate the expectation $ \EE \|X\|_p $, which is already done in the following Proposition:
% \begin{proposition}[Proposition 3 in \cite{Biau2015}]
% For every $p> 0$ exists a constant $c'>0$ such that  
% $$ |\EE \|X\|_p - \moment{p}^{1/p}| \leq c' \tilded^{1/p-1} $$ 
% \end{proposition}

% Hence, we obtain that 
% $$| \|X\|_p - \tilded^{1/p}\moment{p}^{1/p}  | \leq \sqrt{2\log(2/\delta)} L + c' \tilded^{1/p-1}$$
% and using that for $a,b >0$ and $p\geq 1$ we have that $ |a-b| \leq c \implies |a^p - b^p| \leq c(c+a)^{p-1}$. 
% Hence, we conclude that for $p \in [1,2]$
% \begin{align}
%  |\|X\|_p^p - \tilded\moment{p}  | &\leq (\sqrt{2\log(2/\delta)} \tilded^{1/p-1/2} + c' \tilded^{1/p-1}) ( \sqrt{2\log(2/\delta)} \tilded^{1/p-1/2} + c' \tilded^{1/p-1} \moment{p} \tilded^{1/p})^{p-1 }\\
%  &= O(\sqrt{2\log(2/\delta)}^p \tilded^{1-p/2} + (\sqrt{2\log(2/\delta)}+1) \tilded^{1/2})
%  \end{align}
% Furthermore, in the case where $p>2$ we have 
% \begin{align}
%  |\|X\|_p^p - \tilded\moment{p}  | &\leq (\sqrt{2\log(2/\delta)}  + c' ) ( \sqrt{2\log(2/\delta)}  + c' \moment{p} \tilded^{1/p})^{p-1 }\\
%  &= O(\sqrt{2\log(2/\delta)}^p + (\sqrt{2\log(2/\delta)}+1) \tilded^{1-1/p})
%  \end{align}
% \end{proof}
% Throughout this proof we abbreviate $|\frac{\EE \|X\|_p^p}{\tilded} -  \moment{p} | \leq \bigO{p,\delta}$. 

% % We can now proceed to bound the quantities of interest. 
% % First, we study $\gamma(1)_i = (\frac{ |H_i|^{q-1}}{\|H\|^{q-1}_{q}})_i =(\frac{ |H_i|^{q/p}}{\|H\|^{q/p}_{q}})_i$. We have
% % \begin{lemma}
% % \begin{align}
% %      \|\gamma(1)\|_p &= 1
% %       \\
% %   \|\gamma(1)\|_2^2 &= \frac{\|H\|_{2q/p}^{2q/p}}{\|H\|_q^{2q/p}} = \tilded^{2/q} \frac{\moment{2q/p}}{\moment{q}^{2/q}} \frac{1+\bigO{2q/p,\delta}}{(1+\bigO{q,\delta})^{2/q}} 
% % \\
% %   \langle H, \gamma(1)\rangle &= \|H\|_q = \tilded^{1/q} \moment{q}^{1/q} (1+\bigO{q,\delta})^{1/q} 
% % \end{align}
% % \end{lemma}
% % \begin{proof}
% % Just check...
% % \end{proof}
% % Furthermore, we have $\gamma(\olalpha) = H \frac{\|H\|_q}{\|H\|_2^2}$.






% We assume that $\wgt$ is 1-sparse, and hence, $\nu$ is a scalar.
%  In the regression case, we have:

% \begin{align}
% \tag{$P_N$} \label{eq:PhiN}
%     \PhiNR &= \min_w \abs{\nu + \wgt}^p + \|\wtwo\|_p^p
%     \subjto \datamat w = \xi \\
% \tag{$P_+$} \label{eq:Phip}
%     \PhipR &= \min_w \abs{\nu }^2 + \|\wtwo\|_2^2
%     \subjto \begin{cases}
%          \datamat w = \xi \\ 
%         \abs{\wone + \wgt}^p + \|\wtwo\|_p^p \leq \lonebound
%     \end{cases}\\
% \tag{$P_-$} \label{eq:Phim}
%     \PhimR &= \max_w \abs{\wone }^2 + \|\wtwo\|_2^2 
%     \subjto \begin{cases}
%          \datamat w = \xi \\ 
%         \abs{\wone + \wgt}^p + \|\wtwo\|_p^p \leq \lonebound
%     \end{cases}
% \end{align}
% and in the classification case we have
% \begin{align}
% \tag{$P_N$} \label{eq:PhiN}
%     \PhiNC &= \min_w \abs{\wone + \wgt}^p + \|\wtwo\|_p^p
%     \subjto  \minin y_i\innerprod{x_i}{w}\geq 1 \\
% \tag{$P_+$} \label{eq:Phip}
%     \PhipC &= \min_w \abs{\wone }^2 + \|\wtwo\|_2^2
%     \subjto \begin{cases}
%          \minin y_i\innerprod{x_i}{w}\geq 1 \\ 
%         \abs{\wone + \wgt}^p + \|\wtwo\|_p^p \leq \lonebound
%     \end{cases}\\
% \tag{$P_-$} \label{eq:Phim}
%     \PhimC&= \max_w \abs{\wone }^2 + \|\wtwo\|_2^2 
%     \subjto \begin{cases}
%           \minin y_i\innerprod{x_i}{w}\geq 1 \\ 
%         \abs{\wone + \wgt}^p + \|\wtwo\|_p^p \leq \lonebound
%     \end{cases}
% \end{align}



% \begin{restatable}{proposition}{propCGMT}
% % \begin{proposition} 
% \label{prop:CGMT_application}
%     % Denote $\gennormboundp = \gennormbound + \norm{w^*}_1$. % CONVENTION 1
%     %Denote $\gennormboundp =  \gennormbound + 2\norm{w^*}_1$. % CONVENTION 2
%     For $\Hgaussian \sim \NNN(0,I_n), \Ggaussian \sim \NNN(0,I_d)$ define the stochastic auxiliary optimization problems:
%         \begin{align}
%         \tag{$A_N$} \label{eq:phin}
%             \phidn &= \min_{(\wone,\wtwo)} \norm{\wone+\wgt}_p^p+\norm{\wtwo}_p^p
%             \subjto \frac{1}{n} \innerprod{\wtwo}{\Hgaussian}^2 \geq  \fn(\|\wone\|_2,\|\wtwo\|_2) \\
%         \tag{$A_+$} \label{eq:phip}
%             \phidp &= \max_{(\wone,\wtwo)} \abs{\wone }^2 + \|\wtwo\|_2^2
%             \subjto \begin{cases}
%                 \frac{1}{n} \innerprod{\wtwo}{\Hgaussian}^2 \geq  \fn(\|\wone\|_2,\|\wtwo\|_2)\\
%               \abs{\wone+\wgt}^p+\norm{\wtwo}_p^p \leq \lonebound
%             \end{cases}\\
%         \tag{$A_-$} \label{eq:phim}
%             \phidm &= \min_{(\wone,\wtwo)} \abs{\wone }^2 + \|\wtwo\|_2^2
%             \subjto \begin{cases}
%               \frac{1}{n} \innerprod{\wtwo}{\Hgaussian}^2 \geq  \fn(\|\wone\|_2,\|\wtwo\|_2) \\
%               \abs{\wone+\wgt}^p+\norm{\wtwo}_p^p  \leq \lonebound
%             \end{cases}
%         \end{align}
%     where $\lonebound>0$ is a constant such that $\lonebound\geq \phidn$.
%     For regression, we choose $f_n = \|\xi - \Xone \wone - G \|\wtwo\|_2 \|_2^2$ and for classification, choose $\fn(x,y) = \frac{1}{n} \sumin \possq{1-\xi_i\abs{\Xone_i}x-\Ggaussian_i y}$.
%     Then, for both  $\Phi = \Phi^{C}$ and $\Phi = \Phi^{R}$, we have that for any$t \in \RR$:
%         \begin{align}
%             \PP( \Phi_N > t \vert \xi,  \Xone ) &\leq 2\PP( \phidn \geq t \vert \xi, \Xone)
%             \label{eq:probeq1} \\
%             \PP( \Phi_+ > t \vert \xi,\Xone) &\leq 2\PP( \phidp \geq t \vert \xi, \Xone) 
%             \label{eq:probeq2} \\
%             \PP( \Phi_- < t \vert \xi, \Xone) &\leq 2\PP( \phidm \leq t \vert \xi, \Xone) 
%             \label{eq:probeq3} ,
%         \end{align}
%         where the probabilities on the left and on the right are over the draws of $\{x_i\}_{i=2}^n$ and of $\Ggaussian,\Hgaussian$ respectively.
% \end{restatable}   

% Following the work in \cite{konst} we can recast \eqref{eq:phin}, \eqref{eq:phip}, \eqref{eq:phim} as optimization problems in three scalar variables. Let $b,\alpha$ be scalar variables with $b\geq 0$, $\alpha\in[1,\alpham]$ with $\alpham = \tilded\frac{\norm{\Hgaussian}_{\infty}}{\norm{\Hgaussian}_1}$. Then we define parametric path $b\gamma(\alpha)$ with $\RR^\tilded$-valued function $\gamma$ given by:
% \begin{equation}
%     \gamma(\alpha) = \argmin_{\wtwo} \norm{\wtwo}_2^2
%     \subjto \begin{cases}
%                 \innerprod{\wtwo}{\Hgaussian} \geq \norm{\Hgaussian}_{\infty}\\
%                 \wtwo\geq 0\\
%                 \transp{\onevec} \wtwo = \norm{\wtwo}_1 = \alpha
%             \end{cases}
% \end{equation}
% \begin{restatable}{proposition}{propparam}
% % \begin{proposition} 
% \label{prop:parametrization}
% Optimization problems \eqref{eq:phin}, \eqref{eq:phip}, \eqref{eq:phim} are equivalently given by:
%         \begin{align}
%         \tag{$A_N$}\label{eq:phin}
%             \phidn &= \min_{\nu,b,\alpha} \nu + \alpha b
%             \subjto \frac{1}{n}  b^2\norm{\Hgaussian}_{\infty}^2  \geq  \fn(\|\wone\|_2,b\|\gamma(\alpha)\|_2). \\
%         \tag{$A_+$} \label{eq:phip}
%             \phidp &= \max_{\nu,b,\alpha}  \frac{\nu}{\sqrt{\nu^2+b^2\norm{\gamma(\alpha)}_2^2}}
%             \subjto \begin{cases}
%               \frac{1}{n}  b^2\norm{\Hgaussian}_{\infty}^2  \geq  \fn(\|\wone\|_2,b\|\gamma(\alpha)\|_2)\\
%                 \nu+b  \leq \lonebound
%             \end{cases}\\
%         \tag{$A_-$} \label{eq:phim}
%             \phidm &= \min_{\nu,b,\alpha}  \frac{\nu}{\sqrt{\nu^2+b^2\norm{\gamma(\alpha)}_2^2}}
%             \subjto \begin{cases}
%               \frac{1}{n}  b^2\norm{\Hgaussian}_{\infty}^2  \geq  \fn(\|\wone\|_2,b\|\gamma(\alpha)\|_2)\\
%                 \nu+b \leq \lonebound
%             \end{cases}
%         \end{align}
% for some scalars $\nu,b>0$ and $\alpha\in[1,\alpham]$.

% \end{restatable}   





==> ICML 22-3/sections_proof/L_gamma_conc.tex <==

% \onecolumn

% \begin{lemma}
% (Concentration of norms of $\gamma(\alpha_s)$, proposition 4 in \cite{konst}) Let $\ts$ be given by $2\Phic(\ts) = s/d$. There exists universal positive constants $c,c_s,c_l,c_u>0$ such that for any $s,d$ with $s\geq c_s$ and $c_ls\leq d\leq \exp(c_u s^{1/5})$ we have that:
%     \begin{align}
%         \abs{
%             \frac{\norm{\gamma(\alphathr{s})}_1}{\norm{\Hgaussian}_\infty} - \left(\frac{1}{\ts} - \frac{2}{\ts^3}\right)
%         }
%         &\leq \frac{c}{\ts^5}
%         \qquad \andtxt \qquad
%         \abs{
%             \frac{\norm{\gamma(\alphathr{s})}_2^2}{\norm{\Hgaussian}_\infty^2} - \frac{2}{s \ts^2}
%         }
%         \leq \frac{c}{s \ts^4}, \label{eq:concentration}
%     \end{align}
% with probability at least $1-6\exp\left(-\frac{s}{\log(d/s)^5}\right)$ over the draws of $h$.
% \label{lemma_gamma_conc}
% \end{lemma}




==> ICML 22-3/sections_proof/TL1_quadratic_bound_fn.tex <==

% \onecolumn


Throughout this section, for simplicity of the notation, we abbreviate $\{\xui'\}_{i=1}^n$ as $\gausswone$ and $G$ from Proposition~\ref{prop:CGMT_application_classification} as $\gausswtwo$. Thus, we have $\fnclas (\nu, \eta) := \frac{1}{n} \sumin \possq{ 1 - \xi_i \abs{\gausswone_i} \nu - \eta \gausswtwo_i }$ and  
\begin{equation}
\label{eq:defoff}
    \fclas(\nu,\eta) :=  \EE \fnclas(\nu,\eta) = \EE_{Z_1,Z_2 \sim \NNN(0,1)} \EE_{\xi \sim \probsigma(\cdot; Z_1)} \left( 1- \xi \nu \vert Z_1 \vert - \eta Z_2\right)_+^2.  
\end{equation}


\subsection{Lower bounding \texorpdfstring{$\fnclas$}{fn} by a quadratic form}
\label{apx:subsec:quadratic_bound_fn}
  We show the following lemma.
\begin{lemma} \label{quadratic_bound_fn}
    There exist universal positive constants $\constnu, \consteta$ only depending on $\probsigma$ and $c$ such that for any $\nu,\eta$ we have that: 
        \begin{align}
        \label{eq:quadratic_bound_fn}
            \fnclas(\nu,\eta) \geq \constnu \nu^2  + \consteta \eta^2
        \end{align}
    with probability at least $1 - \exp \left( -cn \right)$ over the draws of $\gausswone,\gausswtwo,\xi$.
\end{lemma}

\begin{proof}
 We can assume that $\nu ,\eta \geq 0$ as the other cases follow from exactly the same argument. 
 First we show an auxiliary statement which we use later in the proof. Namely, we claim that there exists some positive constant $c_1$ such that for all $z \in [z_1,z_2]$,  $\probsigma \left( \xi = -1; z \right) > c_1$ for some $z_1, z_2 \in \RR$ and $z_1\neq z_2$. Let's prove this statement by contradiction and assume that there exists no $z \in [z_1,z_2]$ which satisfy the previous equation. Then, for almost any $z \sim N(0,1)$, we have $\probsigma (\xi; z) = +1$ and hence the minimum of the function $\fclas(\nu, \eta) = \EE \fnclas (\nu, \eta)$ is obtained for $\nu = \infty$. However, this is in contradiction with the assumption on $\probsigma$ in Section \ref{subsec:clasetting}. Hence there exists some $z$ for which $\prob \left( \xi = -1;  z \right) > c_1$. By the assumption on $\probsigma$ in Section \ref{subsec:clasetting} we assume piece-wise continuity of $z \to \probsigma(\xi=-1;z)$ and hence there exists some interval $[z-\delta, z+\delta] =: [z_1,z_2]$ in which the given probability is bounded away from zero. 

We can assume without loss of generality that this interval does not contain zero, since in that case we can always define a new interval of the form $[\epsilon, z_2]$ or $[z_1, -\epsilon]$ for $\epsilon>0$ small enough, which does not contain zero. Let's define $\tilde{z} = \max \{ \abs{z_1}, \abs{z_2} \}$.

 We can now bound $\fnclas(\nu,\eta)$ as follows:
\begin{align}
    \fnclas(\nu,\eta) 
    & =
    \frac{1}{n} \sumin \possq{ 1 - \xi_i \abs{\gausswone_i} \nu - \eta \gausswtwo_i }
    \geq
    \frac{1}{n}\sumin \idvec \left[ \xi_i = -1, \gausswone \in [z_1,z_2], \gausswtwo < - c_2 \right] \possq{ 1 - \xi_i \abs{\gausswone_i} \nu - \eta \gausswtwo_i }
    \\
    & \geq \left( 1 + \tilde{z} \abs{\nu} + c_2 \eta \right)^2 \frac{1}{n}\sumin \idvec \left[ \xi_i = -1, \gausswone_i \in [z_1,z_2], \gausswtwo_i < -c_2 \right]
\end{align}
for arbitrary positive constant $c_2$.
From section \ref{apx:subsec:gmtclas} we have that $\gausswtwo$ is independent of $\xi$ and $\gausswone$ and hence:
\begin{align}
    \prob \left( \xi = \sign (\nu), \gausswone \in [z_1,z_2], \gausswtwo < - c_2 \right) 
    &=
    \prob \left( \xi = \sign (\nu) \vert \gausswone \in [z_1,z_2]\right) \prob \left( \gausswone \in [z_1,z_2] \right) \prob \left( \gausswtwo < - c_2 \right)
    \\
    &\geq
    c_1 \left( \Phic(z_1) - \Phic(z_2) \right) \Phic(c_2) 
    \geq
    c
\end{align}
for some positive constant $c$. Now using concentration of i.i.d. Bernoulli random variables we obtain:
\begin{align}
    \fnclas (\nu,\eta) \geq \left( 1 + \tilde{z}\abs{\nu} + c_2 \eta \right)^2 \frac{c}{2} 
    \geq
    \frac{\tilde{z}^2 c_3}{2} \nu^2 + \frac{c_2^2 c_3}{2} \eta^2
    % \prob \left( \xi = \sign (\nu), \gausswone \in [z_1,z_2], \gausswtwo > \kappa_2 \right) 
\end{align}
with universal constant $c_3>0$ and with probability at least $ 1 - \exp \left( - n D (c || \frac{c}{2} ) \right) \geq 1 - \exp \left( - n c\right)$.
\end{proof}



% \begin{lemma} \label{quadratic_bound_fn}
%     There exist positive constants $\constnu$ and $\consteta$ such that for any $\nu,\eta$ we have that: 
%         \begin{align}
%             \fnclas(\nu,\eta) \geq \constnu \nu^2  + \consteta \eta^2
%         \end{align}
%     with probability at least $1 - \exp \left( - n \kldiv{\frac{\sigma}{2}}{\frac{\sigma}{4}} \right) - \exp \left( -\frac{ n\sigma }{ 128 } \right)$ over the draws of $\gausswone,\gausswtwo,\xi$.
% \end{lemma}

% \begin{proof}
% Denote by $\kldiv{\delta}{\alpha}$ Kullback-Leibler divergence between two parameters $\alpha \in (0,1/2]$ and $\delta \in (0,\alpha)$. We use concentration result for i.i.d. Bernoulli random variables $x_i$'s with parameter $\alpha$ which states that $\prob \left( \frac{1}{n} \sumin x_i \geq \delta \right) \geq 1 - \exp \left ( - n \kldiv{\delta}{\alpha} \right) $. Note first that $\sign (\gausswtwo)$ is a Bernoulli random variable (after mapping all $-1$'s to $0$'s). We now want to condition on the event that at least $k$ of $n$ samples satisfy that $\gausswtwo_i < 0$ and $\xi_i < 0$ if $\nu > 0$ and $\xi_i > 0$ if $\nu < 0$. Under this event we have that:
% \begin{align}
%     \fnclas (\nu, \eta) = \frac{1}{n} \sumin \possq{ 1 - \xi_i \abs{\gausswone_i} \nu - \gausswtwo_i \eta } 
%     \geq
%     \frac{1}{n} \sum_{i=1}^k \left( 1 + \abs{\gausswone_i \nu} + \abs{ \gausswtwo_i} \eta \right)^2
%     \geq
%     \frac{1}{n} \sum_{i=1}^k \left( 1 + \gausswone_i \abs{\nu} + \gausswtwo_i \eta \right)^2
%     \label{eq:fnbound}
% \end{align}

% Define a random variable $\chi$ which is Bernoulli with parameter $\sigma/2$. It is easy to see that event described above appears with probability at least as big as $\prob ( \sumin \chi_i \geq k )$. Choose $\delta = \sigma/4$ to get that $\prob ( \frac{1}{n} \sumin \chi_i \geq \sigma/4) \geq 1 - \exp \left( - n \kldiv{\frac{\sigma}{2}}{\frac{\sigma}{4}} \right) $. Hence we choose that $k = \bfloor{\frac{n\sigma}{4}}$ and condition on this even with probability $1-\exp \left( -n c_{\sigma} \right)$.

% Now note that terms inside the brackets in \eqref{eq:fnbound} are normally distributed according to $\NNN ( 1 , 1 + \nu^2 + \eta^2 )$. Hence squaring these Gaussian r.v. we get sub-exponential random variables and we will use concentration result for sub-exponential variables. Let $Y =  1 + \Gausswone \abs{\nu} + \Gausswtwo \eta $ and $X = Y^2$. First note that each of the terms in the sum is sub-exponential with parameters $(2,4)$ since:
% \begin{align}
%     \EE &\left[ \exp \left( \lambda(X-(1+\nu^2+\eta^2)) \right) \right] = \frac{1}{\sqrt{2\pi}} \int \exp \left( \lambda(y^2-(1+\nu^2+\eta^2)) \right) \exp \left( -\frac{y^2}{2} \right) dy 
%     \\
%     &=
%     \frac{ \exp \left( -\lambda (1+\nu^2+\eta^2) \right) }{\sqrt{ 1 - 2\lambda }}
%     \leq
%     \frac{ \exp \left( -\lambda \right) }{\sqrt{ 1 - 2\lambda }} 
%     \leq
%     \exp \left( \frac{4 \lambda^2}{2} \right)
% \end{align}
% for all $\abs{\lambda} < \frac{1}{4}$. Now we have that $\sum_{i=1}^k Y_k^2$ is sub-exponential with parameters $(2\sqrt{k},4)$ implying the following tail bound:
% \begin{align}
%     \prob \left( (1+\nu^2+\eta^2) - \frac{1}{k} \sum_{i=1}^k Y_k^2 \geq t \right) \leq \exp \left( -\frac{ k t^2 }{ 8 } \right)
% \end{align}
% for all $t\in(0,1)$. Now choosing $t=1/2$ we get the following result:
% \begin{align}
%     \fn (\nu, \eta) \geq \bfloor{\frac{\sigma}{4}} \frac{1}{k}\sum_{i=1}^k \left( 1 + \gausswone_i \abs{\nu} + \gausswtwo_i \eta \right)^2 \geq \bfloor{\frac{\sigma}{4}} ( 1 + \nu^2 + \eta^2 - \frac{1}{2}) =  \bfloor{\frac{\sigma}{4}} \nu^2 +  \bfloor{\frac{\sigma}{4}} \eta^2
% \end{align}
% with probability at least $1 - \exp \left( - n \kldiv{\frac{\sigma}{2}}{\frac{\sigma}{4}} \right) - \exp \left( -\frac{ n\sigma }{ 128 } \right)$
% \end{proof}



==> ICML 22-3/sections_proof/TL2_quadratic_plus_fstar_bound.tex <==


% \onecolumn

\subsection{Lower bounding \texorpdfstring{$\fnclas$}{fn} by a quadratic form with constant}
\label{apx:subsec:quadratic_plus_fstar_bound}
We use the notation as described in Appendix~\ref{apx:subsec:localisationproofcla} and the beginning of Appendix~\ref{apx:technicallemmas}.
 We show the following lemma. 
\begin{lemma} \label{lemma_quadratic_plus_fstar_bound}
    Let $\boundnuone, \boundetaone>0$ be two positive constants. Then, there exist positive constants $\tconstnu,\tconsteta>0$ and $c_1, c_2,c_3 >0$ only depending on $\probsigma$, such that for any $\epsilon \geq  c_1 \sqrt{\frac{\log(n)}{n}}$ and any $\nu \leq \boundnuone, \eta \leq \boundetaone$ we have that: 
        \begin{align}
        \label{eq:quadratic_plus_fstar_bound}
            \fnclas(\nu,\eta) \geq \fstar + \tconstnu \left( \deltanu \right)^2  + \tconsteta \eta^2 - \epsilon
        \end{align}
    with probability at least $1 - c_2 \exp \left( - \frac{c_3 n \epsilon^2}{\log(n)}  \right)$ over the draws of $\gausswone,\gausswtwo,\xi$.
\end{lemma}
%\fy{what is $\zeta$?, couldn't find the def in Appendix F so have to redefine at least?}
\begin{proof}
First note that from the uniform convergence result in Proposition \ref{prop:unifConv} we have that $\fclas(\nu,\eta) \geq \fnclas(\nu,\eta) - \epsilon$, with $f$ from Equation~\eqref{eq:defoff}, with probability at least $1 - c_2 \exp \left( - \frac{c_3 n\epsilon^2}{\log(n)}  \right)$. Thus, it is sufficient to study $\fclas$.  Clearly, by the convexity of $\fclas$ we have that $\fclas \geq \fstar$ with $\fstar = \fclas(\nubar, 0)$ where we use the simple fact that $(\nubar, 0)$ is the global minimizer of $\fclas$, which follows from the  assumption on $\probsigma$ in Section \ref{subsec:clasetting}. 
Furthermore, it is not difficult to check that for for any $\nu,\eta$, $\nabla^2 \fclas(\nu,\eta) \succ 0$ and therefore, $\fclas$ is strictly convex on every compact set. Hence, the proof follows. 
% Hence, $f$ attains its minimum $\fstar$ on the compact set given by bounded sets of $\nu \leq \boundnuone$ and $\eta \leq \boundetaone$. As stated in assumption (A1), $\fstar$ is attained at some point $(\nubar,0)$ with $\nubar>0$. Hence we have $f(\nu,\eta)-\fstar \geq 0$.Hence Lemma \ref{quadratic_bound_fn} implies that $f(\nu,\eta) + \epsilon \geq \constnu \nu^2 + \consteta \eta^2$. Now define:
% \begin{align}
%     \tconstnu = \min_{\nu,\eta} \frac{f(\nu,\eta)-\fstar + \epsilon}{2\deltanu^2}
%     \quad
%     \andtxt
%     \quad
%     \tconsteta = \min_{\nu,\eta} \frac{f(\nu,\eta)-\fstar + \epsilon}{2 \eta^2}
% \end{align}
% which are positive and finite constants since $f(\nu, \eta)+\epsilon>\fstar$ and $f$ grows at least quadratically in $\nu$ and $\eta$, respectively. It is simple to check that these constants indeed satisfy inequality above.
\end{proof}



==> ICML 22-3/sections_proof/TL3_uniform_convergence_fn.tex <==
\subsection{Uniform convergence of $\fnclas$ to $\fclas$}
\label{apx:subsec:unif_conv}
We use the notation as described in the beginning of Appendix~\ref{apx:technicallemmas} and denote with $\Gausswone,\Gausswtwo \sim \Normal(0,1)$ independent Gaussian random variables and let $\xirv \vert \Gausswone \sim \probsigma(.;\Gausswone)$. 

Let $P$ be the distribution of $(\Gausswone,\Gausswtwo,\xirv)$ and let $P_n = \frac{1}{n} \sumin \delta_{\gausswone_i,\gausswtwo_i,\xi_i}$. Define $\gnueta(Z,\xi) = \possq{1-\xirv \abs{\Gausswone}\nu - \eta\Gausswtwo}$ with $Z = (\Gausswone, \Gausswtwo)$. Note that using this notation, we have $P\gnueta = \EE \gnueta(Z,\xi) = \fclas (\nu,\eta)$, with $f$ from Equation~\eqref{eq:defoff}, and $P_n \gnueta = \fnclas(\nu,\eta)$. Let $\GB = \left\{ \gnueta\ |\ \nu \leq \boundnuone, \eta \leq \boundetaone \right\}$ with positive constants $\boundetaone$ and $\boundnuone$. Moreover define:
\begin{align}
    \norm{ P_n - P }_{\GB} := \sup_{\gnueta \in \GB} \abs{(P_n - P)\gnueta}
\end{align}
We then obtain from an application of Theorem 4 in \cite{adamczak2008tail} the following uniform convergence result
\begin{proposition}
\label{prop:unifConv}
There exist positive universal constants $c_1,c_2,c_3>0$ such that
    % \begin{align}
    %     \prob \left( \norm{ P_n - P }_{\GB} \leq t \right) \geq 1 - \exp \left( - \frac{ n t^2 }{2 ( 1 + \delta ) c_{\sigma} \left( \boundnuone^4 + \boundetaone^4 \right) } \right) - 3\exp \left( -\frac{ n t }{C c_\psi \log n} \right)
    % \end{align}
    \begin{align}
        \prob \left( \norm{ P_n - P }_{\GB} \leq \frac{c_1}{\sqrt{n}} + \epsilon \right) 
        \geq
        1 - c_2\exp \left( -c_3 \frac{ n \epsilon^2 }{\log n} \right)
    \end{align}
\end{proposition}

\begin{proof}

The proof follows from an application of the tail-bound result from Theorem 4 in \cite{adamczak2008tail}. More precisely, 

\begin{theorem}[Corollary of Theorem 4 in \cite{adamczak2008tail}]
\label{thm:unifconvmain}
For any $0<t<1$, $\delta>0$, $\alpha \in (0,1] $ there exists a constant $C = C ( \alpha, t, \delta )$ such that
\begin{align}
\label{eq:tailuniformconv}
    \prob \left( \norm{ P_n - P }_{\GB} \geq (1+t) \EE \norm{ P_n - P }_{\GB} + \epsilon \right)
    \leq
    \exp & \left( -\frac{\epsilon^2}{2(1+\delta)\sigma_{\GB}^2} \right) + 3 \exp \left( - \left( \frac{\epsilon}{C \psi_{\GB}} \right)^{\alpha} \right)
\end{align}
with variance term 
\begin{equation}
    \sigma_{\GB}^2 :=  \sup_{ \gnueta \in \GB } \frac{1}{n}\left( \EE \left[ \gnueta^2 \right] - \left( \EE \left[ \gnueta \right] \right)^2 \right),
\end{equation}
and $\psi_{\GB}$ defined as:
\begin{align}
    \psi_{\GB} = \orlicznorm{\max_{1\leq i\leq n} \sup_{\gnueta \in \GB} \frac{1}{n} \left\vert\gnueta(z_i,\xi_i) - \EE [\gnueta] \right\vert}
\end{align}
where $\orlicznorm{\cdot}$ denotes Orlicz norm. 
\end{theorem}

We choose $\alpha = 1$ and explicitly show that condition from Theorem 4 in \cite{adamczak2008tail} requiring finite Orlicz norms is indeed satisfied for this choice of $\alpha$.
We separate the proof into two steps, where in a first step we bound the $ \psi_{\GB}$ and then apply Theorem~\ref{thm:unifconvmain}. 

\paragraph{Step 1: Bounding $\psi_{\GB}$}

By the definition of Orlicz norms, $\psi_{\GB}$ is given by:
\begin{align}\label{eq_psi_GB_def}
    &\psi_{\GB} 
     =
    \orlicznorm{ \max_{1 \leq i \leq n} \sup_{\nu,\eta} \frac{1}{n} \abs{ \possq{ 1 - \xi_i \abs{\gausswone_i} \nu - \gausswtwo_i \eta } - \EE \left[ \possq{ 1 - \xi \abs{\gausswone} \nu - \gausswtwo \eta } \right] } } 
    \\ 
    & = \inf \left\{ \lambda>0:\ \EE \left[ \exp \left( \frac{1}{\lambda} \max_i \sup_{\nu,\eta} \frac{1}{n}
    \abs{ \possq{ 1 - \xi_i \abs{\gausswone_i} \nu - \gausswtwo_i \eta} - \EE \left[ \possq{ 1 - \xi \abs{\gausswone} \nu - \gausswtwo \eta } \right] } \right) - 1 \right] \leq 1\right\}
\end{align}
Applying the triangle inequality and using that $\nu,\eta$ are bounded by constants, we can bound the expectation from the expression above as:
\begin{align}
    & \EE \left[ \exp \left( \frac{1}{\lambda} \max_i \sup_{\nu,\eta} \frac{1}{n}
    \abs{ \possq{ 1 - \xi_i \abs{\gausswone_i} \nu - \gausswtwo_i \eta} - \EE \left[ \possq{ 1 - \xi \abs{\gausswone} \nu - \gausswtwo \eta } \right] } \right) \right]
    \\
    & \leq 
    % \EE \left[ \exp \left(  \frac{1}{n\lambda} \max_i \sup_{\nu,\eta} 
    % \possq{ 1 - \xi_i \abs{\gausswone_i} \nu -  \gausswtwo_i \eta} + \frac{1}{n\lambda}\sup_{\nu,\eta} \EE \left[ \possq{ 1 - \xi \abs{\gausswone} \nu - \gausswtwo \eta } \right]  \right) \right]
    % \\
    % & = 
    \EE \left[ \exp \left(  \frac{1}{n\lambda} \max_i \sup_{\nu,\eta} 
    \possq{ 1 - \xi_i \abs{\gausswone_i} \nu -  \gausswtwo_i \eta} \right) \right]
     \exp \left( \frac{1}{n\lambda}\sup_{\nu,\eta} \EE \left[ \possq{ 1 - \xi \abs{\gausswone} \nu - \gausswtwo \eta } \right] \right) 
    \\
    & \leq
    \EE \left[ \exp \left(  \frac{B}{n\lambda}\zmax^2 \right) \right] \exp \left( \frac{B}{n\lambda} \right)  
\end{align}
with $B := 3\left( 1 + \boundnuone^2 + \boundetaone^2 \right)$ and $z_{(1)} = \max_{1\leq i\leq 2n} z_i = \max \left\{ \abs{\gausswone_1},\abs{\gausswtwo_1},\dots,\abs{\gausswone_n},\abs{\gausswtwo_n} \right\}$. Now we split the expectation from the above inequality into two terms:
\begin{align}
   \tilde{T}_1 = \EE \left[\onevec[\zmax< \sqrt{2 \log n}] \exp \left(  \frac{B}{n\lambda}\zmax^2 \right) \right]
%   &= \int_{-\sqrt{2\log n}}^{\sqrt{2\log n}}\cdots\int_{-\sqrt{2\log n}}^{\sqrt{2\log n}} \exp \left( \frac{B}{n\lambda}  \zmax^2 \right) \prod_{i=1}^{2n} \frac{ \exp \left( -\frac{1}{2} z_i^2 \right) }{\sqrt{2\pi}}dz_i
   \leq
   \exp \left( \frac{2B\log n}{n\lambda} \right)
\end{align}
and
\begin{align}
    \tilde{T}_2 
    &=
    \EE \left[\onevec[\zmax\geq \sqrt{2 \log n}] \exp \left(  \frac{B}{n\lambda}\zmax^2 \right) \right]
    =
    4n \int_{\sqrt{2 \log n}}^{\infty} \int_{-z_1}^{z_1} \cdots \int_{-z_1}^{z_1} \exp \left( \frac{B}{n\lambda}  z_1^2 \right) \prod_{i=1}^{2n} \frac{\exp(-\frac{1}{2}z_i^2)}{\sqrt{2\pi}} dz_i
    \\
    &\leq
    4n \int_{\sqrt{2 \log n}}^{\infty} \frac{1}{\sqrt{2\pi}} \exp \left( -\frac{1}{2} z_1^2 \right) \exp \left( \frac{B}{n\lambda} z_1^2 \right) dz_1 
    \lesssim
    \frac{n^{\frac{2B}{n\lambda}}}{\sqrt{\log n}(1-\frac{2B}{n\lambda})}
\end{align}
where we assumed that $\lambda > \frac{2B}{n}$. Now choosing $\lambda = c_{\lambda} \frac{\log n}{n}$ with a positive constant $c_{\lambda}$ sufficiently large, we find that the condition in Equality \eqref{eq_psi_GB_def} is satisfied for this $\lambda$, which implies that $\psi_{\GB} \leq c_{\lambda}\frac{\log n}{n}$.
\paragraph{Step 2: Proof of the statement}
To apply Theorem~\ref{thm:unifconvmain}, we also need to bound the variance $\sigma_{\GB}^2$ and use that $\EE \norm{P_n-P}_{\GB} \leq 2 \rademacher(\GB)$  where $ \rademacher(\GB)$ is the Rademacher complexity given by $\rademacher(\GB) = \EE \left[ \sup_{\gnueta\in \GB} \left|\frac{1}{n}\sumin \epsilon_i g_{\eta,v}(z_i,\xi_i) \right| \right]$. 
The bound on the variance follows from a straightforward calculation:
\begin{align}
    \sigma_{\GB}^2
   % & =  \sup_{ \gnueta \in \GB } \frac{1}{n}\left( \EE \left[ \gnueta^2 \right] - \left( \EE \left[ \gnueta \right] \right)^2 \right)
    \leq 
    \frac{1}{n} \sup_{ \gnueta \in \GB } \EE \left[ \gnueta^2 \right]
    % \leq
    % \frac{1}{n} \EE \left[ 1 + \boundnuone \nu + \boundetaone \eta \right]^4 
    \leq
    \frac{1}{n} c_{\sigma_{\GB}} \left( 1 + \boundnuone^4 + \boundetaone^4 \right)
\end{align}
which holds for some positive universal constant $c_{\sigma_{\GB}}>0$. 

Next, note that we can upper bound the Rademacher complexity using the triangle inequality and the fact that $(\cdot)_+$ is $1$-Lipschitz:
\begin{align}
     \rademacher(\GB) &\leq 
    \EE \left[\sup_{\nu\leq \boundnuone,\eta\leq \boundetaone}\left| \frac{1}{n}\sumin \epsilon_i (1-\xi_i \abs{\gausswone_i}\nu - \eta\gausswtwo_i)^2\right| \right] 
    \\ 
    &\lesssim \EE \left[ \sup_{\nu\leq \boundnuone,\eta\leq \boundetaone}\left| \frac{1}{n}\sumin \epsilon_i\right| \right] +  \EE \left[ \sup_{\nu\leq \boundnuone,\eta\leq \boundetaone}\left| \frac{1}{n}\sumin \epsilon_i (\xi_i \abs{\gausswone_i}\nu)^2\right| \right] \\
    &+  \EE \left[ \sup_{\nu\leq \boundnuone,\eta\leq \boundetaone}\left| \frac{1}{n}\sumin \epsilon_i ( \eta\gausswtwo_i)^2\right| \right] 
    \lesssim \frac{1}{\sqrt{n}}
\end{align}
where the last line follows from applying the standard concentration results. Thus, we obtain:
    \begin{align}
        % \prob \left( \norm{ P_n - P }_{\GB} \geq \kappa_1 \sqrt{\frac{\log(n)}{n}} + t \right) 
        \prob \left( \norm{ P_n - P }_{\GB} \geq 2(1+t) \mathcal{R}_{\GB} + \epsilon \right) 
        \leq
        \exp \left( - c_2 n \epsilon^2 \right) + 3\exp \left( -c_3 \frac{ n \epsilon }{\log n} \right)
    \end{align}
with $c_2^{-1} = 2(1+\delta)c_{\sigma_{\GB}} B^2$ and $c_3^{-1} = C c_{\lambda}$, which concludes the proof. 

%Recalling result from Lemma \ref{lm:rademacher} concludes the proof.
\end{proof}
















% In the following Section~\ref{sec:rademacher} we give an upper bound on the Rademacher complexity of $\GB$ denoted by $\mathcal{R}_n(\GB)$, which we then use for proving Proposition \ref{prop:unifConv} in Section \ref{sec_proof_unifconv}.

% \subsubsection{Rademacher complexity}\label{sec:rademacher}
% \begin{lemma}
% \label{lm:rademacher}
% There exists universal positive constant $\kappa$ such that Rademacher complexity of $\GB$ satisfies: 
% \begin{align}
%     \mathcal{R}_n(\GB)\leq \kappa \sqrt{\frac{\log n}{n}}
% \end{align}
% \end{lemma}
% \begin{proof}
% Let's denote by $\epsilon_1,\dots,\epsilon_n$ i.i.d. Rademacher random variables. From definition of Rademacher complexity follows that:
% \begin{align} \label{eq:rademacher_terms}
%     \RRR_n(\GB) &= \EE \left[ \sup_{\gnueta\in \GB} \left|\frac{1}{n}\sumin \epsilon_i g_{\eta,v}(z_i,\xi_i) \right| \right] \\
%     &= 
%   \underbrace{ \EE \left[\onevec[\zmax< B_n]\sup_{g_{\eta,v}\in \GB} \left| \frac{1}{n}\sumin \epsilon_i \gnueta(z_i,\xi_i) \right| \right] }_{T_1}
%     + \underbrace{\EE \left[\onevec[\zmax\geq B_n]\sup_{\gnueta\in \GB} \left| \frac{1}{n}\sumin \epsilon_i \gnueta(z_i,\xi_i) \right| \right]}_{T_2}
% \end{align}
% where $B_n$ is a bound term depending on $n$, which we choose appropriatelly in the following discussion and define $z_{(1)} = \max \left\{ \abs{\gausswone_1},\abs{\gausswtwo_1},\dots,\abs{\gausswone_n},\abs{\gausswtwo_n} \right\}$.

% Let's consider now the first term $T_1$ from equation \eqref{eq:rademacher_terms}. First note that function $(1-\xi \abs{\gausswone}\nu - \eta\gausswtwo)\mapsto (1-\xi \abs{\gausswone}\nu - \eta\gausswtwo)_+$ is Lipschitz with $L_1=1$ and $(1-\xi \abs{\gausswone}\nu - \eta\gausswtwo)_+ \mapsto \possq{1-\xi \abs{\gausswone}\nu - \eta\gausswtwo}$ is Lipschitz with $L_2 = 2(1+(\boundnuone+\boundetaone)B_n)$ conditioned on the event that $\zmax< B_n$. Now applying Theorem 12.4 from \cite{bartlett2002rademacher} we have: 
% % (if $\phi:\mathbb{R}\to \mathbb{R}$ is Lipschitz with constant $L_{\phi}$ and satisfies $\phi(0)=0$, then $R_n(\phi\circ F)\leq 2L_{\phi}R_n(F)$ for real function $F$) 
% \begin{align}
%     T_1 &\leq 
%     4 L_1 L_2 \EE \left[\sup_{\nu\leq \boundnuone,\eta\leq \boundetaone}\left| \frac{1}{n}\sumin \epsilon_i (1-\xi_i \abs{\gausswone_i}\nu - \eta\gausswtwo_i)\right| \right] 
%     \\ 
%     &\leq 8 \left( 1 + \left( \boundetaone + \boundnuone \right) B_n \right) \EE \left[ \sup_{\nu\leq \boundnuone,\eta\leq \boundetaone}\left| \frac{1}{n}\sumin \epsilon_i (1-\xi_i \abs{\gausswone_i}\nu - \eta\gausswtwo_i)\right| \right]
% \end{align}

% Applying triangle inequality to the obtained expression gives the following upper bound:
% \begin{align}
%     T_1 \leq 8 \left( 1 + \left( \boundetaone + \boundnuone \right) B_n \right) 
%     \left( \EE \left| \frac{1}{n}\sumin \epsilon_i \right|  
%     +
%     \boundnuone \EE \left| \frac{1}{n}\sumin \epsilon_i \xi_i \abs{\gausswone_i} \right| 
%     +
%     \boundetaone\EE \left| \frac{1}{n}\sumin \epsilon_i \gausswtwo_i \right| \right)
% \end{align}

% Now note that $\epsilon_i \xi_i \abs{\gausswone_i}, \epsilon_i \gausswtwo_i$ are i.i.d standard normal random variables. Then we use the fact that the absolute value of a Gaussian random variable with distribution $\NNN(0,\frac{1}{n})$ has half-normal distribution with mean $\sqrt{\frac{2}{\pi n}}$. After a straightforward calculation we get the same bound for the first term. Combining these results and choosing $B_n = \sqrt{2\log n}$ we have $T_1 \lesssim \sqrt{\frac{\log n}{n}}$. %with $c_1 = 10 \left( 1 + \boundnuone + \boundetaone \right)^2$.

% Now we consider the second term $T_2$ from equation \eqref{eq:rademacher_terms}.
% \begin{align} \label{eq:rademacher_second_term}
%     T_2 &= \sum_{i=1}^{2n} \EE \left[ \onevec\left[ \abs{z_i}\geq \abs{z_{j}}, \forall j\neq i \right] \onevec[\zmax \geq B_n]\sup_{\gnueta\in \GB} \left| \frac{1}{n}\sumin \epsilon_i \gnueta(z_i,\xi_i) \right| \right]
%     \\
%     & = 2n \int_{\abs{z_1}\geq \sqrt{2\log n}} \int_{-z_1}^{z_1}\cdots \int_{-z_1}^{z_1} \EE_{\xi,\epsilon} \left[ \sup_{\gnueta\in \GB} \left| \frac{1}{n}\sumin \epsilon_i \gnueta(z_i,\xi_i) \right| \right] \prod_{i=1}^{2n}\frac{1}{\sqrt{2\pi}}\exp \left( -\frac{z_i^2}{2} \right) dz_i
%     \\
%     & \leq 2 \int_{\abs{z_1}\geq \sqrt{2\log n}} \sup_{\gnueta\in \GB}  \gnueta(z_1,\xi_1)  \frac{1}{\sqrt{2\pi}}\exp \left( -\frac{z_1^2}{2} \right) dz_1 
%     \\
%     & +2n \int_{\abs{z_1}\geq \sqrt{2\log n}} \int_{-z_1}^{z_1}\cdots \int_{-z_1}^{z_1} \EE_{\xi,\epsilon} \left[ \sup_{\gnueta\in \GB} \left| \frac{1}{n}\sum_{i=2}^n \epsilon_i \gnueta(z_i,\xi_i) \right| \right] \prod_{i=1}^{2n}\frac{1}{\sqrt{2\pi}}\exp \left( -\frac{z_i^2}{2} \right) dz_i
%     \\
%     & \leq 4 \int_{\sqrt{2\log n}}^{\infty} \left( 1+ z_1 \left( \boundnuone + \boundetaone \right) \right)^2  \frac{1}{\sqrt{2\pi}}\exp \left( -\frac{z_1^2}{2} \right) dz_1  
%     \\
%     & +4n \int_{\sqrt{2\log n}}^{\infty} \EE_{\xi,\epsilon} \left[ 1\{\zmax \leq  z_1\}\sup_{\gnueta\in \GB} \left| \frac{1}{n-1}\sum_{i=2}^n \epsilon_i \gnueta(z_i,\xi_i) \right| \right]\frac{1}{\sqrt{2\pi}}\exp \left( -\frac{z_1^2}{2} \right) dz_1 =: T_{2,1} + T_{2,2}
% \end{align}

% We bound the first term $T_{2,1}$ as follows:
% \begin{align}
%     T_{2,1} &\leq 
%     % 4 \int_{\sqrt{2\log n}}^{\infty} \left( 1+z_1 \left( \boundnuone + \boundetaone \right) \right)^2  \frac{1}{\sqrt{2\pi}}\exp \left( -\frac{z_1^2}{2} \right) dz_1  
%     % \\
%     % &= 
%     4\left( \left( \boundnuone + \boundetaone \right)^2 + 1\right) \Phic ( \sqrt{2 \log n} ) + \frac{8}{\sqrt{2\pi}}( \boundnuone + \boundetaone ) \frac{1}{n} + \frac{4}{\sqrt{\pi}}( \boundnuone + \boundetaone)^2 \frac{\sqrt{\log n}}{n}
%     % \\
%     % &\leq \frac{1}{\sqrt{\pi}} \left( \left( \boundnuone + \boundetaone \right)^2 + 1\right) \frac{1}{n \sqrt{ \log n}} + \frac{8}{\sqrt{2\pi}}( \boundnuone + \boundetaone ) \frac{1}{n} + \frac{4}{\sqrt{\pi}}( \boundnuone + \boundetaone)^2 \frac{\sqrt{\log n}}{n}
%     % \\
%     % & \lesssim c_2 \frac{\sqrt{ \log n}}{n}
% \end{align}
% and using bound $\Phic(x) \leq \frac{\exp \left( -\frac{x^2}{2} \right)}{x\sqrt{2\pi}}$ (Fact 1 in \cite{wang2021tight}) we get $T_{2,1} \lesssim \frac{\sqrt{ \log n}}{n}$. For bounding second term $T_{2,2}$ we use result from first part of the proof that:
% \begin{align}
%     \EE \left[ \onevec[\zmax \leq  z_1]\sup_{\gnueta\in \GB} \left| \frac{1}{n-1}\sum_{i=2}^n \epsilon_i \gnueta(z_i,\xi_i) \right| \right] 
%     \leq \frac{\kappa_1 z_1}{\sqrt{n-1}}
% \end{align}
% to obtain:
% \begin{align}
%     T_{2,2} 
%     &\leq
%     \frac{4\kappa_1}{\sqrt{2\pi}} \frac{n}{\sqrt{n-1}} \int_{\sqrt{2\log n}}^{\infty} z_1 \exp \left( -\frac{z_1^2}{2} \right) dz_1 
%     =
%     \frac{4\kappa_1}{\sqrt{2\pi}} \frac{n}{\sqrt{n-1}} \exp \left(-\log n \right) 
%     % =
%     % \frac{4c_1}{\sqrt{2\pi}}\frac{1}{\sqrt{n-1}} 
%     \lesssim 
%     \frac{1}{\sqrt{n}}
% \end{align}

% Combining all previous results we get:
% \begin{align}
%     \RRR_n(\GB) 
%     \lesssim
%     \sqrt{\frac{\log n}{n}} + \frac{\sqrt{\log n}}{n} + \frac{1}{\sqrt{n}} 
%     \leq
%     \kappa \sqrt{\frac{\log n}{n}}
% \end{align}
% for some positive universal constant $\kappa$.
% \end{proof}



% \subsubsection{Proof of Proposition \ref{prop:unifConv}}\label{sec_proof_unifconv}
% % \begin{proof} 
% First we recall a tail bound result from Theorem 4 in \cite{adamczak2008tail}. Let $0<\epsilon<1$, $\delta>0$, $\alpha \in (0,1] $ and define constant $C = C ( \alpha, \epsilon, \delta )$. Then:
% \begin{align}
% \label{eq:tailuniformconv}
%     \prob \left( \norm{ P_n - P }_{\GB} \geq (1+\epsilon) \EE \norm{ P_n - P }_{\GB} + t \right)
%     \leq
%     \exp & \left( -\frac{t^2}{2(1+\delta)\sigma_{\GB}^2} \right) + 3 \exp \left( - \left( \frac{t}{C \psi_{\GB}} \right)^{\alpha} \right)
% \end{align}
% with variance term 
% \begin{equation}
%     \sigma_{\GB}^2 :=  \sup_{ \gnueta \in \GB } \frac{1}{n}\left( \EE \left[ \gnueta^2 \right] - \left( \EE \left[ \gnueta \right] \right)^2 \right),
% \end{equation}
% and $\psi_{\GB}$ defined as:
% \begin{align}
%     \psi_{\GB} = \orlicznorm{\max_{1\leq i\leq n} \sup_{\gnueta \in \GB} \frac{1}{n} \left\vert\gnueta(z_i,\xi_i) - \EE [\gnueta] \right\vert}
% \end{align}
% where $\orlicznorm{\cdot}$ denotes Orlicz norm. We choose $\alpha = 1$ and explicitly show that condition from Theorem 4 in \cite{adamczak2008tail} requiring finite Orlicz norms is indeed satisfied for this choice of $\alpha$.

% %  Note that we can control the term $ \EE \left[ \norm{ P_n - P }_{\GB} \right] \leq 2\RRR_n(\GB) $ using the upper bound on the Rademacher complexity in Lemma~\ref{lm:rademacher}. 
 
%  To bound the tail in Equation~\eqref{eq:tailuniformconv}, let's first bound the variance $\sigma_{\GB}^2$ for our setting:
% \begin{align}
%     \sigma_{\GB}^2
%   % & =  \sup_{ \gnueta \in \GB } \frac{1}{n}\left( \EE \left[ \gnueta^2 \right] - \left( \EE \left[ \gnueta \right] \right)^2 \right)
%     \leq 
%     \frac{1}{n} \sup_{ \gnueta \in \GB } \EE \left[ \gnueta^2 \right]
%     % \leq
%     % \frac{1}{n} \EE \left[ 1 + \boundnuone \nu + \boundetaone \eta \right]^4 
%     \leq
%     \frac{1}{n} \kappa_{\sigma_{\GB}} \left( 1 + \boundnuone^4 + \boundetaone^4 \right)
% \end{align}
% for some positive constant $\kappa_{\sigma_{\GB}}$. 


% By the definition of Orlicz norms, $\psi_{\GB}$ is  given by:
% \begin{align}\label{eq_psi_GB}
%     &\psi_{\GB} 
%      =
%     \orlicznorm{ \max_{1 \leq i \leq n} \sup_{\nu,\eta} \frac{1}{n} \abs{ \possq{ 1 - \xi_i \abs{\gausswone_i} \nu - \gausswtwo_i \eta } - \EE \left[ \possq{ 1 - \xi \abs{\gausswone} \nu - \gausswtwo \eta } \right] } } 
%     \\ 
%     & = \inf \left\{ \lambda>0:\ \EE \left[ \exp \left( \frac{1}{\lambda} \max_i \sup_{\nu,\eta} \frac{1}{n}
%     \abs{ \possq{ 1 - \xi_i \abs{\gausswone_i} \nu - \gausswtwo_i \eta} - \EE \left[ \possq{ 1 - \xi \abs{\gausswone} \nu - \gausswtwo \eta } \right] } \right) - 1 \right] \leq 1\right\}
% \end{align}
% Bounding the expectation from the expression above yields:
% \begin{align}
%     & \EE \left[ \exp \left( \frac{1}{\lambda} \max_i \sup_{\nu,\eta} \frac{1}{n}
%     \abs{ \possq{ 1 - \xi_i \abs{\gausswone_i} \nu - \gausswtwo_i \eta} - \EE \left[ \possq{ 1 - \xi \abs{\gausswone} \nu - \gausswtwo \eta } \right] } \right) \right]
%     \\
%     & \leq 
%     % \EE \left[ \exp \left(  \frac{1}{n\lambda} \max_i \sup_{\nu,\eta} 
%     % \possq{ 1 - \xi_i \abs{\gausswone_i} \nu -  \gausswtwo_i \eta} + \frac{1}{n\lambda}\sup_{\nu,\eta} \EE \left[ \possq{ 1 - \xi \abs{\gausswone} \nu - \gausswtwo \eta } \right]  \right) \right]
%     % \\
%     % & = 
%     \EE \left[ \exp \left(  \frac{1}{n\lambda} \max_i \sup_{\nu,\eta} 
%     \possq{ 1 - \xi_i \abs{\gausswone_i} \nu -  \gausswtwo_i \eta} \right) \right]
%      \exp \left( \frac{1}{n\lambda}\sup_{\nu,\eta} \EE \left[ \possq{ 1 - \xi \abs{\gausswone} \nu - \gausswtwo \eta } \right] \right) 
%     \\
%     & \leq
%     \EE \left[ \exp \left(  \frac{B}{n\lambda}\zmax^2 \right) \right] \exp \left( \frac{B}{n\lambda} \right)  
% \end{align}
% for constant $B := 2\left( 1 + \boundnuone^2 + \boundetaone^2 \right)$. Similarly as in equation \eqref{eq:rademacher_terms} we split the expectation above into two parts which we bound as follows:
% \begin{align}
%     \tilde{T}_1 &= \int_{-\sqrt{2\log n}}^{\sqrt{2\log n}}\cdots\int_{-\sqrt{2\log n}}^{\sqrt{2\log n}} \exp \left( \frac{B}{n\lambda}  \zmax^2 \right) \prod_{i=1}^{2n} \frac{ \exp \left( -\frac{1}{2} z_i^2 \right) }{\sqrt{2\pi}}dz_i
%     \leq
%     \exp \left( \frac{2B\log n}{n\lambda} \right)
% \end{align}
% and applying the same procedure as for term $T_2$ in the previous section we get:
% \begin{align}
%     \tilde{T}_2  &= 4n \int_{\sqrt{2 \log n}}^{\infty} \int_{-z_1}^{z_1} \cdots \int_{-z_1}^{z_1} \exp \left( \frac{B}{n\lambda}  \zmax^2 \right) \prod_{i=1}^{2n} \frac{\exp(-\frac{1}{2}z_i^2)}{\sqrt{2\pi}} dz_i
%     \\
%     &\leq
%     4n \int_{\sqrt{2 \log n}}^{\infty} \frac{1}{\sqrt{2\pi}} \exp \left( -\frac{1}{2} z_1^2 \right) \exp \left( \frac{B}{n\lambda} z_1^2 \right) dz_1 
%     % =
%     % \frac{4n}{\sqrt{2\pi}} \int_{\sqrt{2\log n}}^{\infty} \exp \left( -z_1^2 \left( \frac{1}{2}-\frac{B}{n\lambda} \right) \right) dz_1 = 
%     % \\
%     % &=
%     % \frac{4n}{\sqrt{1-\frac{2B}{n\lambda}}} \Phic \left( \sqrt{2 \left( 1-\frac{2B}{n\lambda} \right) \log n} \right)
%     \lesssim
%     % \frac{4n}{  1 - \frac{2B}{n\lambda}} \frac{ \exp \left( - \left( 1-\frac{2B}{n\lambda} \right) \log n \right) }{ \sqrt{ 2\pi }  \sqrt{2 \log n}}
%     % \\
%     % &= 
%     % \frac{2}{\sqrt{\pi}}
%     \frac{n^{\frac{2B}{n\lambda}}}{\sqrt{\log n}(1-\frac{2B}{n\lambda})}
% \end{align}
% where we assumed that $\lambda > \frac{2B}{n}$. Now choosing $\lambda = \kappa_{\lambda} \frac{\log n}{n}$ with positive constant $\kappa_{\lambda}$ sufficiently large, we obtain that condition in equality \eqref{eq_psi_GB} is satisfied for this $\lambda$ implying that $\psi_{\GB} \leq \kappa_{\lambda}\frac{\log n}{n}$.
% % and note that then we have:
% % \begin{align}
% %     \EE \left[ \exp \left(  \frac{2}{n\lambda} \left( 1 + \boundnuone^2 + \boundetaone^2 \right)\zmax^2 \right) \right] 
% %     \leq
% %     \exp \left( \frac{2}{c} \right) \left( 1 + \frac{2}{\sqrt{\pi} \left( 1-\frac{2}{c} \right)} \frac{1}{\sqrt{\log n}} \right)
% % \end{align}
% From equation \eqref{eq:tailuniformconv} and using $\EE \norm{P_n-P}_{\GB} \leq 2 \mathcal{R}(\GB)$  we obtain:
% % with constant $c_{\psi} = 2c ( 1 + \boundnuone^2 + \boundetaone^2)$ where $c$ satisfies condition:
% % \begin{align}
% %      \exp \left( \frac{c_1 ( \boundnuone^4 + \boundetaone^4) }{2 c ( 1 + \boundnuone^2 + \boundetaone^2 ) \log n} \right) \exp \left( \frac{2}{c} \right) \left( 1 + \frac{2}{\sqrt{\pi} \left( 1-\frac{2}{c} \right)} \frac{1}{\sqrt{\log n}} \right) \leq 2 
% % \end{align}
% % This completes the proof of uniform convergence.
% % \end{proof}
%     \begin{align}
%         % \prob \left( \norm{ P_n - P }_{\GB} \geq \kappa_1 \sqrt{\frac{\log(n)}{n}} + t \right) 
%         \prob \left( \norm{ P_n - P }_{\GB} \geq 2(1+\epsilon) \mathcal{R}_{\GB} + t \right) 
%         \leq
%         \exp \left( - \kappa_2 n t^2 \right) + 3\exp \left( -\kappa_3 \frac{ n t }{\log n} \right)
%     \end{align}
% with $\kappa_2^{-1} = (1+\delta)\kappa_{\sigma_{\GB}} B$ and $\kappa_3^{-1} = C \kappa_{\lambda}$. Recalling result from Lemma \ref{lm:rademacher} concludes the proof.

==> ICML 22-3/sections_proof/TL4_boundingfnlp.tex <==

\subsection{Tighter bound for \texorpdfstring{$\fnclas$}{fn} around \texorpdfstring{$(\nubarn, 0)$}{(nu,0)}}
\label{apx:subsec:prooffnlp}

% We use the notation as described in the beginning of Appendix~\ref{apx:claslpproof} where we defined 
% \begin{align}
% \label{eq:defineg1}
%     \fnstar &:= \min_{\nu} \fnclas(\nu,0) ~~\mathrm{and}~~ \nubarn := \argmin_{\nu} \fnclas(\nu,0)~~\mathrm{and}\\
%      \cfnone &:= \frac{\partial^2}{\partial\nu^2}\fnclas(\nubarn,0) = \frac{2}{n}\sum_{i=1}^n \idvec[ 1- \xi_i\nubarn \abs{\gausswone_i}] (\gausswone_i)^2 ~~\mathrm{and}~~ \cfntwo := \frac{2}{n}\sum_{i=1}^n \idvec[ 1- \xi_i\nubarn \abs{\gausswone_i}].
%      \label{eq:defineg2}
% \end{align}

% The quantities $\fnstar,\nubarn,\cfnone$ and $\cfntwo$ are random variables depending on $\xi$ and $\gausswone$. We first show the concentration of these variables in  Lemma~\ref{lm:quantconcentration}. 
% Recall $\nubar$ from Assumption A in Section~\ref{subsec:clasetting} and define the quantities ${\fstar = f(\nubar, 0)>0}$ and ${\fnnstar = \frac{d^2}{d^2 \nu}\vert_{(\nu, \eta) = (\nubar, 0)} f(\nu,\eta)>0}$.   Further define ${\feestar = \frac{d^2}{d^2 \eta}\vert_{(\nu, \eta) = (\nubar, 0)} f(\nu,\eta)>0}$. We have:

% \begin{lemma}
% \label{lm:quantconcentration}
% There exists universal constants $c_1,c_2>0$ such that with probability  $\geq 1-c_1 d^{-c_2}$ over the draws of $\gausswone$ and $\xi$, we have that
% \begin{align}
%     \max\left(\vert \nubar - \nubarn \vert, \vert \fstar - \fnstar\vert, \vert \cfnone - \fnnstar \vert, \vert \cfntwo -\feestar \vert \right) \lesssim \left(\frac{\log(d)}{n}\right)^{1/4}
% \end{align}
% \end{lemma}

% \begin{proof}
% Both $\fn$ and $f$ are convex functions with a unique global minima. In particular, because of Lemma~\ref{quadratic_bound_fn} we know that $\nubarn$ is with high probability attained in a bounded domain around zero. Further, by Lemma~\ref{lemma_quadratic_plus_fstar_bound} we see that with high probability $\vert \fnstar - \fstar \vert \lesssim \frac{\log(d)}{\sqrt{n}}$ and $\vert \nubar - \nubarn \vert \lesssim (\frac{\log(d)}{\sqrt{n}})^{1/2}$.

% To control the quantities $\cfnone,\cfntwo$,
% note that we can use exactly the same uniform convergence argument as for Proposition~\ref{prop:unifConv} to show that the functions $\nu \mapsto  \frac{2}{n}\sum_{i=1}^n \idvec[ 1- \xi_i\nu \abs{\gausswone_i}] (\gausswone_i)^2$ and  $\nu \mapsto  \frac{2}{n}\sum_{i=1}^n \idvec[ 1- \xi_i\nu \abs{\gausswone_i}]$ also converge uniformly for any bounded domain $\nu \in [\nubar - \delta, \nubar + \delta]$ with $\delta >0$. Thus, the proof then follows from  $\nubarn \to \nubar$  and the fact that 
% $h_1(\nu) = \EE_{\gausswone,\xi} 
% 2\idvec[ 1- \xi \nu \abs{\gausswone}] (\gausswone)^2$ and $h_2(\nu) = \EE_{\gausswone,\xi} 
% 2\idvec[ 1- \xi\nu \abs{\gausswone}]$ are both Lipschitz continuous functions
% in the domain $[\nubar - \delta, \nubar + \delta]$ with $h_1(\nubar) = \fnnstar$, $h_2(\nubar) = \feestar$.
% \end{proof}




% using on standard exponential tail bounds. In particular, note  that $\idvec[ 1- \xi_i\nubarn \abs{\gausswone_i}]$ is a sub-Gaussian random variable and $[ 1- \xi_i\nubarn \abs{\gausswone_i}] (\gausswone_i)^2$ 
% is a sub-exponential random variable. Thus, we have that $\vert g_1 - \EE_{\gausswone,\xi} 
% \idvec[ 1- \xi\nubarn \abs{\gausswone}] (\gausswone)^2  \vert \lesssim \frac{\sqrt{\log(d)}}{\sqrt{n}}$
% and similar for $\cfntwo$. 

% First note that by the $\fn \to f$ uniform convergence proof in Appendix~\ref{apx:subsec:unif_conv}

% $\fnstar$ and $\nubarn$ can be controlled using the fact that $\fnclas$ is a convex function and $\fnclas \to f$ uniformly in a neighbourhood of zero as described in Appendix~\ref{apx:subsec:unif_conv}. 
The bound in Lemma~\ref{lemma_quadratic_plus_fstar_bound} contains a term $\epsilon$
which is at least of order $\frac{1}{\sqrt{n}}$. This term arises from the uniform convergence of $\fnclas$ to $\fclas$ in Proposition~\ref{prop:unifConv} and cannot be avoided. Instead, we show that $\fnclas$ uniformly converges much faster to a different expression. 
%where we do not rely on uniform convergence to $f$. 
%to   without relying 

\begin{lemma}
\label{lm:lpfn}
 With probability at least $1-c_1d^{-c_2}$ over the draws of $\gausswone,\gausswtwo,\xi$, we have that 
\begin{equation}
\label{eq:lpfn}
    \sup_{ \eta\geq0, \deltanu} \left\| \fnclas(\nu, \eta) -  \fnstar - \deltanu^2 \frac{\cfnone}{2} - \eta^2 \frac{\cfntwo}{2} \right\| \lesssim (\deltanu^2 + \eta^2) \rho +   \rho \eta +(\rho + \sqrt{\log(d)}(\vert\deltanu\vert + \eta))^3,
\end{equation}
with  $\rho = \frac{\sqrt{\log(d)}}{\sqrt{n}}$.
\end{lemma}

\begin{proof}
We write
\begin{align}
    \fnclas(\nu,\eta) =& \frac{1}{n} \sum_{i=1}^n \idvec[ 1- \xi_i\nu \abs{\gausswone_i} - \eta \gausswtwo_i  ]( \underbrace{ ( 1- \xi_i\nubarn \abs{\gausswone_i} )^2}_{=:T_{1,i}} +  \underbrace{\xi_i^2 \deltanu^2 \abs{ \gausswone_i }^2}_{=:T_{2,i}}+  \underbrace{\eta^2 (\gausswtwo_i)^2 }_{=:T_{3,i}} 
    \\
    &  \underbrace{-2 \xi_i \deltanu \abs{ \gausswone_i } (1- \xi_i\nubarn \abs{ \gausswone_i } )}_{T_{4,i}} \underbrace{ -  2 \eta \gausswtwo_i (1- \xi_i\nubarn \abs{ \gausswone_i })}_{=:T_{5,i}}  + \underbrace{ 2\xi_i\deltanu \abs{ \gausswone_i } \eta \gausswtwo_i }_{T_{6,i}} \vphantom{\sum} )
    \\
    =& \frac{1}{n}\sum_{i=1}^n \idvec[ 1- \xi_i\nu \abs{ \gausswone_i } - \eta \gausswtwo_i ] \left( T_{1,i} + T_{2,i} + T_{3,i} + T_{4,i} + T_{5,i} + T_{6,i} \right)
\end{align}

We now separately apply concentration inequalities to the different terms. We first need to control the difference of the term $\idvec[ 1- \xi_i\nu \abs{ \gausswone_i } - \eta \gausswtwo_i]$ to the term $\idvec[ 1- \xi_i\nubarn \abs{ \gausswone_i }]$. Denote by $F_n(x) = \frac{1}{n}\sum_{i=1}^n \idvec[\xi_i\abs{ \gausswone_i } \leq x ]$ and by $F(x) = \prob \left( \xi\abs{ \gausswone } \leq x \right) $. By  the Dvoretzky-Kiefer-Wolfowitz inequality (see \cite{massart}), we have that, with probability at least $ 1 - \frac{2}{d} $,
\begin{equation}
    \sup_{ x \in \RR } |F_n(x) - F(x) | \leq  \sqrt{ \frac{\log(d)}{2n} } =: \rho 
\end{equation}
for any $ n \geq 3 $. Furthermore, note that with probability $\geq 1-\frac{1}{d}$, we have that $\max_i \{ \abs{\gausswtwo_i}, \abs{\gausswone_i} \} = \gamma_m \lesssim \sqrt{\log(d)}$ (see e.g., \cite{boucheron_2012}).  Therefore, we can upper bound 
\begin{align}
    \frac{1}{n} \sum_{i=1}^n &\left( \idvec[ 1- \xi_i\nu \abs{\gausswone_i} - \eta \gausswtwo_i] - \idvec[ 1- \xi_i\nubarn \abs{\gausswone_i} ] \right)\\
    &\leq F_n \left( \frac{1}{\nubarn} ( 1 + \gamma_m (\abs{\deltanu} + \eta) ) \right) - F_n \left( \frac{1}{\nubarn} ( 1 - \gamma_m (\abs{\deltanu} + \eta) ) \right) 
    \\
    & \leq 2\rho + F \left( \frac{1}{\nubarn} (1+ \gamma_m (\abs{\deltanu} + \eta)) \right) - F \left( \frac{1}{\nubarn} (1- \gamma_m (\abs{\deltanu} + \eta)) \right)  \lesssim \rho + \gamma_m (|\deltanu| + \eta)
\end{align}
where we condition on the event where $\nubarn$ concentrates around the constant $\nubar$ in Lemma~\ref{lm:quantconcentration}.
Therefore, we get
\begin{align}
    &\left|\fnclas(\nu,\eta) - \frac{1}{n}\sum_{i=1}^n \idvec[ 1- \xi_i\nubarn \abs{\gausswone_i}] \left( T_{1,i} + T_{2,i} + T_{3,i} + T_{4,i} + T_{5,i} + T_{6,i} \right) \right| 
    \\
    =& \left|\frac{1}{n}\sum_{i=1}^n \left(\idvec[ 1- \xi_i\nu |\gausswone_i| - \eta \gausswtwo_i] - \idvec[ 1- \xi_i\nubarn |\gausswone_i|]  \right) \left( T_{1,i} + T_{2,i} + T_{3,i} + T_{4,i} + T_{5,i} + T_{6,i} \right) \right|
    \\ 
    \lesssim & (\rho + \gamma_m(|\deltanu|  + \eta))^3 
\end{align}

Thus, we only need to study $\frac{1}{n} \sum_{i=1}^n \idvec[ 1- \xi_i\nubarn \abs{\gausswone_i}] \left( T_{1,i} + T_{2,i} + T_{3,i} + T_{4,i} + T_{5,i} + T_{6,i} \right)$.
We now separately bound the different terms involving $T_{j,i}$ for every $j$ which all hold with probability at least $1- c_1 d^{-c_2}$ with universal constants $c_1,c_2>0$.
\begin{enumerate}
    \item[$T_{1,i}$] First, note that by definition, $ \frac{1}{n}\sum_{i=1}^n \idvec[ 1- \xi_i\nubarn \abs{\gausswone_i}] T_{1,i} = \fnstar$.
    \item[$T_{2,i}$] Recall that $ \frac{\cfnone}{2} = \frac{1}{n}\sum_{i=1}^n \idvec[ 1- \xi_i\nubarn \abs{\gausswone_i}] (\gausswone_i)^2$.
        % \begin{align}
        %     \left| \frac{1}{n} \sum_{i=1}^n \idvec[ 1- \xi_i\nubarn \abs{\gausswone_i}] \xi_i^2 \deltanu^2 \abs{\gausswone_i}^2 - \deltanu^2 \cfnone  \right| 
        %     \leq 
        %     \deltanu^2 \left| \frac{1}{n}\sum_{i=1}^{k(n)} \gausswone_i^2 - 1  \right| \lesssim
        % \end{align}
    \item[$T_{3,i}$] Recall that  $ \frac{\cfntwo}{2} = \frac{1}{n}\sum_{i=1}^n \idvec[ 1- \xi_i\nubarn \abs{\gausswone_i}] $.
        \begin{equation}
            \left| \frac{1}{n} \sum_{i=1}^n \idvec[ 1- \xi_i\nubarn \abs{\gausswone_i}] \eta^2 (\gausswtwo_i)^2 - \eta^2 \frac{\cfntwo}{2}  \right| 
            \leq 
            \eta^2 \left| \frac{1}{n}\sum_{i=1}^{k} ((\gausswtwo_i)^2 - 1) \right| 
           \lesssim \eta^2 \rho 
        \end{equation}
    with probability at least $ 1 - \frac{1}{d} $ over the draws of $\gausswtwo_i$. We used that $ \sum_{i=1}^n \idvec[ 1- \xi_i\nubarn \abs{\gausswone_i}] = k \leq n$. We apply the same reasoning in the following concentration inequalities.
    \item[$T_{4,i}$] Note that by definition of $\nubarn$ we have that
        \begin{equation}
            \frac{d}{d\nu}|_{\nubarn} f_n(\nu,0)  = \frac{1}{n} \sum_{i=1}^n \idvec[ 1- \xi_i\nubarn \abs{\gausswone_i}] 2(1- \xi_i\nubarn \abs{\gausswone_i})\xi_i \abs{\gausswone_i} = 0
        \end{equation}
    \item[$T_{5,i}$] We can bound the term involving $T_{5,i}$ by
        \begin{align}
            \left| \frac{1}{n} \sum_{i=1}^n \idvec[ 1- \xi_i\nubarn \abs{\gausswone_i}] 2\eta \gausswtwo_i \left( 1 - \xi_i\nubarn \abs{\gausswone_i} \right)  \right| 
            \leq
            2\eta \left| \frac{1}{n} \sum_{i=1}^n ( 1 + \nubarn \abs{\gausswone_i}) \gausswtwo_i 
            \right|
            \lesssim
            \eta \rho
        \end{align}
    \item[$T_{6,i}$]  We can bound the term involving $T_{6,i}$ by
        \begin{align}
            \left| \frac{1}{n} \sum_{i=1}^n \idvec[ 1- \xi_i\nubarn \abs{\gausswone_i}] 2 \xi_i \deltanu \abs{\gausswone_i} \eta \gausswtwo_i \right| 
            \leq
            2 \eta \abs{\deltanu}  \left| \frac{1}{n} \sum_{i=1}^n \gausswone_i \gausswtwo_i \right| \lesssim \eta \abs{\deltanu} \rho
        \end{align}
    % In both of previous points we use that:
    % \begin{align}
    %     \left| \frac{1}{n} \sum_{i=1}^n \gausswone_i \gausswtwo_i \right| 
    %     =
    %     \norm{\gausswone} \left| \frac{1}{n} \left( \frac{\gausswone}{\norm{\gausswone}}\right)^T \gausswtwo \right| 
    %     =
    %     \frac{\norm{\gausswone}}{\sqrt{n}} \left| \tilde{\gausswtwo} \right|
    % \end{align}
    % where $\tilde{\gausswtwo} \sim \NNN (0,\frac{1}{n})$. Then we have that $\prob \left( \norm{\gausswone}\geq \sqrt{2n} \right) \leq \exp(-n/16)$ and $ \prob \left( \abs{\tilde{\gausswtwo}} \geq \sqrt{\frac{2\log(d)}{n}} \right) \leq \frac{2}{d}$. Hence we have that:
    % \begin{align}
    %     \left| \frac{1}{n} \sum_{i=1}^n \gausswone_i \gausswtwo_i \right| \lesssim \rho
    % \end{align}
    % with probability at least $ 1 - \exp(-n/16) - \frac{2}{d} $.
\end{enumerate} 

%Finally, we obtain the desired bound when using that $\nu, \eta \lesssim \log^{-1}(d)$. 





% $\cfnone = \frac{1}{n}\sum_{i=1}^n \idvec[ 1- \xi_i\nubarn |\gausswone_i|] \xi_i |\gausswone_i|^2$.





% \paragraph{Bounding $T_1$}
% The bound for $T_1$ follows now straight forwardly from 
% \begin{equation}
%     T_1 -\fnstar :=  \frac{1}{n}\sum_{i=1}^n \left(\idvec[ 1- \xi_i\nu |\gausswone_i| - \eta \gausswtwo_i]-\idvec[ 1- \xi_i\nubarn |\gausswone_i|]\right) ( 1- \xi_i\nubarn \|\gausswone_i\|)^2
%     \lesssim (\rho + \gamma_m(|\deltanu|  + \eta)) \gamma_m(|\deltanu|  + \eta)^2
% \end{equation}
% \paragraph{Bounding $T_2$}
% Define $\cfnone = \frac{1}{n}\sum_{i=1}^n \idvec[ 1- \xi_i\nubarn |\gausswone_i|] \xi_i |\gausswone_i|^2$. We have
% \begin{equation}
%     T_2 - \nu^2 \cfnone  := \nu^2 \frac{1}{n}\sum_{i=1}^n   \left(\idvec[ 1- \xi_i\nu |\gausswone_i| - \eta \gausswtwo_i]-\idvec[ 1- \xi_i\nubarn |\gausswone_i|]\right) \xi_i |\gausswone_i|^2
%     \lesssim (\rho + \gamma_m(|\deltanu|  + \eta)) \gamma_m^2
%     \end{equation}
%     \red{bounds can be significantly improved though}
% \paragraph{Bounding $T_3$}

% Define $\cfntwo = \frac{1}{n} \sum_{i=1}^n \idvec[ 1- \xi_i\nubarn |\gausswone_i|]$. First of all, note that 
% \begin{equation}
%     |\cfone \frac{1}{n} \sum_{i=1}^n \idvec[ 1- \xi_i\nubarn |\gausswone_i|] \gausswtwo_i^2| \leq 
%     \sum_{i=1}^n |G_i^2 -1| \lesssim \frac{\log(n)}{\sqrt{n}} = \rho 
% \end{equation}
% Thus, we get
% \begin{equation}
%     T_3 - \nu^2 \cfntwo  := \nu^2 \frac{1}{n}\sum_{i=1}^n   \left(\idvec[ 1- \xi_i\nu |\gausswone_i| - \eta \gausswtwo_i]-\idvec[ 1- \xi_i\nubarn |\gausswone_i|]\right) \xi_i |\gausswone_i|^2
%     \lesssim (\rho + \gamma_m(|\deltanu|  + \eta)) \gamma_m^2
%     \end{equation}
%     \red{bounds can be significantly improved though}
% \paragraph{Bounding $T_4$}
% Note that by definition of $\nubarn$ we have that
% \begin{equation}
%     \frac{d}{d\nu}|_{\nubarn} f_n(0,\nu) = \frac{1}{n} \sum_{i=1}^n 2\idvec[ 1- \xi_i\nubarn |\gausswone_i|] (1- \xi_i\nubarn \|\gausswone_i\|)\xi_i|\gausswone_i| =0
% \end{equation}
% Therefore, we can bound
% \begin{align}
%   |T_4| = |T_4 - \frac{1}{n} \sum_{i=1}^n \idvec[ 1- \xi_i\nubarn |\gausswone_i|] (1- \xi_i\nubarn \|\gausswone_i\|)\deltanu \xi_i|\gausswone_i| | \\
%   =
%   |\frac{1}{n} \sum_{i=1}^n \left( \idvec[ 1- \xi_i\nu |\gausswone_i| - \eta \gausswtwo_i] - \idvec[ \idvec[ 1- \xi_i\nubarn |\gausswone_i|]\right)(1- \xi_i\nubarn \|\gausswone_i\|)\deltanu \xi_i|\gausswone_i| |
% \\
% \leq (\rho + \gamma_m(|\deltanu|  + \eta))^3 
% \end{align}
% \paragraph{Bounding $T_5$}




% \begin{equation}
%       \frac{1}{n}\sum_{i=1}^n \idvec[ 1- \xi_i\nu |\gausswone_i| - \eta \gausswtwo_i] \left( ( 1- \xi_i\nubarn \|\gausswone_i\|)^2 +  \xi^2 \deltanu^2 \|\gausswone_i\|^2 +  \eta^2 \gausswtwo_i^2 - \right. \\
%   \left. (1- \xi_i\nubarn \|\gausswone_i\|)(\xi_i\deltanu |\gausswone_i|) -  (1- \xi_i\nubarn \|\gausswone_i\|) \eta \gausswtwo_i + \xi_i\deltanu |\gausswone_i| )\eta \gausswtwo_i \right)
%     \\
%     = \frac{1}{n}\sum_{i=1}^n \idvec[ 1- \xi_i\nu |\gausswone_i| - \eta \gausswtwo_i] \left( T_{1,i} + T_{2,i} + T_{3,i} + T_{4,i} + T_{5,i}\right)
% \end{equation}


\end{proof}





% \begin{lemma}
% Let $\rho = \frac{\sqrt{\log(d)^c}}{\sqrt{n}}$. With probability at least $1-c_1d^{-c_2}$, we have that 
% \begin{equation}
%     \sup_{|\deltanu, \eta| \leq c_0 \log^{-1}(d)} \left| f_n(\nu, \eta) -  \fnstar - \deltanu^2 \cfnone - \eta^2 \cfntwo \right| \lesssim \rho(\deltanu^2 + \eta^2)  +   \rho(\deltanu + \eta) +(\rho + \sqrt{\log(d)}(\deltanu + \eta))^3
% \end{equation}
% \end{lemma}
















% \begin{restatable}{theorem}{MainThm}
% \label{thm:MainThm}
% There exist universal constants $ c, c_n, c_l, c_u > 0 $ such that, if $ n\geq c_n $ and $ c_l n \leq d \leq \exp \left( c_u n^{1/5} \right) $, then
% \begin{align}
%     R \left( w \right) = \frac{1}{\pi} \arccos \left( \frac{ \innerprod{ w }{ \wgt } }{ \norm{w}_2 } \right) = \Omega\left( \frac{1}{\log \left( d/n \right)^{1/2}}\right)
% \end{align}
% with probability at least $ 1 - $.
% \end{restatable}







% \section{Main result Lp} \label{sec:main_result}
% We are now interested in studying the risk of LP norm interpolators. Trivially, we have again:
% \begin{align}
% \tag{$P_N$} \label{eq:PhiN}
%     \PhiN &= \min_w \norm{w}_p^p
%     \subjto \minin y_i\innerprod{\gausswone_i}{w}\geq 1\\
% \tag{$P_+$} \label{eq:Phip}
%     \Phip &= \max_w \frac{\innerprod{w}{\wgt}}{\norm{w}_2}  
%     \subjto \begin{cases}
%         \minin y_i\innerprod{\gausswone_i}{w}\geq 1\\
%         \norm{w}_p^p \leq \lonebound
%     \end{cases}\\
% \tag{$P_-$} \label{eq:Phim}
%     \Phim &= \min_w \frac{\innerprod{w}{\wgt}}{\norm{w}_2}  
%     \subjto \begin{cases}
%         \minin y_i\innerprod{\gausswone_i}{w}\geq 1\\
%         \norm{w}_p^p \leq \lonebound
%     \end{cases}
% \end{align}

% Again, define $\fnclas(x,y) = \frac{1}{n} \sumin \possq{1-\xi_i\abs{\gausswone_i}x-\gausswtwo_i y}$.
% \begin{restatable}{proposition}{propCGMT}
% % \begin{proposition} 
% \label{prop:CGMT_application}
%     % Denote $\gennormboundp = \gennormbound + \norm{w^*}_1$. % CONVENTION 1
%     %Denote $\gennormboundp =  \gennormbound + 2\norm{w^*}_1$. % CONVENTION 2
%     For $\Ggaussian \sim \NNN(0,I_d)$ and $\gausswone,\gausswtwo \sim \NNN(0,I_n)$, define the stochastic auxiliary optimization problems:
%         \begin{align}
%         \tag{$A_N$} \label{eq:phin}
%             \phidn &= \min_{(\wone,\wtwo)} \norm{\wone}_p^p+\norm{\wtwo}_p^p
%             \subjto \frac{1}{n} \innerprod{\wtwo}{\Ggaussian}^2 \geq \sumin \fnclas(\|\wone\|_2,\|\wtwo\|_2) \\
%         \tag{$A_+$} \label{eq:phip}
%             \phidp &= \max_{(\wone,\wtwo)} \frac{\wone}{\sqrt{\norm{\wone}_2^2+\norm{\wtwo}_2^2}} 
%             \subjto \begin{cases}
%                 \frac{1}{n} \innerprod{\wtwo}{\Ggaussian}^2 \geq \sumin \fnclas(\|\wone\|_2,\|\wtwo\|_2)\\
%               \norm{\wone}_p^p+\norm{\wtwo}_p^p \leq \lonebound
%             \end{cases}\\
%         \tag{$A_-$} \label{eq:phim}
%             \phidm &= \min_{(\wone,\wtwo)} \frac{\wone}{\sqrt{\norm{\wone}_2^2+\norm{\wtwo}_2^2}}  
%             \subjto \begin{cases}
%               \frac{1}{n} \innerprod{\wtwo}{\Ggaussian}^2 \geq \sumin \fnclas(\|\wone\|_2,\|\wtwo\|_2) \\
%               \norm{\wone}_p^p+\norm{\wtwo}_p^p  \leq \lonebound
%             \end{cases}
%         \end{align}
%     where $\lonebound>0$ is a constant such that $\lonebound\geq \phidn$. Then for any $t \in \RR$ we have:
%         \begin{align}
%             \PP( \Phi_N > t ) &\leq 2\PP( \phidn \geq t )
%             \label{eq:probeq1} \\
%             \PP( \Phi_+ > t ) &\leq 2\PP( \phidp \geq t ) 
%             \label{eq:probeq2} \\
%             \PP( \Phi_- < t ) &\leq 2\PP( \phidm \leq t ) 
%             \label{eq:probeq3} ,
%         \end{align}
%         where the probabilities on the left and on the right are over the draws of $\{\gausswone_i,y_i\}_{i=1}^n$ and of $\Ggaussian,\gausswone,\gausswtwo$, respectively.
% \end{restatable}   

% % Following the work in \cite{konst} we can recast \eqref{eq:phin}, \eqref{eq:phip}, \eqref{eq:phim} as optimization problems in three scalar variables. Let $b,\alpha$ be scalar variables with $b\geq 0$, $\alpha\in[1,\alpham]$ with $\alpham = d\frac{\norm{\Hgaussian}_{\infty}}{\norm{\Hgaussian}_1}$. Then we define parametric path $b\gamma(\alpha)$ with $\RR^d$-valued function $\gamma$ given by:
% % \begin{equation}
% %     \gamma(\alpha) = \argmin_{\wtwo} \norm{\wtwo}_2^2
% %     \subjto \begin{cases}
% %                 \innerprod{\wtwo}{\Hgaussian} \geq \norm{\Hgaussian}_{\infty}\\
% %                 \wtwo\geq 0\\
% %                 \transp{\idvec} \wtwo = \norm{\wtwo}_1 = \alpha
% %             \end{cases}
% % \end{equation}
% % \begin{restatable}{proposition}{propparam}
% % % \begin{proposition} 
% % \label{prop:parametrization}
% % Optimization problems \eqref{eq:phin}, \eqref{eq:phip}, \eqref{eq:phim} are equivalently given by:
% %         \begin{align}
% %         \tag{$A_N$}\label{eq:phin}
% %             \phidn &= \min_{\nu,b,\alpha} \nu + \alpha b
% %             \subjto \frac{1}{n}  b^2\norm{\Hgaussian}_{\infty}^2  \geq  \fnclas(\|\wone\|_2,b\|\gamma(\alpha)\|_2). \\
% %         \tag{$A_+$} \label{eq:phip}
% %             \phidp &= \max_{\nu,b,\alpha}  \frac{\nu}{\sqrt{\nu^2+b^2\norm{\gamma(\alpha)}_2^2}}
% %             \subjto \begin{cases}
% %               \frac{1}{n}  b^2\norm{\Hgaussian}_{\infty}^2  \geq  \fnclas(\|\wone\|_2,b\|\gamma(\alpha)\|_2)\\
% %                 \nu+b  \leq \lonebound
% %             \end{cases}\\
% %         \tag{$A_-$} \label{eq:phim}
% %             \phidm &= \min_{\nu,b,\alpha}  \frac{\nu}{\sqrt{\nu^2+b^2\norm{\gamma(\alpha)}_2^2}}
% %             \subjto \begin{cases}
% %               \frac{1}{n}  b^2\norm{\Hgaussian}_{\infty}^2  \geq  \fnclas(\|\wone\|_2,b\|\gamma(\alpha)\|_2)\\
% %                 \nu+b \leq \lonebound
% %             \end{cases}
% %         \end{align}
% % for some scalars $\nu,b>0$ and $\alpha\in[1,\alpham]$.

% % \end{restatable}   



% Let's define empirical function $f_n(\nu,\eta) = \frac{1}{n}\sumin \possq{1-\xi_i\abs{\gausswone_i}\nu-\gausswtwo_i \eta}$ and its expectation $f(\nu,\eta) = \EE \left[ \possq{1-\xi\abs{\gausswone}\nu-\gausswtwo \eta} \right] $ where expectation is over $\gausswone$, $\gausswtwo$ and $\xi$. Global minimum of function $f$ is at point $(\nuopt,0)$.






% \begin{restatable}{proposition}{propRbound}
% \label{prop:Rbound}
% Let $t_{\nopt}$ be given by $2\Phic(t_{\nopt}) = \nopt/d$ with $\nopt = n\fetaeta/2$. There exist universal constants $c,c_n,c_l,c_u,c_p$ such that, if $n\geq c_n$ and $c_l n\leq d\leq \exp(c_u n^{1/5})$ then
%     \begin{align}
%         (\phidn)^2 \leq \frac{nf(\nuopt,0)}{t_{\nopt}^2}\left(1-\frac{2}{t_{\nopt}^2}+\frac{c}{t_{\nopt}^3} \right) =:\lonebound^2(n,d)
%     \end{align}
% with probability at least $1-c_p\exp \left(-\frac{\nopt}{{\log(d/\nopt)}^5}\right)-\OOO_c(!)$ over the draws of $\Hgaussian$, $\gausswone$ and $\gausswtwo$.

% \end{restatable}  





==> ICML 22-3/sections_proof/TL5_boundinghq.tex <==
%\subsection{Concentration of $\|H\|_q$ and $\norm{\wgrad}_2^2$}

%\section{Technical lemmas: Concentration of the dual norm $\|H\|_q$ and $\|\wgrad\|_2$}
\section{Proof of Lemma~\ref{lm:dualnormconc}}
\label{apx:proofdualnormconc}
\label{apx:concentrationdual}

% We now discuss the concentration of the dual norm $\|H\|_q$ and the $\ell_2$ norm of the subgradient $\|\wgrad\|_2$

% % \begin{comment}
% %=  \frac{\norm{H}_{2q/p}^{2q/p}}{\norm{H}_q^{2q/p}}$. 
% Essentially, both are direct consequences of the following two theorems from the literature. Recall the definitions $\dmoment{q} = \EE \|H\|_{q}$ and
% $\mutild := \frac{\dmoment{2q/p}^{2q/p}}{\dmoment{q}^{2q/p}}$. We have,
% %Note that  begin with the following lemma of Theorem~1 in \cite{paouris_2017}:
% % The proof of Lemma~\ref{lm:dualnormconc} can be found in Appendix~\ref{apx:proofdualnormconc}.
% % The lemma above is essentially a consequence of the following two corollaries:
% % These tools allow us to study the concentration of the sub gradient $\wgrad = \partial \norm{H}_p$, i.e. the vector which satisifes $\langle \wgrad, H \rangle = \norm{H}_q$ and $\norm{\wgrad}_p =1$ with $q$ the dual number of $p$. In particular, we show that:
%  \begin{theorem}[Corollary of Theorem 1 \cite{paouris_2017}]
%  \label{cor:hqbound1}
% For all sufficiently large $d$ and any $2<q <c_1\log(d)$ and $\epsilon \in (0,1)$, we have: 
% \begin{equation}
% \label{eq:paouris}
%     \prob(|\|H\|_q - \dmoment{q} | \geq \epsilon \EE \|H\|_q ) \leq c_2 \exp(-c_3 \min(q^2 2^{-q} \epsilon^2 d, (\epsilon d )^{2/q}))
% \end{equation}
% where $c_1\in (0,1),c_2,c_3>0$ are universal constants.
% \end{theorem}
% and
% \begin{proposition}[Proposition 2.4 \cite{paouris_2017}, \cite{schechtman_89}]
% \label{cor:hqbound2}
% For all $q \leq \logjone{d}$, we have that $\dmoment{q} \asymp \sqrt{q} d^{1/q}$.
% \end{proposition}

% In particular, as a direct application of these two results, we can show that when choosing $q \lesssim \log\log(d)$, $\|H\|_q^q \asymp d$ with high probability over the draws of $H$. More precisely, we show that 
% \begin{lemma}
% \label{lm:dualnormconc}
% There exists a universal constant $c_1,c_2,c_3,c_4,c_5,c_6>0$ such that for any $n \geq c_1$ and $n \lesssim d \lesssim \exp(n^{c_2})$ and $q \lesssim \log\logjone{d}$ 
% and for $\epsilon = \max\left(\frac{n}{d}, \frac{\log^{c_3}(d)}{n}\right)$ 
% %\red{fix macro, also seems unclear regarding log notation, also after moving the $\epsilon$ notation should be adjusted to this section}
%  with probability at least $ 1-c_4 d^{-c_5}$, 
% \begin{align}
% \langle \wgrad, H\rangle &= \norm{H}_q = \dmoment{q}\left(1+O\left(\epsilon \right)\right)   = \Theta(d^{\frac{1}{q} +\frac{\log(q)}{2\logjone{d}}})~~\mathrm{and} \label{eq:dualnormconc1}
% \\
% \norm{\wgrad}_2^2 &= \frac{\norm{H}_{2q/p}^{2q/p}}{\norm{H}_q^{2q/p}} = \mutild
% \left( 1 + O\left(\epsilon q \right)\right) = O\left(d^{\frac{1}{q}-\frac{1}{p} + \frac{c_6 q}{\logjone{d}}}\right) \lor \Omega\left(d^{\frac{1}{q}-\frac{1}{p} - \frac{c_6 q}{\logjone{d}}}\right)\label{eq:dualnormconc2},
% \end{align}
% where $p$ is such that $\frac{1}{p} + \frac{1}{q} = 1$. %\red{make fractions consistent}
% \end{lemma}
% % The proof of the  of the lemma is deferred to Appendix~\ref{apx:proofdualnormconc}. Further, we make use of the following lemma which gives tight bounds for the expectation $\dmoment{q}$.
% \end{comment}

% \begin{proof}






%\subsection{Proof of Lemma~\ref{lm:dualnormconc}}

% This section presents convergence inequalities for the norm of the sub-gradient  $\wgrad = \partial \norm{H}_q$, i.e., the vector which satisfies $\langle \wgrad, H \rangle = \norm{H}_q$ and $\norm{\wgrad}_p =1$.  Denote with $\dmoment{q} = \EE \|H\|_{q}$, the expected $\ell_q$-norm of $H$, and define  $\mutild := \frac{\dmoment{2q/p}^{2q/p}}{\dmoment{q}^{2q/p}}$. We have
% \begin{lemma}
% \label{lm:dualnormconc}
% There exists a universal constant $c_1,c_2,c_3,c_4,c_5,c_6>0$ such that for any $n \geq c_1$ and $n \lesssim d \lesssim \exp(n^{c_2})$ and $q \lesssim \log\log(d)$ and for $\epsilon  = \max\left(\frac{1}{\log(d)^2}\frac{n}{d}, \frac{\log^{c_3}(d)}{n}\right)$
%  with probability $\geq 1-c_4 d^{-c_5}$, 
% \begin{align}
% \langle \wgrad, H\rangle &= \norm{H}_q = \dmoment{q}\left(1+O\left(\epsilon  \right)\right)   = \Theta(d^{1/q +\frac{\log(q)}{2\log(d)}})~~\mathrm{and} \label{eq:dualnormconc1}
% \\
% \norm{\wgrad}_2^2 &= \frac{\norm{H}_{2q/p}^{2q/p}}{\norm{H}_q^{2q/p}} = \mutild
% \left( 1 + O\left(\epsilon  q \right)\right) = O\left(d^{1/q-1/p + \frac{c_6 q}{\log(d)}}\right) \lor \Omega\left(d^{1/q-1/p - \frac{c_6 q}{\log(d)}}\right)\label{eq:dualnormconc2},
% \end{align}
% where $p$ is such that $\frac{1}{p} + \frac{1}{q} = 1$.
% \end{lemma}

% We begin with the following lemma of Theorem~1 in \cite{paouris_2017}:
% % The proof of Lemma~\ref{lm:dualnormconc} can be found in Appendix~\ref{apx:proofdualnormconc}.
% % The lemma above is essentially a consequence of the following two corollaries:
% % These tools allow us to study the concentration of the sub gradient $\wgrad = \partial \norm{H}_p$, i.e. the vector which satisifes $\langle \wgrad, H \rangle = \norm{H}_q$ and $\norm{\wgrad}_p =1$ with $q$ the dual number of $p$. In particular, we show that:
%  \begin{lemma}[Theorem 1 \cite{paouris_2017}]
%  \label{cor:hqbound1}
% For all sufficiently large $d$ and any $2<q <c_1\log(d)$ and $\epsilon \in (0,1)$, one has: 
% \begin{equation}
% \label{eq:paouris}
%     \prob(|\|H\|_q - \dmoment{q} | \geq \epsilon \EE \|H\|_q ) \leq c_2 \exp(-c_3 \min(q^2 2^{-q} \epsilon^2 d, (\epsilon d )^{2/q}))
% \end{equation}
% where $c_1\in (0,1),c_2,c_3>0$ are universal constants.
% \end{lemma}
First note that by taking subgradients we directly obtain $\langle \wgrad, H\rangle = \norm{H}_q$ and 
$\norm{\wgrad}_2^2 = \left(\frac{\norm{H}_{2q/p}}{\norm{H}_q}\right)^{2q/p}$. 

Recall the definitions $\dmoment{q} = \EE \|H\|_{q}$ and
$\mutild := \left( \frac{\dmoment{2q/p}}{\dmoment{q}} \right)^{2q/p}$. We use the following well-known concentration result on $\ell_q$-norms to control these quantities.
 \begin{theorem}[Corollary of Theorem 1 \cite{paouris_2017}]
 \label{cor:hqbound1}
For all sufficiently large $d$ and any $2<q <c_1\log(d)$ and $\epsilon \in (0,1)$, we have: 
\begin{equation}
\label{eq:paouris}
    \prob(|\|H\|_q - \dmoment{q} | \geq \epsilon \EE \|H\|_q ) \leq c_2 \exp(-c_3 \min(q^2 2^{-q} \epsilon^2 d, (\epsilon d )^{2/q}))
\end{equation}
where $c_1\in (0,1),c_2,c_3>0$ are universal constants.
\end{theorem}


The proof of the lemma follows by showing that the choice of $\epsilon$ leads to sufficiently small terms in the exponent on the RHS of Equation~\eqref{eq:paouris}. More precisely, we show that there  exists a universal constant $c>0$, such that for all $n,d$ sufficiently large with $d \geq n$ and  $2\leq  q \leq c \log\log(d)$, we have that
\begin{equation}
    \min(q^2 2^{-q} \epsilon ^2 d, (\epsilon  d )^{2/q}) \geq \log(d), \label{eq:proofconctempeq}
\end{equation}
\label{claim_hq_proof}
and similarly for $2q/p$ instead of $q$. 

Equation~\eqref{eq:dualnormconc1} then follows directly from the claim and Theorem~\ref{cor:hqbound1}. To see Equation~\eqref{eq:dualnormconc2}, we have that with probability $\geq 1-c_1 d^{-c_2}$,
\begin{align}
     \norm{H}_{2q/p}^{2q/p} = \dmoment{2q/p}^{2q/p} \left(1+ O(\epsilon )\right)^{2q/p}
     = \dmoment{2q/p}^{2q/p} \left(1+  O( q\epsilon ))\right),
\end{align}
where we have used in the last equality that $q\lesssim \log\log(d)$ and that $\epsilon  = O(\log^{-1}(d))$ (by assumption on $d,n$ and $\epsilon$). Furthermore, the proof follows from the fact that a similar argument also applies to $\norm{H}_{q}^{2q/p}$. 

Thus, the only thing left to show is Equation~\eqref{eq:proofconctempeq}. 
We separately check the different conditions in Theorem~\ref{cor:hqbound1}. First, note that it is sufficient to only consider the case where $q = c \log\log(d)$. We separate the proof into two cases where   $n^2 \geq d \log^{c_2}(d)$  and $n^2 \leq d \log^{c_2}(d)$ with constant $c_2>0$. 
\paragraph{Case  $n^2 \geq d \log^{c_2}(d) \implies \epsilon  =\frac{n}{d}$} 
%For the first case we note that the  RHS in Equation~\eqref{eq:proofconctempeq} monotonically increases with $\epsilon$, and thus it is sufficient if we prove the result for $\epsilon  =\frac{n}{d}$.
Looking only at the first term on the RHS in Equation~\eqref{eq:proofconctempeq}, we have 
\begin{align}
    \log(q^2 2^{-q} \epsilon ^2 d) = 2\log(q) - q\log(2) + 2\log(n) - \log(d) \geq \log\log(d),
\end{align}
Furthermore, looking only at the second term on the RHS in  Equation~\eqref{eq:proofconctempeq}, we have 
\begin{align}
   \frac{2}{q} \log(\epsilon d)=  \frac{2}{q}\log(n) \geq \log\log(d),
\end{align}
which holds also under weaker assumptions on $n,d$. Hence the proof for the first case is complete. 

\paragraph{Case $n^2 \leq d \log^{c_2}(d) \implies \epsilon  =\frac{\log^{c_1}(d)}{n}$.} 
From straight forward calculation, we note that there exists a universal constant  $c_1>0$ only depending on $c_2$ such that 
\begin{align}
    \log(q^2 2^{-q} \epsilon ^2 d) = 2\log(q) - q\log(2) + \log(d) - 2\log(n) + 2c_1\log\log(d) \geq \log\log(d),
\end{align}
for any $n$ such that $n^2 \leq d \log^{c_2}(d)$. 
Furthermore, under the same assumption on $d,n$, we have
\begin{align}
   \frac{2}{q} \log(\epsilon d)=  \frac{2}{q} (\log(d)-\log(n) +c_1 \log\log(d)) \geq \log\log(d).
\end{align}

Finally the expectations $\mutild, \dmoment{q}$ are directly obtained using the following well-known result on the expectations of the $\ell_q$ norms of Gaussian vectors
\begin{proposition}[Proposition 2.4 \cite{paouris_2017}, \cite{schechtman_89}]
\label{cor:hqbound2}
For all $q \leq \logjone{d}$, we have that $\dmoment{q} \asymp \sqrt{q} d^{1/q}$.
\end{proposition}
This concludes the proof. 


% \end{proof}


==> ICML 22-3/sections_proof/low_noise_reg.tex <==
\section{Bounds for low noise regimes}
\label{apx:lownoise}

\red{this is nonsense so far, do we need this? Maybe not...}


\begin{proposition}
\label{prop:noiseless}
\red{ put in the appendix}
Under the same assumptions on $n,d$ and $p$ as in Theorem~\ref{thm:regressionlpmain} and for any $\sigma^2 \lesssim \frac{d^2}{n^{q}}$ the risk is upper and lower bounded by. 
\begin{align}
\Risk(\what) = O\left(\frac{d^2}{n^{q}}\right) ~~\mathrm{and}~~ \Risk(\what) = \Omega\left(\frac{d^2}{qn^{q}}\right)
    % \Risk\left( \what \right) &\leq \nu_0^2(1+ O\left(\frac{1}{\log(d)}\right
    % + O\left(\nu_0\sqrt{\frac{ \mutild \sigmaxi^2 n}{\dmoment{q}^2}} + \frac{ \mutild \sigmaxi^2 n}{\dmoment{q}^2}\right) = O\left(\frac{\sigmaxi^2 n  \exp(cq)}{d}\lor \frac{d^{2p-2}}{n^p}\right)\\
    % \Risk\left( \what \right) &\geq  \nu_0^2(1+ O\left(\frac{1}{\log(d)}\right) 
    % + O\left(\nu_0\sqrt{\frac{ \mutild \sigmaxi^2 n}{\dmoment{q}^2}} + \frac{ \mutild \sigmaxi^2 n}{\dmoment{q}^2}\right) \lor \Omega(\frac{\sigmaxi^2 n}{d}) = \Omega\left(\frac{\sigmaxi^2 n}{d}\lor \frac{d^{2p-2}}{n^p} - c_4\frac{\sigmaxi n 
    % \exp(cq)}{d}\right)
    % \nu_0^2(1+ O\left(\frac{1}{\log(d)}\right) 
    % + O\left(\nu_0\sqrt{\frac{ \mutild \sigmaxi^2 n}{\dmoment{q}^2}} + \frac{ \mutild \sigmaxi^2 n}{\dmoment{q}^2}\right)
    % \vor c_3 \frac{n}{d} = \Omega(...)
\end{align}
with probability at least $ 1 - c_1 d^{c_2}$ over the draws of $X$ and $\xi$.
\end{proposition}




\subsection{Proof of Proposition~\ref{prop:lownoise}} 
The proof for the low noise regime follows essentially the same structure as the proof for the high noise regime. We use exactly the same notation as in Appendix~\ref{apx:subsec:highnoise} except for $\nu_0 = -\frac{\sigmaxi^q}{\bnull^q}$. 
\subsubsection{Step 1: Localization step - bounding $\phidn$.}
In a first step, we again upper bound $\phidn$:
% The proof of the lemma is deferred to and follows straight forwardly from a similar argument as used in \cite{koehler2021uniform} \red{cite correctly}.  The goal of this section is to show the upper bound on $\phidn:$
\begin{proposition}
\label{prop:phidnlowreg}
Under the same conditions as in Theorem~\ref{thm:regressionlp} with $\sigma \lesssim \frac{\sigma^p}{\bnull^p}$, we have that with probability $\geq 1- c_1 d^{c_2}$ over the draws of $\Ggaussian,\Hgaussian,\Xs,\xi$ that
\begin{align}
\phidn  \leq \vert \nu_0 \vert  \left(1+ O\left(\frac{1}{\log(d)}\right) 
 \right)
% \frac{\mutild  n}{\dmoment{q}^2}\right)(1+O\left(\frac{1}{\log(d)}\right)) + O\left(\rho \sqrt{\frac{ \nu_0^2}{\sigmaxi^2} + 
% \frac{\mutild  n}{\dmoment{q}^2}}\right) \right) \\
+ 1 + p\nu_0\left(1+ O(\log(d)^{-1}\right) =: \lonebound,
\end{align}
\end{proposition}
\begin{proof}
Following exactly the same argument as in the high noise regime,  
%  To upper bound the solution of a minimization problem, we only need to find one suitable point. We choose $\wtwo$ to be the Sub-gradient of $H$, i.e. $\wtwo = b \wgrad = b \partial \|H\|_p$ and choose $b$ appropriately as described below. Furthermore, we recall that $\wone$ is just a one dimensional scalar. We abbreviate $\wone= \nu$ and $\norm{\wtwo}_2 = \eta$. Further, we denote with $\nugt = \wgt_1 \in \RR^d$ to be the only non-zero entry. 
% In order to have a feasible point satisfying the constraints in the definition of $\phidn$,
we require that
\begin{align}\frac{1}{n} 
b^2 &\geq \frac{ \sigmaxi^2 +  \nu^2(1+O( \rho)) + O(\sigmaxi\rho)(\vert \nu\vert+b\|\wgrad\|_2) }{\norm{H}_q^2/n - \norm{\wgrad}_2^2 (1+O(\rho)) }. \label{eq:lpboundphinb} 
\end{align}
% \begin{align}\frac{1}{n} \innerprod{\wtwo}{\Ggaussian}^2 \geq \fn(\|\wone\|_2,\|\wtwo\|_2) \\ \impliedby
% b^2 \norm{H}_q^2/n \geq  \sigmaxi^4 + \rho \sigmaxi^2 \vert b \norm{\wgrad}_2 \vert +\rho b \norm{\wgrad}_2 \vert \nu\vert + \rho \sigmaxi^2 \vert \nu \vert + (1+\rho) (\nu^2 + b^2 \norm{\wgrad}_2^2) \\
% \impliedby
% b^2 \geq \frac{1}{\norm{H}_q^2/n - (1+\rho)\norm{\wgrad}_2^2 } \left(  \sigmaxi^4 + \rho \sigmaxi^2 \vert b \norm{\wgrad}_2 \vert + \rho \sigmaxi^2 \vert \nu \vert +  (1+\rho) \nu^2  \right)\\
% \end{align}
While in the high-noise regime $\sigmaxi^2$ was the dominant term in the expression for $b$, in the low noise regime the term involving $\nu^2$ is dominant. In particular, we now argue  why the choice  $\nu_0 = -\frac{  \sigmaxi^q}{\bnull^q} = O\left(\frac{1}{\log(d)}\right)$ (using the assumption on $\sigma$ in Theorem~\ref{thm:regressionlp} and that $\sigmaxi \to \sigma$) with $\bnull^2 = \frac{n \sigmaxi^2}{\dmoment{q}^2}$  is approximately optimal for $\nu$:
% By Lemma~\ref{lm:fnlpconcentration} we have that $\norm{H}_q$ concentrates around $\dmoment{q}$. Let $\bnull^2 = \frac{n \sigmaxi^2}{\dmoment{q}^2}$, 
we have $\frac{ \nu^2}{\sigmaxi^2} = \Omega(\log(d))$ and thus
\begin{equation}
 \norm{\wone+\wgt}_p^p + \norm{\wtwo}_p^p \approx (\nugt + \nu)^p + \bnull^{p} \frac{\nu^p}{\sigmaxi^p} \approx 
(1+ p\nu) + \bnull^{p} \frac{ \nu^p}{\sigmaxi^p}.
\end{equation}
Hence, as desired, we find an approximate optimal solution when choosing $\nu = \nu_0$. Further, we can again  verify that 
\begin{equation}
b^2 = \bnull^2 \frac{ \nu_0^2}{\sigmaxi^2}\left(1+ O\left(\frac{1}{\log(d)}\right) 
 \right)
\end{equation}
satisfies Equation~\eqref{eq:lpboundphinb} when applying Lemma~\ref{lm:dualnormconc}. Hence, we can conclude the proof.
% which is essentially a direct consequence of Lemma~\ref{lm:dualnormconc} and the following Lemma: 
% \begin{lemma}
% \begin{equation}
% \label{eq:lpboundrho}
%   O(\sigmaxi \rho) = \left(\nu_0+\sqrt{\frac{\mutild  n}{\dmoment{q}^2}}\right)  O\left(\frac{1}{\log(d)}\right).
% \end{equation}
% \end{lemma}
% The proof is deferred to section bla. 
%Thus, applying Lemma~\ref{lm:fnlpconcentration} the claim follows straight forwardly. 
% In particular, by Lemma~\ref{lm:fnlpconcentration} it is straight forward to check that the choice
% $$ b^2 = \bnull^2 \left(1+\right(\frac{ \nu_0^2}{\sigmaxi^4} + 
% \frac{\mutild  n}{\dmoment{q}^2}\left)(1+O\left(\frac{1}{\log(d)}\right))\right)$$
% satisfies Equation~\eqref{eq:lpboundphinb} \red{here we make use of the assumptions on n,d}. 
% Hence, in summary we obtain the upper bound:
% \begin{align}
% \phidn \leq b^p &+ (\nugt + \nu)^p \leq \bnull^p\left(1+ \frac{p}{2} \right(\frac{\nu_0^2}{\sigmaxi^2} + 
% \frac{\mutild  n}{\dmoment{q}^2}\left)(1+O\left(\frac{1}{\log(d)}\right)) + O\left(\rho \sqrt{\frac{ \nu_0^2}{\sigmaxi^2} + 
% \frac{\mutild  n}{\dmoment{q}^2}}\right) \right) \\
% &+ \nugt + p\nugt\nu_0(1+ O\left(\frac{1}{\log(d)}\right) =: \lonebound,
% \end{align}
% where we used that $\frac{\nu_0^2}{\sigmaxi^2} = O\left(\frac{1}{\log(d)}\right)$ and $\frac{\mutild  n}{\dmoment{q}^2}=O\left(\frac{1}{\log(d)}\right)$ which follows from Lemma~\ref{lm:dualnormconc} and the assumption on $\sigma$ and $d,n$.


% \paragraph{Case 2: $\frac{\log(d)}{\log\log(d)} \lesssim q \lesssim \log(d)$}
% In this case, another term appears which is responsible for the fitting of the noise. 

\end{proof}



\subsubsection{Step 2: Uniform convergence step}
The goal of the second step is again to bound the set $\Gamma_b$ from which the proof then follows. 
% For brevity of notation define $\nu := \wone$, $\eta := \norm{\wtwo}_2$ and $\nugt := 
% \wgt_1$. 
% In a first step, we use that by the definition of the sub-gradient norm, we have that $\langle w, \Hgaussian \rangle \leq \|\Hgaussian\|_q \|w\|_p$. Thus, we can relax the optimization problems: define $\Omega_b = \{ (\nu, \eta)\vert  \frac{1}{n} \norm{H}_q^2 b^2  \geq  f_n(\nu, \eta) ~~\mathrm{and}~~ (\nu+\nugt)^p + b^p \leq M \}$ and define $\numin := \min_{b\geq0, \nu} \nu \in \Omega_b, \numax := \max_{b\geq0, \nu} \nu \in \Omega_b$ and $\etamax := \max_{b\geq 0,\eta\geq 0} \eta \in \Omega_b$, we have:
% \begin{align}
%     \tag{$A_+$} \label{eq:phip}
%         \phidp \leq  \max_{\eta\geq 0 ,b\geq 0, \nu} \frac{\nu }{\sqrt{\nu^2+\eta^2}} 
%         \subjto \begin{cases}
%             \frac{1}{n} \norm{H}_q^2 b^2 \geq  \fn(\nu,\eta)\\
%           \vert \nu \vert^p+b^p \leq M
%         \end{cases}\\
%     \tag{$A_-$} \label{eq:phim}
%         \phidm \geq \min_{\eta\geq 0 ,b\geq 0, \nu} \frac{\nu }{\sqrt{\nu^2+\eta^2}} 
%         \subjto \begin{cases}
%     \frac{1}{n} \norm{H}_q^2 b^2 \geq  \fn(\nu,\eta)\\                     \vert \nu \vert+b^p \leq M
%         \end{cases}
%     \end{align}
% \begin{align}
%   \label{eq:phiplpv1}
%         \phidp \leq  \max_{\eta\geq 0 ,b\geq 0, \nu} \nu^2 +\eta^2
%         \subjto (\nu,\eta) \in \Omega_b \leq \numax^2 + \etamax^2
%     \\
%  \label{eq:phimlpv1}
%         \phidm \geq \min_{\eta\geq 0 ,b\geq 0, \nu} \nu^2 +\eta^2
%                 \subjto (\nu,\eta) \in \Omega_b \geq \numin^2
%     \end{align}
% The goal of this section is to proof the following proposition, from which the result then straight forwardly follows as described in Appendix bla. 
\begin{proposition}
\label{prop:highnoiselpreg}
Under the same conditions as in Theorem~\ref{thm:regressionlp} and for the choice $B$ as in Proposition~\ref{prop:phidnhighreg}, we have that with probability $\geq 1- c_1 d^{c_2}$ over the draws of $\Ggaussian,\Hgaussian,\Xs,\xi$ that for all $b\geq 0$ and any $\nu,\eta \in \Gamma_b$:


\end{proposition}

%  As a consequence of Proposition~\ref{prop:highnoiselpreg}  upper respectively lower bound Equation~\eqref{eq:phiplpv1},\eqref{eq:phimlpv1} by:
% \begin{align}
%         \phidp \leq   \frac{\sgn(\numax) }{\sqrt{1+\frac{\etamax^2}{\numax^2}}} 
%     ~~\mathrm{and}~~ \phidm \geq  \frac{\sgn(\numin) }{\sqrt{1+\frac{\etamax^2}{\numin^2}}} 
%     \end{align}





\begin{proof}
% Before being able to exploit the Lemma 1, we first need to show that $\nu, \eta = O\left(\frac{1}{\log(d)}\right)$. This follows from iterative naively bounding $\nu, \eta$ based on the relaxation $\|\wtwo\|_p^p \leq B$, which implies that $\frac{1}{n} \norm{H}_q^2 B^{2/p}  \geq  f_n(\nu, \eta) $.
The proof is again divided into two steps:

% \paragraph{Step 1, naive bound 1.} By Lemma \ref{lemma_quadratic_plus_fstar_bound} we have that $f_n(\nu, \eta) \geq c_1 \nu^2 + c_2 \eta^2$. Thus, we obtain the first naive upper bound
% \begin{equation}
%     \frac{B^{2/p}\|\Hgaussian\|_q^2}{n} \geq  c_1 \nu^2 + c_2 \eta^2
% \end{equation}
% In particular, applying Lemma concentration, we obtain that with high probability $\geq 1- c_1 d^{-c_2}$, 
% \begin{align}
% \label{eq:bound1lpeq}
%         \nu^2 + \eta^2 = O(\sigmaxi^2) 
% \end{align}

\paragraph{Step 1, naive bound 1.} 


% Following the same argument as in \cite{wang2021tight} Lemma bla, we have uniformly over $\nu, \eta$,  with probability $\geq 1-c_1d^{c_2}$ over the draws of $\Ggaussian,\xi,\Xs$ that
% \begin{equation}
%     \fn(\nu,\eta) \geq (1-O(\rho))(\sigma^2 + \nu^2 + \eta^2). 
% \end{equation}

% Hence, conditioning on the event where Equation~\eqref{eq:bound1lpeq} holds for some universal constant, we can apply Lemma concentration 2, which allows us to upper bound:
% \begin{equation}
%     \frac{B^{2/p}\|\Hgaussian\|_q^2}{n} \geq  \left(\sigma^2 +   \nu^2 +  \eta^2\right)(1+O(\rho))
% \end{equation}

In a first step, we again use the lower bound for $\fn$ from Equation \eqref{eq:regressionfn2}. In particular, note that $\lonebound = O(1)$ and thus, we have that 
\begin{equation}
\label{eq:bound2lpeqlownoise}
   \nu^2 +  \eta^2 = O\left(\frac{\norm{H}_q^2}{n}\right) = O\left(\frac{1}{\log(d)}\right).
\end{equation}




\paragraph{Step 2, tight bound for $\nu$ and upper bound for $\eta$.}
% Conditioning on the event where Equation~\eqref{eq:bound2lpeq} holds and thus $\Omega \subset \{(\nu,\eta) \vert \vert \nu - \nugt\vert \leq O\left(\frac{1}{\log(d)}\right)  ~~\mathrm{and}~~ \eta \leq O\left(\frac{1}{\log(d)}\right)\}$, we can 

Conditioning on Equation~\eqref{eq:bound2lpeqlownoise} we have
\begin{align}
   0 &\leq  b^p \leq \lonebound - (\nugt + \nu)^p =  \bnull^p \frac{\nu_0^p}{\sigmaxi^p}  \left(1+ O\left(\frac{1}{\log(d)}\right) 
 \right)
% \frac{\mutild  n}{\dmoment{q}^2}\right)(1+O\left(\frac{1}{\log(d)}\right)) + O\left(\rho \sqrt{\frac{ \nu_0^2}{\sigmaxi^2} + 
% \frac{\mutild  n}{\dmoment{q}^2}}\right) \right) \\
+ \nugt + p\nu_0\left(1+ O(\log(d)^{-1})\right) - \nugt - p  \nu (1+ O(\log(d)^{-1}) \\
&= \frac{\sigmaxi^q}{\bnull^q} (1 - p) (1+ O(\log(d)^{-1})
% \frac{\mutild  n}{\dmoment{q}^2}\right)(1+O\left(\frac{1}{\log(d)}\right)) + O\left(\rho \sqrt{\frac{ \nu_0^2}{\sigmaxi^2} + 
% \frac{\mutild  n}{\dmoment{q}^2}}\right) \right) \\
- \nugt - p  \nu (1+ O(\log(d)^{-1}) \\
\end{align}
As a result, we immediately obtain the lower bound for \begin{equation}
    \vert \nu\vert \geq \frac{p-1}{p} \frac{\nugt}{\bnull^q} ( 1+  O(\log(d)^{-1}))
\end{equation}
We now argue that this gives us the correct rate for $\nu$ up to a factor of $q$, i.e. we show $ \vert \nu\vert  = O(\frac{\sigmaxi^q}{\bnull^q})$. Thus, we can assume that $\nu = \frac{\sigmaxi^q}{\bnull^q} \nutild +  \frac{1-p}{p} \frac{ \sigmaxi^q}{\bnull^q} ( 1+  O(\log(d)^{-1}))$ with $\nutild \leq -\nugt$. We have $b^p \leq \frac{ \sigmaxi^{q}}{\bnull^q} p \vert \nutild\vert (1+O\left(\frac{1}{\log(d)}\right))$. Further, following the same argument as used for Equation~\eqref{eq:lpreghighnoisestep1}, we obtain the condition:
\begin{align}
    &\frac{b^2\|\Hgaussian\|_q^2}{n} \geq  \left(\sigma^2 +   \nu^2 +  \eta^2\right)(1+O(\rho))\\
\implies &\frac{\sigmaxi^{2q/p}}{\bnull^{2q/p}} p^{2/p} \vert \nutild \vert ^{2/p} \frac{\sigmaxi^2}{\bnull^2} (1+ O\left(\frac{1}{\log(d)}\right)) \geq \left(\sigma^2 +   \nu^2 +  \eta^2\right)(1+O(\rho))
\end{align}
We now make twice use of this equation. First to upper bound $\vert \nu\vert$ and then to upper bound $\eta^2$. 
For the upper bound on $\nu^2$, we can further relax to:
\begin{align}
&\frac{ \sigmaxi^{2q/p}}{\bnull^{2q/p}} p^{2/p} \vert \nutild \vert ^{2/p} \frac{\sigmaxi^2}{\bnull^2} (1+ O\left(\frac{1}{\log(d)}\right)) \geq   \nu^2 +  \eta^2(1+O(\rho))\\
\implies & \frac{ \sigmaxi^{2q}}{\bnull^{2q}} p^{2/p} \vert \nutild \vert ^{2/p} (1+ O\left(\frac{1}{\log(d)}\right))  \geq   \vert \nu \vert^2  \geq \nutild^2 \frac{\sigmaxi^{2q}}{\bnull^{2q}}\\
\implies &  p^{2/p} (1+ O\left(\frac{1}{\log(d)}\right))  \geq   \vert \nutild \vert^{2/q} \implies \vert \nutild \vert = O(1),
\end{align}
as desired. Finally, following the same argument for $\eta$, we obtain $\eta^2 = O(\frac{ \sigmaxi^{2q/p}}{\bnull^{2q/p}})$
and thus we can conclude the proof. 






% In a second step, we apply again Lemma~\ref{eq:regressionfn}, which allows us to relax the first constraints in $\Omega$ to 
% \begin{align}
% \label{eq:lptightcond1}
%      \frac{1}{n} \norm{H}_q^2 b^2 \geq   \fn(\wone,\|\wtwo\|_2) &\geq  \sigmaxi^2 + \nu^2  + \eta^2  +(\nu^2 + \eta^2) O\left(\frac{1}{\log(d)}\right) +  O( \rho(\nu + \eta)) 
%      \end{align}


% % Using the fact that with high probability $\eta^2 + \nu^2 \leq c \sigmax^2$, we can lower bound (using $\delta = c\sqrt{\frac
% % {\log(d)}{n}}$):
% % \begin{equation}
% %     \frac{1}{n} \fn \geq \sigmaxi^4 + ( v - \sigmaxi^2 \delta)^2 + (\nu - \sigmaxi^2 \delta)^2 - 2 \sigmaxi^4 \delta^2 
% % \end{equation}
% % Thus, we obtain the conditions:
% % \begin{align}
% % \frac{1}{n} \innerprod{\wtwo}{\Ggaussian}^2 \geq  \sigmaxi^4 + ( v - \sigmaxi^2 \delta)^2 + (\nu - \sigmaxi^2 \delta)^2 - 2 \sigmaxi^4 \delta^2 \\
% % (\nu+\nugt)^p + \norm{\wtwo}_p^p \leq \lonebound
% % \end{align}
% Furthermore, the second constraint in $\Omega$ states that $b^p \leq \lonebound - (\nu+\nugt)^p$ with $\lonebound$ from Proposition \ref{prop:phipnboundreglp}. Thus, by definition, we have:
% \begin{align}
% \label{eq:lptightcond2}
%     b^p \leq \lonebound - (\nu+\nugt)^p &= \bnull^p\left(1+ \frac{p}{2} \right(\frac{\nu_0^2}{\sigmaxi^2} + 
% \frac{\mutild  n}{\dmoment{q}^2}\left)(1+O\left(\frac{1}{\log(d)}\right))\right) + p\nugt\left(\nu_0-\nu\right)(1+ O\left(\frac{1}{\log(d)}\right),
% \end{align}
% where we have used that $\nu = O\left(\frac{1}{\log(d)}\right)$ since we condition on Equation~\eqref{eq:bound2lpeq}. Further, using the Taylorseries approximation for $(1+x)^{2/p} = 1 + \frac{2}{p} x + O(x^2)$, we get
% \begin{align}
%     \frac{1}{n} \norm{H}_q^2 b^2 &\leq   \frac{1}{n} \norm{H}_q^2 \bnull^2\left(1+ \left(\frac{\nu_0^2}{\sigmaxi^2} + 
% \frac{\mutild  n}{\dmoment{q}^2}\right)(1+O\left(\frac{1}{\log(d)}\right)) \right. \\ &+ \left.  O\left(\rho \sqrt{\frac{ \nu_0^2}{\sigmaxi^2} + 
% \frac{\mutild  n}{\dmoment{q}^2}}\right)  + \frac{2\nugt}{\bnull^p}\left(\nu_0-\nu\right)(1+ O\left(\frac{1}{\log(d)}\right)\right) \\
% &=
% \sigmaxi^2 \left(1+ \left(\frac{\nu_0^2}{\sigmaxi^2} + 
% \frac{\mutild  n}{\dmoment{q}^2}\right)(1+O\left(\frac{1}{\log(d)}\right)) +  O\left(\rho \sqrt{\frac{ \nu_0^2}{\sigmaxi^2} + 
% \frac{\mutild  n}{\dmoment{q}^2}}\right)  - \frac{2\nu_0 \left(\nu_0-\nu\right)}{\sigmaxi^2}(1+ O\left(\frac{1}{\log(d)}\right)\right)   \\
% &=\sigmaxi^2 + \left(\nu_0^2+
% \frac{\mutild \sigmaxi^2 n}{\dmoment{q}^2} - 2\nu_0 \left(\nu_0-\nu\right) \right)(1+O\left(\frac{1}{\log(d)}\right)) +  O\left(\sigmaxi^2\rho \sqrt{\frac{ \nu_0^2}{\sigmaxi^2} + 
% \frac{\mutild  n}{\dmoment{q}^2}}\right) \\
% &= \sigmaxi^2 + \left( 
% \frac{\mutild \sigmaxi^2 n}{\dmoment{q}^2} + 2\nu_0 \nu - \nu_0^2  \right)(1+O\left(\frac{1}{\log(d)}\right)) +  O\left(\sigmaxi^2\rho \sqrt{\frac{ \nu_0^2}{\sigmaxi^2} + 
% \frac{\mutild  n}{\dmoment{q}^2}}\right) 
% \label{eq:lpboundonb}
% \end{align}

% where we used Lemma concentration in the second line, in the third line that $\frac{\bnull \dmoment{q}^2}{n} = \sigmaxi^2$ and that $\nu_0  = -\frac{ \nugt \sigmaxi^2}{\bnull^p}$ by definition. Plugging the inequality from Equation~\eqref{eq:lpboundonb} in  Equation~\eqref{eq:lptightcond1}, we obtain:
% \begin{align}
% \label{eq:lptightcond1}
%      &\sigmaxi^2 + \left( 
% \frac{\mutild \sigmaxi^2 n}{\dmoment{q}^2} + 2\nu_0 \nu - \nu_0^2  \right)(1+O\left(\frac{1}{\log(d)}\right)) + O\left(\sigmaxi^2 \rho \sqrt{\frac{ \nu_0^2}{\sigmaxi^2} + 
% \frac{\mutild  n}{\dmoment{q}^2}}\right) 
% \\
% &\geq   \sigmaxi^2 + \nu^2  + \eta^2  +(\nu^2 + \eta^2) O(\rho) +  O( \sigmaxi\rho(\nu + \eta)) \\
% \implies &\left( 
% \frac{\mutild \sigmaxi^2 n}{\dmoment{q}^2} + 2\nu_0 \nu - \nu_0^2  \right)(1+O\left(\frac{1}{\log(d)}\right))
% + O\left(\sigmaxi^2 \rho \sqrt{\frac{ \nu_0^2}{\sigmaxi^2} + 
% \frac{\mutild  n}{\dmoment{q}^2}}\right) 
% \geq  \left(\nu^2  + \eta^2 \right) (1+ O(\rho)) +  O(\sigmaxi \rho(\nu + \eta))\\
% \implies &\left( 
% \frac{\mutild \sigmaxi^2 n}{\dmoment{q}^2} - \nu_0^2  \right)(1+O\left(\frac{1}{\log(d)}\right)) + O\left( \sigmaxi^2 \rho \sqrt{\frac{ \nu_0^2}{\sigmaxi^2} + 
% \frac{\mutild  n}{\dmoment{q}^2}}\right) 
% \geq  \left( \nu- \nu_0- c\rho\sigmaxi\right)^2 - \left( \eta- c\rho\sigmaxi\right)^2  - \nu_0^2 -2\sigmaxi^2c^2\rho^2 - 2 \nu_0 c\sigmaxi \rho \\
% \implies & 
% \frac{\mutild \sigmaxi^2 n}{\dmoment{q}^2}(1+O\left(\frac{1}{\log(d)}\right)) + O( \nu_0^2\log(d)^{-1}) + O\left( \sigmaxi^2 \rho \sqrt{\frac{ \nu_0^2}{\sigmaxi^2} + 
% \frac{\mutild  n}{\dmoment{q}^2}}\right) 
% \geq  \left( \nu- \nu_0- c\sigmaxi\rho\right)^2 + \left( \eta- c\sigmaxi\rho\right)^2  
% \end{align}
% where we have used in the second line Equation~\eqref{eq:lpboundrho} and let $c>0$ in the third line be a universal constant. 

% Hence, we obtain the desired bounds and thus can conclude the proof. 


% \begin{align}
%     ( \nu - \nu_0)^2 &\leq \frac{ \mutild \sigmaxi^2 n}{\dmoment{q}^2}(1+O\left(\frac{1}{\log(d)}\right)) + O( \nu_0^2\log(d)^{-1}) + O\left( \sigmaxi^2 \rho \sqrt{\frac{ \nu_0^2}{\sigmaxi^2} + 
% \frac{\mutild  n}{\dmoment{q}^2}}\right) 
%     \\
%     ~\mathrm{and}~\eta^2 &\leq \frac{ \mutild \sigmaxi^2 n}{\dmoment{q}^2}(1+O\left(\frac{1}{\log(d)}\right)) + O( \nu_0^2\log(d)^{-1}) + O\left( \sigmaxi^2 \rho \sqrt{\frac{ \nu_0^2}{\sigmaxi^2} + 
% \frac{\mutild  n}{\dmoment{q}^2}}\right) 
% \end{align}

% \paragraph{Step 3, tight bound for $\eta$.}







% And therefore
% \begin{align}
%     T^{2/p}\|\Ggaussian\|_q^2 &\leq b^2\left(1+ 2\nugt \frac{\nu - \nu_0}{b^p} +O(\nugt^{p-2}\frac{\nu_0^2+\nu^2}{b^p})\right)\|\Ggaussian\|_q^2 \\
%     &\leq \bnull^2 \left(1+\right(\frac{\nu_0^2}{\sigmaxi^4} + 
% \frac{\mutild  n}{\dmoment{q}^2}\left)(1+O\left(\frac{1}{\log(d)}\right)) \right)\left(1+ 2\nugt \frac{\nu - \nu_0}{b^p} +O(\nugt^{p-2}\frac{\nu_0^2+\nu^2}{b^p})\right)\|\Ggaussian\|_q^2\\
% &\leq \bnull^2 \left(1+\left( \frac{\nu_0^2}{\sigmaxi^4} + 
% \frac{\mutild  n}{\dmoment{q}^2} \right)(1+O\left(\frac{1}{\log(d)}\right)) +  2\nugt \frac{\nu - \nu_0}{b^p} +O(\nugt^{p-2}\frac{\nu_0^2+\nu^2}{b^p})\right)\|\Ggaussian\|_q^2\\
% &\leq \bnull^2\dmoment{q}^2 \left(1+\left( \frac{\nu_0^2}{\sigmaxi^4} + 
% \frac{\mutild  n}{\dmoment{q}^2} \right)(1+O\left(\frac{1}{\log(d)}\right)) +  2\nugt \frac{\nu - \nu_0}{b^p} +O(\nugt^{p-2}\frac{\nu_0^2+\nu^2}{b^p})\right)\\
% \end{align}
% Next, using the fact that by definition $\bnull = \frac{n \sigmaxi^4}{\dmoment{q}^2}$, and plugin in the upper bound for $T^{2/q} \|\Ggaussian\|_q$, we have the upper bound
% \begin{align}
% &\bnull^2\dmoment{q}^2 \left(1+\left( \frac{\nu_0^2}{\sigmaxi^4} + 
% \frac{\mutild  n}{\dmoment{q}^2} \right)(1+O\left(\frac{1}{\log(d)}\right)) +  2\nugt \frac{\nu - \nu_0}{b^p} +O(\nugt^{p-2}\frac{\nu_0^2+\nu^2}{b^p})\right) \\ \geq& 
% \sigmaxi^4 + ( v - \sigmaxi^2 \delta)^2 + (\nu - \sigmaxi^2 \delta)^2 - 2 \sigmaxi^4 \delta^2
% \\
% \impliedby &\sigmaxi^4\left(\left( \frac{\nu_0^2}{\sigmaxi^4} + 
% \frac{\mutild  n}{\dmoment{q}^2} \right)(1+O\left(\frac{1}{\log(d)}\right)) +  2\nugt \frac{\nu - \nu_0}{b^p} +O(\nugt^{p-2}\frac{\nu_0^2+\nu^2}{b^p})\right) \\ \geq& 
% ( v - \sigmaxi^2 \delta)^2 + (\nu - \sigmaxi^2 \delta)^2 - 2 \sigmaxi^4 \delta^2 \\
% \impliedby &\nu_0^2 O\left(\frac{1}{\log(d)}\right) + \sigmaxi^4\left(  
% \frac{\mutild  n}{\dmoment{q}^2} \right)(1+O\left(\frac{1}{\log(d)}\right)) +   2 \sigmaxi^4 \delta^2 \\ \geq& 
% ( v - \sigmaxi^2 \delta)^2 + (\nu - \sigmaxi^2 \delta)^2 -  \nu \nu_0  +O(\nu_0^3+\nu^2\nu_0) +   2 \sigmaxi^4 \delta^2 \\
% \impliedby &\nu_0^2 (-1+O\left(\frac{1}{\log(d)}\right)) + \sigmaxi^4\left(  
% \frac{\mutild  n}{\dmoment{q}^2} \right)(1+O\left(\frac{1}{\log(d)}\right))  \geq
% ( \eta - \sigmaxi^2 \delta)^2 + (\nu - \sigmaxi^2 \delta)^2 -  \nu \nu_0  +O(\nu^2\nu_0)
% \\
% \impliedby \tilde{T} := &\nu_0^2 (O\left(\frac{1}{\log(d)}\right)) + \sigmaxi^4\left(  
% \frac{\mutild  n}{\dmoment{q}^2} \right)(1+O\left(\frac{1}{\log(d)}\right))  +   2 \sigmaxi^4 \delta^2 
% + 2 \sigmaxi^2 \delta \nu_0 \geq
% ( \eta - \sigmaxi^2 \delta)^2 + (\nu - \sigmaxi^2 \delta-\nu_0)^2 
% \end{align}

% Therefore, we get that 
% \begin{align}
%     \eta \leq \sigmaxi^2 \delta + \sqrt{\tilde{T}} \implies \eta^2 \lesssim \tilde{T} \\
%   \vert \nu \vert \leq \nu_0 + \sigmaxi^2 \delta + \sqrt{\tilde{T}} \implies   \nu^2 \lesssim \nu_0^2 + \tilde{T}
% \end{align}
% \red{we use here that $\nu_0 \gtrsim \sigmaxi^2 \delta$.}
%  Furthermore, we have
% \begin{align}
%     \nu_0 + \sigmaxi^2 \delta - \sqrt{\tilde{T}}  \leq \vert \nu \vert \implies \nu^2 \gtrsim ...
% \end{align}


\end{proof}




==> ICML 22-3/sections_proof/section_CGMT.tex <==
\subsection{Proof of Proposition \ref{prop:CGMT_application_classification}: Application of the (C)GMT for classification}
\label{apx:subsec:cgmtproof}

% \subsection{Proof of Proposition~\ref{prop:CGMT_application_classification}: CGMT}
% \label{apx:subsec:cgmtproof}
% \red{Stefan, can you take care of this one? not yet worked on this}
% Proof of this proposition is based on (Convex) Gaussian Minimax Theorem \cite{gordon1988milman,thrampoulidis2015regularized} which relates auxiliary optimization $\PhiCdn$, $\PhiCdp$ and $\PhiCdm$ with vector random variables with $\PhiCN$, $\PhiCp$ and $\PhiCm$ depending on random matrix $\matX$. 
The proof essentially follows exactly the same steps as in \cite{koehler2021uniform} except for a few simple modifications which we describe next. First we introduce a more general form of  the (C)GMT:

\begin{lemma}
\label{lemma:CGMT_variant}
Let $X'' \in \RR^{n\times {d-s}}$ be a matrix with i.i.d. $\NNN(0,1)$ entries and let $\Ggaussian \sim \NNN(0,I_n)$ and $H \sim \NNN(0,I_{d-s})$ be independent random vectors. Let $\compactw \subset \RR^{s}\times \RR^{d-s}$ and $\compactv \subset \RR^{n}$ be compact sets, and let $\psi: \compactw \times \compactv \to \RR$ be a continuous function. Then for the following two optimization problems:
    \begin{equation}
        \Phi = \min_{(\wone,\wtwo)\in \compactw}\max_{v\in \compactv} \innerprod{v}{X'' \wtwo} + \psifcn((\wone,\wtwo),v)
    \end{equation}
    \begin{equation}
        \phi = \min_{(\wone,\wtwo)\in \compactw}\max_{v \in \compactv} \norm{\wtwo}_2\innerprod{v}{G} + \norm{v}_2\innerprod{\wtwo}{H}+\psifcn((\wone,\wtwo),v)
    \end{equation}
    and any $t\in\RR$ holds that:
    \begin{equation}
        \prob(\Phi < t)\leq 2\prob(\phi \leq t) 
    \end{equation}
    
    If in addition $\psi$ is convex-concave function we also have for any $t\in\RR$:
    \begin{equation}
        \prob(\Phi > t)\leq 2\prob(\phi \geq t) 
    \end{equation}
    In both inequalities the probabilities on the LHS and RHS are over the draws of $X''$, and of $G$, $H$, respectively.
\end{lemma}
% Similarly we can give a more general statement of the CGMT which includes additional variables affecting only the deterministic term in the problem. Namely, we have:
% \begin{lemma}
% \label{lemma:CGMT_variant}
% Let $\matX'' \in \RR^{n\times {d-s}}$ be a matrix with i.i.d. $\NNN(0,1)$ entries and let $\Ggaussian \sim \NNN(0,I_n)$ and $\Hgaussian \sim \NNN(0,I_{d-s})$ independent of $\matX$ and each other. Let $\compactw \subset \RR^{s}\times \RR^{d-s}$ and $\compactv \subset \RR^{n}$ be compact and convex sets, and let $\psi: \compactw \times \compactv \to \RR$ be continuous convex-concave function. Then for the following two optimization problems:
%     \begin{equation}
%         \Phi = \min_{(\wone,\wtwo)\in \compactw}\max_{v\in \compactv} \innerprod{v}{\matX'' \wtwo} + \psifcn((\wone,\wtwo),v)
%     \end{equation}
%     \begin{equation}
%         \phi = \min_{(\wone,\wtwo)\in \compactw}\max_{v \in \compactv} \norm{\wtwo}_2\innerprod{G}{v} + \norm{v}_2\innerprod{H}{\wtwo}+\psifcn((\wone,\wtwo),v)
%     \end{equation}
%     and any $t\in\RR$ holds that:
%     \begin{equation}
%         \prob(\Phi>t)\leq 2\prob(\phi\geq t) 
%     \end{equation}
%     where the probabilities on the LHS and RHS are over the draws of $\matX''$, and of $G$, $H$, respectively
% \end{lemma}
\begin{proof}
The first part of the lemma is equivalent to Theorem 10 in \cite{koehler2021uniform}. The proof of the second part follows from Theorem 9 in \cite{koehler2021uniform} and proof of Theorem 10 in \cite{koehler2021uniform}.
\end{proof}
% The proof of this theorem follows from Theorem 10 in \cite{koehler2021uniform} and proof of CGMT as discussed in Theorem 3 in \cite{thrampoulidis2015regularized}.

We first rewrite $\PhiCN$  using the Lagrange multipliers $\lmult\in\RR^n$ to be able to apply Lemma \ref{lemma:CGMT_variant}:
\begin{align}
    \PhiCN 
    % = \min_{w} \max_{\lmult\geq 0} \norm{w}_p^p + \sumin \lmult_i                 (1-y_i\innerprod{x_i}{w})
      &= \min_{w} \max_{\lmult\geq 0} \norm{w}_p^p + \innerprod{\lmult}{\onevec - \matDy\matX w}
% \end{align}
% Rewriting this optimization problem in terms of $\wone$ and $\wtwo$ we get:
% \begin{align}
%     \PhiCN = \min_{(\wone,\wtwo)} \max_{\lmult\geq 0} \norm{\wone}_p^p + \norm{\wtwo}_p^p + \transp{\lmult}\onevec - \transp{\lmult}\matDy\matX'' \wone- \transp{\lmult}\matDy\matX'' \wtwo
% \end{align}
% \begin{align}
    &= \min_{(\wone,\wtwo)} \max_{\lmult\geq 0} \norm{\wone}_p^p + \norm{\wtwo}_p^p + \innerprod{\lmult}{\onevec - \matDy\matXs \wone} - \innerprod{\matDy\lmult}{\matXsc \wtwo}
\end{align}
where $\matDy = \mathrm{diag}(y_1,y_2,\dots,y_n)$ and $\matXsc$ is the sub-matrix containing the  $d-s$ columns of $X$ from the complement of the support of $\wstar$.
We  note that $\matDy\matX \in \RR^{n\times d}$ has i.i.d. entries distributed according to the standard normal distribution and that the random matrices $-\matXsc$ and $\matXsc$ have the same distribution. Also, the function $\psi((\wone,\wtwo),\lmult) := \norm{\wone}_p^p + \norm{\wtwo}_p^p + \innerprod{\lmult}{ \onevec - \matDy \matXs \wone}$ is a continuous convex-concave function on the whole domain. 
%, we need to ensure that we optimize over compact sets, which we discuss after the following paragraph. Nonetheless, motivated by Lemma \ref{lemma:CGMT_variant} we can define: \fy{the last two sentences don't flow}
We further define
\begin{align}
    \PhiCdn &= \min_{(\wone,\wtwo)} \max_{\lmult\geq 0} \norm{\wone}_p^p + \norm{\wtwo}_p^p + \innerprod{\lmult}{\onevec - \matDy\matXs \wone} - \norm{\wtwo}_2 \innerprod{\matDy \lmult}{ \Ggaussian} - \norm{\matDy\lmult}_2 \innerprod{\wtwo}{\Hgaussian}\\
    % &= \min_{(\wone,\wtwo)} \max_{\lmult\geq 0} \norm{\wone}_p^p + \norm{\wtwo}_p^p + \transp{\lmult}(\onevec - \matDy\matXs \wone- \matDy \Ggaussian\norm{\wtwo}_2) - \norm{\lmult}_2\transp{\Hgaussian}\wtwo\\
    &= \min_{(\wone,\wtwo)} \max_{\lambda\geq 0} \norm{\wone}_p^p + \norm{\wtwo}_p^p - \lambda \left(\innerprod{\wtwo}{\Hgaussian}-\norm{\pos{\onevec - \matDy\matXs \wone- \matDy \Ggaussian\norm{\wtwo}_2}}_2 \right) \\
    % & = \min_{(\wone,\wtwo)} \max_{\lambda\geq 0} \norm{\wone}_p^p + \norm{\wtwo}_p^p - \lambda(\innerprod{\wtwo}{\Hgaussian}-\norm{\pos{\onevec - \matDy\matXs \wone- \matDy \Ggaussian\norm{\wtwo}_2}}_2\\
    & = \min_{(\wone,\wtwo)} \norm{\wone}_p^p + \norm{\wtwo}_p^p
    \subjto \innerprod{\wtwo}{\Hgaussian}\geq \norm{\pos{\onevec - \matDy\matXs \wone- \matDy \Ggaussian\norm{\wtwo}_2}}_2
\end{align}
where in the second equality we set $\lambda:= \norm{\lmult}_2$. Since $\norm{\wtwo}_p^p$ and $\norm{\wtwo}_2$ do not depend on the signs of the entries of $\wtwo$, any minimizer $w = (\wone, \wtwo)$ of $\PhiCdn$ satisfies $\innerprod{\wtwo}{H}\geq 0$. Hence squaring the last inequality and scaling with $\frac{1}{n}$, we note that the RHS is given by
    \begin{align}
    \frac{1}{n}\norm{\pos{\onevec - \matDy\matXs \wone- \matDy \Ggaussian\norm{\wtwo}_2}}_2^2 = \frac{1}{n} \sumin \possq{1-\xi_i\sgn(\langle \xsui, \wgtp \rangle) \langle \xsui, \wone \rangle -\Ggaussian_i \norm{\wtwo}_2}, 
    \end{align}
which is exactly the function $\fnclas(\wone, \norm{\wtwo}_2)$, as defined in Equation \eqref{eq:fnclas_def}. Hence, we obtain the desired expression for $\PhiCdn$ in Proposition~\ref{prop:CGMT_application_classification}.

In order to complete the proof of the proposition, we need to discuss
compactness of the feasible sets in the optimization problem 
so that we can apply Lemma~\ref{lemma:CGMT_variant}.
% Let's now define truncated optimization problem:
% \begin{align}
%         \PhiCN^r(t) = \min_{\norm{\wone}+\norm{\wtwo}\leq t} \max_{\lmult\geq 0,\norm{\lmult}\leq r} \norm{\wone}_p^p + \norm{\wtwo}_p^p + \transp{\lmult}\onevec - \transp{\lmult}\matDy\matXs \wone- \transp{\lmult}\matDy \matXsc \wtwo
% \end{align}
%We now discuss the problem of the compactness of the underlying optimization sets.
For this purpose, we define the following truncated optimization problems $\PhiCN^r(t)$ and $\PhiCdn^r(t)$ for some $r,t \geq 0$:
\begin{align}
    \PhiCN^r(t) &:= \min_{\norm{w}_p^p\leq t} \max_{\substack{\norm{v}\leq r\\ v\geq 0}} \norm{w}_p^p + \innerprod{v}{1-D_y X w}
    \\
    \PhiCdn^r(t) &:= \min_{\norm{\wone}_p^p+\norm{\wtwo}_p^p \leq t} \max_{0\leq \lambda\leq n r} \norm{\wone}_p^p + \norm{\wtwo}_p^p - \lambda \left(  \frac{1}{n}\innerprod{\wtwo}{\Hgaussian}^2 - \fnclas(\wone,\|\wtwo\|_2) \right).
\end{align}
By definition it then follow that %\fy{uh would be useful to have half sentence of explanation?}
\begin{equation}
        \PP ( \PhiCN > t | \xi, X') \leq \inf_{r\geq 0} \PP (\PhiCN^r(t) > t | \xi,X').
\end{equation}
Furthermore, by making use of the simple (linear) dependency on $\lambda$ in the optimization objective in the definition of $\PhiCdn$,  a standard limit argument as in the proof of Lemma 7 in \cite{koehler2021uniform} shows that:
\begin{align}
    %\PP ( \PhiCN > t | \xi, X') \leq \inf_{r\geq 0} \PP (\PhiCN^r(t) > t | \xi,X')\\
    \PP (\PhiCdn \geq t | \xi, X') \geq \inf_{r\geq 0} \PP (\PhiCdn^r(t) \geq t | \xi, X')
\end{align}
Finally, the proof follows when noting that we can apply Lemma~\ref{lemma:CGMT_variant} directly to $\PhiCN^r(t)$ and $\PhiCdn^r(t)$ for any $r,t\geq 0$, which gives us $\prob(\PhiCN^r>t|\xi,\Xs) \leq 2\prob(\PhiCdn^r\geq t|\xi,\Xs)$. Combining the previous two statements completes the proof for $\PhiCN$.

% \begin{align}
%     \PhiCdn^r(t) &= \min_{\norm{\wone}+\norm{\wtwo}\leq t} \max_{\lmult\geq 0,\norm{\lmult}\leq r} \norm{\wone}_p^p + \norm{\wtwo}_p^p + \transp{\lmult}\onevec - \transp{\lmult}\matDy\matXs \wone- \transp{\lmult} \matDy \Ggaussian\norm{\wtwo}_2 - \norm{\transp{\lmult}\matDy}_2\transp{\Hgaussian}\wtwo
% \end{align}

% Combining previous results we have that:
% \begin{align}
%     \prob(\PhiCN^r(t)>t)\leq 2\prob(\PhiCdn^r(t)\geq t) .....\lim_{r\to\infty}\prob(\PhiCdn^r(t)\geq t)\leq \prob(\PhiCdn\geq t)
% \end{align}

The proof for $\PhiCp$ and $\PhiCm$ uses the same steps as discussed above. We only detail the proof for $\PhiCm$ here, as the the proof for $\PhiCp$ follows from the exact same reasoning.
Let $\BBB_p(M) = \{w\in\RRR^d: \norm{w}_p^p \leq M \}$ be an $l_p$-ball of radius $M$ and note that we optimize over $(\wone,\wtwo)\in \compactw$ where $\compactw = \setSdelta \cap \BBB_p(\loneboundclas)$ is a compact set for $\delta>0$ sufficiently small. Furthermore, define the function $\psi$ by $\psi((\wone,\wtwo),v) := \frac{\innerprod{\wone}{\wgtp}}{\sqrt{\norm{\wone}_2^2+\norm{\wtwo}_2^2}} + \innerprod{v}{\onevec - \matDy \matXs \wone}$, which is a continuous function on $\compactw$. Similarly as above, we can overcome the issue with the compactness of the set $\compactv$ by using a truncation argument as proposed in Lemma 4 in \cite{koehler2021uniform}. In particular, we define
\begin{align}
    \PhiCm^r&:= \min_{\substack{w\in \setSdelta\\ \norm{w}_p^p \leq \loneboundclas}} \max_{\substack{\norm{v}\leq r\\ v\geq 0}} \frac{\langle w, \wgt \rangle}{\norm{w}_2}  + \innerprod{v}{1-D_y X w},
    \\
    \PhiCdm^r &:= \min_{\substack{(\wone,\wtwo)\in \setSdelta\\ \norm{\wone}_p^p+\norm{\wtwo}_p^p \leq \loneboundclas}} \max_{0 \leq \lambda\leq n r} \frac{\langle \wone, \wgtp \rangle }{\sqrt{\norm{\wone}_2^2+\norm{\wtwo}_2^2}} - \lambda \left( \frac{1}{n}\innerprod{\wtwo}{\Hgaussian}^2 - \fnclas(\wone,\|\wtwo\|_2) \right)
\end{align}
for which we have
\begin{align}
    \PP(\PhiCm < t| \xi,X') &\leq \inf_{r\geq 0} \PP(\PhiCm^r < t | \xi,X')\\
    \text{ and } \: \PP(\PhiCdm \leq t|\xi,X') &\geq \inf_{r\geq 0} \PP(\PhiCdm^r \leq t| \xi,X').
\end{align}
We note that the first statement again follows from the definition of $\PhiCm$,  while the second statement follows from a limit argument as in Lemma 4 in \cite{koehler2021uniform}. Finally, we conclude the proof by applying the first part of Lemma~\ref{lemma:CGMT_variant} to $\PhiCm^r$ and $\PhiCdm^r$. 
%above mentioned inequalities we conclude the proof.
% \begin{remark}
% Say that this can be generalized?
% \end{remark}




==> sections/experiments.tex <==




% \section{Empirical results}
% % I suggest the following structure here: Scope ( at most 3/4 of a page!)
% % \begin{itemize}
% %     \item Regression lp - Indeed, we can see that the optimal p is in (1,2). We wonder whether this trade-off is also captured by the bias and variance terms =... . Indeed, as we can see, one term goes down and one goes up. We discuss the relation between the bias variance trade-off and Thm 1 in the future work section (because currently it is not well understood). 
% %     \item We also observe this trade-off for classification with lp-svm on synthetic data. 
% %     \item While real world regression data sets are usually inherently noisy and thus regularized estimators are a nat ural choice, classification datasets used in real world examples can sometimes also be considered as noiselss (when being labeled by some human representing the  ground truth). Thus, the use of hard margin support vector machine relevant in practice ( cite here). Figure bla the performance with respect to $p$. We observe that in the noiseless case $p=1$ performs indeed the best. However, in the presence of random label flips, we observe that the expected trade-off occurs. \red{i feel like this real world motivation is quite weak...}
% % \end{itemize}


% We saw from the results in the previous two sections that $p\in(1,2)$ achieves faster rates compared to $p=1,2$. In this section we present numerical simulations addressing the following two question: is the optimal $p$ also attained in $(1,2)$ for finite $n,d$ of practically relevant order? Furthermore, can this phenomenon be related to a bias-variance trade-off in regression?


% % Yet, it is unclear whether a trade-off between $p=1$ and $2$ also occurs for finite $n,d$ of practically relevant orders. In this Section, we study the performance of interpolating for different values of $p$ in practical scenarios and observe a correspondence with the trend predicted by the theoretical results.
% % \kd{in practical scenarios but not on real world data? rephrase}


% \paragraph{Regression and the bias-variance trade-off}
% \begin{figure}
%     \centering
%     \includegraphics[width=0.5\textwidth]{figures/synthetic_regression_bias_variance.pdf}
%     \caption{Risk and bias-variance trade-off of the minimum $\ell_p$ norm interpolator as a function of $p$ on a synthetic dataset generated as described in Section~\ref{subsec:regsetting}, with $n=100, d=5000$. The risk is plotted for a noiseless training dataset as well as for noise $\sigma=2$. The bias and variance terms are computed on the noisy dataset. All results are averaged over 50 simulations.}
%     \label{fig:synthetic regression}
% \end{figure}
% Figure~\ref{fig:synthetic regression} shows the performance of the min-$\ell_p$ norm interpolator $\what$ from Equation~\eqref{eq:minlpnomrinterpol} on a synthetic dataset with 1-sparse ground truth, as described in Section~\ref{subsec:regsetting}.
% The optimal risk on noiseless data is achieved for the strongest structural bias $p=1$, while $p=2$ yields constant risk. However, in agreement with the theoretical observations from Theorem~\kd{thm:regressionlp}, noise causes a shift in the optimal $p$ which lies inside $(0, 1)$.
% %\red{for this i would like to see an experiment} Importantly, and differently form regularized models, the optimum is therefore attained when the structural bias is balanced to compensate the effects of noise. \\
% %\kd{rewrite:}
% In addition to the risk, Figure~\ref{fig:synthetic regression} shows the estimated bias and variance terms. We can clearly see that the optimal $p$ can also be explained as a trade-off of these two terms.  We further discuss this relation in Section~\ref{sec:trade-off}.

% %While our theorems do not present an explicit connection with the classical notions of bias and variance for the mean squared error, we observe the presence of the noise $\sigma$ in the $\frac{\sigma^{4-2p} d^{2p-2}}{n^p} $ term from bound \eqref{eq:thmregboundhighnoiseupper}. We wonder whether this can be understood as some sort of variance of the final estimator, and leave the study of this connection for future work.

% \paragraph{Classification with $\ell_p$ support vector machines.} 


% % \begin{figure*}[t!]
% %     \centering
% %     \begin{subfigure}[t][width=0.4\textwidth]
% %          \centering
% %          \includegraphics[width=\textwidth]{figures/synthetic_lp_svm_p_vs_risk.pdf}
% %          \caption{Synthetic data. The data are generated with a 1-sparse ground truth $w^{\star}$ and $y=\sign(<x, w^{\star}>)$. Here $n=100$, $d=5000$.}
% %          \label{fig:synthetic classification subplot}
% %      \end{subfigure}
% %      \hfill
% %      \begin{subfigure}[t][width=0.4\textwidth]
% %          \centering
% %          \includegraphics[width=\textwidth]{figures/leukemia_lp_svm_p_vs_risk.pdf}
% %          \caption{Leukemia dataset. The results are averaged over 100 random train-validation splits of the dataset, resulting in $n=65$. The data dimension is $d=7070$.}
% %          \label{fig:leukemia classification subplot}
% %      \end{subfigure}
% %     \caption{Risk for $\ell_p$ support vector machine \eqref{eq:svm prob} on synthetic (a) and real (b) data.}
% %     \label{fig:classification svm}
% % \end{figure*}


% Real world regression tasks are in general considered to be noisy, thus in such scenarios regularized estimators are a natural choice. Oppositely, classification datasets can sometimes be considered noiseless. In such cases, classification with hard-margin support vector machines is a practically relevant case \cite{noble2004support, brown1999support, guyon2002gene, furey2000support, cervantes2020comprehensive} \red{check if these are enough, the last is a survey and we can find many more there}. Figure~\ref{fig:classification svm} shows the performance of the max-$\ell_p$-margin interpolator, or also called \emph{hard-margin $\ell_p$-support vector machine}, on the Leukemia dataset \cite{leukemiapaper}, and a synthetic dataset with 1-sparse ground truth $w^{\star}$ as in Section~\ref{subsec:clasetting} with random label flips given by $\mathbb{P}(\xi=-1)=\sigma, \mathbb{P}(\xi=+1)=1-\sigma$. Again, in the noiseless case the optimal choice of $p=1$ yields the best risk. However, and as expected from the Theorems~\ref{thm:mainl1} and \ref{thm:classificationlp}, for higher levels of noise higher values of $p$ yield the optimal estimator.
% \begin{figure*}[t]
%     \centering
%      \begin{subfigure}[b]{0.45\linewidth}
%          \centering
%   \includegraphics[width=\textwidth]{figures/synthetic_lp_svm_p_vs_risk.pdf}
%          \caption{Synthetic data.}
%          \label{fig:synthetic classification subplot}
%      \end{subfigure}
%           \begin{subfigure}[b]{0.45\linewidth}
%          \centering
%          \includegraphics[width=\textwidth]{figures/leukemia_lp_svm_p_vs_risk.pdf}
%          \caption{Leukemia dataset.}
%          \label{fig:leukemia classification subplot}
%      \end{subfigure}
%          \caption{\red{update this caption when we have confidence intervals for regression as well} Risk for the $\ell_p$ support vector machine \eqref{eq:svm problem} on synthetic (a) and real (b) data. (a) the data is generated with a 1-sparse ground truth $w^{\star}$ and $y=\sign(<x, w^{\star}>) \xi$, with $\mathbb{P}(\xi=-1)=\sigma, \mathbb{P}(\xi=+1)=1-\sigma$. Here $n=100$, $d=5000$. (b)  The results are averaged over 100 random train-test splits of the dataset, resulting in $n=65$. The data dimension is $d=7070$.}
%     \label{fig:classification svm}
% \end{figure*}




% % Figure a shows the risk for lp svm.. \red{describe the setting}

% % Figure bla shows the risk for regression \red{also say here what the setting is}



==> sections/notation.tex <==


% %%%%%%%%%%%%%%%%%%%%



% \section{Notation} \label{sec:notation}
% \red{some of the notation will be moved to the appendix}

% We begin by introducing the notation used throughout the proof. 
% On the finite-dimensional space $\RR^d$, we write $\norm{\cdot}_2$ for the Euclidean norm and $\innerprod{\cdot}{\cdot}$ for the inner product.
% The $\ell_1$ and $\ell_{\infty}$-norms are denoted by $\norm{\cdot}_1$ and $\norm{\cdot}_\infty$, respectively. We denote by $\loneball{\lonebound}$ $l_1$-ball with radius $\lonebound$. $\onevec \in \RR^d$ is the vector with all components equal to $1$.
% $\NNN(\mu, \Sigma)$ is the normal distribution with mean $\mu$ and covariance $\Sigma$, $\Phi(x)$ is
% the cumulative distribution function of the scalar standard normal distribution, $\Phic(x) = 1-\Phi(x)$,
% and $\log$ denotes the natural logarithm. An arbitrary vector $v$ with all nonnegative entries we denote by $v\geq 0$. If $v$ is a vector, then we denote by $v_i$ its $i$-th component.

% The $n$ samples $x_i \in \RR^d$
% form the rows of the data matrix \mbox{$\matX = \left[ x_1 ~...~ x_n
%     \right]^\top$}, with $\matX_{ij} \sim \NNN(0,1)$ for each $i,j$.  The
% measurements $y_i \in \{\pm 1\}$ for $i=1,\dots,n$ are given by $y_i = \sign(\innerprod{x_i}{\wgt})\xi_i$ where $\wgt \in \RR^d$ is the ground truth signal and $\xi_i\in\{\pm 1\}$ is the noise distributed according to $\prob_{\xi}$. We define a diagonal matrix $\matDy \in \RR^{n\times n}$ with $(\matDy)_{i,i} = y_i$. 

% Projection operators to the space spanned by $\wgt$ and orthogonal complement are denoted by $\projpar$ and $\projperp$, respectively. For vector $w\in \RR^d$ we use notation $w=(\wone,\wtwo)$ to denote that $w$ is split into components such that $\wone = \projpar{w}$ and $\wtwo = \projperp{w}$. For the time being we assume that $\wgt$ is 1-sparse vector and without loss of generality assume that $\wgt = \left[ 1\ 0 ~...~ 0\right]^\top$. Furthermore we define $\nu = \norm{\wone}_1$ and $\eta = \norm{\wtwo}_2$.

% For vector $z=(\gausswone ,\gausswtwo)$ we define $z_{(1)} = \max_{i=1,\dots,n} \{ \abs{\gausswone_i}, \abs{\gausswtwo_i} \}$. 

% To easily keep track of the dependency on dimension and
% sample size,
% we reserve the $O(\cdot)$ notation to contain only universal constants, without any hidden dependency
% on $d$, $n$ or $\sigma^2$.





==> sections_proof/2_thm1.tex <==















\section{Proof of Theorem \ref{thm:mainl1}}
\label{apx:proofl1}
Recall the definition of  $f(\nu,\eta) = \EE_{Z_1,Z_2 \sim \NNN(0,1)} \EE_{\xi \sim \prob(\cdot\vert Z_1)} \left( 1- \xi \nu \vert Z_1 \vert - \eta Z_2\right)_+^2 $ and $\nubar := \arg\min f(\nu, 0)$ in Section~\ref{subsec:clasetting}. Further, as in the proof of Theorem~\ref{thm:classificationlp} in Appendix~\ref{apx:claslpproof}, define the quantities ${\fstar = f(\nubar, 0)}$, ${\feestar = \frac{d^2}{d^2 \eta}\vert_{(\nu, \eta) = (\nubar, 0)} f(\nu,\eta)}$ and ${\fnnstar = \frac{d^2}{d^2 \nu}\vert_{(\nu, \eta) = (\nubar, 0)} f(\nu,\eta)}$ which are all non-zero positive constants.  We now show the proof of Theorem~\ref{thm:mainl1} with  
% \kd{stefan, we need ot check this once more}
\begin{equation}
\label{eq:kappanoise}
  \kappanoise = \frac{ 2 \fstar }{\feestar \nubar^2}.
\end{equation}

The proof follows a similar structure as the proof of Theorem~\ref{thm:regressionlpmain},\ref{thm:classificationlp} in Appendix~\ref{apx:regproof},\ref{apx:claslpproof}. In particular, we first apply the CGMT in Proposition~\ref{prop:CGMT_application_classification} (which also holds for $p=1$) and then separately bound $\phidn$ in the localization step  and $\phidp,\phidm$ in the uniform convergence step. 
However, as also noted in \cite{wang2021tight} for the related min $\ell_1$-norm interpolator (basis pursuit), the relaxation $\|H\|_{\infty} \|w\|_1 \geq \langle w, H\rangle$ in the constraint sets defining $\phidn,\phidp$ and $\phidm$ in Proposition ~\ref{prop:CGMT_application_classification} leads to non-tight bounds. Instead, as described in Appendix~\ref{apx:subsec:l1path}, we use a path approach as described in \cite{wang2021tight} to show that $\phidn,\phidp$ and $\phidm$ are also the solution of a simpler $3$-dimensional optimization problem. This allows us to then obtain tight bounds for $\phidn$ in Appendix~\ref{apx:subsec:l1localization} and $\phidp,\phidm$ in Appendix~\ref{apx:subsec:l1uniform}. The proof then follows straight forwardly from Proposition~\ref{prop:CGMT_application_classification} and the fact that $\RiskC(\what) =\norm{\frac{w}{\norm{w}_2} - \wgt}_2^2 = 2 - 2\frac{\langle w, \wgt\rangle}{\norm{w}_2}$.






% By definition of $\gennormbound$ is an upper bound for \eqref{eq:Phi_N}, with high probability the min-$\ell_1$-norm interpolator $\what$ belongs to the set of feasible solutions in \eqref{eq:Phi_+} and \eqref{eq:Phi_-},
% and hence the second step yields high-probability upper and lower bounds on $\frac{\langle \what, \wgtbar\rangle}{\norm{\what}_2} $ and thus also on the prediction error. 
% % = \Risk(\what)$. %, proving Theorem~\ref{thm:main}.






% Essentially, both the proof of Theorem~\ref{thm:mainl1} and \ref{thm:mainlp} rely on an application of the (Convex) Guassian Minimax Theorem \cite{gordon1988milman,thrampoulidis2015regularized}, which allows us to equivalently study optimization problems involving random vectors $H \in \RR^d, G\in \RR^n$ instead of the random matrix $X\in \RR^{d \timex n}$. For this, note that by assumption, $\wgt$ is $s$-sparse. We therefore separate $w$ into two vectors $\wone \in \RR^s$ and $\wtwo \in \RR^{d-s}$ with the first one on containing the support $\wgt$. In particular, we have $\yui \langle \xui, w \rangle = \yui \left(\langle \xsui, \wone \rangle + \langle \xscui, \wtwo \rangle\right)$ with $\xsui$ and $\xscui$ the corresponding subvectors of $\xui$. We write and $\Xs = \{ \xsui \}_{i=1}^n$.
% Because $\xscui$ is independent on $\yui$ and $\xsui$, we can use a standard arguemnt as presented in (cite some works) to apply the (C)GMT, resulting in Proposition~\ref{prop:CGMT_application}. Details for the proof are given in Appendix.... 






% Following the work in \cite{konst} we can recast \eqref{eq:phin}, \eqref{eq:phip}, \eqref{eq:phim} as optimization problems in three scalar variables. Let $b,\alpha$ be scalar variables with $b\geq 0$, $\alpha\in[1,\alpham]$ with $\alpham = d\frac{\norm{\Hgaussian}_{\infty}}{\norm{\Hgaussian}_p^p}$. Then we define parametric path $b\gamma(\alpha)$ with $\RR^d$-valued function $\gamma$ given by:
% \begin{equation}
%     \gamma(\alpha) = \argmin_{\wtwo} \norm{\wtwo}_2^2
%     \subjto \begin{cases}
%                 \innerprod{\wtwo}{\Hgaussian} \geq \norm{\Hgaussian}_{\infty}\\
%                 \wtwo\geq 0\\
%                 \transp{\onevec} \wtwo = \norm{\wtwo}_p^p = \alpha
%             \end{cases}
% \end{equation}
% \begin{restatable}{proposition}{propparam}
% % \begin{proposition} 
% \label{prop:parametrization}
% Optimization problems \eqref{eq:phin}, \eqref{eq:phip}, \eqref{eq:phim} are equivalently given by:
%         \begin{align}
%         \tag{$A_N$}\label{eq:phin}
%             \phidn &= \min_{\nu,b,\alpha} \nu + \alpha b
%             \subjto \frac{1}{n}  b^2\norm{\Hgaussian}_{\infty}^2  \geq  \fnclas(\|\wone\|_2,b\|\gamma(\alpha)\|_2). \\
%         \tag{$A_+$} \label{eq:phip}
%             \phidp &= \max_{\nu,b,\alpha}  \frac{\nu}{\sqrt{\nu^2+b^2\norm{\gamma(\alpha)}_2^2}}
%             \subjto \begin{cases}
%               \frac{1}{n}  b^2\norm{\Hgaussian}_{\infty}^2  \geq  \fnclas(\|\wone\|_2,b\|\gamma(\alpha)\|_2)\\
%                 \nu+b  \leq \loneboundclas
%             \end{cases}\\
%         \tag{$A_-$} \label{eq:phim}
%             \phidm &= \min_{\nu,b,\alpha}  \frac{\nu}{\sqrt{\nu^2+b^2\norm{\gamma(\alpha)}_2^2}}
%             \subjto \begin{cases}
%               \frac{1}{n}  b^2\norm{\Hgaussian}_{\infty}^2  \geq  \fnclas(\|\wone\|_2,b\|\gamma(\alpha)\|_2)\\
%                 \nu+b \leq \loneboundclas
%             \end{cases}
%         \end{align}
% for some scalars $\nu,b>0$ and $\alpha\in[1,\alpham]$.

% \end{restatable}   






































\paragraph{A simplifying modification of the proof.}
Following the same reasoning as in the prove of Theorem~\ref{thm:regressionlp} in Appendix~\ref{apx:regproof}, we instead proof the result
assuming that $\wgt, x_i \in \RR^{d+1}$, which implies that  $H \in \RR^{d}$. This modification does not affect the expression for the bounds in Equation~\eqref{eq:mainboundl1} in Theorem~\ref{thm:mainl1}. 


















































\subsection{Step 1: Reduce the optimization problem via a path approach.}
\label{apx:subsec:l1path}
\label{step_1_thm3_proof}

Following the work in \cite{wang2021tight} we can recast the optimization problems defining $\phidn,\phidp$ and $\phidm$ in Proposition~\ref{prop:CGMT_application_classification} as optimization problems in three scalar variables. Let $b,\alpha$ be scalar variables with $b\geq 0$, $\alpha\in[1,\alpham]$ and $\alpham = d\frac{\norm{\Hgaussian}_{\infty}}{\norm{\Hgaussian}_1}$.  We define the parametric path $\alpha  \mapsto \gamma(\alpha) \in \RR^{d}$ given by:
\begin{equation}
\label{eq:def_gamma_alpha}
    \gamma(\alpha) = \argmin_{\wtwo} \norm{\wtwo}_2^2
    \subjto \begin{cases}
                \innerprod{\wtwo}{\Hgaussian} \geq \norm{\Hgaussian}_{\infty}\\
                \wtwo\geq 0\\
                \transp{\onevec} \wtwo = \norm{\wtwo}_1 = \alpha
            \end{cases}
\end{equation}

Following exactly the same arguments as in Lemma 1 in \cite{wang2021tight} we obtain: 
\begin{proposition}
% \begin{proposition} 
\label{prop:parametrization}
The optimization defining $\phidn,\phidp$ and $\phidm$ in
Proposition~\ref{prop:CGMT_application_classification} are equivalently given by optimization problems \eqref{eq:phin_par}, \eqref{eq:phip_par}, \eqref{eq:phim_par} respectively, defined by:
    \begin{align}
        \tag{$A_N'$}\label{eq:phin_par}
            \phidn &= \min_{\nu,b,\alpha} \vert \nu \vert  + b \alpha
            \subjto \frac{1}{n}  b^2\norm{\Hgaussian}_{\infty}^2  \geq  \fnclas(\nu,b\|\gamma(\alpha)\|_2).
            \\
        \tag{$A_+'$} \label{eq:phip_par}
            \phidp &= \max_{\nu,b,\alpha}  \frac{\nu}{\sqrt{\nu^2+b^2\norm{\gamma(\alpha)}_2^2}}
            \subjto 
            (\nu, b, \alpha) \in \Gamma_0
            \\
        \tag{$A_-'$} \label{eq:phim_par}
            % \phidm &= \min_{\nu,b,\alpha}  \frac{\nu}{\sqrt{\nu^2+b^2\norm{\gamma(\alpha)}_2^2}}
            % \subjto \begin{cases}
            %   \frac{1}{n}  b^2\norm{\Hgaussian}_{\infty}^2  \geq  \fnclas(\wone,b\|\gamma(\alpha)\|_2)\\
            %     \nu+b \leq \loneboundclas
            % \end{cases}
            \phidm &= \min_{\nu,b,\alpha}  \frac{\nu}{\sqrt{\nu^2+b^2\norm{\gamma(\alpha)}_2^2}}
            \subjto
            (\nu, b, \alpha) \in \Gamma_0
    \end{align}
for some scalars $\nu, b>0, \alpha\in[1,\alpham]$ and set $\Gamma_0$ given by:
\begin{align}
    \Gamma_0 = \left\{ (\nu, b, \alpha) \subjto\frac{1}{n}  b^2\norm{\Hgaussian}_{\infty}^2  \geq  \fnclas(\nu,b\|\gamma(\alpha)\|_2) ~~\andtxt~~  \nu + b\alpha \leq \loneboundclas \right\}.
    \label{eq:Omega_0_def}
\end{align}
% \begin{align}
%     \Gamma_0 = \left\{ (\nu,\eta) \subjto\frac{1}{n}  b^2\norm{\Hgaussian}_{\infty}^2  \geq  \fnclas(\nu,b\|\gamma(\alpha)\|_2) ~~\andtxt~~  \nu+b \leq \loneboundclas \right\}.
% \end{align}
% \begin{align}
%     \Gamma_0 = \left\{ (\wone,\wtwo) \subjto \frac{\innerprod{\wtwo}{H}}{n}^2  \geq  \fnclas( \wone, \wtwo ) ~~\andtxt~~  \norm{\wone}_1 + \norm{\wtwo}_1 \leq \loneboundclas \right\}.
% \end{align}
\end{proposition}  
For the reminder of the proof, we can assume without loss of generality that $H_i >0$ and that $H_i > H_j$ for all $i>j$ (see also \cite{wang2021tight}). 
In order to study this reformulated optimization problem, we make use of the following three properties of the path $\gamma(\alpha)$:


\paragraph{Concentration of $\norm{\gamma(\alpha)}_1$ and $\norm{\gamma(\alpha)}_2$.} 
As proven in Section 3.4 in \cite{wang2021tight} the path $ \gamma ( \alpha ) $ is a piecewise linear with breakpoints at $ \alpha_s $ for integers $ s = 2, \dots, d$, with
\begin{equation}
    \alpha_s = \frac{ \left( \norm{\Hvecs}_1-s H_s \right) \norm{H}_{\infty} } {\norm{\Hvecs}_2^2 - \norm{\Hvecs}_1 H_s }
\end{equation}
where $\Hvecs \in \RR^{d}$ denotes vector which is equal to $H \in \RR^{d}$ on first $s$ components and zero elsewhere. Moreover, the following concentration result holds as shown in Proposition 4 in \cite{wang2021tight}.

\begin{proposition}
\label{prop:concentrationl1}
Let $\ts$ be given by $2\Phic(\ts) = s/d$. There exists universal positive constants $c_1,c_2,c_3,c_4>0$ such that for any $s,d$ with $s\geq c_1$ and $c_2 s\leq d\leq \exp(c_3 s^{1/5})$ we have that:
    \begin{align}
        \abs{
            \frac{\norm{\gamma(\alphathr{s})}_1}{\norm{\Hgaussian}_\infty} - \left(\frac{1}{\ts} - \frac{2}{\ts^3}\right)
        }
        &\leq \frac{c_4}{\ts^5}
        \qquad \andtxt \qquad
        \abs{
            \frac{\norm{\gamma(\alphathr{s})}_2^2}{\norm{\Hgaussian}_\infty^2} - \frac{2}{s \ts^2}
        }
        \leq \frac{c_4}{s \ts^4}, \label{eq:concentration}
    \end{align}
with probability at least $1-6\exp\left(-\frac{2s}{\log^5(d/s)}\right)$ over the draws of $H$.
\label{lemma_gamma_conc}
\end{proposition}

\paragraph{Convexity and monotonicity of  $\gamma(\alpha)$. }
According to Lemma 4 in \cite{wang2021tight} the mapping $ \alpha \mapsto \norm{ \gamma(\alpha) }_2^2 $ is convex over $ [ 1, \alpham ]$ and the map $ \alpha \mapsto \frac{ \norm{\gamma(\alpha)}_2^2} {\norm{\gamma(\alpha)}_1^2 }  =\frac{ \norm{\gamma(\alpha)}_2^2} {\alpha^2 }$ is monotonically decreasing.

\paragraph{Inequality constraint at optimal point.} According to Claim 3 in \cite{wang2021tight} the first inequality constraints the definition of $\gamma(\alpha)$ in Equation~\eqref{eq:def_gamma_alpha} is tight for the optimal solution, i.e.,  $\innerprod{\gamma(\alpha)}{H} = \norm{H}_{\infty}$. 


Furthermore we will use the following two characterizations of $t_s$:
\paragraph{Approximation of $t_s$.}
From Remark 2 in \cite{wang2021tight} there exists universal constant $\kappa$ such that, for all $s \leq d/\kappa$ holds that 
\begin{equation}
   t_s^2 = 2 \log(d/s) - \log \log (d/s) -\log(\pi) +\frac{\log\log(d/s)}{2\log(d/s)} + O\left(\frac{1}{\log(d/s)}\right).
\end{equation}

\paragraph{Upper and lower bounds of $\tnstar$.}
Define $\nopt = n\feestar/2$. Following the same argument as in Claim 7 and Claim 9 in \cite{wang2021tight}, we can prove the following lemma:
\begin{lemma}
\label{lemma_uls_ols_exp}
    Let any fixed constant $ 0 < \lambda \leq  \log^{1/4} (c_2) $ where by assumption $d\geq n c_2$ and let $\uls$ be the largest integer such that $\tuls^2 \geq \tnstar^2 + \frac{\lambda}{\sqrt{\tnstar}}$. Then
    \begin{align}
        \uls = \nstar \exp \left( -\frac{ \lambda }{ 2 \sqrt{\tnstar} } \right) \left( 1 + O \left( \frac{1}{\tnstar^2} \right) \right)
        \andtxts
        \left| \tuls^2 - \left( \tnstar^2 + \frac{\lambda}{\sqrt{\tnstar}} \right) \right| \leq O \left( \frac{1}{n} \right)
    \end{align}
    Moreover, let $\ols$ be the smallest integer such that $\tols^2 \leq \tnstar^2 - \frac{\lambda}{\sqrt{\tnstar}}$. Then
    \begin{align}
        \ols = \nstar \exp \left( \frac{ \lambda }{ 2 \sqrt{\tnstar} } \right) \left( 1 + O \left( \frac{1}{\tnstar^2} \right) \right)
        \andtxts
        \left| \tols^2 - \left( \tnstar^2 - \frac{\lambda}{\sqrt{\tnstar}} \right) \right| \leq O \left( \frac{1}{n} \right)
    \end{align}
\end{lemma}
 Furthermore, analogously as in proof of Claim 8 in \cite{wang2021tight} we get:
\begin{align}
    \frac{\tnstar^2}{\tuls^2} 
    =
    \frac{1}{1 + \frac{\lambda}{\tnstar^2\sqrt{\tnstar}} + O \left( \frac{1}{\tnstar^2 \nstar} \right)}
    =
    1 - \frac{\lambda}{\tnstar^2\sqrt{\tnstar}} + O \left( \frac{1}{\tnstar^2 \nstar} \right) + O \left( \frac{\lambda^2}{\tnstar^5} \right)
\end{align}
Similar result holds for $\tols$.



\subsection{Step 2: Localization step - bounding \texorpdfstring{$\phidn$}{phiN}.}
\label{apx:subsec:l1localization}

As in the proof of Theorem~\ref{thm:regressionlpmain},\ref{thm:classificationlp} in Appendix~\ref{apx:regproof},\ref{apx:claslpproof}, we defined $\eta = \norm{\wtwo}_2$ and by using parametric path approach we have that $\eta = b\norm{\gamma(\alpha)}_2$. Hence for the ease of notation we will sometimes only write  $\eta$ with dependence on $b$ and $\alpha$ implicitly assumed. 

We now derive an upper bound on $\phidn$. For this, it is sufficient to find a feasible point satisfying the constraint in the optimisation problem defining $\phidn$. Using the concentration of Lipschitz continuous function (see e.g., \cite{Ledoux1992AHS}), it is straight forward to show that:
\begin{lemma}
\label{lemma_point_conv}
For any $\nu,\eta>0$ holds that:
    \begin{align}
        \prob \left( \abs{ \fnclas \left( \nu, \eta \right) - \EE \left[ \fnclas \left( \nu, \eta \right) \right] }  \geq \epsilon \right) \leq 2 \exp \left( - c \frac{ n \epsilon^2 }{ \nu^2 + \eta^2 } \right)
    \end{align}
where $c>0$ is a positive universal constant. 
\end{lemma} 
To goal is now to use Lemma~\ref{lemma_point_conv} to relax the constraints in the optimization problem defining $\phidn$ to show the following result.

% The goal is now to show that we can find a feasible point $(\nubar, \eta)$ with $\nubar = \argmin f(\nu, 0)$ and $\eta = O \left( \frac{1}{\log(d/n)} \right)$. For this, we can take the Taylor series approximation of $f$ around $(\nuopt,0)$,   $f(\nubar, \eta) \approx \fstar + \frac{\feestar}{2} \eta^2$, which allows us to rewrite the constraint in $\phidn$ to 
% \begin{equation}
%     \frac{1}{n}  b^2\norm{\Hgaussian}_{\infty}^2  \geq  \fstar + \frac{\feestar}{2} \eta^2 + O \left( \frac{1}{\log (d/n)^{3/2}} \right).
% \end{equation}



% Further, following a similar approach as in Proposition~2 in \cite{wang2021tight} by applying the concentration results in Proposition~\ref{prop:concentrationl1}, we can show the following Proposition~\ref{prop:Rbound} which gives an upper bound on $\phidn$.

% a similar approach in the proof of Proposition~2 in \cite{wang2021tight}, where tight bounds for $\phidn$ for min-l1-norm interpolation are derived, we can show the following bound on $\phidn$ given in  Proposition \ref{prop:Rbound}. The proof may be found in Appendix~... 
\begin{proposition}
\label{prop:Rbound}
     Let the data distribution be as described in Section~\ref{subsec:clasetting} and assume that the noise model $\probsigma$ is independent of $n,d$ and $p$.
Let $t_{\nopt}$ be given by $2\Phic(t_{\nopt}) = \nopt/d$ with $\nopt = n\feestar/2$. There exist universal positive constants $c_1,c_2,c_3,c_4,c_5>0$ such that, if $n\geq c_1$ and $c_2 n\leq d\leq \exp(c_3 n^{1/5})$ then
    \begin{align} \label{phidn_bound}
        (\phidn)^2 
        \leq
        \frac{ n \fstar }{ \tnstar^2 } \left( 1 - \frac{ 2 }{ \tnstar^2 } + \frac{c_5}{ \tnstar^3 } \right) =:\loneboundclas^2
    \end{align}
with probability at least $ 1 - 2 \exp \left( -\frac{ c_4 n }{ \tnstar^6 } \right) - 6 \exp \left( -\frac{\nstar}{\log^5(d/\nstar)} \right) $ over the draws of $\Hgaussian$, $\Ggaussian$, $\Xs$ and $\xi$.
\end{proposition}  


\begin{proof}[Proof of Proposition~\ref{prop:Rbound}]

Recall that $\phidn$ is given by:
\begin{align}
    \phidn &= \min_{\nu,b,\alpha} \vert \nu \vert  + b \norm{ \gamma \left( \alpha \right) }_1 
    \subjto \frac{ b^2\norm{\Hgaussian}_{\infty}^2 }{n} \geq \fnclas \left( \nu, b \norm{ \gamma \left( \alpha \right) }_2 \right)
\end{align}

Given that $(\tnu,\tb,\talpha)$ is a feasible point of for the optimization problem defining $\phidn$ in Equation~\eqref{eq:phin_par}, we have that $\phidn \leq  \vert \tnu \vert + \tb \norm{ \gamma( \talpha) }_1$, which gives us an upper bound on $\phidn$. In the following discussion our goal is to find a single feasible point of the constraint set of $\phidn$.

From definition of $\gamma ( \alpha )$ we know that $ \norm{ \gamma ( \alpha ) }_1 = \alpha$ and hence we can equivalently formulate $\phidn$ as an optimization over $\nu$ and $ b_{\alpha} := b \alpha $
\begin{align}
    \phidn &= \min_{ \nu, b_{\alpha} } \nu + b_{\alpha}
    \subjto \frac{ b_{\alpha}^2 \norm{\Hgaussian}_{\infty}^2 }{n \alpha^2} \geq \fnclas \left( \nu, b_{\alpha} \frac{ \norm{ \gamma \left( \alpha \right) }_2}{ \alpha } \right)
\end{align}

 Using Lemma \ref{lemma_point_conv} with $ \epsilon = \fstar \tnstar^{-3} $ and for a feasible point $( \nu, b_{\alpha} \frac{ \norm{ \gamma \left( \alpha \right) }_2}{ \alpha } )$ we have that:
\begin{align} \label{eq:constraint_f_conc}
    \frac{ b_{\alpha}^2 \norm{\Hgaussian}_{\infty}^2 }{n \alpha^2} 
    \geq
    f \left( \nu, b_{\alpha} \frac{ \norm{ \gamma \left( \alpha \right) }_2}{ \alpha } \right) + \frac{\fstar}{\tnstar^{3}}
\end{align}
with probability at least $ 1 - 2 \exp \left( -c \frac{ n }{ \tnstar^6 \left( \nu^2 + b_{\alpha}^2  \norm{ \gamma \left( \alpha \right) }_2^2 / \alpha^2 \right) } \right) $.
% > 1 - 2 \exp \left( - \tc \frac{ n }{ \log^3 \left( \frac{d}{n} \right)  } \right) $.

Let's now choose $ \nu = \nubar $ and show that there exists a pair $ ( b, \alpha )$  such that $ ( \nubar, b, \alpha) $ is feasible for constraint \eqref{eq:constraint_f_conc}. Furthermore, we propose to search for a point with parameter $ ( b, \alpha ) $ such that $ b \norm{ \gamma ( \alpha )}_2 = b_{\alpha} \frac{ \norm{ \gamma \left( \alpha \right) }_2}{ \alpha } $ is near zero. Hence, using Taylor series approximation of the function $ f ( \nubar, \cdot ) : \eta \mapsto f (\nubar, \eta) $ around  the point $(\nuopt,0)$ we can rewrite the constraint \eqref{eq:constraint_f_conc} as:
\begin{align}
     \frac{ b_{\alpha}^2 \norm{\Hgaussian}_{\infty}^2 }{n \alpha^2}   
     \geq
      \fstar + \frac{1}{2}\feestar b_{\alpha}^2 \frac{ \norm{ \gamma \left( \alpha \right) }_2^2}{ \alpha^2 } + O \left( b_{\alpha}^3 \frac{ \norm{ \gamma \left( \alpha \right) }_2^3}{ \alpha^3 } \right) + \frac{\fstar}{\tnstar^{3}}
\end{align}
since $\zeta_{\eta} := \frac{\partial f(\nuopt,\eta)}{\partial \eta}\Big|_{\eta=0} = 0$ and where we recall that by definition $\fstar = f \left( \nubar, 0 \right)$, $\feestar = \frac{\partial^2 f(\nuopt,\eta)}{\partial \eta^2}\Big|_{\eta=0}$ and $\nstar = \frac{1}{2}\feestar n$.

As we mentioned in section \ref{step_1_thm3_proof}, $ \gamma ( \alpha ) $ is a piecewise linear function with breakpoints at $ \alpha_s $ for $ s = 2, \dots, d $. Hence instead of optimizing over $\alpha$ we optimize over $s$. Note that we have only one constraint but two free variables $ ( b, \alpha ) $ and so we can set $ \alpha = \alpha_{\nstar} $ with $ \nstar = \frac{1}{2}\feestar n $. To gain an intuition for why this choice is approximately optimal, one can follow a similar argument as in Remark 1 in \cite{wang2021tight}.  Combining all the previous results we get the constraint:
\begin{align} \label{eq:B_ineq}
     \frac{ b_{\alpha_{\nstar}}^2 \norm{\Hgaussian}_{\infty}^2 }{n \alpha_{\nstar}^2}   
     \geq
      \fstar + \frac{1}{2}\feestar b_{\alpha_{\nstar}}^2 \frac{ \norm{ \gamma \left( \alpha_{\nstar} \right) }_2^2}{ \alpha_{\nstar}^2 } + O \left( b_{\alpha_{\nstar}}^3 \frac{ \norm{ \gamma \left( \alpha_{\nstar} \right) }_2^3}{ \alpha_{\nstar}^3 } \right) + \frac{\fstar}{\tnstar^{3}}
\end{align}

We now claim that
\begin{equation}
    b_{\alpha_{\nstar}}^2 = \frac{ n \alpha_{\nstar}^2 }{ \norm{\Hgaussian}_2^2 } \frac{ \fstar \left( 1 + \frac{1}{\tnstar^{3}} \right) }{ 1 - \frac{1}{2} n \feestar \frac{ \norm{ \gamma \left( \alpha_{\nstar} \right) }_2^2 }{ \norm{H}_{\infty}^2 } - O \left( \frac{1}{\tnstar^3} \right) }
\end{equation}
satisfies inequality \eqref{eq:B_ineq} with probability at least $ 1 - 6 \exp \left( -\frac{2\nstar}{\log^5(d/\nstar)} \right)$. Using Proposition \ref{lemma_gamma_conc} we have that:
\begin{equation}
    1 - \frac{1}{2} n \feestar \frac{ \norm{ \gamma \left( \alpha_{\nstar} \right) }_2^2 }{ \norm{H}_{\infty}^2 } - O \left( \frac{1}{\tnstar^3} \right) > 1 - \frac{1}{2} n \feestar  \frac{2}{\nstar \tnstar^2} - O \left( \frac{1}{\tnstar^3} \right) = 1 - \frac{2}{\tnstar^2} - O \left( \frac{1}{\tnstar^3} \right)  > 0
\end{equation}
holding for $d,n$ sufficiently large. Applying Lemma \ref{lemma_gamma_conc} once again we get:
\begin{equation}
    b_{\alpha_{\nstar}}^2 
    \leq
    \frac{ n \fstar }{ \tnstar^2 } \left( 1 + \frac{1}{\tnstar^3} \right) \left( 1 - \frac{4}{\tnstar^2} + \frac{c}{\tnstar^4} \right) \frac{1}{ 1 - \frac{2}{\tnstar^2} - O \left( \frac{1}{\tnstar^3} \right)}
    \leq
    \frac{ n \fstar }{ \tnstar^2 } \left( 1 - \frac{2}{\tnstar^2} + \frac{c}{\tnstar^3} \right)
\end{equation}

Hence we have that $ O \left( b_{\alpha_{\nstar}}^3 \frac{ \norm{ \gamma \left( \alpha_{\nstar} \right) }_2^3}{ \alpha_{\nstar}^3 } \right) = O \left( \frac{1}{\tnstar^3} \right)$ and this $b_{\alpha_{\nstar}}^2$ indeed satisfies equation \eqref{eq:B_ineq}. Now we define the upper bound on $\phidn$ as:
\begin{align}
\label{eq:lonebound_def}
    \loneboundclas := \sqrt{ \frac{ n \fstar }{ \tnstar^2 } \left( 1 - \frac{2}{\tnstar^2} + \frac{c}{\tnstar^3} \right) }
\end{align}
which holds with probability at least $ 1 - 2 \exp \left( -c \frac{ n }{ \tnstar^6 \left( \nubar^2 + b_{\alpha_{\nstar}}^2  \norm{ \gamma \left( \alpha_{\nstar} \right) }_2^2 / \alpha_{\nstar}^2 \right) } \right) - 6 \exp \left( -\frac{2\nstar}{\log^5(d/\nstar)} \right) $. The proposition is proved after noting that $ \nubar^2 + b_{\alpha_{\nstar}}^2  \norm{ \gamma \left( \alpha_{\nstar} \right) }_2^2 / \alpha_{\nstar}^2 = O(1)$.

\end{proof}

































\subsection{Step 3: Uniform convergence.}
\label{apx:subsec:l1uniform}
The goal of this step is to study the constraint set $\Gamma_0$ from Proposition~\ref{prop:parametrization} with $\loneboundclas \geq \phidn$ from the previous step. In particular, we show the following Proposition ~\ref{prop:BoundOmegal1}. The bounds on $\phidp$ and $\phidm$ then follow straightforwardly as proven after the proposition statement. 

\begin{proposition}
\label{prop:BoundOmegal1}
    Let the data distribution be as described in Section~\ref{subsec:clasetting} and assume that the noise model $\probsigma$ is independent of $n,d$ and $p$.
Under the same conditions on $n,d$ as in Theorem~\ref{thm:mainl1},
there exist universal constants $ c_1, c_2, c_3, c_4 > 0 $ such that, if $ n\geq c_1 $ and $ c_2 n \leq d \leq \exp \left( c_3 n^{1/5} \right) $, then
\begin{align}
    \Gamma_0 
    \subset
    \left\{ (\nu, b, \alpha) \subjto  
    \abs{ \eta^2 - \frac{2\fstar}{\feestar \log(d/\nstar) } } =   O \left( \frac{1}{\log^{5/4}(d/\nstar)} \right) ~~\andtxt~~ 
    \deltanu^2 = \abs{ \nu-\nubar }^2 = O \left( \frac{1}{ \log(d/\nstar)} \right) \right\} =: \tilde{\Gamma}
    % \frac{2 \fstar \lambda}{\fnstar}\frac{1}{\log(d/n)^{5/4}} \left( 1 + O \left( \frac{1}{\log(d/n)^{1/4}} \right) \right) \} %
\end{align}
with probability at least $ 1 - c_4 \exp\left(-\frac{n}{\log^6(d/n)}\right) $ over the draws of $\Hgaussian$, $\Ggaussian$, $\Xs$ and $\xi$ and with $\nstar = n \feestar/2$.
\end{proposition}  
%\subsection{Summary. }
From the Propositions \ref{prop:CGMT_application_classification} and \ref{prop:BoundOmegal1} we get the following bounds on $\phidp$ and $\phidm$:
\begin{align}
    %\max_{\nu,\eta} \frac{ \nu }{ \sqrt{ \nu^2 + \eta^2 } } 
    \phidp
    & \leq \left(1 + \frac{\min_{\eta \in \tilde{\Gamma}} ~\eta^2}{\max_{\nu \in \tilde{\Gamma}}~ \nu^2}  \right)^{-1/2}
    % \frac{1}{ \sqrt{ (1 + \frac{\eta^2 }{ (\nubar + \deltanu)^2}} }
    % \\
    % & = 
    % \left( 1 + \frac {\deltanu}{\nubar} \right) \left( 1 - \frac{1}{2} \left( \frac{2\deltanu}{\nubar} + \frac{\deltanu^2 + \eta^2}{(\nubar)^2} \right) + \frac{3}{8} \left( \frac{2\deltanu}{\nubar}\right)^2 + O \left( \deltanu^3, \deltanu \eta^2, \eta^4 \right) \right)
    % \\
    % & = 1 - \frac{\eta^2}{2(\nubar)^2} + O \left( \frac{1}{ \tnstar^{13/4}} \right) 
    % \leq 
    % %1 - W \left( \frac{1}{\log (d/n) } \right)
    % 1 - \frac{ 2 \fstar }{ \feestar (\nubar)^2 } \frac{1}{\tnstar^2} + \frac{\lambda}{\tnstar^{5/2}} +O \left( \frac{1}{ \tnstar^{13/4}} \right) 
    % \\
    % & = 1 - \frac{ \fstar }{ \feestar (\nubar)^2 } \frac{1}{ \log(d/ \nstar)} + \frac{\lambda}{2\log(d/\nstar)^{5/4}} + O \left( \frac{1}{ \log (d/n)^{13/8}} \right)
    % \\
     \leq 1 - \frac{ \fstar }{ \feestar \nubar^2 } \frac{1}{ \log(d/ \nstar)} \left( 1 -O\left( \frac{1}{\log(d/\nstar)^{1/4}} \right)\right) \\
    & \leq 1 -  \frac{\kappanoise}{2 \log(d/ \nstar)} \left( 1 - O\left(\frac{1}{\log(d/\nstar)^{1/4}}\right) \right) \\
\end{align}
and
\begin{align}
    %\min_{\nu,\eta} \frac{ \nu }{ \sqrt{ \nu^2 + \eta^2 } } 
    \phidm &\geq \left(1 + \frac{\max_{\eta \in \tilde{\Gamma}} ~\eta^2}{\min_{\nu \in \tilde{\Gamma}}~ \nu^2}  \right)^{-1/2}
    % & \geq
    % \frac{ \nubar - \deltanu }{ \sqrt{ ( \nubar - \deltanu )^2 + \eta^2 } }
    % \\
    % & = 
    % \left( 1 - \frac {\deltanu}{\nubar} \right) \left( 1 - \frac{1}{2} \left( -\frac{2\deltanu}{\nubar} + \frac{\deltanu^2 + \eta^2}{(\nubar)^2} \right) + \frac{3}{8} \left( \frac{2\deltanu}{\nubar}\right)^2 + O \left( \deltanu^3, \deltanu \eta^2, \eta^4 \right) \right)
    % \\
    % & = 1 - \frac{\eta^2}{2(\nubar)^2} + O \left( \frac{1}{ \tnstar^{13/4}} \right) 
    % \geq 
    % %1 - W \left( \frac{1}{\log (d/n) } \right)
    % 1 - \frac{ 2 \fstar }{ \feestar (\nubar)^2 } \frac{1}{\tnstar^2} - \frac{ \lambda }{\tnstar^{5/2}} +O \left( \frac{1}{ \tnstar^{13/4}} \right) 
    % \\
    % & = 1 - \frac{ \fstar }{ \feestar (\nubar)^2 } \frac{1}{ \log(d/ \nstar)} - \frac{\lambda}{2\log(d/\nstar)^{5/4}} + O \left( \frac{1}{ \log (d/n)^{13/8}} \right)
    % \\
     \geq 1 - \frac{ \fstar }{ \feestar (\nubar)^2 } \frac{1}{ \log(d/ \nstar)} \left( 1 +O\left( \frac{1}{\log(d/\nstar)^{1/4}}\right) \right)\\
    & \geq 1 -  \frac{ \kappanoise}{2 \log(d/ \nstar)} \left( 1 + O\left(\frac{1}{\log(d/\nstar)^{1/4}}\right) \right)
\end{align}

% \red{edit to match new risk} Using approximation $ \arccos(1-x) \approx \sqrt{2x} + O (x\sqrt{x}) $ we can bound $R(\what)$ as follows:
% \begin{align}
%     %W \left( \frac{1}{\log (d/n)^{1/2} }  \right) 
%     \sqrt{\frac{ 2 \fstar }{ \fnstar (\nubar)^2 }} \frac{1}{\sqrt{\log (d/ \nstar)}} \left( 1 - \frac{\lambda'}{\log(d/\nstar)^{1/4}} \right)
%     \leq
%     R(w) = \frac{1}{\pi} \arccos \left( \frac{\innerprod{w}{\wgt}}{\norm{w}_2} \right) 
%     \leq 
%     \sqrt{\frac{ 2 \fstar }{ \fnstar (\nubar)^2 }} \frac{1}{\sqrt{\log (d/ \nstar)}} \left( 1 + \frac{\lambda'}{\log(d/\nstar)^{1/4}} \right)
% \end{align}
% \begin{align}
%     %\frac{1}{\pi} \arccos \left( \frac{\innerprod{ \what }{ \wgt }}{ \norm{\what}_2 } \right)
%     \abs{ R(\what) - \frac{ \sqrt{2 \fstar} }{ \nubar \pi \sqrt{\feestar} } \frac{1}{\sqrt{\log (d/ \nstar)}} }
%     \leq 
%     \frac{\lambda'}{\log(d/n)^{5/4}}
% \end{align}
% Thus, we can bound the risk $\Risk(\what)$ as
% \begin{align}
%     \abs{ \Risk(\what) - \frac{ 2 \fbar }{ \nubar^2 \feebar } \frac{1}{\log (d/ n)} }
%     \leq 
%     \frac{\lambda'}{\log(d/n)^{5/4}}
% \end{align}
% with probability at least $ 1 - $ over the draws of the data set.




\subsection{Proof of Proposition~\ref{prop:BoundOmegal1}}
The proof of the proposition follows from several steps where in each step we approximate $\fnclas$ using the bounds on $(\nu, \eta)$ from the previous steps to obtain a tighter bound on $(\nu, \eta)$ using the tools developed in \cite{wang2021tight}.  
The probability statement in Proposition~\ref{prop:BoundOmegal1} follows when taking the union bound over all equations which we condition on throughout the proof. 
Furthermore, we note that $\Gamma_0$ is not empty as it clearly the choice $\alpha=\alpha_n$ leads with high probability to a feasible point due to the choice of $M$ in Proposition~\ref{prop:Rbound}. 




\subsubsection{Bound 1: \texorpdfstring{$\nu^2,\eta^2 = O(1)$}{}} \label{sec:l1class_nueta_const_bound}
In order to apply Lemma~\ref{lemma_quadratic_plus_fstar_bound} in the next step,  which gives tight bounds for $\fnclas$, we first need to show that with high probability, $\nu^2,\eta^2 = O(1)$. This is the goal of this first step. More specifically, 
the goal of this first step is to show that there exist universal constants $B_{\nu,1}, B_{\eta,1} > 0$ such that for any element $(\nu, b, \alpha)$ of $\Gamma_0$ we have that $ \nu \leq B_{\nu,1} $ and $ \eta = b \norm{ \gamma(\alpha)}_2 \leq B_{\eta,1}$ with probability high probability over the draws of $\Hgaussian,\Ggaussian$ and $\Xs, \xi$. 

For this first step, we use the fact that in the presence of label noise, $\fnclas$ is lower bounded by a quadratic function as stated in Lemma ~\ref{quadratic_bound_fn}. 
As a result, we can relax the first constraint in Definition \eqref{eq:Omega_0_def} of $\Gamma_0$ to 
\begin{equation}
    \frac{1}{n} b^2\norm{\Hgaussian}_{\infty}^2  \geq  \constnu \nu^2  + \consteta  b^2 \norm{\gamma(\alpha)}_2^2 .
\end{equation} 
 
% \red{say more about the intuition, then we can show:}
This approximation leads to an optimization problem similar to the ones discussed in Lemma 1 in \cite{wang2021tight}. After further relaxations we obtain exactly the same form of the inequality, and hence we can use the arguments from \cite{wang2021tight}. 

% \begin{lemma} \label{lemma_first_reduction}
%     There exist universal constants $B_{\nu,1}, B_{\eta,1} > 0$ such that for any element $(\nu, b, \alpha)$ of $\Gamma_0$ we have that $ \nu \leq B_{\nu,1} $ and $ \eta = b \norm{ \gamma(\alpha)}_2 \leq B_{\eta,1}$ with probability at least $ 1 - $ over the draws of $H$ and the data set.
% \end{lemma}


% According to Lemma \ref{quadratic_bound_fn} we have that for any pair $ ( \nu, \eta ) $ with probability at least $ 1 - \exp \left( - n \kldiv{\frac{\sigma}{2}}{\frac{\sigma}{4}} \right) - \exp \left( -\frac{ n\sigma }{ 128 } \right) $ that $ \fnclas ( \nu, \eta) \geq \constnu \nu^2 + \consteta \eta^2 $ for some positive constants $\constnu$ and $\consteta $. Hence with high probability we can relax first constraint defining $\Gamma_0$ to
% % \begin{align}
% %     \frac{ \innerprod{\wtwo}{H}^2 }{ n } \geq \constnu \nu^2 + \consteta  \eta^2
% % \end{align}
% \begin{align}
%     \frac{1}{n} b^2 \norm{H}_{\infty}^2 \geq \constnu \nu^2 + \consteta b^2 \norm{\gamma(\alpha)}_2^2    
% \end{align}

Let's first consider bounding of $\eta$ and then we use the obtained result to bound $\nu$.
\paragraph{Upper bound on $\eta$.}
For this part of the proof we further relax both constraints from Definition \eqref{eq:Omega_0_def} of $\Gamma_0$ and define the following set:
\begin{align}
    \Gamma_1^{\eta} &= \left\{ (\nu, b, \alpha) \subjto \frac{1}{n} b^2 \norm{H}_{\infty}^2 \geq \consteta  b^2 \norm{\gamma(\alpha)}_2^2 \andtxts b \alpha \leq \loneboundclas  \right\} \\
    &= \left\{ (\nu, b, \alpha) \subjto \frac{1}{n} \norm{H}_{\infty}^2 \geq \consteta  \norm{\gamma(\alpha)}_2^2 \andtxts b \alpha \leq \loneboundclas  \right\} \label{eq:lpstep1set}
\end{align}
% \begin{align}
%     \Gamma_1^{\eta} = \left\{ (\wone,\wtwo) \subjto \frac{ \innerprod{\wtwo}{H}^2 }{ n } \geq \consteta  \eta^2 \andtxts \norm{ \wtwo }_1 \leq \loneboundclas  \right\}
% \end{align}
It is evident from definition that $ \Gamma_0 \subset \Gamma_1^{\eta}$ with high probability. Also note that constraints in the set $\Gamma_1^{\eta}$ do not depend on $\nu$ and hence we will now consider only variables $b$ and $\alpha$ and bound $ \eta $ as:
\begin{align}
    &\eta^2 \leq \left[\max_{b,\alpha} b^2 \norm{\gamma(\alpha)}_2^2 \subjto (b,\alpha) \in \Gamma_1^{\eta} \right]
    =  \left[
    \max_{1\leq \alpha \leq \alpham} \loneboundclas^2 \frac{ \norm { \gamma ( \alpha ) }_2^2 }{ \alpha^2 } 
    \subjto
    %B\gamma \left( \alpha \right) \in \Gamma_1^{\eta}
    \left( \frac{\loneboundclas}{\alpha}, \alpha \right) \in \Gamma_1^{\eta} \right]
    \label{eq:l1proofstep1bound}
\end{align}

Now note that as discussed in Appendix~\ref{apx:subsec:l1path} $\norm{\gamma(\alpha)}_2^2$ is convex. Therefore, the set of feasible $\alpha$ in the Set $\Gamma_1^{\eta}$ is an non-empty interval. Indeed, to see that the interval is non empty, recall that we defined $ \loneboundclas $ in such way that $ (b,\alpha_{\nstar}) \in \Gamma_0 $ with high probability for $b \alpha_{\nstar}\leq \loneboundclas$. As $ \Gamma_0 \subset \Gamma_1^{\eta}$, with high probability there exists some $ b > 0 $ such that $ (b, \alpha_{\nstar} ) \in \Gamma_1^{\eta} $ proving that $\Gamma_1^{\eta} \neq \emptyset$. Furthermore,  since $\frac{ \norm { \gamma ( \alpha ) }_2^2 }{ \alpha^2 }$ is monotonically decreasing, to upper bound Equation~\eqref{eq:l1proofstep1bound} it is sufficient to find $\ulalpha < \alpha_{\nstar}$ such that
\begin{align}
\label{eq:s_condition_one}
    \norm{\gamma(\ulalpha)}_2^2 > \frac{1}{\consteta n} \norm{H}_{\infty}^2. 
\end{align}

It is sufficient to only consider the discretized version of $\alpha$, i.e., $\alpha_s$, for which we have access to tight concentration inequalities from Proposition~\ref{prop:concentrationl1}. We now  claim that $\alpha_{\uls}$ with $\uls =\lambda_{\uls} \frac{ n }{ \log (d/n) }$ satisfies the inequality Equation~\eqref{eq:s_condition_one} for some positive universal constant $ \lambda_{\uls} >0  $. Using the characterization $t_s^2 = 2\log (d/s) + O (\log \log (d/s) ) $ from section \ref{step_1_thm3_proof} we get:
\begin{align}
    \frac{ 2 }{ \uls \tuls^2 } \left( 1 - O \left( \frac{ 1 }{ \tuls^2 } \right) \right)
    & >
    \frac{ 1 }{ n \lambda_{\uls} } \left( 1 - O \left( \frac{\log\log (d/n) }{\log (d/n) } \right) \right) > \frac{1}{\consteta n}
\end{align}
where last inequality holds for $d/n$ sufficiently large and $\lambda_{\uls}$ small enough.

Therefore, from Equation~\eqref{eq:l1proofstep1bound} and the concentration inequality from Proposition \ref{lemma_gamma_conc}, we get:
\begin{align}
    \eta^2 \leq \frac{ n \fstar }{ \tnstar^2 } \frac{2}{\uls}\left( 1 + O \left( \frac{1}{\tuls^2} \right) \right) %\leq \boundeta' \left( 1 + O \left( \frac{1}{ \log (d/n) } \right) \right) 
    =: B_{\eta,1}^2,
\end{align}
with $B_{\eta,1}= \Theta (1)$, as desired. 

\paragraph{Upper bound on $\nu$.} Now we derive an upper bound for $\nu$. Using the result from the previous sub-step, we consider the following set:
\begin{align}
    \Gamma_1^{\nu} = \left\{ (\nu, b, \alpha) 
    \subjto
    \frac{1}{n} b^2 \norm{H}_{\infty}^2 \geq \constnu \nu^2 \andtxts b\alpha \leq \loneboundclas \andtxts b\norm{\gamma(\alpha)}_2 \leq B_{\eta,1} \right\}
    %\frac{ \innerprod{\wtwo}{H}^2 }{ n } \geq \constnu \norm{\wone}_2^2 \andtxts \norm{ \wtwo }_1 \leq \loneboundclas \andtxts \norm{ \wtwo }_2 \leq \boundeta  \right\}
\end{align}
% \begin{align}
%     \Gamma_1^{\nu} = \left\{ (\wone,\wtwo) 
%     \subjto
%     \frac{ \innerprod{\wtwo}{H}^2 }{ n } \geq \constnu \nu^2 \andtxts \norm{ \wtwo }_1 \leq \loneboundclas \andtxts \norm{ \wtwo }_2 \leq \boundeta  \right\}
% \end{align}
Clearly, we have again  $\Gamma_0 \subset \Gamma_1^{\nu}$ with high probability. Hence we can upper bound $\nu$ as follows:
\begin{align} \label{eq:nu_opt_first_reduction}
    \nu^2 &\leq \frac{ 1 }{ n \constnu } \left[\max_{b,\alpha} b^2 \norm{H}_{\infty}^2
    \subjto 
    b^2 \leq \frac{\loneboundclas^2}{\alpha^2}
    \andtxts 
    b^2 \leq \frac{B_{\eta,1}^2}{\norm{ \gamma(\alpha)  }_2^2}\right]
    \\
    &= \frac{ 1 }{ n \constnu }  \norm{H}_{\infty}^2 ~\max_{\alpha}\min\left(\frac{\loneboundclas^2}{\alpha^2}, \frac{B_{\eta,1}^2}{\norm{\gamma(\alpha)}_2^2}\right)
\end{align}
Now recall that $\norm{\gamma(\alpha)}_2$ is convex with global minimum at $\alpha_{d+1/2} = \frac{\norm{H}_1 \norm{H}_{\infty}}{\norm{H}_2^2}$ (see Lemma 4 in \cite{wang2021tight}). Thus, the optimal $\alphaopt$ is obtained for $\alphaopt < \alpha_{d+1/2}$ with 
\begin{equation}
    \frac{\loneboundclas^2}{\alphaopt^2} =  \frac{B_{\eta,1}^2 }{\norm{\gamma(\alphaopt)}_2^2}.
\end{equation}
We now show that we can upper and lower bound by $\alpha_{\uls} <\alphaopt < \alpha_{\ols}$ with high probability with $\uls =  \lambda_{\uls} \frac{ \nstar}{ \log (d/\nstar)} $ and $\ols =  \lambda_{\ols} \frac{ \nstar }{ \log (d/\nstar) }$ and $0<\lambda_{\uls}<1< \lambda_{\ols}$ universal constants. For this, we need to show that with high probability, 
\begin{align}
        \frac{\norm{\gamma(\alphaols)}_2^2}{\alphaols^2} <  \frac{B_{\eta,1}^2 }{\loneboundclas^2} < \frac{\norm{\gamma(\alphauls)}_2^2}{\alphauls^2}.
\end{align}
However,  similarly to bounding $\eta$ in the previous sub-step, we can straight forwardly verify that this statement holds with high probability when using Proposition~\ref{prop:concentrationl1} and the characterization $t_s = 2\log (d/s) + O (\log \log (d/s) ) $ from section \ref{step_1_thm3_proof}. 
Therefore, as a result, we obtain the desired upper bound
\begin{align}%\label{eq:nu_opt_first_reduction}
    \nu^2 &\leq  \frac{ 1 }{ n \constnu }  \norm{H}_{\infty}^2 ~\min\left(\frac{\loneboundclas^2}{\alphauls^2}, \frac{B_{\eta,1}^2}{\norm{\gamma(\alphaols)}_2^2}\right) \leq \frac{ 1 }{ n \constnu }  \norm{H}_{\infty}^2 ~\frac{\loneboundclas^2}{\alphauls^2}
    =: B_{\nu,1},
\end{align}
and in particular, we have again that $B_{\nu,1} = \Theta(1)$, which completes the first step of the proof. 














% \subsubsection{Bound 1: $\nu^2,\eta^2 = O(1)$} \label{sec:l1class_nueta_const_bound}
% The goal of this first step is to show that there exist universal constants $B_{\nu,1}, B_{\eta,1} > 0$ such that for any element $(\nu, b, \alpha)$ of $\Gamma_0$ we have that $ \nu \leq B_{\nu,1} $ and $ \eta = b \norm{ \gamma(\alpha)}_2 \leq B_{\eta,1}$ with probability high probability over the draws of $\Hgaussian,\Ggaussian$ and $\Xs, \xi$. 

% For this first step, we use the fact that in the presence of label noise, $\fnclas$ is lower bounded by a quadratic function as stated in Lemma ~\ref{quadratic_bound_fn}. 
% As a result, we can relax the first constraint in definition \eqref{eq:Omega_0_def} of $\Gamma_0$ to 
% \begin{equation}
%     \frac{1}{n} b^2\norm{\Hgaussian}_{\infty}^2  \geq  \constnu \nu^2  + \consteta  b^2 \norm{\gamma(\alpha)}_2^2 .
% \end{equation} 
 
% % \red{say more about the intuition, then we can show:}
% This approximation leads to an optimization problem similar to the ones discussed in Lemma 1 in \cite{wang2021tight}. After further relaxation we obtain exactly the same form of the inequality, and hence we can use arguments from \cite{wang2021tight}. 

% % \begin{lemma} \label{lemma_first_reduction}
% %     There exist universal constants $B_{\nu,1}, B_{\eta,1} > 0$ such that for any element $(\nu, b, \alpha)$ of $\Gamma_0$ we have that $ \nu \leq B_{\nu,1} $ and $ \eta = b \norm{ \gamma(\alpha)}_2 \leq B_{\eta,1}$ with probability at least $ 1 - $ over the draws of $H$ and the data set.
% % \end{lemma}


% % According to Lemma \ref{quadratic_bound_fn} we have that for any pair $ ( \nu, \eta ) $ with probability at least $ 1 - \exp \left( - n \kldiv{\frac{\sigma}{2}}{\frac{\sigma}{4}} \right) - \exp \left( -\frac{ n\sigma }{ 128 } \right) $ that $ \fnclas ( \nu, \eta) \geq \constnu \nu^2 + \consteta \eta^2 $ for some positive constants $\constnu$ and $\consteta $. Hence with high probability we can relax first constraint defining $\Gamma_0$ to
% % % \begin{align}
% % %     \frac{ \innerprod{\wtwo}{H}^2 }{ n } \geq \constnu \nu^2 + \consteta  \eta^2
% % % \end{align}
% % \begin{align}
% %     \frac{1}{n} b^2 \norm{H}_{\infty}^2 \geq \constnu \nu^2 + \consteta b^2 \norm{\gamma(\alpha)}_2^2    
% % \end{align}

% Let's first consider bounding of $\eta$ and then we use obtained result to bound $\nu$.
% \paragraph{Upper bound on $\eta$.}
% For this part of the proof we further relax both constraints from definition \eqref{eq:Omega_0_def} of $\Gamma_0$ and define the following set:
% \begin{align}
%     \Gamma_1^{\eta} = \left\{ (\nu, b, \alpha) \subjto \frac{1}{n} b^2 \norm{H}_{\infty}^2 \geq \consteta  b^2 \norm{\gamma(\alpha)}_2^2 \andtxts b \alpha \leq \loneboundclas  \right\}
% \end{align}
% % \begin{align}
% %     \Gamma_1^{\eta} = \left\{ (\wone,\wtwo) \subjto \frac{ \innerprod{\wtwo}{H}^2 }{ n } \geq \consteta  \eta^2 \andtxts \norm{ \wtwo }_1 \leq \loneboundclas  \right\}
% % \end{align}


% It is evident from definition that $ \Gamma_0 \subset \Gamma_1^{\eta}$ with high probability. Also note that constraints in the set $\Gamma_1^{\eta}$ do not depend on $\nu$ and hence we will now consider only variables $b$ and $\alpha$. Now we bound $ \eta $ as:
% \begin{align}
%     \eta^2 \leq \max_{b,\alpha} b^2 \norm{\gamma(\alpha)}_2^2 \subjto (b,\alpha) \in \Gamma_1^{\eta}
% \end{align}

% We proceed following the path arguments established in \cite{wang2021tight}. First we show that set $\Gamma_1^{\eta}$ is not empty. Let's choose $ \alpha = \alpha_{\nstar}$ with $\nstar = n\feestar/2$. Recall that we defined $ \loneboundclas $ in such way that $ (b,\alpha_{\nstar}) \in \Gamma_0 $ with high probability for $b \alpha_{\nstar}\leq \loneboundclas$. As $ \Gamma_0 \subset \Gamma_1^{\eta}$, with high probability there exists some $ b > 0 $ such that $ (b, \alpha_{\nstar} ) \in \Gamma_1^{\eta} $ proving that $\Gamma_1^{\eta} \neq \emptyset$.

% Recall from definition \eqref{eq:def_gamma_alpha} that $\norm{\gamma(\alpha)}_1 = \alpha$. Then using the same arguments as in Lemma 1 in \cite{wang2021tight}, we set $ b = \frac{\loneboundclas}{\alpha} $ and obtain:
% \begin{align}
% \label{eq:step_one_eta_bound_alpha}
%     \eta^2 
%     \leq
%     \max_{1\leq \alpha \leq \alpham} \loneboundclas^2 \frac{ \norm { \gamma ( \alpha ) }_2^2 }{ \norm { \gamma ( \alpha ) }_1^2 } 
%     \subjto
%     %B\gamma \left( \alpha \right) \in \Gamma_1^{\eta}
%     \left( \frac{\loneboundclas}{\alpha}, \alpha \right) \in \Gamma_1^{\eta}
% \end{align}

% As mentioned in section \ref{step_1_thm3_proof} the map $ \alpha \mapsto \frac{ \norm{ \gamma ( \alpha ) }_2^2 }{ \norm{ \gamma ( \alpha ) }_1^2 } $ is monotonically decreasing and the mapping $ \alpha \mapsto \consteta b^2 \norm{\gamma(\alpha)}_2^2 $ is convex. The interval of $\alpha \in [1,\alpham]$ for which constraint in equation \eqref{eq:step_one_eta_bound_alpha} holds is an interval since it is as a sublevel set of a convex function. Therefore if we find value of $\alpha_{\uls}$ such that $\alphauls \leq \alpha_{\nstar}$ and $ ( \frac{M}{\alphauls}, \alphauls ) \not \in \Gamma_1^{\eta}$, then we have:
% \begin{align} \label{eq:eta_bound_first_reduction}
%     \eta^2 \leq  \loneboundclas^2 \frac{ \norm { \gamma ( \alphauls ) }_2^2 }{ \norm { \gamma ( \alphauls ) }_1^2 }
% \end{align}

% % In order to saturate constraint $ \norm{ \wtwo }_1 \leq \loneboundclas $ let $ b = \frac{\loneboundclas}{\alphauls}$. 
% In order to have $ ( \frac{M}{\alphauls}, \alphauls ) \not \in \Gamma_1^{\eta}$ we will chose $\uls$ as the smallest integer for which first constraint in definition of $\Gamma_1^{\eta}$ is not satisfied, i.e. choose  $\uls$ satisfying
% % \begin{align}
% %     \loneboundclas^2 \frac{ \innerprod{ \gamma ( \alphauls )}{H}^2 }{ n \alphauls^2 } < \consteta \loneboundclas^2 \frac{ \norm{ \gamma ( \alphauls ) }_2^2 }{ \alphauls^2 }
% % \end{align}
% \begin{align}
% \label{eq:s_condition_one}
%     \frac{1}{n} \frac{\loneboundclas^2}{\alphauls^2} \norm{H}_{\infty}^2 
%     <
%     \consteta \frac{\loneboundclas^2}{\alphauls^2} \norm{ \gamma ( \alphauls ) }_2^2 
% \end{align}
% % Rewriting this inequality gives:
% % \begin{align} \label{eq:s_condition_one}
% %   \frac{ \norm{ \gamma ( \alphauls ) }_2^2 }{ \norm{H}_{\infty}^2 } > \frac{ 1 }{ \consteta n } 
% % \end{align}
% After rewriting and using concentration result from Proposition \ref{lemma_gamma_conc} we obtain the following condition on $\uls$:
% \begin{align}
%     \frac{ 2 }{ \uls \tuls^2 } \left( 1 - O \left( \frac{ 1 }{ \tuls^2 } \right) \right) > \frac{ 1 }{ \consteta n }
% \end{align}

%  We claim that $\uls =\lambda_{\uls} \frac{ n }{ \log (d/n) }$ satisfies this inequality for some positive universal constant $ \lambda_{\uls} >0  $. Using characterization $t_s = 2\log (d/s) + O (\log \log (d/s) ) $ from section \ref{step_1_thm3_proof} we get:
% \begin{align}
%     \frac{ 2 }{ \uls \tuls^2 } \left( 1 - O \left( \frac{ 1 }{ \tuls^2 } \right) \right) 
%     & >
%     % \frac{ 2\log (d/n)  }{ n \lambda_{\uls} } \frac{ 1 }{ 2\log (d/\uls) + O \left(\log \log (d/\uls) \right) } \left( 1 - O \left( \frac{1}{\log (d/n)} \right) \right)
%     % \\
%     % & = 
%     \frac{ 1 }{ n \lambda_{\uls} } \left( 1 - O \left( \frac{\log\log (d/n) }{\log (d/n) } \right) \right) > \frac{1}{\consteta n}
% \end{align}
% where last inequality holds for $d/n$ sufficiently large and $\lambda_{\uls}$ small enough.

% Now from equation \eqref{eq:eta_bound_first_reduction} and concentration Proposition \ref{lemma_gamma_conc}, for some positive constant $B_{\eta,1}$ we get:
% \begin{align}
%     \eta^2 \leq \frac{ n \fstar }{ \tnstar^2 } \frac{2}{\uls}\left( 1 + O \left( \frac{1}{\tuls^2} \right) \right) %\leq \boundeta' \left( 1 + O \left( \frac{1}{ \log (d/n) } \right) \right) 
%     =: B_{\eta,1}^2
% \end{align}
% since for the chosen $\uls$ the term on the right hand side of inequality is of the order $O (1)$.


% \paragraph{Upper bound on $\nu$.} Now we derive an upper bound for $\nu$. We consider the following set:
% \begin{align}
%     \Gamma_1^{\nu} = \left\{ (\nu, b, \alpha) 
%     \subjto
%     \frac{1}{n} \innerprod{b\gamma(\alpha)}{H}^2 \geq \constnu \nu^2 \andtxts b\alpha \leq \loneboundclas \andtxts b\norm{\gamma(\alpha)}_2 \leq B_{\eta,1} \right\}
%     %\frac{ \innerprod{\wtwo}{H}^2 }{ n } \geq \constnu \norm{\wone}_2^2 \andtxts \norm{ \wtwo }_1 \leq \loneboundclas \andtxts \norm{ \wtwo }_2 \leq \boundeta  \right\}
% \end{align}
% % \begin{align}
% %     \Gamma_1^{\nu} = \left\{ (\wone,\wtwo) 
% %     \subjto
% %     \frac{ \innerprod{\wtwo}{H}^2 }{ n } \geq \constnu \nu^2 \andtxts \norm{ \wtwo }_1 \leq \loneboundclas \andtxts \norm{ \wtwo }_2 \leq \boundeta  \right\}
% % \end{align}
% and note that we have again with high probability that $\Gamma_0 \subset \Gamma_1^{\nu}$. 

% As we noted in Section \ref{step_1_thm3_proof}, from Claim 3 in \cite{wang2021tight} follows that $\innerprod{\gamma(\alpha)}{H} = \norm{H}_{\infty}$ and we obtain that $\Gamma_0 \subset \Gamma_1^{\nu}$ with high probability. Hence we can upper bound $\nu$ as follows:
% \begin{align} \label{eq:nu_opt_first_reduction}
%     \nu^2 \leq \frac{ 1 }{ n \constnu } \max_{b,\alpha} b^2 \innerprod{\frac{\gamma(\alpha)}{\alpha}}{H}^2
%     \subjto 
%     b \leq \loneboundclas 
%     \andtxts 
%     b\norm{ \frac{\gamma(\alpha) }{\alpha} }_2 \leq B_{\eta,1}
% \end{align}

% First note that choosing $b=M$ maximizes the objective if the second constraint is satisfied as well. Now we show how this optimization problem can be rewritten in a more suitable form for solving via parametrized path approach. Similarly as in \cite{wang2021tight} we define function $\olw : \left[ \frac{1}{d}, 1 \right] \to \RR^{d-1}$ as
% \begin{align}
%     \olw(\beta) = \argmax_{\wtwo} \innerprod{\wtwo}{\Hgaussian}
%     \subjto \begin{cases}
%                 \norm{\wtwo}_2^2 \leq \beta \\
%                 \wtwo\geq 0\\
%                 \norm{\wtwo}_1 = 1
%             \end{cases}
% \end{align}
% From Claim 2 in \cite{wang2021tight} we know that for any $\beta \in \left[ \frac{1}{d}, 1 \right] $ there exists $ \alpha \in \left[ 1, \alpham \right] $ such that $ \olw (\beta) = \frac{ \gamma(\alpha) }{ \alpha }$. Following similar argument as in Lemma 4 in \cite{wang2021tight} we have that $ \olw (\beta) $ is monotonically increasing function in $\beta$. Hence we can rewrite \eqref{eq:nu_opt_first_reduction} as:
% \begin{align} 
% \label{eq:first_iteration_nu_gamma_beta}
%     \nu^2 \leq \frac{ \loneboundclas^2 }{ n \constnu } \max_{\beta} \innerprod{ \olw(\beta) }{ H }^2
%     \subjto 
%     \norm{ \olw(\beta) }_2 \leq \frac{ B_{\eta,1} }{ \loneboundclas }
% \end{align}

% Similarly as in the first part of this proof, we first show that there exists $\beta_{\nstar}$ which satisfies constraints, and then find smallest $\beta_{\ols}$ which does not satisfy constraints in \eqref{eq:first_iteration_nu_gamma_beta} and such that $ \beta_{\ols} \geq \beta_{\nstar}$. From monotonicity of $ \olw (\beta)$ follows that $ \olw (\beta_{\ols}) \geq \olw (\beta_{\nstar})$. Since the constraints in \eqref{eq:first_iteration_nu_gamma_beta} are convex in $\olw(\beta)$, the expression is maximized for $\beta = \beta_{\ols}$.

% Since $\alpha = \alpha_{\nstar}$ satisfies constraints in \eqref{eq:nu_opt_first_reduction} by definition of $M$, we define $\beta_{\nstar}$ such that $\gamma(\beta_{\nstar}) = \frac{\gamma(\alpha_{\nstar})}{\alpha_{\nstar}}$ and hence $\beta_{\nstar}$ satisfies constraints in \eqref{eq:first_iteration_nu_gamma_beta}. Furthermore, if we find $\alpha_{\uls}$ such that $\alpha_{\uls} \leq \alpha_{\nstar}$ and
% \begin{align}\label{s_condition_nu_first_reduction}
%     \frac{ \norm{ \gamma ( \alphauls ) }_2 }{ \alphauls } 
%     >
%     \frac{ B_{\eta,1} }{ \loneboundclas }
% \end{align}
% we automatically obtain $\beta_{\uls}$ such that $\gamma(\beta_{\uls}) = \frac{\gamma(\alpha_{\uls})}{\alpha_{\uls}}$ which does not satisfy constraint in \eqref{eq:first_iteration_nu_gamma_beta}. 
% Now from \eqref{s_condition_nu_first_reduction} and using concentration result from Proposition \ref{lemma_gamma_conc} and expression \eqref{phidn_bound} we obtain condition:
% \begin{align}
%     \frac{2}{\uls} \left( 1 - O \left( \frac{1}{\tuls^2} \right) \right)
%     >
%     \frac{B_{\eta,1}^2 \tnstar^2}{ n \fstar } \left( 1 + O \left( \frac{1}{\tnstar^2} \right) \right)
% \end{align}
% Once again we claim that this equality is satisfied for $ \uls = \lambda_{\uls} \frac{ n }{ \log (d/n) } $ for some positive constant $\lambda_{\uls}$. The proof follows use the same reasoning as in the previous part of the proof.

% Hence we can bound $\nu$ from expression \eqref{eq:nu_opt_first_reduction} as follows:
% \begin{align}\label{nu_bound_first_reduction}
%     \nu^2 
%     \leq
%     \frac{ \loneboundclas^2 }{ n \constnu } \frac{ \innerprod{ \gamma (\alphauls) }{ H }^2 }{ \alphauls^2 }
%     =
%     \frac{ \loneboundclas^2 }{ n \constnu } \frac{ \norm{H}_{\infty}^2 }{ \alphauls^2 }
% \end{align}
% with the equality holding for $\gamma(\alpha)$ as discussed in Section \ref{step_1_thm3_proof}. Using concentration results from Proposition \ref{lemma_gamma_conc} we conclude that there exists a positive constant $B_{\nu,1}$ such that:
% \begin{align}
%     \nu^2 \leq \frac{ \fstar \tuls^2 }{ \constnu \tnstar^2 } \left( 1 + O \left( \frac{1}{\tuls^2} \right) \right)
%     % \leq c'_{\nu} \left( 1 + O \left( \frac{ \log \log (d/n) }{\log (d/n) } \right) \right) \leq
%     =: B_{\nu,1}^2
% \end{align}
% since the term on the right hand side is of the order $O(1)$ for chosen $\uls$. This concludes the proof of the lemma.













































\subsubsection{Bound 2: \texorpdfstring{$\nu^2,\eta^2 = O\left(\frac{1}{\log(d/n)}\right)$}{} =}

Conditioning on the event where the bounds form the first step hold for $\nu,\eta$, the goal of this second step is to show that for any element $(\nu, b, \alpha)$ of $\Gamma_0$ we have that $\deltanu^2 = O \left( \frac{1}{ \log \left( d/n \right) }  \right) $ and $ \eta^2 = b^2 \norm{\gamma(\alpha)}_2^2 = O \left( \frac{1}{ \log \left( d/n \right) } \right)$ with high probability over the draws of $\Hgaussian, \Ggaussian, \Xs$ and $\xi$. 

% Define $\deltanu = \nu - \nubar$. Using the fact from the previous section that $\nu \leq B_{\nu,1}, \eta \leq B_{\eta,1}$, we obtain a tighter uniform lower bound for $\fnclas$ from Lemma~\ref{lemma_quadratic_4lus_fstar_bound}. 

% Plugging in this expression, we can again show:
% \begin{lemma} \label{lemma_second_reduction}
%     For any element $(\nu, b, \alpha)$ of $\Gamma_0$ we have that $\deltanu^2 = O \left( \frac{1}{ \log \left( d/n \right) }  \right) $ and $ \eta^2 = b^2 \norm{\gamma(\alpha)}_2^2 = O \left( \frac{1}{ \log \left( d/n \right) } \right)$ with probability at least $ 1 - $ over the draws of $H$ and the data set.
% \end{lemma}

Define $\deltanu = \nu - \nubar$. 
From the previous step, we know that with high probability, $ \nu \leq B_{\nu,1} $ and $ \eta \leq B_{\eta,1} $. Hence we can use Lemma~\ref{lemma_quadratic_plus_fstar_bound} to obtain a tight lower bound for $\fnclas$, which is based on uniform convergence of $\fnclas$ to its expectation in Proposition \ref{prop:unifConv}, and relax the constraint from definition of the set $\Gamma_0$ as follows:
\begin{align}
\label{eq:second_iteration_relaxed_constraint_f}
    \frac{1}{n} b^2 \norm{H}_{\infty}^2 \geq \fnclas (\nu, b\norm{\gamma(\alpha)}_2) \geq f ( \nu, b\norm{\gamma(\alpha)}_2 ) - \constconc \geq  \fstar  + \tconstnu \deltanu^2 + \tconsteta b^2\norm{\gamma(\alpha)}_2^2 - \constconc, 
\end{align}
where we choose $\constconc =  O \left( \frac{1}{\tnstar^3} \right)$. 
Again we first consider the bounding of $\eta$ and then use the obtained result to bound $\deltanu = \nu -\nubar$.

\paragraph{Upper bound on $\eta$.} 
We similarily to the previous step, we consider the set:
\begin{align}
    \Gamma_2^{\eta} = \left\{ (\nu, b, \alpha) 
    \subjto 
    \frac{ 1 }{ n } b^2 \norm{H}_{\infty}^2 \geq \fstar +  \tconsteta b^2 \norm{\gamma(\alpha)}_2^2 - \constconc
    \andtxts
    b\alpha \leq \loneboundclas
    \right\} 
\end{align}
% \begin{align}
%     \Gamma_2^{\eta} = \left\{ (\wone,\wtwo) \subjto \frac{ \innerprod{\wtwo}{H}^2 }{ n } \geq \fstar - \constconc +  \tconsteta \norm{\wtwo}_2^2  \andtxts \norm{ \wtwo }_1 \leq \loneboundclas  \right\}
% \end{align}
% \begin{align}
%     \Gamma_2^{\eta} = \left\{ (\wone,\wtwo) \subjto \frac{ \innerprod{\wtwo}{H}^2 }{ n } \geq \fstar - \constconc +  \tconsteta \eta^2  \andtxts \norm{ \wtwo }_1 \leq \loneboundclas  \right\}
% \end{align}
Again, we have that with high probability $\Gamma_0 \subset \Gamma_2^{\eta} $.
Clearly, to upper bound $\eta = b \norm{\gamma(\alpha)}_2$, we can again set $ b = \frac{\loneboundclas}{\alpha} $ and thus obtain:
\begin{align}
    \eta^2 &\leq \max_{b,\alpha} b^2 \norm{\gamma(\alpha)}_2^2 \subjto \left(\frac{M}{\alpha},\alpha \right) \in \Gamma_2^{\eta}  \\
    &= \max_{\alpha} \frac{M^2}{\alpha^2} \norm{\gamma(\alpha)}_2^2 \subjto \frac{ 1 }{ n } \frac{M^2}{\alpha^2} \norm{H}_{\infty}^2 \geq \fstar +  \tconsteta \frac{M^2}{\alpha^2} \norm{\gamma(\alpha)}_2^2 - \constconc.
    \label{eq:l1proofstep2eta}
\end{align}
Multiplying the constraint on both sides with $\alpha^2$ and using the fact that $\norm{\gamma(\alpha)}_2^2$ is convex shows that the set of feasible $\alpha$ is again a (non-empty) interval. 
Thus, by the monotonicity of $ \frac{\norm{\gamma(\alpha)}_2^2}{\alpha^2} $ the problem reduces again to finding $\alphauls < \alpha_{\nstar}$ (where we use again that $\alpha_{\nstar}$ satisfies the constraints with high probability) such that $\alphauls$ violates the constraint in Equation~\eqref{eq:l1proofstep2eta}, i.e., 
\begin{align}
\label{eq:l1proofstep2eta2}
    \left( \fstar - \constconc \right) \frac{ n \alphauls^2 }{  \loneboundclas^2 \norm{H}_{\infty}^2 } + \tconsteta n \frac{ \norm{ \gamma(\alphauls) }_2^2 }{ \norm{H}_{\infty}^2 } > 1
\end{align}
% In order for inequality above to be satisfied we need:
% \begin{align}
%     \left( 1 - \frac{ \constconc }{ \fstar } \right) 
%     \frac{\tnstar^2}{t_s^2}
%     \left( 1 - \frac{4}{t_s^2} + O \left( \frac{1}{\tnstar^3} \right) \right) 
%     \left( 1 + \frac{2}{\tnstar^2} + O \left( \frac{1}{\tnstar^3} \right) \right) 
%     + \frac{2 n \tconsteta}{s t_s^2} \left( 1 + O \left( \frac{1}{t_s^2} \right) \right) 
%     > 1
% \end{align}
We now show that we can choose $ \uls = \lambda_{\uls} \nstar$ with universal constant $\lambda_{\uls} \in (0,1)$. Indeed, applying  Propositions \ref{prop:concentrationl1} and using the characterization $t_s =   2 \log(d/s) - \log \log (d/s) -\log(\pi) +\frac{\log\log(d/s)}{2\log(d/s)} + O\left(\frac{1}{\log(d/s)}\right)$ from section \ref{step_1_thm3_proof} we get:
\begin{align}
 \left( \fstar - \constconc \right) \frac{ n \alphauls^2 }{  \loneboundclas^2 \norm{H}_{\infty}^2} &= 1 + \frac{\log(\lambda_{\uls})-2}{\tnstar^2} + O\left(\frac{1}{\tnstar^3}\right) \\
 \mathrm{and}~~\tconsteta n \frac{ \norm{ \gamma(\alphauls) }_2^2 }{ \norm{H}_{\infty}^2 } &= 
\frac{1}{\tnstar^2}\frac{4\tconsteta}{\lambda_{\uls}}  +  O \left( \frac{1}{ \tnstar^3} \right)
\end{align}
where $O(.)$ has hidden dependencies on $\lambda_{\uls}$. Hence, it is straight forward to see that for any $d \geq c n$ with universal constant $c>0$ (and thus $\tnstar$ lower bounded), we can find a universal constant $\lambda_{\uls}$ such that Equation~\eqref{eq:l1proofstep2eta2} holds. 


% \begin{align}
%     \frac{\tnstar^2}{t_s^2}
%     \left( 1 + \frac{ \frac{4\tconsteta}{\lambda\feestar}  - 4}{t_s^2} + \frac{2}{\tnstar^2} + O \left( \frac{1}{\tnstar^3}, \frac{1}{t_s^3} \right) \right)
%     > 1
% \end{align}
% Fix $\ulambda > 0$. Choose $\uls = \lambda_{\uls} \nstar$ such that $\uls < n$ is the largest integer for which $ \tuls^2 \geq \tnstar^2 + \ulambda $. Then we have condition:
% \begin{align}
%     \left( 1 - \frac{\ulambda}{\tuls^2} \right) \left( 1 + \frac{ \frac{4\tconsteta}{\lambda_{\uls}\feestar}  - 4}{\tuls^2} + \frac{2}{\tnstar^2} + O \left( \frac{1}{t_n^3} \right) \right)
%     > 1
% \end{align}
% For $\ulambda$ large enough inequality holds (Note: second brackets grow as $\lambda_{\uls}^{-1}$ and the first decays like $\log ( \lambda_{\uls} )$ - TO CHECK).


% \red{okay I messed this up - sorry. Can you make the following section a bit clearer? In particular, the connection to tn and s is not clear, cite the result form our paper. . So here we need to say that essentially we obtain the same problem as studied in my paper.}

% Fix $\olambda > 0$. Now we choose $\ols = c_{\ols} \nstar$ such that $ \ols > n $ is the smallest integer for which $ t_{\ols}^2 \leq \tnstar^2 - \olambda $. Then we have:
% \begin{align}
%     \left( 1 + \frac{\olambda}{\tols^2} \right) \left( 1 + \frac{ \frac{4\tconsteta}{c_{\ols}\feestar}  - 4}{\tols^2} + \frac{2}{\tnstar^2} + O \left( \frac{1}{t_n^3} \right) \right)
%     > 1
% \end{align}
% We claim that there exists $\olambda$ large enough such that this inequality holds (e.g. $\ulambda > 4$).

Hence, we can upper bound $\eta^2$ in Equation \eqref{eq:l1proofstep2eta} as follows:
\begin{align} \label{eq:eta_bound_second_reduction}
    \eta^2 
    \leq
    \loneboundclas^2 \frac{ \norm { \gamma ( \alphauls ) }_2^2 }{ \alpha_{\uls}^2 } 
    \leq
    \frac{ n \fstar }{ \tnstar^2 } \frac{2}{\uls}\left( 1 + O \left( \frac{1}{\tuls^2} \right) \right) 
    \leq
    % \frac{c_{\eta,2}}{\log (d/n) } \left( 1 + O \left( \frac{1}{ \log (d/n) } \right) \right) 
    \frac{2\fstar}{\feestar \lambda_{\uls} \log (d/n) } \left( 1 + O \left( \frac{1}{ \log (d/n) } \right) \right) 
    =:
    \frac{B_{\eta,2}^2}{\tnstar^2}
\end{align}
with $B_{\eta,2}^2 = \Theta(1)$.
% and similarly we get:
% \begin{align}
%     \eta^2 
%     \geq
%     B^2 \frac{ \norm { \gamma ( \alphaols ) }_2^2 }{ \norm { \gamma ( \alphaols ) }_1^2 } 
%     \geq
%     \left( \frac{ \overline{B}_{\eta,2} }{ \sqrt{\log (d/n)} } \right)^2
% \end{align}

















\paragraph{Upper bound on $\deltanu$.}
We now again bound $\nu$ using the previous upper bound on $\eta^2 = O(\log^{-1}(d/n))$. More specifically, we bound $\deltanu$ with $\nu = \nubar +\deltanu$ and thus obtain both an upper and lower bound for $\nu$. 
 First, we again define
\begin{align}
    \Gamma_2^{\nu} = \left\{ (\nu, b, \alpha) 
    \subjto
    \frac{1}{n}b^2\norm{H}_{\infty}^2 \geq \fstar - \constconc + \tconstnu \deltanu^2
    \andtxts
    b\alpha \leq \loneboundclas 
    \andtxts
    b\norm{ \gamma(\alpha) }_2 \leq \frac{B_{\eta,2}}{\tnstar}  \right\}
\end{align}
as in the previous step. 

Clearly, we have again  $\Gamma_0 \subset \Gamma_2^{\nu}$ with high probability. Hence we can upper bound $\deltanu$ by:
\begin{align} %\label{eq:nu_opt_first_reduction}
    \nu^2 &\leq \frac{1}{\tconstnu}\left(\frac{ 1 }{ n } \norm{H}_{\infty}^2 \max_{\alpha}\min\left(\frac{\loneboundclas^2}{\alpha^2}, \frac{B_{\eta,2}^2}{\tnstar^2 \norm{\gamma(\alpha)}_2^2}\right) - \fstar + \constconc \right)
\end{align}
In particular, we obtain again an upper bound for $\deltanu$ (as for $\nu$ in the previous step) when bounding finding $\alpha_{\uls} < \alphaopt < \alpha_{\ols}$ where $\alphaopt \leq \alpha_{d+1/2}$ is the $\alpha$ such that the two terms in the $\min$ match. However, we can verify from a similar argument as for the upper bound for $\eta^2$ in the previous sub-step that we can choose $ \uls = \lambda_{\uls} \nstar$ with universal constant $\lambda_{\uls} \in (0,1)$ and $\ols =\lambda_{\ols} \nstar$ with universal constant $\lambda_{\ols} >1$. Hence, we obtain the upper bound

\begin{align}
    \deltanu^2 
    &\leq
    \frac{\norm{H}_{\infty}^2}{ n \tconstnu }  \frac{ \loneboundclas^2}{\alphauls^2}
    \leq 
    \frac{ \fstar t_{\uls}^2}{\tnstar^2 \tconstnu } \left( 1 + \frac{2}{\tnstar^2}  \right)
    - \frac{\fstar}{\tconstnu} + O \left( \frac{1}{\tnstar^3} \right)\\
    & = \frac{\fstar(2 -2\log(\lambda_{\uls})) }{\tconstnu 2\log(d/n)}\left( 1 + O \left( \frac{1}{\sqrt{\log(d/n)}} \right) \right)
    =: 
    \frac{B_{\deltanu,2}^2}{\tnstar^2} 
\end{align}
which concludes the proof.








\subsubsection{Bound 3: Proof of the proposition. }
We already know that $\nu$ concentrates around $\nubar$. However, in order to get a tight expression for the risk and also a valid lower bound, we need to get tighter bounds for $\eta^2$ conditioning on the bounds on $\eta^2,\deltanu^2$ from the previous step,  leading to Proposition~\ref{prop:BoundOmegal1}.


% In this part of the proof we use Taylor series approximation of function $f$ up to quadratic terms as shown in equation \eqref{eq:f_taylor_approx}. Using similar arguments as in previous two bounding steps, we obtain Proposition \ref{prop:BoundOmegal1}.
% \begin{lemma}
%     There exist universal constant $B_{\nu,3} > 0, B_{\eta,3} > 0$ such that for any element $(\wone,\wtwo)$ of $\Gamma_0$ we have that $\deltanu^2 \leq \frac{B_{\nu,3}^2}{ \left( \log \left( d/n \right) \right)^{3/2} }$ and $ \eta^2 \leq \frac{B_{\eta,3}^2}{ \log \left( d/n \right) }$ with probability at least $ 1 - $ over the draws of $..$.
% \end{lemma}
% \begin{proof}
% Conditioning on the event where the bounds for $\nu,\eta$ from the previous second step hold, we now derive the tight bounds
In this part of the proof we use Taylor series approximation of the function $f$ where we use the result form the last step to bound the  higher order terms involving $\eta$. Similarly as in equation \eqref{eq:second_iteration_relaxed_constraint_f}, we obtain form Proposition~\ref{prop:unifConv} and the second order Taylor series approximation of $f$ around the point $(\nubar, 0)$ that with high probability,
\begin{align}
    \label{eq:f_taylor_approx}
    \frac{1}{n} b^2 \norm{H}_{\infty}^2 
    \geq 
    % f ( \nu, \eta ) =
    \fstar + \frac{1}{2}\feestar b^2 \norm{\gamma(\alpha)}_2^2 + \frac{1}{2}\fnnstar \deltanu^2 - \constconc - \OOOc
    % \underbrace{O \left( \frac{1}{ \log (d/n)^{3/2} } \right)}_{\OOOc}
\end{align}
with $\OOO_f = O(\deltanu^3 + \eta^3) =  O \left( \frac{1}{\tnstar^3} \right)$ and $\OOOc = O \left( \frac{1}{\tnstar^3} \right)$. 
% \end{proof}

\paragraph{Upper and lower bound on $\eta$.}
We proceed in the same manner as in the previous two steps. We relax the constraint in definition of $\Gamma_0$ and define the following set:
\begin{align}
    \Gamma_3^{\eta} = \left\{ (\nu, b, \alpha) 
    \subjto 
    \frac{ 1 }{ n } b^2 \norm{H}_{\infty}^2 \geq \fstar +  \frac{1}{2}\feestar  b^2 \norm{\gamma(\alpha)}_2^2  -\constconc - \OOOc
    \andtxts
    b\alpha \leq \loneboundclas
    \right\}
\end{align}
Clearly, we have again with high probability that $\Gamma_0 \subset \Gamma_3^{\eta}$. The only difference between $\Gamma_3^{\eta}$ and $\Gamma_2^{\eta}$ lies in the constant $\tconsteta$ which is replaced by the tighter constant $\feestar/2$. However, this makes a big difference, as this allows us to choose $\uls < \nstar <\ols$ much tighter. Similar to Equation~\eqref{eq:l1proofstep2eta2} we again require that $s=\uls,\ols$ satisfies
\begin{align}
\label{eq:l1thirdeta}
    \left( \fstar - \constconc - \OOOc \right) \frac{ \alpha_s^2 }{ \norm{H}_{\infty}^2 } \frac{ n }{ \loneboundclas^2 } 
    +
    \frac{1}{2} \feestar n \frac{ \norm{ \gamma (\alpha_s) }_2^2 }{ \norm{H}_{\infty}^2 } 
    > 1.
\end{align}
However, this expression allows us to choose $\uls$ and $\ols$ as in Lemma~\ref{lemma_uls_ols_exp}. We only show it for $\uls$ as the same argument holds for $\ols$. Applying Proposition~\ref{prop:concentrationl1}, the LHS from Equation~\eqref{eq:l1thirdeta} can be bounded by

% \begin{align} (this is the last version of this equation)
%     \left( \fstar -\constconc - \OOOc \right) \frac{ \alphauls^2 }{ \norm{H}_{\infty}^2 } \frac{ n }{ \loneboundclas^2 } 
%     \geq 
%     1 - \frac{2}{\tnstar^2} - \frac{\lambda}{\tnstar^{5/2}} + O \left( \frac{1}{\tnstar^3} \right) + O \left( \frac{1}{\tnstar^5} \right) + O \left( \frac{1}{\tnstar^2 \nstar} \right)
% \end{align}
% 
% \begin{align}
%     \left( \fstar -\constconc - \OOOc \right) \frac{ \alphauls^2 }{ \norm{H}_{\infty}^2 } \frac{ n }{ \loneboundclas^2 } \geq &
%     \fstar \left( 1 + O \left( \frac{1}{\tnstar^3} \right) \right) \frac{1}{\tuls^2}\left( 1 - \frac{4}{\tuls^2} + O \left( \frac{1}{\tuls^4} \right) \right)\frac{n \tnstar^2}{n\fstar} \left( 1 + \frac{2}{\tnstar^2} + O \left( \frac{1}{\tnstar^3} \right) \right)
%     \\
%     \geq &
%     \left( 1 - \frac{\lambda}{\tnstar^2\sqrt{\tnstar}} + O \left( \frac{1}{\tnstar^2 \nstar} \right) + O \left( \frac{\lambda^2}{\tnstar^5} \right) \right) \left( 1 - \frac{2}{\tnstar^2} + O \left( \frac{1}{\tnstar^3} \right) \right)
% \end{align}
% 
% \begin{align} (this is the last version of this equation)
%     \frac{1}{2} \feestar n \frac{ \norm{ \gamma (\alphauls) }_2^2 }{ \norm{H}_{\infty}^2 } 
%     \geq 
%     \frac{2}{\tnstar^2} + \frac{\lambda}{(\tnstar)^{5/2}} + \frac{\lambda^2}{2\tnstar^3} + O \left( \frac{1}{\tnstar^{7/2}} \right) 
% \end{align}
% 
% \begin{align}
%     \frac{1}{2} \feestar n \frac{ \norm{ \gamma (\alphauls) }_2^2 }{ \norm{H}_{\infty}^2 } 
%     \geq &
%     \nstar \frac{2}{\uls \tuls^2} \left( 1 + O \left( \frac{1}{\tuls^2} \right) \right)\\
%     \geq &
%     \frac{2}{\tnstar^2} \exp \left( \frac{\lambda}{2\sqrt{\tnstar}} \right)  \left( 1 + O \left( \frac{1}{\tnstar^2} \right) \right) \\
%     \geq &
%     \frac{2}{\tnstar^2} \left( 1 + \frac{\lambda}{2\sqrt{\tnstar}} + \frac{\lambda^2}{4\tnstar} + O \left( \frac{\lambda^3}{\tnstar\sqrt{\tnstar}} \right) \right) \left( 1 + O \left( \frac{1}{\tnstar^2} \right) \right) 
% \end{align}
% 
% Hence we have:
\begin{align}
    \left( \fstar - \constconc - \OOOc \right) \frac{ \alphauls^2 }{ \norm{H}_{\infty}^2 } \frac{ n }{ \loneboundclas^2 } 
    &= \frac{\tnstar^2}{t_{\uls}^2}\left(1 -\frac{4}{t_{\uls}^2}+\frac{2}{\tnstar^2} + O\left(\frac{1}{\tnstar^3}\right)\right)  = 1- \frac{\lambda}{\tnstar^{5/2}} -\frac{2}{\tnstar^2} + O\left(\frac{1}{\tnstar^3}\right) + O\left(\frac{1}{\tnstar^2 \nstar}\right)
    \\
    ~~\mathrm{and}\:\: \frac{1}{2} \feestar n \frac{ \norm{ \gamma (\alphauls) }_2^2 }{ \norm{H}_{\infty}^2 } &= 
    \frac{2}{\tnstar^2} + \frac{\lambda}{\tnstar^{5/2}} + \frac{\lambda^2}{2\tnstar^3} + O \left( \frac{1}{\tnstar^3} \right) + O \left( \frac{1}{\tnstar^2 \nstar} \right)
\end{align}
with $O(.)$ having hidden dependencies on $\lambda$. In particular, as a result, we see that we can choose $\lambda$ such that Equation~\eqref{eq:l1thirdeta} hold for any $d >c n$ with universal constant $c>0$. 
Hence we can bound $\eta^2$ as follows:
\begin{align} \label{eq:eta_bound_third_reduction}
    \eta^2 
    \leq
    \loneboundclas^2 \frac{ \norm { \gamma ( \alphauls ) }_2^2 }{ \norm { \gamma ( \alphauls ) }_1^2 } 
    & \leq
    \frac{ n \fstar }{ \tnstar^2 } \frac{2}{\uls}\left( 1 + O\left( \frac{1}{\tnstar^2} \right) \right)
    \leq
    % \frac{4\fstar}{\feestar} \frac{1}{\tnstar^2}  \exp \left( \frac{\lambda}{2\sqrt{\tnstar}} \right) \left( 1 + O\left( \frac{1}{\tnstar^2} \right) \right) \\
    % & \leq
    \frac{4\fstar}{\feestar} \frac{1}{\tnstar^2} \left( 1 + \frac{\lambda}{2\sqrt{\tnstar}} + O \left( \frac{1}{\tnstar} \right) \right) =: B_{\eta,3}^2
\end{align}
Furthermore, we also obtain a lower bound for $\eta^2$. Similar as in Lemma~5/6 \cite{wang2021tight}, we can lower bound (using again the monotonicity of $\frac{\norm{\gamma(\alpha)}_2}{\alpha}$ and the fact that any feasible $\alpha \leq \alphaols$)
\begin{align}
    \eta^2 &\geq \left[\min_b b^2 \norm{\gamma(\alpha_{\ols})}_2^2 \subjto b^2   
    \geq \frac{\fstar   -\constconc - \OOOc}{\frac{  \norm{H}_{\infty}^2}{ n } -\frac{1}{2}\feestar  \norm{\gamma(\alpha_{\ols})}_2^2} \right] =\frac{\fstar  -\constconc - \OOOc}{\frac{  \norm{H}_{\infty}^2}{ n } -\frac{1}{2}\feestar  \norm{\gamma(\alpha_{\ols})}_2^2} \norm{\gamma(\alpha_{\ols})}_2^2 \\
    &\geq  \frac{4\fstar}{\feestar} \frac{1}{\tnstar^2} \left( 1 - \frac{\lambda}{2\sqrt{\tnstar}} + O \left( \frac{1}{\tnstar} \right) \right) 
\end{align}
Hence we can conclude the proof. 



% \paragraph{Upper bound on $\deltanu$.}
% Now let
% % \begin{align}
% %     \Gamma_3^{\nu} = \left\{ (\nu, b, \alpha) 
% %     \subjto
% %     \frac{1}{n}\innerprod{b\gamma(\alpha)}{H}^2 \geq \fstar + \frac{1}{2}\feestar \eta^2 + \frac{1}{2}\fnstar \deltanu^2 - O \left( \frac{1}{\tnstar^3} \right)
% %     \andtxts 
% %     b\alpha \leq \loneboundclas 
% %     \andtxts
% %     b\norm{ \gamma(\alpha) }_2 \leq \frac{B_{\eta,3}}{\log (d/n) }  \right\}
% % \end{align}
% \begin{equation}
%     \Gamma_3^{\nu} = \Bigg\{ (\nu, b, \alpha) 
%     \subjto \begin{cases}
%                 \frac{1}{n}\innerprod{b\gamma(\alpha)}{H}^2 \geq \fstar - \constconc - \OOOc + \frac{1}{2}\feestar b\norm{\gamma(\alpha)}_2^2 + \frac{1}{2}\fnstar \deltanu^2
%                 \\
%                 b\alpha \leq \loneboundclas
%                 \\
%                 b\norm{ \gamma(\alpha) }_2 \leq B_{\eta,3}
%             \end{cases}
%              \Bigg\}
% \end{equation}
% % \begin{align}
% %     \Gamma_3^{\nu} = \left\{ (\wone,\wtwo) 
% %     \subjto
% %     \frac{ \innerprod{\wtwo}{H}^2 }{ n } \geq \fstar - \constconc - \OOOc + \frac{1}{2}\feestar \eta^2 + \frac{1}{2}\fnstar \deltanu^2
% %     \andtxts 
% %     \norm{ \wtwo }_1 \leq \loneboundclas 
% %     \andtxts
% %     \norm{ \wtwo }_2 \leq B_{\eta,3}  \right\}
% % \end{align}

% % \begin{align}
% % \label{s_condition_nu_third_reduction}
% %     \frac{ \norm{ \gamma ( \alphauls ) }_2 }{ \alphauls } > \frac{B_{\eta,3}}{\loneboundclas}
% % \end{align}
% Analogously to equation \eqref{s_condition_nu_first_reduction} we derive new condition for $\uls$ with new bound $B_{\eta,3}$. Using concentration result from Proposition \ref{lemma_gamma_conc} and expression \eqref{phidn_bound} we get the condition:
% % \begin{align}
% %     \frac{2}{\uls} \left( 1 + O\left( \frac{1}{\tuls^2} \right) \right) 
% %     >
% %     \frac{4\fstar}{\feestar} \frac{1}{\tnstar^2} \left( 1 + \frac{\lambda}{2\sqrt{\tnstar}} + O \left( \frac{1}{\tnstar} \right) \right) \frac{\tnstar^2}{ n \fstar } \left( 1 + \frac{2}{\tnstar^2} + O \left( \frac{1}{\tnstar^3} \right) \right)
% % \end{align}
% % then
% \begin{align}
%     \frac{2}{\uls} \left( 1 + O \left( \frac{1}{\tuls^2} \right) \right) > \frac{4}{\feestar} \frac{1}{n} \left( 1 + \frac{\lambda}{2\sqrt{\tnstar}} + O \left( \frac{1}{\tnstar} \right) \right)
% \end{align}
% Hence let $\uls = \nstar \exp \left( -\frac{\lambda}{2\sqrt{\tnstar}} \right)$. %\frac{n\feestar}{2} \left( 1 - \frac{\lambda}{\sqrt{\tnstar}} + O \left( \frac{1}{\tnstar} \right) \right)$.  
% \begin{align}
%     \deltanu^2 
%     \leq
%     \frac{ 2\loneboundclas^2 }{ n \fnstar } \frac{ \norm{H}_{\infty}^2 }{ \alphauls^2 } - \frac{2}{\fnstar} \left( \fstar - \constconc - \OOOc \right) - \frac{\feestar}{\fnstar} \frac{ \norm{ \gamma(\alphaols) }_2^2 }{ \alphaols^2 } \loneboundclas^2
%     \leq
%     \frac{4 \fstar \lambda}{\fnstar \tnstar^{5/2}} \left( 1 + O \left( \frac{1}{\sqrt{\tnstar}} \right) \right) =: B_{\deltanu,3}^2
% \end{align}
% \begin{align}
%     \deltanu^2 
%     &\leq
%     \frac{ 2\loneboundclas^2 }{ n \fnstar } \frac{ \norm{H}_{\infty}^2 }{ \alphauls^2 } - \frac{2\fstar}{\fnstar} \left( 1 - \constconc - \OOOc \right) - \frac{\feestar}{\fnstar} \frac{ \norm{ \gamma(\alphaols) }_2^2 }{ \alphaols^2 } \loneboundclas^2\\
%     &\leq 
%     \frac{2}{n\fnstar} \frac{n\fstar}{\tnstar^2} \left(1-\frac{2}{\tnstar^2}+O \left( \frac{1}{\tnstar^3} \right) \right) \tuls^2 \left( 1 + \frac{4}{\tuls^2} + O \left( \frac{1}{\tuls^4} \right) \right)
%     - \frac{2\fstar}{\fnstar} \left( 1 + O \left( \frac{1}{\tnstar^3} \right) \right)
%     \\
%      & - \frac{\feestar}{\fnstar} \frac{2}{\nstar} \exp \left( -\frac{\lambda}{2\sqrt{\tnstar}} \right) \left( 1 + O \left( \frac{1}{\tnstar^2} \right) \right) \frac{n\fstar}{\tnstar^2}  \left( 1 - \frac{2}{\tnstar^2} + O \left( \frac{1}{\tnstar^3} \right) \right)
%      \\
%      &\leq \frac{2\fstar}{\fnstar} \left( 1 + \frac{2}{\tnstar^2} + \frac{\lambda}{\tnstar^{5/2}} + O \left( \frac{1}{\tnstar^3} \right) \right) 
%      - \frac{2\fstar}{\fnstar} \left( 1 + O \left( \frac{1}{\tnstar^3} \right) \right)
%      -\frac{2\fstar}{\fnstar}\left( \frac{2}{\tnstar^2} - \frac{\lambda}{\tnstar^{5/2}} + O \left( \frac{1}{\tnstar^3} \right) \right)
%      \\
%      & \leq \frac{4 \fstar \lambda}{\fnstar}\frac{1}{\tnstar^{5/2}} \left( 1 + O \left( \frac{1}{\sqrt{\tnstar}} \right) \right) =: B_{\deltanu,3}^2
% \end{align}





% \begin{align}
%     f ( \nu, \eta ) = \fstar + \frac{1}{2}\feestar \eta^2 + \frac{1}{2}\fnstar \deltanu^2 + O \left( \frac{1}{ \log (d/n)^{3/2} } \right)
% \end{align}


% \begin{lemma}
%     There exist universal constant $B_{\nu,3} > 0, B_{\eta,3} > 0$ such that for any element $(\wone,\wtwo)$ of $\Gamma_0$ we have that $\deltanu^2 \leq \frac{B_{\nu,3}^2}{ \left( \log \left( d/n \right) \right)^{3/2} }$ and $ \eta^2 \leq \frac{B_{\eta,3}^2}{ \log \left( d/n \right) }$ with probability at least $ 1 - $ over the draws of $..$.
% \end{lemma}







% \subsection{Proof of Proposition~\ref{prop:Rbound}}


% Recall that $\phidn$ is given by:
% \begin{align}
%     \phidn &= \min_{\nu,b,\alpha} \nu + b \norm{ \gamma \left( \alpha \right) }_1 
%     \subjto \frac{ b^2\norm{\Hgaussian}_{\infty}^2 }{n} \geq \fnclas \left( \nu, b \norm{ \gamma \left( \alpha \right) }_2 \right)
% \end{align}

% Given that $(\tnu,\tb,\talpha)$ is a feasible point of $\phidn$ we have that $\phidn \leq  \tnu + \tb \norm{ \gamma( \talpha) }_1$, which gives us an upper bound on $\phidn$. In the following discussion our goal is to find a single feasible point of the constraint set of $\phidn$.

% From definition of $\gamma ( \alpha )$ we know that $ \norm{ \gamma ( \alpha ) }_1 = \alpha$ and hence we can equivalently formulate $\phidn$ as an optimization over $\nu$ and $ b_{\alpha} := b \alpha $
% \begin{align}
%     \phidn &= \min_{ \nu, b_{\alpha} } \nu + b_{\alpha}
%     \subjto \frac{ b_{\alpha}^2 \norm{\Hgaussian}_{\infty}^2 }{n \alpha^2} \geq \fnclas \left( \nu, b_{\alpha} \frac{ \norm{ \gamma \left( \alpha \right) }_2}{ \alpha } \right)
% \end{align}

% Define $\fstar = f \left( \nubar, 0 \right)$, $\feestar = \frac{\partial^2 f(\nuopt,\eta)}{\partial \eta^2}\Big|_{\eta=0}$ and $\nstar = \frac{1}{2}\feestar n$. Now using lemma \ref{lemma_point_conv} with $ t = \fstar \tnstar^{-3} $ and for a feasible point $( \nu, b_{\alpha} \frac{ \norm{ \gamma \left( \alpha \right) }_2}{ \alpha } )$ we have that:
% \begin{align} \label{eq:constraint_f_conc}
%     \frac{ b_{\alpha}^2 \norm{\Hgaussian}_{\infty}^2 }{n \alpha^2} 
%     \geq
%     f \left( \nu, b_{\alpha} \frac{ \norm{ \gamma \left( \alpha \right) }_2}{ \alpha } \right) + \frac{\fstar}{\tnstar^{3}}
% \end{align}
% with probability at least $ 1 - 2 \exp \left( -c \frac{ n }{ \tnstar^6 \left( \nu^2 + b_{\alpha}^2  \norm{ \gamma \left( \alpha \right) }_2^2 / \alpha^2 \right) } \right) $.
% % > 1 - 2 \exp \left( - \tc \frac{ n }{ \log^3 \left( \frac{d}{n} \right)  } \right) $.

% Let's now choose $ \nu = \nubar $ and show that there exists a pair $ ( b, \alpha )$  such that $ ( \nubar, b, \alpha) $ is feasible for constraint \eqref{eq:constraint_f_conc}. Furthermore, we propose to search for a point with parameter $ ( b, \alpha ) $ such that $ b \norm{ \gamma ( \alpha )}_2 = b_{\alpha} \frac{ \norm{ \gamma \left( \alpha \right) }_2}{ \alpha } $ is near zero. Hence, using Taylor series approximation of function $ f ( \nubar, \cdot ) : \eta \mapsto f (\nubar, \eta) $ around point $(\nuopt,0)$ we can rewrite constraint \eqref{eq:constraint_f_conc} as:
% \begin{align}
%      \frac{ b_{\alpha}^2 \norm{\Hgaussian}_{\infty}^2 }{n \alpha^2}   
%      \geq
%       \fstar + \frac{1}{2}\feestar b_{\alpha}^2 \frac{ \norm{ \gamma \left( \alpha \right) }_2^2}{ \alpha^2 } + O \left( b_{\alpha}^3 \frac{ \norm{ \gamma \left( \alpha \right) }_2^3}{ \alpha^3 } \right) + \frac{\fstar}{\tnstar^{3}}
% \end{align}
% since $\feta = \frac{\partial f(\nuopt,\eta)}{\partial \eta}\Big|_{\eta=0} = 0$.

% Now from \cite{wang2021tight} we know that $ \gamma ( \alpha ) $ is a piecewise linear function with breakpoints at $ \alpha_s $ for $ s = 2, \dots, d $. Hence instead of optimizing over $\alpha$ we optimize over $s$. Note that we have only one constraint but two free variables $ ( b, \alpha ) $ and so we can set $ \alpha = \alpha_{\nstar} $ with $ \nstar = \frac{1}{2}\feestar n $. We explain this choice of $s$ in the remark after the proof. Combining all these results we get constraint:
% \begin{align} \label{eq:B_ineq}
%      \frac{ b_{\alpha_{\nstar}}^2 \norm{\Hgaussian}_{\infty}^2 }{n \alpha_{\nstar}^2}   
%      \geq
%       \fstar + \frac{1}{2}\feestar b_{\alpha_{\nstar}}^2 \frac{ \norm{ \gamma \left( \alpha_{\nstar} \right) }_2^2}{ \alpha_{\nstar}^2 } + O \left( b_{\alpha_{\nstar}}^3 \frac{ \norm{ \gamma \left( \alpha_{\nstar} \right) }_2^3}{ \alpha_{\nstar}^3 } \right) + \frac{\fstar}{\tnstar^{3}}
% \end{align}

% Now we claim that
% \begin{equation}
%     b_{\alpha_{\nstar}}^2 = \frac{ n \alpha_{\nstar}^2 }{ \norm{\Hgaussian}_2^2 } \frac{ \fstar \left( 1 + \frac{1}{\tnstar^{3}} \right) }{ 1 - \frac{1}{2} n \feestar \frac{ \norm{ \gamma \left( \alpha_{\nstar} \right) }_2^2 }{ \norm{H}_{\infty}^2 } - O \left( \frac{1}{\tnstar^3} \right) }
% \end{equation}
% satisfies inequality \eqref{eq:B_ineq} with probability at least $ 1 - 6 \exp \left( -\frac{\nstar}{\log^5(d/\nstar)} \right)$. Using lemma \ref{lemma_gamma_conc} we have that:
% \begin{equation}
%     1 - \frac{1}{2} n \feestar \frac{ \norm{ \gamma \left( \alpha_{\nstar} \right) }_2^2 }{ \norm{H}_{\infty}^2 } - O \left( \frac{1}{\tnstar^3} \right) > 1 - \frac{1}{2} n \feestar  \frac{2}{\nstar \tnstar^2} - O \left( \frac{1}{\tnstar^3} \right) = 1 - \frac{2}{\tnstar^2} - O \left( \frac{1}{\tnstar^3} \right)  > 0
% \end{equation}
% holding for $d,n$ sufficiently large. Applying lemma \ref{lemma_gamma_conc} once again we get:
% \begin{equation}
%     b_{\alpha_{\nstar}}^2 
%     \leq
%     \frac{ n \fstar }{ \tnstar^2 } \left( 1 + \frac{1}{\tnstar^3} \right) \left( 1 - \frac{4}{\tnstar^2} + \frac{c}{\tnstar^4} \right) \frac{1}{ 1 - \frac{2}{\tnstar^2} - O \left( \frac{1}{\tnstar^3} \right)}
%     \leq
%     \frac{ n \fstar }{ \tnstar^2 } \left( 1 - \frac{2}{\tnstar^2} + \frac{c}{\tnstar^3} \right)
% \end{equation}

% Hence we have that $ O \left( b_{\alpha_{\nstar}}^3 \frac{ \norm{ \gamma \left( \alpha_{\nstar} \right) }_2^3}{ \alpha_{\nstar}^3 } \right) = O \left( \frac{1}{\tnstar^3} \right)$ and this $b_{\alpha_{\nstar}}^2$ indeed satisfies equation \ref{eq:B_ineq}. Now we define the upper bound on $\phidn$ as:
% \begin{align}
%     \loneboundclas := \sqrt{ \frac{ n \fstar }{ \tnstar^2 } \left( 1 - \frac{2}{\tnstar^2} + \frac{c}{\tnstar^3} \right) }
% \end{align}
% which holds with probability at least $ 1 - 2 \exp \left( -c \frac{ n }{ \tnstar^6 \left( (\nubar)^2 + b_{\alpha_{\nstar}}^2  \norm{ \gamma \left( \alpha_{\nstar} \right) }_2^2 / \alpha_{\nstar}^2 \right) } \right) - 6 \exp \left( -\frac{\nstar}{\log^5(d/\nstar)} \right) $. The proposition is proved after noting that $ (\nubar)^2 + b_{\alpha_{\nstar}}^2  \norm{ \gamma \left( \alpha_{\nstar} \right) }_2^2 / \alpha_{\nstar}^2 = O(1)$.

% \subsection{Proof of Lemma~\ref{lemma_first_reduction}}
% According to lemma \ref{quadratic_bound_fn} we have that for any pair $ ( \nu, \eta ) $ with probability at least $ 1 - \exp \left( - n \kldiv{\frac{\sigma}{2}}{\frac{\sigma}{4}} \right) - \exp \left( -\frac{ n\sigma }{ 128 } \right) $ that $ \fnclas ( \nu, \eta) \geq \constnu \nu^2 + \consteta \eta^2 $ for some positive constants $\constnu$ and $\consteta $. Hence with high probability we can relax first constraint defining $\Gamma_0$ to
% \begin{align}
%     \frac{ \innerprod{\wtwo}{H}^2 }{ n } \geq \constnu \nu^2 + \consteta  \eta^2
% \end{align}

% \paragraph{Bounding $\eta$.}
% We can furthermore relax both constraints to define the following set:
% \begin{align}
%     \Gamma_1^{\eta} = \left\{ (\wone,\wtwo) \subjto \frac{ \innerprod{\wtwo}{H}^2 }{ n } \geq \consteta  \eta^2 \andtxts \norm{ \wtwo }_1 \leq \loneboundclas  \right\}
% \end{align}
% It is evident from definition that $ \Gamma_0 \subset \Gamma_1^{\eta}$ with high probability. Also note that constraints in the set $\Gamma_1^{\eta}$ depend only on $\wtwo$ and hence we will now consider only this variable. Now we bound $ \eta = \norm{ \wtwo }_2 $ as:
% \begin{align}
%     \eta^2 \leq \max_{\wtwo} \norm { \wtwo }_2 \subjto \wtwo \in \Gamma_1^{\eta}
% \end{align}

% We proceed following the path arguments established in \cite{wang2021tight}. We parametrize variable $\wtwo$ as $ \wtwo = b \norm { \gamma ( \alpha ) } $. 

% First we show that set $\Gamma_1^{\eta}$ is not empty. Let's choose $ \alpha = \alpha_{\nstar}$ with $\nstar = n\feestar/2$. Since we defined $ \loneboundclas $ in such way that $ \alpha_{\nstar} \in \Gamma_0 $ with high probability and we have $ \Gamma_0 \subset \Gamma_1^{\eta}$, this implies that with high probability there exists some $ b > 0 $ such that $ b \gamma ( \alpha ) \in \Gamma_1^{\eta} $.

% Using the same argument as in lemma 1 in \cite{wang2021tight} for $\phidp$ we can write:
% \begin{align}
%     \eta^2 \leq \max_{1\leq \alpha \leq \alpham} B^2 \frac{ \norm { \gamma ( \alpha ) }_2^2 }{ \norm { \gamma ( \alpha ) }_1^2 } \subjto B\gamma \left( \alpha \right) \in \Gamma_1^{\eta}
% \end{align}

% Now from lemma 4 in \cite{wang2021tight} we have that map $ \alpha \mapsto \frac{ \norm{ \gamma ( \alpha ) }_2^2 }{ \norm{ \gamma ( \alpha ) }_1^2 } $ is monotonically decreasing. 
% \red{Say that it is a interval - this follows from the convexity.}



% Hence if we find value of $\alpha_{\uls}$ such that $\alpha_{\uls} \leq \alpha_{\nstar}$ and $ b \gamma ( \alpha_{\uls} ) \not \in \Gamma_1^{\eta}$ for any $ b > 0 $ then we have:
% \begin{align} \label{eq:eta_bound_first_reduction}
%     \eta^2 \leq  B^2 \frac{ \norm { \gamma ( \alphauls ) }_2^2 }{ \norm { \gamma ( \alphauls ) }_1^2 }
% \end{align}

% In order to saturate constraint $ \norm{ \wtwo }_1 \leq B $ let $ b = \frac{B}{\alphauls}$. Since we want that $  b \gamma ( \alpha_{\uls} ) \not \in \Gamma_1^{\eta} $ we will chose $s$ such that:
% \begin{align}
%     B^2 \frac{ \innerprod{ \gamma ( \alphauls )}{H}^2 }{ n \alphauls^2 } < \consteta B^2 \frac{ \norm{ \gamma ( \alphauls ) }_2^2 }{ \alphauls^2 }
% \end{align}
% Rewriting this inequality gives:
% \begin{align} \label{eq:s_condition_one}
%   \frac{ \norm{ \gamma ( \alphauls ) }_2^2 }{ \norm{H}_{\infty}^2 } > \frac{ 1 }{ \consteta n } 
% \end{align}
% Now we use concentration result from lemma \ref{lemma_gamma_conc} to get the following condition on $s$:
% \begin{align}
%     \frac{ 2 }{ \uls t_s^2 } \left( 1 - \frac{ c }{ \tuls^2 } \right) > \frac{ 1 }{ \consteta n }
% \end{align}

%  We claim that $\uls =\lambda_{\uls} \frac{ n }{ \log (d/n) }$ satisfies this inequality for some positive universal constant $ \lambda_{\uls} >0  $. From lemma 3 in \cite{wang2021tight} we know that if $ d/\uls \geq 11 $ we have that $ \log (d/\uls) \leq \tuls^2 \leq 2 \log (d/\uls) $. Using both of these bounds into expression \eqref{eq:s_condition_one} gives that:
% \begin{align}
%     \frac{ 2 }{ \uls \tuls^2 } \left( 1 - \frac{ c }{ \tuls^2 } \right) &> \frac{ 1 }{ 2 n \lambda_{\uls} } \frac{ \log (d/n) }{ \log (d/n) + \log \log (d/n) - \log \lambda_{\uls} } \left( 1 - \frac{c}{ \log (d/n) + \log \log (d/n) - \log \lambda_{\uls} } \right)
%     \\
%     & = \frac{ 1 }{ 2 n \lambda_{\uls} } \left( 1 - O \left( \frac{\log (d/n) }{\log \log (d/n) } \right) \right) > \frac{1}{\consteta n}
% \end{align}
% where last inequality holds for $d/n$ sufficiently large.

% Now from equation \eqref{eq:eta_bound_first_reduction} and concentration lemma \ref{lemma_gamma_conc} we have:
% \begin{align}
%     \eta^2 \leq \frac{ n \fstar }{ \tnstar^2 } \frac{2}{\uls}\left( 1 + \frac{c}{\tuls^2} \right) \leq \boundeta' \left( 1 + O \left( \frac{1}{ \log (d/n) } \right) \right) \leq \boundeta^2
% \end{align}

% \paragraph{Upper bound on $\nu$.} Now we derive an upper bound for $\nu$. We consider the following set:
% \begin{align}
%     \Gamma_1^{\nu} = \left\{ (\wone,\wtwo) 
%     \subjto
%     \frac{ \innerprod{\wtwo}{H}^2 }{ n } \geq \constnu \nu^2 \andtxts \norm{ \wtwo }_1 \leq \loneboundclas \andtxts \norm{ \wtwo }_2 \leq \boundeta  \right\}
% \end{align}
% Once again it follows that $\Gamma_0 \subset \Gamma_1^{\nu}$. Hence we can upper bound $\nu$ as follows:
% \begin{align} \label{eq:nu_opt_first_reduction}
%     \nu^2 \leq \frac{ 1 }{ n \constnu } \max_{\wtwo} \innerprod{\wtwo}{H}^2
%     \subjto 
%     \norm{ \wtwo }_1 \leq \loneboundclas 
%     \andtxts 
%     \norm{ \wtwo }_2 \leq \boundeta
% \end{align}

% Now we show can this optimization problem can be rewritten in a form suitable for using parametrized path approach. Similarly as in \cite{wang2021tight} we define function $\olw : \left[ \frac{1}{d}, 1 \right] \to \RR^{d-1}$ as
% \begin{align}
%     \olw(\beta) = \argmax_{\wtwo} \innerprod{\wtwo}{\Hgaussian}
%     \subjto \begin{cases}
%                 \norm{\wtwo}_2^2 \leq \beta \\
%                 \wtwo\geq 0\\
%                 \norm{\wtwo}_1 = 1
%             \end{cases}
% \end{align}
% From claim 2 in \cite{wang2021tight} we know that for any $\beta \in \left[ \frac{1}{d}, 1 \right] $ there exists $ \alpha \in \left[ 1, \alpham \right] $ such that $ \olw (\beta) = \frac{ \gamma(\alpha) }{ \alpha }$. Following similar argument as in fourth statement of lemma 4 in \cite{wang2021tight} we have that $ \olw (\beta) $ is monotonically increasing function in $\beta$. 

% Setting $ \tildewtwo = \frac{ \wtwo }{ B }$ we can rewrite \eqref{eq:nu_opt_first_reduction} as:
% \begin{align} 
%     \nu^2 \leq \frac{ B^2 }{ n \constnu } \max_{\tildewtwo} \innerprod{ \tildewtwo }{ H }^2
%     \subjto 
%     \norm{ \tildewtwo }_1 \leq 1 
%     \andtxts 
%     \norm{ \tildewtwo }_2 \leq \frac{ \boundeta }{ B }
% \end{align}
% Hence solution of this problem must be of the form $ \tildewtwo = \olw (\beta) $ for some $\beta$. 
% Similarly as in the first part of this proof, we first show that there exists $\beta_{\nstar}$ which satisfies constraints, and then find $\beta_{\ols}$ such that $ \beta_{\ols} \geq \beta_{\nstar}$. From monotonicity of $ \olw (\beta)$ follows that $ \olw (\beta_{\ols}) \geq \olw (\beta_{\nstar})$. \red{so this is unclear: explain why equivalentely.} Equivalently, we can find $\alpha_{\uls}$ such that $\alpha_{\uls} \leq \alpha_{\nstar}$.

% \begin{align}\label{nu_bound_first_reduction}
%     \nu^2 
%     \leq
%     \frac{ B^2 }{ n \constnu } \frac{ \innerprod{ \gamma (\alphauls) }{ H }^2 }{ \alphauls^2 } 
%     \leq 
%     \frac{ B^2 }{ n \constnu } \frac{ \norm{H}_{\infty}^2 }{ \alphauls^2 }
% \end{align}

% Let $\tildewtwo = \frac{ \gamma (\alpha) }{ \alpha }$. The claim that $\alpha_{\nstar}$ satisfies constraints is once again straightforward from our definition of $B$. Now we want to find $\alphauls$ such that:
% \begin{align}\label{s_condition_nu_first_reduction}
%     \norm{ \tildewtwo }_2^2 = \frac{ \norm{ \gamma ( \alphauls ) }_2^2 }{ \alphauls^2 } > \frac{ \boundeta^2 }{ B^2 }
% \end{align}
% Using concentration result from lemma \ref{lemma_gamma_conc} and expression \eqref{phidn_bound} we get the condition:
% \begin{align}
%     \frac{2}{\uls} \left( 1 - \frac{c}{\tuls^2} \right) > \frac{\boundeta^2 \tnstar^2}{ n \fstar }
% \end{align}
% Once again we claim that this equality is satisfied for $ \uls = \frac{ c n }{ \log (d/n) } $ for some positive constant $c$. It is easy to see that this is the same condition as in the previous part of the proof up to the constants and hence we can use the same proof here.

% From \eqref{nu_bound_first_reduction} we now have:
% \begin{align}
%     \nu^2 \leq \frac{ \fstar \tuls^2 }{ \constnu \tnstar^2 } \left( 1 - \frac{4}{\tuls^2} \right)^{-1} 
%     \leq c'_{\nu} \left( 1 + O \left( \frac{ \log \log (d/n) }{\log (d/n) } \right) \right) \leq \boundnu^2
% \end{align}
% concluding the proof.



% \subsection{Proof of Lemma~\ref{lemma_second_reduction}}


% From lemma \ref{lemma_first_reduction} we know that with high probability $ \nu \leq c_{\nu} $ and $ \eta \leq c_{\eta} $. Hence we can use uniform convergence of $\fnclas$ to its expectation (proposition \ref{prop:unifConv}). Hence we can relax constraints from definition of set $\Gamma_0$ as follows:
% \begin{align}
%     \frac{ \innerprod{\wtwo}{H}^2 }{ n } \geq f ( \nu, \eta ) - \constconc \geq  \fstar  + \tconstnu \deltanu^2 + \tconsteta \eta^2 - \constconc
% \end{align}
% where the second inequality follows from lemma \ref{lemma_quadratic_4lus_fstar_bound}. Hence we consider set:
% \begin{align}
%     \Gamma_2^{\eta} = \left\{ (\wone,\wtwo) \subjto \frac{ \innerprod{\wtwo}{H}^2 }{ n } \geq \fstar - \constconc +  \tconsteta \eta^2  \andtxts \norm{ \wtwo }_1 \leq \loneboundclas  \right\}
% \end{align}

% \paragraph{Bounding $\eta$} 
% Following the same argument as in proof of lemma \ref{lemma_first_reduction} instead of inequality \eqref{eq:s_condition_one} we get:
% \begin{align}
%     \frac{ \left( \fstar - \constconc \right) \alpha_s^2 }{ B^2 \norm{H}_{\infty}^2 } + \tconsteta \frac{ \norm{ \gamma(\alpha_s) }_2^2 }{ \norm{H}_{\infty}^2 } > \frac{1}{n}
% \end{align}
% In order for inequality above to be satisfied we need:
% \begin{align}
%     \left( 1 - \frac{ \constconc }{ \fstar } \right) 
%     \frac{\tnstar^2}{t_s^2}
%     \left( 1 - \frac{4}{t_s^2} + O \left( \frac{1}{t_s^4} \right) \right) 
%     \left( 1 + \frac{2}{\tnstar^2} + O \left( \frac{1}{\tnstar^3} \right) \right) 
%     + \frac{2 n \tconsteta}{s t_s^2} \left( 1 + O \left( \frac{1}{t_s^2} \right) \right) 
%     > 1
% \end{align}
% Assuming that $ s = \lambda \nstar$ and $ \constconc = O \left( \frac{1}{\tnstar^3} \right) $ we have:
% \begin{align}
%     \frac{\tnstar^2}{t_s^2}
%     \left( 1 + \frac{ \frac{4\tconsteta}{\lambda\feestar}  - 4}{t_s^2} + \frac{2}{\tnstar^2} + O \left( \frac{1}{\tnstar^3}, \frac{1}{t_s^3} \right) \right)
%     > 1
% \end{align}
% Fix $\ulambda > 0$. Choose $\uls = \lambda_{\uls} \nstar$ such that $\uls < n$ is the largest integer for which $ \tuls^2 \geq \tnstar^2 + \ulambda $. Then we have condition:
% \begin{align}
%     \left( 1 - \frac{\ulambda}{\tuls^2} \right) \left( 1 + \frac{ \frac{4\tconsteta}{\lambda_{\uls}\feestar}  - 4}{\tuls^2} + \frac{2}{\tnstar^2} + O \left( \frac{1}{t_n^3} \right) \right)
%     > 1
% \end{align}
% For $\ulambda$ large enough inequality holds (Note: second brackets grow as $\lambda_{\uls}^{-1}$ and the first decays like $\log ( \lambda_{\uls} )$ - TO CHECK).


% \red{okay I messed this up - sorry. Can you make the following section a bit clearer? In particular, the connection to tn and s is not clear, cite the result form our paper. . So here we need to say that essentially we obtain the same problem as studied in my paper.}
% Fix $\olambda > 0$. Now we choose $\ols = c_{\ols} \nstar$ such that $ \ols > n $ is the smallest integer for which $ t_{\ols}^2 \leq \tnstar^2 - \olambda $. Then we have:
% \begin{align}
%     \left( 1 + \frac{\olambda}{\tols^2} \right) \left( 1 + \frac{ \frac{4\tconsteta}{c_{\ols}\feestar}  - 4}{\tols^2} + \frac{2}{\tnstar^2} + O \left( \frac{1}{t_n^3} \right) \right)
%     > 1
% \end{align}
% We claim that there exists $\olambda$ large enough such that this inequality holds (e.g. $\ulambda > 4$).

% Hence we can bound $\eta^2$ as follows:
% \begin{align} \label{eq:eta_bound_first_reduction}
%     \eta^2 
%     \leq
%     B^2 \frac{ \norm { \gamma ( \alphauls ) }_2^2 }{ \norm { \gamma ( \alphauls ) }_1^2 } 
%     \leq
%     \frac{ n \left( \fstar - \constconc \right) }{ \tnstar^2 } \frac{2}{\uls}\left( 1 + \frac{c}{\tuls^2} \right) 
%     \leq
%     \frac{c_{\eta}'}{\log (d/n) } \left( 1 + O \left( \frac{1}{ \log (d/n) } \right) \right) 
%     \leq
%     \left( \frac{ B_{\eta,2} }{ \sqrt{\log (d/n)} } \right)^2
% \end{align}
% and similarly we get:
% \begin{align}
%     \eta^2 
%     \geq
%     B^2 \frac{ \norm { \gamma ( \alphaols ) }_2^2 }{ \norm { \gamma ( \alphaols ) }_1^2 } 
%     \geq
%     \left( \frac{ \overline{B}_{\eta,2} }{ \sqrt{\log (d/n)} } \right)^2
% \end{align}

% \paragraph{Bounding $\nu$.}
% Following the proof of lemma \ref{lemma_first_reduction} we determine tighter upper bound for $\nu^2$.
% \begin{align}
%     \Gamma_2^{\nu} = \left\{ (\wone,\wtwo) 
%     \subjto
%     \frac{ \innerprod{\wtwo}{H}^2 }{ n } \geq \fstar - \constconc + \tconstnu \nu^2 \andtxts \norm{ \wtwo }_1 \leq \loneboundclas \andtxts \norm{ \wtwo }_2 \leq \frac{B_{\eta,2}}{\sqrt{ \log (d/n) }}  \right\}
% \end{align}

% Analogously to equation \eqref{s_condition_nu_first_reduction} we derive new condition for $\uls$ as:
% \begin{align}
%     \norm{ \tildewtwo }_2^2 = \frac{ \norm{ \gamma ( \alphauls ) }_2^2 }{ \alphauls^2 } > \frac{ B_{\eta,2}^2 }{ B^2 \log (d/n) }
% \end{align}
% which is again satisfied for some $\uls = \lambda_{\uls} n$ with $ \lambda_{\uls} > 0 $. Hence from \eqref{nu_bound_first_reduction} we obtain bound:
% \begin{align}
%     \deltanu^2 
%     \leq
%     \frac{ B^2 }{ n \tconstnu } \frac{ \norm{H}_{\infty}^2 }{ \alphauls^2 } - \frac{\fstar - \constconc }{\tconstnu}
%     \leq 
%     \frac{ \fstar }{ \tconstnu \tnstar^2 } \left( 1 + \frac{4}{\tuls^2} \right) - \frac{\fstar - \constconc }{\tconstnu}
%     \leq 
%     \left( \frac{ B_{\nu,2} }{ \sqrt{\log (d/n)} } \right)^2
% \end{align}
% which concludes the proof.











































% \section{Proof of Theorem \ref{thm:mainl1}}

% \red{Improve this, here we need to have the proof for L1}.

% \end{document}




















































% \subsection{Step 1: Reduce optimization problem via a path approach.}
% Following the work in \cite{wang2021tight} we can recast \eqref{eq:phin}, \eqref{eq:phip}, \eqref{eq:phim} as optimization problems in three scalar variables. Let $b,\alpha$ be scalar variables with $b\geq 0$, $\alpha\in[1,\alpham]$ with $\alpham = d\frac{\norm{\Hgaussian}_{\infty}}{\norm{\Hgaussian}_1}$. Then we define parametric path $b\gamma(\alpha)$ with $\RR^d$-valued function $\gamma$ given by:
% \begin{equation}
%     \gamma(\alpha) = \argmin_{\wtwo} \norm{\wtwo}_2^2
%     \subjto \begin{cases}
%                 \innerprod{\wtwo}{\Hgaussian} \geq \norm{\Hgaussian}_{\infty}\\
%                 \wtwo\geq 0\\
%                 \transp{\onevec} \wtwo = \norm{\wtwo}_1 = \alpha
%             \end{cases}
% \end{equation}

% We then obtain the following result. 
% \begin{restatable}{proposition}{propparam}
% % \begin{proposition} 
% \label{prop:parametrization}
% Optimization problems \eqref{eq:phin}, \eqref{eq:phip}, \eqref{eq:phim} are equivalently given by:
%         \begin{align}
%         \tag{$A_N$}\label{eq:phin}
%             \phidn &= \min_{\nu,b,\alpha} \nu + \alpha b
%             \subjto \frac{1}{n}  b^2\norm{\Hgaussian}_{\infty}^2  \geq  \fnclas(\nu,b\|\gamma(\alpha)\|_2). \\
%         \tag{$A_+$} \label{eq:phip}
%             \phidp &= \max_{\nu,b,\alpha}  \frac{\nu}{\sqrt{\nu^2+b^2\norm{\gamma(\alpha)}_2^2}}
%             \subjto 
%                   (\nu, b\norm{ \gamma(\alpha) }_2) \in \Gamma_0 \\
%         \tag{$A_-$} \label{eq:phim}
%             % \phidm &= \min_{\nu,b,\alpha}  \frac{\nu}{\sqrt{\nu^2+b^2\norm{\gamma(\alpha)}_2^2}}
%             % \subjto \begin{cases}
%             %   \frac{1}{n}  b^2\norm{\Hgaussian}_{\infty}^2  \geq  \fnclas(\wone,b\|\gamma(\alpha)\|_2)\\
%             %     \nu+b \leq \loneboundclas
%             % \end{cases}
%     \phidm &= \min_{\nu,b,\alpha}  \frac{\nu}{\sqrt{\nu^2+b^2\norm{\gamma(\alpha)}_2^2}}
%             \subjto
%               (\nu, b\norm{ \gamma(\alpha) }_2) \in \Gamma_0
%         \end{align}
% for some scalars $\nu,b>0$ and $\alpha\in[1,\alpham]$,
%  with
% $ \eta = b\norm{ \gamma(\alpha) }_2 $ and
% \begin{align}
%     \Gamma_0 = \left\{ (\nu,\eta) \subjto\frac{1}{n}  b^2\norm{\Hgaussian}_{\infty}^2  \geq  \fnclas(\nu,b\|\gamma(\alpha)\|_2) ~~\andtxt~~  \nu+b \leq \loneboundclas \right\}.
% \end{align}

% \end{restatable}  
% In order to study this reformulated optimization problem, we make use of the following two properties of $\gamma(\alpha)$ from \cite{wang2021tight}:

% \paragraph{Concentration of  $\norm{\gamma(\alpha)}_2$.} 
% From \cite{wang2021tight} we know that $ \gamma ( \alpha ) $ is a piecewise linear function with breakpoints at $ \alpha_s $ for $ s = 2, \dots, d$, with
% \begin{equation}
%     \alpha_s =....
% \end{equation}


% \begin{proposition}[Proposition 4 form \cite{wang2021tight}]
% \label{prop:concentrationl1}
% (Concentration of norms of $\gamma(\alpha_s)$, proposition 4 in \cite{konst}) Let $\ts$ be given by $2\Phic(\ts) = s/d$. There exists universal positive constants $c,c_s,c_2,c_3>0$ such that for any $s,d$ with $s\geq c_s$ and $c_2s\leq d\leq \exp(c_3 s^{1/5})$ we have that:
%     \begin{align}
%         \abs{
%             \frac{\norm{\gamma(\alphathr{s})}_1}{\norm{\Hgaussian}_\infty} - \left(\frac{1}{\ts} - \frac{2}{\ts^3}\right)
%         }
%         &\leq \frac{c}{\ts^5}
%         \qquad \andtxt \qquad
%         \abs{
%             \frac{\norm{\gamma(\alphathr{s})}_2^2}{\norm{\Hgaussian}_\infty^2} - \frac{2}{s \ts^2}
%         }
%         \leq \frac{c}{s \ts^4}, \label{eq:concentration}
%     \end{align}
% with probability at least $1-6\exp\left(-\frac{s}{\log(d/s)^5}\right)$ over the draws of $h$.
% \label{lemma_gamma_conc}
% \end{proposition}

% \paragraph{Convexity and monotonicity of  $\gamma(\alpha)$. }


% \red{State monotinicity result here.}


% \subsection{Step 2: Localisation step - bounding $\phidn$}
% In a first step, we derive an upper bound on $\phidn$. For this, it is sufficient to find a feasible point. Let $f(\nu,\eta) = \EE \left[ \possq{1-\xi\abs{\gausswone}\nu-\gausswtwo \eta} \right] $ be the expectation of $\fnclas$ over $\xsui$, $\Ggaussian$ and $\xi$. Using the concentration of Lipschitz continuous function, we can show that:
% \begin{lemma}
% \label{lemma_point_conv}
% For any $\nu,\eta>0$ holds that:
%     \begin{align}
%         \prob \left( \abs{ \fnclas \left( \nu, \eta \right) - \EE \left[ \fnclas \left( \nu, \eta \right) \right] }  \geq t \right) \leq 2 \exp \left( - c \frac{ n t^2 }{ \nu^2 + \eta^2 } \right)
%     \end{align}
% where $c$ is a positive universal constant. 
% \end{lemma} 

% The goal is now to show that we can find a feasible point $(\nubar, \eta)$ with $\nubar = \argmin f(\nu, 0)$ and $\eta = O(\frac{1}{\log(d/n)}$. For this, we can take the Taylor series approximation of $f$ around$(\nuopt,0)$,   $f(\nu, \vstar) \approx \fstar + \fnclasunu \nu^2$, which allows us to rewrite the constraint in $\phidn$ to 
% \begin{equation}
%     \frac{1}{n}  b^2\norm{\Hgaussian}_{\infty}^2  \geq  \fstar + \fnclasunu \nu^2 + O(...).
% \end{equation}

% Further, following a similar approach as in Proposition~2 in \cite{wang2021tight} by applying the concentration results in Proposition~\ref{prop:concentrationl1}, we can show the following Proposition~\ref{prop:Rbound} which gives an upper bound on $\phdn$. The proof is devoted to Appendix ...

% % a similar approach in the proof of Proposition~2 in \cite{wang2021tight}, where tight bounds for $\phidn$ for min-l1-norm interpolation are derived, we can show the following bound on $\phidn$ given in  Proposition \ref{prop:Rbound}. The proof may be found in Appendix~... 
% \begin{restatable}{proposition}{propRbound}
% \label{prop:Rbound}
% Let $t_{\nopt}$ be given by $2\Phic(t_{\nopt}) = \nopt/d$ with $\nopt = n\feestar/2$. There exist universal positive constants $c,c_1,c_2,c_3,c_4$ such that, if $n\geq c_1$ and $c_2 n\leq d\leq \exp(c_3 n^{1/5})$ then
%     \begin{align} \label{phidn_bound}
%         (\phidn)^2 
%         \leq
%         \frac{ n f (\nuopt, 0) }{ \tnstar^2 } \left( 1 - \frac{ 2 }{ \tnstar^2 } + \frac{c}{ \tnstar^3 } \right) =:\loneboundclas^2
%     \end{align}
% with probability at least $ 1 - 2 \exp \left( -\frac{ c_4 n }{ \tnstar^6 } \right) - 6 \exp \left( -\frac{\nstar}{\log^5(d/\nstar)} \right) $ over the draws of $\Hgaussian$, $\gausswone$ and $\gausswtwo$.
% \end{restatable}  





% \subsection{Step 3: Uniform convergence.}
% The goal of this is to study the constraint set $\Gamma_0$ given the bound $M \geq \phidn$ from the previous step. In particular, we show the following Proposition ~\ref{prop:BoundOmegal1}. The bounds on $\phidn$ and $\phidp$ then follow straightforwardly in the next section. 

% \begin{restatable}{proposition}{BoundOmegal1}
% \label{prop:BoundOmegal1}
% There exist universal constants $ c_1, c_2, c_1, c_2, c_3 > 0 $ such that, if $ n\geq c_1 $ and $ c_2 n \leq d \leq \exp \left( c_3 n^{1/5} \right) $, then
% \red{Stefan, need to make this tighter!}
% \begin{align}
% \Gamma_0 \subset \{(\nu, \eta) \subjto  \vert \eta^2 \vert = \Gamma(1/\log(d/n))~~\andtxt~~ \vert \nu-\nubar\vert = O(1/\log(d/n))\}
% \end{align}
% with probability at least $ 1 - $.
% \end{restatable}  
% \begin{proof}
% The proof of the proposition follows from several steps where in each step we approximate $\fnclas$ using the the bounds on $(\nu, \eta)$ from the previous steps to obtain a tighter bound on $(\nu, \eta)$ using the tools developed in \cite{wang2021tight}.  



% \paragraph{Bound 1:}
% In a first step, we use the fact that in the presence of label noise, $\fnclas$ is lower bounded by a quadratic function:
% \begin{lemma} \label{quadratic_bound_fn}
%     There exist positive constants $\constnu$ and $\consteta$ such that for any $\nu,\eta$ we have that: 
%         \begin{align}
%             \fnclas(\nu,\eta) \geq \constnu \nu^2  + \consteta \eta^2
%         \end{align}
%     with probability at least $1 - \exp \left( - n \kldiv{\frac{\sigma}{2}}{\frac{\sigma}{4}} \right) - \exp \left( -\frac{ n\sigma }{ 128 } \right)$ over the draws of $\gausswone,\gausswtwo,\xi$.
% \end{lemma}
% As a result, we can approximate relax the first constraint in $\Gamma_0$ to 
% \begin{equation}
%     b^2\norm{\Hgaussian}_{\infty}^2  \geq  \constnu \nu^2  + \consteta \eta^2.
% \end{equation} 

% \red{say more about the intuition, then we can show:}

% \begin{lemma} \label{lemma_first_reduction}
%     There exist universal constant $c > 0$ such that for any element $(\wone,\wtwo)$ of $\Gamma_0$ we have that $\norm{ \wone }_2 = \nu \leq \boundnu $ and $\norm{ \wtwo }_2 = \eta \leq \boundeta$ with probability at least $ 1 - $ over the draws of $..$.
% \end{lemma}


% \paragraph{Bound 2:}
% Define $\deltanu= \nu - \nubar$. Using the fact from the previous section that $\nu \leq \constnu, \eta \leq \consteta$, we obtain a tigher lower bound for $\fnclas$ form the following lemma. 

% \begin{lemma} \label{lemma_quadratic_4lus_fstar_bound}
%     There exist positive constants $\tconstnu$ and $\tconsteta$ such that for any $\nu \leq \constnu, \eta \leq \consteta$ we have that: 
%         \begin{align}
%             f(\nu,\eta) \geq \fstar + \tconstnu \left( \deltanu \right)^2  + \tconsteta \eta^2+ \OOOc
%         \end{align}
%     with probability at least $1 - \exp \left( - n \kldiv{\frac{\sigma}{2}}{\frac{\sigma}{4}} \right) - \exp \left( -\frac{ n\sigma }{ 128 } \right)$ over the draws of $\gausswone,\gausswtwo,\xi$.
% \end{lemma}

% Plugging in this expression, we can again show:
% \begin{lemma} \label{lemma_second_reduction}
%     There exist universal constants $B_{\nu,2} > 0, B_{\eta,2} > 0$ such that for any element $(\wone,\wtwo)$ of $\Gamma_0$ we have that $\deltanu^2 \leq \frac{B_{\nu,2}^2}{ \log \left( d/n \right) }$ and $ \eta^2 \leq \frac{B_{\eta,2}^2}{ \log \left( d/n \right) }$ with probability at least $ 1 - $ over the draws of $..$.
% \end{lemma}


% \paragraph{Bound 3:}
% This is still under work...
% \begin{lemma}
%     There exist universal constant $B_{\nu,3} > 0, B_{\eta,3} > 0$ such that for any element $(\wone,\wtwo)$ of $\Gamma_0$ we have that $\deltanu^2 \leq \frac{B_{\nu,3}^2}{ \left( \log \left( d/n \right) \right)^{3/2} }$ and $ \eta^2 \leq \frac{B_{\eta,3}^2}{ \log \left( d/n \right) }$ with probability at least $ 1 - $ over the draws of $..$.
% \end{lemma}






% \end{proof}



% \subsection{Summary. }
% We have:
% \begin{align}
%     \max \frac{ \nu }{ \sqrt{ \nu^2 + \eta^2 } } 
%     & \leq
%     \frac{ \nubar + \deltanu }{ \sqrt{ ( \nubar + \deltanu )^2 + \eta^2 } }
%     \\
%     & = 
%     \left( 1 + \frac {\deltanu}{\nubar} \right) \left( 1 - \frac{1}{2} \left( \frac{2\deltanu}{\nubar} + \frac{\deltanu^2 + \eta^2}{(\nubar)^2} \right) + \frac{3}{8} \left( \frac{2\deltanu}{\nubar}\right)^2 + O \left( \frac{1}{ \log (d/n)^{3/2}} \right) \right)
%     \\
%     & = 1 - \frac{\eta^2}{2(\nubar)^2} + O \left( \frac{1}{ \log (d/n)^{3/2}} \right) 
%     \leq 
%     1 - W \left( \frac{1}{\log (d/n) } \right)
% \end{align}
% and
% \begin{align}
%     \min \frac{ \nu }{ \sqrt{ \nu^2 + \eta^2 } } 
%     & \geq
%     \frac{ \nubar - \deltanu }{ \sqrt{ ( \nubar - \deltanu )^2 + \eta^2 } }
%     \\
%     & = 
%     \left( 1 - \frac {\deltanu}{\nubar} \right) \left( 1 - \frac{1}{2} \left( -\frac{2\deltanu}{\nubar} + \frac{\deltanu^2 + \eta^2}{(\nubar)^2} \right) + \frac{3}{8} \left( \frac{2\deltanu}{\nubar}\right)^2 + O \left( \frac{1}{ \log (d/n)^{3/2}} \right) \right)
%     \\
%     & = 1 - \frac{\eta^2}{2(\nubar)^2} + O \left( \frac{1}{ \log (d/n)^{3/2}} \right) 
%     \geq 
%     1 - O \left( \frac{1}{\log (d/n) } \right)
% \end{align}

% Using approximation $ \arccos(1-x) \approx \sqrt{2x} + O (x\sqrt{x}) $ we have
% \begin{align}
%     W \left( \frac{1}{\log (d/n)^{1/2} }  \right) 
%     \leq
%     R(w) = \frac{1}{\pi} \arccos \left( \frac{\innerprod{w}{\wgt}}{\norm{w}_2} \right) 
%     \leq 
%     O \left( \frac{1}{\log (d/n)^{1/2} } \right)
% \end{align}
% with high probability $ 1 - $.





% \subsection{Proof of Proposition~\ref{prop:Rbound}}


% Recall that $\phidn$ is given by:
% \begin{align}
%     \phidn &= \min_{\nu,b,\alpha} \nu + b \norm{ \gamma \left( \alpha \right) }_1 
%     \subjto \frac{ b^2\norm{\Hgaussian}_{\infty}^2 }{n} \geq \fnclas \left( \nu, b \norm{ \gamma \left( \alpha \right) }_2 \right)
% \end{align}

% Given that $(\tnu,\tb,\talpha)$ is a feasible point of $\phidn$ we have that $\phidn \leq  \tnu + \tb \norm{ \gamma( \talpha) }_1$, which gives us an upper bound on $\phidn$. In the following discussion our goal is to find a single feasible point of the constraint set of $\phidn$.

% From definition of $\gamma ( \alpha )$ we know that $ \norm{ \gamma ( \alpha ) }_1 = \alpha$ and hence we can equivalently formulate $\phidn$ as an optimization over $\nu$ and $ b_{\alpha} := b \alpha $
% \begin{align}
%     \phidn &= \min_{ \nu, b_{\alpha} } \nu + b_{\alpha}
%     \subjto \frac{ b_{\alpha}^2 \norm{\Hgaussian}_{\infty}^2 }{n \alpha^2} \geq \fnclas \left( \nu, b_{\alpha} \frac{ \norm{ \gamma \left( \alpha \right) }_2}{ \alpha } \right)
% \end{align}

% Define $\fstar = f \left( \nubar, 0 \right)$, $\feestar = \frac{\partial^2 f(\nuopt,\eta)}{\partial \eta^2}\Big|_{\eta=0}$ and $\nstar = \frac{1}{2}\feestar n$. Now using lemma \ref{lemma_point_conv} with $ t = \fstar \tnstar^{-3} $ and for a feasible point $( \nu, b_{\alpha} \frac{ \norm{ \gamma \left( \alpha \right) }_2}{ \alpha } )$ we have that:
% \begin{align} \label{eq:constraint_f_conc}
%     \frac{ b_{\alpha}^2 \norm{\Hgaussian}_{\infty}^2 }{n \alpha^2} 
%     \geq
%     f \left( \nu, b_{\alpha} \frac{ \norm{ \gamma \left( \alpha \right) }_2}{ \alpha } \right) + \frac{\fstar}{\tnstar^{3}}
% \end{align}
% with probability at least $ 1 - 2 \exp \left( -c \frac{ n }{ \tnstar^6 \left( \nu^2 + b_{\alpha}^2  \norm{ \gamma \left( \alpha \right) }_2^2 / \alpha^2 \right) } \right) $.
% % > 1 - 2 \exp \left( - \tc \frac{ n }{ \log^3 \left( \frac{d}{n} \right)  } \right) $.

% Let's now choose $ \nu = \nubar $ and show that there exists a pair $ ( b, \alpha )$  such that $ ( \nubar, b, \alpha) $ is feasible for constraint \eqref{eq:constraint_f_conc}. Furthermore, we propose to search for a point with parameter $ ( b, \alpha ) $ such that $ b \norm{ \gamma ( \alpha )}_2 = b_{\alpha} \frac{ \norm{ \gamma \left( \alpha \right) }_2}{ \alpha } $ is near zero. Hence, using Taylor series approximation of function $ f ( \nubar, \cdot ) : \eta \mapsto f (\nubar, \eta) $ around point $(\nuopt,0)$ we can rewrite constraint \eqref{eq:constraint_f_conc} as:
% \begin{align}
%      \frac{ b_{\alpha}^2 \norm{\Hgaussian}_{\infty}^2 }{n \alpha^2}   
%      \geq
%       \fstar + \frac{1}{2}\feestar b_{\alpha}^2 \frac{ \norm{ \gamma \left( \alpha \right) }_2^2}{ \alpha^2 } + O \left( b_{\alpha}^3 \frac{ \norm{ \gamma \left( \alpha \right) }_2^3}{ \alpha^3 } \right) + \frac{\fstar}{\tnstar^{3}}
% \end{align}
% since $\feta = \frac{\partial f(\nuopt,\eta)}{\partial \eta}\Big|_{\eta=0} = 0$.

% Now from \cite{wang2021tight} we know that $ \gamma ( \alpha ) $ is a piecewise linear function with breakpoints at $ \alpha_s $ for $ s = 2, \dots, d $. Hence instead of optimizing over $\alpha$ we optimize over $s$. Note that we have only one constraint but two free variables $ ( b, \alpha ) $ and so we can set $ \alpha = \alpha_{\nstar} $ with $ \nstar = \frac{1}{2}\feestar n $. We explain this choice of $s$ in the remark after the proof. Combining all these results we get constraint:
% \begin{align} \label{eq:B_ineq}
%      \frac{ b_{\alpha_{\nstar}}^2 \norm{\Hgaussian}_{\infty}^2 }{n \alpha_{\nstar}^2}   
%      \geq
%       \fstar + \frac{1}{2}\feestar b_{\alpha_{\nstar}}^2 \frac{ \norm{ \gamma \left( \alpha_{\nstar} \right) }_2^2}{ \alpha_{\nstar}^2 } + O \left( b_{\alpha_{\nstar}}^3 \frac{ \norm{ \gamma \left( \alpha_{\nstar} \right) }_2^3}{ \alpha_{\nstar}^3 } \right) + \frac{\fstar}{\tnstar^{3}}
% \end{align}

% Now we claim that
% \begin{equation}
%     b_{\alpha_{\nstar}}^2 = \frac{ n \alpha_{\nstar}^2 }{ \norm{\Hgaussian}_2^2 } \frac{ \fstar \left( 1 + \frac{1}{\tnstar^{3}} \right) }{ 1 - \frac{1}{2} n \feestar \frac{ \norm{ \gamma \left( \alpha_{\nstar} \right) }_2^2 }{ \norm{H}_{\infty}^2 } - O \left( \frac{1}{\tnstar^3} \right) }
% \end{equation}
% satisfies inequality \eqref{eq:B_ineq} with probability at least $ 1 - 6 \exp \left( -\frac{\nstar}{\log^5(d/\nstar)} \right)$. Using lemma \ref{lemma_gamma_conc} we have that:
% \begin{equation}
%     1 - \frac{1}{2} n \feestar \frac{ \norm{ \gamma \left( \alpha_{\nstar} \right) }_2^2 }{ \norm{H}_{\infty}^2 } - O \left( \frac{1}{\tnstar^3} \right) > 1 - \frac{1}{2} n \feestar  \frac{2}{\nstar \tnstar^2} - O \left( \frac{1}{\tnstar^3} \right) = 1 - \frac{2}{\tnstar^2} - O \left( \frac{1}{\tnstar^3} \right)  > 0
% \end{equation}
% holding for $d,n$ sufficiently large. Applying lemma \ref{lemma_gamma_conc} once again we get:
% \begin{equation}
%     b_{\alpha_{\nstar}}^2 
%     \leq
%     \frac{ n \fstar }{ \tnstar^2 } \left( 1 + \frac{1}{\tnstar^3} \right) \left( 1 - \frac{4}{\tnstar^2} + \frac{c}{\tnstar^4} \right) \frac{1}{ 1 - \frac{2}{\tnstar^2} - O \left( \frac{1}{\tnstar^3} \right)}
%     \leq
%     \frac{ n \fstar }{ \tnstar^2 } \left( 1 - \frac{2}{\tnstar^2} + \frac{c}{\tnstar^3} \right)
% \end{equation}

% Hence we have that $ O \left( b_{\alpha_{\nstar}}^3 \frac{ \norm{ \gamma \left( \alpha_{\nstar} \right) }_2^3}{ \alpha_{\nstar}^3 } \right) = O \left( \frac{1}{\tnstar^3} \right)$ and this $b_{\alpha_{\nstar}}^2$ indeed satisfies equation \ref{eq:B_ineq}. Now we define the upper bound on $\phidn$ as:
% \begin{align}
%     \loneboundclas := \sqrt{ \frac{ n \fstar }{ \tnstar^2 } \left( 1 - \frac{2}{\tnstar^2} + \frac{c}{\tnstar^3} \right) }
% \end{align}
% which holds with probability at least $ 1 - 2 \exp \left( -c \frac{ n }{ \tnstar^6 \left( (\nubar)^2 + b_{\alpha_{\nstar}}^2  \norm{ \gamma \left( \alpha_{\nstar} \right) }_2^2 / \alpha_{\nstar}^2 \right) } \right) - 6 \exp \left( -\frac{\nstar}{\log^5(d/\nstar)} \right) $. The proposition is proved after noting that $ (\nubar)^2 + b_{\alpha_{\nstar}}^2  \norm{ \gamma \left( \alpha_{\nstar} \right) }_2^2 / \alpha_{\nstar}^2 = O(1)$.

% \subsection{Proof of Lemma~\ref{lemma_first_reduction}}
% According to lemma \ref{quadratic_bound_fn} we have that for any pair $ ( \nu, \eta ) $ with probability at least $ 1 - \exp \left( - n \kldiv{\frac{\sigma}{2}}{\frac{\sigma}{4}} \right) - \exp \left( -\frac{ n\sigma }{ 128 } \right) $ that $ \fnclas ( \nu, \eta) \geq \constnu \nu^2 + \consteta \eta^2 $ for some positive constants $\constnu$ and $\consteta $. Hence with high probability we can relax first constraint defining $\Gamma_0$ to
% \begin{align}
%     \frac{ \innerprod{\wtwo}{H}^2 }{ n } \geq \constnu \nu^2 + \consteta  \eta^2
% \end{align}
% Furthermore we can relax both constraints to define the following set:
% \begin{align}
%     \Gamma_1^{\eta} = \left\{ (\wone,\wtwo) \subjto \frac{ \innerprod{\wtwo}{H}^2 }{ n } \geq \consteta  \eta^2 \andtxts \norm{ \wtwo }_1 \leq \loneboundclas  \right\}
% \end{align}
% It is evident from definition that $ \Gamma_0 \subset \Gamma_1^{\eta}$ with high probability. Also note that constraints in the set $\Gamma_1^{\eta}$ depend only on $\wtwo$ and hence we will now consider only this variable. Now we bound $ \eta = \norm{ \wtwo }_2 $ as:
% \begin{align}
%     \eta^2 \leq \max_{\wtwo} \norm { \wtwo }_2 \subjto \wtwo \in \Gamma_1^{\eta}
% \end{align}

% We proceed following the path arguments established in \cite{wang2021tight}. We parametrize variable $\wtwo$ as $ \wtwo = b \norm { \gamma ( \alpha ) } $. 

% First we show that set $\Gamma_1^{\eta}$ is not empty. Let's choose $ \alpha = \alpha_{\nstar}$ with $\nstar = n\feestar/2$. Since we defined $ \loneboundclas $ in such way that $ \alpha_{\nstar} \in \Gamma_0 $ with high probability and we have $ \Gamma_0 \subset \Gamma_1^{\eta}$, this implies that with high probability there exists some $ b > 0 $ such that $ b \gamma ( \alpha ) \in \Gamma_1^{\eta} $.

% Using the same argument as in lemma 1 in \cite{wang2021tight} for $\phidp$ we can write:
% \begin{align}
%     \eta^2 \leq \max_{1\leq \alpha \leq \alpham} B^2 \frac{ \norm { \gamma ( \alpha ) }_2^2 }{ \norm { \gamma ( \alpha ) }_1^2 } \subjto B\gamma \left( \alpha \right) \in \Gamma_1^{\eta}
% \end{align}

% Now from lemma 4 in \cite{wang2021tight} we have that map $ \alpha \mapsto \frac{ \norm{ \gamma ( \alpha ) }_2^2 }{ \norm{ \gamma ( \alpha ) }_1^2 } $ is monotonically decreasing. Hence if we find value of $\alpha_{\uls}$ such that $\alpha_{\uls} \leq \alpha_{\nstar}$ and $ b \gamma ( \alpha_{\uls} ) \not \in \Gamma_1^{\eta}$ for any $ b > 0 $ then we have:
% \begin{align} \label{eq:eta_bound_first_reduction}
%     \eta^2 \leq  B^2 \frac{ \norm { \gamma ( \alphauls ) }_2^2 }{ \norm { \gamma ( \alphauls ) }_1^2 }
% \end{align}

% In order to saturate constraint $ \norm{ \wtwo }_1 \leq B $ let $ b = \frac{B}{\alphauls}$. Since we want that $  b \gamma ( \alpha_{\uls} ) \not \in \Gamma_1^{\eta} $ we will chose $s$ such that:
% \begin{align}
%     B^2 \frac{ \innerprod{ \gamma ( \alphauls )}{H}^2 }{ n \alphauls^2 } < \consteta B^2 \frac{ \norm{ \gamma ( \alphauls ) }_2^2 }{ \alphauls^2 }
% \end{align}
% Rewriting this inequality gives:
% \begin{align} \label{eq:s_condition_one}
%   \frac{ \norm{ \gamma ( \alphauls ) }_2^2 }{ \norm{H}_{\infty}^2 } > \frac{ 1 }{ \consteta n } 
% \end{align}
% Now we use concentration result from lemma \ref{lemma_gamma_conc} to get the following condition on $s$:
% \begin{align}
%     \frac{ 2 }{ \uls t_s^2 } \left( 1 - \frac{ c }{ \tuls^2 } \right) > \frac{ 1 }{ \consteta n }
% \end{align}

% We claim that $\uls = \lambda_{\uls} \frac{ n }{ \log (d/n) }$ satisfies this inequality for some positive constant $ \lambda_{\uls} $. From lemma 3 in \cite{wang2021tight} we know that if $ d/\uls \geq 11 $ we have that $ \log (d/\uls) \leq \tuls^2 \leq 2 \log (d/\uls) $. Using both of these bounds into expression \eqref{eq:s_condition_one} gives that:
% \begin{align}
%     \frac{ 2 }{ \uls \tuls^2 } \left( 1 - \frac{ c }{ \tuls^2 } \right) &> \frac{ 1 }{ 2 n \lambda_{\uls} } \frac{ \log (d/n) }{ \log (d/n) + \log \log (d/n) - \log \lambda_{\uls} } \left( 1 - \frac{c}{ \log (d/n) + \log \log (d/n) - \log \lambda_{\uls} } \right)
%     \\
%     & = \frac{ 1 }{ 2 n \lambda_{\uls} } \left( 1 - O \left( \frac{\log (d/n) }{\log \log (d/n) } \right) \right) > \frac{1}{\consteta n}
% \end{align}
% where last inequality holds for $d/n$ sufficiently large.

% Now from equation \eqref{eq:eta_bound_first_reduction} and concentration lemma \ref{lemma_gamma_conc} we have:
% \begin{align}
%     \eta^2 \leq \frac{ n \fstar }{ \tnstar^2 } \frac{2}{\uls}\left( 1 + \frac{c}{\tuls^2} \right) \leq \boundeta' \left( 1 + O \left( \frac{1}{ \log (d/n) } \right) \right) \leq \boundeta^2
% \end{align}

% Now we derive an upper bound for $\nu$. We consider the following set:
% \begin{align}
%     \Gamma_1^{\nu} = \left\{ (\wone,\wtwo) 
%     \subjto
%     \frac{ \innerprod{\wtwo}{H}^2 }{ n } \geq \constnu \nu^2 \andtxts \norm{ \wtwo }_1 \leq \loneboundclas \andtxts \norm{ \wtwo }_2 \leq \boundeta  \right\}
% \end{align}
% Once again it follows that $\Gamma_0 \subset \Gamma_1^{\nu}$. Hence we can upper bound $\nu$ as follows:
% \begin{align} \label{eq:nu_opt_first_reduction}
%     \nu^2 \leq \frac{ 1 }{ n \constnu } \max_{\wtwo} \innerprod{\wtwo}{H}^2
%     \subjto 
%     \norm{ \wtwo }_1 \leq \loneboundclas 
%     \andtxts 
%     \norm{ \wtwo }_2 \leq \boundeta
% \end{align}

% Now we show can this optimization problem can be rewritten in a form suitable for using parametrized path approach. Similarly as in \cite{wang2021tight} we define function $\olw : \left[ \frac{1}{d}, 1 \right] \to \RR^{d-1}$ as
% \begin{align}
%     \olw(\beta) = \argmax_{\wtwo} \innerprod{\wtwo}{\Hgaussian}
%     \subjto \begin{cases}
%                 \norm{\wtwo}_2^2 \leq \beta \\
%                 \wtwo\geq 0\\
%                 \norm{\wtwo}_1 = 1
%             \end{cases}
% \end{align}
% From claim 2 in \cite{wang2021tight} we know that for any $\beta \in \left[ \frac{1}{d}, 1 \right] $ there exists $ \alpha \in \left[ 1, \alpham \right] $ such that $ \olw (\beta) = \frac{ \gamma(\alpha) }{ \alpha }$. Following similar argument as in fourth statement of lemma 4 in \cite{wang2021tight} we have that $ \olw (\beta) $ is monotonically increasing function in $\beta$. 

% Setting $ \tildewtwo = \frac{ \wtwo }{ B }$ we can rewrite \eqref{eq:nu_opt_first_reduction} as:
% \begin{align} 
%     \nu^2 \leq \frac{ B^2 }{ n \constnu } \max_{\tildewtwo} \innerprod{ \tildewtwo }{ H }^2
%     \subjto 
%     \norm{ \tildewtwo }_1 \leq 1 
%     \andtxts 
%     \norm{ \tildewtwo }_2 \leq \frac{ \boundeta }{ B }
% \end{align}
% Hence solution of this problem must be of the form $ \tildewtwo = \olw (\beta) $ for some $\beta$. Similarly as in the first part of this proof, we first show that there exists $\beta_{\nstar}$ which satisfies constraints, and then find $\beta_{\ols}$ such that $ \beta_{\ols} \geq \beta_{\nstar}$. From monotonicity of $ \olw (\beta)$ follows that $ \olw (\beta_{\ols}) \geq \olw (\beta_{\nstar})$. Equivalently, we can find $\alpha_{\uls}$ such that $\alpha_{\uls} \leq \alpha_{\nstar}$.

% \begin{align}\label{nu_bound_first_reduction}
%     \nu^2 
%     \leq
%     \frac{ B^2 }{ n \constnu } \frac{ \innerprod{ \gamma (\alphauls) }{ H }^2 }{ \alphauls^2 } 
%     \leq 
%     \frac{ B^2 }{ n \constnu } \frac{ \norm{H}_{\infty}^2 }{ \alphauls^2 }
% \end{align}

% Let $\tildewtwo = \frac{ \gamma (\alpha) }{ \alpha }$. The claim that $\alpha_{\nstar}$ satisfies constraints is once again straightforward from our definition of $B$. Now we want to find $\alphauls$ such that:
% \begin{align}\label{s_condition_nu_first_reduction}
%     \norm{ \tildewtwo }_2^2 = \frac{ \norm{ \gamma ( \alphauls ) }_2^2 }{ \alphauls^2 } > \frac{ \boundeta^2 }{ B^2 }
% \end{align}
% Using concentration result from lemma \ref{lemma_gamma_conc} and expression \eqref{phidn_bound} we get the condition:
% \begin{align}
%     \frac{2}{\uls} \left( 1 - \frac{c}{\tuls^2} \right) > \frac{\boundeta^2 \tnstar^2}{ n \fstar }
% \end{align}
% Once again we claim that this equality is satisfied for $ \uls = \frac{ c n }{ \log (d/n) } $ for some positive constant $c$. It is easy to see that this is the same condition as in the previous part of the proof up to the constants and hence we can use the same proof here.

% From \eqref{nu_bound_first_reduction} we now have:
% \begin{align}
%     \nu^2 \leq \frac{ \fstar \tuls^2 }{ \constnu \tnstar^2 } \left( 1 - \frac{4}{\tuls^2} \right)^{-1} 
%     \leq c'_{\nu} \left( 1 + O \left( \frac{ \log \log (d/n) }{\log (d/n) } \right) \right) \leq \boundnu^2
% \end{align}
% concluding the proof.



% \subsection{Proof of Lemma~\ref{lemma_second_reduction}}


% From lemma \ref{lemma_first_reduction} we know that with high probability $ \nu \leq c_{\nu} $ and $ \eta \leq c_{\eta} $. Hence we can use uniform convergence of $\fnclas$ to its expectation (proposition \ref{prop:unifConv}). Hence we can relax constraints from definition of set $\Gamma_0$ as follows:
% \begin{align}
%     \frac{ \innerprod{\wtwo}{H}^2 }{ n } \geq f ( \nu, \eta ) - \constconc \geq  \fstar  + \tconstnu \deltanu^2 + \tconsteta \eta^2 - \constconc
% \end{align}
% where the second inequality follows from lemma \ref{lemma_quadratic_4lus_fstar_bound}. Hence we consider set:
% \begin{align}
%     \Gamma_2^{\eta} = \left\{ (\wone,\wtwo) \subjto \frac{ \innerprod{\wtwo}{H}^2 }{ n } \geq \fstar - \constconc +  \tconsteta \eta^2  \andtxts \norm{ \wtwo }_1 \leq \loneboundclas  \right\}
% \end{align}

% Following the same argument as in proof of lemma \ref{lemma_first_reduction} instead of inequality \eqref{eq:s_condition_one} we get:
% \begin{align}
%     \frac{ \left( \fstar - \constconc \right) \alpha_s^2 }{ B^2 \norm{H}_{\infty}^2 } + \tconsteta \frac{ \norm{ \gamma(\alpha_s) }_2^2 }{ \norm{H}_{\infty}^2 } > \frac{1}{n}
% \end{align}
% In order for inequality above to be satisfied we need:
% \begin{align}
%     \left( 1 - \frac{ \constconc }{ \fstar } \right) 
%     \frac{\tnstar^2}{t_s^2}
%     \left( 1 - \frac{4}{t_s^2} + O \left( \frac{1}{t_s^4} \right) \right) 
%     \left( 1 + \frac{2}{\tnstar^2} + O \left( \frac{1}{\tnstar^3} \right) \right) 
%     + \frac{2 n \tconsteta}{s t_s^2} \left( 1 + O \left( \frac{1}{t_s^2} \right) \right) 
%     > 1
% \end{align}
% Assuming that $ s = c \nstar$ and $ \constconc = O \left( \frac{1}{\tnstar^3} \right) $ we have:
% \begin{align}
%     \frac{\tnstar^2}{t_s^2}
%     \left( 1 + \frac{ \frac{4\tconsteta}{c\feestar}  - 4}{t_s^2} + \frac{2}{\tnstar^2} + O \left( \frac{1}{\tnstar^3}, \frac{1}{t_s^3} \right) \right)
%     > 1
% \end{align}
% Fix $\ulambda > 0$. Choose $\uls = \lambda_{\uls} \nstar$ such that $\uls < n$ is the largest integer for which $ \tuls^2 \geq \tnstar^2 + \ulambda $. Then we have condition:
% \begin{align}
%     \left( 1 - \frac{\ulambda}{\tuls^2} \right) \left( 1 + \frac{ \frac{4\tconsteta}{\lambda_{\uls}\feestar}  - 4}{\tuls^2} + \frac{2}{\tnstar^2} + O \left( \frac{1}{t_n^3} \right) \right)
%     > 1
% \end{align}
% For $\ulambda$ large enough inequality holds (Note: second brackets grow as $\lambda_{\uls}^{-1}$ and the first decays like $\log ( \lambda_{\uls} )$ - TO CHECK).

% Fix $\olambda > 0$. Now we choose $\ols = c_{\ols} \nstar$ such that $ \ols > n $ is the smallest integer for which $ t_{\ols}^2 \leq \tnstar^2 - \olambda $. Then we have:
% \begin{align}
%     \left( 1 + \frac{\olambda}{\tols^2} \right) \left( 1 + \frac{ \frac{4\tconsteta}{c_{\ols}\feestar}  - 4}{\tols^2} + \frac{2}{\tnstar^2} + O \left( \frac{1}{t_n^3} \right) \right)
%     > 1
% \end{align}
% We claim that there exists $\olambda$ large enough such that this inequality holds (e.g. $\ulambda > 4$).

% Hence we can bound $\eta^2$ as follows:
% \begin{align} \label{eq:eta_bound_first_reduction}
%     \eta^2 
%     \leq
%     B^2 \frac{ \norm { \gamma ( \alphauls ) }_2^2 }{ \norm { \gamma ( \alphauls ) }_1^2 } 
%     \leq
%     \frac{ n \left( \fstar - \constconc \right) }{ \tnstar^2 } \frac{2}{\uls}\left( 1 + \frac{c}{\tuls^2} \right) 
%     \leq
%     \frac{c_{\eta}'}{\log (d/n) } \left( 1 + O \left( \frac{1}{ \log (d/n) } \right) \right) 
%     \leq
%     \left( \frac{ B_{\eta,2} }{ \sqrt{\log (d/n)} } \right)^2
% \end{align}
% and similarly we get:
% \begin{align}
%     \eta^2 
%     \geq
%     B^2 \frac{ \norm { \gamma ( \alphaols ) }_2^2 }{ \norm { \gamma ( \alphaols ) }_1^2 } 
%     \geq
%     \left( \frac{ \overline{B}_{\eta,2} }{ \sqrt{\log (d/n)} } \right)^2
% \end{align}

% Following the proof of lemma \ref{lemma_first_reduction} we determine tighter upper bound for $\nu^2$.
% \begin{align}
%     \Gamma_2^{\nu} = \left\{ (\wone,\wtwo) 
%     \subjto
%     \frac{ \innerprod{\wtwo}{H}^2 }{ n } \geq \fstar - \constconc + \tconstnu \nu^2 \andtxts \norm{ \wtwo }_1 \leq \loneboundclas \andtxts \norm{ \wtwo }_2 \leq \frac{B_{\eta,2}}{\sqrt{ \log (d/n) }}  \right\}
% \end{align}

% Analogously to equation \eqref{s_condition_nu_first_reduction} we derive new condition for $\uls$ as:
% \begin{align}
%     \norm{ \tildewtwo }_2^2 = \frac{ \norm{ \gamma ( \alphauls ) }_2^2 }{ \alphauls^2 } > \frac{ B_{\eta,2}^2 }{ B^2 \log (d/n) }
% \end{align}
% which is again satisfied for some $\uls = \lambda_{\uls} n$ with $ \lambda_{\uls} > 0 $. Hence from \eqref{nu_bound_first_reduction} we obtain bound:
% \begin{align}
%     \deltanu^2 
%     \leq
%     \frac{ B^2 }{ n \tconstnu } \frac{ \norm{H}_{\infty}^2 }{ \alphauls^2 } - \frac{\fstar - \constconc }{\tconstnu}
%     \leq 
%     \frac{ \fstar }{ \tconstnu \tnstar^2 } \left( 1 + \frac{4}{\tuls^2} \right) - \frac{\fstar - \constconc }{\tconstnu}
%     \leq 
%     \left( \frac{ B_{\nu,2} }{ \sqrt{\log (d/n)} } \right)^2
% \end{align}
% which concludes the proof.















% \subsection{Proof of Lemma~}


% \begin{lemma}
%     There exist universal constant $B_{\nu,3} > 0, B_{\eta,3} > 0$ such that for any element $(\wone,\wtwo)$ of $\Gamma_0$ we have that $\deltanu^2 \leq \frac{B_{\nu,3}^2}{ \left( \log \left( d/n \right) \right)^{3/2} }$ and $ \eta^2 \leq \frac{B_{\eta,3}^2}{ \log \left( d/n \right) }$ with probability at least $ 1 - $ over the draws of $..$.
% \end{lemma}

% \begin{proof}
% In this part of the proof we use Taylor series approximation of function $f$:
% \begin{align}
%     f ( \nu, \eta ) = \fstar + \frac{1}{2}\feestar \eta^2 + \frac{1}{2}\fnstar \deltanu^2 + \underbrace{O \left( \frac{1}{ \log (d/n)^{3/2} } \right)}_{\OOOc}
% \end{align}
% where we bound higher terms by results from lemma \ref{lemma_second_reduction}.
% \end{proof}
% Now we proceed in the same manner as in the previous two steps. We relax constraint from definition of $\Gamma_0$ and define the following set:
% \begin{align}
%     \Gamma_3^{\eta} = \left\{ (\wone,\wtwo) \subjto \frac{ \innerprod{\wtwo}{H}^2 }{ n } \geq \fstar - \constconc - \OOOc + \frac{1}{2}\feestar \eta^2  \andtxts \norm{ \wtwo }_1 \leq \loneboundclas  \right\}
% \end{align}
% \begin{align}
%     \left( \fstar - \constconc - \OOOc \right) \frac{ \alpha_s^2 }{ \norm{H}_{\infty}^2 } \frac{ n }{ B^2 } + \frac{1}{2} \feestar n \frac{ \norm{ \gamma (\alpha_s) }_2^2 }{ \norm{H}_{\infty}^2 } > 1
% \end{align}
% \begin{lemma}
%     Let any fixed constant $ 0 < \lambda \leq ( \log (c_2) )^{1/4} $ where by assumption $d\geq n c_2$ and let $\uls$ be the largest integer $s$ such that $t_s^2 \geq \tnstar^2 + \frac{\lambda}{\sqrt{\tnstar}}$. Then
%     \begin{align}
%         \uls = \nstar \exp \left( -\frac{ \lambda }{ 2 \sqrt{\tnstar} } \right) \left( 1 + O \left( \frac{1}{\tnstar^2} \right) \right)
%         \andtxts
%         \left| \tuls^2 - \left( \tnstar^2 + \frac{\lambda}{\sqrt{\tnstar}} \right) \right| \leq O \left( \frac{1}{n} \right)
%     \end{align}
%     Moreover, let $\ols$ be the smallest integer $s$ such that $t_s^2 \leq \tnstar^2 - \frac{\lambda}{\sqrt{\tnstar}}$. Then
%     \begin{align}
%         \ols = \nstar \exp \left( \frac{ \lambda }{ 2 \sqrt{\tnstar} } \right) \left( 1 + O \left( \frac{1}{\tnstar^2} \right) \right)
%         \andtxts
%         \left| \tols^2 - \left( \tnstar^2 - \frac{\lambda}{\sqrt{\tnstar}} \right) \right| \leq O \left( \frac{1}{n} \right)
%     \end{align}
% \end{lemma}
% Proof follows the same steps as in Claim 7 in \cite{wang2021tight}. From these results follows:
% \begin{align}
%     \frac{\tnstar^2}{\tuls^2} 
%     =
%     \frac{1}{1 + \frac{\lambda}{\tnstar^2\sqrt{\tnstar}} + O \left( \frac{1}{\tnstar^2 \nstar} \right)}
%     =
%     1 - \frac{\lambda}{\tnstar^2\sqrt{\tnstar}} + O \left( \frac{1}{\tnstar^2 \nstar} \right) + O \left( \frac{\lambda^2}{\tnstar^5} \right)
% \end{align}
% Then for $ \constconc + \OOOc = O \left( \frac{1}{\tnstar^3} \right)$ we have
% \begin{align}
%     \left( \fstar -\constconc - \OOOc \right) \frac{ \alphauls^2 }{ \norm{H}_{\infty}^2 } \frac{ n }{ B^2 } \geq &
%     \fstar \left( 1 + O \left( \frac{1}{\tnstar^3} \right) \right) \frac{1}{\tuls^2}\left( 1 - \frac{4}{\tuls^2} + O \left( \frac{1}{\tuls^4} \right) \right)\frac{n \tnstar^2}{n\fstar} \left( 1 + \frac{2}{\tnstar^2} + O \left( \frac{1}{\tnstar^3} \right) \right)\\
%     \geq &
%     \left( 1 + O \left( \frac{1}{\tnstar^3} \right) \right) \left( 1 - \frac{\lambda}{\tnstar^2\sqrt{\tnstar}} + O \left( \frac{1}{\tnstar^2 \nstar} \right) + O \left( \frac{\lambda^2}{\tnstar^5} \right) \right) \left( 1 - \frac{2}{\tnstar^2} + O \left( \frac{1}{\tnstar^3} \right) \right)
% \end{align}
% \begin{align}
%     \frac{1}{2} \feestar n \frac{ \norm{ \gamma (\alphauls) }_2^2 }{ \norm{H}_{\infty}^2 } 
%     \geq &
%     \nstar \frac{2}{\uls \tuls^2} \left( 1 + O \left( \frac{1}{\tuls^2} \right) \right)\\
%     \geq &
%     \frac{2}{\tnstar^2} \exp \left( \frac{\lambda}{2\sqrt{\tnstar}} \right)  \left( 1 + O \left( \frac{1}{\tnstar^2} \right) \right) \\
%     \geq &
%     \frac{2}{\tnstar^2} \left( 1 + \frac{\lambda}{2\sqrt{\tnstar}} + \frac{\lambda^2}{4\tnstar} + O \left( \frac{\lambda^3}{\tnstar\sqrt{\tnstar}} \right) \right) \left( 1 + O \left( \frac{1}{\tnstar^2} \right) \right) 
% \end{align}
% Hence we have:
% \begin{align}
%     \left( \fstar - \constconc - \OOOc \right) \frac{ \alphauls^2 }{ \norm{H}_{\infty}^2 } \frac{ n }{ B^2 } + \frac{1}{2} \feestar n \frac{ \norm{ \gamma (\alphauls) }_2^2 }{ \norm{H}_{\infty}^2 } 
%     >
%     1 + \frac{\lambda^2}{2\tnstar^3} + O \left( \frac{1}{\tnstar^3} \right) + O (...)
% \end{align}

% Hence we can bound $\eta^2$ as follows:
% \begin{align} \label{eq:eta_bound_third_reduction}
%     \eta^2 
%     \leq
%     B^2 \frac{ \norm { \gamma ( \alphauls ) }_2^2 }{ \norm { \gamma ( \alphauls ) }_1^2 } 
%     & \leq
%     \frac{ n \fstar }{ \tnstar^2 } \frac{2}{\uls}\left( 1 + O\left( \frac{1}{\tnstar^2} \right) \right)
%     \leq
%     \frac{4\fstar}{\feestar} \frac{1}{\tnstar^2}  \exp \left( \frac{\lambda}{2\sqrt{\tnstar}} \right) \left( 1 + O\left( \frac{1}{\tnstar^2} \right) \right) \\
%     & \leq
%     \frac{4\fstar}{\feestar} \frac{1}{\tnstar^2} \left( 1 + \frac{\lambda}{2\sqrt{\tnstar}} + O \left( \frac{1}{\tnstar} \right) \right) =: B_{\eta,3}^2
% \end{align}
% and similarly we get:
% \begin{align}
%     \eta^2 
%     \geq
%     B^2 \frac{ \norm { \gamma ( \alphaols ) }_2^2 }{ \norm { \gamma ( \alphaols ) }_1^2 } 
%     \geq
%     \frac{4\fstar}{\feestar} \frac{1}{\tnstar^2} \left( 1 - \frac{\lambda}{2\sqrt{\tnstar}} + O \left( \frac{1}{\tnstar} \right) \right) 
% \end{align}
% Now let
% \begin{align}
%     \Gamma_3^{\nu} = \left\{ (\wone,\wtwo) 
%     \subjto
%     \frac{ \innerprod{\wtwo}{H}^2 }{ n } \geq \fstar - \constconc - \OOOc + \frac{1}{2}\feestar \eta^2 + \frac{1}{2}\fnstar \deltanu^2
%     \andtxts 
%     \norm{ \wtwo }_1 \leq \loneboundclas 
%     \andtxts
%     \norm{ \wtwo }_2 \leq B_{\eta,3}  \right\}
% \end{align}
% \begin{align}\label{s_condition_nu_third_reduction}
%     \norm{ \tildewtwo }_2^2 = B^2 \frac{ \norm{ \gamma ( \alphauls ) }_2^2 }{ \alphauls^2 } > B_{\eta,3}^2 
% \end{align}
% Using concentration result from lemma \ref{lemma_gamma_conc} and expression \eqref{phidn_bound} we get the condition:
% \begin{align}
%     \frac{2}{\uls} \left( 1 + O\left( \frac{1}{\tuls^2} \right) \right) 
%     >
%     \frac{4\fstar}{\feestar} \frac{1}{\tnstar^2} \left( 1 + \frac{\lambda}{2\sqrt{\tnstar}} + O \left( \frac{1}{\tnstar} \right) \right) \frac{\tnstar^2}{ n \fstar } \left( 1 + \frac{2}{\tnstar^2} + O \left( \frac{1}{\tnstar^3} \right) \right)
% \end{align}
% then
% \begin{align}
%     \frac{2}{\uls} \left( 1 + O \left( \frac{1}{\tuls^2} \right) \right) > \frac{4}{\feestar} \frac{1}{n} \left( 1 + \frac{\lambda}{2\sqrt{\tnstar}} + O \left( \frac{1}{\tnstar} \right) \right)
% \end{align}
% Hence let $\uls = \nstar \exp \left( -\frac{\lambda}{2\sqrt{\tnstar}} \right)$. %\frac{n\feestar}{2} \left( 1 - \frac{\lambda}{\sqrt{\tnstar}} + O \left( \frac{1}{\tnstar} \right) \right)$.  
% \begin{align}
%     \deltanu^2 
%     &\leq
%     \frac{ 2B^2 }{ n \fnstar } \frac{ \norm{H}_{\infty}^2 }{ \alphauls^2 } - \frac{2\fstar}{\fnstar} \left( 1 - \constconc - \OOOc \right) - \frac{\feestar}{\fnstar} \frac{ \norm{ \gamma(\alphaols) }_2^2 }{ \alphaols^2 }B^2\\
%     &\leq 
%     \frac{2}{n\fnstar} \frac{n\fstar}{\tnstar^2} \left(1-\frac{2}{\tnstar^2}+O \left( \frac{1}{\tnstar^3} \right) \right) \tuls^2 \left( 1 + \frac{4}{\tuls^2} + O \left( \frac{1}{\tuls^4} \right) \right)
%     - \frac{2\fstar}{\fnstar} \left( 1 + O \left( \frac{1}{\tnstar^3} \right) \right)
%     \\
%      & - \frac{\feestar}{\fnstar} \frac{2}{\nstar} \exp \left( -\frac{\lambda}{2\sqrt{\tnstar}} \right) \left( 1 + O \left( \frac{1}{\tnstar^2} \right) \right) \frac{n\fstar}{\tnstar^2}  \left( 1 - \frac{2}{\tnstar^2} + O \left( \frac{1}{\tnstar^3} \right) \right)
%      \\
%      &\leq \frac{2\fstar}{\fnstar} \left( 1 + \frac{2}{\tnstar^2} + \frac{\lambda}{\tnstar^{5/2}} + O \left( \frac{1}{\tnstar^3} \right) \right) 
%      - \frac{2\fstar}{\fnstar} \left( 1 + O \left( \frac{1}{\tnstar^3} \right) \right)
%      -\frac{2\fstar}{\fnstar}\left( \frac{2}{\tnstar^2} - \frac{\lambda}{\tnstar^{5/2}} + O \left( \frac{1}{\tnstar^3} \right) \right)
%      \\
%      & \leq \frac{4 \fstar \lambda}{\fnstar}\frac{1}{\tnstar^{5/2}} \left( 1 + O \left( \frac{1}{\sqrt{\tnstar}} \right) \right)
% \end{align}







==> sections_proof/3_bound_phiN.tex <==

% \subsection{Proof of Proposition~\ref{prop:Rbound}: $l_1$ bound}
% \label{apx:subsec:probRbound}





% Recall that $\phidn$ is given by:
% \begin{align}
%     \phidn &= \min_{\nu,b,\alpha} \nu + b \norm{ \gamma \left( \alpha \right) }_1 
%     \subjto \frac{ b^2\norm{\Hgaussian}_{\infty}^2 }{n} \geq \fn \left( \nu, b \norm{ \gamma \left( \alpha \right) }_2 \right)
% \end{align}

% Given that $(\tnu,\tb,\talpha)$ is a feasible point of $\phidn$ we have that $\phidn \leq  \tnu + \tb \norm{ \gamma( \talpha) }_1$, which gives us an upper bound on $\phidn$. In the following discussion our goal is to find a single feasible point of the constraint set of $\phidn$.

% From definition of $\gamma ( \alpha )$ we know that $ \norm{ \gamma ( \alpha ) }_1 = \alpha$ and hence we can equivalently formulate $\phidn$ as an optimization over $\nu$ and $ b_{\alpha} := b \alpha $
% \begin{align}
%     \phidn &= \min_{ \nu, b_{\alpha} } \nu + b_{\alpha}
%     \subjto \frac{ b_{\alpha}^2 \norm{\Hgaussian}_{\infty}^2 }{n \alpha^2} \geq \fn \left( \nu, b_{\alpha} \frac{ \norm{ \gamma \left( \alpha \right) }_2}{ \alpha } \right)
% \end{align}

% Define $\fstar = f \left( \nustar, 0 \right)$, $\feestar = \frac{\partial^2 f(\nuopt,\eta)}{\partial \eta^2}\Big|_{\eta=0}$ and $\nstar = \frac{1}{2}\feestar n$. Now using lemma \ref{lemma_point_conv} with $ t = \fstar \tnstar^{-3} $ and for a feasible point $( \nu, b_{\alpha} \frac{ \norm{ \gamma \left( \alpha \right) }_2}{ \alpha } )$ we have that:
% \begin{align} \label{eq:constraint_f_conc}
%     \frac{ b_{\alpha}^2 \norm{\Hgaussian}_{\infty}^2 }{n \alpha^2} 
%     \geq
%     f \left( \nu, b_{\alpha} \frac{ \norm{ \gamma \left( \alpha \right) }_2}{ \alpha } \right) + \frac{\fstar}{\tnstar^{3}}
% \end{align}
% with probability at least $ 1 - 2 \exp \left( -c \frac{ n }{ \tnstar^6 \left( \nu^2 + b_{\alpha}^2  \norm{ \gamma \left( \alpha \right) }_2^2 / \alpha^2 \right) } \right) $.
% % > 1 - 2 \exp \left( - \tc \frac{ n }{ \log^3 \left( \frac{d}{n} \right)  } \right) $.

% Let's now choose $ \nu = \nustar $ and show that there exist a pair $ ( b, \alpha )$  such that $ ( \nustar, b, \alpha) $ is feasible for constraint \eqref{eq:constraint_f_conc}. Furthermore, we propose to search for a point with parameter $ ( b, \alpha ) $ such that $ b \norm{ \gamma ( \alpha )}_2 = b_{\alpha} \frac{ \norm{ \gamma \left( \alpha \right) }_2}{ \alpha } $ is near zero. Hence, using Taylor series approximation of function $ f ( \nustar, \cdot ) : \eta \mapsto f (\nustar, \eta) $ around point $(\nuopt,0)$ we can rewrite constraint \eqref{eq:constraint_f_conc} as:
% \begin{align}
%      \frac{ b_{\alpha}^2 \norm{\Hgaussian}_{\infty}^2 }{n \alpha^2}   
%      \geq
%       \fstar + \frac{1}{2}\feestar b_{\alpha}^2 \frac{ \norm{ \gamma \left( \alpha \right) }_2^2}{ \alpha^2 } + \OOO \left( b_{\alpha}^3 \frac{ \norm{ \gamma \left( \alpha \right) }_2^3}{ \alpha^3 } \right) + \frac{\fstar}{\tnstar^{3}}
% \end{align}
% since $\feta = \frac{\partial f(\nuopt,\eta)}{\partial \eta}\Big|_{\eta=0} = 0$.

% Now from \cite{wang2021tight} we know that $ \gamma ( \alpha ) $ is a piecewise linear function with breakpoints at $ \alpha_s $ for $ s = 2, \dots, d $. Hence instead of optimizing over $\alpha$ we optimize over $s$. Note that we have only one constraint but two free variables $ ( b, \alpha ) $ and so we can set $ \alpha = \alpha_{\nstar} $ with $ \nstar = \frac{1}{2}\feestar n $. We explain this choice of $s$ in the remark after the proof. Combining all these results we get constraint:
% \begin{align} \label{eq:B_ineq}
%      \frac{ b_{\alpha_{\nstar}}^2 \norm{\Hgaussian}_{\infty}^2 }{n \alpha_{\nstar}^2}   
%      \geq
%       \fstar + \frac{1}{2}\feestar b_{\alpha_{\nstar}}^2 \frac{ \norm{ \gamma \left( \alpha_{\nstar} \right) }_2^2}{ \alpha_{\nstar}^2 } + \OOO \left( b_{\alpha_{\nstar}}^3 \frac{ \norm{ \gamma \left( \alpha_{\nstar} \right) }_2^3}{ \alpha_{\nstar}^3 } \right) + \frac{\fstar}{\tnstar^{3}}
% \end{align}

% Now we claim that
% \begin{equation}
%     b_{\alpha_{\nstar}}^2 = \frac{ n \alpha_{\nstar}^2 }{ \norm{\Hgaussian}_2^2 } \frac{ \fstar \left( 1 + \frac{1}{\tnstar^{3}} \right) }{ 1 - \frac{1}{2} n \feestar \frac{ \norm{ \gamma \left( \alpha_{\nstar} \right) }_2^2 }{ \norm{H}_{\infty}^2 } - \OOO \left( \frac{1}{\tnstar^3} \right) }
% \end{equation}
% satisfies inequality \eqref{eq:B_ineq} with probability at least $ 1 - 6 \exp \left( -\frac{\nstar}{\log(d/\nstar)^5} \right)$. Using lemma \ref{lemma_gamma_conc} we have that:
% \begin{equation}
%     1 - \frac{1}{2} n \feestar \frac{ \norm{ \gamma \left( \alpha_{\nstar} \right) }_2^2 }{ \norm{H}_{\infty}^2 } - \OOO \left( \frac{1}{\tnstar^3} \right) > 1 - \frac{1}{2} n \feestar  \frac{2}{\nstar \tnstar^2} - \OOO \left( \frac{1}{\tnstar^3} \right) = 1 - \frac{2}{\tnstar^2} - \OOO \left( \frac{1}{\tnstar^3} \right)  > 0
% \end{equation}
% holding for $d,n$ sufficiently large. Applying lemma \ref{lemma_gamma_conc} once again we get:
% \begin{equation}
%     b_{\alpha_{\nstar}}^2 
%     \leq
%     \frac{ n \fstar }{ \tnstar^2 } \left( 1 + \frac{1}{\tnstar^3} \right) \left( 1 - \frac{4}{\tnstar^2} + \frac{c}{\tnstar^4} \right) \frac{1}{ 1 - \frac{2}{\tnstar^2} - \OOO \left( \frac{1}{\tnstar^3} \right)}
%     \leq
%     \frac{ n \fstar }{ \tnstar^2 } \left( 1 - \frac{2}{\tnstar^2} + \frac{c}{\tnstar^3} \right)
% \end{equation}

% Hence we have that $ \OOO \left( b_{\alpha_{\nstar}}^3 \frac{ \norm{ \gamma \left( \alpha_{\nstar} \right) }_2^3}{ \alpha_{\nstar}^3 } \right) = \OOO \left( \frac{1}{\tnstar^3} \right)$ and this $b_{\alpha_{\nstar}}^2$ indeed satisfies equation \ref{eq:B_ineq}. Now we define the upper bound on $\phidn$ as:
% \begin{align}
%     \lonebound := \sqrt{ \frac{ n \fstar }{ \tnstar^2 } \left( 1 - \frac{2}{\tnstar^2} + \frac{c}{\tnstar^3} \right) }
% \end{align}
% which holds with probability at least $ 1 - 2 \exp \left( -c \frac{ n }{ \tnstar^6 \left( \nustar^2 + b_{\alpha_{\nstar}}^2  \norm{ \gamma \left( \alpha_{\nstar} \right) }_2^2 / \alpha_{\nstar}^2 \right) } \right) - 6 \exp \left( -\frac{\nstar}{\log(d/\nstar)^5} \right) $. The proposition is proved after noting that $ \nustar^2 + b_{\alpha_{\nstar}}^2  \norm{ \gamma \left( \alpha_{\nstar} \right) }_2^2 / \alpha_{\nstar}^2 = \OOO(1)$.


==> sections_proof/4_1st_reduction.tex <==
% \documentclass[appendix.tex]{subfiles}
% \begin{document}


% Recall that we defined $ \nu = \wone $ and $ \eta = \norm{ \wtwo }_1 $. Define the following set:
% \begin{align}
%     \Omega_0 = \left\{ (\wone,\wtwo) \subjto \frac{ \innerprod{\wtwo}{H}^2 }{ n } \geq \fn \left( \nu, \eta \right) \andtxts \abs{ \nu } + \norm{ \wtwo }_1 \leq \lonebound \right\}
% \end{align}

% \subsubsection{Step 1: Bounding $\nu,\eta$ by universal constants}
% \label{apx:subsec:firstReduction}

% \begin{lemma} \label{lemma_first_reduction}
%     There exist universal constant $c > 0$ such that for any element $(\wone,\wtwo)$ of $\Omega_0$ we have that $\norm{ \wone }_2 = \nu \leq \boundnu $ and $\norm{ \wtwo }_2 = \eta \leq \boundeta$ with probability at least $ 1 - $ over the draws of $..$.
% \end{lemma}

% \begin{proof}
% According to lemma \ref{quadratic_bound_fn} we have that for any pair $ ( \nu, \eta ) $ with probability at least $ 1 - \exp \left( - n \kldiv{\frac{\sigma}{2}}{\frac{\sigma}{4}} \right) - \exp \left( -\frac{ n\sigma }{ 128 } \right) $ that $ \fn ( \nu, \eta) \geq \constnu \nu^2 + \consteta \eta^2 $ for some positive constants $\constnu$ and $\consteta $. Hence with high probability we can relax first constraint defining $\Omega_0$ to
% \begin{align}
%     \frac{ \innerprod{\wtwo}{H}^2 }{ n } \geq \constnu \nu^2 + \consteta  \eta^2
% \end{align}
% Furthermore we can relax both constraints to define the following set:
% \begin{align}
%     \Omega_1^{\eta} = \left\{ (\wone,\wtwo) \subjto \frac{ \innerprod{\wtwo}{H}^2 }{ n } \geq \consteta  \eta^2 \andtxts \norm{ \wtwo }_1 \leq \lonebound  \right\}
% \end{align}
% It is evident from definition that $ \Omega_0 \subset \Omega_1^{\eta}$ with high probability. Also note that constraints in the set $\Omega_1^{\eta}$ depend only on $\wtwo$ and hence we will now consider only this variable. Now we bound $ \eta = \norm{ \wtwo }_2 $ as:
% \begin{align}
%     \eta^2 \leq \max_{\wtwo} \norm { \wtwo }_2 \subjto \wtwo \in \Omega_1^{\eta}
% \end{align}

% We proceed following the path arguments established in \cite{wang2021tight}. We parametrize variable $\wtwo$ as $ \wtwo = b \norm { \gamma ( \alpha ) } $. 

% First we show that set $\Omega_1^{\eta}$ is not empty. Let's choose $ \alpha = \alpha_{\nstar}$ with $\nstar = n\fetaeta/2$. Since we defined $ \lonebound $ in such way that $ \alpha_{\nstar} \in \Omega_0 $ with high probability and we have $ \Omega_0 \subset \Omega_1^{\eta}$, this implies that with high probability there exists some $ b > 0 $ such that $ b \gamma ( \alpha ) \in \Omega_1^{\eta} $.

% Using the same argument as in lemma 1 in \cite{wang2021tight} for $\phidp$ we can write:
% \begin{align}
%     \eta^2 \leq \max_{1\leq \alpha \leq \alpham} B^2 \frac{ \norm { \gamma ( \alpha ) }_2^2 }{ \norm { \gamma ( \alpha ) }_1^2 } \subjto B\gamma \left( \alpha \right) \in \Omega_1^{\eta}
% \end{align}

% Now from lemma 4 in \cite{wang2021tight} we have that map $ \alpha \mapsto \frac{ \norm{ \gamma ( \alpha ) }_2^2 }{ \norm{ \gamma ( \alpha ) }_1^2 } $ is monotonically decreasing. Hence if we find value of $\alpha_{\uls}$ such that $\alpha_{\uls} \leq \alpha_{\nstar}$ and $ b \gamma ( \alpha_{\uls} ) \not \in \Omega_1^{\eta}$ for any $ b > 0 $ then we have:
% \begin{align} \label{eq:eta_bound_first_reduction}
%     \eta^2 \leq  B^2 \frac{ \norm { \gamma ( \alphauls ) }_2^2 }{ \norm { \gamma ( \alphauls ) }_1^2 }
% \end{align}

% In order to saturate constraint $ \norm{ \wtwo }_1 \leq B $ let $ b = \frac{B}{\alphauls}$. Since we want that $  b \gamma ( \alpha_{\uls} ) \not \in \Omega_1^{\eta} $ we will chose $s$ such that:
% \begin{align}
%     B^2 \frac{ \innerprod{ \gamma ( \alphauls )}{H}^2 }{ n \alphauls^2 } < \consteta B^2 \frac{ \norm{ \gamma ( \alphauls ) }_2^2 }{ \alphauls^2 }
% \end{align}
% Rewriting this inequality gives:
% \begin{align} \label{eq:s_condition_one}
%   \frac{ \norm{ \gamma ( \alphauls ) }_2^2 }{ \norm{H}_{\infty}^2 } > \frac{ 1 }{ \consteta n } 
% \end{align}
% Now we use concentration result from lemma \ref{lemma_gamma_conc} to get the following condition on $s$:
% \begin{align}
%     \frac{ 2 }{ \uls t_s^2 } \left( 1 - \frac{ c }{ \tuls^2 } \right) > \frac{ 1 }{ \consteta n }
% \end{align}

% We claim that $\uls = c_{\uls} \frac{ n }{ \log (d/n) }$ satisfies this inequality for some positive constant $ c_{\uls} $. From lemma 3 in \cite{wang2021tight} we know that if $ d/\uls \geq 11 $ we have that $ \log (d/\uls) \leq \tuls^2 \leq 2 \log (d/\uls) $. Using both of these bounds into expression \eqref{eq:s_condition_one} gives that:
% \begin{align}
%     \frac{ 2 }{ \uls \tuls^2 } \left( 1 - \frac{ c }{ \tuls^2 } \right) &> \frac{ 1 }{ 2 n c_{\uls} } \frac{ \log (d/n) }{ \log (d/n) + \log \log (d/n) - \log c_{\uls} } \left( 1 - \frac{c}{ \log (d/n) + \log \log (d/n) - \log c_{\uls} } \right)
%     \\
%     & = \frac{ 1 }{ 2 n c_{\uls} } \left( 1 - \OOO \left( \frac{\log (d/n) }{\log \log (d/n) } \right) \right) > \frac{1}{\consteta n}
% \end{align}
% where last inequality holds for $d/n$ sufficiently large.

% Now from equation \eqref{eq:eta_bound_first_reduction} and concentration lemma \ref{lemma_gamma_conc} we have:
% \begin{align}
%     \eta^2 \leq \frac{ n \fstar }{ \tnstar^2 } \frac{2}{\uls}\left( 1 + \frac{c}{\tuls^2} \right) \leq \boundeta' \left( 1 + \OOO \left( \frac{1}{ \log (d/n) } \right) \right) \leq \boundeta^2
% \end{align}

% Now we derive an upper bound for $\nu$. We consider the following set:
% \begin{align}
%     \Omega_1^{\nu} = \left\{ (\wone,\wtwo) 
%     \subjto
%     \frac{ \innerprod{\wtwo}{H}^2 }{ n } \geq \constnu \nu^2 \andtxts \norm{ \wtwo }_1 \leq \lonebound \andtxts \norm{ \wtwo }_2 \leq \boundeta  \right\}
% \end{align}
% Once again it follows that $\Omega_0 \subset \Omega_1^{\nu}$. Hence we can upper bound $\nu$ as follows:
% \begin{align} \label{eq:nu_opt_first_reduction}
%     \nu^2 \leq \frac{ 1 }{ n \constnu } \max_{\wtwo} \innerprod{\wtwo}{H}^2
%     \subjto 
%     \norm{ \wtwo }_1 \leq \lonebound 
%     \andtxts 
%     \norm{ \wtwo }_2 \leq \boundeta
% \end{align}

% Now we show can this optimization problem can be rewritten in a form suitable for using parametrized path approach. Similarly as in \cite{wang2021tight} we define function $\olw : \left[ \frac{1}{d}, 1 \right] \to \RR^{d-1}$ as
% \begin{align}
%     \olw(\beta) = \argmax_{\wtwo} \innerprod{\wtwo}{\Hgaussian}
%     \subjto \begin{cases}
%                 \norm{\wtwo}_2^2 \leq \beta \\
%                 \wtwo\geq 0\\
%                 \norm{\wtwo}_1 = 1
%             \end{cases}
% \end{align}
% From claim 2 in \cite{wang2021tight} we know that for any $\beta \in \left[ \frac{1}{d}, 1 \right] $ there exists $ \alpha \in \left[ 1, \alpham \right] $ such that $ \olw (\beta) = \frac{ \gamma(\alpha) }{ \alpha }$. Following similar argument as in fourth statement of lemma 4 in \cite{wang2021tight} we have that $ \olw (\beta) $ is monotonically increasing function in $\beta$. 

% Setting $ \tildewtwo = \frac{ \wtwo }{ B }$ we can rewrite \eqref{eq:nu_opt_first_reduction} as:
% \begin{align} 
%     \nu^2 \leq \frac{ B^2 }{ n \constnu } \max_{\tildewtwo} \innerprod{ \tildewtwo }{ H }^2
%     \subjto 
%     \norm{ \tildewtwo }_1 \leq 1 
%     \andtxts 
%     \norm{ \tildewtwo }_2 \leq \frac{ \boundeta }{ B }
% \end{align}
% Hence solution of this problem must be of the form $ \tildewtwo = \olw (\beta) $ for some $\beta$. Similarly as in the first part of this proof, we first show that there exists $\beta_{\nstar}$ which satisfies constraints, and then find $\beta_{\ols}$ such that $ \beta_{\ols} \geq \beta_{\nstar}$. From monotonicity of $ \olw (\beta)$ follows that $ \olw (\beta_{\ols}) \geq \olw (\beta_{\nstar})$. Equivalently, we can find $\alpha_{\uls}$ such that $\alpha_{\uls} \leq \alpha_{\nstar}$.

% \begin{align}\label{nu_bound_first_reduction}
%     \nu^2 
%     \leq
%     \frac{ B^2 }{ n \constnu } \frac{ \innerprod{ \gamma (\alphauls) }{ H }^2 }{ \alphauls^2 } 
%     \leq 
%     \frac{ B^2 }{ n \constnu } \frac{ \norm{H}_{\infty}^2 }{ \alphauls^2 }
% \end{align}

% Let $\tildewtwo = \frac{ \gamma (\alpha) }{ \alpha }$. The claim that $\alpha_{\nstar}$ satisfies constraints is once again straightforward from our definition of $B$. Now we want to find $\alphauls$ such that:
% \begin{align}\label{s_condition_nu_first_reduction}
%     \norm{ \tildewtwo }_2^2 = \frac{ \norm{ \gamma ( \alphauls ) }_2^2 }{ \alphauls^2 } > \frac{ \boundeta^2 }{ B^2 }
% \end{align}
% Using concentration result from lemma \ref{lemma_gamma_conc} and expression \eqref{phidn_bound} we get condition:
% \begin{align}
%     \frac{2}{\uls} \left( 1 - \frac{c}{\tuls^2} \right) > \frac{\boundeta^2 \tnstar^2}{ n \fstar }
% \end{align}
% Once again we claim that this equality is satisfied for $ \uls = \frac{ c n }{ \log (d/n) } $ for some positive constant $c$. It is easy to see that this is the same condition as in the previous part of the proof up to the constants and hence we can use the same proof here.

% From \eqref{nu_bound_first_reduction} we now have:
% \begin{align}
%     \nu^2 \leq \frac{ \fstar \tuls^2 }{ \constnu \tnstar^2 } \left( 1 - \frac{4}{\tuls^2} \right)^{-1} 
%     \leq c'_{\nu} \left( 1 + \OOO \left( \frac{ \log \log (d/n) }{\log (d/n) } \right) \right) \leq \boundnu^2
% \end{align}
% concluding the proof.
% \end{proof}

% \end{document}

==> sections_proof/5_2nd_reduction.tex <==
% \documentclass[appendix.tex]{subfiles}
% \begin{document}

% \subsubsection{Step 2: Bounding $\deltanu,\eta$ by terms of the order $\frac{1}{\sqrt{\log (d/n)}}$}
% \label{apx:subsec:secondReduction}

% \begin{lemma} \label{lemma_second_reduction}
%     There exist universal constants $B_{\nu,2} > 0, B_{\eta,2} > 0$ such that for any element $(\wone,\wtwo)$ of $\Omega_0$ we have that $\deltanu^2 \leq \frac{B_{\nu,2}^2}{ \log \left( d/n \right) }$ and $ \eta^2 \leq \frac{B_{\eta,2}^2}{ \log \left( d/n \right) }$ with probability at least $ 1 - $ over the draws of $..$.
% \end{lemma}

% \begin{proof}



% From lemma \ref{lemma_first_reduction} we know that with high probability $ \nu \leq c_{\nu} $ and $ \eta \leq c_{\eta} $. Hence we can use uniform convergence of $f_n$ to its expectation (proposition \ref{prop:unifConv}). Hence we can relax constraints from definition of set $\Omega_0$ as follows:
% \begin{align}
%     \frac{ \innerprod{\wtwo}{H}^2 }{ n } \geq f ( \nu, \eta ) - \constconc \geq  \fstar  + \tconstnu \deltanu^2 + \tconsteta \eta^2 - \constconc
% \end{align}
% where the second inequality follows from lemma \ref{lemma_quadratic_plus_fstar_bound}. Hence we consider set:
% \begin{align}
%     \Omega_2^{\eta} = \left\{ (\wone,\wtwo) \subjto \frac{ \innerprod{\wtwo}{H}^2 }{ n } \geq \fstar - \constconc +  \tconsteta \eta^2  \andtxts \norm{ \wtwo }_1 \leq \lonebound  \right\}
% \end{align}

% Following the same argument as in proof of lemma \ref{lemma_first_reduction} instead of inequality \eqref{eq:s_condition_one} we get:
% \begin{align}
%     \frac{ \left( \fstar - \constconc \right) \alpha_s^2 }{ B^2 \norm{H}_{\infty}^2 } + \tconsteta \frac{ \norm{ \gamma(\alpha_s) }_2^2 }{ \norm{H}_{\infty}^2 } > \frac{1}{n}
% \end{align}
% In order for inequality above to be satisfied we need:
% \begin{align}
%     \left( 1 - \frac{ \constconc }{ \fstar } \right) 
%     \frac{\tnstar^2}{t_s^2}
%     \left( 1 - \frac{4}{t_s^2} + \OOO \left( \frac{1}{t_s^4} \right) \right) 
%     \left( 1 + \frac{2}{\tnstar^2} + \OOO \left( \frac{1}{\tnstar^3} \right) \right) 
%     + \frac{2 n \tconsteta}{s t_s^2} \left( 1 + \OOO \left( \frac{1}{t_s^2} \right) \right) 
%     > 1
% \end{align}
% Assuming that $ s = c \nstar$ and $ \constconc = \OOO \left( \frac{1}{\tnstar^3} \right) $ we have:
% \begin{align}
%     \frac{\tnstar^2}{t_s^2}
%     \left( 1 + \frac{ \frac{4\tconsteta}{c\feestar}  - 4}{t_s^2} + \frac{2}{\tnstar^2} + \OOO \left( \frac{1}{\tnstar^3}, \frac{1}{t_s^3} \right) \right)
%     > 1
% \end{align}
% Fix $\ulambda > 0$. Choose $\uls = c_{\uls} \nstar$ such that $\uls < n$ is the largest integer for which $ \tuls^2 \geq \tnstar^2 + \ulambda $. Then we have condition:
% \begin{align}
%     \left( 1 - \frac{\ulambda}{\tuls^2} \right) \left( 1 + \frac{ \frac{4\tconsteta}{c_{\uls}\feestar}  - 4}{\tuls^2} + \frac{2}{\tnstar^2} + \OOO \left( \frac{1}{t_n^3} \right) \right)
%     > 1
% \end{align}
% For $\ulambda$ large enough inequality holds (Note: second brackets grow as $c_{\uls}^{-1}$ and the first decays like $\log ( c_{\uls} )$ - TO CHECK).

% Fix $\olambda > 0$. Now we choose $\ols = c_{\ols} \nstar$ such that $ \ols > n $ is the smallest integer for which $ t_{\ols}^2 \leq \tnstar^2 - \olambda $. Then we have:
% \begin{align}
%     \left( 1 + \frac{\olambda}{\tols^2} \right) \left( 1 + \frac{ \frac{4\tconsteta}{c_{\ols}\feestar}  - 4}{\tols^2} + \frac{2}{\tnstar^2} + \OOO \left( \frac{1}{t_n^3} \right) \right)
%     > 1
% \end{align}
% We claim that there exists $\olambda$ large enough such that this inequality holds (e.g. $\ulambda > 4$).

% Hence we can bound $\eta^2$ as follows:
% \begin{align} \label{eq:eta_bound_first_reduction}
%     \eta^2 
%     \leq
%     B^2 \frac{ \norm { \gamma ( \alphauls ) }_2^2 }{ \norm { \gamma ( \alphauls ) }_1^2 } 
%     \leq
%     \frac{ n \left( \fstar - \constconc \right) }{ \tnstar^2 } \frac{2}{\uls}\left( 1 + \frac{c}{\tuls^2} \right) 
%     \leq
%     \frac{c_{\eta}'}{\log (d/n) } \left( 1 + \OOO \left( \frac{1}{ \log (d/n) } \right) \right) 
%     \leq
%     \left( \frac{ B_{\eta,2} }{ \sqrt{\log (d/n)} } \right)^2
% \end{align}
% and similarly we get:
% \begin{align}
%     \eta^2 
%     \geq
%     B^2 \frac{ \norm { \gamma ( \alphaols ) }_2^2 }{ \norm { \gamma ( \alphaols ) }_1^2 } 
%     \geq
%     \left( \frac{ \overline{B}_{\eta,2} }{ \sqrt{\log (d/n)} } \right)^2
% \end{align}

% Following the proof of lemma \ref{lemma_first_reduction} we determine tighter upper bound for $\nu^2$.
% \begin{align}
%     \Omega_2^{\nu} = \left\{ (\wone,\wtwo) 
%     \subjto
%     \frac{ \innerprod{\wtwo}{H}^2 }{ n } \geq \fstar - \constconc + \tconstnu \nu^2 \andtxts \norm{ \wtwo }_1 \leq \lonebound \andtxts \norm{ \wtwo }_2 \leq \frac{B_{\eta,2}}{\sqrt{ \log (d/n) }}  \right\}
% \end{align}

% Analogously to equation \eqref{s_condition_nu_first_reduction} we derive new condition for $\uls$ as:
% \begin{align}
%     \norm{ \tildewtwo }_2^2 = \frac{ \norm{ \gamma ( \alphauls ) }_2^2 }{ \alphauls^2 } > \frac{ B_{\eta,2}^2 }{ B^2 \log (d/n) }
% \end{align}
% which is again satisfied for some $\uls = c_{\uls} n$ with $ c_{\uls} > 0 $. Hence from \eqref{nu_bound_first_reduction} we obtain bound:
% \begin{align}
%     \deltanu^2 
%     \leq
%     \frac{ B^2 }{ n \tconstnu } \frac{ \norm{H}_{\infty}^2 }{ \alphauls^2 } - \frac{\fstar - \constconc }{\tconstnu}
%     \leq 
%     \frac{ \fstar }{ \tconstnu \tnstar^2 } \left( 1 + \frac{4}{\tuls^2} \right) - \frac{\fstar - \constconc }{\tconstnu}
%     \leq 
%     \left( \frac{ B_{\nu,2} }{ \sqrt{\log (d/n)} } \right)^2
% \end{align}
% which concludes the proof.
% \end{proof}

% \end{document}

==> sections_proof/8_Regression.tex <==





\red{this is for regressino, just adavpt}


We have $f_n(\nu,\eta) = \|\xi - Z\eta - G\nu\|_2^2 $. We use the following approximations for $f_n$:
\begin{itemize}
    \item $\frac{1}{n} f_n \geq \sigmaxi^2 - \rho \sigmaxi \vert \eta\vert - \rho \sigmaxi \vert \nu \vert + (1-\rho) (\nu^2 + \eta^2)$
        \item $\frac{1}{n} f_n \leq \sigmaxi^2 + \rho \sigmaxi \vert \eta\vert + \rho \sigmaxi \vert \nu \vert + (1+\rho) (\nu^2 + \eta^2)$
\end{itemize}
where $\rho = \frac{\log(2/\delta}{\sqrt{n}}$. We use these approximations throughout the proof. 
We begin with the bound for $\phidn$.


==> sections_proof/9_Technical_proofs_thm1.tex <==
\section{Auxiliary proofs for Theorem 1}

\subsection{Proof of Proposition~\ref{prop:Rbound}}
\label{sec:appendix_proof_bound_phidn}

Recall that $\phidn$ is given by:
\begin{align}
    \phidn &= \min_{\nu,b,\alpha} \nu + b \norm{ \gamma \left( \alpha \right) }_1 
    \subjto \frac{ b^2\norm{\Hgaussian}_{\infty}^2 }{n} \geq \fn \left( \nu, b \norm{ \gamma \left( \alpha \right) }_2 \right)
\end{align}

Given that $(\tnu,\tb,\talpha)$ is a feasible point of $\phidn$ we have that $\phidn \leq  \tnu + \tb \norm{ \gamma( \talpha) }_1$, which gives us an upper bound on $\phidn$. In the following discussion our goal is to find a single feasible point of the constraint set of $\phidn$.

From definition of $\gamma ( \alpha )$ we know that $ \norm{ \gamma ( \alpha ) }_1 = \alpha$ and hence we can equivalently formulate $\phidn$ as an optimization over $\nu$ and $ b_{\alpha} := b \alpha $
\begin{align}
    \phidn &= \min_{ \nu, b_{\alpha} } \nu + b_{\alpha}
    \subjto \frac{ b_{\alpha}^2 \norm{\Hgaussian}_{\infty}^2 }{n \alpha^2} \geq \fn \left( \nu, b_{\alpha} \frac{ \norm{ \gamma \left( \alpha \right) }_2}{ \alpha } \right)
\end{align}

Define $\fstar = f \left( \nustar, 0 \right)$, $\feestar = \frac{\partial^2 f(\nuopt,\eta)}{\partial \eta^2}\Big|_{\eta=0}$ and $\nstar = \frac{1}{2}\feestar n$. Now using lemma \ref{lemma_point_conv} with $ t = \fstar \tnstar^{-3} $ and for a feasible point $( \nu, b_{\alpha} \frac{ \norm{ \gamma \left( \alpha \right) }_2}{ \alpha } )$ we have that:
\begin{align} \label{eq:constraint_f_conc}
    \frac{ b_{\alpha}^2 \norm{\Hgaussian}_{\infty}^2 }{n \alpha^2} 
    \geq
    f \left( \nu, b_{\alpha} \frac{ \norm{ \gamma \left( \alpha \right) }_2}{ \alpha } \right) + \frac{\fstar}{\tnstar^{3}}
\end{align}
with probability at least $ 1 - 2 \exp \left( -c \frac{ n }{ \tnstar^6 \left( \nu^2 + b_{\alpha}^2  \norm{ \gamma \left( \alpha \right) }_2^2 / \alpha^2 \right) } \right) $.
% > 1 - 2 \exp \left( - \tc \frac{ n }{ \log^3 \left( \frac{d}{n} \right)  } \right) $.

Let's now choose $ \nu = \nustar $ and show that there exists a pair $ ( b, \alpha )$  such that $ ( \nustar, b, \alpha) $ is feasible for constraint \eqref{eq:constraint_f_conc}. Furthermore, we propose to search for a point with parameter $ ( b, \alpha ) $ such that $ b \norm{ \gamma ( \alpha )}_2 = b_{\alpha} \frac{ \norm{ \gamma \left( \alpha \right) }_2}{ \alpha } $ is near zero. Hence, using Taylor series approximation of function $ f ( \nustar, \cdot ) : \eta \mapsto f (\nustar, \eta) $ around point $(\nuopt,0)$ we can rewrite constraint \eqref{eq:constraint_f_conc} as:
\begin{align}
     \frac{ b_{\alpha}^2 \norm{\Hgaussian}_{\infty}^2 }{n \alpha^2}   
     \geq
      \fstar + \frac{1}{2}\feestar b_{\alpha}^2 \frac{ \norm{ \gamma \left( \alpha \right) }_2^2}{ \alpha^2 } + \OOO \left( b_{\alpha}^3 \frac{ \norm{ \gamma \left( \alpha \right) }_2^3}{ \alpha^3 } \right) + \frac{\fstar}{\tnstar^{3}}
\end{align}
since $\feta = \frac{\partial f(\nuopt,\eta)}{\partial \eta}\Big|_{\eta=0} = 0$.

As we mentioned in section \ref{step_1_thm3_proof}, $ \gamma ( \alpha ) $ is a piecewise linear function with breakpoints at $ \alpha_s $ for $ s = 2, \dots, d-1 $. Hence instead of optimizing over $\alpha$ we optimize over $s$. Note that we have only one constraint but two free variables $ ( b, \alpha ) $ and so we can set $ \alpha = \alpha_{\nstar} $ with $ \nstar = \frac{1}{2}\feestar n $. We explain this choice of $s$ in the remark after the proof. Combining all these results we get constraint:
\begin{align} \label{eq:B_ineq}
     \frac{ b_{\alpha_{\nstar}}^2 \norm{\Hgaussian}_{\infty}^2 }{n \alpha_{\nstar}^2}   
     \geq
      \fstar + \frac{1}{2}\feestar b_{\alpha_{\nstar}}^2 \frac{ \norm{ \gamma \left( \alpha_{\nstar} \right) }_2^2}{ \alpha_{\nstar}^2 } + \OOO \left( b_{\alpha_{\nstar}}^3 \frac{ \norm{ \gamma \left( \alpha_{\nstar} \right) }_2^3}{ \alpha_{\nstar}^3 } \right) + \frac{\fstar}{\tnstar^{3}}
\end{align}

Now we claim that
\begin{equation}
    b_{\alpha_{\nstar}}^2 = \frac{ n \alpha_{\nstar}^2 }{ \norm{\Hgaussian}_2^2 } \frac{ \fstar \left( 1 + \frac{1}{\tnstar^{3}} \right) }{ 1 - \frac{1}{2} n \feestar \frac{ \norm{ \gamma \left( \alpha_{\nstar} \right) }_2^2 }{ \norm{H}_{\infty}^2 } - \OOO \left( \frac{1}{\tnstar^3} \right) }
\end{equation}
satisfies inequality \eqref{eq:B_ineq} with probability at least $ 1 - 6 \exp \left( -\frac{\nstar}{\log(d/\nstar)^5} \right)$. Using lemma \ref{lemma_gamma_conc} we have that:
\begin{equation}
    1 - \frac{1}{2} n \feestar \frac{ \norm{ \gamma \left( \alpha_{\nstar} \right) }_2^2 }{ \norm{H}_{\infty}^2 } - \OOO \left( \frac{1}{\tnstar^3} \right) > 1 - \frac{1}{2} n \feestar  \frac{2}{\nstar \tnstar^2} - \OOO \left( \frac{1}{\tnstar^3} \right) = 1 - \frac{2}{\tnstar^2} - \OOO \left( \frac{1}{\tnstar^3} \right)  > 0
\end{equation}
holding for $d,n$ sufficiently large. Applying Lemma \ref{lemma_gamma_conc} once again we get:
\begin{equation}
    b_{\alpha_{\nstar}}^2 
    \leq
    \frac{ n \fstar }{ \tnstar^2 } \left( 1 + \frac{1}{\tnstar^3} \right) \left( 1 - \frac{4}{\tnstar^2} + \frac{c}{\tnstar^4} \right) \frac{1}{ 1 - \frac{2}{\tnstar^2} - \OOO \left( \frac{1}{\tnstar^3} \right)}
    \leq
    \frac{ n \fstar }{ \tnstar^2 } \left( 1 - \frac{2}{\tnstar^2} + \frac{c}{\tnstar^3} \right)
\end{equation}

Hence we have that $ \OOO \left( b_{\alpha_{\nstar}}^3 \frac{ \norm{ \gamma \left( \alpha_{\nstar} \right) }_2^3}{ \alpha_{\nstar}^3 } \right) = \OOO \left( \frac{1}{\tnstar^3} \right)$ and this $b_{\alpha_{\nstar}}^2$ indeed satisfies equation \eqref{eq:B_ineq}. Now we define the upper bound on $\phidn$ as:
\begin{align}
\label{eq:lonebound_def}
    \lonebound := \sqrt{ \frac{ n \fstar }{ \tnstar^2 } \left( 1 - \frac{2}{\tnstar^2} + \frac{c}{\tnstar^3} \right) }
\end{align}
which holds with probability at least $ 1 - 2 \exp \left( -c \frac{ n }{ \tnstar^6 \left( \nustar^2 + b_{\alpha_{\nstar}}^2  \norm{ \gamma \left( \alpha_{\nstar} \right) }_2^2 / \alpha_{\nstar}^2 \right) } \right) - 6 \exp \left( -\frac{\nstar}{\log(d/\nstar)^5} \right) $. The proposition is proved after noting that $ \nustar^2 + b_{\alpha_{\nstar}}^2  \norm{ \gamma \left( \alpha_{\nstar} \right) }_2^2 / \alpha_{\nstar}^2 = \OOO(1)$.









\subsection{Proof of Lemma~\ref{lemma_first_reduction}}
According to Lemma \ref{quadratic_bound_fn} we have that for any pair $ ( \nu, \eta ) $ with probability at least $ 1 - \exp \left( - n \kldiv{\frac{\sigma}{2}}{\frac{\sigma}{4}} \right) - \exp \left( -\frac{ n\sigma }{ 128 } \right) $ that $ \fn ( \nu, \eta) \geq \constnu \nu^2 + \consteta \eta^2 $ for some positive constants $\constnu$ and $\consteta $. Hence with high probability we can relax first constraint defining $\Gamma_0$ to
% \begin{align}
%     \frac{ \innerprod{\wtwo}{H}^2 }{ n } \geq \constnu \nu^2 + \consteta  \eta^2
% \end{align}
\begin{align}
    \frac{1}{n} b^2 \norm{H}_{\infty}^2 \geq \constnu \nu^2 + \consteta b^2 \norm{\gamma(\alpha)}_2^2    
\end{align}

Let's first consider bounding of $\eta$ and then we use obtained result to bound $\nu$.
\paragraph{Upper bound on $\eta$.}
For this part of the proof we further relax both constraints from definition \eqref{eq:Omega_0_def} of $\Gamma_0$ and define the following set:
\begin{align}
    \Gamma_1^{\eta} = \left\{ (\nu, b, \alpha) \subjto \frac{1}{n} b^2 \norm{H}_{\infty}^2 \geq \consteta  b^2 \norm{\gamma(\alpha)}_2^2 \andtxts b \alpha \leq \lonebound  \right\}
\end{align}
% \begin{align}
%     \Gamma_1^{\eta} = \left\{ (\wone,\wtwo) \subjto \frac{ \innerprod{\wtwo}{H}^2 }{ n } \geq \consteta  \eta^2 \andtxts \norm{ \wtwo }_1 \leq \lonebound  \right\}
% \end{align}
It is evident from definition that $ \Gamma_0 \subset \Gamma_1^{\eta}$ with high probability. Also note that constraints in the set $\Gamma_1^{\eta}$ do not depend on $\nu$ and hence we will now consider only variables $b$ and $\alpha$. Now we bound $ \eta $ as:
\begin{align}
    \eta^2 \leq \max_{b,\alpha} b^2 \norm{\gamma(\alpha)}_2^2 \subjto (b,\alpha) \in \Gamma_1^{\eta}
\end{align}

We proceed following the path arguments established in \cite{wang2021tight}. First we show that set $\Gamma_1^{\eta}$ is not empty. Let's choose $ \alpha = \alpha_{\nstar}$ with $\nstar = n\fetaeta/2$. Recall that we defined $ \lonebound $ in such way that $ (b,\alpha_{\nstar}) \in \Gamma_0 $ with high probability for $b \alpha_{\nstar}\leq \lonebound$. As $ \Gamma_0 \subset \Gamma_1^{\eta}$, with high probability there exists some $ b > 0 $ such that $ (b, \alpha_{\nstar} ) \in \Gamma_1^{\eta} $ proving that $\Gamma_1^{\eta} \neq \emptyset$.

Recall from definition \eqref{eq:def_gamma_alpha} that $\norm{\gamma(\alpha)}_1 = \alpha$. Then using the same arguments as in Lemma 1 in \cite{wang2021tight}, we set $ b = \frac{\lonebound}{\alpha} $ and obtain:
\begin{align}
\label{eq:step_one_eta_bound_alpha}
    \eta^2 
    \leq
    \max_{1\leq \alpha \leq \alpham} \lonebound^2 \frac{ \norm { \gamma ( \alpha ) }_2^2 }{ \norm { \gamma ( \alpha ) }_1^2 } 
    \subjto
    %B\gamma \left( \alpha \right) \in \Gamma_1^{\eta}
    \left( \frac{\lonebound}{\alpha}, \alpha \right) \in \Gamma_1^{\eta}
\end{align}

As mentioned in section \ref{step_1_thm3_proof} the map $ \alpha \mapsto \frac{ \norm{ \gamma ( \alpha ) }_2^2 }{ \norm{ \gamma ( \alpha ) }_1^2 } $ is monotonically decreasing and the mapping $ \alpha \mapsto \consteta b^2 \norm{\gamma(\alpha)}_2^2 $ is convex. The interval of $\alpha \in [1,\alpham]$ for which constraint in equation \eqref{eq:step_one_eta_bound_alpha} holds is an interval since it is as a sublevel set of a convex function. Therefore if we find value of $\alpha_{\uls}$ such that $\alphauls \leq \alpha_{\nstar}$ and $ ( \frac{M}{\alphauls}, \alphauls ) \not \in \Gamma_1^{\eta}$, then we have:
\begin{align} \label{eq:eta_bound_first_reduction}
    \eta^2 \leq  \lonebound^2 \frac{ \norm { \gamma ( \alphauls ) }_2^2 }{ \norm { \gamma ( \alphauls ) }_1^2 }
\end{align}

% In order to saturate constraint $ \norm{ \wtwo }_1 \leq \lonebound $ let $ b = \frac{\lonebound}{\alphauls}$. 
In order to have $ ( \frac{M}{\alphauls}, \alphauls ) \not \in \Gamma_1^{\eta}$ we will chose $\uls$ as the smallest integer for which first constraint in definition of $\Gamma_1^{\eta}$ is not satisfied, i.e. choose  $\uls$ satisfying
% \begin{align}
%     \lonebound^2 \frac{ \innerprod{ \gamma ( \alphauls )}{H}^2 }{ n \alphauls^2 } < \consteta \lonebound^2 \frac{ \norm{ \gamma ( \alphauls ) }_2^2 }{ \alphauls^2 }
% \end{align}
\begin{align}
\label{eq:s_condition_one}
    \frac{1}{n} \frac{\lonebound^2}{\alphauls^2} \norm{H}_{\infty}^2 
    <
    \consteta \frac{\lonebound^2}{\alphauls^2} \norm{ \gamma ( \alphauls ) }_2^2 
\end{align}
% Rewriting this inequality gives:
% \begin{align} \label{eq:s_condition_one}
%   \frac{ \norm{ \gamma ( \alphauls ) }_2^2 }{ \norm{H}_{\infty}^2 } > \frac{ 1 }{ \consteta n } 
% \end{align}
After rewriting and using concentration result from Proposition \ref{lemma_gamma_conc} we obtain the following condition on $\uls$:
\begin{align}
    \frac{ 2 }{ \uls \tuls^2 } \left( 1 - \OOO \left( \frac{ 1 }{ \tuls^2 } \right) \right) > \frac{ 1 }{ \consteta n }
\end{align}

 We claim that $\uls =\lambda_{\uls} \frac{ n }{ \log (d/n) }$ satisfies this inequality for some positive universal constant $ \lambda_{\uls} >0  $. Using characterization $t_s = 2\log (d/s) + \OOO (\log \log (d\s) ) $ from section \ref{step_1_thm3_proof} we get:
\begin{align}
    \frac{ 2 }{ \uls \tuls^2 } \left( 1 - \OOO \left( \frac{ 1 }{ \tuls^2 } \right) \right) 
    & >
    % \frac{ 2\log (d/n)  }{ n \lambda_{\uls} } \frac{ 1 }{ 2\log (d/\uls) + \OOO \left(\log \log (d/\uls) \right) } \left( 1 - \OOO \left( \frac{1}{\log (d/n)} \right) \right)
    % \\
    % & = 
    \frac{ 1 }{ n \lambda_{\uls} } \left( 1 - \OOO \left( \frac{\log\log (d/n) }{\log (d/n) } \right) \right) > \frac{1}{\consteta n}
\end{align}
where last inequality holds for $d/n$ sufficiently large and $\lambda_{\uls}$ small enough.

Now from equation \eqref{eq:eta_bound_first_reduction} and concentration Proposition \ref{lemma_gamma_conc}, for some positive constant $B_{\eta,1}$ we get:
\begin{align}
    \eta^2 \leq \frac{ n \fstar }{ \tnstar^2 } \frac{2}{\uls}\left( 1 + \OOO \left( \frac{1}{\tuls^2} \right) \right) %\leq \boundeta' \left( 1 + \OOO \left( \frac{1}{ \log (d/n) } \right) \right) 
    =: B_{\eta,1}^2
\end{align}
since for the chosen $\uls$ the term on the right hand side of inequality is of the order $\OOO (1)$.


\paragraph{Upper bound on $\nu$.} Now we derive an upper bound for $\nu$. We consider the following set:
\begin{align}
    \Gamma_1^{\nu} = \left\{ (\nu, b, \alpha) 
    \subjto
    \frac{1}{n} \innerprod{b\gamma(\alpha)}{H}^2 \geq \constnu \nu^2 \andtxts b\alpha \leq \lonebound \andtxts b\norm{\gamma(\alpha)}_2 \leq B_{\eta,1} \right\}
    %\frac{ \innerprod{\wtwo}{H}^2 }{ n } \geq \constnu \norm{\wone}_2^2 \andtxts \norm{ \wtwo }_1 \leq \lonebound \andtxts \norm{ \wtwo }_2 \leq \boundeta  \right\}
\end{align}
% \begin{align}
%     \Gamma_1^{\nu} = \left\{ (\wone,\wtwo) 
%     \subjto
%     \frac{ \innerprod{\wtwo}{H}^2 }{ n } \geq \constnu \nu^2 \andtxts \norm{ \wtwo }_1 \leq \lonebound \andtxts \norm{ \wtwo }_2 \leq \boundeta  \right\}
% \end{align}
As we noted in Section \ref{step_1_thm3_proof}, from Claim 3 in \cite{wang2021tight} follows that $\innerprod{\gamma(\alpha)}{H} = \norm{H}_{\infty}$ and we obtain that $\Gamma_0 \subset \Gamma_1^{\nu}$ with high probability. Hence we can upper bound $\nu$ as follows:
\begin{align} \label{eq:nu_opt_first_reduction}
    \nu^2 \leq \frac{ 1 }{ n \constnu } \max_{b,\alpha} b^2 \innerprod{\frac{\gamma(\alpha)}{\alpha}}{H}^2
    \subjto 
    b \leq \lonebound 
    \andtxts 
    b\norm{ \frac{\gamma(\alpha) }{\alpha} }_2 \leq B_{\eta,1}
\end{align}

First note that choosing $b=M$ maximizes the objective if the second constraint is satisfied as well. Now we show how this optimization problem can be rewritten in a more suitable form for solving via parametrized path approach. Similarly as in \cite{wang2021tight} we define function $\olw : \left[ \frac{1}{d}, 1 \right] \to \RR^{d-1}$ as
\begin{align}
    \olw(\beta) = \argmax_{\wtwo} \innerprod{\wtwo}{\Hgaussian}
    \subjto \begin{cases}
                \norm{\wtwo}_2^2 \leq \beta \\
                \wtwo\geq 0\\
                \norm{\wtwo}_1 = 1
            \end{cases}
\end{align}
From Claim 2 in \cite{wang2021tight} we know that for any $\beta \in \left[ \frac{1}{d}, 1 \right] $ there exists $ \alpha \in \left[ 1, \alpham \right] $ such that $ \olw (\beta) = \frac{ \gamma(\alpha) }{ \alpha }$. Following similar argument as in Lemma 4 in \cite{wang2021tight} we have that $ \olw (\beta) $ is monotonically increasing function in $\beta$. Hence we can rewrite \eqref{eq:nu_opt_first_reduction} as:
\begin{align} 
\label{eq:first_iteration_nu_gamma_beta}
    \nu^2 \leq \frac{ \lonebound^2 }{ n \constnu } \max_{\beta} \innerprod{ \olw(\beta) }{ H }^2
    \subjto 
    \norm{ \olw(\beta) }_2 \leq \frac{ B_{\eta,1} }{ \lonebound }
\end{align}

Similarly as in the first part of this proof, we first show that there exists $\beta_{\nstar}$ which satisfies constraints, and then find smallest $\beta_{\ols}$ which does not satisfy constraints in \eqref{eq:first_iteration_nu_gamma_beta} and such that $ \beta_{\ols} \geq \beta_{\nstar}$. From monotonicity of $ \olw (\beta)$ follows that $ \olw (\beta_{\ols}) \geq \olw (\beta_{\nstar})$. Since the constraints in \eqref{eq:first_iteration_nu_gamma_beta} are convex in $\olw(\beta)$, the expression is maximized for $\beta = \beta_{\ols}$.

Since $\alpha = \alpha_{\nstar}$ satisfies constraints in \eqref{eq:nu_opt_first_reduction} by definition of $M$, we define $\beta_{\nstar}$ such that $\gamma(\beta_{\nstar}) = \frac{\gamma(\alpha_{\nstar})}{\alpha_{\nstar}}$ and hence $\beta_{\nstar}$ satisfies constraints in \eqref{eq:first_iteration_nu_gamma_beta}. Furthermore, if we find $\alpha_{\uls}$ such that $\alpha_{\uls} \leq \alpha_{\nstar}$ and
\begin{align}\label{s_condition_nu_first_reduction}
    \frac{ \norm{ \gamma ( \alphauls ) }_2 }{ \alphauls } 
    >
    \frac{ B_{\eta,1} }{ \lonebound }
\end{align}
we automatically obtain $\beta_{\uls}$ such that $\gamma(\beta_{\uls}) = \frac{\gamma(\alpha_{\uls})}{\alpha_{\uls}}$ which does not satisfy constraint in \eqref{eq:first_iteration_nu_gamma_beta}. 
Now from \eqref{s_condition_nu_first_reduction} and using concentration result from Proposition \ref{lemma_gamma_conc} and expression \eqref{phidn_bound} we obtain condition:
\begin{align}
    \frac{2}{\uls} \left( 1 - \OOO \left( \frac{1}{\tuls^2} \right) \right)
    >
    \frac{B_{\eta,1}^2 \tnstar^2}{ n \fstar } \left( 1 + \OOO \left( \frac{1}{\tnstar^2} \right) \right)
\end{align}
Once again we claim that this equality is satisfied for $ \uls = \lambda_{\uls} \frac{ n }{ \log (d/n) } $ for some positive constant $\lambda_{\uls}$. The proof follows use the same reasoning as in the previous part of the proof.

Hence we can bound $\nu$ from expression \eqref{eq:nu_opt_first_reduction} as follows:
\begin{align}\label{nu_bound_first_reduction}
    \nu^2 
    \leq
    \frac{ \lonebound^2 }{ n \constnu } \frac{ \innerprod{ \gamma (\alphauls) }{ H }^2 }{ \alphauls^2 }
    =
    \frac{ \lonebound^2 }{ n \constnu } \frac{ \norm{H}_{\infty}^2 }{ \alphauls^2 }
\end{align}
with the equality holding for $\gamma(\alpha)$ as discussed in Section \ref{step_1_thm3_proof}. Using concentration results from Proposition \ref{lemma_gamma_conc} we conclude that there exists a positive constant $B_{\nu,1}$ such that:
\begin{align}
    \nu^2 \leq \frac{ \fstar \tuls^2 }{ \constnu \tnstar^2 } \left( 1 + \OOO \left( \frac{1}{\tuls^2} \right) \right)
    % \leq c'_{\nu} \left( 1 + \OOO \left( \frac{ \log \log (d/n) }{\log (d/n) } \right) \right) \leq
    =: B_{\nu,1}^2
\end{align}
since the term on the right hand side is of the order $\OOO(1)$ for chosen $\uls$. This concludes the proof of the lemma.











\subsection{Proof of Lemma~\ref{lemma_second_reduction}}

From Lemma \ref{lemma_first_reduction} we know that with high probability $ \nu \leq B_{\nu,1} $ and $ \eta \leq B_{\eta,1} $. Hence we can use uniform convergence of $f_n$ to its expectation (Proposition \ref{prop:unifConv}) and relax constraint from definition of set $\Gamma_0$ as follows:
\begin{align}
\label{eq:second_iteration_relaxed_constraint_f}
    \frac{1}{n} b^2 \norm{H}_{\infty}^2 \geq f_n (\nu, b\norm{\gamma(\alpha)}_2) \geq f ( \nu, b\norm{\gamma(\alpha)}_2 ) - \constconc \geq  \fstar  + \tconstnu \deltanu^2 + \tconsteta b^2\norm{\gamma(\alpha)}_2^2 - \constconc
\end{align}
Again we first consider bounding of $\eta$ and then use obtained result for bounding of $\deltanu = \nu -\nustar$.

\paragraph{Upper bound on $\eta$.} 
We consider the set:
\begin{align}
    \Gamma_2^{\eta} = \left\{ (\nu, b, \alpha) 
    \subjto 
    \frac{ 1 }{ n } b^2 \norm{H}_{\infty}^2 \geq \fstar +  \tconsteta b^2 \norm{\gamma(\alpha)}_2^2 - \constconc
    \andtxts
    b\alpha \leq \lonebound
    \right\}
\end{align}
% \begin{align}
%     \Gamma_2^{\eta} = \left\{ (\wone,\wtwo) \subjto \frac{ \innerprod{\wtwo}{H}^2 }{ n } \geq \fstar - \constconc +  \tconsteta \norm{\wtwo}_2^2  \andtxts \norm{ \wtwo }_1 \leq \lonebound  \right\}
% \end{align}
% \begin{align}
%     \Gamma_2^{\eta} = \left\{ (\wone,\wtwo) \subjto \frac{ \innerprod{\wtwo}{H}^2 }{ n } \geq \fstar - \constconc +  \tconsteta \eta^2  \andtxts \norm{ \wtwo }_1 \leq \lonebound  \right\}
% \end{align}
Now we can use the same arguments as in proof of Lemma \ref{lemma_first_reduction} since adding a constant term to the constraint essentially does not change the problem. Instead of inequality \eqref{eq:s_condition_one} we get condition:
\begin{align}
    \left( \fstar - \constconc \right) \frac{ n \alphauls^2 }{  \lonebound^2 \norm{H}_{\infty}^2 } + \tconsteta n \frac{ \norm{ \gamma(\alphauls) }_2^2 }{ \norm{H}_{\infty}^2 } > 1
\end{align}
% In order for inequality above to be satisfied we need:
% \begin{align}
%     \left( 1 - \frac{ \constconc }{ \fstar } \right) 
%     \frac{\tnstar^2}{t_s^2}
%     \left( 1 - \frac{4}{t_s^2} + \OOO \left( \frac{1}{\tnstar^3} \right) \right) 
%     \left( 1 + \frac{2}{\tnstar^2} + \OOO \left( \frac{1}{\tnstar^3} \right) \right) 
%     + \frac{2 n \tconsteta}{s t_s^2} \left( 1 + \OOO \left( \frac{1}{t_s^2} \right) \right) 
%     > 1
% \end{align}
Assuming that $ \uls = \lambda_{\uls} \nstar$ and $ \constconc = \OOO \left( \frac{1}{\tnstar^3} \right) $ and using Propositions \ref{prop:concentrationl1} and \ref{prop:Rbound} we get condition:
\begin{align}
    1 + \frac{1}{\tnstar^2} \left( \frac{2\tconsteta}{\lambda} - 2 \right) + \OOO \left( \frac{1}{\tnstar^3} \right) > 1
\end{align}
which holds for $\lambda_{\uls}$ sufficiently small.

% \begin{align}
%     \frac{\tnstar^2}{t_s^2}
%     \left( 1 + \frac{ \frac{4\tconsteta}{\lambda\feestar}  - 4}{t_s^2} + \frac{2}{\tnstar^2} + \OOO \left( \frac{1}{\tnstar^3}, \frac{1}{t_s^3} \right) \right)
%     > 1
% \end{align}
% Fix $\ulambda > 0$. Choose $\uls = \lambda_{\uls} \nstar$ such that $\uls < n$ is the largest integer for which $ \tuls^2 \geq \tnstar^2 + \ulambda $. Then we have condition:
% \begin{align}
%     \left( 1 - \frac{\ulambda}{\tuls^2} \right) \left( 1 + \frac{ \frac{4\tconsteta}{\lambda_{\uls}\feestar}  - 4}{\tuls^2} + \frac{2}{\tnstar^2} + \OOO \left( \frac{1}{t_n^3} \right) \right)
%     > 1
% \end{align}
% For $\ulambda$ large enough inequality holds (Note: second brackets grow as $\lambda_{\uls}^{-1}$ and the first decays like $\log ( \lambda_{\uls} )$ - TO CHECK).


% \red{okay I messed this up - sorry. Can you make the following section a bit clearer? In particular, the connection to tn and s is not clear, cite the result form our paper. . So here we need to say that essentially we obtain the same problem as studied in my paper.}

% Fix $\olambda > 0$. Now we choose $\ols = c_{\ols} \nstar$ such that $ \ols > n $ is the smallest integer for which $ t_{\ols}^2 \leq \tnstar^2 - \olambda $. Then we have:
% \begin{align}
%     \left( 1 + \frac{\olambda}{\tols^2} \right) \left( 1 + \frac{ \frac{4\tconsteta}{c_{\ols}\feestar}  - 4}{\tols^2} + \frac{2}{\tnstar^2} + \OOO \left( \frac{1}{t_n^3} \right) \right)
%     > 1
% \end{align}
% We claim that there exists $\olambda$ large enough such that this inequality holds (e.g. $\ulambda > 4$).

Hence, as in \eqref{eq:eta_bound_first_reduction}, we can bound $\eta^2$ as follows:
\begin{align} \label{eq:eta_bound_second_reduction}
    \eta^2 
    \leq
    \lonebound^2 \frac{ \norm { \gamma ( \alphauls ) }_2^2 }{ \norm { \gamma ( \alphauls ) }_1^2 } 
    \leq
    \frac{ n \fstar }{ \tnstar^2 } \frac{2}{\uls}\left( 1 + \OOO \left( \frac{1}{\tuls^2} \right) \right) 
    \leq
    % \frac{c_{\eta,2}}{\log (d/n) } \left( 1 + \OOO \left( \frac{1}{ \log (d/n) } \right) \right) 
    \frac{2\fstar}{\feestar \lambda_{\uls} \log (d/n) } \left( 1 + \OOO \left( \frac{1}{ \log (d/n) } \right) \right) 
    =:
    B_{\eta,2}^2
\end{align}
% and similarly we get:
% \begin{align}
%     \eta^2 
%     \geq
%     B^2 \frac{ \norm { \gamma ( \alphaols ) }_2^2 }{ \norm { \gamma ( \alphaols ) }_1^2 } 
%     \geq
%     \left( \frac{ \overline{B}_{\eta,2} }{ \sqrt{\log (d/n)} } \right)^2
% \end{align}

\paragraph{Upper bound on $\deltanu$.}
Following the proof of Lemma \ref{lemma_first_reduction} we determine tighter upper bound for $\nu^2$. First we define
\begin{align}
    \Gamma_2^{\nu} = \left\{ (\nu, b, \alpha) 
    \subjto
    \frac{1}{n}\innerprod{b\gamma(\alpha)}{H}^2 \geq \fstar - \constconc + \tconstnu \deltanu^2 
    \andtxts
    b\alpha \leq \lonebound 
    \andtxts
    b\norm{ \gamma(\alpha) }_2 \leq B_{\eta,2}  \right\}
\end{align}

% \begin{align}
%     \Gamma_2^{\nu} = \left\{ (\wone,\wtwo) 
%     \subjto
%     \frac{ \innerprod{\wtwo}{H}^2 }{ n } \geq \fstar - \constconc + \tconstnu \norm{\wone}_2^2 \andtxts \norm{ \wtwo }_1 \leq \lonebound \andtxts \norm{ \wtwo }_2 \leq \frac{B_{\eta,2}}{\sqrt{ \log (d/n) }}  \right\}
% \end{align}
% \begin{align}
%     \Gamma_2^{\nu} = \left\{ (\wone,\wtwo) 
%     \subjto
%     \frac{ \innerprod{\wtwo}{H}^2 }{ n } \geq \fstar - \constconc + \tconstnu \nu^2 \andtxts \norm{ \wtwo }_1 \leq \lonebound \andtxts \norm{ \wtwo }_2 \leq \frac{B_{\eta,2}}{\sqrt{ \log (d/n) }}  \right\}
% \end{align}

Analogously to equation \eqref{s_condition_nu_first_reduction} we derive new condition for $\uls$ with new bound $B_{\eta,2}$ 
% \begin{align}
%     \frac{ \norm{ \gamma ( \alphauls ) }_2 }{ \alphauls } > \frac{ B_{\eta,2} }{ \lonebound }
% \end{align}
which is again satisfied for some $\uls = \lambda_{\uls} n$ with $ \lambda_{\uls} > 0 $. Hence from \eqref{nu_bound_first_reduction} we obtain bound:
\begin{align}
    \deltanu^2 
    &\leq
    \frac{ \lonebound^2 }{ n \tconstnu } \frac{ \norm{H}_{\infty}^2 }{ \alphauls^2 } - \frac{\fstar - \constconc }{\tconstnu}
    \leq 
    \frac{ \fstar }{ \tconstnu } \left( 1 + \frac{2}{\tnstar^2}  \right) - \frac{\fstar}{\tconstnu} + \OOO \left( \frac{1}{\tnstar^3} \right)\\
    & = \frac{\fstar}{\tconstnu \log(d/n)}\left( 1 + \OOO \left( \frac{1}{\sqrt{\log(d/n)}} \right) \right)
    =: 
    B_{\deltanu,2}^2 
\end{align}
which concludes the proof.
































\subsection{Proof of Proposition \ref{prop:BoundOmegal1}}


% \begin{lemma}
%     There exist universal constant $B_{\nu,3} > 0, B_{\eta,3} > 0$ such that for any element $(\wone,\wtwo)$ of $\Gamma_0$ we have that $\deltanu^2 \leq \frac{B_{\nu,3}^2}{ \left( \log \left( d/n \right) \right)^{3/2} }$ and $ \eta^2 \leq \frac{B_{\eta,3}^2}{ \log \left( d/n \right) }$ with probability at least $ 1 - $ over the draws of $..$.
% \end{lemma}

% \begin{proof}
In this part of the proof we use Taylor series approximation of function $f$ with higher order terms bounded by results from Lemma \ref{lemma_second_reduction}. Similarly as in equation \eqref{eq:second_iteration_relaxed_constraint_f} we obtain the following relaxation of constraint defining $\Gamma_0$:
\begin{align}
    \label{eq:f_taylor_approx}
    \frac{1}{n} b^2 \norm{H}_{\infty}^2 
    \geq 
    % f ( \nu, \eta ) =
    \fstar + \frac{1}{2}\feestar b^2 \norm{\gamma(\alpha)}_2^2 + \frac{1}{2}\fnnstar \deltanu^2 - \constconc - \OOOc
    % \underbrace{\OOO \left( \frac{1}{ \log (d/n)^{3/2} } \right)}_{\OOOc}
\end{align}
% \end{proof}

\paragraph{Upper and lower bound on $\eta$.}
Now we proceed in the same manner as in the previous two steps. We further relax constraint from definition of $\Gamma_0$ and define the following set:
\begin{align}
    \Gamma_3^{\eta} = \left\{ (\nu, b, \alpha) 
    \subjto 
    \frac{ 1 }{ n } b^2 \norm{H}_{\infty}^2 \geq \fstar +  \frac{1}{2}\feestar  b^2 \norm{\gamma(\alpha)}_2^2  -\constconc - \OOOc
    \andtxts
    b\alpha \leq \lonebound
    \right\}
\end{align}

% \begin{align}
%     \Gamma_3^{\eta} = \left\{ (\wone,\wtwo) \subjto \frac{ \innerprod{\wtwo}{H}^2 }{ n } \geq \fstar - \constconc - \OOOc + \frac{1}{2}\feestar \eta^2  \andtxts \norm{ \wtwo }_1 \leq \lonebound  \right\}
% \end{align}
Let $\uls$ and $\ols$ be given as in Lemma \ref{lemma_uls_ols_exp}.
\begin{align}
\label{eq:third_iteration_eta_condition}
    \left( \fstar - \constconc - \OOOc \right) \frac{ \alpha_s^2 }{ \norm{H}_{\infty}^2 } \frac{ n }{ \lonebound^2 } 
    +
    \frac{1}{2} \feestar n \frac{ \norm{ \gamma (\alpha_s) }_2^2 }{ \norm{H}_{\infty}^2 } 
    > 1
\end{align}
for $s = \uls \leq \nstar $ and $ s = \ols \geq \nstar $.

Let $ \constconc + \OOOc = \OOO \left( \frac{1}{\tnstar^3} \right)$. Then following similar arguments as in proof of Claim 7 in \cite{wang2021tight} we obtain:
% \begin{align} (this is the last version of this equation)
%     \left( \fstar -\constconc - \OOOc \right) \frac{ \alphauls^2 }{ \norm{H}_{\infty}^2 } \frac{ n }{ \lonebound^2 } 
%     \geq 
%     1 - \frac{2}{\tnstar^2} - \frac{\lambda}{\tnstar^{5/2}} + \OOO \left( \frac{1}{\tnstar^3} \right) + \OOO \left( \frac{1}{\tnstar^5} \right) + \OOO \left( \frac{1}{\tnstar^2 \nstar} \right)
% \end{align}
% 
% \begin{align}
%     \left( \fstar -\constconc - \OOOc \right) \frac{ \alphauls^2 }{ \norm{H}_{\infty}^2 } \frac{ n }{ \lonebound^2 } \geq &
%     \fstar \left( 1 + \OOO \left( \frac{1}{\tnstar^3} \right) \right) \frac{1}{\tuls^2}\left( 1 - \frac{4}{\tuls^2} + \OOO \left( \frac{1}{\tuls^4} \right) \right)\frac{n \tnstar^2}{n\fstar} \left( 1 + \frac{2}{\tnstar^2} + \OOO \left( \frac{1}{\tnstar^3} \right) \right)
%     \\
%     \geq &
%     \left( 1 - \frac{\lambda}{\tnstar^2\sqrt{\tnstar}} + \OOO \left( \frac{1}{\tnstar^2 \nstar} \right) + \OOO \left( \frac{\lambda^2}{\tnstar^5} \right) \right) \left( 1 - \frac{2}{\tnstar^2} + \OOO \left( \frac{1}{\tnstar^3} \right) \right)
% \end{align}
% 
% \begin{align} (this is the last version of this equation)
%     \frac{1}{2} \feestar n \frac{ \norm{ \gamma (\alphauls) }_2^2 }{ \norm{H}_{\infty}^2 } 
%     \geq 
%     \frac{2}{\tnstar^2} + \frac{\lambda}{(\tnstar)^{5/2}} + \frac{\lambda^2}{2\tnstar^3} + \OOO \left( \frac{1}{\tnstar^{7/2}} \right) 
% \end{align}
% 
% \begin{align}
%     \frac{1}{2} \feestar n \frac{ \norm{ \gamma (\alphauls) }_2^2 }{ \norm{H}_{\infty}^2 } 
%     \geq &
%     \nstar \frac{2}{\uls \tuls^2} \left( 1 + \OOO \left( \frac{1}{\tuls^2} \right) \right)\\
%     \geq &
%     \frac{2}{\tnstar^2} \exp \left( \frac{\lambda}{2\sqrt{\tnstar}} \right)  \left( 1 + \OOO \left( \frac{1}{\tnstar^2} \right) \right) \\
%     \geq &
%     \frac{2}{\tnstar^2} \left( 1 + \frac{\lambda}{2\sqrt{\tnstar}} + \frac{\lambda^2}{4\tnstar} + \OOO \left( \frac{\lambda^3}{\tnstar\sqrt{\tnstar}} \right) \right) \left( 1 + \OOO \left( \frac{1}{\tnstar^2} \right) \right) 
% \end{align}
% 
% Hence we have:
\begin{align}
    \left( \fstar - \constconc - \OOOc \right) \frac{ \alphauls^2 }{ \norm{H}_{\infty}^2 } \frac{ n }{ \lonebound^2 } + \frac{1}{2} \feestar n \frac{ \norm{ \gamma (\alphauls) }_2^2 }{ \norm{H}_{\infty}^2 } 
    >
    1 + \frac{\lambda^2}{2\tnstar^3} + \OOO \left( \frac{1}{\tnstar^3} \right) + \OOO \left( \frac{1}{\tnstar^{7/2}} \right) + \OOO \left( \frac{1}{\tnstar^2 \nstar} \right)
\end{align}
By choosing $\lambda$ sufficiently large the inequality \eqref{eq:third_iteration_eta_condition} is satisfied. Hence we can bound $\eta^2$ as follows:
\begin{align} \label{eq:eta_bound_third_reduction}
    \eta^2 
    \leq
    \lonebound^2 \frac{ \norm { \gamma ( \alphauls ) }_2^2 }{ \norm { \gamma ( \alphauls ) }_1^2 } 
    & \leq
    \frac{ n \fstar }{ \tnstar^2 } \frac{2}{\uls}\left( 1 + \OOO\left( \frac{1}{\tnstar^2} \right) \right)
    \leq
    % \frac{4\fstar}{\feestar} \frac{1}{\tnstar^2}  \exp \left( \frac{\lambda}{2\sqrt{\tnstar}} \right) \left( 1 + \OOO\left( \frac{1}{\tnstar^2} \right) \right) \\
    % & \leq
    \frac{4\fstar}{\feestar} \frac{1}{\tnstar^2} \left( 1 + \frac{\lambda}{2\sqrt{\tnstar}} + \OOO \left( \frac{1}{\tnstar} \right) \right) =: B_{\eta,3}^2
\end{align}
and similarly we get:
\begin{align}
    \eta^2 
    \geq
    \lonebound^2 \frac{ \norm { \gamma ( \alphaols ) }_2^2 }{ \norm { \gamma ( \alphaols ) }_1^2 } 
    \geq
    \frac{4\fstar}{\feestar} \frac{1}{\tnstar^2} \left( 1 - \frac{\lambda}{2\sqrt{\tnstar}} + \OOO \left( \frac{1}{\tnstar} \right) \right) 
\end{align}



\paragraph{Upper bound on $\deltanu$.}
Now let
% \begin{align}
%     \Gamma_3^{\nu} = \left\{ (\nu, b, \alpha) 
%     \subjto
%     \frac{1}{n}\innerprod{b\gamma(\alpha)}{H}^2 \geq \fstar + \frac{1}{2}\feestar \eta^2 + \frac{1}{2}\fnnstar \deltanu^2 - \OOO \left( \frac{1}{\tnstar^3} \right)
%     \andtxts 
%     b\alpha \leq \lonebound 
%     \andtxts
%     b\norm{ \gamma(\alpha) }_2 \leq \frac{B_{\eta,3}}{\log (d/n) }  \right\}
% \end{align}
\begin{equation}
    \Gamma_3^{\nu} = \Bigg\{ (\nu, b, \alpha) 
    \subjto \begin{cases}
                \frac{1}{n}\innerprod{b\gamma(\alpha)}{H}^2 \geq \fstar - \constconc - \OOOc + \frac{1}{2}\feestar b\norm{\gamma(\alpha)}_2^2 + \frac{1}{2}\fnnstar \deltanu^2
                \\
                b\alpha \leq \lonebound
                \\
                b\norm{ \gamma(\alpha) }_2 \leq B_{\eta,3}
            \end{cases}
             \Bigg\}
\end{equation}
% \begin{align}
%     \Gamma_3^{\nu} = \left\{ (\wone,\wtwo) 
%     \subjto
%     \frac{ \innerprod{\wtwo}{H}^2 }{ n } \geq \fstar - \constconc - \OOOc + \frac{1}{2}\feestar \eta^2 + \frac{1}{2}\fnnstar \deltanu^2
%     \andtxts 
%     \norm{ \wtwo }_1 \leq \lonebound 
%     \andtxts
%     \norm{ \wtwo }_2 \leq B_{\eta,3}  \right\}
% \end{align}

% \begin{align}
% \label{s_condition_nu_third_reduction}
%     \frac{ \norm{ \gamma ( \alphauls ) }_2 }{ \alphauls } > \frac{B_{\eta,3}}{\lonebound}
% \end{align}
Analogously to equation \eqref{s_condition_nu_first_reduction} we derive new condition for $\uls$ with new bound $B_{\eta,3}$. Using concentration result from Proposition \ref{lemma_gamma_conc} and expression \eqref{phidn_bound} we get condition:
% \begin{align}
%     \frac{2}{\uls} \left( 1 + \OOO\left( \frac{1}{\tuls^2} \right) \right) 
%     >
%     \frac{4\fstar}{\feestar} \frac{1}{\tnstar^2} \left( 1 + \frac{\lambda}{2\sqrt{\tnstar}} + \OOO \left( \frac{1}{\tnstar} \right) \right) \frac{\tnstar^2}{ n \fstar } \left( 1 + \frac{2}{\tnstar^2} + \OOO \left( \frac{1}{\tnstar^3} \right) \right)
% \end{align}
% then
\begin{align}
    \frac{2}{\uls} \left( 1 + \OOO \left( \frac{1}{\tuls^2} \right) \right) > \frac{4}{\feestar} \frac{1}{n} \left( 1 + \frac{\lambda}{2\sqrt{\tnstar}} + \OOO \left( \frac{1}{\tnstar} \right) \right)
\end{align}
Hence let $\uls = \nstar \exp \left( -\frac{\lambda}{2\sqrt{\tnstar}} \right)$. %\frac{n\feestar}{2} \left( 1 - \frac{\lambda}{\sqrt{\tnstar}} + \OOO \left( \frac{1}{\tnstar} \right) \right)$.  
\begin{align}
    \deltanu^2 
    \leq
    \frac{ 2\lonebound^2 }{ n \fnnstar } \frac{ \norm{H}_{\infty}^2 }{ \alphauls^2 } - \frac{2}{\fnnstar} \left( \fstar - \constconc - \OOOc \right) - \frac{\feestar}{\fnnstar} \frac{ \norm{ \gamma(\alphaols) }_2^2 }{ \alphaols^2 } \lonebound^2
    \leq
    \frac{4 \fstar \lambda}{\fnnstar \tnstar^{5/2}} \left( 1 + \OOO \left( \frac{1}{\sqrt{\tnstar}} \right) \right) =: B_{\deltanu,3}^2
\end{align}
% \begin{align}
%     \deltanu^2 
%     &\leq
%     \frac{ 2\lonebound^2 }{ n \fnnstar } \frac{ \norm{H}_{\infty}^2 }{ \alphauls^2 } - \frac{2\fstar}{\fnnstar} \left( 1 - \constconc - \OOOc \right) - \frac{\feestar}{\fnnstar} \frac{ \norm{ \gamma(\alphaols) }_2^2 }{ \alphaols^2 } \lonebound^2\\
%     &\leq 
%     \frac{2}{n\fnnstar} \frac{n\fstar}{\tnstar^2} \left(1-\frac{2}{\tnstar^2}+\OOO \left( \frac{1}{\tnstar^3} \right) \right) \tuls^2 \left( 1 + \frac{4}{\tuls^2} + \OOO \left( \frac{1}{\tuls^4} \right) \right)
%     - \frac{2\fstar}{\fnnstar} \left( 1 + \OOO \left( \frac{1}{\tnstar^3} \right) \right)
%     \\
%      & - \frac{\feestar}{\fnnstar} \frac{2}{\nstar} \exp \left( -\frac{\lambda}{2\sqrt{\tnstar}} \right) \left( 1 + \OOO \left( \frac{1}{\tnstar^2} \right) \right) \frac{n\fstar}{\tnstar^2}  \left( 1 - \frac{2}{\tnstar^2} + \OOO \left( \frac{1}{\tnstar^3} \right) \right)
%      \\
%      &\leq \frac{2\fstar}{\fnnstar} \left( 1 + \frac{2}{\tnstar^2} + \frac{\lambda}{\tnstar^{5/2}} + \OOO \left( \frac{1}{\tnstar^3} \right) \right) 
%      - \frac{2\fstar}{\fnnstar} \left( 1 + \OOO \left( \frac{1}{\tnstar^3} \right) \right)
%      -\frac{2\fstar}{\fnnstar}\left( \frac{2}{\tnstar^2} - \frac{\lambda}{\tnstar^{5/2}} + \OOO \left( \frac{1}{\tnstar^3} \right) \right)
%      \\
%      & \leq \frac{4 \fstar \lambda}{\fnnstar}\frac{1}{\tnstar^{5/2}} \left( 1 + \OOO \left( \frac{1}{\sqrt{\tnstar}} \right) \right) =: B_{\deltanu,3}^2
% \end{align}








==> sections_proof/L_gamma_conc.tex <==

% \onecolumn

% \begin{lemma}
% (Concentration of norms of $\gamma(\alpha_s)$, proposition 4 in \cite{konst}) Let $\ts$ be given by $2\Phic(\ts) = s/d$. There exists universal positive constants $c,c_s,c_l,c_u>0$ such that for any $s,d$ with $s\geq c_s$ and $c_ls\leq d\leq \exp(c_u s^{1/5})$ we have that:
%     \begin{align}
%         \abs{
%             \frac{\norm{\gamma(\alphathr{s})}_1}{\norm{\Hgaussian}_\infty} - \left(\frac{1}{\ts} - \frac{2}{\ts^3}\right)
%         }
%         &\leq \frac{c}{\ts^5}
%         \qquad \andtxt \qquad
%         \abs{
%             \frac{\norm{\gamma(\alphathr{s})}_2^2}{\norm{\Hgaussian}_\infty^2} - \frac{2}{s \ts^2}
%         }
%         \leq \frac{c}{s \ts^4}, \label{eq:concentration}
%     \end{align}
% with probability at least $1-6\exp\left(-\frac{s}{\log(d/s)^5}\right)$ over the draws of $h$.
% \label{lemma_gamma_conc}
% \end{lemma}




==> sections_proof/low_noise_reg.tex <==
\section{Bounds for low noise regimes}
\label{apx:lownoise}

\red{this is nonsense so far, do we need this? Maybe not...}


\begin{proposition}
\label{prop:noiseless}
\red{ put in the appendix}
Under the same assumptions on $n,d$ and $p$ as in Theorem~\ref{thm:regressionlpmain} and for any $\sigma^2 \lesssim \frac{d^2}{n^{q}}$ the risk is upper and lower bounded by. 
\begin{align}
\Risk(\what) = O\left(\frac{d^2}{n^{q}}\right) ~~\mathrm{and}~~ \Risk(\what) = \Omega\left(\frac{d^2}{qn^{q}}\right)
    % \Risk\left( \what \right) &\leq \nu_0^2(1+ O\left(\frac{1}{\log(d)}\right
    % + O\left(\nu_0\sqrt{\frac{ \mutild \sigmaxi^2 n}{\dmoment{q}^2}} + \frac{ \mutild \sigmaxi^2 n}{\dmoment{q}^2}\right) = O\left(\frac{\sigmaxi^2 n  \exp(cq)}{d}\lor \frac{d^{2p-2}}{n^p}\right)\\
    % \Risk\left( \what \right) &\geq  \nu_0^2(1+ O\left(\frac{1}{\log(d)}\right) 
    % + O\left(\nu_0\sqrt{\frac{ \mutild \sigmaxi^2 n}{\dmoment{q}^2}} + \frac{ \mutild \sigmaxi^2 n}{\dmoment{q}^2}\right) \lor \Omega(\frac{\sigmaxi^2 n}{d}) = \Omega\left(\frac{\sigmaxi^2 n}{d}\lor \frac{d^{2p-2}}{n^p} - c_4\frac{\sigmaxi n 
    % \exp(cq)}{d}\right)
    % \nu_0^2(1+ O\left(\frac{1}{\log(d)}\right) 
    % + O\left(\nu_0\sqrt{\frac{ \mutild \sigmaxi^2 n}{\dmoment{q}^2}} + \frac{ \mutild \sigmaxi^2 n}{\dmoment{q}^2}\right)
    % \vor c_3 \frac{n}{d} = \Omega(...)
\end{align}
with probability at least $ 1 - c_1 d^{c_2}$ over the draws of $X$ and $\xi$.
\end{proposition}




\subsection{Proof of Proposition~\ref{prop:lownoise}} 
The proof for the low noise regime follows essentially the same structure as the proof for the high noise regime. We use exactly the same notation as in Appendix~\ref{apx:subsec:highnoise} except for $\nu_0 = -\frac{\sigmaxi^q}{\bnull^q}$. 
\subsubsection{Step 1: Localization step - bounding $\phidn$.}
In a first step, we again upper bound $\phidn$:
% The proof of the lemma is deferred to and follows straight forwardly from a similar argument as used in \cite{koehler2021uniform} \red{cite correctly}.  The goal of this section is to show the upper bound on $\phidn:$
\begin{proposition}
\label{prop:phidnlowreg}
Under the same conditions as in Theorem~\ref{thm:regressionlp} with $\sigma \lesssim \frac{\sigma^p}{\bnull^p}$, we have that with probability $\geq 1- c_1 d^{c_2}$ over the draws of $\Ggaussian,\Hgaussian,\Xs,\xi$ that
\begin{align}
\phidn  \leq \vert \nu_0 \vert  \left(1+ O\left(\frac{1}{\log(d)}\right) 
 \right)
% \frac{\mutild  n}{\dmoment{q}^2}\right)(1+O\left(\frac{1}{\log(d)}\right)) + O\left(\rho \sqrt{\frac{ \nu_0^2}{\sigmaxi^2} + 
% \frac{\mutild  n}{\dmoment{q}^2}}\right) \right) \\
+ 1 + p\nu_0\left(1+ O(\log(d)^{-1}\right) =: \lonebound,
\end{align}
\end{proposition}
\begin{proof}
Following exactly the same argument as in the high noise regime,  
%  To upper bound the solution of a minimization problem, we only need to find one suitable point. We choose $\wtwo$ to be the Sub-gradient of $H$, i.e. $\wtwo = b \wgrad = b \partial \|H\|_p$ and choose $b$ appropriately as described below. Furthermore, we recall that $\wone$ is just a one dimensional scalar. We abbreviate $\wone= \nu$ and $\norm{\wtwo}_2 = \eta$. Further, we denote with $\nugt = \wgt_1 \in \RR^d$ to be the only non-zero entry. 
% In order to have a feasible point satisfying the constraints in the definition of $\phidn$,
we require that
\begin{align}\frac{1}{n} 
b^2 &\geq \frac{ \sigmaxi^2 +  \nu^2(1+O( \rho)) + O(\sigmaxi\rho)(\vert \nu\vert+b\|\wgrad\|_2) }{\norm{H}_q^2/n - \norm{\wgrad}_2^2 (1+O(\rho)) }. \label{eq:lpboundphinb} 
\end{align}
% \begin{align}\frac{1}{n} \innerprod{\wtwo}{\Ggaussian}^2 \geq \fn(\|\wone\|_2,\|\wtwo\|_2) \\ \impliedby
% b^2 \norm{H}_q^2/n \geq  \sigmaxi^4 + \rho \sigmaxi^2 \vert b \norm{\wgrad}_2 \vert +\rho b \norm{\wgrad}_2 \vert \nu\vert + \rho \sigmaxi^2 \vert \nu \vert + (1+\rho) (\nu^2 + b^2 \norm{\wgrad}_2^2) \\
% \impliedby
% b^2 \geq \frac{1}{\norm{H}_q^2/n - (1+\rho)\norm{\wgrad}_2^2 } \left(  \sigmaxi^4 + \rho \sigmaxi^2 \vert b \norm{\wgrad}_2 \vert + \rho \sigmaxi^2 \vert \nu \vert +  (1+\rho) \nu^2  \right)\\
% \end{align}
While in the high-noise regime $\sigmaxi^2$ was the dominant term in the expression for $b$, in the low noise regime the term involving $\nu^2$ is dominant. In particular, we now argue  why the choice  $\nu_0 = -\frac{  \sigmaxi^q}{\bnull^q} = O\left(\frac{1}{\log(d)}\right)$ (using the assumption on $\sigma$ in Theorem~\ref{thm:regressionlp} and that $\sigmaxi \to \sigma$) with $\bnull^2 = \frac{n \sigmaxi^2}{\dmoment{q}^2}$  is approximately optimal for $\nu$:
% By Lemma~\ref{lm:fnlpconcentration} we have that $\norm{H}_q$ concentrates around $\dmoment{q}$. Let $\bnull^2 = \frac{n \sigmaxi^2}{\dmoment{q}^2}$, 
we have $\frac{ \nu^2}{\sigmaxi^2} = \Omega(\log(d))$ and thus
\begin{equation}
 \norm{\wone+\wgt}_p^p + \norm{\wtwo}_p^p \approx (\nugt + \nu)^p + \bnull^{p} \frac{\nu^p}{\sigmaxi^p} \approx 
(1+ p\nu) + \bnull^{p} \frac{ \nu^p}{\sigmaxi^p}.
\end{equation}
Hence, as desired, we find an approximate optimal solution when choosing $\nu = \nu_0$. Further, we can again  verify that 
\begin{equation}
b^2 = \bnull^2 \frac{ \nu_0^2}{\sigmaxi^2}\left(1+ O\left(\frac{1}{\log(d)}\right) 
 \right)
\end{equation}
satisfies Equation~\eqref{eq:lpboundphinb} when applying Lemma~\ref{lm:dualnormconc}. Hence, we can conclude the proof.
% which is essentially a direct consequence of Lemma~\ref{lm:dualnormconc} and the following Lemma: 
% \begin{lemma}
% \begin{equation}
% \label{eq:lpboundrho}
%   O(\sigmaxi \rho) = \left(\nu_0+\sqrt{\frac{\mutild  n}{\dmoment{q}^2}}\right)  O\left(\frac{1}{\log(d)}\right).
% \end{equation}
% \end{lemma}
% The proof is deferred to section bla. 
%Thus, applying Lemma~\ref{lm:fnlpconcentration} the claim follows straight forwardly. 
% In particular, by Lemma~\ref{lm:fnlpconcentration} it is straight forward to check that the choice
% $$ b^2 = \bnull^2 \left(1+\right(\frac{ \nu_0^2}{\sigmaxi^4} + 
% \frac{\mutild  n}{\dmoment{q}^2}\left)(1+O\left(\frac{1}{\log(d)}\right))\right)$$
% satisfies Equation~\eqref{eq:lpboundphinb} \red{here we make use of the assumptions on n,d}. 
% Hence, in summary we obtain the upper bound:
% \begin{align}
% \phidn \leq b^p &+ (\nugt + \nu)^p \leq \bnull^p\left(1+ \frac{p}{2} \right(\frac{\nu_0^2}{\sigmaxi^2} + 
% \frac{\mutild  n}{\dmoment{q}^2}\left)(1+O\left(\frac{1}{\log(d)}\right)) + O\left(\rho \sqrt{\frac{ \nu_0^2}{\sigmaxi^2} + 
% \frac{\mutild  n}{\dmoment{q}^2}}\right) \right) \\
% &+ \nugt + p\nugt\nu_0(1+ O\left(\frac{1}{\log(d)}\right) =: \lonebound,
% \end{align}
% where we used that $\frac{\nu_0^2}{\sigmaxi^2} = O\left(\frac{1}{\log(d)}\right)$ and $\frac{\mutild  n}{\dmoment{q}^2}=O\left(\frac{1}{\log(d)}\right)$ which follows from Lemma~\ref{lm:dualnormconc} and the assumption on $\sigma$ and $d,n$.


% \paragraph{Case 2: $\frac{\log(d)}{\log\log(d)} \lesssim q \lesssim \log(d)$}
% In this case, another term appears which is responsible for the fitting of the noise. 

\end{proof}



\subsubsection{Step 2: Uniform convergence step}
The goal of the second step is again to bound the set $\Gamma_b$ from which the proof then follows. 
% For brevity of notation define $\nu := \wone$, $\eta := \norm{\wtwo}_2$ and $\nugt := 
% \wgt_1$. 
% In a first step, we use that by the definition of the sub-gradient norm, we have that $\langle w, \Hgaussian \rangle \leq \|\Hgaussian\|_q \|w\|_p$. Thus, we can relax the optimization problems: define $\Omega_b = \{ (\nu, \eta)\vert  \frac{1}{n} \norm{H}_q^2 b^2  \geq  f_n(\nu, \eta) ~~\mathrm{and}~~ (\nu+\nugt)^p + b^p \leq M \}$ and define $\numin := \min_{b\geq0, \nu} \nu \in \Omega_b, \numax := \max_{b\geq0, \nu} \nu \in \Omega_b$ and $\etamax := \max_{b\geq 0,\eta\geq 0} \eta \in \Omega_b$, we have:
% \begin{align}
%     \tag{$A_+$} \label{eq:phip}
%         \phidp \leq  \max_{\eta\geq 0 ,b\geq 0, \nu} \frac{\nu }{\sqrt{\nu^2+\eta^2}} 
%         \subjto \begin{cases}
%             \frac{1}{n} \norm{H}_q^2 b^2 \geq  \fn(\nu,\eta)\\
%           \vert \nu \vert^p+b^p \leq M
%         \end{cases}\\
%     \tag{$A_-$} \label{eq:phim}
%         \phidm \geq \min_{\eta\geq 0 ,b\geq 0, \nu} \frac{\nu }{\sqrt{\nu^2+\eta^2}} 
%         \subjto \begin{cases}
%     \frac{1}{n} \norm{H}_q^2 b^2 \geq  \fn(\nu,\eta)\\                     \vert \nu \vert+b^p \leq M
%         \end{cases}
%     \end{align}
% \begin{align}
%   \label{eq:phiplpv1}
%         \phidp \leq  \max_{\eta\geq 0 ,b\geq 0, \nu} \nu^2 +\eta^2
%         \subjto (\nu,\eta) \in \Omega_b \leq \numax^2 + \etamax^2
%     \\
%  \label{eq:phimlpv1}
%         \phidm \geq \min_{\eta\geq 0 ,b\geq 0, \nu} \nu^2 +\eta^2
%                 \subjto (\nu,\eta) \in \Omega_b \geq \numin^2
%     \end{align}
% The goal of this section is to proof the following proposition, from which the result then straight forwardly follows as described in Appendix bla. 
\begin{proposition}
\label{prop:highnoiselpreg}
Under the same conditions as in Theorem~\ref{thm:regressionlp} and for the choice $B$ as in Proposition~\ref{prop:phidnhighreg}, we have that with probability $\geq 1- c_1 d^{c_2}$ over the draws of $\Ggaussian,\Hgaussian,\Xs,\xi$ that for all $b\geq 0$ and any $\nu,\eta \in \Gamma_b$:


\end{proposition}

%  As a consequence of Proposition~\ref{prop:highnoiselpreg}  upper respectively lower bound Equation~\eqref{eq:phiplpv1},\eqref{eq:phimlpv1} by:
% \begin{align}
%         \phidp \leq   \frac{\sgn(\numax) }{\sqrt{1+\frac{\etamax^2}{\numax^2}}} 
%     ~~\mathrm{and}~~ \phidm \geq  \frac{\sgn(\numin) }{\sqrt{1+\frac{\etamax^2}{\numin^2}}} 
%     \end{align}





\begin{proof}
% Before being able to exploit the Lemma 1, we first need to show that $\nu, \eta = O\left(\frac{1}{\log(d)}\right)$. This follows from iterative naively bounding $\nu, \eta$ based on the relaxation $\|\wtwo\|_p^p \leq B$, which implies that $\frac{1}{n} \norm{H}_q^2 B^{2/p}  \geq  f_n(\nu, \eta) $.
The proof is again divided into two steps:

% \paragraph{Step 1, naive bound 1.} By Lemma \ref{lemma_quadratic_plus_fstar_bound} we have that $f_n(\nu, \eta) \geq c_1 \nu^2 + c_2 \eta^2$. Thus, we obtain the first naive upper bound
% \begin{equation}
%     \frac{B^{2/p}\|\Hgaussian\|_q^2}{n} \geq  c_1 \nu^2 + c_2 \eta^2
% \end{equation}
% In particular, applying Lemma concentration, we obtain that with high probability $\geq 1- c_1 d^{-c_2}$, 
% \begin{align}
% \label{eq:bound1lpeq}
%         \nu^2 + \eta^2 = O(\sigmaxi^2) 
% \end{align}

\paragraph{Step 1, naive bound 1.} 


% Following the same argument as in \cite{wang2021tight} Lemma bla, we have uniformly over $\nu, \eta$,  with probability $\geq 1-c_1d^{c_2}$ over the draws of $\Ggaussian,\xi,\Xs$ that
% \begin{equation}
%     \fn(\nu,\eta) \geq (1-O(\rho))(\sigma^2 + \nu^2 + \eta^2). 
% \end{equation}

% Hence, conditioning on the event where Equation~\eqref{eq:bound1lpeq} holds for some universal constant, we can apply Lemma concentration 2, which allows us to upper bound:
% \begin{equation}
%     \frac{B^{2/p}\|\Hgaussian\|_q^2}{n} \geq  \left(\sigma^2 +   \nu^2 +  \eta^2\right)(1+O(\rho))
% \end{equation}

In a first step, we again use the lower bound for $\fn$ from Equation \eqref{eq:regressionfn2}. In particular, note that $\lonebound = O(1)$ and thus, we have that 
\begin{equation}
\label{eq:bound2lpeqlownoise}
   \nu^2 +  \eta^2 = O\left(\frac{\norm{H}_q^2}{n}\right) = O\left(\frac{1}{\log(d)}\right).
\end{equation}




\paragraph{Step 2, tight bound for $\nu$ and upper bound for $\eta$.}
% Conditioning on the event where Equation~\eqref{eq:bound2lpeq} holds and thus $\Omega \subset \{(\nu,\eta) \vert \vert \nu - \nugt\vert \leq O\left(\frac{1}{\log(d)}\right)  ~~\mathrm{and}~~ \eta \leq O\left(\frac{1}{\log(d)}\right)\}$, we can 

Conditioning on Equation~\eqref{eq:bound2lpeqlownoise} we have
\begin{align}
   0 &\leq  b^p \leq \lonebound - (\nugt + \nu)^p =  \bnull^p \frac{\nu_0^p}{\sigmaxi^p}  \left(1+ O\left(\frac{1}{\log(d)}\right) 
 \right)
% \frac{\mutild  n}{\dmoment{q}^2}\right)(1+O\left(\frac{1}{\log(d)}\right)) + O\left(\rho \sqrt{\frac{ \nu_0^2}{\sigmaxi^2} + 
% \frac{\mutild  n}{\dmoment{q}^2}}\right) \right) \\
+ \nugt + p\nu_0\left(1+ O(\log(d)^{-1})\right) - \nugt - p  \nu (1+ O(\log(d)^{-1}) \\
&= \frac{\sigmaxi^q}{\bnull^q} (1 - p) (1+ O(\log(d)^{-1})
% \frac{\mutild  n}{\dmoment{q}^2}\right)(1+O\left(\frac{1}{\log(d)}\right)) + O\left(\rho \sqrt{\frac{ \nu_0^2}{\sigmaxi^2} + 
% \frac{\mutild  n}{\dmoment{q}^2}}\right) \right) \\
- \nugt - p  \nu (1+ O(\log(d)^{-1}) \\
\end{align}
As a result, we immediately obtain the lower bound for \begin{equation}
    \vert \nu\vert \geq \frac{p-1}{p} \frac{\nugt}{\bnull^q} ( 1+  O(\log(d)^{-1}))
\end{equation}
We now argue that this gives us the correct rate for $\nu$ up to a factor of $q$, i.e. we show $ \vert \nu\vert  = O(\frac{\sigmaxi^q}{\bnull^q})$. Thus, we can assume that $\nu = \frac{\sigmaxi^q}{\bnull^q} \nutild +  \frac{1-p}{p} \frac{ \sigmaxi^q}{\bnull^q} ( 1+  O(\log(d)^{-1}))$ with $\nutild \leq -\nugt$. We have $b^p \leq \frac{ \sigmaxi^{q}}{\bnull^q} p \vert \nutild\vert (1+O\left(\frac{1}{\log(d)}\right))$. Further, following the same argument as used for Equation~\eqref{eq:lpreghighnoisestep1}, we obtain the condition:
\begin{align}
    &\frac{b^2\|\Hgaussian\|_q^2}{n} \geq  \left(\sigma^2 +   \nu^2 +  \eta^2\right)(1+O(\rho))\\
\implies &\frac{\sigmaxi^{2q/p}}{\bnull^{2q/p}} p^{2/p} \vert \nutild \vert ^{2/p} \frac{\sigmaxi^2}{\bnull^2} (1+ O\left(\frac{1}{\log(d)}\right)) \geq \left(\sigma^2 +   \nu^2 +  \eta^2\right)(1+O(\rho))
\end{align}
We now make twice use of this equation. First to upper bound $\vert \nu\vert$ and then to upper bound $\eta^2$. 
For the upper bound on $\nu^2$, we can further relax to:
\begin{align}
&\frac{ \sigmaxi^{2q/p}}{\bnull^{2q/p}} p^{2/p} \vert \nutild \vert ^{2/p} \frac{\sigmaxi^2}{\bnull^2} (1+ O\left(\frac{1}{\log(d)}\right)) \geq   \nu^2 +  \eta^2(1+O(\rho))\\
\implies & \frac{ \sigmaxi^{2q}}{\bnull^{2q}} p^{2/p} \vert \nutild \vert ^{2/p} (1+ O\left(\frac{1}{\log(d)}\right))  \geq   \vert \nu \vert^2  \geq \nutild^2 \frac{\sigmaxi^{2q}}{\bnull^{2q}}\\
\implies &  p^{2/p} (1+ O\left(\frac{1}{\log(d)}\right))  \geq   \vert \nutild \vert^{2/q} \implies \vert \nutild \vert = O(1),
\end{align}
as desired. Finally, following the same argument for $\eta$, we obtain $\eta^2 = O(\frac{ \sigmaxi^{2q/p}}{\bnull^{2q/p}})$
and thus we can conclude the proof. 






% In a second step, we apply again Lemma~\ref{eq:regressionfn}, which allows us to relax the first constraints in $\Omega$ to 
% \begin{align}
% \label{eq:lptightcond1}
%      \frac{1}{n} \norm{H}_q^2 b^2 \geq   \fn(\wone,\|\wtwo\|_2) &\geq  \sigmaxi^2 + \nu^2  + \eta^2  +(\nu^2 + \eta^2) O\left(\frac{1}{\log(d)}\right) +  O( \rho(\nu + \eta)) 
%      \end{align}


% % Using the fact that with high probability $\eta^2 + \nu^2 \leq c \sigmax^2$, we can lower bound (using $\delta = c\sqrt{\frac
% % {\log(d)}{n}}$):
% % \begin{equation}
% %     \frac{1}{n} \fn \geq \sigmaxi^4 + ( v - \sigmaxi^2 \delta)^2 + (\nu - \sigmaxi^2 \delta)^2 - 2 \sigmaxi^4 \delta^2 
% % \end{equation}
% % Thus, we obtain the conditions:
% % \begin{align}
% % \frac{1}{n} \innerprod{\wtwo}{\Ggaussian}^2 \geq  \sigmaxi^4 + ( v - \sigmaxi^2 \delta)^2 + (\nu - \sigmaxi^2 \delta)^2 - 2 \sigmaxi^4 \delta^2 \\
% % (\nu+\nugt)^p + \norm{\wtwo}_p^p \leq \lonebound
% % \end{align}
% Furthermore, the second constraint in $\Omega$ states that $b^p \leq \lonebound - (\nu+\nugt)^p$ with $\lonebound$ from Proposition \ref{prop:phipnboundreglp}. Thus, by definition, we have:
% \begin{align}
% \label{eq:lptightcond2}
%     b^p \leq \lonebound - (\nu+\nugt)^p &= \bnull^p\left(1+ \frac{p}{2} \right(\frac{\nu_0^2}{\sigmaxi^2} + 
% \frac{\mutild  n}{\dmoment{q}^2}\left)(1+O\left(\frac{1}{\log(d)}\right))\right) + p\nugt\left(\nu_0-\nu\right)(1+ O\left(\frac{1}{\log(d)}\right),
% \end{align}
% where we have used that $\nu = O\left(\frac{1}{\log(d)}\right)$ since we condition on Equation~\eqref{eq:bound2lpeq}. Further, using the Taylorseries approximation for $(1+x)^{2/p} = 1 + \frac{2}{p} x + O(x^2)$, we get
% \begin{align}
%     \frac{1}{n} \norm{H}_q^2 b^2 &\leq   \frac{1}{n} \norm{H}_q^2 \bnull^2\left(1+ \left(\frac{\nu_0^2}{\sigmaxi^2} + 
% \frac{\mutild  n}{\dmoment{q}^2}\right)(1+O\left(\frac{1}{\log(d)}\right)) \right. \\ &+ \left.  O\left(\rho \sqrt{\frac{ \nu_0^2}{\sigmaxi^2} + 
% \frac{\mutild  n}{\dmoment{q}^2}}\right)  + \frac{2\nugt}{\bnull^p}\left(\nu_0-\nu\right)(1+ O\left(\frac{1}{\log(d)}\right)\right) \\
% &=
% \sigmaxi^2 \left(1+ \left(\frac{\nu_0^2}{\sigmaxi^2} + 
% \frac{\mutild  n}{\dmoment{q}^2}\right)(1+O\left(\frac{1}{\log(d)}\right)) +  O\left(\rho \sqrt{\frac{ \nu_0^2}{\sigmaxi^2} + 
% \frac{\mutild  n}{\dmoment{q}^2}}\right)  - \frac{2\nu_0 \left(\nu_0-\nu\right)}{\sigmaxi^2}(1+ O\left(\frac{1}{\log(d)}\right)\right)   \\
% &=\sigmaxi^2 + \left(\nu_0^2+
% \frac{\mutild \sigmaxi^2 n}{\dmoment{q}^2} - 2\nu_0 \left(\nu_0-\nu\right) \right)(1+O\left(\frac{1}{\log(d)}\right)) +  O\left(\sigmaxi^2\rho \sqrt{\frac{ \nu_0^2}{\sigmaxi^2} + 
% \frac{\mutild  n}{\dmoment{q}^2}}\right) \\
% &= \sigmaxi^2 + \left( 
% \frac{\mutild \sigmaxi^2 n}{\dmoment{q}^2} + 2\nu_0 \nu - \nu_0^2  \right)(1+O\left(\frac{1}{\log(d)}\right)) +  O\left(\sigmaxi^2\rho \sqrt{\frac{ \nu_0^2}{\sigmaxi^2} + 
% \frac{\mutild  n}{\dmoment{q}^2}}\right) 
% \label{eq:lpboundonb}
% \end{align}

% where we used Lemma concentration in the second line, in the third line that $\frac{\bnull \dmoment{q}^2}{n} = \sigmaxi^2$ and that $\nu_0  = -\frac{ \nugt \sigmaxi^2}{\bnull^p}$ by definition. Plugging the inequality from Equation~\eqref{eq:lpboundonb} in  Equation~\eqref{eq:lptightcond1}, we obtain:
% \begin{align}
% \label{eq:lptightcond1}
%      &\sigmaxi^2 + \left( 
% \frac{\mutild \sigmaxi^2 n}{\dmoment{q}^2} + 2\nu_0 \nu - \nu_0^2  \right)(1+O\left(\frac{1}{\log(d)}\right)) + O\left(\sigmaxi^2 \rho \sqrt{\frac{ \nu_0^2}{\sigmaxi^2} + 
% \frac{\mutild  n}{\dmoment{q}^2}}\right) 
% \\
% &\geq   \sigmaxi^2 + \nu^2  + \eta^2  +(\nu^2 + \eta^2) O(\rho) +  O( \sigmaxi\rho(\nu + \eta)) \\
% \implies &\left( 
% \frac{\mutild \sigmaxi^2 n}{\dmoment{q}^2} + 2\nu_0 \nu - \nu_0^2  \right)(1+O\left(\frac{1}{\log(d)}\right))
% + O\left(\sigmaxi^2 \rho \sqrt{\frac{ \nu_0^2}{\sigmaxi^2} + 
% \frac{\mutild  n}{\dmoment{q}^2}}\right) 
% \geq  \left(\nu^2  + \eta^2 \right) (1+ O(\rho)) +  O(\sigmaxi \rho(\nu + \eta))\\
% \implies &\left( 
% \frac{\mutild \sigmaxi^2 n}{\dmoment{q}^2} - \nu_0^2  \right)(1+O\left(\frac{1}{\log(d)}\right)) + O\left( \sigmaxi^2 \rho \sqrt{\frac{ \nu_0^2}{\sigmaxi^2} + 
% \frac{\mutild  n}{\dmoment{q}^2}}\right) 
% \geq  \left( \nu- \nu_0- c\rho\sigmaxi\right)^2 - \left( \eta- c\rho\sigmaxi\right)^2  - \nu_0^2 -2\sigmaxi^2c^2\rho^2 - 2 \nu_0 c\sigmaxi \rho \\
% \implies & 
% \frac{\mutild \sigmaxi^2 n}{\dmoment{q}^2}(1+O\left(\frac{1}{\log(d)}\right)) + O( \nu_0^2\log(d)^{-1}) + O\left( \sigmaxi^2 \rho \sqrt{\frac{ \nu_0^2}{\sigmaxi^2} + 
% \frac{\mutild  n}{\dmoment{q}^2}}\right) 
% \geq  \left( \nu- \nu_0- c\sigmaxi\rho\right)^2 + \left( \eta- c\sigmaxi\rho\right)^2  
% \end{align}
% where we have used in the second line Equation~\eqref{eq:lpboundrho} and let $c>0$ in the third line be a universal constant. 

% Hence, we obtain the desired bounds and thus can conclude the proof. 


% \begin{align}
%     ( \nu - \nu_0)^2 &\leq \frac{ \mutild \sigmaxi^2 n}{\dmoment{q}^2}(1+O\left(\frac{1}{\log(d)}\right)) + O( \nu_0^2\log(d)^{-1}) + O\left( \sigmaxi^2 \rho \sqrt{\frac{ \nu_0^2}{\sigmaxi^2} + 
% \frac{\mutild  n}{\dmoment{q}^2}}\right) 
%     \\
%     ~\mathrm{and}~\eta^2 &\leq \frac{ \mutild \sigmaxi^2 n}{\dmoment{q}^2}(1+O\left(\frac{1}{\log(d)}\right)) + O( \nu_0^2\log(d)^{-1}) + O\left( \sigmaxi^2 \rho \sqrt{\frac{ \nu_0^2}{\sigmaxi^2} + 
% \frac{\mutild  n}{\dmoment{q}^2}}\right) 
% \end{align}

% \paragraph{Step 3, tight bound for $\eta$.}







% And therefore
% \begin{align}
%     T^{2/p}\|\Ggaussian\|_q^2 &\leq b^2\left(1+ 2\nugt \frac{\nu - \nu_0}{b^p} +O(\nugt^{p-2}\frac{\nu_0^2+\nu^2}{b^p})\right)\|\Ggaussian\|_q^2 \\
%     &\leq \bnull^2 \left(1+\right(\frac{\nu_0^2}{\sigmaxi^4} + 
% \frac{\mutild  n}{\dmoment{q}^2}\left)(1+O\left(\frac{1}{\log(d)}\right)) \right)\left(1+ 2\nugt \frac{\nu - \nu_0}{b^p} +O(\nugt^{p-2}\frac{\nu_0^2+\nu^2}{b^p})\right)\|\Ggaussian\|_q^2\\
% &\leq \bnull^2 \left(1+\left( \frac{\nu_0^2}{\sigmaxi^4} + 
% \frac{\mutild  n}{\dmoment{q}^2} \right)(1+O\left(\frac{1}{\log(d)}\right)) +  2\nugt \frac{\nu - \nu_0}{b^p} +O(\nugt^{p-2}\frac{\nu_0^2+\nu^2}{b^p})\right)\|\Ggaussian\|_q^2\\
% &\leq \bnull^2\dmoment{q}^2 \left(1+\left( \frac{\nu_0^2}{\sigmaxi^4} + 
% \frac{\mutild  n}{\dmoment{q}^2} \right)(1+O\left(\frac{1}{\log(d)}\right)) +  2\nugt \frac{\nu - \nu_0}{b^p} +O(\nugt^{p-2}\frac{\nu_0^2+\nu^2}{b^p})\right)\\
% \end{align}
% Next, using the fact that by definition $\bnull = \frac{n \sigmaxi^4}{\dmoment{q}^2}$, and plugin in the upper bound for $T^{2/q} \|\Ggaussian\|_q$, we have the upper bound
% \begin{align}
% &\bnull^2\dmoment{q}^2 \left(1+\left( \frac{\nu_0^2}{\sigmaxi^4} + 
% \frac{\mutild  n}{\dmoment{q}^2} \right)(1+O\left(\frac{1}{\log(d)}\right)) +  2\nugt \frac{\nu - \nu_0}{b^p} +O(\nugt^{p-2}\frac{\nu_0^2+\nu^2}{b^p})\right) \\ \geq& 
% \sigmaxi^4 + ( v - \sigmaxi^2 \delta)^2 + (\nu - \sigmaxi^2 \delta)^2 - 2 \sigmaxi^4 \delta^2
% \\
% \impliedby &\sigmaxi^4\left(\left( \frac{\nu_0^2}{\sigmaxi^4} + 
% \frac{\mutild  n}{\dmoment{q}^2} \right)(1+O\left(\frac{1}{\log(d)}\right)) +  2\nugt \frac{\nu - \nu_0}{b^p} +O(\nugt^{p-2}\frac{\nu_0^2+\nu^2}{b^p})\right) \\ \geq& 
% ( v - \sigmaxi^2 \delta)^2 + (\nu - \sigmaxi^2 \delta)^2 - 2 \sigmaxi^4 \delta^2 \\
% \impliedby &\nu_0^2 O\left(\frac{1}{\log(d)}\right) + \sigmaxi^4\left(  
% \frac{\mutild  n}{\dmoment{q}^2} \right)(1+O\left(\frac{1}{\log(d)}\right)) +   2 \sigmaxi^4 \delta^2 \\ \geq& 
% ( v - \sigmaxi^2 \delta)^2 + (\nu - \sigmaxi^2 \delta)^2 -  \nu \nu_0  +O(\nu_0^3+\nu^2\nu_0) +   2 \sigmaxi^4 \delta^2 \\
% \impliedby &\nu_0^2 (-1+O\left(\frac{1}{\log(d)}\right)) + \sigmaxi^4\left(  
% \frac{\mutild  n}{\dmoment{q}^2} \right)(1+O\left(\frac{1}{\log(d)}\right))  \geq
% ( \eta - \sigmaxi^2 \delta)^2 + (\nu - \sigmaxi^2 \delta)^2 -  \nu \nu_0  +O(\nu^2\nu_0)
% \\
% \impliedby \tilde{T} := &\nu_0^2 (O\left(\frac{1}{\log(d)}\right)) + \sigmaxi^4\left(  
% \frac{\mutild  n}{\dmoment{q}^2} \right)(1+O\left(\frac{1}{\log(d)}\right))  +   2 \sigmaxi^4 \delta^2 
% + 2 \sigmaxi^2 \delta \nu_0 \geq
% ( \eta - \sigmaxi^2 \delta)^2 + (\nu - \sigmaxi^2 \delta-\nu_0)^2 
% \end{align}

% Therefore, we get that 
% \begin{align}
%     \eta \leq \sigmaxi^2 \delta + \sqrt{\tilde{T}} \implies \eta^2 \lesssim \tilde{T} \\
%   \vert \nu \vert \leq \nu_0 + \sigmaxi^2 \delta + \sqrt{\tilde{T}} \implies   \nu^2 \lesssim \nu_0^2 + \tilde{T}
% \end{align}
% \red{we use here that $\nu_0 \gtrsim \sigmaxi^2 \delta$.}
%  Furthermore, we have
% \begin{align}
%     \nu_0 + \sigmaxi^2 \delta - \sqrt{\tilde{T}}  \leq \vert \nu \vert \implies \nu^2 \gtrsim ...
% \end{align}


\end{proof}



